Elucidation of Conformational Hysteresis on a Giant DNA

The conformational behavior of a giant DNA mediated by condensing agents in the bulk solution has been investigated through experimental and theoretical approaches. Experimentally, a pronounced conformational hysteresis is observed for folding and unfolding processes, by increasing and decreasing the concentration of condensing agent PEG (Polyethylene glycol), respectively. To elucidate the observed hysteresis, a semiflexible chain model is studied by using Monte Carlo simulations for the coil-globule transition. In the simulations, the hysteresis loop emerges for stiff enough chains, indicating distinct pathways for folding and unfolding processes. Also, our results show that globular state is thermodynamically more stable than coiled state in the hysteresis loop. Our findings suggest that increasing chain stiffness may reduce the chain conformations relevant to the folding pathway, which impedes the folding process.

==> figure_jcp_ps <==
%-12345X@PJL JOB NAME="figures_jcp.pdf"
@PJL SET STRINGCODESET=UTF8
@PJL COMMENT "HP Universal Printing PS (60.51.342.0); Microsoft Windows XP 5.1.2600.1; PScript 0.3.1296.1"
@PJL COMMENT "Username: Chwen-Yang Shew; App Filename: figures_jcp.pdf; 5-4-2007"
@PJL SET JOBATTR="JobAcct1=Chwen-Yang Shew"
@PJL SET JOBATTR="JobAcct2=SHEW"
@PJL SET JOBATTR="JobAcct3=SHEW"
@PJL SET JOBATTR="JobAcct4=20070504132048"
@PJL SET JOBATTR="JobAcct5=389ed0ac-aa79-4963-981b-6c377de933ab"
@PJL DMINFO ASCIIHEX="0400040101020D101001153230303730353034313732303438"
@PJL SET RESOLUTION=600
@PJL ENTER LANGUAGE=POSTSCRIPT
%!PS-Adobe-3.0
%%Title: figures_jcp.pdf
%%Creator: PScript5.dll Version 5.2.2
%%CreationDate: 5/4/2007 13:20:48
%%For: Chwen-Yang Shew
%%BoundingBox: (atend)
%%Pages: (atend)
%%Orientation: Portrait
%%PageOrder: Special
%%DocumentNeededResources: (atend)
%%DocumentSuppliedResources: (atend)
%%DocumentData: Clean7Bit
%%TargetDevice: (HP Universal Printing PS) (3010.107) 0
%%LanguageLevel: 2
%%EndComments

%%BeginDefaults
%%PageBoundingBox: 12 13 598 780
%%ViewingOrientation: 1 0 0 1
%%EndDefaults


%%BeginProlog
%%BeginResource: file Pscript_WinNT_ErrorHandler 5.0 0
/currentpacking where{pop/oldpack currentpacking def/setpacking where{pop false
setpacking}if}if/$brkpage 64 dict def $brkpage begin/prnt{dup type/stringtype
ne{=string cvs}if dup length 6 mul/tx exch def/ty 10 def currentpoint/toy exch
def/tox exch def 1 setgray newpath tox toy 2 sub moveto 0 ty rlineto tx 0
rlineto 0 ty neg rlineto closepath fill tox toy moveto 0 setgray show}bind def
/nl{currentpoint exch pop lmargin exch moveto 0 -10 rmoveto}def/=={/cp 0 def
typeprint nl}def/typeprint{dup type exec}readonly def/lmargin 72 def/rmargin 72
def/tprint{dup length cp add rmargin gt{nl/cp 0 def}if dup length cp add/cp
exch def prnt}readonly def/cvsprint{=string cvs tprint( )tprint}readonly def
/integertype{cvsprint}readonly def/realtype{cvsprint}readonly def/booleantype
{cvsprint}readonly def/operatortype{(--)tprint =string cvs tprint(-- )tprint}
readonly def/marktype{pop(-mark- )tprint}readonly def/dicttype{pop
(-dictionary- )tprint}readonly def/nulltype{pop(-null- )tprint}readonly def
/filetype{pop(-filestream- )tprint}readonly def/savetype{pop(-savelevel- )
tprint}readonly def/fonttype{pop(-fontid- )tprint}readonly def/nametype{dup
xcheck not{(/)tprint}if cvsprint}readonly def/stringtype{dup rcheck{(\()tprint
tprint(\))tprint}{pop(-string- )tprint}ifelse}readonly def/arraytype{dup rcheck
{dup xcheck{({)tprint{typeprint}forall(})tprint}{([)tprint{typeprint}forall(])
tprint}ifelse}{pop(-array- )tprint}ifelse}readonly def/packedarraytype{dup
rcheck{dup xcheck{({)tprint{typeprint}forall(})tprint}{([)tprint{typeprint}
forall(])tprint}ifelse}{pop(-packedarray- )tprint}ifelse}readonly def/courier
/Courier findfont 10 scalefont def end errordict/handleerror{systemdict begin
$error begin $brkpage begin newerror{/newerror false store vmstatus pop pop 0
ne{grestoreall}if errorname(VMerror)ne{showpage}if initgraphics courier setfont
lmargin 720 moveto errorname(VMerror)eq{userdict/ehsave known{clear userdict
/ehsave get restore 2 vmreclaim}if vmstatus exch pop exch pop PrtVMMsg}{
(ERROR: )prnt errorname prnt nl(OFFENDING COMMAND: )prnt/command load prnt
$error/ostack known{nl nl(STACK:)prnt nl nl $error/ostack get aload length{==}
repeat}if}ifelse systemdict/showpage get exec(%%[ Error: )print errorname
=print(; OffendingCommand: )print/command load =print( ]%%)= flush}if end end
end}dup 0 systemdict put dup 4 $brkpage put bind readonly put/currentpacking
where{pop/setpacking where{pop oldpack setpacking}if}if
%%EndResource
userdict /Pscript_WinNT_Min 100 dict dup begin put
%%BeginResource: file Pscript_WinNT_Min 5.0 0
/b{bind def}bind def/|{def}b/LH/showpage load def/min_initialize{begin userdict
begin}b/min_terminate{pop end end}b/Pscript_Win_Data where{pop}{userdict
/Pscript_Win_Data currentdict put}ifelse/setjn{{statusdict/jobname known
{statusdict/jobname 3 -1 roll put}if}stopped cleartomark}b/colspRefresh{}b
%%EndResource
%%BeginResource: file Pscript_Win_Basic 5.0 0
/d/def load def/,/load load d/~/exch , d/?/ifelse , d/!/pop , d/`/begin , d/^
/index , d/@/dup , d/+/translate , d/$/roll , d/U/userdict , d/M/moveto , d/-
/rlineto , d/&/currentdict , d/:/gsave , d/;/grestore , d/F/false , d/T/true ,
d/N/newpath , d/E/end , d/Ac/arc , d/An/arcn , d/A/ashow , d/D/awidthshow , d/C
/closepath , d/V/div , d/O/eofill , d/L/fill , d/I/lineto , d/-c/curveto , d/-M
/rmoveto , d/+S/scale , d/Ji/setfont , d/Lc/setlinecap , d/Lj/setlinejoin , d
/Lw/setlinewidth , d/Lm/setmiterlimit , d/sd/setdash , d/S/show , d/LH/showpage
, d/K/stroke , d/W/widthshow , d/R/rotate , d/L2? false/languagelevel where{pop
languagelevel 2 ge{pop true}if}if d L2?{/xS/xshow , d/yS/yshow , d/zS/xyshow ,
d}if/b{bind d}bind d/bd{bind d}bind d/xd{~ d}bd/ld{, d}bd/bn/bind ld/lw/Lw ld
/lc/Lc ld/lj/Lj ld/sg/setgray ld/ADO_mxRot null d/self & d/OrgMx matrix
currentmatrix d/reinitialize{: OrgMx setmatrix[/TextInit/GraphInit/UtilsInit
counttomark{@ where{self eq}{F}?{cvx exec}{!}?}repeat cleartomark ;}b
/initialize{`{/Pscript_Win_Data where{!}{U/Pscript_Win_Data & put}?/ADO_mxRot ~
d/TextInitialised? F d reinitialize E}{U/Pscript_Win_Data 230 dict @ ` put
/ADO_mxRot ~ d/TextInitialised? F d reinitialize}?}b/terminate{!{& self eq
{exit}{E}?}loop E}b/suspend/terminate , d/resume{` Pscript_Win_Data `}b U `
/lucas 21690 d/featurebegin{countdictstack lucas[}b/featurecleanup{stopped
{cleartomark @ lucas eq{! exit}if}loop countdictstack ~ sub @ 0 gt{{E}repeat}
{!}?}b E/snap{transform 0.25 sub round 0.25 add ~ 0.25 sub round 0.25 add ~
itransform}b/dsnap{dtransform round ~ round ~ idtransform}b/nonzero_round{@ 0.5
ge{round}{@ -0.5 lt{round}{0 ge{1}{-1}?}?}?}b/nonzero_dsnap{dtransform
nonzero_round ~ nonzero_round ~ idtransform}b U<04>cvn{}put/rr{1 ^ 0 - 0 ~ -
neg 0 - C}b/irp{4 -2 $ + +S fx 4 2 $ M 1 ^ 0 - 0 ~ - neg 0 -}b/rp{4 2 $ M 1 ^ 0
- 0 ~ - neg 0 -}b/solid{[]0 sd}b/g{@ not{U/DefIf_save save put}if U/DefIf_bool
2 ^ put}b/DefIf_El{if U/DefIf_bool get not @{U/DefIf_save get restore}if}b/e
{DefIf_El !}b/UDF{L2?{undefinefont}{!}?}b/UDR{L2?{undefineresource}{! !}?}b
/freeVM{/Courier findfont[40 0 0 -40 0 0]makefont Ji 2 vmreclaim}b/hfRedefFont
{findfont @ length dict `{1 ^/FID ne{d}{! !}?}forall & E @ ` ~{/CharStrings 1
dict `/.notdef 0 d & E d}if/Encoding 256 array 0 1 255{1 ^ ~/.notdef put}for d
E definefont !}bind d/hfMkCIDFont{/CIDFont findresource @ length 2 add dict `{1
^ @/FID eq ~ @/XUID eq ~/UIDBase eq or or{! !}{d}?}forall/CDevProc ~ d/Metrics2
16 dict d/CIDFontName 1 ^ d & E 1 ^ ~/CIDFont defineresource ![~]composefont !}
bind d
%%EndResource
%%BeginResource: file Pscript_Win_Utils_L2 5.0 0
/rf/rectfill , d/fx{1 1 dtransform @ 0 ge{1 sub 0.5}{1 add -0.5}? 3 -1 $ @ 0 ge
{1 sub 0.5}{1 add -0.5}? 3 1 $ 4 1 $ idtransform 4 -2 $ idtransform}b/BZ{4 -2 $
snap + +S fx rf}b/rs/rectstroke , d/rc/rectclip , d/UtilsInit{currentglobal{F
setglobal}if}b/scol{! setcolor}b/colspA/DeviceGray d/colspABC/DeviceRGB d
/colspRefresh{colspABC setcolorspace}b/SetColSpace{colspABC setcolorspace}b
/resourcestatus where{!/ColorRendering/ProcSet resourcestatus{! ! T}{F}?}{F}?
not{/ColorRendering<</GetHalftoneName{currenthalftone @/HalftoneName known{
/HalftoneName get}{!/none}?}bn/GetPageDeviceName{currentpagedevice @
/PageDeviceName known{/PageDeviceName get @ null eq{!/none}if}{!/none}?}bn
/GetSubstituteCRD{!/DefaultColorRendering/ColorRendering resourcestatus{! !
/DefaultColorRendering}{(DefaultColorRendering*){cvn exit}127 string
/ColorRendering resourceforall}?}bn>>/defineresource where{!/ProcSet
defineresource !}{! !}?}if/buildcrdname{/ColorRendering/ProcSet findresource `
mark GetHalftoneName @ type @/nametype ne ~/stringtype ne and{!/none}if(.)
GetPageDeviceName @ type @/nametype ne ~/stringtype ne and{!/none}if(.)5 ^ 0 5
-1 1{^ length add}for string 6 1 $ 5 ^ 5{~ 1 ^ cvs length 1 ^ length 1 ^ sub
getinterval}repeat ! cvn 3 1 $ ! ! E}b/definecolorrendering{~ buildcrdname ~
/ColorRendering defineresource !}b/findcolorrendering where{!}{
/findcolorrendering{buildcrdname @/ColorRendering resourcestatus{! ! T}{
/ColorRendering/ProcSet findresource ` GetSubstituteCRD E F}?}b}?
/selectcolorrendering{findcolorrendering !/ColorRendering findresource
setcolorrendering}b/G2UBegin{findresource/FontInfo get/GlyphNames2Unicode get
`}bind d/G2CCBegin{findresource/FontInfo get/GlyphNames2HostCode get `}bind d
/G2UEnd{E}bind d/AddFontInfoBegin{/FontInfo 8 dict @ `}bind d/AddFontInfo{
/GlyphNames2Unicode 16 dict d/GlyphNames2HostCode 16 dict d}bind d
/AddFontInfoEnd{E d}bind d/T0AddCFFMtx2{/CIDFont findresource/Metrics2 get ` d
E}bind d
%%EndResource
end
%%BeginResource: l2check
%%Copyright: Copyright 1993 Adobe Systems Incorporated. All Rights Reserved.
systemdict /languagelevel known
{ systemdict /languagelevel get 1 eq }
{ true }
ifelse
{
initgraphics /Helvetica findfont 18 scalefont setfont
72 600 moveto (Error: Your printer driver needs to be configured) dup show
72 580 moveto (for printing to a PostScript Language Level 1 printer.) dup show
exch = =
/Helvetica-Bold findfont 16 scalefont setfont
72 520 moveto (Windows and Unix) show
/Times-Roman findfont 16 scalefont setfont
72 500 moveto (Select \252Language Level 1\272 in the PostScript options section) show
72 480 moveto (of the Acrobat print dialog.) show
/Helvetica-Bold findfont 16 scalefont setfont
72 440 moveto (Macintosh) show
/Times-Roman findfont 16 scalefont setfont
72 420 moveto (In the Chooser, select your printer driver.) show
72 400 moveto (Then select your printer and click the Setup button.) show
72 380 moveto (Follow any on-screen dialogs that may appear.) show
showpage
quit
}
if
%%EndResource
userdict /pdf_svglb currentglobal put true setglobal
%%BeginResource: procset Adobe_CoolType_Utility_MAKEOCF 1.13 0
%%Copyright: Copyright 1987-2001 Adobe Systems Incorporated.
%%Version: 1.13 0
systemdict/languagelevel known dup{currentglobal false setglobal}{false}ifelse
exch userdict/Adobe_CoolType_Utility 2 copy known{2 copy get dup maxlength 25
add dict copy}{25 dict}ifelse put Adobe_CoolType_Utility begin/ct_Level2? exch
def/ct_Clone? 1183615869 internaldict dup/CCRun known not exch/eCCRun known
not ct_Level2? and or def/ct_UseNativeCapability? systemdict/composefont known
def/ct_MakeOCF 35 dict def/ct_Vars 25 dict def/ct_GlyphDirProcs 6 dict def
/ct_BuildCharDict 15 dict dup begin/charcode 2 string def/dst_string 1500
string def/nullstring()def/usewidths? true def end def ct_Level2?{setglobal}{
pop}ifelse ct_GlyphDirProcs begin/GetGlyphDirectory{systemdict/languagelevel
known{pop/CIDFont findresource/GlyphDirectory get}{1 index/CIDFont
findresource/GlyphDirectory get dup type/dicttype eq{dup dup maxlength exch
length sub 2 index lt{dup length 2 index add dict copy 2 index/CIDFont
findresource/GlyphDirectory 2 index put}if}if exch pop exch pop}ifelse +}def/+
{systemdict/languagelevel known{currentglobal false setglobal 3 dict begin/vm
exch def}{1 dict begin}ifelse/$ exch def systemdict/languagelevel known{vm
setglobal/gvm currentglobal def $ gcheck setglobal}if ?{$ begin}if}def/?{$
type/dicttype eq}def/|{userdict/Adobe_CoolType_Data known{Adobe_CoolType_Data
/AddWidths? known{currentdict Adobe_CoolType_Data begin begin AddWidths?{
Adobe_CoolType_Data/CC 3 index put ?{def}{$ 3 1 roll put}ifelse CC charcode
exch 1 index 0 2 index 256 idiv put 1 index exch 1 exch 256 mod put
stringwidth 2 array astore currentfont/Widths get exch CC exch put}{?{def}{$ 3
1 roll put}ifelse}ifelse end end}{?{def}{$ 3 1 roll put}ifelse}ifelse}{?{def}{
$ 3 1 roll put}ifelse}ifelse}def/!{?{end}if systemdict/languagelevel known{gvm
setglobal}if end}def/:{string currentfile exch readstring pop}executeonly def
end ct_MakeOCF begin/ct_cHexEncoding[/c00/c01/c02/c03/c04/c05/c06/c07/c08/c09
/c0A/c0B/c0C/c0D/c0E/c0F/c10/c11/c12/c13/c14/c15/c16/c17/c18/c19/c1A/c1B/c1C
/c1D/c1E/c1F/c20/c21/c22/c23/c24/c25/c26/c27/c28/c29/c2A/c2B/c2C/c2D/c2E/c2F
/c30/c31/c32/c33/c34/c35/c36/c37/c38/c39/c3A/c3B/c3C/c3D/c3E/c3F/c40/c41/c42
/c43/c44/c45/c46/c47/c48/c49/c4A/c4B/c4C/c4D/c4E/c4F/c50/c51/c52/c53/c54/c55
/c56/c57/c58/c59/c5A/c5B/c5C/c5D/c5E/c5F/c60/c61/c62/c63/c64/c65/c66/c67/c68
/c69/c6A/c6B/c6C/c6D/c6E/c6F/c70/c71/c72/c73/c74/c75/c76/c77/c78/c79/c7A/c7B
/c7C/c7D/c7E/c7F/c80/c81/c82/c83/c84/c85/c86/c87/c88/c89/c8A/c8B/c8C/c8D/c8E
/c8F/c90/c91/c92/c93/c94/c95/c96/c97/c98/c99/c9A/c9B/c9C/c9D/c9E/c9F/cA0/cA1
/cA2/cA3/cA4/cA5/cA6/cA7/cA8/cA9/cAA/cAB/cAC/cAD/cAE/cAF/cB0/cB1/cB2/cB3/cB4
/cB5/cB6/cB7/cB8/cB9/cBA/cBB/cBC/cBD/cBE/cBF/cC0/cC1/cC2/cC3/cC4/cC5/cC6/cC7
/cC8/cC9/cCA/cCB/cCC/cCD/cCE/cCF/cD0/cD1/cD2/cD3/cD4/cD5/cD6/cD7/cD8/cD9/cDA
/cDB/cDC/cDD/cDE/cDF/cE0/cE1/cE2/cE3/cE4/cE5/cE6/cE7/cE8/cE9/cEA/cEB/cEC/cED
/cEE/cEF/cF0/cF1/cF2/cF3/cF4/cF5/cF6/cF7/cF8/cF9/cFA/cFB/cFC/cFD/cFE/cFF]def
/ct_CID_STR_SIZE 8000 def/ct_mkocfStr100 100 string def/ct_defaultFontMtx[.001
0 0 .001 0 0]def/ct_1000Mtx[1000 0 0 1000 0 0]def/ct_raise{exch cvx exch
errordict exch get exec stop}bind def/ct_reraise{cvx $error/errorname get
(Error: )print dup(                    )cvs print errordict exch get exec stop
}bind def/ct_cvnsi{1 index add 1 sub 1 exch 0 4 1 roll{2 index exch get exch 8
bitshift add}for exch pop}bind def/ct_GetInterval{Adobe_CoolType_Utility
/ct_BuildCharDict get begin/dst_index 0 def dup dst_string length gt{dup
string/dst_string exch def}if 1 index ct_CID_STR_SIZE idiv/arrayIndex exch def
2 index arrayIndex get 2 index arrayIndex ct_CID_STR_SIZE mul sub{dup 3 index
add 2 index length le{2 index getinterval dst_string dst_index 2 index
putinterval length dst_index add/dst_index exch def exit}{1 index length 1
index sub dup 4 1 roll getinterval dst_string dst_index 2 index putinterval
pop dup dst_index add/dst_index exch def sub/arrayIndex arrayIndex 1 add def 2
index dup length arrayIndex gt{arrayIndex get}{pop exit}ifelse 0}ifelse}loop
pop pop pop dst_string 0 dst_index getinterval end}bind def ct_Level2?{
/ct_resourcestatus currentglobal mark true setglobal{/unknowninstancename
/Category resourcestatus}stopped{cleartomark setglobal true}{cleartomark
currentglobal not exch setglobal}ifelse{{mark 3 1 roll/Category findresource
begin ct_Vars/vm currentglobal put({ResourceStatus} stopped)0()/SubFileDecode
filter cvx exec{cleartomark false}{{3 2 roll pop true}{cleartomark false}
ifelse}ifelse ct_Vars/vm get setglobal end}}{{resourcestatus}}ifelse bind def
/CIDFont/Category ct_resourcestatus{pop pop}{currentglobal true setglobal
/Generic/Category findresource dup length dict copy dup/InstanceType/dicttype
put/CIDFont exch/Category defineresource pop setglobal}ifelse
ct_UseNativeCapability?{/CIDInit/ProcSet findresource begin 12 dict begin
begincmap/CIDSystemInfo 3 dict dup begin/Registry(Adobe)def/Ordering(Identity)
def/Supplement 0 def end def/CMapName/Identity-H def/CMapVersion 1 def
/CMapType 1 def 1 begincodespacerange<0000><ffff>endcodespacerange 1
begincidrange<0000><ffff>0 endcidrange endcmap CMapName currentdict/CMap
defineresource pop end end}if}{/ct_Category 2 dict begin/CIDFont 10 dict def
/ProcSet 2 dict def currentdict end def/defineresource{ct_Category 1 index 2
copy known{get dup dup maxlength exch length eq{dup length 10 add dict copy
ct_Category 2 index 2 index put}if 3 index 3 index put pop exch pop}{pop pop
/defineresource/undefined ct_raise}ifelse}bind def/findresource{ct_Category 1
index 2 copy known{get 2 index 2 copy known{get 3 1 roll pop pop}{pop pop
/findresource/undefinedresource ct_raise}ifelse}{pop pop/findresource
/undefined ct_raise}ifelse}bind def/resourcestatus{ct_Category 1 index 2 copy
known{get 2 index known exch pop exch pop{0 -1 true}{false}ifelse}{pop pop
/findresource/undefined ct_raise}ifelse}bind def/ct_resourcestatus
/resourcestatus load def}ifelse/ct_CIDInit 2 dict begin/ct_cidfont_stream_init
{{dup(Binary)eq{pop null currentfile ct_Level2?{{cid_BYTE_COUNT()
/SubFileDecode filter}stopped{pop pop pop}if}if/readstring load exit}if dup
(Hex)eq{pop currentfile ct_Level2?{{null exch/ASCIIHexDecode filter/readstring
}stopped{pop exch pop(>)exch/readhexstring}if}{(>)exch/readhexstring}ifelse
load exit}if/StartData/typecheck ct_raise}loop cid_BYTE_COUNT ct_CID_STR_SIZE
le{2 copy cid_BYTE_COUNT string exch exec pop 1 array dup 3 -1 roll 0 exch put
}{cid_BYTE_COUNT ct_CID_STR_SIZE div ceiling cvi dup array exch 2 sub 0 exch 1
exch{2 copy 5 index ct_CID_STR_SIZE string 6 index exec pop put pop}for 2
index cid_BYTE_COUNT ct_CID_STR_SIZE mod string 3 index exec pop 1 index exch
1 index length 1 sub exch put}ifelse cid_CIDFONT exch/GlyphData exch put 2
index null eq{pop pop pop}{pop/readstring load 1 string exch{3 copy exec pop
dup length 0 eq{pop pop pop pop pop true exit}if 4 index eq{pop pop pop pop
false exit}if}loop pop}ifelse}bind def/StartData{mark{currentdict dup/FDArray
get 0 get/FontMatrix get 0 get .001 eq{dup/CDevProc known not{/CDevProc
1183615869 internaldict/stdCDevProc 2 copy known{get}{pop pop{pop pop pop pop
pop 0 -1000 7 index 2 div 880}}ifelse def}if}{/CDevProc{pop pop pop pop pop 0
1 cid_temp/cid_CIDFONT get/FDArray get 0 get/FontMatrix get 0 get div 7 index
2 div 1 index .88 mul}def}ifelse/cid_temp 15 dict def cid_temp begin
/cid_CIDFONT exch def 3 copy pop dup/cid_BYTE_COUNT exch def 0 gt{
ct_cidfont_stream_init FDArray{/Private get dup/SubrMapOffset known{begin
/Subrs SubrCount array def Subrs SubrMapOffset SubrCount SDBytes ct_Level2?{
currentdict dup/SubrMapOffset undef dup/SubrCount undef/SDBytes undef}if end
/cid_SD_BYTES exch def/cid_SUBR_COUNT exch def/cid_SUBR_MAP_OFFSET exch def
/cid_SUBRS exch def cid_SUBR_COUNT 0 gt{GlyphData cid_SUBR_MAP_OFFSET
cid_SD_BYTES ct_GetInterval 0 cid_SD_BYTES ct_cvnsi 0 1 cid_SUBR_COUNT 1 sub{
exch 1 index 1 add cid_SD_BYTES mul cid_SUBR_MAP_OFFSET add GlyphData exch
cid_SD_BYTES ct_GetInterval 0 cid_SD_BYTES ct_cvnsi cid_SUBRS 4 2 roll
GlyphData exch 4 index 1 index sub ct_GetInterval dup length string copy put}
for pop}if}{pop}ifelse}forall}if cleartomark pop pop end CIDFontName
currentdict/CIDFont defineresource pop end end}stopped{cleartomark/StartData
ct_reraise}if}bind def currentdict end def/ct_saveCIDInit{/CIDInit/ProcSet
ct_resourcestatus{true}{/CIDInitC/ProcSet ct_resourcestatus}ifelse{pop pop
/CIDInit/ProcSet findresource ct_UseNativeCapability?{pop null}{/CIDInit
ct_CIDInit/ProcSet defineresource pop}ifelse}{/CIDInit ct_CIDInit/ProcSet
defineresource pop null}ifelse ct_Vars exch/ct_oldCIDInit exch put}bind def
/ct_restoreCIDInit{ct_Vars/ct_oldCIDInit get dup null ne{/CIDInit exch/ProcSet
defineresource pop}{pop}ifelse}bind def/ct_BuildCharSetUp{1 index begin
CIDFont begin Adobe_CoolType_Utility/ct_BuildCharDict get begin/ct_dfCharCode
exch def/ct_dfDict exch def CIDFirstByte ct_dfCharCode add dup CIDCount ge{pop
0}if/cid exch def{GlyphDirectory cid 2 copy known{get}{pop pop nullstring}
ifelse dup length FDBytes sub 0 gt{dup FDBytes 0 ne{0 FDBytes ct_cvnsi}{pop 0}
ifelse/fdIndex exch def dup length FDBytes sub FDBytes exch getinterval
/charstring exch def exit}{pop cid 0 eq{/charstring nullstring def exit}if/cid
0 def}ifelse}loop}def/ct_SetCacheDevice{0 0 moveto dup stringwidth 3 -1 roll
true charpath pathbbox 0 -1000 7 index 2 div 880 setcachedevice2 0 0 moveto}
def/ct_CloneSetCacheProc{1 eq{stringwidth pop -2 div -880 0 -1000 setcharwidth
moveto}{usewidths?{currentfont/Widths get cid 2 copy known{get exch pop aload
pop}{pop pop stringwidth}ifelse}{stringwidth}ifelse setcharwidth 0 0 moveto}
ifelse}def/ct_Type3ShowCharString{ct_FDDict fdIndex 2 copy known{get}{
currentglobal 3 1 roll 1 index gcheck setglobal ct_Type1FontTemplate dup
maxlength dict copy begin FDArray fdIndex get dup/FontMatrix 2 copy known{get}
{pop pop ct_defaultFontMtx}ifelse/FontMatrix exch dup length array copy def
/Private get/Private exch def/Widths rootfont/Widths get def/CharStrings 1
dict dup/.notdef<d841272cf18f54fc13>dup length string copy put def currentdict
end/ct_Type1Font exch definefont dup 5 1 roll put setglobal}ifelse dup
/CharStrings get 1 index/Encoding get ct_dfCharCode get charstring put
rootfont/WMode 2 copy known{get}{pop pop 0}ifelse exch 1000 scalefont setfont
ct_str1 0 ct_dfCharCode put ct_str1 exch ct_dfSetCacheProc ct_SyntheticBold{
currentpoint ct_str1 show newpath moveto ct_str1 true charpath ct_StrokeWidth
setlinewidth stroke}{ct_str1 show}ifelse}def/ct_Type4ShowCharString{ct_dfDict
ct_dfCharCode charstring FDArray fdIndex get dup/FontMatrix get dup
ct_defaultFontMtx ct_matrixeq not{ct_1000Mtx matrix concatmatrix concat}{pop}
ifelse/Private get Adobe_CoolType_Utility/ct_Level2? get not{ct_dfDict/Private
3 -1 roll{put}1183615869 internaldict/superexec get exec}if 1183615869
internaldict Adobe_CoolType_Utility/ct_Level2? get{1 index}{3 index/Private
get mark 6 1 roll}ifelse dup/RunInt known{/RunInt get}{pop/CCRun}ifelse get
exec Adobe_CoolType_Utility/ct_Level2? get not{cleartomark}if}bind def
/ct_BuildCharIncremental{{Adobe_CoolType_Utility/ct_MakeOCF get begin
ct_BuildCharSetUp ct_ShowCharString}stopped{stop}if end end end end}bind def
/BaseFontNameStr(BF00)def/ct_Type1FontTemplate 14 dict begin/FontType 1 def
/FontMatrix[.001 0 0 .001 0 0]def/FontBBox[-250 -250 1250 1250]def/Encoding
ct_cHexEncoding def/PaintType 0 def currentdict end def/BaseFontTemplate 11
dict begin/FontMatrix[.001 0 0 .001 0 0]def/FontBBox[-250 -250 1250 1250]def
/Encoding ct_cHexEncoding def/BuildChar/ct_BuildCharIncremental load def
ct_Clone?{/FontType 3 def/ct_ShowCharString/ct_Type3ShowCharString load def
/ct_dfSetCacheProc/ct_CloneSetCacheProc load def/ct_SyntheticBold false def
/ct_StrokeWidth 1 def}{/FontType 4 def/Private 1 dict dup/lenIV 4 put def
/CharStrings 1 dict dup/.notdef<d841272cf18f54fc13>put def/PaintType 0 def
/ct_ShowCharString/ct_Type4ShowCharString load def}ifelse/ct_str1 1 string def
currentdict end def/BaseFontDictSize BaseFontTemplate length 5 add def
/ct_matrixeq{true 0 1 5{dup 4 index exch get exch 3 index exch get eq and dup
not{exit}if}for exch pop exch pop}bind def/ct_makeocf{15 dict begin exch/WMode
exch def exch/FontName exch def/FontType 0 def/FMapType 2 def/FontMatrix
matrix def/bfCount 1 index/CIDCount get 256 idiv 1 add dup 256 gt{pop 256}if
def/Encoding 256 array 0 1 bfCount 1 sub{2 copy dup put pop}for bfCount 1 255{
2 copy bfCount put pop}for def/FDepVector bfCount dup 256 lt{1 add}if array
def BaseFontTemplate BaseFontDictSize dict copy begin/CIDFont exch def CIDFont
/FontBBox known{CIDFont/FontBBox get/FontBBox exch def}if CIDFont/CDevProc
known{CIDFont/CDevProc get/CDevProc exch def}if currentdict end
BaseFontNameStr 3(0)putinterval 0 1 bfCount dup 256 eq{1 sub}if{FDepVector
exch 2 index BaseFontDictSize dict copy begin dup/CIDFirstByte exch 256 mul
def FontType 3 eq{/ct_FDDict 2 dict def}if currentdict end 1 index 16
BaseFontNameStr 2 2 getinterval cvrs pop BaseFontNameStr exch definefont put}
for ct_Clone?{/Widths 1 index/CIDFont get/GlyphDirectory get length dict def}
if FontName currentdict end definefont ct_Clone?{gsave dup 1000 scalefont
setfont ct_BuildCharDict begin/usewidths? false def currentfont/Widths get
begin exch/CIDFont get/GlyphDirectory get{pop dup charcode exch 1 index 0 2
index 256 idiv put 1 index exch 1 exch 256 mod put stringwidth 2 array astore
def}forall end/usewidths? true def end grestore}{exch pop}ifelse}bind def
/ct_ComposeFont{ct_UseNativeCapability?{2 index/CMap ct_resourcestatus{pop pop
exch pop}{/CIDInit/ProcSet findresource begin 12 dict begin begincmap/CMapName
3 index def/CMapVersion 1 def/CMapType 1 def exch/WMode exch def/CIDSystemInfo
3 dict dup begin/Registry(Adobe)def/Ordering CMapName ct_mkocfStr100 cvs
(Adobe-)search{pop pop(-)search{dup length string copy exch pop exch pop}{pop
(Identity)}ifelse}{pop(Identity)}ifelse def/Supplement 0 def end def 1
begincodespacerange<0000><ffff>endcodespacerange 1 begincidrange<0000><ffff>0
endcidrange endcmap CMapName currentdict/CMap defineresource pop end end}
ifelse composefont}{3 2 roll pop 0 get/CIDFont findresource ct_makeocf}ifelse}
bind def/ct_MakeIdentity{ct_UseNativeCapability?{1 index/CMap
ct_resourcestatus{pop pop}{/CIDInit/ProcSet findresource begin 12 dict begin
begincmap/CMapName 2 index def/CMapVersion 1 def/CMapType 1 def/CIDSystemInfo
3 dict dup begin/Registry(Adobe)def/Ordering CMapName ct_mkocfStr100 cvs
(Adobe-)search{pop pop(-)search{dup length string copy exch pop exch pop}{pop
(Identity)}ifelse}{pop(Identity)}ifelse def/Supplement 0 def end def 1
begincodespacerange<0000><ffff>endcodespacerange 1 begincidrange<0000><ffff>0
endcidrange endcmap CMapName currentdict/CMap defineresource pop end end}
ifelse composefont}{exch pop 0 get/CIDFont findresource ct_makeocf}ifelse}bind
def currentdict readonly pop end end
%%EndResource
%%BeginResource: file Pscript_T42Hdr PSVER
userdict/ct_T42Dict 15 dict put ct_T42Dict begin/Is2015?{version cvi 2015 ge}
bind def/AllocGlyphStorage{Is2015?{pop}{{string}forall}ifelse}bind def
/Type42DictBegin{25 dict begin/FontName exch def/CharStrings 256 dict begin
/.notdef 0 def currentdict end def/Encoding exch def/PaintType 0 def/FontType
42 def/FontMatrix[1 0 0 1 0 0]def 4 array astore cvx/FontBBox exch def/sfnts}
bind def/Type42DictEnd{currentdict dup/FontName get exch definefont pop end}
bind def/RD{string currentfile exch readstring pop}executeonly def/PrepFor2015
{Is2015?{/GlyphDirectory 16 dict def sfnts 0 get dup 2 index(glyx)putinterval
2 index(locx)putinterval pop pop}{pop pop}ifelse}bind def/AddT42Char{Is2015?{
findfont/GlyphDirectory get begin def end pop pop}{findfont/sfnts get 4 index
get 3 index 2 index putinterval pop pop pop pop}ifelse}bind def/IDStr{dup 1
add 2 mul string 0 1 3 index{1 index exch dup 2 mul exch 3 copy 256 idiv put
exch 1 add exch 256 mod put}for exch pop}bind def
%0 -8961 -256 -9472
%G00GFFEncoding /TT3782070272t0CID
%CIDT42Begin
/CIDT42Begin{25 dict begin dup/WMode exch def 0 gt{/Metrics2 16 dict def
/CDevProc{pop dup 1.9 gt 3 index neg .99 gt or{pop .85}{4 index add}ifelse}
bind def/FontMatrix[0 1 -1 0 0 0]def}{/FontMatrix[1 0 0 1 0 0]def}ifelse
/CIDMap exch def/CIDCount exch def/CIDSystemInfo 3 dict dup begin 3 -1 roll
/Supplement exch def 3 -1 roll/Ordering exch def 3 -1 roll/Registry exch def
end def/CIDFontName exch def/Encoding exch def 4 array astore cvx/FontBBox
exch def/CharStrings 2 dict dup begin/.notdef 0 def end def/GDBytes 2 def
/CIDFontType 2 def/FontType 42 def/PaintType 0 def/sfnts}bind def/CIDT42End{
CIDFontName currentdict end/CIDFont defineresource pop}bind def/T42CIDCP32K{
/CIDFont findresource dup length dict copy dup/FID undef begin/CIDFontName
exch def/CIDMap exch def/CIDCount exch def/Metrics2 8 dict def CIDFontName
currentdict end/CIDFont defineresource pop}bind def/T42CIDCPR{/CIDFont
findresource dup length dict copy dup/FID undef begin/CDevProc{pop}def
/CIDFontName exch def CIDFontName currentdict end/CIDFont defineresource pop}
bind def/T0AddT42Char{/CIDFont findresource/GlyphDirectory get begin def end
pop pop}bind def/T0AddT42Mtx2{/CIDFont findresource/Metrics2 get begin def end
}bind def end
%%EndResource
%%BeginResource: file Pscript_CFF PSVER
userdict/ct_CffDict 6 dict put ct_CffDict begin/F0Subr{systemdict/internaldict
known{1183615869 systemdict/internaldict get exec/FlxProc known{save true}{
false}ifelse}{userdict/internaldict known not{userdict/internaldict{count 0 eq
{/internaldict errordict/invalidaccess get exec}if dup type/integertype ne{
/internaldict errordict/invalidaccess get exec}if dup 1183615869 eq{pop 0}{
/internaldict errordict/invalidaccess get exec}ifelse}dup 14 get 1 25 dict put
bind executeonly put}if 1183615869 userdict/internaldict get exec/FlxProc
known{save true}{false}ifelse}ifelse[systemdict/internaldict known not{100
dict/begin cvx/mtx matrix/def cvx}if systemdict/currentpacking known{
currentpacking true setpacking}if{systemdict/internaldict known{1183615869
systemdict/internaldict get exec dup/$FlxDict known not{dup dup length exch
maxlength eq{pop userdict dup/$FlxDict known not{100 dict begin/mtx matrix def
dup/$FlxDict currentdict put end}if}{100 dict begin/mtx matrix def dup
/$FlxDict currentdict put end}ifelse}if/$FlxDict get begin}if grestore/exdef{
exch def}def/dmin exch abs 100 div def/epX exdef/epY exdef/c4y2 exdef/c4x2
exdef/c4y1 exdef/c4x1 exdef/c4y0 exdef/c4x0 exdef/c3y2 exdef/c3x2 exdef/c3y1
exdef/c3x1 exdef/c3y0 exdef/c3x0 exdef/c1y2 exdef/c1x2 exdef/c2x2 c4x2 def
/c2y2 c4y2 def/yflag c1y2 c3y2 sub abs c1x2 c3x2 sub abs gt def/PickCoords{{
c1x0 c1y0 c1x1 c1y1 c1x2 c1y2 c2x0 c2y0 c2x1 c2y1 c2x2 c2y2}{c3x0 c3y0 c3x1
c3y1 c3x2 c3y2 c4x0 c4y0 c4x1 c4y1 c4x2 c4y2}ifelse/y5 exdef/x5 exdef/y4 exdef
/x4 exdef/y3 exdef/x3 exdef/y2 exdef/x2 exdef/y1 exdef/x1 exdef/y0 exdef/x0
exdef}def mtx currentmatrix pop mtx 0 get abs 1e-05 lt mtx 3 get abs 1e-05 lt
or{/flipXY -1 def}{mtx 1 get abs 1e-05 lt mtx 2 get abs 1e-05 lt or{/flipXY 1
def}{/flipXY 0 def}ifelse}ifelse/erosion 1 def systemdict/internaldict known{
1183615869 systemdict/internaldict get exec dup/erosion known{/erosion get
/erosion exch def}{pop}ifelse}if yflag{flipXY 0 eq c3y2 c4y2 eq or{false
PickCoords}{/shrink c3y2 c4y2 eq{0}{c1y2 c4y2 sub c3y2 c4y2 sub div abs}ifelse
def/yshrink{c4y2 sub shrink mul c4y2 add}def/c1y0 c3y0 yshrink def/c1y1 c3y1
yshrink def/c2y0 c4y0 yshrink def/c2y1 c4y1 yshrink def/c1x0 c3x0 def/c1x1
c3x1 def/c2x0 c4x0 def/c2x1 c4x1 def/dY 0 c3y2 c1y2 sub round dtransform
flipXY 1 eq{exch}if pop abs def dY dmin lt PickCoords y2 c1y2 sub abs .001 gt{
c1x2 c1y2 transform flipXY 1 eq{exch}if/cx exch def/cy exch def/dY 0 y2 c1y2
sub round dtransform flipXY 1 eq{exch}if pop def dY round dup 0 ne{/dY exdef}{
pop dY 0 lt{-1}{1}ifelse/dY exdef}ifelse/erode PaintType 2 ne erosion .5 ge
and def erode{/cy cy .5 sub def}if/ey cy dY add def/ey ey ceiling ey sub ey
floor add def erode{/ey ey .5 add def}if ey cx flipXY 1 eq{exch}if itransform
exch pop y2 sub/eShift exch def/y1 y1 eShift add def/y2 y2 eShift add def/y3
y3 eShift add def}if}ifelse}{flipXY 0 eq c3x2 c4x2 eq or{false PickCoords}{
/shrink c3x2 c4x2 eq{0}{c1x2 c4x2 sub c3x2 c4x2 sub div abs}ifelse def/xshrink
{c4x2 sub shrink mul c4x2 add}def/c1x0 c3x0 xshrink def/c1x1 c3x1 xshrink def
/c2x0 c4x0 xshrink def/c2x1 c4x1 xshrink def/c1y0 c3y0 def/c1y1 c3y1 def/c2y0
c4y0 def/c2y1 c4y1 def/dX c3x2 c1x2 sub round 0 dtransform flipXY -1 eq{exch}
if pop abs def dX dmin lt PickCoords x2 c1x2 sub abs .001 gt{c1x2 c1y2
transform flipXY -1 eq{exch}if/cy exch def/cx exch def/dX x2 c1x2 sub round 0
dtransform flipXY -1 eq{exch}if pop def dX round dup 0 ne{/dX exdef}{pop dX 0
lt{-1}{1}ifelse/dX exdef}ifelse/erode PaintType 2 ne erosion .5 ge and def
erode{/cx cx .5 sub def}if/ex cx dX add def/ex ex ceiling ex sub ex floor add
def erode{/ex ex .5 add def}if ex cy flipXY -1 eq{exch}if itransform pop x2
sub/eShift exch def/x1 x1 eShift add def/x2 x2 eShift add def/x3 x3 eShift add
def}if}ifelse}ifelse x2 x5 eq y2 y5 eq or{x5 y5 lineto}{x0 y0 x1 y1 x2 y2
curveto x3 y3 x4 y4 x5 y5 curveto}ifelse epY epX}systemdict/currentpacking
known{exch setpacking}if/exec cvx/end cvx]cvx executeonly exch{pop true exch
restore}{systemdict/internaldict known not{1183615869 userdict/internaldict
get exec exch/FlxProc exch put true}{1183615869 systemdict/internaldict get
exec dup length exch maxlength eq{false}{1183615869 systemdict/internaldict
get exec exch/FlxProc exch put true}ifelse}ifelse}ifelse{systemdict
/internaldict known{1183615869 systemdict/internaldict get exec/FlxProc get
exec}{1183615869 userdict/internaldict get exec/FlxProc get exec}ifelse}if}
executeonly def/F1Subr{gsave currentpoint newpath moveto}bind def/F2Subr{
currentpoint grestore gsave currentpoint newpath moveto}bind def/HSSubr{
systemdict/internaldict known not{pop 3}{1183615869 systemdict/internaldict
get exec dup/startlock known{/startlock get exec}{dup/strtlck known{/strtlck
get exec}{pop 3}ifelse}ifelse}ifelse}bind def end
%%EndResource

userdict /pdf_svglb get setglobal
/currentpacking where{pop currentpacking true setpacking}if
%%BeginResource: procset pdfvars
%%Copyright: Copyright 1987-2001 Adobe Systems Incorporated. All Rights Reserved.
%%Version: 5.0 6
%%Title: definition of dictionary of variables used by PDF & PDFText procsets
userdict /PDF 160 dict put
userdict /PDFVars 89 dict dup begin put
/docSetupDone false def
/InitAll 0 def
/TermAll 0 def
/DocInitAll 0 def
/DocTermAll 0 def
/_pdfEncodings 2 array def
/_pdf_str1 1 string def
/_pdf_i 0 def
/_pdf_na 0 def
/_pdf_showproc 0 def
/_italMtx [1 0 .212557 1 0 0] def
/_italMtx_WMode1 [1 -.212557 0 1 0 0] def
/_italMtxType0 [1 0 .1062785 1 0 0] def
/_italMtx_WMode1Type0 [1 -.1062785 0 1 0 0] def
/_basefont 0 def
/_basefonto 0 def
/_pdf_oldCIDInit null def
/_pdf_FontDirectory 30 dict def
/_categories 10 dict def
/_sa? true def
/_ColorSep5044? false def
/nulldict 0 dict def
/_processColors 0 def
/overprintstack null def
/_defaulttransfer currenttransfer def
/_defaultflatness currentflat def
/_defaulthalftone null def
/_defaultcolortransfer null def
/_defaultblackgeneration null def
/_defaultundercolorremoval null def
/_defaultcolortransfer null def
PDF begin
[/c/cs/cm/d/d0/f/h/i/j/J/l/m/M/n/q/Q/re/ri/S/sc/sh/Tf/w/W
/applyInterpFunc/applystitchFunc/domainClip/encodeInput
/initgs/int/limit/rangeClip
/defineRes/findRes/setSA/pl
%% to keep CoolType entries in GlyphDirProcs safe from collisions with Win PS driver
/? /! /| /: /+ /GetGlyphDirectory
/pdf_flushFilters /pdf_readstring /pdf_dictOp /pdf_image /pdf_maskedImage
/pdf_shfill /pdf_sethalftone
] {null def} bind forall
end
end
%%EndResource
PDFVars begin PDF begin
%%BeginResource: procset pdfutil
%%Copyright: Copyright 1993-1999 Adobe Systems Incorporated. All Rights Reserved.
%%Version: 4.0 2
%%Title: Basic utilities used by other PDF procsets
/bd {bind def} bind def
/ld {load def} bd
/bld {
dup length dict begin
{ null def } forall
bind
end
def
} bd
/dd { PDFVars 3 1 roll put } bd
/xdd { exch dd } bd
/Level2?
systemdict /languagelevel known
{ systemdict /languagelevel get 2 ge } { false } ifelse
def
/Level1? Level2? not def
/Level3?
systemdict /languagelevel known
{systemdict /languagelevel get 3 eq } { false } ifelse
def
/getifknown {
2 copy known { get true } { pop pop false } ifelse
} bd
/here {
currentdict exch getifknown
} bd
/isdefined? { where { pop true } { false } ifelse } bd
%%EndResource
%%BeginResource: procset pdf
%%Version: 5.0 6
%%Copyright: Copyright 1998-2001 Adobe Systems Incorporated. All Rights Reserved.
%%Title: General operators for PDF, common to all Language Levels.
/cm { matrix astore concat } bd
/d /setdash ld
/f /fill ld
/h /closepath ld
/i {dup 0 eq {pop _defaultflatness} if setflat} bd
/j /setlinejoin ld
/J /setlinecap ld
/M /setmiterlimit ld
/n /newpath ld
/S /stroke ld
/w /setlinewidth ld
/W /clip ld
/initgs {
0 setgray
[] 0 d
0 j
0 J
10 M
1 w
false setSA
/_defaulttransfer load settransfer
0 i
/RelativeColorimetric ri
newpath
} bd
/int {
dup 2 index sub 3 index 5 index sub div 6 -2 roll sub mul
exch pop add exch pop
} bd
/limit {
dup 2 index le { exch } if pop
dup 2 index ge { exch } if pop
} bd
/domainClip {
Domain aload pop 3 2 roll
limit
} [/Domain] bld
/applyInterpFunc {
0 1 DimOut 1 sub
{
dup C0 exch get exch
dup C1 exch get exch
3 1 roll
1 index sub
3 index
N exp mul add
exch
currentdict /Range_lo known
{
dup Range_lo exch get exch
Range_hi exch get
3 2 roll limit
}
{
pop
}
ifelse
exch
} for
pop
} [/DimOut /C0 /C1 /N /Range_lo /Range_hi] bld
/encodeInput {
NumParts 1 sub
0 1 2 index
{
dup Bounds exch get
2 index gt
{ exit }
{ dup
3 index eq
{ exit }
{ pop } ifelse
} ifelse
} for
3 2 roll pop
dup Bounds exch get exch
dup 1 add Bounds exch get exch
2 mul
dup Encode exch get exch
1 add Encode exch get
int
} [/NumParts /Bounds /Encode] bld
/rangeClip {
exch dup Range_lo exch get
exch Range_hi exch get
3 2 roll
limit
} [/Range_lo /Range_hi] bld
/applyStitchFunc {
Functions exch get exec
currentdict /Range_lo known {
0 1 DimOut 1 sub {
DimOut 1 add -1 roll
rangeClip
} for
} if
} [/Functions /Range_lo /DimOut] bld
/pdf_flushfilters
{
aload length
{ dup status
1 index currentfile ne and
{ dup flushfile closefile }
{ pop }
ifelse
} repeat
} bd
/pdf_readstring
{
1 index dup length 1 sub get
exch readstring pop
exch pdf_flushfilters
} bind def
/pdf_dictOp
{
3 2 roll
10 dict copy
begin
_Filters dup length 1 sub get def
currentdict exch exec
_Filters pdf_flushfilters
end
} [/_Filters] bld
/pdf_image {{image} /DataSource pdf_dictOp} bd
/pdf_imagemask {{imagemask} /DataSource pdf_dictOp} bd
/pdf_shfill {{sh} /DataSource pdf_dictOp} bd
/pdf_sethalftone {{sethalftone} /Thresholds pdf_dictOp} bd
/pdf_maskedImage
{
10 dict copy begin
/miDict currentdict def
/DataDict DataDict 10 dict copy def
DataDict begin
/DataSource
_Filters dup length 1 sub get
def
miDict image
_Filters pdf_flushfilters
end
end
} [/miDict /DataDict /_Filters] bld
%%EndResource
%%BeginResource: procset pdflev2
%%Version: 5.0 14
%%Copyright: Copyright 1987-2001 Adobe Systems Incorporated. All Rights Reserved.
%%LanguageLevel: 2
%%Title: PDF operators, with code specific for Level 2
/docinitialize {
PDF begin
/_defaulthalftone currenthalftone dd
/_defaultblackgeneration currentblackgeneration dd
/_defaultundercolorremoval currentundercolorremoval dd
/_defaultcolortransfer [currentcolortransfer] dd
/_defaulttransfer currenttransfer dd
end
PDFVars /docSetupDone true put
} bd
/initialize {
PDFVars /docSetupDone get {
_defaulthalftone sethalftone
/_defaultblackgeneration load setblackgeneration
/_defaultundercolorremoval load setundercolorremoval
_defaultcolortransfer aload pop setcolortransfer
} if
false setoverprint
} bd
/terminate { } bd
/c /curveto ld
/cs /setcolorspace ld
/l /lineto ld
/m /moveto ld
/q /gsave ld
/Q /grestore ld
/sc /setcolor ld
/setSA/setstrokeadjust ld
/re {
4 2 roll m
1 index 0 rlineto
0 exch rlineto
neg 0 rlineto
h
} bd
/concattransferfuncs {
[ 3 1 roll /exec load exch /exec load ] cvx
} bd
/concatandsettransfer {
/_defaulttransfer load concattransferfuncs settransfer
} bd
/concatandsetcolortransfer {
_defaultcolortransfer aload pop
8 -1 roll 5 -1 roll concattransferfuncs 7 1 roll
6 -1 roll 4 -1 roll concattransferfuncs 5 1 roll
4 -1 roll 3 -1 roll concattransferfuncs 3 1 roll
concattransferfuncs
setcolortransfer
} bd
/defineRes/defineresource ld
/findRes/findresource ld
currentglobal
true systemdict /setglobal get exec
[/Function /ExtGState /Form /Shading /FunctionDictionary /MadePattern /PatternPrototype /DataSource /Image]
{ /Generic /Category findresource dup length dict copy /Category defineresource pop }
forall
systemdict /setglobal get exec
/ri
{
/findcolorrendering isdefined?
{
mark exch
findcolorrendering
counttomark 2 eq
{ type /booleantype eq
{ dup type /nametype eq
{ dup /ColorRendering resourcestatus
{ pop pop
dup /DefaultColorRendering ne
{
/ColorRendering findresource
setcolorrendering
} if
} if
} if
} if
} if
cleartomark
}
{ pop
} ifelse
} bd
/knownColorants? {
pop false
} bd
/getrampcolor {
/indx exch def
0 1 NumComp 1 sub {
dup
Samples exch get
dup type /stringtype eq { indx get } if
exch
Scaling exch get aload pop
3 1 roll
mul add
} for
setcolor
} bd
/GenStrips {
40 dict begin
/background exch def
/ext1 exch def
/ext0 exch def
/BBox exch def
/y2 exch def
/x2 exch def
/y1 exch def
/x1 exch def
/rampdict exch def
gsave
BBox length 0 gt {
BBox 0 get BBox 1 get
BBox 2 get BBox 0 get sub
BBox 3 get BBox 1 get sub
rectclip
} if
x1 x2 eq
{
y1 y2 lt {/theta 90 def}{/theta 270 def} ifelse
}
{
/slope y2 y1 sub x2 x1 sub div def
/theta slope 1 atan def
x2 x1 lt y2 y1 ge and { /theta theta 180 sub def} if
x2 x1 lt y2 y1 le and { /theta theta 180 add def} if
}
ifelse
gsave
clippath
x1 y1 translate
theta rotate
pathbbox
/yMax exch def
/xMax exch def
/yMin exch def
/xMin exch def
grestore
xMax xMin eq yMax yMin eq or
{
grestore
end
}
{
rampdict begin
background length 0 gt { background aload pop setcolor gsave clippath fill grestore } if
gsave
x1 y1 translate
theta rotate
/xStart 0 def
/xEnd x2 x1 sub dup mul y2 y1 sub dup mul add 0.5 exp def
/ySpan yMax yMin sub def
/numsteps NumSamples def
/rampIndxInc 1 def
/subsampling false def
xStart 0 transform
xEnd 0 transform
3 -1 roll
sub dup mul
3 1 roll
sub dup mul
add 0.5 exp 72 div
0 72 matrix defaultmatrix dtransform dup mul exch dup mul add sqrt
72 0 matrix defaultmatrix dtransform dup mul exch dup mul add sqrt
1 index 1 index lt { exch } if pop
mul
/numpix exch def
numpix 0 ne
{
NumSamples numpix div 0.5 gt
{
/numsteps numpix 2 div round cvi dup 1 le { pop 2 } if def
/rampIndxInc NumSamples 1 sub numsteps div def
/subsampling true def
} if
} if
ext0 {
0 getrampcolor
xMin xStart lt
{ xMin yMin xMin neg ySpan rectfill } if
} if
/xInc xEnd xStart sub numsteps div def
/x xStart def
0
numsteps
{
dup
subsampling { round cvi } if
getrampcolor
x yMin xInc ySpan rectfill
/x x xInc add def
rampIndxInc add
}
repeat
pop
ext1 {
xMax xEnd gt
{ xEnd yMin xMax xEnd sub ySpan rectfill } if
} if
grestore
grestore
end
end
} ifelse
} bd
/RadialShade {
40 dict begin
/background exch def
/ext1 exch def
/ext0 exch def
/BBox exch def
/r2 exch def
/c2y exch def
/c2x exch def
/r1 exch def
/c1y exch def
/c1x exch def
/rampdict exch def
gsave
BBox length 0 gt {
BBox 0 get BBox 1 get
BBox 2 get BBox 0 get sub
BBox 3 get BBox 1 get sub
rectclip
} if
gsave
clippath
pathbbox
/BByMax exch def
/BBxMax exch def
/BByMin exch def
/BBxMin exch def
grestore
BBxMax BBxMin eq BByMax BByMin eq or
{
grestore
end
}
{
rampdict begin
background length 0 gt { background aload pop setcolor gsave clippath fill grestore } if
/areaOfConcern
BBxMin BByMin BBxMax BByMax
BBxMin BByMin
BBxMax BBxMin sub 0
0 BByMax BByMin sub
BBxMin BBxMax sub 0
12 packedarray
< 0B 00 01 04 04 04 0A>
2 packedarray
def
c1x c2x sub dup mul
c1y c2y sub dup mul
add 0.5 exp
r1 add
r2 sub
abs
0 dtransform
dup mul exch dup mul add 0.5 exp 72 div
0 72 matrix defaultmatrix dtransform dup mul exch dup mul add sqrt
72 0 matrix defaultmatrix dtransform dup mul exch dup mul add sqrt
1 index 1 index lt { exch } if pop
/hires exch def
hires mul
/numpix exch def
/numsteps NumSamples def
/rampIndxInc 1 def
/subsampling false def
numpix 0 ne
{
NumSamples numpix div 0.5 gt
{
/numsteps numpix 2 div round cvi dup 1 le { pop 2 } if def
/rampIndxInc NumSamples 1 sub numsteps div def
/subsampling true def
} if
} if
/xInc c2x c1x sub numsteps div def
/yInc c2y c1y sub numsteps div def
/rInc r2 r1 sub numsteps div def
ext0 {
0 getrampcolor
r1 r2 eq c1x c2x eq and c1y c2y eq and
{
c1x c1y r1 0 360 arc fill
}
{
r1 r2 lt
{
/backsteps r1 rInc div floor def
/cx c1x xInc backsteps mul sub def
/cy c1y yInc backsteps mul sub def
/radius r1 rInc backsteps mul sub def
newpath
{
cx cy radius 0 360 arc
fill
radius r1 ge { exit} if
/radius radius rInc add def
/cx cx xInc add def
/cy cy yInc add def
} loop
}
{
/cx c1x def
/cy c1y def
/radius r1 def
newpath
{
cx cy radius 360 0 arcn
/cx cx xInc sub def
/cy cy yInc sub def
/radius radius rInc sub def
cx cy radius 0 360 arc
areaOfConcern ineofill not { exit } if
eofill
} loop
} ifelse
} ifelse
} if
/cx c1x def
/cy c1y def
/radius r1 def
newpath
xInc 0 eq yInc 0 eq rInc 0 eq and and
{
0 getrampcolor
cx cy radius 0 360 arc
stroke
NumSamples 1 sub getrampcolor
cx cy radius 72 hires div add 0 360 arc
0 setlinewidth
stroke
}
{
0
numsteps
{
dup
subsampling { round cvi } if
getrampcolor
cx cy radius 0 360 arc
/cx cx xInc add def
/cy cy yInc add def
/radius radius rInc add def
cx cy radius 360 0 arcn
eofill
rampIndxInc add
}
repeat
pop
} ifelse
ext1 {
r2 r1 le
{
r2 r1 eq c1x c2x eq and c1y c2y eq and
{
c1x c1y r1 0 360 arc
areaOfConcern uappend
eofill
}
{
{
cx cy radius 0 360 arc
areaOfConcern infill not { exit } if
fill
/radius radius rInc add def
/cx cx xInc add def
/cy cy yInc add def
} loop
} ifelse
}
{
{
cx cy radius 0 360 arc
/cx cx xInc add def
/cy cy yInc add def
/radius radius rInc add def
cx cy radius 360 0 arcn
areaOfConcern ineofill not { exit } if
eofill
} loop
} ifelse
} if
grestore
end
end
} ifelse
} bd
%%EndResource
%%BeginResource: procset pdftext
%%Version: 5.0 5
%%Copyright: Copyright 1987-2001 Adobe Systems Incorporated. All Rights Reserved.
%%Title: Text operators for PDF
PDF /PDFText 78 dict dup begin put
/docinitialize
{
/resourcestatus where {
pop
/CIDParams /ProcSet resourcestatus {
pop pop
false /CIDParams /ProcSet findresource /SetBuildCompatible get exec
} if
} if
PDF begin
PDFText /_pdfDefineIdentity-H known
{ PDFText /_pdfDefineIdentity-H get exec}
if
end
} bd
/initialize {
PDFText begin
} bd
/terminate { end } bd
Level2?
{
/_safeput
{
3 -1 roll load 3 1 roll put
}
bd
}
{
/_safeput
{
2 index load dup dup length exch maxlength ge
{ dup length 5 add dict copy
3 index xdd
}
{ pop }
ifelse
3 -1 roll load 3 1 roll put
}
bd
}
ifelse
/pdf_has_composefont? systemdict /composefont known def
/CopyFont {
{
1 index /FID ne 2 index /UniqueID ne and
{ def } { pop pop } ifelse
} forall
} bd
/Type0CopyFont
{
exch
dup length dict
begin
CopyFont
[
exch
FDepVector
{
dup /FontType get 0 eq
{
1 index Type0CopyFont
/_pdfType0 exch definefont
}
{
/_pdfBaseFont exch
2 index exec
}
ifelse
exch
}
forall
pop
]
/FDepVector exch def
currentdict
end
} bd
Level2? {currentglobal true setglobal} if
/cHexEncoding
[/c00/c01/c02/c03/c04/c05/c06/c07/c08/c09/c0A/c0B/c0C/c0D/c0E/c0F/c10/c11/c12
/c13/c14/c15/c16/c17/c18/c19/c1A/c1B/c1C/c1D/c1E/c1F/c20/c21/c22/c23/c24/c25
/c26/c27/c28/c29/c2A/c2B/c2C/c2D/c2E/c2F/c30/c31/c32/c33/c34/c35/c36/c37/c38
/c39/c3A/c3B/c3C/c3D/c3E/c3F/c40/c41/c42/c43/c44/c45/c46/c47/c48/c49/c4A/c4B
/c4C/c4D/c4E/c4F/c50/c51/c52/c53/c54/c55/c56/c57/c58/c59/c5A/c5B/c5C/c5D/c5E
/c5F/c60/c61/c62/c63/c64/c65/c66/c67/c68/c69/c6A/c6B/c6C/c6D/c6E/c6F/c70/c71
/c72/c73/c74/c75/c76/c77/c78/c79/c7A/c7B/c7C/c7D/c7E/c7F/c80/c81/c82/c83/c84
/c85/c86/c87/c88/c89/c8A/c8B/c8C/c8D/c8E/c8F/c90/c91/c92/c93/c94/c95/c96/c97
/c98/c99/c9A/c9B/c9C/c9D/c9E/c9F/cA0/cA1/cA2/cA3/cA4/cA5/cA6/cA7/cA8/cA9/cAA
/cAB/cAC/cAD/cAE/cAF/cB0/cB1/cB2/cB3/cB4/cB5/cB6/cB7/cB8/cB9/cBA/cBB/cBC/cBD
/cBE/cBF/cC0/cC1/cC2/cC3/cC4/cC5/cC6/cC7/cC8/cC9/cCA/cCB/cCC/cCD/cCE/cCF/cD0
/cD1/cD2/cD3/cD4/cD5/cD6/cD7/cD8/cD9/cDA/cDB/cDC/cDD/cDE/cDF/cE0/cE1/cE2/cE3
/cE4/cE5/cE6/cE7/cE8/cE9/cEA/cEB/cEC/cED/cEE/cEF/cF0/cF1/cF2/cF3/cF4/cF5/cF6
/cF7/cF8/cF9/cFA/cFB/cFC/cFD/cFE/cFF] def
Level2? {setglobal} if
/modEnc {
/_enc xdd
/_icode 0 dd
counttomark 1 sub -1 0
{
index
dup type /nametype eq
{
_enc _icode 3 -1 roll put
_icode 1 add
}
if
/_icode xdd
} for
cleartomark
_enc
} bd
/trEnc {
/_enc xdd
255 -1 0 {
exch dup -1 eq
{ pop /.notdef }
{ Encoding exch get }
ifelse
_enc 3 1 roll put
} for
pop
_enc
} bd
/TE {
/_i xdd
StandardEncoding 256 array copy modEnc
_pdfEncodings exch _i exch put
} bd
/TZ
{
/_usePDFEncoding xdd
findfont
dup length 6 add dict
begin
{
1 index /FID ne { def } { pop pop } ifelse
} forall
/pdf_origFontName FontName def
/FontName exch def
currentdict /PaintType known
{ PaintType 2 eq {/PaintType 0 def} if }
if
_usePDFEncoding 0 ge
{
/Encoding _pdfEncodings _usePDFEncoding get def
pop
}
{
_usePDFEncoding -1 eq
{
counttomark 0 eq
{ pop }
{
Encoding 256 array copy
modEnc /Encoding exch def
}
ifelse
}
{
256 array
trEnc /Encoding exch def
}
ifelse
}
ifelse
pdf_EuroProcSet pdf_origFontName known
{
pdf_origFontName pdf_AddEuroGlyphProc
} if
Level2?
{
currentdict /pdf_origFontName undef
} if
FontName currentdict
end
definefont pop
}
bd
Level2?
{
/TZG
{
currentglobal true setglobal
2 index _pdfFontStatus
{
2 index findfont
false setglobal
3 index findfont
true setglobal
ne
{
2 index findfont dup rcheck
{
dup length dict begin
{
1 index /FID ne { def } { pop pop } ifelse
} forall
currentdict end
}
if
3 index exch definefont pop
}
if
} if
setglobal
TZ
} bd
}
{
/TZG {TZ} bd
} ifelse
Level2?
{
currentglobal false setglobal
userdict /pdftext_data 5 dict put
pdftext_data
begin
/saveStacks
{
pdftext_data
begin
/vmmode currentglobal def
false setglobal
count array astore /os exch def
end
countdictstack array dictstack pdftext_data exch /ds exch put
cleardictstack pdftext_data /dscount countdictstack put
pdftext_data /vmmode get setglobal
} bind def
/restoreStacks
{
pdftext_data /vmmode currentglobal put false setglobal
clear cleardictstack
pdftext_data /ds get dup
pdftext_data /dscount get 1 2 index length 1 sub
{ get begin dup } for
pop pop
pdftext_data /os get aload pop
pdftext_data /vmmode get setglobal
} bind def
/testForClonePrinterBug
{
currentglobal true setglobal
/undefinedCategory /Generic /Category findresource
dup length dict copy /Category defineresource pop
setglobal
pdftext_data /saveStacks get exec
pdftext_data /vmmode currentglobal put false setglobal
/undefined /undefinedCategory { resourcestatus } stopped
pdftext_data exch /bugFound exch put
pdftext_data /vmmode get setglobal
pdftext_data /restoreStacks get exec
pdftext_data /bugFound get
} bind def
end
setglobal
/pdf_resourcestatus
pdftext_data /testForClonePrinterBug get exec
{
{
pdftext_data /saveStacks get exec
pdftext_data /os get dup dup length 1 sub
dup 1 sub dup 0 lt { pop 0 } if
exch 1 exch { get exch dup } for
pop pop
{ resourcestatus }
stopped
{
clear cleardictstack pdftext_data /restoreStacks get exec
{ pop pop } stopped pop false
}
{
count array astore pdftext_data exch /results exch put
pdftext_data /restoreStacks get exec pop pop
pdftext_data /results get aload pop
}
ifelse
}
}
{ { resourcestatus } }
ifelse
bd
}
if
Level2?
{
/_pdfUndefineResource
{
currentglobal 3 1 roll
_pdf_FontDirectory 2 index 2 copy known
{undef}
{pop pop}
ifelse
1 index (pdf) exch _pdfConcatNames 1 index
1 index 1 _pdfConcatNames 1 index
5 index 1 _pdfConcatNames 1 index
4
{
2 copy pdf_resourcestatus
{
pop 2 lt
{2 copy findresource gcheck setglobal undefineresource}
{pop pop}
ifelse
}
{ pop pop}
ifelse
} repeat
setglobal
} bd
}
{
/_pdfUndefineResource { pop pop} bd
}
ifelse
Level2?
{
/_pdfFontStatus
{
currentglobal exch
/Font pdf_resourcestatus
{pop pop true}
{false}
ifelse
exch setglobal
} bd
}
{
/_pdfFontStatusString 50 string def
_pdfFontStatusString 0 (fonts/) putinterval
/_pdfFontStatus
{
FontDirectory 1 index known
{ pop true }
{
_pdfFontStatusString 6 42 getinterval
cvs length 6 add
_pdfFontStatusString exch 0 exch getinterval
{ status } stopped
{pop false}
{
{ pop pop pop pop true}
{ false }
ifelse
}
ifelse
}
ifelse
} bd
}
ifelse
Level2?
{
/_pdfCIDFontStatus
{
/CIDFont /Category pdf_resourcestatus
{
pop pop
/CIDFont pdf_resourcestatus
{pop pop true}
{false}
ifelse
}
{ pop false }
ifelse
} bd
}
if
/_pdfString100 100 string def
/_pdfComposeFontName
{
dup length 1 eq
{
0 get
1 index
type /nametype eq
{
_pdfString100 cvs
length dup dup _pdfString100 exch (-) putinterval
_pdfString100 exch 1 add dup _pdfString100 length exch sub getinterval
2 index exch cvs length
add 1 add _pdfString100 exch 0 exch getinterval
exch pop
true
}
{
pop pop
false
}
ifelse
}
{
false
}
ifelse
dup {exch cvn exch} if
} bd
/_pdfConcatNames
{
exch
_pdfString100 cvs
length dup dup _pdfString100 exch (-) putinterval
_pdfString100 exch 1 add dup _pdfString100 length exch sub getinterval
3 -1 roll exch cvs length
add 1 add _pdfString100 exch 0 exch getinterval
cvn
} bind def
/_pdfTextTempString 50 string def
/_pdfRegOrderingArray [(Adobe-Japan1) (Adobe-CNS1) (Adobe-Korea1) (Adobe-GB1)] def
/_pdf_CheckCIDSystemInfo
{
1 index _pdfTextTempString cvs
(Identity) anchorsearch
{
pop pop pop pop true
}
{
false
_pdfRegOrderingArray
{
2 index exch
anchorsearch
{ pop pop pop true exit}
{ pop }
ifelse
}
forall
exch pop
exch /CIDFont findresource
/CIDSystemInfo get
3 -1 roll /CMap findresource
/CIDSystemInfo get
exch
3 -1 roll
{
2 copy
/Supplement get
exch
dup type /dicttype eq
{/Supplement get}
{pop 0 }
ifelse
ge
}
{ true }
ifelse
{
dup /Registry get
2 index /Registry get eq
{
/Ordering get
exch /Ordering get
dup type /arraytype eq
{
1 index type /arraytype eq
{
true
1 index length 1 sub -1 0
{
dup 2 index exch get exch 3 index exch get ne
{ pop false exit}
if
} for
exch pop exch pop
}
{ pop pop false }
ifelse
}
{
eq
}
ifelse
}
{ pop pop false }
ifelse
}
{ pop pop false }
ifelse
}
ifelse
} bind def
pdf_has_composefont?
{
/_pdfComposeFont
{
2 copy _pdfComposeFontName not
{
2 index
}
if
(pdf) exch _pdfConcatNames
dup _pdfFontStatus
{ dup findfont 5 2 roll pop pop pop true}
{
4 1 roll
1 index /CMap pdf_resourcestatus
{
pop pop
true
}
{false}
ifelse
1 index true exch
{
_pdfCIDFontStatus not
{pop false exit}
if
}
forall
and
{
1 index 1 index 0 get _pdf_CheckCIDSystemInfo
{
3 -1 roll pop
2 index 3 1 roll
composefont true
}
{
pop pop exch pop false
}
ifelse
}
{
_pdfComposeFontName
{
dup _pdfFontStatus
{
exch pop
1 index exch
findfont definefont true
}
{
pop exch pop
false
}
ifelse
}
{
exch pop
false
}
ifelse
}
ifelse
{ true }
{
dup _pdfFontStatus
{ dup findfont true }
{ pop false }
ifelse
}
ifelse
}
ifelse
} bd
}
{
/_pdfComposeFont
{
_pdfComposeFontName not
{
dup
}
if
dup
_pdfFontStatus
{exch pop dup findfont true}
{
1 index
dup type /nametype eq
{pop}
{cvn}
ifelse
eq
{pop false}
{
dup _pdfFontStatus
{dup findfont true}
{pop false}
ifelse
}
ifelse
}
ifelse
} bd
}
ifelse
/_pdfStyleDicts 4 dict dup begin
/Adobe-Japan1 4 dict dup begin
Level2?
{
/Serif
/HeiseiMin-W3-83pv-RKSJ-H _pdfFontStatus
{/HeiseiMin-W3}
{
/HeiseiMin-W3 _pdfCIDFontStatus
{/HeiseiMin-W3}
{/Ryumin-Light}
ifelse
}
ifelse
def
/SansSerif
/HeiseiKakuGo-W5-83pv-RKSJ-H _pdfFontStatus
{/HeiseiKakuGo-W5}
{
/HeiseiKakuGo-W5 _pdfCIDFontStatus
{/HeiseiKakuGo-W5}
{/GothicBBB-Medium}
ifelse
}
ifelse
def
/HeiseiMaruGo-W4-83pv-RKSJ-H _pdfFontStatus
{/HeiseiMaruGo-W4}
{
/HeiseiMaruGo-W4 _pdfCIDFontStatus
{/HeiseiMaruGo-W4}
{
/Jun101-Light-RKSJ-H _pdfFontStatus
{ /Jun101-Light }
{ SansSerif }
ifelse
}
ifelse
}
ifelse
/RoundSansSerif exch def
/Default Serif def
}
{
/Serif /Ryumin-Light def
/SansSerif /GothicBBB-Medium def
{
(fonts/Jun101-Light-83pv-RKSJ-H) status
}stopped
{pop}{
{ pop pop pop pop /Jun101-Light }
{ SansSerif }
ifelse
/RoundSansSerif exch def
}ifelse
/Default Serif def
}
ifelse
end
def
/Adobe-Korea1 4 dict dup begin
/Serif /HYSMyeongJo-Medium def
/SansSerif /HYGoThic-Medium def
/RoundSansSerif SansSerif def
/Default Serif def
end
def
/Adobe-GB1 4 dict dup begin
/Serif /STSong-Light def
/SansSerif /STHeiti-Regular def
/RoundSansSerif SansSerif def
/Default Serif def
end
def
/Adobe-CNS1 4 dict dup begin
/Serif /MKai-Medium def
/SansSerif /MHei-Medium def
/RoundSansSerif SansSerif def
/Default Serif def
end
def
end
def
/TZzero
{
/_wmode xdd
/_styleArr xdd
/_regOrdering xdd
3 copy
_pdfComposeFont
{
5 2 roll pop pop pop
}
{
[
0 1 _styleArr length 1 sub
{
_styleArr exch get
_pdfStyleDicts _regOrdering 2 copy known
{
get
exch 2 copy known not
{ pop /Default }
if
get
}
{
pop pop pop /Unknown
}
ifelse
}
for
]
exch pop
2 index 3 1 roll
_pdfComposeFont
{3 -1 roll pop}
{
findfont dup /FontName get exch
}
ifelse
}
ifelse
dup /WMode 2 copy known
{ get _wmode ne }
{ pop pop _wmode 1 eq}
ifelse
{
exch _wmode _pdfConcatNames
dup _pdfFontStatus
{ exch pop dup findfont false}
{ exch true }
ifelse
}
{
dup /FontType get 0 ne
}
ifelse
{
dup /FontType get 3 eq _wmode 1 eq and
{
_pdfVerticalRomanT3Font dup length 10 add dict copy
begin
/_basefont exch
dup length 3 add dict
begin
{1 index /FID ne {def}{pop pop} ifelse }
forall
/Encoding Encoding dup length array copy
dup 16#27 /quotesingle put
dup 16#60 /grave put
_regOrdering /Adobe-Japan1 eq
{dup 16#5c /yen put dup 16#a5 /yen put dup 16#b4 /yen put}
if
def
FontName
currentdict
end
definefont
def
/Encoding _basefont /Encoding get def
/_fauxfont true def
}
{
dup length 3 add dict
begin
{1 index /FID ne {def}{pop pop} ifelse }
forall
FontType 0 ne
{
/Encoding Encoding dup length array copy
dup 16#27 /quotesingle put
dup 16#60 /grave put
_regOrdering /Adobe-Japan1 eq
{dup 16#5c /yen put}
if
def
/_fauxfont true def
} if
} ifelse
/WMode _wmode def
dup dup /FontName exch def
currentdict
end
definefont pop
}
{
pop
}
ifelse
/_pdf_FontDirectory 3 1 roll _safeput
}
bd
Level2?
{
/Tf {
_pdf_FontDirectory 2 index 2 copy known
{get exch 3 -1 roll pop}
{pop pop}
ifelse
selectfont
} bd
}
{
/Tf {
_pdf_FontDirectory 2 index 2 copy known
{get exch 3 -1 roll pop}
{pop pop}
ifelse
exch findfont exch
dup type /arraytype eq
{makefont}
{scalefont}
ifelse
setfont
} bd
}
ifelse
/cshow where
{
pop /pdf_cshow /cshow load dd
/pdf_remove2 {pop pop} dd
}
{
/pdf_cshow {exch forall} dd
/pdf_remove2 {} dd
} ifelse
/pdf_xshow
{
/_pdf_na xdd
/_pdf_i 0 dd
currentpoint
/_pdf_y xdd
/_pdf_x xdd
{
pdf_remove2
_pdf_str1 exch 0 exch put
_pdf_str1 /_pdf_showproc load exec
{_pdf_na _pdf_i get} stopped
{ pop pop }
{
_pdf_x _pdf_y moveto
0
rmoveto
}
ifelse
_pdf_i 1 add /_pdf_i xdd
currentpoint
/_pdf_y xdd
/_pdf_x xdd
}
exch
pdf_cshow
} bd
/pdf_yshow
{
/_pdf_na xdd
/_pdf_i 0 dd
currentpoint
/_pdf_y xdd
/_pdf_x xdd
{
pdf_remove2
_pdf_str1 exch 0 exch put
_pdf_str1 /_pdf_showproc load exec
{_pdf_na _pdf_i get} stopped
{ pop pop }
{
_pdf_x _pdf_y moveto
0 exch
rmoveto
}
ifelse
_pdf_i 1 add /_pdf_i xdd
currentpoint
/_pdf_y xdd
/_pdf_x xdd
}
exch
pdf_cshow
} bd
/pdf_xyshow
{
/_pdf_na xdd
/_pdf_i 0 dd
currentpoint
/_pdf_y xdd
/_pdf_x xdd
{
pdf_remove2
_pdf_str1 exch 0 exch put
_pdf_str1 /_pdf_showproc load exec
{_pdf_na _pdf_i get} stopped
{ pop pop }
{
{_pdf_na _pdf_i 1 add get} stopped
{ pop pop pop}
{
_pdf_x _pdf_y moveto
rmoveto
}
ifelse
}
ifelse
_pdf_i 2 add /_pdf_i xdd
currentpoint
/_pdf_y xdd
/_pdf_x xdd
}
exch
pdf_cshow
} bd
/pdfl1xs {/_pdf_showproc /show load dd pdf_xshow} bd
/pdfl1ys {/_pdf_showproc /show load dd pdf_yshow} bd
/pdfl1xys {/_pdf_showproc /show load dd pdf_xyshow} bd
Level2? _ColorSep5044? not and
{
/pdfxs {{xshow} stopped {pdfl1xs} if} bd
/pdfys {{yshow} stopped {pdfl1ys} if} bd
/pdfxys {{xyshow} stopped {pdfl1xys} if} bd
}
{
/pdfxs /pdfl1xs load dd
/pdfys /pdfl1ys load dd
/pdfxys /pdfl1xys load dd
} ifelse
/pdf_charpath {false charpath} bd
/pdf_xcharpath {/_pdf_showproc /pdf_charpath load dd pdf_xshow} bd
/pdf_ycharpath {/_pdf_showproc /pdf_charpath load dd pdf_yshow} bd
/pdf_xycharpath {/_pdf_showproc /pdf_charpath load dd pdf_xyshow} bd
/pdf_strokepath
{
{
pdf_remove2
_pdf_str1 exch 0 exch put
_pdf_str1 false charpath
currentpoint S moveto
} bind
exch pdf_cshow
} bd
/pdf_xstrokepath {/_pdf_showproc {pdf_charpath S} dd pdf_xshow} bd
/pdf_ystrokepath {/_pdf_showproc {pdf_charpath S} dd pdf_yshow} bd
/pdf_xystrokepath {/_pdf_showproc {pdf_charpath S} load dd pdf_xyshow} bd
Level2? {currentglobal true setglobal} if
/d0/setcharwidth ld
/nND {{/.notdef} repeat} bd
/T3Defs {
/BuildChar
{
1 index /Encoding get exch get
1 index /BuildGlyph get exec
}
def
/BuildGlyph {
exch begin
GlyphProcs exch get exec
end
} def
/_pdfT3Font true def
} bd
/_pdfBoldRomanWidthProc
{
stringwidth 1 index 0 ne { exch .03 add exch }if setcharwidth
0 0
} bd
/_pdfType0WidthProc
{
dup stringwidth 0 0 moveto
2 index true charpath pathbbox
0 -1
7 index 2 div .88
setcachedevice2
pop
0 0
} bd
/_pdfType0WMode1WidthProc
{
dup stringwidth
pop 2 div neg -0.88
2 copy
moveto
0 -1
5 -1 roll true charpath pathbbox
setcachedevice
} bd
/_pdfBoldBaseFont
11 dict begin
/FontType 3 def
/FontMatrix[1 0 0 1 0 0]def
/FontBBox[0 0 1 1]def
/Encoding cHexEncoding def
/_setwidthProc /_pdfBoldRomanWidthProc load def
/_bcstr1 1 string def
/BuildChar
{
exch begin
_basefont setfont
_bcstr1 dup 0 4 -1 roll put
dup
_setwidthProc
3 copy
moveto
show
_basefonto setfont
moveto
show
end
}bd
currentdict
end
def
pdf_has_composefont?
{
/_pdfBoldBaseCIDFont
11 dict begin
/CIDFontType 1 def
/CIDFontName /_pdfBoldBaseCIDFont def
/FontMatrix[1 0 0 1 0 0]def
/FontBBox[0 0 1 1]def
/_setwidthProc /_pdfType0WidthProc load def
/_bcstr2 2 string def
/BuildGlyph
{
exch begin
_basefont setfont
_bcstr2 1 2 index 256 mod put
_bcstr2 0 3 -1 roll 256 idiv put
_bcstr2 dup _setwidthProc
3 copy
moveto
show
_basefonto setfont
moveto
show
end
}bd
currentdict
end
def
/_pdfDefineIdentity-H
{
/Identity-H /CMap PDFText /pdf_resourcestatus get exec
{
pop pop
}
{
/CIDInit/ProcSet findresource begin 12 dict begin
begincmap
/CIDSystemInfo
3 dict begin
/Registry (Adobe) def
/Ordering (Identity) def
/Supplement 0 def
currentdict
end
def
/CMapName /Identity-H def
/CMapVersion 1 def
/CMapType 1 def
1 begincodespacerange
<0000> <ffff>
endcodespacerange
1 begincidrange
<0000> <ffff> 0
endcidrange
endcmap
CMapName currentdict/CMap defineresource pop
end
end
} ifelse
} def
} if
/_pdfVerticalRomanT3Font
10 dict begin
/FontType 3 def
/FontMatrix[1 0 0 1 0 0]def
/FontBBox[0 0 1 1]def
/_bcstr1 1 string def
/BuildChar
{
exch begin
_basefont setfont
_bcstr1 dup 0 4 -1 roll put
dup
_pdfType0WidthProc
moveto
show
end
}bd
currentdict
end
def
Level2? {setglobal} if
/MakeBoldFont
{
dup /ct_SyntheticBold known
{
dup length 3 add dict begin
CopyFont
/ct_StrokeWidth .03 0 FontMatrix idtransform pop def
/ct_SyntheticBold true def
currentdict
end
definefont
}
{
dup dup length 3 add dict
begin
CopyFont
/PaintType 2 def
/StrokeWidth .03 0 FontMatrix idtransform pop def
/dummybold currentdict
end
definefont
dup /FontType get dup 9 ge exch 11 le and
{
_pdfBoldBaseCIDFont
dup length 3 add dict copy begin
dup /CIDSystemInfo get /CIDSystemInfo exch def
/_Type0Identity /Identity-H 3 -1 roll [ exch ] composefont
/_basefont exch def
/_Type0Identity /Identity-H 3 -1 roll [ exch ] composefont
/_basefonto exch def
currentdict
end
/CIDFont defineresource
}
{
_pdfBoldBaseFont
dup length 3 add dict copy begin
/_basefont exch def
/_basefonto exch def
currentdict
end
definefont
}
ifelse
}
ifelse
} bd
/MakeBold {
1 index
_pdf_FontDirectory 2 index 2 copy known
{get}
{exch pop}
ifelse
findfont
dup
/FontType get 0 eq
{
dup /WMode known {dup /WMode get 1 eq }{false} ifelse
version length 4 ge
and
{version 0 4 getinterval cvi 2015 ge }
{true}
ifelse
{/_pdfType0WidthProc}
{/_pdfType0WMode1WidthProc}
ifelse
_pdfBoldBaseFont /_setwidthProc 3 -1 roll load put
{MakeBoldFont} Type0CopyFont definefont
}
{
dup /_fauxfont known not 1 index /SubstMaster known not and
{
_pdfBoldBaseFont /_setwidthProc /_pdfBoldRomanWidthProc load put
MakeBoldFont
}
{
2 index 2 index eq
{ exch pop }
{
dup length dict begin
CopyFont
currentdict
end
definefont
}
ifelse
}
ifelse
}
ifelse
pop pop
dup /dummybold ne
{/_pdf_FontDirectory exch dup _safeput }
{ pop }
ifelse
}bd
/MakeItalic {
_pdf_FontDirectory exch 2 copy known
{get}
{exch pop}
ifelse
dup findfont
dup /FontInfo 2 copy known
{
get
/ItalicAngle 2 copy known
{get 0 eq }
{ pop pop true}
ifelse
}
{ pop pop true}
ifelse
{
exch pop
dup /FontType get 0 eq Level2? not and
{ dup /FMapType get 6 eq }
{ false }
ifelse
{
dup /WMode 2 copy known
{
get 1 eq
{ _italMtx_WMode1Type0 }
{ _italMtxType0 }
ifelse
}
{ pop pop _italMtxType0 }
ifelse
}
{
dup /WMode 2 copy known
{
get 1 eq
{ _italMtx_WMode1 }
{ _italMtx }
ifelse
}
{ pop pop _italMtx }
ifelse
}
ifelse
makefont
dup /FontType get 42 eq Level2? not or
{
dup length dict begin
CopyFont
currentdict
end
}
if
1 index exch
definefont pop
/_pdf_FontDirectory exch dup _safeput
}
{
pop
2 copy ne
{
/_pdf_FontDirectory 3 1 roll _safeput
}
{ pop pop }
ifelse
}
ifelse
}bd
/MakeBoldItalic {
/dummybold exch
MakeBold
/dummybold
MakeItalic
}bd
Level2?
{
/pdf_CopyDict
{1 index length add dict copy}
def
}
{
/pdf_CopyDict
{
1 index length add dict
1 index wcheck
{ copy }
{ begin
{def} forall
currentdict
end
}
ifelse
}
def
}
ifelse
/pdf_AddEuroGlyphProc
{
currentdict /CharStrings known
{
CharStrings /Euro known not
{
dup
/CharStrings
CharStrings 1 pdf_CopyDict
begin
/Euro pdf_EuroProcSet 4 -1 roll get def
currentdict
end
def
/pdf_PSBuildGlyph /pdf_PSBuildGlyph load def
/pdf_PathOps /pdf_PathOps load def
/Symbol eq
{
/Encoding Encoding dup length array copy
dup 160 /Euro put def
}
if
}
{ pop
}
ifelse
}
{ pop
}
ifelse
}
def
Level2? {currentglobal true setglobal} if
/pdf_PathOps 4 dict dup begin
/m {moveto} def
/l {lineto} def
/c {curveto} def
/cp {closepath} def
end
def
/pdf_PSBuildGlyph
{
gsave
8 -1 roll pop
7 1 roll
currentdict /PaintType 2 copy known {get 2 eq}{pop pop false} ifelse
dup 9 1 roll
{
currentdict /StrokeWidth 2 copy known
{
get 2 div
5 1 roll
4 -1 roll 4 index sub
4 1 roll
3 -1 roll 4 index sub
3 1 roll
exch 4 index add exch
4 index add
5 -1 roll pop
}
{
pop pop
}
ifelse
}
if
setcachedevice
pdf_PathOps begin
exec
end
{
currentdict /StrokeWidth 2 copy known
{ get }
{ pop pop 0 }
ifelse
setlinewidth stroke
}
{
fill
}
ifelse
grestore
} def
/pdf_EuroProcSet 13 dict def
pdf_EuroProcSet
begin
/Courier-Bold
{
600 0 6 -12 585 612
{
385 274 m
180 274 l
179 283 179 293 179 303 c
179 310 179 316 180 323 c
398 323 l
423 404 l
197 404 l
219 477 273 520 357 520 c
409 520 466 490 487 454 c
487 389 l
579 389 l
579 612 l
487 612 l
487 560 l
449 595 394 612 349 612 c
222 612 130 529 98 404 c
31 404 l
6 323 l
86 323 l
86 304 l
86 294 86 284 87 274 c
31 274 l
6 193 l
99 193 l
129 77 211 -12 359 -12 c
398 -12 509 8 585 77 c
529 145 l
497 123 436 80 356 80 c
285 80 227 122 198 193 c
360 193 l
cp
600 0 m
}
pdf_PSBuildGlyph
} def
/Courier-BoldOblique /Courier-Bold load def
/Courier
{
600 0 17 -12 578 584
{
17 204 m
97 204 l
126 81 214 -12 361 -12 c
440 -12 517 17 578 62 c
554 109 l
501 70 434 43 366 43 c
266 43 184 101 154 204 c
380 204 l
400 259 l
144 259 l
144 270 143 281 143 292 c
143 299 143 307 144 314 c
418 314 l
438 369 l
153 369 l
177 464 249 529 345 529 c
415 529 484 503 522 463 c
522 391 l
576 391 l
576 584 l
522 584 l
522 531 l
473 566 420 584 348 584 c
216 584 122 490 95 369 c
37 369 l
17 314 l
87 314 l
87 297 l
87 284 88 272 89 259 c
37 259 l
cp
600 0 m
}
pdf_PSBuildGlyph
} def
/Courier-Oblique /Courier load def
/Helvetica
{
556 0 24 -19 541 703
{
541 628 m
510 669 442 703 354 703 c
201 703 117 607 101 444 c
50 444 l
25 372 l
97 372 l
97 301 l
49 301 l
24 229 l
103 229 l
124 67 209 -19 350 -19 c
435 -19 501 25 509 32 c
509 131 l
492 105 417 60 343 60 c
267 60 204 127 197 229 c
406 229 l
430 301 l
191 301 l
191 372 l
455 372 l
479 444 l
194 444 l
201 531 245 624 348 624 c
433 624 484 583 509 534 c
cp
556 0 m
}
pdf_PSBuildGlyph
} def
/Helvetica-Oblique /Helvetica load def
/Helvetica-Bold
{
556 0 12 -19 563 710
{
563 621 m
537 659 463 710 363 710 c
216 710 125 620 101 462 c
51 462 l
12 367 l
92 367 l
92 346 l
92 337 93 328 93 319 c
52 319 l
12 224 l
102 224 l
131 58 228 -19 363 -19 c
417 -19 471 -12 517 18 c
517 146 l
481 115 426 93 363 93 c
283 93 254 166 246 224 c
398 224 l
438 319 l
236 319 l
236 367 l
457 367 l
497 462 l
244 462 l
259 552 298 598 363 598 c
425 598 464 570 486 547 c
507 526 513 517 517 509 c
cp
556 0 m
}
pdf_PSBuildGlyph
} def
/Helvetica-BoldOblique /Helvetica-Bold load def
/Symbol
{
750 0 20 -12 714 685
{
714 581 m
650 645 560 685 465 685 c
304 685 165 580 128 432 c
50 432 l
20 369 l
116 369 l
115 356 115 347 115 337 c
115 328 115 319 116 306 c
50 306 l
20 243 l
128 243 l
165 97 300 -12 465 -12 c
560 -12 635 25 685 65 c
685 155 l
633 91 551 51 465 51 c
340 51 238 131 199 243 c
555 243 l
585 306 l
184 306 l
183 317 182 326 182 336 c
182 346 183 356 184 369 c
614 369 l 644 432 l
199 432 l
233 540 340 622 465 622 c
555 622 636 580 685 520 c
cp
750 0 m
}
pdf_PSBuildGlyph
} def
/Times-Bold
{
500 0 16 -14 478 700
{
367 308 m
224 308 l
224 368 l
375 368 l
380 414 l
225 414 l
230 589 257 653 315 653 c
402 653 431 521 444 457 c
473 457 l
473 698 l
444 697 l
441 679 437 662 418 662 c
393 662 365 700 310 700 c
211 700 97 597 73 414 c
21 414 l
16 368 l
69 368 l
69 359 68 350 68 341 c
68 330 68 319 69 308 c
21 308 l
16 262 l
73 262 l
91 119 161 -14 301 -14 c
380 -14 443 50 478 116 c
448 136 l
415 84 382 40 323 40 c
262 40 231 77 225 262 c
362 262 l
cp
500 0 m
}
pdf_PSBuildGlyph
} def
/Times-BoldItalic
{
500 0 9 -20 542 686
{
542 686 m
518 686 l
513 673 507 660 495 660 c
475 660 457 683 384 683 c
285 683 170 584 122 430 c
58 430 l
34 369 l
105 369 l
101 354 92 328 90 312 c
34 312 l
9 251 l
86 251 l
85 238 84 223 84 207 c
84 112 117 -14 272 -14 c
326 -14 349 9 381 9 c
393 9 393 -10 394 -20 c
420 -20 l
461 148 l
429 148 l
416 109 362 15 292 15 c
227 15 197 55 197 128 c
197 162 204 203 216 251 c
378 251 l
402 312 l
227 312 l
229 325 236 356 241 369 c
425 369 l
450 430 l
255 430 l
257 435 264 458 274 488 c
298 561 337 654 394 654 c
437 654 484 621 484 530 c
484 516 l
516 516 l
cp
500 0 m
}
pdf_PSBuildGlyph
} def
/Times-Italic
{
500 0 23 -10 595 692
{
399 317 m
196 317 l
199 340 203 363 209 386 c
429 386 l
444 424 l
219 424 l
246 514 307 648 418 648 c
448 648 471 638 492 616 c
529 576 524 529 527 479 c
549 475 l
595 687 l
570 687 l
562 674 558 664 542 664 c
518 664 474 692 423 692 c
275 692 162 551 116 424 c
67 424 l
53 386 l
104 386 l
98 363 93 340 90 317 c
37 317 l
23 279 l
86 279 l
85 266 85 253 85 240 c
85 118 137 -10 277 -10 c
370 -10 436 58 488 128 c
466 149 l
424 101 375 48 307 48 c
212 48 190 160 190 234 c
190 249 191 264 192 279 c
384 279 l
cp
500 0 m
}
pdf_PSBuildGlyph
} def
/Times-Roman
{
500 0 10 -12 484 692
{
347 298 m
171 298 l
170 310 170 322 170 335 c
170 362 l
362 362 l
374 403 l
172 403 l
184 580 244 642 308 642 c
380 642 434 574 457 457 c
481 462 l
474 691 l
449 691 l
433 670 429 657 410 657 c
394 657 360 692 299 692 c
204 692 94 604 73 403 c
22 403 l
10 362 l
70 362 l
69 352 69 341 69 330 c
69 319 69 308 70 298 c
22 298 l
10 257 l
73 257 l
97 57 216 -12 295 -12 c
364 -12 427 25 484 123 c
458 142 l
425 101 384 37 316 37 c
256 37 189 84 173 257 c
335 257 l
cp
500 0 m
}
pdf_PSBuildGlyph
} def
end
Level2? {setglobal} if
currentdict readonly pop end
%%EndResource
PDFText begin
[userdict /pdf_svglb currentglobal put true setglobal
39/quotesingle 96/grave 128/Adieresis/Aring/Ccedilla/Eacute/Ntilde/Odieresis
/Udieresis/aacute/agrave/acircumflex/adieresis/atilde/aring/ccedilla/eacute
/egrave/ecircumflex/edieresis/iacute/igrave/icircumflex/idieresis/ntilde
/oacute/ograve/ocircumflex/odieresis/otilde/uacute/ugrave/ucircumflex
/udieresis/dagger/degree/cent/sterling/section/bullet/paragraph/germandbls
/registered/copyright/trademark/acute/dieresis/.notdef/AE/Oslash
/.notdef/plusminus/.notdef/.notdef/yen/mu/.notdef/.notdef
/.notdef/.notdef/.notdef/ordfeminine/ordmasculine/.notdef/ae/oslash
/questiondown/exclamdown/logicalnot/.notdef/florin/.notdef/.notdef
/guillemotleft/guillemotright/ellipsis/space/Agrave/Atilde/Otilde/OE/oe
/endash/emdash/quotedblleft/quotedblright/quoteleft/quoteright/divide
/.notdef/ydieresis/Ydieresis/fraction/currency/guilsinglleft/guilsinglright
/fi/fl/daggerdbl/periodcentered/quotesinglbase/quotedblbase/perthousand
/Acircumflex/Ecircumflex/Aacute/Edieresis/Egrave/Iacute/Icircumflex
/Idieresis/Igrave/Oacute/Ocircumflex/.notdef/Ograve/Uacute/Ucircumflex
/Ugrave/dotlessi/circumflex/tilde/macron/breve/dotaccent/ring/cedilla
/hungarumlaut/ogonek/caron
0 TE
[1/dotlessi/caron 39/quotesingle 96/grave 
127/bullet/Euro/bullet/quotesinglbase/florin/quotedblbase/ellipsis
/dagger/daggerdbl/circumflex/perthousand/Scaron/guilsinglleft/OE
/bullet/Zcaron/bullet/bullet/quoteleft/quoteright/quotedblleft
/quotedblright/bullet/endash/emdash/tilde/trademark/scaron
/guilsinglright/oe/bullet/zcaron/Ydieresis/space/exclamdown/cent/sterling
/currency/yen/brokenbar/section/dieresis/copyright/ordfeminine
/guillemotleft/logicalnot/hyphen/registered/macron/degree/plusminus
/twosuperior/threesuperior/acute/mu/paragraph/periodcentered/cedilla
/onesuperior/ordmasculine/guillemotright/onequarter/onehalf/threequarters
/questiondown/Agrave/Aacute/Acircumflex/Atilde/Adieresis/Aring/AE/Ccedilla
/Egrave/Eacute/Ecircumflex/Edieresis/Igrave/Iacute/Icircumflex/Idieresis
/Eth/Ntilde/Ograve/Oacute/Ocircumflex/Otilde/Odieresis/multiply/Oslash
/Ugrave/Uacute/Ucircumflex/Udieresis/Yacute/Thorn/germandbls/agrave
/aacute/acircumflex/atilde/adieresis/aring/ae/ccedilla/egrave/eacute
/ecircumflex/edieresis/igrave/iacute/icircumflex/idieresis/eth/ntilde
/ograve/oacute/ocircumflex/otilde/odieresis/divide/oslash/ugrave/uacute
/ucircumflex/udieresis/yacute/thorn/ydieresis
1 TE
end

userdict /pdf_svglb get setglobal
%%BeginResource: pdfasc.prc
%%Version: 4.0 2
%%Copyright: Copyright 1992-1997 Adobe Systems Incorporated. All Rights Reserved.
/AS {
9 dict begin
/shrink? xdd
/Pury xdd
/Purx xdd
/Plly xdd
/Pllx xdd
gsave newpath clippath pathbbox newpath grestore
/Dury xdd
/Durx xdd
/Dlly xdd
/Dllx xdd
Durx Dllx sub Dury Dlly sub
Pury Plly sub div exch Purx Pllx sub div
2 copy gt { exch } if pop
Durx Dllx add 2 div Dury Dlly add 2 div translate
shrink? { dup scale } { pop } ifelse
Purx Pllx add -2 div Pury Plly add -2 div translate
end
} [/shrink? /Pury /Purx /Plly /Pllx /Durx /Dury /Dllx /Dlly]
bld
%%EndResource
currentdict readonly pop
end end
/currentpacking where {pop setpacking}if
PDFVars/DocInitAll{[PDF PDFText]{/docinitialize get exec}forall }put
PDFVars/InitAll{[PDF PDFText]{/initialize get exec}forall initgs}put
PDFVars/TermAll{[PDFText PDF]{/terminate get exec}forall}put
PDFVars begin PDF begin
PDFVars/DocInitAll get exec PDFVars/InitAll get exec
/N278 [/CIEBasedABC  9 dict 
dup /CreationDate (19980209064900) put
dup /RenderingIntent (RelativeColorimetric) put
dup /Description (sRGB IEC61966-2.1) put
dup /ColorSpace (RGB ) put
dup /Copyright (Copyright (c) 1998 Hewlett-Packard Company) put
dup /DecodeLMN [

{{0.0000 0.0003 0.0006 0.0009 0.0012 0.0015 0.0018 0.0021 0.0024 0.0027 0.0030 0.0034 0.0037 0.0040 0.0044 0.0048 
0.0052 0.0056 0.0060 0.0065 0.0070 0.0075 0.0080 0.0086 0.0091 0.0097 0.0103 0.0110 0.0116 0.0123 0.0130 0.0137 
0.0144 0.0152 0.0160 0.0168 0.0176 0.0185 0.0194 0.0203 0.0212 0.0222 0.0232 0.0242 0.0252 0.0262 0.0273 0.0284 
0.0296 0.0307 0.0319 0.0331 0.0343 0.0356 0.0369 0.0382 0.0395 0.0409 0.0423 0.0437 0.0452 0.0467 0.0482 0.0497 
0.0513 0.0529 0.0545 0.0561 0.0578 0.0595 0.0612 0.0630 0.0648 0.0666 0.0685 0.0704 0.0723 0.0742 0.0762 0.0782 
0.0802 0.0823 0.0844 0.0865 0.0886 0.0908 0.0931 0.0953 0.0976 0.0999 0.1022 0.1046 0.1070 0.1095 0.1119 0.1144 
0.1170 0.1195 0.1221 0.1248 0.1274 0.1301 0.1329 0.1356 0.1384 0.1413 0.1441 0.1470 0.1500 0.1529 0.1559 0.1590 
0.1620 0.1651 0.1683 0.1714 0.1746 0.1779 0.1812 0.1845 0.1878 0.1912 0.1946 0.1981 0.2016 0.2051 0.2086 0.2122 
0.2159 0.2195 0.2232 0.2270 0.2307 0.2346 0.2384 0.2423 0.2462 0.2502 0.2542 0.2582 0.2622 0.2664 0.2705 0.2747 
0.2789 0.2832 0.2874 0.2918 0.2961 0.3005 0.3050 0.3095 0.3140 0.3185 0.3231 0.3278 0.3325 0.3372 0.3419 0.3467 
0.3515 0.3564 0.3613 0.3663 0.3712 0.3763 0.3813 0.3864 0.3916 0.3967 0.4020 0.4072 0.4125 0.4179 0.4233 0.4287 
0.4342 0.4397 0.4452 0.4508 0.4564 0.4621 0.4678 0.4735 0.4793 0.4851 0.4910 0.4969 0.5029 0.5089 0.5149 0.5210 
0.5271 0.5333 0.5395 0.5457 0.5520 0.5583 0.5647 0.5711 0.5776 0.5841 0.5906 0.5972 0.6038 0.6105 0.6172 0.6240 
0.6308 0.6376 0.6445 0.6514 0.6584 0.6654 0.6724 0.6795 0.6867 0.6939 0.7011 0.7084 0.7157 0.7231 0.7305 0.7379 
0.7454 0.7529 0.7605 0.7682 0.7758 0.7835 0.7913 0.7991 0.8069 0.8148 0.8228 0.8308 0.8388 0.8469 0.8550 0.8632 
0.8714 0.8796 0.8879 0.8963 0.9047 0.9131 0.9216 0.9301 0.9387 0.9473 0.9560 0.9647 0.9734 0.9822 0.9911 1.0000 }
dup 3 -1 roll 0.0000 1.0000 3 copy 3 -1 roll exch ge
{pop pop pop pop pop 255 get}
{pop 3 copy pop le{pop pop pop pop 0 get}{exch dup 4 -1 roll exch sub 3 1 roll sub div 255 mul dup floor dup 3 1 roll sub exch cvi dup 1 add 4 -1 roll exch get 4 -1 roll 3 -1 roll get dup 4 1 roll sub mul add}
ifelse}ifelse}bind
{{0.0000 0.0003 0.0006 0.0009 0.0012 0.0015 0.0018 0.0021 0.0024 0.0027 0.0030 0.0034 0.0037 0.0040 0.0044 0.0048 
0.0052 0.0056 0.0060 0.0065 0.0070 0.0075 0.0080 0.0086 0.0091 0.0097 0.0103 0.0110 0.0116 0.0123 0.0130 0.0137 
0.0144 0.0152 0.0160 0.0168 0.0176 0.0185 0.0194 0.0203 0.0212 0.0222 0.0232 0.0242 0.0252 0.0262 0.0273 0.0284 
0.0296 0.0307 0.0319 0.0331 0.0343 0.0356 0.0369 0.0382 0.0395 0.0409 0.0423 0.0437 0.0452 0.0467 0.0482 0.0497 
0.0513 0.0529 0.0545 0.0561 0.0578 0.0595 0.0612 0.0630 0.0648 0.0666 0.0685 0.0704 0.0723 0.0742 0.0762 0.0782 
0.0802 0.0823 0.0844 0.0865 0.0886 0.0908 0.0931 0.0953 0.0976 0.0999 0.1022 0.1046 0.1070 0.1095 0.1119 0.1144 
0.1170 0.1195 0.1221 0.1248 0.1274 0.1301 0.1329 0.1356 0.1384 0.1413 0.1441 0.1470 0.1500 0.1529 0.1559 0.1590 
0.1620 0.1651 0.1683 0.1714 0.1746 0.1779 0.1812 0.1845 0.1878 0.1912 0.1946 0.1981 0.2016 0.2051 0.2086 0.2122 
0.2159 0.2195 0.2232 0.2270 0.2307 0.2346 0.2384 0.2423 0.2462 0.2502 0.2542 0.2582 0.2622 0.2664 0.2705 0.2747 
0.2789 0.2832 0.2874 0.2918 0.2961 0.3005 0.3050 0.3095 0.3140 0.3185 0.3231 0.3278 0.3325 0.3372 0.3419 0.3467 
0.3515 0.3564 0.3613 0.3663 0.3712 0.3763 0.3813 0.3864 0.3916 0.3967 0.4020 0.4072 0.4125 0.4179 0.4233 0.4287 
0.4342 0.4397 0.4452 0.4508 0.4564 0.4621 0.4678 0.4735 0.4793 0.4851 0.4910 0.4969 0.5029 0.5089 0.5149 0.5210 
0.5271 0.5333 0.5395 0.5457 0.5520 0.5583 0.5647 0.5711 0.5776 0.5841 0.5906 0.5972 0.6038 0.6105 0.6172 0.6240 
0.6308 0.6376 0.6445 0.6514 0.6584 0.6654 0.6724 0.6795 0.6867 0.6939 0.7011 0.7084 0.7157 0.7231 0.7305 0.7379 
0.7454 0.7529 0.7605 0.7682 0.7758 0.7835 0.7913 0.7991 0.8069 0.8148 0.8228 0.8308 0.8388 0.8469 0.8550 0.8632 
0.8714 0.8796 0.8879 0.8963 0.9047 0.9131 0.9216 0.9301 0.9387 0.9473 0.9560 0.9647 0.9734 0.9822 0.9911 1.0000 }
dup 3 -1 roll 0.0000 1.0000 3 copy 3 -1 roll exch ge
{pop pop pop pop pop 255 get}
{pop 3 copy pop le{pop pop pop pop 0 get}{exch dup 4 -1 roll exch sub 3 1 roll sub div 255 mul dup floor dup 3 1 roll sub exch cvi dup 1 add 4 -1 roll exch get 4 -1 roll 3 -1 roll get dup 4 1 roll sub mul add}
ifelse}ifelse}bind
{{0.0000 0.0003 0.0006 0.0009 0.0012 0.0015 0.0018 0.0021 0.0024 0.0027 0.0030 0.0034 0.0037 0.0040 0.0044 0.0048 
0.0052 0.0056 0.0060 0.0065 0.0070 0.0075 0.0080 0.0086 0.0091 0.0097 0.0103 0.0110 0.0116 0.0123 0.0130 0.0137 
0.0144 0.0152 0.0160 0.0168 0.0176 0.0185 0.0194 0.0203 0.0212 0.0222 0.0232 0.0242 0.0252 0.0262 0.0273 0.0284 
0.0296 0.0307 0.0319 0.0331 0.0343 0.0356 0.0369 0.0382 0.0395 0.0409 0.0423 0.0437 0.0452 0.0467 0.0482 0.0497 
0.0513 0.0529 0.0545 0.0561 0.0578 0.0595 0.0612 0.0630 0.0648 0.0666 0.0685 0.0704 0.0723 0.0742 0.0762 0.0782 
0.0802 0.0823 0.0844 0.0865 0.0886 0.0908 0.0931 0.0953 0.0976 0.0999 0.1022 0.1046 0.1070 0.1095 0.1119 0.1144 
0.1170 0.1195 0.1221 0.1248 0.1274 0.1301 0.1329 0.1356 0.1384 0.1413 0.1441 0.1470 0.1500 0.1529 0.1559 0.1590 
0.1620 0.1651 0.1683 0.1714 0.1746 0.1779 0.1812 0.1845 0.1878 0.1912 0.1946 0.1981 0.2016 0.2051 0.2086 0.2122 
0.2159 0.2195 0.2232 0.2270 0.2307 0.2346 0.2384 0.2423 0.2462 0.2502 0.2542 0.2582 0.2622 0.2664 0.2705 0.2747 
0.2789 0.2832 0.2874 0.2918 0.2961 0.3005 0.3050 0.3095 0.3140 0.3185 0.3231 0.3278 0.3325 0.3372 0.3419 0.3467 
0.3515 0.3564 0.3613 0.3663 0.3712 0.3763 0.3813 0.3864 0.3916 0.3967 0.4020 0.4072 0.4125 0.4179 0.4233 0.4287 
0.4342 0.4397 0.4452 0.4508 0.4564 0.4621 0.4678 0.4735 0.4793 0.4851 0.4910 0.4969 0.5029 0.5089 0.5149 0.5210 
0.5271 0.5333 0.5395 0.5457 0.5520 0.5583 0.5647 0.5711 0.5776 0.5841 0.5906 0.5972 0.6038 0.6105 0.6172 0.6240 
0.6308 0.6376 0.6445 0.6514 0.6584 0.6654 0.6724 0.6795 0.6867 0.6939 0.7011 0.7084 0.7157 0.7231 0.7305 0.7379 
0.7454 0.7529 0.7605 0.7682 0.7758 0.7835 0.7913 0.7991 0.8069 0.8148 0.8228 0.8308 0.8388 0.8469 0.8550 0.8632 
0.8714 0.8796 0.8879 0.8963 0.9047 0.9131 0.9216 0.9301 0.9387 0.9473 0.9560 0.9647 0.9734 0.9822 0.9911 1.0000 }
dup 3 -1 roll 0.0000 1.0000 3 copy 3 -1 roll exch ge
{pop pop pop pop pop 255 get}
{pop 3 copy pop le{pop pop pop pop 0 get}{exch dup 4 -1 roll exch sub 3 1 roll sub div 255 mul dup floor dup 3 1 roll sub exch cvi dup 1 add 4 -1 roll exch get 4 -1 roll 3 -1 roll get dup 4 1 roll sub mul add}
ifelse}ifelse}bind] put
dup /MatrixLMN [0.4361 0.2225 0.0139 0.3851 0.7169 0.0971 0.1431 0.0606 0.7141] put
dup /WhitePoint [0.9642 1.0000 0.8249] put]
/ColorSpace defineRes pop

userdict /pdf_svglb currentglobal put true setglobal
ct_T42Dict begin
-0.566 -0.305 2 1.004
 256 array 0 1 255 {1 index exch /.notdef put} for  /EKJCLI+TimesNewRoman
Type42DictBegin
[<00010000000a000a000a000a63767420f32cda81000000ac000007c66670
676dc3a61d010000087400000631676c79665f5e2a010000528c000029d2
68656164cf5b1d8300000ea8000000366868656112ef12f600000ee00000
0024686d7478b14216ca00000f0400001a286c6f636101065dd60000292c
00001a2c6d6178700d02019a000043580000002070726570e43894a40000
437800000f1367646972000000000000000000000000058e0000054c001f
054c001c0394001b0000ffe10000ffe40000ffe8fe4afffc056b0023fe6a
ffe00313000000ad000000ad0000000000250096009f002400f0013100c2
00c0004a00a6004100500094004700cf00af000e007901cb000400230044
00a80025011f0002004600170105009900d9005c007200e500e00028004b
00de011200240045007000160039ffe90016004b0088ffb900d9000a0043
00ae00ba016c0153002f00430048022c012b0025008fffc000170028ffcd
ffd80025009d00e50124ffb10048009d00e600110027007f00910012006a
00cafffc00000024006200a7017c01e900210060008b0434048aff6b003b
00b500d5014bff6b004d007905d809b5006c009100a3011701c0ffdfffe7
00be04010065007f00820088009900b200c0022e034305a000200026003d
004e00610065007b00d9011301310340ff27ff42ff99004e00a700f2022b
02c603070011002b0049005f008d00a100af00d600e400f5010b0135019d
01ab01ab01d101ee05d80000004b0075007a0080009d00a600a700ac00b9
013101310217021700020017002900550080008f00a500b200b300d0014b
015901c001c103a50530fe3fff14ff15ffe7ffff002a00580099009f00c1
00e400f40130015901ab01ab03220374041e04740532fd81004d0064009c
00d000d100d600de00e500f500f8012a012a01e1027e027fff57ffa8ffe5
00000008001f00380051005a006f0076007700a200c000c200c400f101fb
0209027e02cf04c5057a05f0ff92001200260042004b004f005100530064
008b00ae00b200b800b800d600f50111012001310138014e01520167018f
019601b801d901d902060221027102ea03b003cb03dc04360505ff3a0012
0016001e001f002300570068006c007e0088009200a500a800c500c90115
0126012d013001d601d901f6023b0244024402a302cf02de0385038f04fc
0586fee0feebfefbff8a0007004400470058007500aa00e400ef01160120
0129016a017301e3027e029002b4030e0310032303350341035403590388
039403c803ce047204ab04da0549056105ab0761fe6efed1ff4bff840000
00010006001e0027002c0034003700620066006a006b006c007000700072
007c0081008a008e0091009200a000ab00b800bf00c900d500dd00ec00f4
0100012101300169016a016d017c0185018e018e019901ac01c101c501c9
01e101f601f601f60222022202280236023f024302460267028502850294
02d002d602e8031c0363037f03800380039e03b603d90400040404ff0532
05320548058b05a706cb07280748076208ccfcedfd2afd59fddefe00fe1a
fe5bfe96fec1fee7ff56ff7900010025002d002e007c00870091009900a1
00a500a500aa00af00b600c600cc00d700dd00ec00f20102010501170118
0123012a012c0131013f014701490149014d01510151015501550157015a
015a0161016201680168017f0180018201830184018d0195019501950198
019901a501a901b601b601b701ba01ba01d501df01e601ea01f202000200
0203021702250227022f0239024302430247024f025202520267026f026f
027002720276027e02a702b302b902d603130325032d03610371039903ae
03c203d403f90402042c042f043c04560467048304cf04d104d804fb051f
05450568059e05c2061b06340655066a069806af06e806fc070607500762
077c07d407ff082500ad00c700aa00b5000000000000000000000000002f
06cf01730514047802df009c0018037005870155002500060254036c038e
03d2056601f0032001da018a0369036bffa3034602f8036f015602bf0122
031f053a0366008c00ff01ab02e102f402e70415015402e90128049101b7
026f034302060000000005d30415048305e8000002d7003a027d01c002c5
03830383ffbd003a059e01df059e02d1002004e0021300df01c001870297
000000ce0269028b0058043405fb0069015a01a905780182013e0288012a
03d4049e00e5032302f301f00196007a00cd014a0424025e023901ab00cf
00fd011e00ed017100700195004001bb01dd01b8000101a803a7014c020c
018d01b0020d0137010000cd032101d4030a005900000000012602150150
02f0025503bc06d00335010100d000d2007a01030130007c000000000000
000000fe006e006600940227002b0045004d00d3013200180097004100f4
febcffe9001605d8058b009100a1032c00520030005d02cb003a009200e5
00e500580086003200ba0099008800300298007cff8001640028004d0065
000200b8016a002f010b001100170100007f00040016022200a6005f0000
00f8000a00ca0043004b01ee0077012000f401c00028045f0000008c0445
00c20060007b008b008b0064005d00c2009c009206b505d3004f01170000
0420fe9e00cc00dc005e004600e30032001a003c0091005a00a1042c0041
002000490071009c009cfe4800400040008600cb0102007d003a003e006a
0050044800290096ff6a0097006900e0004c001b00c90069ff970043ffbd
0052ff83ff8b005fffa1ff5c00670053ffa8002a0076ffb2003600870559
0256052b043400de00c901c4004800db018b00b3004800da011601250118
00ea00ea00ae0000003e05bb008a04d70053003fff8cffd5001500280022
00990062004a00e4006d00ee00e5004803c00033fe4e02b1ff4603700079
05df0051ffa7ff1f010a0068ff6c004f00bc00a5070500ab0080001e05a5
00256c6540425554403f3e3d3c3b3a393837363534333231302f2e2d2c2b
2a292827262524232221201f1e1d1c1b1a1918171614131211100f0e0d0c
0b0a090807060504030201002c4523466020b02660b004262348482d2c45
2346236120b02661b004262348482d2c45234660b0206120b04660b00426
2348482d2c4523462361b0206020b02661b02061b004262348482d2c4523
4660b0406120b06660b004262348482d2c4523462361b0406020b02661b0
4061b004262348482d2c0110203c003c2d2c20452320b0cd442320b8015a
51582320b08d44235920b0ed51582320b04d44235920b09051582320b00d
44235921212d2c20204518684420b001602045b04676688a4560442d2c01
b10b0a432343650a2d2c00b10a0b4323430b2d2c00b0172370b101173e01
b0172370b10217453ab10200080d2d2c45b01a234445b01923442d2c2045
b00325456164b050515845441b2121592d2cb00143632362b0002342b00f
2b2d2c2045b0004360442d2c01b00643b00743650a2d2c2069b04061b000
8b20b12cc08a8cb8100062602b0c642364615c58b00361592d2c45b0112b
b0172344b0177ae4182d2c45b0112bb01723442d2cb01243588745b0112b
b0172344b0177ae41b038a45186920b01723448a8a8720b0a05158b0112b
b0172344b0177ae41b21b0177ae45959182d2cb0022546608a46b040618c
482d2c4b53205c58b002855958b00185592d2c20b0032545b019234445b0
1a23444565234520b00325606a20b009234223688a6a606120b01a8ab000
527921b21a1a40b9ffe0001a45208a54582321b03f1b235961441cb11400
8a5279b31940201945208a54582321b03f1b235961442d2cb11011432343
0b2d2cb10e0f4323430b2d2cb10c0d4323430b2d2cb10c0d432343650b2d
2cb10e0f432343650b2d2cb11011432343650b2d2c4b525845441b212159
2d2c0120b003252349b04060b0206320b000525823b002253823b0022565
38008a63381b212121212159012d2c4bb06451584569b00943608a103a1b
212110592d2c01b005251023208af500b0016023edec2d2c01b005251023
208af500b0016123edec2d2c01b0062510f500edec2d2c20b00160011020
3c003c2d2c20b001610110203c003c2d2cb02b2bb02a2a2d2c00b00743b0
06430b2d2c3eb02a2a2d2c352d2c76b802b023701020b802b04520b00050
58b00161593a2f182d2c21210c6423648bb84000622d2c21b08051580c64
23648bb82000621bb200402f2b59b002602d2c21b0c051580c6423648bb8
1555621bb200802f2b59b002602d2c0c6423648bb84000626023212d2cb4
000100000015b00826b00826b00826b008260f10161345683ab001162d2c
b4000100000015b00826b00826b00826b008260f1016134568653ab00116
2d2c4b53234b515a5820458a60441b2121592d2c4b545820458a60441b21
21592d2c4b53234b515a58381b2121592d2c4b5458381b2121592d2c014b
53234b515ab00225b00425b006254923451869525a58b00225b00225b005
25462345696048592121212d2cb0134358031b02592d2cb0134358021b03
592d2c4b54b012435c5a58381b2121592d2cb012435c580cb00425b00425
060c6423646164b807085158b00425b00425012046b01060482046b01060
48590a21211b2121592d2cb012435c580cb00425b00425060c6423646164
b807085158b00425b00425012046b8fff060482046b8fff06048590a2121
1b2121592d2c4b53234b515a58b03a2b1b2121592d2c4b53234b515a58b0
3b2b1b2121592d2c4b53234b515ab012435c5a58381b2121592d2c0c8a03
4b54b00426024b545a8a8a0ab012435c5a58381b2121592d2c462346608a
8a462320468a608a61b8ff8062232010238ab9035803588a70456020b000
5058b00161b8ffba8b1bb0468c59b0106068013a2d2cb1020042b1230188
51b1400188535a58b910000020885458b202010243604259b12401885158
b920000040885458b2020202436042b12401885458b2022002436042004b
014b5258b2020802436042591bb940000080885458b202040243604259b9
4000008063b80100885458b202080243604259b94000010063b802008854
58b202100243604259b94000020063b80400885458b20240024360425959
5959592d2cb0024354584b53234b515a58381b2121591b21212121592d35
33390001000000030000c1d8ef195f0f3cf50819080000000000a2e31dc2
00000000b9d5b528fb74fd8c1000080e0000000900010001000039300001
00000721fe4500571000fb74fe2610000001000000000000000000000000
0000068a0639011c00000000020000000200000002aa00e4034400850400
00250400006c06aa00480639004b0171005102aa005402aa002e04000091
048300250200006e02aa005302000091023900030400004a040000f00400
002c040000530400002004000062040000580400004c0400007c04000051
023900b00239008e048300250483002504830025038d005c075e006105c7
0010055600220556004a05c7002304e3002a0473002105c7004805c70023
02aa0033031d002a05c7002204e30029071d002205c7ffe505c700480473
002205c70048055600230473008004e3003e05c7000b05c70012078d001b
05c7000f05c7001304e3001a02aa00a80239000302aa004b03c100250400
ffef02aa0076038d00490400fffb038d004604000044038d004c02aa004f
0400003d0400000d0239003c0239ff63040000110239003d063900110400
000c040000450400fff90400004402aa000d031d00640239001404000002
0400001105c7000d0400001b0400000c038d002903d7011b019a00a103d7
00b10454001405c7000e05c7000e0556004a04e3002a05c7ffe505c70048
05c7000b038d0049038d0049038d0049038d0049038d0049038d0049038d
0046038d004c038d004c038d004c038d004c0239003c0239003c0239000d
023900020400000c04000045040000450400004504000045040000450400
00020400000204000002040000020400006503330062040000810400003d
0400009c02cd007003a0fff204000023061400450614004507d7001e02aa
00ec02aa003904640019071dffe805c7004905b400350464000804640018
0464001804000002049c008603f4004005b4002b0696002e0464003e0231
00000235fffa027b001d062500470556004904000027038d005902aa00e4
0483002404640053040000020464001e04e5001a04000040040000400800
00e605c7000e05c7000e05c70048071d004b05c700430400ffee0800ffed
038d0043038d004302aa00b902aa00c10464001703f4002f0400000c05c7
00130156feab0400ffe902aa007702aa007304730019047300170400008b
0200009102aa00c1038d00430800004105c7000e04e3002a05c7001004e3
002a04e3002a02aa003302aa003202aa003202aa003205c7004805c70048
05c7004805c7000b05c7000b05c7000b0239003c02aa003c02aa001602aa
001702aa003702aa00e902aa009602aa00bb02aa004e02aa009402aa003c
04e300160239001e0473007e031d006404e3001a038d0029019a00a105c7
00230400004405c700130400000c047300240400fff904830025048300a5
02660088026600140266002c06000086060000860600002a0400002105c7
00480400003d02aa003304730080031d00640556004a038d00460556004a
038d0046040000260400ffef02aa01ef05c70010038d004905c70010038d
004905c70023052c004405c7002304e3002a038d004c04e3002a038d004c
04e300290239003d04e300290340003c04e3002902c0003605c7ffe50400
000c05c7ffe50400000c05c70048040000450556002302aa000d05560023
02aa000d04730080031d006404e3003e0239001404e3003e036b001305c7
000b0400000205c7000b0400000204e3001a038d002904e3001a038d0029
04a0002505c7004c05d900470431005703c50046035c0047045000460337
000c049e00450400ffef049500e40285000207c0002c0800004f04000099
0800004f040000990800004f040000980400009807d5016a05c700c00483
002604cd00990483002604d5022204d5010505abffe905ab027e05ab027e
05abffe905ab027e05abffe905ab027e05abffe905abffe905abffe905ab
ffe905abffe905ab01c005ab027e05ab01c005ab01c005abffe905abffe9
05abffe905ab027e05ab01c005ab01c005abffe905abffe905abffe905ab
027e05ab01c005ab01c005abffe905abffe905abffe905abffe905abffe9
05abffe905abffe905abffe905abffe905abffe905abffe905abffe905ab
ffe905abffe905abffe905abffe905ab02d605ab006605abffea05d5ffff
04d500920800000007eb013007eb012007eb013007eb012004d500b204d5
008004d5002a082b0198086b01b807550010060000f40600006f0440003a
0540003704c0003f04150040040000250600005505ab002f046b003b04d5
000301c00089035500a206ab003403d5006404d5009202d6008302d60083
04d500b202d6007005c70010038d00490556004a038d00460556004a038d
004604e3002a038d004c04e3002a038d004c04e3002a038d004c05c70048
0400003d05c700480400003d05c700480400003d05c700230400000d05c7
00230400000d02aa00160239ffde02aa00170239ffdf02aa00330239fffe
02aa003302390039031d002a0239ff6305c70022040000110400001104e3
00290239003d05c7ffe50400000c059d002603f5000c05c7004804000045
05c70048040000450556002302aa000d04730080031d006404e3003b0239
001005c7000b0400000205c7000b0400000205c7000b0400000205c7000e
04000002078d001b05c7000d05c700130400000c0239001605c7000f038d
0049071dffe80556004905c7004904000027023900b2078d001b05c7000d
078d001b05c7000d078d001b05c7000d05c700130400000c02aa00b802aa
ffdb0400003d04cd005a060000860600002a060000310600002502aa00c3
02aa00bb02aa00ec02aaffea05c70010058dff5c0677ff5c034aff5c05c7
ffb60687ff5c05f2ffb30227ffb105c70010055600220525003204e3002a
04e3001a05c7002302aa003305c7002205cd001c071d002205c7ffe50525
004f05c7004805c700250473002204a8002004e3003e05c7001305c7000f
05e7001805f2003c02aa003205c7001304310057035c0047042f000b0227
002503f6fffa0412006e0389000003500046042f000b03d5005102270025
0408001503e10019044a0074039effd3039100460400004503fe0059032b
004603f6fffa038d00180502001c0544004b0227000003f6fffa04000045
03f6fffa0544004b04e3002a0604003704a000250548004b0473008002aa
003302aa0032031d002a06fa000d06fa002705ee00360556002505aa001a
05c7002505c70010049800240556002204a000250575001a04e3002a072b
00120402002b05c7002505c7002505560025056d0012071d002205c70023
05c7004805c70025047300220556004a04e3003e05aa001a0652004c05c7
000f05c700250533fffa081200390812003905a6003606fa002504980024
0548003a083900260556ffee038d00490412004e03c700300348001f0412
001a038d004c05870017032900180448002e0448002e03e3002e03fe000c
0510002e0448002e040000450448002e0400fff9038d0046037f000c0400
000c052f00570400001b0448002e0406001e0629002e0629002e0423000c
0560002d03a6002e036f001b05fa002d03aeffff038d004c03dd00110348
001f036f0046031d00640239003c023900020239ff6305d1000c05c9002d
0400000d03e3002e0400000c0448002e039a002502cf001f0800004107a2
0010040a000d02aa010102aa001c02aa003202aa001202aa010202aa008f
02aa008f02aa008f02aa009002aa010202aa001c02aa010202aa012102d9
005602aa008f025400e002be02af02beff6b023900b003da005f03a40033
02af0021035a004303c5004e023b0043024a004e03d0005803ce00430222
0043039e0043037600330374000f040f006403e2004e0232004302700021
03cd005f03a2004303a200430386005803dc004303ae003d03ca006903c0
004304e200430400002104750043045d00430444004301ac006b02f9006b
06360096023bff9d039e0043039e00430374ff5b0374ff5b03a2003304e2
004304e2004304e2004304e2004303da005f03da005f03da005f03a40033
02af0021035a004303c5004e023b00430279000c03ce004302220043039e
0043037600330374000f03e2004e0270002103cd005f03a2004303860058
03ae003d03ca006903c0004304e2004304000021023b004303a400330376
0033038600580404000f0000ffdc0000ff250000ffdc0000fe51028d00ab
028d00a002da0043034d007901a8ffba019c004601e50046019c0046019c
004601ad0048019c004601b10046015100460435017c0435012e043500b7
043500810435012c043500be043500af043500810435009a043500db0435
0085028d00c1043500b3060001000600010002420036060001000435009e
04350098043500cb060001000600010006000100060001000600010001b1
004606000100060001000600010006000100060001000600010006000100
06000100051bffba06000100060001000600010005b5003a05b5003a01f4
ffba01f4ffba060001000600010006000100060001000481003604350036
043dffba043dffba03e9004a03e9004a067f0014077600140327ffba041e
ffba067f0014077600140327ffba041effba051b003204b5002406000100
060001000600010006000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
01cf003001b1004601b1004601b1004001b1004606000100060001000600
010006000100060001000600010006000100060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
01000400001b080000000600010006000100060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
0100028d007f028d005d0600010004ee0015034d007901a8000e01d6ffdc
01a8005601d60010037500320375003201a8002d01d60013051b003204b5
002401f4ffba01f4ffba01a8009301d6001305b5003a05b5003a01f4ffba
01f4ffba024200000300fff705b5003a05b5003a01f4ffba01f4ffba05b5
003a05b5003a01f4ffba01f4ffba0481003604350036043dffba043dffba
0481003604350036043dffba043dffba0481003604350036043dffba043d
ffba02b3005f02b3005f02b3005f02b3005f03e9004a03e9004a03e9004a
03e9004a0692003e0692003e043fffba043fffba0692003e0692003e043f
ffba043fffba08c9003e08c9003e06c5ffba06c5ffba08c9003e08c9003e
06c5ffba06c5ffba04a7ffba04a7ffba04a7ffba04a7ffba04a7ffba04a7
ffba04a7ffba04a7ffba045a002a039a00360435ffba0327ffba045a002a
039a00360435ffba0327ffba064f0027064f00270224ffba021affba04a7
004604a700460224ffba021affba04cf002d04cf002d0327ffba0327ffba
040d0047040d004701a8ffba01a8ffba02b4002302b400230327ffba0327
ffba043500450435004501f4ffba01f4ffba024200360300fff7039affba
0327ffba0375003203750032051b003204b50024051b003204b5002401f4
ffba01f4ffba045a004004ce0040045a002604ce0030045a005304ce0041
045a005304ce00410600010006000100019c0046019c0046060001000600
0100060001000151004601b10046060001000600010001ad004801e50046
06000100060001000600010001b1004601b1004601b1004601b1004601b1
004001cf003006000100019c0046019c0046060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
060001000600010006000100060001000600010006000100028d00ca028d
00c7028d00c6060001000600010006000100060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
0600010006000100060001000100ffba0800ffba1000ffba05c70048043b
00450635000b045600020000fdcc0000fc140000fd130000fe420000fce0
0000fdd40000fe620000fe2b0000fdb70000fc980000fd880000fc080000
fcfe0000feff0000ff030000fe9e041a00a206000088060000140000fe70
0000fdd40000fdf60000fd770000fe620000fdbb0000fbd80000fbd80000
fb740000fcfe0000fc8c0000fc460000fd270000fcb40000fca80000fcae
0000fc440000fe140000fe700000fd910000fc710000fdc30000fe470000
fe620000fcc30000fde10000fd870000fd4b0000fd970000fd4b0000fc8a
0000fc620000fc090000fbd70239003c05c70010038d004905c70010038d
004905c70010038d004905c70010038d004905c70010038d004905c70010
038d004905c70010038d004905c70010038d004905c70010038d004905c7
0010038d004905c70010038d004905c70010038d004904e3002a038d004c
04e3002a038d004c04e3002a038d004c04e3002a038d004c04e3002a038d
004c04e3002a038d004c04e3002a038d004c04e3002a038d004c02aa0033
0239003c02aa00330239003c05c700480400004505c700480400004505c7
00480400004505c700480400004505c700480400004505c7004804000045
05c700480400004505c70048043b004505c70048043b004505c70048043b
004505c70048043b004505c70048043b004505c7000b0400000205c7000b
040000020635000b045600020635000b045600020635000b045600020635
000b045600020635000b0456000205c700130400000c05c700130400000c
05c700130400000c05c70010038d004902aa00330239000605c700480400
004505c7000b0400000205c7000b0400000205c7000b0400000205c7000b
0400000205c7000b040000020000ff090000ff090000ff090000ff0904a0
00230348001f072b0012058700170556002503e3002e0556002503e3002e
05c700230448002e05c700130400000205c700130400000205c7000f0400
001b0533fffa0406001e053300250400000d05c7002b038d004c05c70048
0400004505b5003a01f4ffba0224ffba021affba04a7004601f4009e01f4
001001f4001b01f4001001f4006b01f4fff90227ffce01a8000f01a8fff5
02aa00a402aa00a401a8000e01a8005601a800560000ffcf01a8000f01d6
ffbf01a8fff501d6ffcd01a8001d01d6fff501a8009301d6001303750032
037500320375003203750032051b003204b5002405b5003a05b5003a01f4
ffba01f4ffba05b5003a05b5003a01f4ffba01f4ffba05b5003a05b5003a
01f4ffba01f4ffba05b5003a05b5003a01f4ffba01f4ffba05b5003a05b5
003a01f4ffba01f4ffba05b5003a05b5003a01f4ffba01f4ffba05b5003a
05b5003a01f4ffba01f4ffba0481003604350036043dffba043dffba0481
003604350036043dffba043dffba0481003604350036043dffba043dffba
0481003604350036043dffba043dffba0481003604350036043dffba043d
ffba0481003604350036043dffba043dffba02b3003202b3003202b3005f
02b3005f02b3005f02b3005f02b3003202b3003202b3005f02b3005f02b3
005f02b3005f02b3005f02b3005f02b3003802b3003802b3004902b30049
03e9004a03e9004a03e9004a03e9004a03e9004a03e9004a03e9004a03e9
004a03e9004a03e9004a03e9004a03e9004a03e9004a03e9004a03e9004a
03e9004a0692003e0692003e043fffba043fffba0692003e0692003e043f
ffba043fffba0692003e0692003e043fffba043fffba08c9003e08c9003e
06c5ffba06c5ffba08c9003e08c9003e06c5ffba06c5ffba04a7ffba04a7
ffba045a002a039a00360435ffba0327ffba064f0027064f0027064f0027
0224ffba021affba064f0027064f00270224ffba021affba064f0027064f
00270224ffba021affba064f0027064f00270224ffba021affba064f0027
064f00270224ffba021affba04a7004604a7004604a7004604a70046067f
0014077600140327ffba041effba067f0014077600140327ffba041effba
04cf002d04cf002d0327ffba0327ffba04cf002d04cf002d0327ffba0327
ffba04cf002d04cf002d0327ffba0327ffba067f0014077600140327ffba
041effba067f0014077600140327ffba041effba067f0014077600140327
ffba041effba067f0014077600140327ffba041effba067f001407760014
0327ffba041effba040d0047040d004701a8ffba01a8ffba040d0047040d
004701a8ffba01a8ffba040d0047040d004701a8ffba01a8ffba040d0047
040d004701a8ffba01a8ffba043500450435004501f4ffba01f4ffba0435
0045043500450435004504350045043500450435004501f4ffba01f4ffba
04350045043500450481003604350036043dffba043dffba024200360300
fff7031a001a031a001a031a001a03750032037500320375003203750032
037500320375003203750032037500320375003203750032037500320375
003203750032037500320375003203750032051bffba04b5ffba051b0032
04b5002401f4ffba01f4ffba0375003203750032051b003204b5002401f4
ffba01f4ffba051b003204b50024067f0045067f0045067f0045067f0045
01a800280000fe290000fea20000ff300000ff1d0000ff120000ff920000
fe7e08fc003208ad00320000ffb50000ffb60000feed0000ff640000fe7e
0000ff9f018d000002f6fffd0000fe820000ff1004cd00320000ff580000
ff580000ff640692003e0692003e043fffba043fffba08c9003e08c9003e
06c5ffba06c5ffba045a002a039a00360435ffba0327ffba034d007902b4
00230242003601f4ffba0290ffba01f4002f01f4003b01f4001201f400b1
01f4006d067f001407760014022200430000fee702bc000004440043045a
fff504cefff5045a005304ce0041045a005304ce0041045a005304ce0041
045a005304ce0041045a005304ce0041045a005304ce0041043500710435
00ad045a000f04ce000f0000000000000076000000760000007600000076
000000760000007600000076000000760000007600000076000000760000
007600000076000000760000007600000114000001140000016c0000016c
0000016c0000016c0000016c0000016c0000016c000002f8000004720000
056800000568000005680000056800000568000005680000056800000568
000005680000056800000568000005680000056800000568000005680000
071800000718000007180000071800000718000007180000071800000718
000007180000071800000718000007180000071800000a1200000a120000
0a1200000a1200000a1200000a1200000a1200000a1200000a1200000a12
00000a1200000a1200000a1200000a1200000e0c00000e0c00000e0c0000
0e0c000011ec000011ec00001684000019b400001c6a00001c6a00001c6a
00001e4600001e4600001e4600001e4600001e4600001e46000020760000
2076000022cc0000257000002570000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d2000029d2000029d20000
29d2000029d2000029d2000029d2000029d2000029d2000029d2000029d2
000029d2000029d2000029d2000029d2000029d200010000068a00f2003c
0076000700020010002f0056000005caffff00030002ba0054ffc003e1b3
45453240b803e1b32b2e3240b803e1b2282932b9ffc003e1b21a1c32bd03
e102ac0027001fffc003dfb2161b32b9ffc003deb2424232b9ffc003deb2
363832b9ffc003deb32a2d32df410a03de00ef03de000203de03df002800
1fffc003dfb3282e32f0410d03df0001037e000f0101001f00a003dd00b0
03dd0002004003dab32426329fbf03cc000103ca03c90064001fffc003c9
b20d1132410a03c703b70012001f03b603b50064001fffc003b5b30e1132
004173038d000100c0038d00d0038d00e0038d00f0038d0004006f03a700
7f03a7008f03a700af03a70004000f03a7001f03a7002f03a7004f03a700
0403ab03ab00ef03a50001000f03a5002f03a5006f03a5008f03a5000400
5403aa0001006b03aa000103a8036a0022001f038c03940015001f038b03
930015001f03a40393001a001f03a20394001e001f03a10393001e001f03
9f0394001e001f039b0394001a001f039a0393001e001f03990394001600
1f039803940016001f03970393001b001f03960394001b001f0395039300
1b001f03760375001a001f03740375001a001f03a00373b21e1f10411e03
930020039300300393000300200394003003940040039400030000039400
010383036c001e001f03b1036c0032001f036d036c0032001fffc0037db2
212332b9ffc0037db3171932a0410a037d00b0037d00c0037d00d0037d00
04ffc0037cb2212332b9ffc0037cb3171932a0412d037c00b0037c00c003
7c00d0037c00040030037300400373000200000373001003730020037300
0300e0037300f00373000200b0037300c0037300d0037300030084037300
90037300a0037300030377036a0029001f0389036ab2281f40b80367b339
40323fbb0366000100400366b3191d328fbb0366000100400366b3090a32
40b80366b3090e3240b80366b3090f323fbb0365000100400365b3090c32
40b80365b31a1d3240b80365b3090e326b410e0363007b03630002001403
6300240363003403630044036300040363b2242f1fba034e006d0800400e
1f7f027f037f047f050430440112bf033200500800001f0012032d003c08
0040291f5f3c01376009700980090310092009300940095009056f037f03
8f03031f032f033f034f035f0305b8ffc0b2073a33b8ffc04047063a3390
0ba00bb00bc00bd00b05b006c006d006e006f00605200630064006500660
06700680069006a006099006900702600b700b800b03100b200b300b400b
500b051f0701a04185036200010000036200100362007003620090036200
0400f0035f00010020035e0020035f0030035f0040035e00040000035e00
00035f0010035f00d0035e00e0035f00050010030f0020030f0030030f00
d0030f00e0030f00050000030f0010030f0050030f0060030f0070030f00
d0030f00060000030f0010030f0020030f0030030f00e0030f00f0030f00
06030f00270000030e0030030e000200e0030e00f0030e0002030e004a00
e0030d00f0030d0002030d002700d002fc0001001002fc002002fc005002
fc000300d002fc00e002fc0002000002fc001002fc002002fc003002fc00
5002fc006002fc000600e002fc00f002fc0002002002fc003002fc004002
fc000302fc406127c02901b02901a02901902901403c3f413240223f4132
1212125f235f255f285fa5046f236f256f286fa5044f234f254f284fa504
3f233f253f283fa5042f232f252f282fa5041f231f251f281fa5048f4caf
4cbf4ccf4c045f4c6f4c7f4c0337b8ffc0b3b22b3032b8ffc0b3b2222532
b8ffc0b5b2191a32370f413b02af0001005f02af009f02af00df02af0003
001f02af002f02af003f02af006f02af000402af02af001f02ad002f02ad
003f02ad004f02ad005f02ad000500df02ad0001000f02ad001f02ad003f
02ad005f02ad009f02ad0005005f02ad00df02ad0002000f02ad001f02ad
003f02ad0003004002acb23a334f414a02ac005f02ac009f02ac0003002f
02ac003f02ac0002000f02ac003f02ac00af02ac000300b002ac00e002ac
0002004f02ac005f02ac00a002ac0003001f02ac002f02ac003f02ac0003
000f035a0001000f035a001f035a003f035a005f035a0070035a000500cf
035700df03570002000f0357001f03570070035700af03570004035a035a
0357035702ad02ad02ac02ac032c400d31151f0016160000001211081041
10020c004a000d01a8004a000d0198004a000d0189004a000d013f004a00
0d0124400e4a0df64a0dbe4a0d864a0d274a0dbe02280041000d01940041
000d0121400b410db4410d4f410d29410d411002170021000d0215002100
0d02060021000d01eb0021000d014e0021000d012c4014210df9210df321
0df1210d9d210d71210d3d210d4110021c001f000d0214001f000d020b00
1f000d0196001f000d014a001f000d0126400b1f0dc61f0d571f0d371f0d
410d019e0141000d00420141000d001e0141000d001b0141000d01f2b40f
440f0009bb01f20044000d0201b23c291fb80200b23c291fb801ffb23c41
1fb801feb23c471fb801fdb23c9e1fb801fab23c931fbc01f9010f010100
1f01f6b224e41f411501f401490401001f01f301490401001f01f1014900
ab001f01f001490067001f01a6003c0125001f01a4b23c811f411501a301
0f019a001f01a200220801001f01a100500401001f019f0149019a001f01
9d01490067001f019cb22c621fb8019bb22c791fbc019a002c0101001f01
97b22ce41fb80193b22c891fb80192b22c6c1fb8018fb2259e1fb8016ab2
3c2a1f4111016700240201001f0163002502ab001f014c010f019a001f01
480149006c001f0147b22c891fb80145b22c9e1fb80144b22c791fb80143
b223311fb80127b23c811fbc012300500101001f011fb223e41f4115011d
0023019a001f011c00230801001f011b00250801001f010e010f0401001f
010d00220401001f0108b223811fb80106b425e41ff73cbb0125001f00f5
010fb29e1fe3bc01490156001f00e20149b2ab1fd1b901490401b21fcf2c
b80125b61fce23bb1fc524b80156b21fc02cb80801b21fbf2cb80201b51f
b124e41fb0b901490201b61faf2c671fad23b80801b21fa523b80201400b
1f9f3c2d1f9b235a1f9925b80201b21f812cbc0401001f006d010f015640
0b1f592c3e1f4c3cab1f4625b80101b21f403cb80125400a1f3a23721f39
3cab1f38b80149b3ab1f3124b80401b21f3025b802abb61f2a24e41f2623
b80156b21f5537ba023500070175402c0774076207560751073b0733072d
0720071d071c071408120810080e080c080a080808060804080208000814
b8ffe0402b00000100140610000001000604000001000410000001001002
000001000200000001000002010802004a00b013034b024b534201b0124b
004b5442b0372b4bb807ff52b0382b4bb008505b58b101018e59b0382bb0
0288b801005458b801ffb101018e851bb0124358b90001012f858d1bb900
01017c858d5959014bb0c063004b6220b0f65323b8010a515ab005234218
0016763f183f123e113946443e113946443e113946443e113946443e1139
4660443e11394660442b2b2b2b2b2b2b2b2b2b2b182b2b2b2b2b2b2b2b2b
2b2b2b2b181db0964b5358b0aa1d59b0324b5358b0ff1d594bb04753205c
58b90271026f4544b90270026f45445958b9017a0271455258b90271017a
4459594bb04753205c58b9002202704544b9003c027045445958b901b300
22455258b9002201b34459594bb04c53205c58b9014900224544b1222245
445958b901c20149455258b9014901c24459594bb06753205c58b9002402
714544b90050027145445958b9021e0024455258b90024021e4459594bb8
020153205c58b9010f00224544b1222245445958b90c00010f455258b901
0f0c004459594bb01c53205c58b125254544b12c2545445958b137254552
58b125374459594bb0ab53205c58b125254544b1232545445958b9015900
25455258b9002501594459594bb8010153205c58b125254544b128254544
5958b902080025455258b9002502084459592b2b2b2b2b2b2b2b2b2b2b2b
2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b
2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b
2b2b2b2b2b65422b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b
2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b01b361dc646345652345
6023456560234560b08b766818b080622020b164dc4565234520b0032660
62636820b003266165b0dc236544b064234420b161634565234520b00326
6062636820b003266165b063236544b0612344b10063455458b163406544
b26140614523614459b3a67f434b456523456023456560234560b0897668
18b080622020b1437f4565234520b003266062636820b003266165b07f23
6544b043234420b1a64b4565234520b003266062636820b003266165b04b
236544b0a62344b1004b455458b14b406544b2a640a645236144594b5242
014b5058b108004259435c58b108004259b3020b0a124358601b21594216
10703eb0124358b93b21187e1bba040001a8000b2b59b00c2342b00d2342
b0124358b92d412d411bba04000400000b2b59b00e2342b00f2342b01243
58b9187e3b211bba01a80400000b2b59b0102342b0112342002b00184569
44456944456944456944737373747373737475752b737374747518456944
7373742b4bb021534bb046515a58b03cb03c45b040604459012b2b2b2b75
7575757575757543584010bf3ccf3c026f3c7f3c8f3c9f3caf3c05757559
43584012bf22cf22025f226f227f228f229f22af2206757559435c58b640
3c9f22ef220375592b2b0174747474454473737474757545447345447374
4544737475737373737300757575737575752b2b757575752b752b435841
220063032d00010003032d0013032d0023032d0033032d0053032d000500
c3032d00d3032d00e3032d00f3032d00040083032d0093032d00a3032d00
b3032d0004032d032d4518694474747575592b4358b900180332b3303532
38b80332b361663238b80332b3535a3238b80332b3454e3238b80332b33c
413218b80332b23f330a410f0332000100ba033200ca033200da033200ea
033200fa03320005033203324518694474752b2b2b2b2b2b597300732b01
2b7575002b2b2b74002b2b2b732b74012b002b2b017373737474732b2b00
732b2b002b2b2b017374732b012b2b012b2b2b2b2b2b2b2b2b2b2b2b2b2b
00017375007373004569440073730173742b2b2b2b2b732b00732b752b2b
732b2b2b2b2b2b2b2b2b2b6e00>
[10707 ] AllocGlyphStorage
]def 
108 44 
PrepFor2015
Type42DictEnd
1 0 0 <0002011c0000051c050000030007004db10201bb02be0006000702bfb200
0504b802beb403000a0704b802beb5010019080605bf02be000200030129
0009016b015e00182b10f63cfd3c4e10f43c4dfd3c003f3cfd3c10fc3cfd
3c31302111211125211121011c0400fc2003c0fc400500fb002004c0>/EKJCLI+TimesNewRoman AddT42Char 

1 0 3 <> /EKJCLI+TimesNewRoman AddT42Char 
1 118 15 <0001006efeab019800c800170053402759025917c4160309176019d01903
0901000704040f081200b612400c0b043a0f151f1580150315b8012a400b
1f0f5f0f020f19189ca4182b4e10f45d4dfd5ded003fede4123901111217
393130015d01711335363635342726232207062322263534363332161514
066e67710907070b251214313a4b3642678ffeab2c228f50130d0914093a
333146735f67b100>/EKJCLI+TimesNewRoman AddT42Char 
1 276 17 <00010091ffe4016f00c2000b002b401c0040060b034009403a3509403f35
5f09019f09af090209850c6a7a182b10f671722b2bed003fed3130253216
15140623222635343601002f40412e2e4141c2412e2e41412e2f4000>/EKJCLI+TimesNewRoman AddT42Char 
1 364 24 <00010062ffe80379054c0021011e4043a4040112591e691e7f057f067f1d
8c048d1d07350235215503552057216b1c7605791c87028a1a8a1ca303a8
09a023e0230f0023010f1011121315161708140d020303b8011c40112021
1420030420211a1b1c030718040503b8019fb320202113ba01f900180313
400c0d0d01e20002e22121000400ba013e001b0147b58007a0070207b801
f5400a40230140236023022316b801f9b61002a021012103b8019f400920
4010a01002101922ba019501e900182b4e10e45d4d10ed105d3c10ed105d
71f65dede4003f3c10ed10ed3feded12392fed0111391112173987082e2b
057d10c40011121739b10602435458400d72017202722082018202822006
005d59313001715d005d435c58400b6b046f12641e7005701d055d59015d
010721070417161514060607062322263534363332161716333236353426
2726270103794efe685901099b8557845173797a6f2e231a272f4b4d75b1
9e8b6dbc0104054caab6279e88b86bb680273753321c2b102134b17f7bd5
3a2d07020f00>/EKJCLI+TimesNewRoman AddT42Char 
1 760 25 <00020058ffe803b105680018002800fc402a7509760a770e8209d925e925
060603017d037a047a168517043c0828060503231928190603205f080108
b80143b620260126260f01b8018db318000520b80106b30f0d0100ba0140
0023010f40120b1a002a402a02402a602aa02ae02a042a19ba013e001b01
0f4012001310132013301340139013a01307131929ba011e010100182b4e
10fc5d4dfde44e105d71f64dedf43c003fed3f3ced12392f5ded72121739
0111121739b10602435458b40b061b0602005d5931304379402c1c250912
1d1c1e1c020611250d2625092362011f101b6200210e236201240a266201
1c12206200220c206200002b2b2b012b2b2b2b2b2a8181005d01715d0115
0e0307363332161514070623222726113412243633010615141617163332
36353426232206039684a7a36b2490918bcc677ccc8b61be92010ff86bfd
cc12474633495789887d26570568250d4fa2c78963e0b0aa8caa5cb3011d
b60148fe58fd44875360e1422fa498abfa20>/EKJCLI+TimesNewRoman AddT42Char 
1 1138 26 <0001004cffe403a5054c000b00c1b90004ffe0b3131b3e05b8ffe0402b13
1b3e19080105032a094200400d600da00dca01c902d801d802e00d0b1a00
010b01000d400d0302050404b80193401a03021403030204030d05404735
05e2010640473506e201000400b80199b6a00b010b190c05ba02e8000302
e7400c0004100440045004a0040504bc02e6000c011e010100182b10f65d
ede44e10f45d4df4003f3ced2b10ed2b3f3c87052e2b870e7dc4b1060243
54584009740574068405840604005d5931300171725d0072012b2b132115
012301212207060727ce02d7fe3c700195fe8b713054331d054c26fabe04
c51b2e600b00>/EKJCLI+TimesNewRoman AddT42Char 
1 1384 41 <000100210000041f054c002d012ab1282fb8011e40372564360904090ab0
2f03982bba2bc62bd903d32be904e90afb04fb0a09700570067f077f0880
0580068f078f0808070a092a0207210c0cb80126400d081b071d1f1b1721
2206210202b801264029051b060e1f1b1621231e1f1b2621232b2c280a08
0c0405020201230c0d0d172d002326002810280228b802d3402527272602
161708272b28ac002901002930294029702904299006061f07014f0701bf
070107b801b5402e000e06131302550e0c0f0f02550e0c0d0d02550e221e
1d0c101002551d0c0f0f02551d1a0d0d02551d9e2e6163182b4e10f42b2b
2b3c4dfd2b2b2b3cf45d71723c10f65d71fde4003f3c3f3c10ee5d10fd3c
12392f3cfd3c111239111239011112392b2b0110edec0010fd2b0110edec
0010fd313000715d015d712b0111333236373311232e0223231114171617
16333315213533323736351134272627262323352113232e022301a3f755
4f0d252501274544f70d0a202c3031fdba305426180d0a1f2b313003f10d
231a45656a0502fdeb4b6ffe354f4a25fe566721191218252531207a036c
672119121825fed65f592800>/EKJCLI+TimesNewRoman AddT42Char 
1 1816 54 <00010080ffe10405056b00380257401912952c010f010f020b03000f0428
0029052b4f014f0209113ab8014640d03638361a031b045f185f195f1a5f
1b06050d050e002ac03a04740b740d740e760f701e701f702f7030890886
0b870d870e840f872ba804a83310120d330d340d351d331d341d352f012f
022d04201e201f29292d333e013e023f043019301e301f30213d343d3548
0d482a540b560d57105629562b1d1f011f021b331f351b3654185419541a
59325c335c345c355c365a370e030b0b29130b1b29230b203a3b29303a72
12721389249807982f9930a82fc028c12ac62bc03af03a144e08381b006f
021baf01cf0102017f010101ba00b8034b400d359a311c1b1d6f1f1b1e1e
ba1db8034b4034199a142a2b2b3c0c0e140c0c0e2b0c2a0e0426092b0c2a
0e04062301fd0000062831032328140902ac01401e223401011f260126b8
012340102f11bf1102df11012011af11df110311b80287b71fac1e2b1009
0109b80123401f9f2e01bf2eef2eff2e032e404735402ecf2eef2e03002e
202e302ec02e042ebc014600390146011800182b4e10f45d5d2b71724ded
72f4edfd5d7172fd72392f2bed003fed3fed3c10ed111217390111121739
870e2e2b0e7d10c4180010ecf4ed0110edf4ed0010ecf4ed5d011071edf4
ed3130437940362430071328260b2c093300290f26330124132633010730
0933000a2d0c33000b0c2c2b27102a33010f0e292a2512233300082f0633
01002b2b103c103c2b103c103c2b012b2b2b2b2b8181015d00725d435840
09630b660d6710632b045d595d0171722b0071005d435c58400c0b180f39
04300f3933300f39002b2b2b590111232e0223220615141716171e021514
062322272626232206072311331e02333236353426272624262635343633
3217163332363703ab25125dac5c68882b3ee9be8b4befbc3b341fc31a19
1d0725251a58b56c7d91373a27fea4934ce0ad6c7938171a210a056bfe2b
87a05e7f513e334b7d666d94519adf09053f1e2f01d1929160845a32662c
1ec3748c5492d335191f2f00>/EKJCLI+TimesNewRoman AddT42Char 
1 2578 68 <00020049ffed038903af0032003d0349b1020243545840203f400d0d0255
3f4013130255151b072e25080b0b0255250c0d0d025525000c33b8fff040
0b1212025533161313025533b8ffdeb41010025533b8fff440150f0f0255
330c0d0d02553339070c0d0d0255072d2eb8ffc04020091202552e33001e
04292c30340c40090b02550c401d1d02550c40111202550cb8ffd4401e09
1202550c0c047f180118401112025518401d1d02551810251e073c2c0400
2fed3fedc42b2b5d12392f2b2b2b2bcd2ffd11123939d42bcd012f2bcd2f
2b2b2b2b2bc0c0dd2b2bc410d4cd31302b2b1b406f0b1c8a330212533601
12201f39803fa809b60a03122b127d007d3386008b0b8b35061d12163a10
3f803f04091c4c054c06452045224c3a403f891d080a0e0720002249014b
0a490b49354b37433a493d570b670b8509840a840b0f54168316021f3f5f
3f0260083300343c2e292d34bb011b000c000cffc0b609390c280b390cb8
ffc0401a3a35100c500c02400c500c600c03200c500c600c760c040c3c18
b8ffd840290b394f185f186f18032f187f1802187e1f100110251e07303c
403c023c2c04702d802d022d35292c30b803464011040b2ec02d012d6025
00330d0c0c343433b8fffcb41010065533bb016700240025ffc0401a0e39
00251f2580259025044025f0250280250125101010065525bb0243000700
15ffc0b21f3915b80167401e1b2f393107400e3920075007800703100701
f0070150070107433e436e182b4e10f45d7172722b4dedf4ed2b10fd2b5d
71722b3cfd2b3c103c103c103c10f65d3c003ff4fde45d10ed713fed72fd
5d712b11395d71722b2b2b2fb10602435458b2030c01005d59ed11123911
123939313043794047353b1c23051337383638020609080a080206212220
220206350b392000111d131c0012130f1f0d1c0122233b05391c00380834
200135340b121c101c010e22101c013a063c1c002b2b2b3c103c2b012b10
3c2b103c2b2b2a2a2a818181017201710071017172005d4358b23f12015d
59015d2b0072435c58b431400e392eb8ffe0b210392eb8ffe0b60e393720
0e3920b8ffe8b20c3920b8ffe0400b0b3918200b3917200b391cb8fff040
1a0b390a280b3937280b390a280a3937280a390a28093937280939002b2b
2b2b2b2b2b2b2b2b2b2b2b2b2b59005d5925060706232226353437363637
353426232207061517140623222635343633321716171615111416163332
3736371506232226271106070606151416333202478d24363d5f7b1e29cb
ec57533f2526022f26252fb09f7a4e3b1c120a170f100c153c7066313a01
972c4f4456384c846d1119826a433144785624896622222c3a2e32342d56
90291f422b85fec9833b14070d3c38964493015d3c192c6039485f00>/EKJCLI+TimesNewRoman AddT42Char 
1 3596 72 <0002004cffe4035303b00014001d037db10202435458402808161415000c
0f100255000e0c0f1002550e0c0d0d02550e153040000120003000020000
10000200b8ffc0b41314025500b8ffc040111111025500000b1b25110700
0710070207b8ffc0b40f10025507b8ffc0b5131402550704b8ffd6b41314
025504b8ffcab71212025504310b0b003fed2b2bc42b2b5d3fed12392f2b
2b5d5d5ded012f2b2bdd2bc02fcdc031301bb10602435458401d158000a0
00b0000320003000400003000010000200000b1b2511070807b8ffc04024
1010065510072007b00703000760078007a00704079204a204b204030431
0b0b07081614b8fff440260d0d065514141f1e15000c0d0d0655000c0f0f
0655000e0c0f0f06550e160d0d06550e0e1f1e1112392f2b2bdd2b2bc011
12392f2bcdd0cd003fed5dc45d5d2b323fed12392f5d5d5dcd31301b4019
125f185d1960006014d6030519201c3917201c3916401c391fb8ffc0400a
434a34081f430d5d361fb8ffc0b32828341fb8ffc040532a2e341b061909
58135e165f175a185b1a07010309060709080c0515490689028c06870c8a
10851da302ab18b513d402d90fda10f402f3031312600760087007800789
09c107c80ff007080401070d84020309baffe00006ffe0404a3609460247
094f1f5402540962027202891389199913a409a40ab808b509b00ac702e7
02e00cf40a1408d007010007d007027107010007100720079007a007b007
06077d041400301615b8ffc040131239125f157f159f15df150415151bd3
040104b8ffd0b2143904b8ffe8b2133904b8ffd84048123904310b0b5c1b
011b25110707cc0816281b390f16016f167f168f160316f4141480080130
0890080230088f08df08031008400860087008b008e0080608aa0e150400
89000200b8032c4012300e400e500e03000e100e200e03f00e010eb8ffc0
4009434a340e431e434b182b4e10f42b7172724dfd713c10fd5d715d713c
10ed5d712b10ed003fed723fed2b2b2b7211392f5d4358b26f15015d592b
3cfd3c10f45d5d7172393130015d00383800715d014358b4060001020271
5971722b2b2b2b2b2b2b0072435c58b90007ffc0400b23390c402d390d40
2d3908b8ffc0b2283907b8ffc0b2283906b8ffc0b21b3907b8ffc0b21b39
08b8ffc0b21b3907b8ffc0b20a3908b8ffc0b20a3907b8ffc0b2093908b8
ffc0400e093915101939192011390d201139002b2b012b002b2b2b2b2b2b
2b2b2b2b2b2b595959130617163332363717060623220235341233321615
252126272626232206da016464875a852d1f15ca98a5ebf1b69ac6fd8701
a805101963365383023bcc747463781489e10101d9eb0107cbaa3a582438
4081>/EKJCLI+TimesNewRoman AddT42Char 
1 4588 74 <0003003dfe4603db03af003b00490059039740821216509726993603002d
105b02762a765302002a062e06528b20043f374f5b6f377526705b8f048f
05831784188f358a3e83458f4b864f95179518994fb804b905b417b418c9
34c94bc05bd05be05bf05b1b1a201533103514361f5b05a7084a363f1b00
160336214a1b0019431211100f0e0d0c0b0a090913131409088025011225
b8ffdeb41214025525b8ffc0b3140c3f25b8ffc0400b120b3f9f25af25bf
250325b8019eb5582b80210121b8ffde400d12140255129f21af21bf2103
21b8ffc0b3140c3f21b8ffc0b3120b3f21b8019e4018904a014a40140c3f
4a40120b3f4a2c121202554a50140114b8010840136f08017f0801084011
14025508350699430143b80331400c194a0a2f1901501980190219bd02d2
00060009034d003c0331400a0607195101512c2c0f4dbe03300030001e03
300039004d0330401f1030016f308f309f300330180f100255300c101006
553035392e0380540154b8ffdeb40d0f025554b8ffcab41014025554b8ff
deb41010065554b8fff0400a0d0f065554251f280128b8ffc04016171a34
8f28014f287028c028d02804280e1010065528b8fff4b40f0f025528b8ff
ee4012101002552875205b305b405ba05bd05b055bb8ffc0401c0b0c345b
0e8f96460146101010065546312016010f167016cf160316b8fff2401110
100255160c11110255160c1010065516b802bd4013993f013f3130035003
02500301000310030203b8ffc0b3191d3403b8ffc0b30b0c3403b8fff4b4
1313025503b8fff4b70f10025503695a5bba01780021010ab189182b2bf6
2b2b2b2b5d7172ed72fd2b2b2b5d71ed2b72e4102b71f62b2b2b5d712b72
ed2b2b2b2b7110e4f42b2b5d72ed10ed10ed003fed723ffde610ed5d713f
10ed7210f42b5d5ded72102b2b2b5ded2b2b5d4358b4cf21df21025d592b
72f4ed5d2b2b2b4358b4cf25df25025d5972103c103c1112173911123939
111239011112393912393931304379407a4b573a4524351c1d1718010526
25323133313431030641264f262e252a265625541c011c3b1e1c004b354d
200042013f20003d053f1c00502d4d1c00522b5420014418461c01552757
1c0156571d3a1b1c011c1b3b004c314a20014b4a3536400243200001003e
043c1c014e2f511c0053295120004517431c00002b2b2b2b103c2b103c10
3c2b103c103c2b103c2b012b2b2b2b2b2b2b2b2b2b2b2b2a2b8181818181
8101725d00715d01710072435c58400a2e10120b3f351012392eb8fff0b1
1239002b2b2b590126263534363332173332161716151407060623231615
140623222706061514161716171617161615140706232227263534373637
363726263534360122061514171633323635342726010606151417163332
363534272627260135545acda08360c22b0e030605030f2b7738c4a54447
2c1f21301c70ce3d5d6f6a9cfbc1854b0b1135075f342b3901154a644434
504c624533fef82f303a64bdb4ab33349ae1014e29935988c44005060917
1a0a0506487080b614263914112007040305090d70527163925732361818
254209631f311f235e0287767a9e5742727a9f5a42fc8133582530243e7f
483416160406>/EKJCLI+TimesNewRoman AddT42Char 
1 5764 75 <0001000d000003f3058e0036028fb10202435458401d384012120255100a
110a080d0d02550a182412120255181a0d0d025518b8fff8b40f0f025518
b8ffe0400c10100255180e131302551826b8ffea401f1010025526213435
272d0121040c0c025521080d0d0255212d18121202552db8fffab40c0c02
552db8fff6b40d0d02552db8fff4b40f0f02552db8ffec400f101002552d
0e131302552d0120040f410a03e2001203e2002503e2002803e200270034
03e2400f3540090d025535360027111d2c0407003fed2f2f3fdd2bed10ed
edecec123939012f2b2b2b2b2b2bdd2b2bc010c4c63210c42b2f2b2b2b2b
2bcd2bc410c431302b1bb106024354584058341210100655351210100655
01200427343536001d2c040711270a02101006550a060f0f06550a0c0d0d
06550a18021010065518060f0f0655180c0d0d0655181838370121021010
065521060f0f0655210c0d0d0655212db8fff0b4101006552db8fff2b40f
0f06552db8fffcb70d0d06552d2d38371112392f2b2b2bdd2b2b2bc01112
392f2b2b2bcd2b2b2b002f2f3fed3fddcd111239393130012b2b1b402f38
402a350a38600d5d360f250f268038903804b038c038d038032b06015038
60387038903804403801200818291e11b8030f4011222d291e274a220a29
1e104a2321291e26b8030e402e2335272e41341e35440120273600001d2c
04072726261111100a19182409900a01b00a010f0a700a9f0acf0a040ab8
02bd40252d0021242e1f2d502d602d702d04802d902d02b02d01002d102d
c02dd02d042d6037a67f182b10f65d5d71723cfd3c10fd5d71723cfd3c00
3f3c103c103c3fed3f3c113939f5edfc01f52b2b2b2b3130437940141a1c
050806251b261c05191c0107081a071d1c012b01103c2b2b2b8181017172
005d015d712b2b5959011136363332161716151114171616331521353332
363736351134262623220607111416163315213532373636351134262623
22072725014d6f82414e701b130e0a3040fe3e1540320a031f4430316a4a
153946fe3a3d2314180f1f1a152f0e0112058efd627a45565c40aafebc57
20181c24242726104e0144965e2f344ffe1c5e2e1f2424130a3856033d9d
481a10237000>/EKJCLI+TimesNewRoman AddT42Char 
1 6580 76 <0002003c00000207058e000b00220249b10202435458b90024ffc0401d0d
0d0255120d080d0d02550d21181010025521180f0f02552113180309b8ff
eeb41313025509b8ffe0b40d0d025509b8ffd6b40f0f025509b8ffceb610
100255090d18b8fff4b41313025518b8ffe2b40d0d025518b8ffe0b40f0f
025518b8ffd6b5101002551820b803e240174f216f217f210321226f0001
0060060106400f0f025506b8ffc0b71313025506220613002f3fd62b2b5d
cd5d10dd5ded012f2b2b2b2bcd2f2b2b2b2bcd10c4c62b2b102bc4313001
2b1bb10602435458400d20121010065521121010065506b8ffc0b44b4b06
5506b8ffc0b44141065506b8ffc04019373706554006010006a006026006
0106000020212207130309b8fff6401c10100655090924230d0210100655
0d020f0f06550d0c0d0d06550d18b8fff0b41010065518b8fff6b40f0f06
5518b8fff0b70d0d0655181824231112392f2b2b2bcd2b2b2b1112392f2b
cd002f3fddcd3fcd5d71722b2b2b3130012b2b1b40199024016024702490
24a024f024052024502402402450240224b8ffc0b332323424b8ffc0b338
3a3424b8ffc0b32d303424b8ffc0b323253424b8ffc0402e191a3418291e
134a220d291e124a2321271941201e21440c190c1390060106390000220c
0713120a900901093903b8ffc0b2433503b8ffc0400f3f35036b0c0c0d19
0d2418402b3918b8ffc0401a363a34901801501801601870189018a018f0
180518b223b2a3182b10f65d71722b2bed3c103c10f42b2bed72003f3c3f
3c3fed7211123910f5edfc01f52b2b3130012b2b2b2b2b015d715d017259
590132161514062322263534361311141616331521353236363511342726
26232207272501292a3b3b2a2a3c3b7e193141fe43432e1b09071e1a1c28
0e0114058e3b2a2a3c3c2a2a3bfe21fd2056391c24241a3c550161952c20
190f2470>/EKJCLI+TimesNewRoman AddT42Char 
1 7274 79 <0001003d0000020f058e00150191b10202435458b90017fff6401d0d0d02
55140c06010701080d0d025501040f0f025501060c0c0255010cb8fff2b4
131302550cb8ffeab40c0c02550cb8ffe2b40d0d02550cb8ffd6b4101002
550cb8ffdeb50f0f02550c05bd03e2000803e20007001303e2400b131440
090d025514150007002f3fdd2b32ed10eded012f2b2b2b2b2bcd2b2b2bc4
10c410c631302b1bb1060243545840271312101006551414101006551314
1500000007010c0d0d065501021010065501040f0f0655010cb8fff0b410
1006550cb8fff4b40f0f06550cb8fff0b70d0d06550c0c17161112392f2b
2b2bcd2b2b2b002f3f3fddcd3130012b2b1bb79017c017f0170317b8ffc0
b33f463417b8ffc0403a393b340117b20d64365017014017501760177017
9017a017f017070c291e074a2201291e06272314270d41131e1444150000
07060a0001240d0cb8ffc0b33f46340cb8ffc0401a353b34900c01500c01
600c700c900ca00cf00c050cb216b2a3182b10f65d71722b2b3cfd3c003f
3c3f3cf5edfc01f52b2b3130015d0171012b012b2b017259590111141616
3315213532363635113426262322072725017b193447fe3f3f2e1a0e1f18
1a28110111058efb4156381d24241a3c5503409b471a10237000>/EKJCLI+TimesNewRoman AddT42Char 
1 7750 85 <0001000d000002b703af002801b5b1020243545840282a4013130255061f
171127040f0f025527181f0111080d0d025511040f0f025511060c0c0255
111fb8fff4b40f0f02551fb8fff6b40d0d02551fb8ffee4011101002551f
14121202551f0e131302551fb8fffc400b0f0f02551f011003181619bb03
e20018002603e2400e4f276f277f2703272807180c0307003fcd2f3fdd5d
ed10fdc011123939012f2b2b2b2b2b2bdd2b2b2bc010c4c62b10c410c431
302b1bb10602435458402301100318262728076f097f0902090c03071806
1f01110c0d0d0655110410100655111fb8fffab40d0d06551fb8ffeab40f
0f06551fb8ffeab7101006551f1f2a291112392f2b2b2bdd2b2bc010c400
2f3fcdcd5d3fddcd1112393931301b406f2002200f3202320f4002400f82
0407402a015f2a011f291e18272211291e17862327272041261e2744000a
0b2a111420100104188009010939100c010c590303000718170a5f060140
0601062e1f2a012a0011241f1f1f2001802090200200201020b020c020d0
2005206029a66e182b4e10f45d71723c4d10fd3c1072e47172003f3c3f3c
10ed72ed5d11173901111239390010f5edfc01f52b2b3130017271005d59
590115363332161514062322262322070607111417161633152135323736
373635113426262322072725014c73793748342423571512152d30130d42
3efe2b4622190a050d231a1f270a011503afcece432c27364514295efe49
4c271b24242416102311500163a03d1c0f247000>/EKJCLI+TimesNewRoman AddT42Char 
1 8310 87 <00010014fff1023c04c1001b01fdb1020243545840251d40121302551d40
101002550b0c18121202550c15130105131812120255130e1313025513b8
fff8b40f0f025513b8fff4b40d0d025513b8fff0400c10100255130b082c
0f161404b8011bb2000106003fcdfdd0cd2fedc4012f2b2b2b2b2bddc010
c62f2bcd31302b2b1bb106024354584019170c10100655160c1010065515
0c10100655160c101006551bb8ffe8b4101006551ab8ffe8b41010065519
b8ffe8401410100655700b010b0f1b01156914014914011404b8011b401c
0106082c0f0b1b0105021010065505080f0f0655050c0d0d06550513b8ff
eeb41010065513b8fff0b40f0f065513b8fffab70d0d065513131d1c1112
392f2b2b2bdd2b2b2bd0cd003fed3ffdd05d5dc010cd10c45d3130012b2b
2b2b2b002b2b1bb9000dffe840410c395f015f02023f1d99119919bf15bf
16b819e819079f1d01891a014f0c4f0d5f0c5f0df5180506181518271803
161518191a030118191a03141ba00103153004b8011b401c010330020201
060c35082c0f0b16cf15df15ef15031565141bcc000bb801ec402c200c01
0c2e2f1db01d021d000101040405241450130180130100131013b013c013
d013e0130613601cab89182b10f65d71723cfd3c103c103c105df45ded10
ed10f45d3c003ffde43f3c10ed10edfd3c10e40111173900111739123931
3000715d0171725d00722b59590111331523111416333236373306062322
2626351123353636373637014ad6d63328213e11272380442e582a913773
2d172904c1fed346fdae593e29286263335f63026821166948266500>/EKJCLI+TimesNewRoman AddT42Char 
1 8908 88 <00010002ffe403fd039400250230b1020243545840162740121202550801
080d0d0255010b20281212025520b8fffc400b0f0f0255201e0d0d025520
b8ffe4401310100255201a080d0d02551a121c1212025512b8fff8b40f0f
025512b8fffab40d0d025512b8fff4b5101002551224ba03e2001703e240
0e1825060b200e18061d2c0e0b0708b8ffc0b509100255080a002fdd2bcd
3fed3f1239393f10edec012f2b2b2b2bcd2b2f2b2b2b2bc0dd2bc431302b
1bb1060243545840570740086008700803080a0b200b180e242517182506
18061d2c0e0b0b010810100655010a0f0f0655010c0d0d065501201a040f
0f06551a04101006551a0a0d0d06551a1208082620080f0f065520060d0d
065520202612b8fff2b41010065512b8fff6b40f0f065512b8fff6b70d0d
0655121227261112392f2b2b2b11392f2b2b11392f10cd2b2b2b10cd2b2b
2bc0003fed3f3f10cd10cd111239393fdd5dcd31301b40350127600d5d36
202760277027b02704340b371f3a20481f4820051a08134f1e182723214f
1e25272308270141071e0844200b251d08b8014540130a00252519191806
1d2c0e0e0a0b0a0b0b2120b80167400e00b001010f0170019f01cf010401
b802bd402512191a241212501390130280139013b01303001310132013b0
13c013d01306136026c27f182b4e10f45d71723c4d10fd3c10fd5d713cfd
3c3c103c003f3c10ed3f3c103c103c10ed11123939f5edfc01f52b2b3130
437940101b1c0f111c0f1a1c0010111b101d1c002b01103c2b8181005d01
5d2b59590111141616333237170523350606232226263511342626073521
11141633323637113426273503630f21161f270efeee2d767c454d712c1c
37480141593f2b6d4b395a0394fdd59f471c112371c28042598c80019941
321b0125fd9b8050364c02074e370225>/EKJCLI+TimesNewRoman AddT42Char 
1 9584 90 <0001000dffe405b40394002c03cdb10202435458b626211e110e022cb803
e2400e00092618080428251f060f060006003f3f3f2f2f173910fdd0d0d0
d0c0012f31301bb10602435458b90026ffe840440d0d0655181c0d0d0655
081c0d0d065518101010065508101010065508182609040028211e110e02
792c012c00752501250b752801280b1f060f0600062c2c2d21212e2d1112
392f11392f003f3f3f3f5d3f5d10dd5dd0d0d0d0c01112173931302b2b2b
2b2b1bb1122eb8ffc0401c3f351627201020112527202e5f2e6909702ee9
25e928f825f8280c2eb8ffc0b213352eb8ffc040c81b1f34212e2e296436
1d19191f1b23102e040a261d262c2639265517a717a718a726080b253724
37274f004c014d074908472446274d284d298807801080118d2588288829
802e9a109417a718a725bb10b925b928bf2ec825c828d925d928d02e1f00
050407061504170925072709280629351743104311500552075618522989
0b8f1088188919892388258826802e17870986178726030d095901771077
110409090826262725250a0107021e011017111e102023211e2000292c1e
000f0a0e1e0f1f191e1e1fb8ff86b308282720b8ff7d4040182524200807
080907242928142929282627262527300809140808091815181915240a25
140a0a25232424301819141818192926231918170a0908070a002821bb01
ec0020001e01ecb31f010f11bb01ec0010000e01ec400a0f0f10101f1f20
200002bb01ec0001002c01ecb301000618bb016a0025000801a6400f2840
2725252424280b20fc0f650a01b801b1b4c000652923b801084015401b2f
501901a01901bd19cf19df19031992242f18b8011bb7200f250110250125
b8ffc0b30b0c3425bb0110002600150167400c400a2f5f26014026802602
26b801ecb4097d272f08ba011b0008011b400a200028018028f0280228b8
ffc0b50b0c3428a007b80167401b5029018029010029102920294029b029
c029d0290729602dab89182b10f65d7172edf42b5d71191aedfde4f4ed5d
7118f41aed1910f42b5d711afde4f45d717218e41aed10f41aed10f4ed00
3f3c103c103c1a10ed10ed3f3ced10ed103c103c103c103c10ed10ed103c
10ed10ed1112173987052e2b0e7d10c4870e2e182b087d10c487052e182b
087d10c4870e2e182b087d10c42b2b180010ed0110c00010ed0110c00010
ed0110c00010ed0110c00010ed0110c00010ed0110c00710083c083c3130
015d5d71015d005d01722b2b2b015d2b435c58b52610140c3f24b8fff0b3
140c3f13b8ffe0b21d3917b8ffe0b21d3917b8ffe0b2143917b8fff0b217
3925b8fff0b2153917b8fff0b11539012b2b2b2b2b2b2b2b595959132115
060615141713132726272627352115060706151417131336353426273521
1506070123030123012626270d0180352111c4c5341827163c01b4481e14
08d0c114273901215729fece29e5fef525feda1d383c039425041e1c1f2c
fdf101ad873c170e032525031710231415fdf201fb3620131e0225250d69
fceb0249fdb7030249330d00>/EKJCLI+TimesNewRoman AddT42Char 
/EKJCLI+TimesNewRoman findfont /CharStrings get begin
/.notdef 0 def
/space 3 def
/comma 15 def
/period 17 def
/five 24 def
/six 25 def
/seven 26 def
/F 41 def
/S 54 def
/a 68 def
/e 72 def
/g 74 def
/h 75 def
/i 76 def
/l 79 def
/r 85 def
/t 87 def
/u 88 def
/w 90 def
end
/EKJCLI+TimesNewRoman findfont /Encoding get
dup 0 /.notdef put
dup 32 /space put
dup 44 /comma put
dup 46 /period put
dup 53 /five put
dup 54 /six put
dup 55 /seven put
dup 70 /F put
dup 83 /S put
dup 97 /a put
dup 101 /e put
dup 103 /g put
dup 104 /h put
dup 105 /i put
dup 108 /l put
dup 114 /r put
dup 116 /t put
dup 117 /u put
dup 119 /w put
dup 160 /space put
pop
end

userdict /pdf_svglb get setglobal
[/N282/EKJCLI+TimesNewRoman 1 TZG
userdict /pdf_svglb currentglobal put true setglobal
 Adobe_CoolType_Utility begin ct_MakeOCF begin ct_saveCIDInit
%!PS-Adobe-3.0 Resource-CIDFont
%%DocumentNeededResources: procset CIDInit
%%IncludeResource: procset CIDInit
%%BeginResource: CIDFont EKJCFC+SymbolMT
%%Title: (EKJCFC+SymbolMT Adobe Identity 0)
%%Version: 1
/CIDInit /ProcSet findresource begin
20 dict begin
/CIDFontName /EKJCFC+SymbolMT def
/CIDFontVersion 1 def
/CIDFontType 0 def
/CIDSystemInfo 3 dict dup begin
  /Registry (Adobe) def
  /Ordering (Identity) def
  /Supplement 0 def
end def
/CIDMapOffset 0 def
/FDBytes 0 def
/GDBytes 3 def
/FontBBox [0 -220 1113 1005] def
/FontInfo 2 dict dup begin
/FSType 4 def
/OrigFontType /TrueType def
end readonly def
/CIDCount 65535 def
/FDArray 1 array
dup 0
  %ADOBeginFontDict
  10 dict begin
  /FontType 1 def
  /PaintType 0 def
  /FontName /EKJCFC+SymbolMT def
/FontMatrix [1 1000 div 0 0 1 1000 div 0 0 ] def
  %ADOBeginPrivateDict
  /Private 8 dict dup begin
  /BlueValues [-15 0 600 650] def
  /MinFeature {16 16} def
  /LanguageGroup 1 def
  /password 5839 def
  /lenIV 4 def
  end def
  %ADOEndPrivateDict
currentdict end
%ADOEndFontDict
put def
/GlyphDirectory 1 dict def
ct_GlyphDirProcs begin GlyphDirectory +
0 <10bf31704faacd68130743d1032b19039b05d30ed4559c5ecf2da4ace2ab
53168b5c58eb3d8c199cf05ae7> |
!
end
%%BeginData: 21 Binary Bytes
(Binary) 0 StartData
%%EndData
%%EndResource
 ct_restoreCIDInit /EKJCFC+SymbolMT-Identity-H /Identity-H 0 [/EKJCFC+SymbolMT] ct_ComposeFont pop end end 

userdict /pdf_svglb get setglobal
%PDF_BeginEncoding: N287 (EKJCFC+SymbolMT-Identity-H)
/N287 (EKJCFC+SymbolMT-Identity-H) /Identity-H [ (EKJCFC+SymbolMT) ]
 /Adobe-Identity [ /Serif ] 0 TZzero
userdict /pdf_svglb currentglobal put true setglobal
ct_T42Dict begin
-0.625 -0.375 2 1.008
 256 array 0 1 255 {1 index exch /.notdef put} for  /EKJCBF+Arial,Bold
Type42DictBegin
[<00010000000a000a000a000a63767420ef1f94cc000000ac0000073a6670
676d08e8ba28000007e8000005d7676c7966f52f63d90000530000001ed0
68656164cee221a800000dc00000003668686561127e12ff00000df80000
0024686d7478a006329b00000e1c00001a286c6f636100c3363000002844
00001a2c6d6178700d840193000042700000002070726570412164030000
42900000106f6764697200000000000000000000000005ba001c05ba001c
05a7001c0426001c0000ffe40000ffe40000ffe4fe69ffe405ba001cfe69
ffe402ea0000011d0000011d000000000000000000b200ac00d701280120
00b301fa001700f8011901310049000400f7000300af00fd009500140054
00960112002400160055004901040119012b008c019bff76ffe9003d0092
00a2ffb70182ffaa0016008f00c600f8001c00de04010037004e00550055
006500e903e50059ff9a00080087000b003b00520116006100d600d600f5
00000093009400be017cfff80004001400820092003c00410041ffc1fffc
002a008c049005d809b5009100bb0106ff63ff69001e0022008a022bffd6
ffdf0026005900a300ac0104012b01c004480021006b00850098011903c6
006b009500a400fe010c025d034305bf000000490056006e0077008a00aa
00ca0112015005d805f0ff7bffe70006001300280061006900e90135014d
02a5040cff3effda005b00b900c801190119011901c0045b04a7055bfe3f
ff9dffc2001500b7010a01bc01c10532058efd81ffa1ffae000c00260031
003d004e00560062008300c100c900f100f2027fff7f00480053007700c5
011d01200126012801d60219027e027e03d3002e0041005d006b0075009f
00b000b200ba00bb00bd00d600db00e000e50114011b014a0162019101f2
020c026402cf039b03b403d4040104a9001600230025002a007400a500b6
00cc00cd00cf0105012001300150016a016f0197019d01e002b002ec02f7
0408048304fb04fd0526fee0fefbff4efff50018001a004c007a007f0091
00a300b300b400ce00d500f200f300f601100138016801a101b001e001ec
02090222024f0270029602a502ad034e039103c104350442046b04cd04da
0586058b076107fefca6fe93feadfed1ffb7ffd10003000e001800260046
00690081008f00a500bf00d300d500d900dd00e20119012b0138013b015a
015e016801730188019401ad01c501d101ea01f20200020002000222023b
0244024f026f0272027e02820293029402a502cf02cf02d002da02dd02eb
02f5030503220336037103a103b003b803d003e604100426042e0431044f
045a04ff053205320547055305a805ab05c205f0063c0664067006e80782
078408ccfd2afddefe00fe68feb0feb3ffaa00080059007a0091009e00a2
00af00b400bb00ca00cc00ce00d900e000f40114011a01210127012b0139
0146014b014d0157015c01650182018701920198019b01a201ae01c501c5
01d102070222022b024102530261026502840287028d02b402b402ba02c9
02d602d802ed02f503170323032b03310349035a035b036e03710374037e
03840391039103aa03cf03d303e703e803ed04080417041e0475047a0499
04a704b404d1054c056d056d05a205bf05c005d105fc05fc0602061a061c
062f066a06a806e2070607360750078907d407f30870011c012a011a0120
0000000000000000000000000219000b001e02aa0214047f01ed0000001d
0104000f0091002b01880153011201f3003f03fe0168010e047f01ed036e
03150219041300000000064004b00000027401bb003501c5007f06020301
000004e000b201dc02e004c3023d00d50160011904a7036e05ca022100ab
0426009002bc02bb014200b4023c0256029c030001e501a800e5006b0078
0094016b017300ab01ed013a017d0137017f00d4021603530184003cffa2
02040109014901f0006e031500810464005e000000000000000000000000
000000000000000000000000000000000000013900dc00e9fe9e040d047c
012b00b80096005900ac00df01a900fa0105ffec00170003005500610004
008c00a3008500280120005d00d6007f012601190104016c06cf00b40106
00000737063e047a00f000f900e905ba042604420000ffe7fe69049e04e3
ff37ff2d01200105012000a800740068004700f200e500d900bd00a80068
0047005c0048000a0028003200410050005a0064007d00870091ffb0ff9c
ff83ff79ff6f00cb012000fa012c01fa01a000d500b8005c003c00c800c8
008f00d9018b00b300470000000000000000000000000000000000000000
000000000000000000000000000000000000000000000000000000000000
00000000fe6400c000ea01180125013203b003ed0576059005aa05b405be
05cd063100780084009b00cc00e200f4010a0120016300d100ea00f70108
01420019002c00340041003800480058006c025903bd0043011a007000d3
0028003700420050005a0064007300780082008c009c00a500bd00ce00f0
0110015c00be00d801020117012c016300ea01080041004b0055005f0073
00a60109018301b300410064001e002a00eb00fa010e01380274002c0040
0082009600b600c000cc00dc00e600f000ff010a0120012c013b01440156
016300f70057006401100136005001b10000ffb60039004e004403cc00e5
002401100042012201a400f0006000e0000e001d003905e30102002cfe4e
ff38026903bd011600ff000e00a00054001b003d01710041000f005000fd
0015014f0035fe52002c00d30000404154403f3e3d3c3b3a393837353433
3231302f2e2d2c2b2a292827262524232221201f1e1d1c1b1a1918171615
14131211100f0e0d0c0b0a090807060504030201002c4523466020b02660
b004262348482d2c452346236120b02661b004262348482d2c45234660b0
206120b04660b004262348482d2c4523462361b0206020b02661b02061b0
04262348482d2c45234660b0406120b06660b004262348482d2c45234623
61b0406020b02661b04061b004262348482d2c0110203c003c2d2c204523
20b0cd442320b8015a51582320b08d44235920b0ed51582320b04d442359
20b09051582320b00d44235921212d2c20204518684420b001602045b046
76688a4560442d2c01b10b0a432343650a2d2c00b10a0b4323430b2d2c00
b0172370b101173e01b0172370b10217453ab10200080d2d2c45b01a2344
45b01923442d2c2045b00325456164b050515845441b2121592d2cb00143
632362b0002342b00f2b2d2c2045b0004360442d2c01b00643b00743650a
2d2c2069b04061b0008b20b12cc08a8cb8100062602b0c642364615c58b0
0361592d2c45b0112bb0172344b0177ae4182d2c45b0112bb01723442d2c
b01243588745b0112bb0172344b0177ae41b038a45186920b01723448a8a
8720b0c05158b0112bb0172344b0177ae41b21b0177ae45959182d2c2d2c
b0022546608a46b040618c482d2c4b53205c58b002855958b00185592d2c
20b0032545b019234445b01a23444565234520b00325606a20b009234223
688a6a606120b01a8ab000527921b21a1a40b9ffe0001a45208a54582321
b03f1b235961441cb114008a5279b31940201945208a54582321b03f1b23
5961442d2cb110114323430b2d2cb10e0f4323430b2d2cb10c0d4323430b
2d2cb10c0d432343650b2d2cb10e0f432343650b2d2cb11011432343650b
2d2c4b525845441b2121592d2c0120b003252349b04060b0206320b00052
5823b002253823b002256538008a63381b212121212159012d2c4bb06451
584569b00943608a103a1b212121592d2c01b005251023208af500b00160
23edec2d2c01b005251023208af500b0016123edec2d2c01b0062510f500
edec2d2c20b001600110203c003c2d2c20b001610110203c003c2d2cb02b
2bb02a2a2d2c00b00743b006430b2d2c3eb02a2a2d2c352d2c76b8023623
701020b802364520b0005058b00161593a2f182d2c21210c6423648bb840
00622d2c21b08051580c6423648bb82000621bb200402f2b59b002602d2c
21b0c051580c6423648bb81555621bb200802f2b59b002602d2c0c642364
8bb84000626023212d2cb4000100000015b00826b00826b00826b008260f
10161345683ab001162d2cb4000100000015b00826b00826b00826b00826
0f1016134568653ab001162d2c4b53234b515a5820458a60441b2121592d
2c4b545820458a60441b2121592d2c4b53234b515a58381b2121592d2c4b
5458381b2121592d2cb0134358031b02592d2cb0134358021b03592d2c4b
54b012435c5a58381b2121592d2cb012435c580cb00425b00425060c6423
646164b0035158b00425b00425012046b01060482046b0106048590a2121
1b2121592d2cb012435c580cb00425b00425060c6423646164b807085158
b00425b00425012046b8fff060482046b8fff06048590a21211b2121592d
2c4b53234b515a58b03a2b1b2121592d2c4b53234b515a58b03b2b1b2121
592d2c4b53234b515ab012435c5a58381b2121592d2c0c8a034b54b00426
024b545a8a8a0ab012435c5a58381b2121592d2c462346608a8a46232046
8a608a61b8ff8062232010238ab902a702a78a70456020b0005058b00161
b8ffba8b1bb0468c59b0106068013a2d2cb1020042b123018851b1400188
535a58b910000020885458b202010243604259b12401885158b920000040
885458b202020243604259b12401885458b2022002436042004b014b5258
b2020802436042591bb940000080885458b202040243604259b940000080
63b80100885458b202080243604259b94000010063b80200885458b20210
02436042595959592d00000100000002e667e05fd8905f0f3cf508190800
00000000a2e33c1d00000000b9d5b513fafafcfd10000815000000090001
00010000000000010000073efe4e00431000fafafe261000000100000000
00000000000000000000068a0600010000000000023900000239000002aa
00b803cb00700473001204730046071d005905c7005a01e7005c02aa006b
02aa0043031d001c04ac00550239007502aa0073023900930239fffd0473
0056047300a2047300330473004d047300260473005b0473005704730057
047300530473004102aa00c902aa00aa04ac005f04ac005504ac005f04e3
006a07cd003d05c7000005c7009605c7006105c700940556009504e30097
0639006205c700960239008c0473002305c7009904e3009d06aa009105c7
009806390059055600950639005905c700960556004a04e3002c05c70093
0556ffff078d0007055600000556fffd04e3001602aa00920239fffd02aa
002604ac00730473ffed02aa002a0473004904e300870473005504e30054
0473004102aa001804e3005404e30092023900930239ffa2047300890239
0093071d007e04e3009104e3005204e3008b04e3005b031d008704730030
02aa001f04e3008d0473000b063900090473000c0473000e04000022031d
003c023d00b0031d002d04ac004305c7000005c7000005c7006105560095
05c700980639005905c70093047300490473004904730049047300490473
004904730049047300570473004104730041047300410473004102390092
0239ffe90239ffcd0239ffd004e3009104e3005204e3005204e3005204e3
005204e3005204e3008d04e3008d04e3008d04e3008d0473004403330056
047300540473000d0473003b02cd00420473fffe04e3008b05e5fff705e5
fff7080000d802aa00bb02aa0005046400310800ffaa0639003f05b40098
046400320464003c0464003c04730001049c006f03f4002c05b4007a0696
00a1046400000231000002f6002502ec001a06250037071d005804e30057
04e3006502aa00c304ac0055046400540473ffec0464001f04e5001a0473
00600473006a080000c905c7000005c700000639005908000048078d0058
0473fffc08000000040000840400006902390098023900720464003103f4
002f0473000e0556fff70156fea90473ffe002aa004b02aa004b04e3001f
04e3001f047300440239009302390075040000710800000105c700000556
009505c7000005560095055600950239006a0239ffae0239ffbf0239ffc1
06390059063900590639005905c7009305c7009305c700930239009302aa
000302aafff302aa001302aa001a02aa00cd02aa009102aa002602aa0060
02aa00a002aa000304e3000a0239000a0556004a0473003004e300160400
0022023d00b005c7fffd04e300530556fff70473000e0556009504e3008b
04ac005504ac006d02aa005b02aa001902aa002806ac005c06ac005c06ac
0028047300000639006204e300540239008c0556004a0473003005c70061
0473005505c700610473005504e30054046bffed02aa01ea05c700000473
004905c700000473004905c7009405c0005105c7fffd0556009504730041
055600950473004104e3009d0239007904e3009d0315009504e3009a03d5
009005c7009804e3009105c7009804e300910639005904e3005205c70096
031d008705c70096031d00500556004a0473003004e3002c02aa001f04e3
002c03d5001e05c7009304e3008d05c7009304e3008d04e3001604000022
04e300160400002204cf009a063900560691005604eb004e04da004e03cc
004e0579004e0392003005b9004e046bffed04d500b8032b004f08c00029
0800004f040000990800004f040000990800004f040000980400009807d5
016a05c7008f04ab005504d5009d04ac005504d5022204d5010505abffe9
050001c905ab027e05abffe905ab027e05abffe905ab027e05abffe905ab
ffe905abffe905abffe905abffe905ab01c005ab027e05ab01c005ab01c0
05abffe905abffe905abffe905ab027e05ab01c005ab01c005abffe905ab
ffe905abffe905ab027e05ab01c005ab01c005abffe905abffe905abffe9
05abffe905abffe905abffe905abffe905abffe905abffe905abffe905ab
ffe905abffe905abffe905abffe905abffe905abffe905ab02d605ab0066
05abffea05d5ffff04d500920800000007eb013007eb012007eb013007eb
012004d500b204d5008004d5002a082b0198086b01b807550010060000f4
0600006f0440003a0540003704c0003f0415004004000025060000550647
008c0473009005abffc701eb008d03d500860715002303e9001804d50092
02d6005c02d6005c04d500b202d6004d05c700000473004905c700610473
005505c70061047300550556009504730041055600950473004105560095
047300410639006204e300540639006204e300540639006204e3005405c7
009604e3009205c7000504e300190239ffba0239ffbb0239ffda0239ffda
0239ffe10239ffe20239006e02390075047300230239ffa205c700990473
00890473008d04e3009d0239ffed05c7009804e3009105c9009c04e3008e
0639005904e300520639005904e3005205c70096031d002a0556004a0473
003004e3002c02aa000705c7009304e3008d05c7009304e3008d05c70093
04e3008d05c7009304e3008d078d0007063900090556fffd0473000e0239
008d05c70000047300490800ffaa071d00580639003f04e3005702aa00c9
078d000706390009078d000706390009078d0007063900090556fffd0473
000e0239009502aaffd70473000d04cd005a06ac005c06ac002906ac0030
06ac002f02aa00bc02aa002602aa00bb03b8fff405c7ffe806d3ffbb073f
ffbb03caffbb0699ffa6076bffc806b4ff9c0239ff2905c7000005c70096
05c000000556009504e3001605c700960239008c05c700990556000006aa
009105c70098052600660639005905c7009a0556009504cd005a04e3002c
0556fffd0556000006790056066a00620239ffcc0556ffff04eb004e039c
004e04e3008e0239008204a8006c04e200900473000f03af004e04e3008e
0453004e023900930476008e0473000f04e500900473000b0390004e04e3
005204f300760429004e04a80076049b00110607007606c2004e0239ffcd
04a8007604e3004e04a8007606c2004e055a00970715002f048900a405b1
00580556004a0239008c0235ffca0473002308c0001a0880009d07000037
04e2009a04fa000005c0009905c7000005c0009b05c70096048900a405b3
fffa05560095073b00170503002c05c0009905c0009904e2009a059d0020
06aa009105c700960639005905c000990556009505c7006104e3002c04fa
000006d400590556000005d8009a059f007d080a009a0827009a06f5001a
07d5009d05c0009b05b100570840009605c000040473004904f1005c04eb
0096035500880514fff90473004105acffff03fa001804eb008c04eb008c
040100880515001905eb009b04d5008804e3005204d5008804e3008b0473
005503eb00150473000e070000540473000c04eb008904a5007206ab008c
06c0008d05d5002806d5009504eb0099046b003806d5009104abfffb0473
004504e3000003550088046b005104730030023900930240ffd00239ffa2
07c000180740008c04e30000040100880473001204d5008803e500960393
00880800004108eb00a30620003002aa010102aa001e02aa003102aa0031
02aa010102aa007f02aa007e02aa008c02aa008c02aa010102aa001002aa
010102aa01210393007d02aa008c026500c802aa030202aaff0102aa00c9
04a90059049b004103a7000a0466003204ea0082022f0087034e005a04ed
00870503007d022f0087042c002803ed004b03f8004104e30087050a0037
022f00870316004b04e800500459000a04c0006404b2006403ff000a0418
000a04950082042c002805b8005a0563002d045e0087045e0087045e0087
0236005004090050068b0087022fffac042c0028042c002803f8ff1603f8
ff160479003205b8005a05b8005a05b8005a05b8005a04a9005904a90059
04a90059049b004103a2000a0466003204ea008202950000038100000503
007d02950000042c002803ed004b03f80041050a00370316004b04e80050
04c0006404b200640418000a04950082042c002805b8005a0563002d022f
0087049b004103ed004b04b2006404db00410000ffdc0000ff250000ffdc
0000fe51028d00ab028d00a002da004303c0007e0196ffba019c004601e5
0046019c0046019c004601ad0048019c004601b1004601510046047e0188
047e0150047e0104047e009e047e012d047e00ea047e00d5047e009c047e
00bc047e00ee04350085028d00c1043500b3060001000600010002be0058
06000100047e00a5047e00bd047e00de0600010006000100060001000600
01000600010001b100460600010006000100060001000600010006000100
06000100060001000600010004e6ffba0600010006000100060001000532
003905320039022cffba022cffba06000100060001000600010006000100
049e0034047800300430ffba0430ffba0376000a0376000a060e00290708
002902e2ffba0456ffba060e00290708002902e2ffba0456ffba05280097
046f000a0600010006000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
060001000600010001cf003001b1004601b1004601b1004001b100460600
0100060001000000ffdc0000fe510000ff160000ff160000ff160000ff16
0000ff160000ff160000ff160000ff160000ff160000ffdc0000ff160000
ffdc0000ff200000ffdc0473002d08000000060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
01000600010006000100028d007f028d00670600010005a0002e03c0007e
01e800000207ffc301bc005e01e0fffa039c0006039c000601bc005e01e0
001a05280097049e0011022cffba022cffba01bc008801e0001a05320039
05320039022cffba022cffba02be0036035200030532003905320039022c
ffba022cffba0532003c0532003c022cffba022cffba049e003404780030
0430ffba0430ffba049e0034047800300430ffba0430ffba049e00340478
00300430ffba0430ffba02be006902be006902be006902be00690376000a
0376000a0376000a0376000a073200400732004004deffba04deffba0732
00400732004004deffba04deffba0880004008800040062cffba062cffba
0880004008800040062cffba062cffba0430ffba0430ffba0430ffba0430
ffba0430ffba0430ffba0430ffba0430ffba0454003403c000460454ffba
02e2ffba0454003403c000460454ffba02e2ffba0610002f0610002f0270
ffba0298ffba04e6002704e600270270ffba0298ffba0454002904540029
02e2ffba02e2ffba039c0023039c002301e0ffba01e0ffba02e2002102e2
00210352ffba0352ffba0454003e0454003e022cffba022cffba02be0058
0352000303c0ffba039cffba039c0006039c000605280097046f000a0528
0097049e0011022cffba022cffba0454000004c4000003e400220454001a
03e400220454001a03e400220454001a0600010006000100019c0046019c
00460600010006000100060001000151004601b100460600010006000100
01ad004801e5004606000100060001000600010001b1004601b1004601b1
004601b1004601b1004001cf003006000100019c0046019c004606000100
060001000600010006000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
0100028d00ca028d00c7028d00c606000100060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
0600010006000100060001000600010002be00690100ffba0800ffba1000
ffbb06d3005905b0005206a3009305cb008d0000fd880000fbc10000fc5f
0000fe310000fcad0000fd550000fe260000fdf10000fd180000fc690000
fd950000fbe00000fc700000fed40000fecd0000fea0041b007806ac005c
06ac00190000fe450000fd550000fda60000fc5f0000fe250000fd180000
fbe00000fafa0000fb360000fc700000fb870000fb9b0000fcce0000fc54
0000fbc30000fc940000fbf50000fdb00000fe590000fd7e0000fc820000
fd340000fe500000fe460000fcd10000fd3e0000fd020000fc3a0000fce9
0000fc260000fc070000fc2f0000fb9e0000fb760239009305c700000473
004905c700000473004905c700000473004905c700000473004905c70000
0473004905c700000473004905c700000473004905c700000473004905c7
00000473004905c700000473004905c700000473004905c7000004730049
055600950473004105560095047300410556009504730041055600950473
004105560095047300410556009504730041055600950473004105560095
047300410239006a0239005d0239008c023900930639005904e300520639
005904e300520639005904e300520639005904e300520639005904e30052
0639005904e300520639005904e3005206d3005905b0005206d3005905b0
005206d3005905b0005206d3005905b0005206d3005905b0005205c70093
04e3008d05c7009304e3008d06a3009305cb008d06a3009305cb008d06a3
009305cb008d06a3009305cb008d06a3009305cb008d0556fffd0473000e
0556fffd0473000e0556fffd0473000e05c70000047300490239ffca0239
ffca0639005904e3005205c7009304e3008d05c7009304e3008d05c70093
04e3008d05c7009304e3008d05c7009304e3008d0000fef90000fef90000
fef40000feef0489fffd03550007073b001705acffff04e2009a04010088
04e2009a0401008805c7009604d500880473000104730012047300010473
0012055600000473000c059f007d04a50072059f009c04e3009205cf0059
0473004c0639005604e3005205320039022cffba0270ffba0298ffba04e6
0027022c0065022c0016022c0016022c0011022c0043022cffd20000fef0
01a8000f01a8fff502aa009002aa009001e8000001bc005e01bc005e0000
ffcb01bc000f01e0ffbf01bcfff501e0ffcd01bc001d01e0000901bc0088
01e0001a039c0006039c0006039c0006039c000605280097046f000a0532
003905320039022cffba022cffba0532003905320039022cffba022cffba
0532003905320039022cffba022cffba0532003905320039022cffba022c
ffba0532003905320039022cffba022cffba0532003905320039022cffba
022cffba0532003905320039022cffba022cffba049e0034047800300430
ffba0430ffba049e0034047800300430ffba0430ffba049e003404780030
0430ffba0430ffba049e0034047800300430ffba0430ffba049e00340478
00300430ffba0430ffba049e0034047800300430ffba0430ffba02be004f
02be004f02be006902be006902be006902be006902be004f02be004f02be
006602be006602be006902be006902be006902be006902be002f02be002f
02be002202be00220376000a0376000a0376000a0376000a0376000a0376
000a0376000a0376000a0376000a0376000a0376000a0376000a0376000a
0376000a0376000a0376000a073200400732004004deffba04deffba0732
00400732004004deffba04deffba073200400732004004deffba04deffba
0880004008800040062cffba062cffba0880004008800040062cffba062c
ffba0430ffba0430ffba0454003403c000460454ffba02e2ffba0610002f
0610002f0610002f0270ffba0298ffba0610002f0610002f0270ffba0298
ffba0610002f0610002f0270ffba0298ffba0610002f0610002f0270ffba
0298ffba0610002f0610002f0270ffba0298ffba04e6002704e6002704e6
002704e60027060e00290708002902e2ffba0456ffba060e002907080029
02e2ffba0456ffba045400290454002902e2ffba02e2ffba045400290454
002902e2ffba02e2ffba045400290454002902e2ffba02e2ffba060e0029
0708002902e2ffba0456ffba060e00290708002902e2ffba0456ffba060e
00290708002902e2ffba0456ffba060e00290708002902e2ffba0456ffba
060e00290708002902e2ffba0456ffba039c0023039c002301e0ffba01e0
ffba039c0023039c002301e0ffb101e0ffb1039c0023039c002301e0ffba
01e0ffba039c0023039c002301e0ffba01e0ffba0454003e0454003e022c
ffba022cffba0454003e0454003e0454003e0454003e0454003e0454003e
022cffba022cffba0454003e0454003e049e0034047800300430ffba0430
ffba02be005803520003031a001a031a001a031a001a039c0006039c0006
039c0006039c0006039c0006039c0006039c0006039c0006039c0006039c
0006039c0006039c0006039c0006039c0006039c0006039c000605280042
046fffd905280097046f000a022cffba022cffba039c0006039c00060528
0097046f000a022cffba022cffba05280097046f000a067f0044067f0045
067f0044067f004501a800280000fe290000fe8c0000ff250000ff230000
fefa0000ff7a0000fe5908fc003208ad00320000ffb50000ffb60000fef0
0000ff590000fe590000ff8c01b4000002f700000000fe850000ff0704cd
00320000ff580000ff580000ff59073200400732004004deffba04deffba
0880004008800040062cffba062cffba0454003403c000460454ffba02e2
ffba03c0007e02e2002102be0058022cffba0290ffba01f4002f01f4003b
01f4001201f400b101f4006d060e002907080029022f00870000fec80350
0000045e008703e4fff50454fff503e400220454001a03e400220454001a
03e400220454001a03e400220454001a03e400220454001a03e400220454
001a047e0072047e00bd03e4000f0454000f000000000000006c0000006c
0000006c0000006c0000006c0000006c0000006c0000006c0000006c0000
006c0000006c000000f600000180000001800000018000000180000001ce
0000020c0000026200000366000003e80000058e0000058e000006a80000
081a0000094e0000094e00000aec00000aec00000aec00000aec00000b76
00000b7600000c0400000c0400000c0400000c0400000c0400000c040000
0c0400000cc200000cc200000cc200000cc200000cc200000cc200000cc2
00000cc200000cc200000cc200000cc200000d9200000d9200000ef60000
0ef600000ef600000ef600000ef600000ef600000ef600000ef600000ef6
00000ef600000ef600000ef600000ef600000ef600000ef6000011040000
110400001240000013300000153c0000153c0000171800001818000018ba
000018ba000018ba0000192600001ada00001bc400001cb400001db00000
1db000001db000001db000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00000
1ed000001ed000001ed000001ed000001ed000001ed000001ed000001ed0
00001ed000001ed000001ed000001ed000001ed000001ed000001ed00001
0000068a00f2003c006f000600020010002f00550000064effff00030002
be0054039a000f0101001fffc00398b310143240b80399b30f1332404110
039500500395000200b0034d00c0034d0002006f0391007f03910002ffc0
034bb22d3132b9ffc0034bb30a0e32104110038b0020038b0080038b0003
00a0038b00010020038b0040038b0002ffc0038bb313163240b80383b20f
1132b9ffc0037bb2303432b9ffc0037bb310183250411403780001036503
6e0023001f037e036e001e001f0363036e001d001f03620364000d001fff
c00340b30f1032804110033f0001033f03150029001f034103160032001f
0344031a001b001fffc00375b20e1132b9ffc00375b2282a32410a034303
180032001f030f030d0034001f03080307b2321f20bb0340000100400388
b3090b3240b80388b2101532bd038503070014001f03800307b2171f0fbd
030a002f030a0002ffc00354b3090d3290410c035400a003540002001f03
6e0001009f036e00010040036eb2090b32410a0345031c0016001f036b03
1d0015001f0346031eb2151fc0bb0393000100400392b3090d3240b8033e
b2083340b8033eb30d0e32c04109033e000100b0038e00c0038e0002ffc0
0390b326383200412603280030032800020020037f0030037f0002001003
8a0030038a0050038a006f038a007f038a009f038a000600000389003003
890002002f037a0070037700900377009f037a0004ffc00315b20f1032b9
ffc00315b2242832b903190318b2321f10bb031a0001ffc0031ab3090e32
40b80318b2121332b9ffc00318b30c0e323fbd0373004f03730002004003
74b31718326fbb032a00010040032cb3181b3240b80370b2090c32bd0317
03160032001fffc00316b20e1132bd031c031e0016001f031d031eb2151f
b0411f031e0001000f031f000102ca02d00015001f02d302d5000d001f02
cf02d0000d001f02cb02d0000d001f02cd02d0000d001f02ce02d0000d00
1fffc002d0b3090c3240b802d2b3090c32e0411c02e50001005f02dd009f
02e5000202bb02c30030001f02da02b80032001f02d902b9003f001f02d8
02b80064001f02b902b80033001f02bab221c81fb802b8b321c81f40b803
9bb20d1632b9ffc002c3b22b2f32b9ffc002c3b21f2532b9ffc002c3b217
1b32b9ffc002c3b2121632412502c202c1001c001f02d702c10024001f02
c102c00022001f02bf02c00018001f02c0027400c8001f02b50235003b00
1f02b40235003b001f02c402bc001e001f02b702b60038001f02b3b20ec8
1fb802b0b207c81fb802afb206c81fb802aeb200c81fb802afb2502f1fbc
02ae02ab001a001f02adb2261a1fb802a8b326241f0fbb0235000102a502
74b21d1f12410a02a1015801f4001f02a000d801f4001f001202a2b237c8
1fb80290b2bc201fb9029002904018374025402d40a6033025302d30a603
2025202d203720a6204110028e0005009f028b0001028b028b0037002002
89003002890040028900900289b20437b041fd027400c002740002008002
7400a0027400020060027400700274000200000274001002740002008002
7400f002740002003f0285004f028500020090027e0090027f0090028000
90028100040090027a0090027b0090027c0090027d000400900274009002
750090027700030070027e0070027f007002800070028100040070027a00
70027b0070027c0070027d00040070027400700275007002770003006002
7e0060027f006002800060028100040060027a0060027b0060027c006002
7d000400600274006002750060027700030050027e0050027f0050028000
50028100040050027a0050027b0050027c0050027d000400500274005002
750050027700030040027e0040027f004002800040028100040040027a00
40027b0040027c0040027d00040040027400400275004002770003003002
7e0030027f003002800030028100040030027a0030027b0030027c003002
7d000400300274003002750030027700030020027e0020027f0020028000
20028100040020027a0020027b0020027c0020027d000400200274002002
750020027700030010027e0010027f001002800010028100040010027a00
10027b0010027c0010027d0004001002740010027500100277000300e002
7e00e0027f00e0028000e00281000400e0027a00e0027b00e0027c00e002
7d000400e0027400e0027500e00277b103d041c5027e00d0027f00d00280
00d00281000400d0027a00d0027b00d0027c00d0027d000400d0027400d0
027500d0027700030030027400400274000200c0027e00c0027f00c00280
00c00281000400c0027a00c0027b00c0027c00c0027d000400c0027400c0
027500c00277000300b0027e00b0027f00b0028000b00281000400b0027a
00b0027b00b0027c00b0027d000400b0027400b0027500b00277000300a0
027e00a0027f00a0028000a00281000400a0027a00a0027b00a0027c00a0
027d000400a0027400a0027500a0027700030090027e0090027f00900280
0090028100040090027a0090027b0090027c0090027d0004009002740090
02750090027700030020027e0020027f002002800020028100040020027a
0020027b0020027c0020027d000400200274002002750020027700030281
01580801001f028001290801001f027f00ec0801001f027e00d80801001f
027d00b10801001f027c00a60801001f027b00820801001f027a00370801
001f027700260801001f027500200801001f0274001f0801b21f370f4116
0235004f0235005f0235006f0235009f023500af023500bf0235000700af
023500cf023500df023500ff02354022040f074f079f07af07bf0705af07
e007020f064f069f06af06bf0605af06e0060220411b020d0001005f0235
0001008f02350001007f023500ef02350002002f0235003f02350002003f
0234004f0234000202350235023402344011ed20ef2a01cf2a01bf2a01af
2a018f2a01410902470104001e001f022000370201001f0158400c263e1f
d8263e1f3726273e1fb8028eb6ec171fb226361fb801bcb226361fb80129
402b26361fec26361fb126361fa626361f8226361f3726361f3226361f2d
26361f2526361f1f26361f37262a1fb801584022263e1fd8263e1fbc263e
1f27263e1f21263e1f20263e1f3700161600000012110840b9020d01a6b3
c50d0009b801bcb227281fb801bbb227301fb801b8b2274f1fb801b7b227
621f410901b600270101001f01b5002002ab001f01afb21fe41fb801adb2
1fe41fb801acb21fbb1fb801a8b21f341fb8015db2272e1fb8015bb227cd
1f410d0155001f0401001f0154001f0401001f0153001f0201001f0152b2
1f561fb80151b21f291fb8012bb227261f410d012a00270125001f012901
5800e4001f0125001f0401001f0124b21fe41fb80123b21f3b1fb80122b2
1f391f410d010800270801001f0106002d0101001f0105001f0101001f01
03b31fbb1fefb901580401400b1fed1f931fec1fe41feb1fb80201b21fd9
20b80401b21fcf25b80156400a1fbc2d9e1fbb1f411fb2410a0158040100
1f00b101580401001f00b001580401b51fa625891f9bb901580125b61f99
1f2e1f8e2db80801b51f8d1f291f89b901580401b21f8220b802ab40131f
801f301f742de41f731f4a1f611f521f5d25b802abb21f5c1fbc0801001f
0059015802abb61f5025891f491fb80125b21f4725b80401400b1f461f79
1f401f271f3920bc02ab001f003801580401b21f372dbc0125001f003201
580125b61f2c1f341f2a25b80801b21f5537b80111402a07f00790075b07
42073b07230722071e071d071408120810080e080c080a08080806080408
0208000814b8ffe0402b0000010014061000000100060400000100041000
0001001002000001000200000001000002010802004a00b013034b024b53
42014bb0c063004b6220b0f65323b8010a515ab005234201b0124b004b54
42b0382b4bb807ff52b0372b4bb007505b58b101018e59b0382bb00288b8
01005458b801ffb101018e851bb0124358b10100858d1bb900010119858d
5959001816763f183f123e113946443e113946443e113946443e11394644
3e11394660443e11394660442b2b2b2b2b2b2b2b2b2b2b182b2b2b2b2b2b
2b2b2b2b182b1db0964b5358b0aa1d59b0324b5358b0ff1d594bb0815320
5c58b9020f020d4544b9020e020d45445958b90470020f455258b9020f04
704459594bb0e453205c58b90020020e4544b90027020e45445958b90842
0020455258b9002008424459594bb8012553205c58b90026020f4544b900
21020f45445958b90a0d0026455258b900260a0d4459594bb8040153205c
58b1d8204544b1202045445958b9250000d8455258b900d825004459594b
b8040153205c58b9015800264544b1262645445958b923200158455258b9
015823204459594bb02953205c58b11f1f4544b12d1f45445958b9010d00
1f455258b9001f010d4459594bb02f53205c58b11f1f4544b1251f454459
58b90135001f455258b9001f01354459594bb8030153205c58b11f1f4544
b11f1f45445958b91428001f455258b9001f14284459592b2b2b2b2b2b2b
2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b
2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b65422b
01b331757ec3456523456023456560234560b08b766818b080622020b17e
754565234520b003266062636820b003266165b075236544b07e234420b1
31c34565234520b003266062636820b003266165b0c3236544b0312344b1
00c3455458b1c3406544b23140314523614459b33f3c5841456523456023
456560234560b089766818b080622020b1583c4565234520b00326606263
6820b003266165b03c236544b058234420b13f414565234520b003266062
636820b003266165b041236544b03f2344b10041455458b141406544b23f
403f452361445945695342014b5058b108004259435c58b108004259b302
0b0a124358601b2159421610703eb0124358b93b21187e1bba040001a800
0b2b59b00c2342b00d2342b0124358b92d412d411bba04000400000b2b59
b00e2342b00f2342b0124358b9187e3b211bba01a80400000b2b59b01023
42b0112342002b2b2b2b2b2b2b2b00b01243584bb035514bb021535a58b1
262645b040614459592b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b7373
73737345b040614418004569444569447373737473737374737473742b2b
2b2b2b2b2b2b2b2b2b2b0073737373737373737373737373737373737373
737373747474747474747474747474747474747474747474757575737475
7575752b7300004bb02a534bb036515a58b1070745b040604459004bb02e
534bb036515a58b1030345b0406044b1090945b8ffc06044592b45694401
74007373732b4569442b012b435c58400a0006000702a006a00702b9ffc0
0274b31a1d326fbd0277007f02770002ffc00277b22f3132b9ffc00277b3
22253240b80274b32f353240b80274b3282a3240b80274b21a2132b8ffc0
b3371a1d32b8ffc0b3251a1d32b8ffc040112d1a1d329025902d9037a025
a02da03706b8ffc0b6a61a1d321fa61fb8028eb22fa60300742b732b2b2b
2b2b2b2b2b742b737459002b2b435c58b9ffc002a1b21c1d32b9ffc002a0
b21c1d322b2b592b73012b2b2b2b002b2b2b2b2b2b2b2b2b2b2b2b2b2b2b
2b2b2b012b2b2b2b2b2b2b73742b2b2b2b2b2b2b2b73732b2b2b2b2b2b73
2b732b2b2b742b2b2b73737373732b73732b2b2b73002b2b2b2b7374732b
732b2b2b2b752b2b2b2b2b2b2b2b752b2b2b2b2b732b2b2b2b7374752b2b
7373732b2b2b2b0000>
[7889 ] AllocGlyphStorage
]def 
108 44 
PrepFor2015
Type42DictEnd
1 0 0 <00020100000005000500000300070042b40201fe0607b8023f4013000504
fe03000a0704fe010019080605fe0203bc0126000901b0011800182b10f6
3cfd3c4e10f43c4dfd3c003f3cfd3c10fc3cfd3c31302111211125211121
01000400fc2003c0fc400500fb002004c000>/EKJCBF+Arial,Bold AddT42Char 

1 0 3 <> /EKJCBF+Arial,Bold AddT42Char 
1 108 11 <0001006bfe51026805d300100046400e280fa70302080901000910001208
bd012200090001012200000294400a09f30c9b200430040204b80296b311
a56b182b10f65dedfdf4ed10ed003f3f103c103c3130015d012326023510
13363733020215141217160265c199a0635684c089673d3523fe51e701f2
e901210102e0bdfed1fe57eea4fea89b6600>/EKJCBF+Arial,Bold AddT42Char 
1 246 12 <00010043fe51024005d30010004940182702270a6702670a9702a702a80e
07090810000810001210bd012200000009012200000294b408f3059b0cb8
0296b3126a43182b10f6edfde4ed10ed003f3f103c103c3130015d133e03
3534020333161215140702034553443a1c6689bf97a7424bacfe51b2bef8
df75ee01a9012fd7fe1ef8d1effef4fefb00>/EKJCBF+Arial,Bold AddT42Char 
1 384 16 <000100410187026902a00003003240213001400102013700000310032003
30030403440510002000300003001904a56c182b4e10e45d4d10e65d002f
ed5d31301311211141022801870119fee700>/EKJCBF+Arial,Bold AddT42Char 
1 462 17 <00010093000001ac01190003002440150238000a02260f001f0020003000
040019046776182b4e10f45d4dfd003f4ded3130331121119301190119fe
e700>/EKJCBF+Arial,Bold AddT42Char 
1 524 18 <0001fffdffe7023b05d300030038401d0001014902031402020302010003
000a01eb021a0503eb001904936c182b4e10f44ded4e10f64ded003f3c3f
3c87052e2b7d10c431300701330103016bd3fe911905ecfa1400>/EKJCBF+Arial,Bold AddT42Char 
1 610 19 <00020056ffe7040e05c0000e00200093404b780a880aa701aa07aa09a70e
b709c8090856115916591a561f67116816681a671f08390239063609360d
490249064509460da709cb02c906c409c40dd902db06d409d40d11101820
180218b8ffc0402512163418a6080d1f0f2f0f020f401216340fa600051d
d84f0401041a2214d80b1921d3c2182b4e10f44ded4e10f6714ded003fed
2b713fed2b713130015d005d5d0132171611100706232200111037361722
060706111016163332363736111026260232d5788f9077d5d6fefa9077d5
3350161d344f333350161d344f05c098b4fe5ffe60b696014901a6019eb6
96e941546dfefefefec14041546c01020102c141>/EKJCBF+Arial,Bold AddT42Char 
1 870 20 <000100a20000032605c00009005640096b027b028b02030204b80129b35f
050105b8025eb708090501000c0900bb015800020001025d400d0500041f
042004b0040404190aba01a701a000182b4e10f45d3c4df63cfd3c003f3c
3f3cf45ded393130005d212111060735362437330326fee79ad16e010230
e404239045ff24c98600>/EKJCBF+Arial,Bold AddT42Char 
1 1000 21 <000100330000040c05c0001d013f405fb518b61ab91bca04c718d018d019
d01a08431b431c431d56199b049518aa04a61c08061a20002806371a4804
43184319431a0824182419241a03162604560488189c1b9c1c9c1daa1caa
1d0812001d101d201d311d761d841d901dd61d081db8ffc040161415341d
02100c0f1d10002000022000300040000300b8ffc0b312163400b802a1b3
02010c0fb8015640231f0c2f0c020c401216340ca6130509d81616014f00
01001a1f0fd8107702191ed3c2182b4e10f44df4ed4e10f6713c3c4d10ed
003ffd2b71e43f3cfd2b5d713c1112390111332b5d435c58b9001dffc0b2
11391db8ffc0b20f391db8ffc0400e10390408103905081139040811392b
2b2b2b2b2b59b10602435458400b091b191b021b13010413000011123911
12395d593130015d4b5158bd001bffe0001cffe0001dffe0383838590171
5d5d5d011121361237363736353426232206072536243332161514060706
040607040cfc2710a0ecbe2b3a6559586808fee8190108c6d9f8474d33fe
f647160105fefb940109dbb13f57555e656a7b1ce8caeaae63b36241f450
2600>/EKJCBF+Arial,Bold AddT42Char 
1 1422 23 <000200260000044405c0000a000d00df40390c200d39090c190c2b0c530c
6b0ce20c06ed0d01060416042504280d480d5b0da70db70dc60d09010208
000c060d07050a0b0d07000c0c0d0db801ae401a03041403030403020c04
0d030d02040a0007400dc00dd00d030dbb01280008000201b4b600040400
0c0c00b80158b4058f0a010ab80102401210079f07bf0703071a0f3f027f
020202190eba014c014800182b4e10e47110f65d4df45d3cfd3c003f3f10
f43cfd5d3c0111123912393900111239123987052e2b047d10c40f0f0fb1
0602435458400b2d0c3d0c4d0ccd0cdd0c05005d593130015d5d005d2b21
11213501331133152311011101027efda8027cecb6b6fef0feaf0127f603
a3fc5ef7fed9021e01f5fe0b>/EKJCBF+Arial,Bold AddT42Char 
1 1704 24 <0001005bffe7043505a6001d01104029080e200c371245124919990d9e0e
9712da0e0912111312211123128512050004010d0a0c0c0d121111b802a0
40160e0d140e0e0d120a1420013001400103500190010201b80156b51004
20040204b8ffc0b712163404a61b0d0cb8025a400d1f0a2f0a020a401216
340aa614b8ffc0400b1416342014301440140314b801ab401411111f102f
10022f103f104f1003104012163410b802a040130f0f0e040f10e007d8d0
1701401701171a1f0eb8012140120d7701bcd0000140009f00af00030019
1ed3b9014700182b4e10f45d714dedf4e44e10f65d714dedf43c003f3c10
fd2b5d713c10f65d2bfd2b71e43ffd2b71e45d7111123987052e2b0e7d10
c401113900111239111239313001715d1325161633323635342623220727
132111210736333200151407062322245b01180c764d587a79617960e490
02e7fdee2c5e62bb0104698ffecbff0001791d5f6f8f9087876b2102fbfe
f9f92ffef0d9b58ec2da>/EKJCBF+Arial,Bold AddT42Char 
1 2074 25 <00020057ffe7042a05c00017002300bd403b6a0b750887089719a705a708
a90eaa13b90eb611bd13c011cf130d1505361144107a16b502d210d01407
bb00cf0002000401071812101b201b021bb8ffc0401e1216341ba60f0d1f
212f2102214012163421a63f09014009d009ff090309b8014fb3af010101
b8012140221f042f0402044012163404a6150501d800771ed84f0c010c1a
2518d8121924d3c2182b4e10f44ded4e10f6714dedf4ed003ffd2b71f45d
f65d71ed2b713fed2b7101111239001112395d3130015d005d0105262623
220607363332121514002322001110003332160114163332363534262322
06040ffef00a5443597b10699cb0fbfef8cfdefee2012aeea7dbfda17e51
4e687054517004531e5450a0fd7cfef4d4e1fef00159018901930164bbfc
e989957a8b8f857f>/EKJCBF+Arial,Bold AddT42Char 
1 2382 27 <00030053ffe6041705c0001800240030010db530081d1f3426b8fff8406c
1d1f34c711c713d705d707047510761484100326002a0c36003b0c46004c
0c6e0463086711681577278727970d9818a40da918a91aa61ea727a62ca9
30b91ab71e17771386138614872704970c010c970001001c2e980c010c2b
099700010025032e401216343f2e4f2e022eba028e001cffc04010161834
701c801c02a01c011c1c061228b8ffc04009121634302840280228b8028e
400d120d3f224f2202224012163422b8028e401a06051fd809772bd84f0f
010f1a3219d8037725d8161931d3c2182b4e10f44dedf4ed4e10f6714ded
f4ed003fed2b5d3ffd5d2b1011392f5d712bed5d2b011112395d1112395d
001112395d395d313001715d00715d2b2b01262635343633321615140607
161615140423222726353436131416333236353426232206031416333236
35342623220601486d63e5d3d1e76a607a7ffefdd7c8859d76b95f4f5060
5f4e51601a775957727459676503172ea160a4d6d6a4669f2a31bc7bcbfe
697cd877c70151545e5f544f5f60fd3d74827d76677d8e00>/EKJCBF+Arial,Bold AddT42Char 
1 2796 31 <0001005f00a7044c05010006005e4010060501070517055f050301200e11
3402b8ffe0400b0e11343706470602043703b8018a400906370003000606
0403b80184400b40058220020119074d43182b4e10f43c1a194ded1a18fd
3c3c103c003fedfded3130005d2b2b015d7125013501110101044cfc1303
edfd4302bda701b5f201b3fee3fef4feea00>/EKJCBF+Arial,Bold AddT42Char 
1 2934 33 <0001005f00a6044d04ff0006006640100f02010902190250020306200e11
3405b8ffe0400d0e113437014601d70603033704b8018a400a0137400003
0282200506b80184400e00040303014f00010019074d43182b4e10f45d3c
3c103c4d10fd3c1a19ed00183f1aedfded3130005d2b2b015d7137110101
1101155f02befd4203eea6011b011401110119fe4df0>/EKJCBF+Arial,Bold AddT42Char 
1 3076 40 <00010095000004f005ba000b0090403d08050407082506121f05013005af
05020505090304250201020a09250b000807064b0302480a000b010b1a20
0d300d400d030d04092001200030000200b8028bb30c3153182b4e10f45d
3c4dfd3c4e105df65d3c4df43cf43c003f3cfd3c3f3cfd3c11392f5d7143
5c58b90005ffc0b21d3905b8ff80b21a3905b8ff80b113392b2b2b593cfd
3c0305103c3c313033112115211121152111211595043ffce902e0fd2003
3305baf8febbf7fe71f7>/EKJCBF+Arial,Bold AddT42Char 
1 3266 51 <00020095000004f805ba000f001b007740250605b914b918034705016705
d605021211250d0e0e001b10250201020f00081627af070107b8ffc0b309
0b3407b8028c40161f1d301d601d701d801d051d100f2001200030000200
b8028bb31c3153182b4e10f45d3c4dfd3c4d1071f62b714ded003f3c3f3c
fd3c12392f3cfd3c3130005d71015d331121201716161514060607062323
1902333236363534262726239501db010e527eaa62974e6ac9c1a2af7643
5e4835a005ba1621ddaf87b8691115fdd704c2fe602e624150680d0a>/EKJCBF+Arial,Bold AddT42Char 
1 3474 53 <00020096000005bc05ba0015002100f84082390f490f57076a0b6a0caa09
a70ea023b60ed8090a0608060a1708160a360e460e460f0708100911140e
140f1410360e360f470f750e7910d30a0b78097819761d88098819861d06
091614090c0f0e530e750e840e940ea30e050e200d0c140d0d0c0f0c150d
171625131014016014a014021414002021250201020d0e0e1500080eb801
bc4027000d100d020dd41b27a006b006c006d00604068770230120233023
022321152001200030000200b8028bb3223163182b4e10f45d3c4dfd3c10
5d71f65dedf45ded003f3c3c103c3f3cfd3c12392f5d713cfd3c01111239
39872e2b5d0e7d10c4011139001112393130005d01715d5d331121321616
151406071616171321032e0223231111333236363534262726232396026f
ebd580c2c1607d6ab3fe9ed672545e663cdbd56a3c4f4824b4e705ba4fca
82a5d71c3886abfee2013fab5921fd9c034e2458424a5b0c0500>/EKJCBF+Arial,Bold AddT42Char 
1 3830 68 <00020049ffe8042e043e0023003201714068071a081c051d161a4a1b481c
4925db10df11093619461957266619672686269219931aa61ab91bc71ac8
1b0c06060d151606191627062915591977028602a606b506c6060cbf34d9
10021d243231112c0d24402b2e3424402228342440191d346f24fc240224
461db8ffc040300e0f343d1d01001d101db01df91d041d1d2c013300400e
0f340f001f0002005521401c113f21401b103f2140181a3421b80274b504
070c0d0a2cb8ffc0b31c113f2cb8ffc0b31b103f2cb8ffc0b3181a342cb8
02744040140b1e3126082909280d591f0c9f0c021f0c01ff0c010c400e16
340c1a4f340134600001008e300101013329215f1701df17014f175f176f
17031719336941182b4e10f45d71724dedf471ed5d4e105df62b5d71724d
edf4e4fd3c003fed2b2b2b3f3c3ffd2b2b2bf45d2be412392f5d712bb106
02435458b22f1d017159edb10602435458b90024ffc0b71b1d3454246424
025d2b595d2b2b2b111239030e103c3c3c313001715d005d710127363633
321616150314161721262726270606232226353436363736373534262322
060106060706151416333237363736350165ff2bd2cfbcb84b031b25feea
0b10070348a45da4bd569b92c54c506f4b54015e36ea243758444c453310
0b02e22e9a945989b7feb88c854c1c3719084646b2885a8d4b1c25201c51
453bfed2123218273c3b563226372465>/EKJCBF+Arial,Bold AddT42Char 
1 4356 70 <00010055ffe8043f043e001900e14051580f59125916680f691269167d18
79199702970cc610c618d710d618e906e908e913e915f80613381338154a
124a164618590c690c073a1237163718037705770f8705860f8919a812a7
16b912b616090eb8ffc0b3181b340eb8ffc0b51214340e330db8ffc0b319
1e340db8ffc0b30f11340dba0104000a02744012110b0040181b34004012
1434003390010101ba0101000402744020170701401214340121002f0d40
1214340d214f0e010e1a1b072114191a5841182b4e10f44ded4e10f65d4d
ed2bf4ed2b003ffdf45de42b2b3ffdf42b2be42b2b3130005d7101715d01
052626232206151416333236370506062322001110003332160431feeb0e
634f697d7f6b50661501142bf4cde9feeb0116edc2e502ec32535491aabd
9c5b6f2fbec20126010401070125a700>/EKJCBF+Arial,Bold AddT42Char 
1 4672 71 <00020054ffe8046105ba000f001c0090402d125906590a59125616561859
1c98079909f80909701e801e023a03340c3a1534194a03440c4a15441999
090914b80274b2050b1ab80274400e0b070e0f0001000a17290e0d2601b8
0129400f0f001a8f1e011e102108191d583c182b4e10f44ded4e1071f63c
4dedfd3ce6003f3c3f3c3fed3fed3130005d01715d4358400d6906690a69
1266166618691c065d592121350606232200111012333217112101141716
3332363534262322060461fefb41b15ab7fefbfec2b2820119fd122f447a
6188846764879c5b5901270108010e0119940210fc70aa4c6ea5a4b7a19f
>/EKJCBF+Arial,Bold AddT42Char 
1 4912 72 <00020041ffe80427043e0014001c01a3b90010fff840460b3999099a0d96
10a805a70abb09bb0db81a0808140148024706460a4f1ea80db606b61ac7
0ac80cd60ad80cf807f70d0d1c0f1c15401b1d3415400e11340f15bf15cf
150315b8ffc0b30f1e3f15b8ffc0b30e173f15b8028d400c0f0e12500e60
0e020e181201b8ffc0b6191b3401331200b8ffc0b31d203400b8ffc0b322
293400b8ffc0b32b2d3400b8ffc0b3181c3400b8ffc0400f0e0f34a00001
0000100002005f1212b80274b3040b1218b8027440240b070021012f1521
4f0e010e1a2f1e5f1e6f1e9f1e041e0f2108400d0f3408191d6941182b4e
10f42b4ded4e105df65d4dedf4ed003fed435c584014184028143f18401e
0f3f18401b103f18401c113f2b2b2b2b593ffd435c58b90012ffc0b32814
3f12b8ffc0b31e0f3f12b8ffc0b31b103f12b8ffc0b21c113f2b2b2b2b59
f45d712b2b2b2b2b435c58b90000ffc0b2123900b8ffc0b2173900b8ffb0
b3090a3e00b8ffc0b241213f2b002b2b2b59e42b1112395d435c5840140e
400f1e3f0e401c113f0e401b103f0e400e173f002b2b2b2b592f3cfd2b2b
722b2b3c0111333130015d71005d2b010506062320272635100033320003
211616333236132626232207061702fa011836e9affeeb85690114d3ed01
1206fd40038261425a270378565c3c3c0101522f9aa1b591dd0108012bfe
c7febd7d8b48016c7a7f43437300>/EKJCBF+Arial,Bold AddT42Char 
1 5436 74 <00020054fe510460043e0023002f014e4062771d871d02120c0d7031860d
8031042001230223033001330233034001430243035b0f59145925562956
2b592f6b0ff811f813123b0d33163b28332c4b0d44164b28442cf00cfd17
0a8e0c010c0b0c0d0b2a0c0d270e1617152d0d0c171604182401b8ffc0b5
191b34013300b8ffc0b30e113e00b8ffc0b30b0c3e00b8ffc0b3282a3400
b8ffc0b323253400b8ffc0b331343400b8ffc04009151b34600001005f05
b80274b21f0f27b80274b20e0a2db80274400b15071819062a290b261a18
b80129400919191a1a8f31013101b801b8400a00332421121930583c182b
4e10f44dedf4ed4e1071f63c4d10ed10fde4003f3c3fed3fed3ffdf4722b
2b2b2b2b2bb10602435458b90000ffc0b30e113400b8ffc0b2090c342b2b
59e42b01111217390011123939111239390708103c313000715d015d7143
58400d690f691469256729662b692f065d59005d17051617163332373637
3635350623222726351000333217352111140e0223202635341314163332
36353426232206790141081d28566e3725130d7ec0d67d620101bfc58001
073e70bb8ffef2e2fc8360678e88686583462738151e211631235e9bacb5
8fd5010b011aad95fc47bcba6a3cb98e0e0283a99da19ea5a09d>/EKJCBF+Arial,Bold AddT42Char 
1 5912 75 <000100920000045905ba001600b2402b0f011f0139013302331042014211
de01f9010907051605240258116811050101021314111213031402010fb8
0274401d0307090a0a14150a1600000b0a26080940202434af0901ff0901
091a18b8ffc040162224349018a018027018f01802ef1801180014261615
b8ffc0400f202434a01501f015011519173f3c182b4e10f471722b3c4dfd
3c4e105d71722bf671722b3c4dfd3c003f3c3f3c3c103c3fed3939111739
030e103c083c3130015d005d01113633321e021511211134262623220606
1511211101ab88bd619c4f1dfee720513d466e33fee705bafde59f487088
8ffd910231a75a35448986fdec05ba00>/EKJCBF+Arial,Bold AddT42Char 
1 6168 76 <00020093000001ac05ba000300070077b90009ffc0403f110a3f40095009
028009b009c009d009ef09051f0960097f09a009b0090503060700050403
0f00014000d000e00003005d02010006050607040a0207260104b8ffc040
092124340419083f3c182b4e10f42b3c4dfd3c003f3c3f3c3f3cfd5d713c
0305103c3c103c3c313001715d722b1311211101112111930119fee70119
04b60104fefcfb4a0426fbda>/EKJCBF+Arial,Bold AddT42Char 
1 6330 79 <00010093000001ac05ba00030053b90005ffc04029110a3f400550050280
05b005c005d005ef05051f0560057f05a005b0050502010003000a020326
0100b8ffc040092124340019043f3c182b4e10f42b3c4dfd3c003f3c3f3c
313001715d722b3311211193011905bafa46>/EKJCBF+Arial,Bold AddT42Char 
1 6438 80 <0001007e00000698043e0027013bb90029ffc0405d110a3f0506060c1506
160c340334083418342344024508451844230c20032f295309602980299f
29a406a707a60cb506b50cb029d029e0290e00292f2950299f29bf29df29
0629401a1c343f2950298029d029e02905072104071a1d16b80274b20a07
21b80274401e0407101111271b1c1c26270a0100060f10261211405a3560
11016f110111b80246400f1a1b261d1c405a356f1c01601c011cb80246b4
2526262701b80129b2000027b8ffc0b30f093f27b8ffc04036110a3f2740
5a352740413527403c35274024273427403a3d342f27cf27df27030f271f
27802703002720273027ff2704271928e33c182b4e10f45d71722b2b2b2b
2b2b2b3c4d10ed10fd3cf65d712b3cfd3cf6715d2b3cfd3c003f3c3f3c3c
103c103c103c3fed3fed0111123900111239313001722b715d005d012b13
211536333216173636333216171615112111342726232206061511211134
2626232206061511217e01038bc066963046a25c75a2281dfee71d27513b
682efee71e3f3641682dfee7042691a9545555545f5c4498fd59025f9e2e
3c488b96fe0202469b5a2c468499fdfc>/EKJCBF+Arial,Bold AddT42Char 
1 6874 81 <0001009100000459043e0016009f4018071317135a08680804b804013408
34104408440fe9100506b80274401d11070e0d060c0b0b01000a02012616
0040202434af0001ff0001001a18b8ffc040162224349018a018027018f0
1802ef1801180a0b260c0eb80129b20d0d0cb8ffc0400f202434a00c01f0
0c010c19173f3c182b4e10f471722b3c4d10ed10fd3c4e105d71722bf671
722b3c4dfd3c003f3c3c103c3f3c3fed3130005d01715d21211134262623
2206061511211121153633321e02150459fee724513949742bfee701058b
d35d9a4f1f021eac65385084b2fe1f04269cb44368847b00>/EKJCBF+Arial,Bold AddT42Char 
1 7108 82 <00020052ffe8049a043e000d001900974048e801e708f713f71504c702e8
05021219051909025910561356165918970298069808970cb809d502db05
dc09d50ce705e706e80d10a708cb02cc06c308c60c057508890684080311
b80274b20a0b17b80274401404071439071a601b701b021b0e2100191a58
41182b4e10f44ded4e1071f64ded003fed3fed313000715d015d71435840
09691066126616691804015d59005d015d13341236333200151400232224
26251416333236353426232206528afd9cf10134fec9ec92fef78a012096
6e6e95956e6e9602228c01068afec7eff1fec384ffa89ea8a8a09ca8a800
>/EKJCBF+Arial,Bold AddT42Char 
1 7348 83 <0002008bfe6c0497043e0010001c009a402e3813481302123403390d3913
341b4403490d4913441bf91b095606560a591256165618591cf607f91b08
0100061ab80274b2050714b8027440160b0b100f0e1721081a701e011e11
290e0e0f26101001b80129400b700080000200191d3f41182b4e10f4714d
ed3c10fd3c10e44e1071f64ded003f3c3fed3fed3f3c3130015d005d0143
58400d6606660a691266166618691c065d59005d13211536363332001110
002322262711210114163332363534262322068b010633ae6ab90102fefc
b9588f4ffee701168e6662828663678804269c5064fedefefdfef6fed946
55fde903b9b3ab9db3a7a29f>/EKJCBF+Arial,Bold AddT42Char 
1 7600 87 <0001001fffe80291059d001900cd402920002001230a290f3a0e4a0e590f
07191500180316150017121314011712021401180309070a070c18b80101
400f0017a017b017036017a017c0170317b80104b2150114b80274b30015
0607b80274400e0c0b092f0a2f00002f015f010201b80104402818032617
1255153f149f14af1403601480149014d014f01405001410142014301404
14191a78a0182b4e10f45d71724bb037534bb03b515a58b90014ffc03859
3c4dfc3cfd3cf45d3c10f419e400183fed3f3cfd3c10f45d71e411123911
330f0f0f0f3130015d011523111416163332371706232226262726351123
3533352511027ac00b271c274a18627c4c7a390b098181011a0426e0fe54
822b1c1bda2a335145319501cfe0d3a4fe89>/EKJCBF+Arial,Bold AddT42Char 
/EKJCBF+Arial,Bold findfont /CharStrings get begin
/.notdef 0 def
/space 3 def
/parenleft 11 def
/parenright 12 def
/hyphen 16 def
/period 17 def
/slash 18 def
/zero 19 def
/one 20 def
/two 21 def
/four 23 def
/five 24 def
/six 25 def
/eight 27 def
/less 31 def
/greater 33 def
/E 40 def
/P 51 def
/R 53 def
/a 68 def
/c 70 def
/d 71 def
/e 72 def
/g 74 def
/h 75 def
/i 76 def
/l 79 def
/m 80 def
/n 81 def
/o 82 def
/p 83 def
/t 87 def
end
/EKJCBF+Arial,Bold findfont /Encoding get
dup 0 /.notdef put
dup 32 /space put
dup 40 /parenleft put
dup 41 /parenright put
dup 45 /hyphen put
dup 46 /period put
dup 47 /slash put
dup 48 /zero put
dup 49 /one put
dup 50 /two put
dup 52 /four put
dup 53 /five put
dup 54 /six put
dup 56 /eight put
dup 60 /less put
dup 62 /greater put
dup 69 /E put
dup 80 /P put
dup 82 /R put
dup 97 /a put
dup 99 /c put
dup 100 /d put
dup 101 /e put
dup 103 /g put
dup 104 /h put
dup 105 /i put
dup 108 /l put
dup 109 /m put
dup 110 /n put
dup 111 /o put
dup 112 /p put
dup 116 /t put
dup 160 /space put
dup 173 /hyphen put
pop
end

userdict /pdf_svglb get setglobal
[/N292/EKJCBF+Arial,Bold 1 TZG
userdict /pdf_svglb currentglobal put true setglobal
ct_T42Dict begin
-0.664 -0.324 2 1.004
 256 array 0 1 255 {1 index exch /.notdef put} for  /EKJBOB+Arial
Type42DictBegin
[<00010000000a000a000a000a63767420962ad276000000ac000006306670
676dcc79599a000006dc0000066e676c7966a25d6f1500004d1c00001e70
68656164ce98269200000d4c0000003668686561123312ff00000d840000
0024686d74780e34584000000da800001a286c6f636100c218e4000027d0
00001a2c6d6178700b4801a8000041fc000000207072657052fec4e90000
421c00000aff6764697200000000000000000000000005ba001905ba001a
05a70019042600180000ffe70000ffe80000ffe7fe69ffe805ba0019fe69
ffe802ea000000b8000000b80000000000a800ad016900ad00bf00c201f0
001800af00b900b400c800170044009c007c009400870006005a00c80089
005200520005004400940119ffb4002f00a1000300a100cd00170057007e
00ba00160118ffe9007f008503d300870085000d002200410050006f008d
014cff75005c00df04830037004c006e00700180ff58ff8eff92ffa400a5
00b903c8fffd000b001a0063006300cdffee05d8ffdc002d005c00950099
00df019209b500400057008000b9039d0072009a035d0401ff67fffa0003
0021007700cd0004004d00cd01c0022b004c006500e70118017c034305d8
ffa3ffb0ffc40003001c005d0068009a00ba013501470221055cff4dffcd
0016002d00780080009900b200b600b600b800bd00da010c05f0ffa4fff0
0019002c0049007f00b400ce01c003fefd81fe3f00000005001800290039
0049006f00be00c700d0012301c1026f050c05320540057affd400140031
0055005700a700b400e601f7027e027e027f03c60446ff42000e00850091
00bf00c200c500e1011a012f014f01560229026f029e03720008002c0031
0031006400690089009800c700de012b01b6020c02cf03a304ab04fb061d
fee0ff0e00060026009b009d00c1010d011801200173018201d601e30243
025f029b02e2039404a904d20761001c005e006d008d00ab00f701120138
0151015b0168017c01870191019901cd01d001e802410254026b02ef0368
037103bd044204420453047304830586058b06e8fe58fec4fed1fef7ff32
ff860051007c008100910095009e00b400b900cf00d900d900df00e20105
010b010e010e012001210155017b017b017e018d01a201a801a901b401d0
01d001e201e901f201f501fb020002000206021b02210222022202230272
02770294029c02cf02cf02d002ec02f903170322032b0335033c0359036f
037103870390039003b503e1041a04cf04ff053205320596059f05a805ab
05c205f0060c0782080008ccfca3fd2afddefe00fe88fe96feb2feb4ffe1
00150019001a001c001f003c005100610061006a0078009600a500af00d3
010c0118011a012a013e014c0151015f016a0171017801820184019a01a5
01a801a901ae01bc01cd01d701ef0200020d021c02210222022e02350242
024f024f025e026502710290029202b402d602fa0307030b030f0315032a
0347035d036503740379039603b003cc03dd03e203f603fc03fc03ff040a
041f04220426042b0447045f0475049e04e704e7055c05cb05e5060a066d
068606b806f10736073e07500751075d078f07b607d4086000b600c300b5
00b700000000000000000000000001e00381034503b5008e0233041902ce
02ce002d005f0064034d023f000002a80188027d01b402240578063b023b
014e00f00426029402c6029f02f6023b034d014b0153006a023100000000
0000061404aa0000003c04c300ed04bc026502ce03b50078060c017e02ef
060c00b201000239000001c50330042b03cb00da03df010704a100db040a
011701ed02a70350010b01bd043e05580021039c00ae0371017d00b50245
00000afb088c012b014e01aa00870054013201f803ff0003024e00b40037
03e30083006b02d800ed00770088009701640467008e0033017c00e700a6
029e0329056e062a061501c90269048a021301b4000204a9000002390124
010305140084015d039a06ef02d9007500cf040a00de03ac04bc02cf02ae
034d04f005520168006d007d00860071ff810079055804d2016700030156
002504e00094007c033204210094007f0072005c002f00b6001800ba00b8
0041034d00720018001f004c016a01550099009a009a009800b200040078
006900140057006e00ce00b4065402b80067050e016500e7000004cbfe52
005affa60099ff67006eff92002dffd40087ff7c00b800a800e5008f00a8
0185fe7b0070001e00d900de014c054602cf0546ff2d028a02d902530296
00b700000000000000000000000000000125011800ea00ea00ae0000003e
05bb008a04d70053003fff8cffd500150028002200990062004a00e4006d
00ee00e5004803c00033fe4e02b1ff460370007905df0051ffa7ff1f010a
0068ff6c004f00bc00a507050061072b4043555441403f3e3d3c3b3a3938
373534333231302f2e2d2c2b2a292827262524232221201f1e1d1c1b1a19
1817161514131211100f0e0d0c0b0a090807060504030201002c45234660
20b02660b004262348482d2c452346236120b02661b004262348482d2c45
234660b0206120b04660b004262348482d2c4523462361b0206020b02661
b02061b004262348482d2c45234660b0406120b06660b004262348482d2c
4523462361b0406020b02661b04061b004262348482d2c0110203c003c2d
2c20452320b0cd442320b8015a51582320b08d44235920b0ed51582320b0
4d44235920b09051582320b00d44235921212d2c20204518684420b00160
2045b04676688a4560442d2c01b10b0a432343650a2d2c00b10a0b432343
0b2d2c00b0172370b101173e01b0172370b10217453ab10200080d2d2c45
b01a234445b01923442d2c2045b00325456164b050515845441b2121592d
2cb00143632362b0002342b00f2b2d2c2045b0004360442d2c01b00643b0
0743650a2d2c2069b04061b0008b20b12cc08a8cb8100062602b0c642364
615c58b00361592d2c45b0112bb0172344b0177ae4182d2c45b0112bb017
23442d2cb01243588745b0112bb0172344b0177ae41b038a45186920b017
23448a8a8720b0a05158b0112bb0172344b0177ae41b21b0177ae4595918
2d2c2d2cb0022546608a46b040618c482d2c4b53205c58b002855958b001
85592d2c20b0032545b019234445b01a23444565234520b00325606a20b0
09234223688a6a606120b01a8ab000527921b21a1a40b9ffe0001a45208a
54582321b03f1b235961441cb114008a5279b31940201945208a54582321
b03f1b235961442d2cb110114323430b2d2cb10e0f4323430b2d2cb10c0d
4323430b2d2cb10c0d432343650b2d2cb10e0f432343650b2d2cb1101143
2343650b2d2c4b525845441b2121592d2c0120b003252349b04060b02063
20b000525823b002253823b002256538008a63381b212121212159012d2c
4bb06451584569b00943608a103a1b212121592d2c01b005251023208af5
00b0016023edec2d2c01b005251023208af500b0016123edec2d2c01b006
2510f500edec2d2c20b001600110203c003c2d2c20b001610110203c003c
2d2cb02b2bb02a2a2d2c00b00743b006430b2d2c3eb02a2a2d2c352d2c76
b8022323701020b802234520b0005058b00161593a2f182d2c21210c6423
648bb84000622d2c21b08051580c6423648bb82000621bb200402f2b59b0
02602d2c21b0c051580c6423648bb81555621bb200802f2b59b002602d2c
0c6423648bb84000626023212d2cb4000100000015b00826b00826b00826
b008260f10161345683ab001162d2cb4000100000015b00826b00826b008
26b008260f1016134568653ab001162d2c4b53234b515a5820458a60441b
2121592d2c4b545820458a60441b2121592d2c4b53234b515a58381b2121
592d2c4b5458381b2121592d2cb0134358031b02592d2cb0134358021b03
592d2c4b54b012435c5a58381b2121592d2cb012435c580cb00425b00425
060c6423646164b807085158b00425b00425012046b01060482046b01060
48590a21211b2121592d2cb012435c580cb00425b00425060c6423646164
b807085158b00425b00425012046b8fff060482046b8fff06048590a2121
1b2121592d2c4b53234b515a58b03a2b1b2121592d2c4b53234b515a58b0
3b2b1b2121592d2c4b53234b515ab012435c5a58381b2121592d2c0c8a03
4b54b00426024b545a8a8a0ab012435c5a58381b2121592d2c4b5258b004
25b0042549b00425b00425496120b0005458212043b0005558b00325b003
25b8ffc038b8ffc038591bb04054582043b0005458b00225b8ffc038591b
2043b0005458b00325b00325b8ffc038b8ffc0381bb00325b8ffc0385959
5959212121212d2c462346608a8a462320468a608a61b8ff806223201023
8ab902c202c28a70456020b0005058b00161b8ffba8b1bb0468c59b01060
68013a2d2cb1020042b123018851b1400188535a58b910000020885458b2
02010243604259b12401885158b920000040885458b2020202436042b124
01885458b2022002436042004b014b5258b2020802436042591bb9400000
80885458b202040243604259b94000008063b80100885458b20208024360
4259b94000010063b80200885458b202100243604259b94000020063b804
00885458b202400243604259595959592d2cb0024354584b53234b515a58
381b2121591b21212121592d02010001000000030000b79bfaec5f0f3cf5
081b080000000000a2e3272a00000000b9d5b4f6faaffd671000080c0000
00090001000100001bb900010000073efe4e00431000faaffe2610000001
0000000000000000000000000000068a0600010000000000023900000239
0000023900b002d7005e0473001504730049071d0077055600580187005a
02aa007c02aa007c031d004004ac0072023900aa02aa0041023900ba0239
000004730055047300df0473003c047300560473001a047300550473004d
047300610473005304730055023900b9023900aa04ac007004ac007204ac
00700473005a081f006f0556fffd0556009605c7006605c7009e055600a2
04e300a80639006d05c700a4023900bf04000037055600960473009606aa
009805c7009c063900630556009e0639005805c700a10556005c04e30030
05c700a105560009078d0019055600090556000604e300290239008b0239
00000239002703c100360473ffe102aa00590473004a0473008604000050
047300460473004b02390013047300420473008701c7008801c7ffa20400
008801c7008306aa00870473008704730044047300870473004802aa0085
0400003f02390024047300830400001a05c700060400000f040000210400
002802ac0039021400bc02ac002f04ac00570556fffd0556fffd05c70068
055600a205c7009c0639006305c700a10473004a0473004a0473004a0473
004a0473004a0473004a040000500473004b0473004b0473004b0473004b
023900bd023900230239ffe5023900090473008704730044047300440473
004404730044047300440473008304730083047300830473008304730049
033300800473006b0473001b0473005102cd006d044c000104e3009905e5
000305e50003080000e102aa00de02aa003d0464004e0800000106390053
05b4009a0464004e0464004d0464004d0473fffd049c00a003f4003805b4
007a069600a1046400000231000002f6002f02ec002d0625007f071d0044
04e3008104e3009e02aa00e804ac0072046400540473002e0464003304e5
001a047300860473008c080000ef0556fffd0556fffd0639006308000081
078d00520473fffc0800000002aa005302aa004701c7008001c7006c0464
004e03f4002f04000021055600060156fe390473ffe402aa005c02aa005c
040000170400001704730049023900b901c7006c02aa0047080000250556
fffd055600a20556fffd055600a2055600a20239008d0239ffe002390004
0239001506390063063900630639006305c700a105c700a105c700a10239
00c602aa001902aa000602aa001d02aa002e02aa00e502aa00a202aa006b
02aa003a02aa00b702aa00280473000001c700030556005c0400003f04e3
002904000028021400bc05c7fffd0473004905560006040000210556009e
0473008704ac007204ac00a102aa006b02aa001902aa002106ac006b06ac
006b06ac0021047300000639006d04730042023900b10556005c0400003f
05c700660400005005c700660400005004730046046bffe102aa01f10556
fffd0473004a0556fffd0473004a05c7009e04eb004705c7fffd055600a2
0473004b055600a20473004b0473009601c7004204730096025500880473
009a02ac008305c7009c0473008705c7009c047300870639006304730044
05c700a102aa008505c700a102aa003c0556005c0400003f04e300300239
002404e300300300002305c700a10473008305c700a10473008304e30029
0400002804e3002904000028046800a4063900600662005504a000480474
00480391006204f000440329002e05300048046bffe1040000b002eb0052
08c000330800004f040000990800004f040000990800004f040000980400
009807d5016a05c0009e04ab007204d5009d04ac007104d5022204d50105
05abffe9050001c905ab027e05abffe905ab027e05abffe905ab027e05ab
ffe905abffe905abffe905abffe905abffe905ab01c005ab027e05ab01c0
05ab01c005abffe905abffe905abffe905ab027e05ab01c005ab01c005ab
ffe905abffe905abffe905ab027e05ab01c005ab01c005abffe905abffe9
05abffe905abffe905abffe905abffe905abffe905abffe905abffe905ab
ffe905abffe905abffe905abffe905abffe905abffe905abffe905ab02d6
05ab006605abffea05d5ffff04d500920800000007eb013007eb012007eb
013007eb012004d500b204d5008004d5002a082b0198086b01b807550010
060000f40600006f0440003a0540003704c0003f04150040040000250600
005505e100bf038d008904d5ffd90180008002d50086071500610296000f
04d5009202d6008302d6008304d500b202d600700556fffd0473004a05c7
00660400005005c7006604000050055600a20473004b055600a20473004b
055600a20473004b0639006d047300420639006d047300420639006d0473
004205c700a40473008705c7001f047300060239ffce0239ffce0239ffe4
0239ffe40239fff60239fff5023900a301c700660400003701c7ffa20556
009604000088040000860473009601c7fffa05c7009c0473008705c900a5
0473008b0639006304730044063900630473004405c700a102aa006b0556
005c0400003f04e300300239000c05c700a10473008305c700a104730083
05c700a10473008305c700a104730083078d001905c70006055600060400
002101c700890556fffd0473004a08000001071d00440639005304e30081
023900b9078d001905c70006078d001905c70006078d001905c700060556
00060400002101c7008a02aaffe10473001b04cd005a06ac006b06ac0022
06ac002206ac004a02aa00e202aa006b02aa00de02aaffea0557ffff0646
ffa706b4ffa80312ffa80632ffa706d8ffa70605ffa701c7ff780556fffd
055600960558fffe055600a204e3002905c700a4023900bf055600960558
000b06aa009805c7009c0533006d0639006305c700a40556009e04f20094
04e30030055600060556000906af007f05fb0061023900040556000604a0
0048039100620473008b01c7006b04600088049a008c0400001903870048
0473008b0473005c01c700890400008604000018049c00a00400001a0395
005c04730044048d008303db0056046000880433001105b4007a063f0057
01c7ffc9046000880473004804600088063f0057055700a206eb00320455
00a105c000640556005c023900bf02390004040000370875000d081500a4
06d5003104a900a10515000a05c000a00556fffd054000a7055600960455
00a1056b0000055600a20763000704d5004e05c000a105c000a104a900a1
0540001206aa009805c700a40639006305c000a00556009e05c7006604e3
00300515000a061500520556000905eb009f05550057075500a1078000a1
06550000071500a8054000a505c00055081500a405c7001a0473004a0495
005b0440008802eb008804ab00000473004b055afffb03ab003204780087
047800870380008604ab00180580008c046b008804730044045500880473
00870400005003aa0026040000210695004b0400000f0495008a042b0045
066b008d0695008d0500002805c0008b042b008404150030060000890455
001f0473004b0473000002eb00890415004b0400003f01c7008802390009
01c7ffa20740001306800083047300000380008604000021046b008803e9
00a1034a008808000041089500a00585002d02aa010102aa001e02aa0031
02aa003102aa010102aa007e02aa007e02aa008c02aa008c02aa010102aa
001002aa010102aa01210310007d02aa008c023300d202aa030b02aaff04
023900b90481006904560032033100190411002d04d1009601f9009b030f
005f04ca009b04b8008c01f9009b0413002803b0005003b4003c04ca009b
04cf005001f9009b02d2003c0498005a043c00190488006e045f007303b1
001903d4000a0466009604130028058e00640524002803f2009b03f2009b
03f2009b01e3005a0356005a0686009b01f9ffac041300280413002803b4
ff5703b4ff570448002d058e0064058e0064058e0064058e006404810069
048100690481006904560032033100190411002d04d10096024b0000034a
000004b8008c024b00000413002803b0005003b4003c04cf005002d2003c
0498005a0488006e045f007303d4000a0466009604130028058e00640524
002801f9009b0456003203b00050045f0073049b003c0000ffdc0000ff25
0000ffdc0000fe51028d00ab028d00a002da0043034d007901a8ffba019c
004601e50046019c0046019c004601ad0048019c004601b1004601510046
0435017c0435012e043500b7043500810435012c043500be043500af0435
00810435009a043500db04350085028d00c1043500b30600010006000100
02420036060001000435009e04350098043500cb06000100060001000600
0100060001000600010001b1004606000100060001000600010006000100
06000100060001000600010006000100051bffba06000100060001000600
010005b5003a05b5003a01f4ffba01f4ffba060001000600010006000100
060001000481003604350036043dffba043dffba03e9004a03e9004a067f
0014077600140327ffba041effba067f0014077600140327ffba041effba
051b003204b5002406000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
06000100060001000600010001cf003001b1004601b1004601b1004001b1
004606000100060001000000ffdc0000fe510000ff160000ff160000ff16
0000ff160000ff160000ff160000ff160000ff160000ff160000ffdc0000
ff160000ffdc0000ff200000ffdc0473004a080000000600010006000100
060001000600010006000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
0100060001000600010006000100028d007f028d005d0600010004ee0015
034d007901a8000e01d6ffdc01a8005601d60010037500320375003201a8
002d01d60013051b003204b5002401f4ffba01f4ffba01a8009301d60013
05b5003a05b5003a01f4ffba01f4ffba024200000300fff705b5003a05b5
003a01f4ffba01f4ffba05b5003a05b5003a01f4ffba01f4ffba04810036
04350036043dffba043dffba0481003604350036043dffba043dffba0481
003604350036043dffba043dffba02b3005f02b3005f02b3005f02b3005f
03e9004a03e9004a03e9004a03e9004a0692003e0692003e043fffba043f
ffba0692003e0692003e043fffba043fffba08c9003e08c9003e06c5ffba
06c5ffba08c9003e08c9003e06c5ffba06c5ffba04a7ffba04a7ffba04a7
ffba04a7ffba04a7ffba04a7ffba04a7ffba04a7ffba045a002a039a0036
0435ffba0327ffba045a002a039a00360435ffba0327ffba064f0027064f
00270224ffba021affba04a7004604a700460224ffba021affba04cf002d
04cf002d0327ffba0327ffba040d0047040d004701a8ffba01a8ffba02b4
002302b400230327ffba0327ffba043500450435004501f4ffba01f4ffba
024200360300fff7039affba0327ffba0375003203750032051b003204b5
0024051b003204b5002401f4ffba01f4ffba045a004004ce0049045a0026
04ce0039045a005304ce004a045a005304ce004a0600010006000100019c
0046019c00460600010006000100060001000151004601b1004606000100
0600010001ad004801e5004606000100060001000600010001b1004601b1
004601b1004601b1004601b1004001cf003006000100019c0046019c0046
060001000600010006000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
010006000100028d00ca028d00c7028d00c6060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
0600010006000100060001000600010006000100060001000100ffba0800
ffba1000ffba06dc0063053f004406d500a1055b00830000fddc0000fc2f
0000fca60000fe540000fcd70000fd730000fe290000fe0d0000fd110000
fc670000fd9d0000fbf50000fc720000fed50000fed50000ff02041b00a0
06ac006b06ac00190000feb60000fd730000fe080000fca60000fe530000
fd110000fbc80000faf40000faaf0000fc720000fbaa0000fb6a0000fcf1
0000fc7d0000fbdd0000fcc10000fb980000fdea0000fe840000fdc20000
fcf10000fd5f0000fe760000febc0000fceb0000fd6c0000fd580000fc90
0000fd150000fc2c0000fc130000fc120000fb960000fb9601c700880556
fffd0473004a0556fffd0473004a0556fffd0473004a0556fffd0473004a
0556fffd0473004a0556fffd0473004a0556fffd0473004a0556fffd0473
004a0556fffd0473004a0556fffd0473004a0556fffd0473004a0556fffd
0473004a055600a20473004b055600a20473004b055600a20473004b0556
00a20473004b055600a20473004b055600a20473004b055600a20473004b
055600a20473004b0239006301c7001f023900ba01c7007c063900630473
004406390063047300440639006304730044063900630473004406390063
047300440639006304730044063900630473004406dc0063053f004406dc
0063053f004406dc0063053f004406dc0063053f004406dc0063053f0044
05c700a10473008305c700a10473008306d500a1055b008306d500a1055b
008306d500a1055b008306d500a1055b008306d500a1055b008305560006
04000021055600060400002105560006040000210556fffd0473004a0239
ffe201c7ffb0063900630473004405c700a10473008305c700a104730083
05c700a10473008305c700a10473008305c700a1047300830000fefe0000
fefe0000fefe0000fefe0455fffd02eb000c07630007055afffb04a900a1
0380008604a900a10380008605c700a4046b00880473fffd040000140473
fffd04000014055600090400000f05550057042b0045055500a104730087
0605006304730055063900600473004405b5003a01f4ffba0224ffba021a
ffba04a7004601f4009e01f4001001f4001b01f4001001f4006b01f4fff9
0227ffce01a8000f01a8fff502aa00a402aa00a401a8000e01a8005601a8
00560000ffcf01a8000f01d6ffbf01a8fff501d6ffcd01a8001d01d6fff5
01a8009301d6001303750032037500320375003203750032051b003204b5
002405b5003a05b5003a01f4ffba01f4ffba05b5003a05b5003a01f4ffba
01f4ffba05b5003a05b5003a01f4ffba01f4ffba05b5003a05b5003a01f4
ffba01f4ffba05b5003a05b5003a01f4ffba01f4ffba05b5003a05b5003a
01f4ffba01f4ffba05b5003a05b5003a01f4ffba01f4ffba048100360435
0036043dffba043dffba0481003604350036043dffba043dffba04810036
04350036043dffba043dffba0481003604350036043dffba043dffba0481
003604350036043dffba043dffba0481003604350036043dffba043dffba
02b3003202b3003202b3005f02b3005f02b3005f02b3005f02b3003202b3
003202b3005f02b3005f02b3005f02b3005f02b3005f02b3005f02b30038
02b3003802b3004902b3004903e9004a03e9004a03e9004a03e9004a03e9
004a03e9004a03e9004a03e9004a03e9004a03e9004a03e9004a03e9004a
03e9004a03e9004a03e9004a03e9004a0692003e0692003e043fffba043f
ffba0692003e0692003e043fffba043fffba0692003e0692003e043fffba
043fffba08c9003e08c9003e06c5ffba06c5ffba08c9003e08c9003e06c5
ffba06c5ffba04a7ffba04a7ffba045a002a039a00360435ffba0327ffba
064f0027064f0027064f00270224ffba021affba064f0027064f00270224
ffba021affba064f0027064f00270224ffba021affba064f0027064f0027
0224ffba021affba064f0027064f00270224ffba021affba04a7004604a7
004604a7004604a70046067f0014077600140327ffba041effba067f0014
077600140327ffba041effba04cf002d04cf002d0327ffba0327ffba04cf
002d04cf002d0327ffba0327ffba04cf002d04cf002d0327ffba0327ffba
067f0014077600140327ffba041effba067f0014077600140327ffba041e
ffba067f0014077600140327ffba041effba067f0014077600140327ffba
041effba067f0014077600140327ffba041effba040d0047040d004701a8
ffba01a8ffba040d0047040d004701a8ffba01a8ffba040d0047040d0047
01a8ffba01a8ffba040d0047040d004701a8ffba01a8ffba043500450435
004501f4ffba01f4ffba0435004504350045043500450435004504350045
0435004501f4ffba01f4ffba04350045043500450481003604350036043d
ffba043dffba024200360300fff7031a001a031a001a031a001a03750032
037500320375003203750032037500320375003203750032037500320375
003203750032037500320375003203750032037500320375003203750032
051bffba04b5ffba051b003204b5002401f4ffba01f4ffba037500320375
0032051b003204b5002401f4ffba01f4ffba051b003204b50024067f0045
067f0045067f0045067f004501a800280000fe290000fea20000ff300000
ff1d0000ff120000ff920000fe7e08fc003208ad00320000ffb50000ffb6
0000feed0000ff640000fe7e0000ff9f018d000002f6fffd0000fe820000
ff1004cd00320000ff580000ff580000ff640692003e0692003e043fffba
043fffba08c9003e08c9003e06c5ffba06c5ffba045a002a039a00360435
ffba0327ffba034d007902b400230242003601f4ffba0290ffba01f4002f
01f4003b01f4001201f400b101f4006d067f00140776001401f9009b0000
fed902bc000003f2009b045afff504cefff5045a005304ce004a045a0053
04ce004a045a005304ce004a045a005304ce004a045a005304ce004a045a
005304ce004a04350071043500ad045a000f04ce000f000000000000002a
0000002a0000002a0000002a0000002a0000002a0000002a0000002a0000
002a0000002a0000002a000000aa00000150000001500000015000000150
00000196000001d200000242000003fe000004da00000704000008de0000
0a3e00000bf800000dce00000e7a0000110e0000110e0000110e0000110e
0000110e0000117e0000117e0000117e0000117e0000117e000013160000
131600001316000013da000013da000013da000013da000013da000013da
000013da000013da000013da000015840000158400001584000015840000
158400001584000016320000163200001632000016320000163200001632
000016320000163200001632000016320000163200001632000016320000
1632000016320000163200001632000017f0000017f0000017f0000017f0
000017f0000017f000001a8800001a8800001a8800001a8800001a880000
1c4c00001c4c00001c4c00001c4c00001c4c00001c4c00001c4c00001c4c
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000001e7000001e7000001e7000001e7000001e7000001e7000001e70
00001e7000001e7000001e7000001e7000001e7000001e7000001e700000
1e7000010000068a0100003f0076000700020010002f00560000040dffff
00030002b1540f4122031700ef031700ff03170003001f0317002f031700
4f0317005f0317008f0317009f03170006000f0317005f0317006f031700
7f031700bf031700f00317000600400317b2923340b80317b28b3340b803
17b36a6c3240b80317b2613340b80317b35c5d3240b80317b357593240b8
0317b34d513240b80317b344493240b80317b23a3340b80317b331343240
b80317b32e423240b80317b3272c3240b80317b312253280b80317b30a0d
32c04116031600d00316000200700316000102c4000f0101001f00a00315
00b0031500020306000f0101001f00400312b32426329fbf030400010302
03010064001fffc00301b20d1132410a02ff02ef0012001f02ee02ed0064
001fffc002edb30e11329f414a02e200af02e200bf02e2000302e202e202
e102e1007f02e00001001002e0003f02e0009f02e000bf02e000cf02e000
ef02e0000602e002e002df02df02de02de000f02dd002f02dd003f02dd00
5f02dd009f02dd00bf02dd00ef02dd000702dd02dd001002dc0001000002
dc0001001002dc003f02dc000202dc02dc001002db000102db02db000f02
da000102da02daffc002d3b2373932b9ffc002d3b22b2f32b9ffc002d3b2
1f2532b9ffc002d3b2171b32b9ffc002d3b2121632b802d2b2f9291fb802
e3b3202b1fa0413002d400b002d40002000002d4001002d4002002d40050
02d4006002d4007002d40006006002d6007002d6008002d6009002d600a0
02d600b002d60006000002d6001002d6002002ca002002cc002002d60030
02d6004002d6005002d6000802d0b2202b1fb802cfb226421f411602ce02
c70017001f02cd02c80017001f02cc02c60017001f02cb02c50017001f02
c902c5001e001f02ca02c6b21e1f00410b02c6000002c7001002c6001002
c7002f02c5000502c1b324121fff411102bf0001001f02bf002f02bf003f
02bf004f02bf005f02bf008f02bf000602bf0222b2641f12410b02bb00ca
0800001f02b200e90800001f02a600a20800406a1f402643493240204349
3240263a3d3240203a3d329f209f26024026969932402096993240268e92
3240208e92324026848c324020848c3240267a813240207a813240266c76
3240206c76324026646a324020646a3240265a5f3240205a5f3240264f54
3240204f5432b8029eb724271f374f6b0120410f02770030027700400277
00500277000402770277027700f90400001f029bb22a2a1fb8029a402b29
2a1f80ba0180bc0180520180a201806501807e01808101803c01805e0180
2b01801c01801e0180400180bb0138000100800140b40180400180bb0138
00010080013940180180ca0180ad01807301802601802501802401802001
3740b80221b2493340b80221b2453340b80221b341423240b80221b33d3e
320f410f0221003f0221007f0221000300bf022100cf022100ff02210003
00400221b320223240b80221b3191e3240b80222b32a3f3240b80221b32e
3a326f414802c3007f02c3008f02c300df02c30004002f02c3006002c300
cf02c30003000f02c3003f02c3005f02c300c002c300ef02c300ff02c300
0600df02220001008f02220001000f0222002f0222003f0222005f022200
7f022200ef0222000600bf022100ef02210002006f0221007f022100af02
210003002f0221003f0221004f0221000302c302c3022202220221022140
1d101c102b1048038f1c010f1e014f1eff1e023700161600000012110811
b8010db6f70df8f70d00094109028e028f001d001f0290028f001d001f02
8fb2f91d1fb80198b226bb1f41150197001e0401001f013900260125001f
013800730401001f0135001c0801001f0134001c02ab001f0132b21c561f
b8010fb2262c1fba010e001e0401b61ff91ce41fe91cb80201b61fe81cbb
1fd720b80401b21fd51cb802abb61fd41c891fc92fb80801b21fbc26b801
01b21fba20b80201b61fb91c381fadcab80401b21f8126b8019ab21f7e26
b8019ab61f7d1c471f6b1cb80401b21f6526b8019ab21f5e73b80401400f
1f52265a1f481c891f441c621f4073b80801b61f3f1c5e1f3c26b8019ab2
1f351cb80401b61f301cbb1f2b1cb80401b61f2a1c561f291cb80101b21f
231eb80401b21f5537b80168402c07960758074f07360732072c0721071f
071d071b071408120810080e080c080a080808060804080208000814b8ff
e0402b000001001406100000010006040000010004100000010010020000
01000200000001000002010802004a00b013034b024b5342014bb0c06300
4b6220b0f65323b8010a515ab005234201b0124b004b5442b0382b4bb807
ff52b0372b4bb007505b58b101018e59b0382bb00288b801005458b801ff
b101018e851bb0124358b900010111858d1bb900010128858d5959001816
763f183f123e113946443e113946443e113946443e113946443e11394660
443e11394660442b2b2b2b2b2b2b2b2b2b2b182b2b2b2b2b2b2b2b2b2b2b
182b1db0964b5358b0aa1d59b0324b5358b0ff1d594bb09353205c58b901
f201f04544b901f101f045445958b9033e01f2455258b901f2033e445959
4bb8015653205c58b9002001f14544b9002601f145445958b9081e002045
5258b90020081e4459594bb8019a53205c58b9002501f24544b9002401f2
45445958b909090025455258b9002509094459594bb8040153205c58b173
244544b1242445445958b917200073455258b9007317204459594bb80401
53205c58b1ca254544b1252545445958b9168000ca455258b900ca168044
59594bb03e53205c58b11c1c4544b11e1c45445958b9011a001c455258b9
001c011a4459594bb05653205c58b11c1c4544b12f1c45445958b9018900
1c455258b9001c01894459594bb8030153205c58b11c1c4544b11c1c4544
5958b90de0001c455258b9001c0de04459592b2b2b2b2b2b2b2b2b2b2b2b
2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b65
422b2b01b33b59635c456523456023456560234560b08b766818b0806220
20b163594565234520b003266062636820b003266165b059236544b06323
4420b13b5c4565234520b003266062636820b003266165b05c236544b03b
2344b1005c455458b15c406544b23b403b4523614459b347503437456523
456023456560234560b089766818b080622020b134504565234520b00326
6062636820b003266165b050236544b034234420b147374565234520b003
266062636820b003266165b037236544b0472344b10037455458b1374065
44b24740474523614459004b5342014b5058b108004259435c58b1080042
59b3020b0a124358601b2159421610703eb0124358b93b21187e1bba0400
01a8000b2b59b00c2342b00d2342b0124358b92d412d411bba0400040000
0b2b59b00e2342b00f2342b0124358b9187e3b211bba01a80400000b2b59
b0102342b0112342002b7475737500184569444569444569447373737374
757374752b2b2b2b74752b2b2b2b2b737373737373737373737373737373
737373737373737373732b2b2b45b0406144737400004bb02a534bb03f51
5a58b1070745b040604459004bb03a534bb03f515a58b10b0b45b8ffc060
4459004bb02e534bb03a515a58b1030345b040604459004bb02e534bb03c
515a58b1090945b8ffc06044592b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b
2b752b2b2b2b2b2b2b435c58b9008002bbb301401e017400735903b01e4b
5402b0124b545ab012435c5a58ba009f02220001007359002b7473012b01
732b2b2b2b2b2b2b2b737373732b002b2b2b2b2b2b004569447345694473
456944737475456944734569444569444569447374456944456944732b2b
2b2b2b732b002b732b74752b2b2b2b2b2b2b2b2b2b2b2b2b2b7374752b01
00>
[7793 ] AllocGlyphStorage
]def 
108 44 
PrepFor2015
Type42DictEnd
1 0 0 <00020100000005000500000300070000211121112521112101000400fc20
03c0fc400500fb002004c000>/EKJBOB+Arial AddT42Char 
1 42 11 <0001007cfe51026005d30010003d400a270f0100101207081010b80133b3
009f0e08b801334011079f0e5e0003100320030303ac119d8c182b10f65d
fdf6ed10f6ed003f3c3f3c3130015d012602113437363733060706070615
100101df95ce4d5abc8179273d232b012bfe51bc01f8010eeedafdfbd059
8a96bbbdfe1ffe20>/EKJBOB+Arial AddT42Char 
1 170 12 <0001007cfe51026005d300100065400c2802281002090a1001001209b801
33b30a9f0301b80133b4009f035e0eb8fff0b4101002550eb8fff8b40f0f
02550eb8ffe4b40d0d02550eb8ffec400f0a0a02550f0e1f0e020eac129d
8c182b10f65d2b2b2b2bfdf6ed10f6ed003f3c3f3c3130015d1323001134
272627262733161716151002fd81012b2b223d277a81bc5a4dcffe5101e0
01e1bcb9968a5ad2fbfddaeefef2fe08>/EKJBOB+Arial AddT42Char 
1 336 16 <0001004101b8026a026d0003002c401970027003024d014d020201230002
1a05700001001904708d182b4e10e45d10e6002f4ded31300071015d1335
211541022901b8b5b500>/EKJBOB+Arial AddT42Char 
1 406 17 <000100ba0000018700cd000300254018023c000a023c5f006f007f00af00
04a0000100a004a198182b10f65d5ded003fed313033353315bacdcdcd00
>/EKJBOB+Arial AddT42Char 
1 466 18 <00010000ffe7023905d300030053b90003ffdeb2143902b8ffde40201439
97030102039f03af0302037600011400000102010003000a03e80002e801
b801a9b5000004b37a182b103c10f4ed10ed003f3c3f3c87052e2b5d7d10
c43130015d2b2b1501330101a990fe581905ecfa1400>/EKJBOB+Arial AddT42Char 
1 578 19 <00020055ffe7041105c00010001d0155b10202435458400a1a1e0405141e
0d0d1709b8ffe8b40f0f025509b8ffe840190d0d02550911000c0f0f0255
00160c0c0255000c0d0d0255002f2b2b2bcd2f2b2bcd003fed3fed31301b
b10602435458400a1a1e0405141e0d0d1709b8fff4b40f0f065509b8ffe6
b40d0d065509b8ffee40190b0b0655091100100d0d065500100c0c065500
100b0b0655002f2b2b2bcd2f2b2b2bcd003fed3fed31301bb4062019101c
b8fff0b202200bbeffe00016ffe00012ffe0000fffe0406204068702880b
880fc90e0509070b180245134c154a19431b54135c155c19521b6b076b0b
63136c156b19601b79027706760b7a0f870698079610c918da02d606d60b
db0f1a1a1e0405141e0d0d17730940212334300901000910090209901f11
7300b8ffc0400e212334200040000200901ec78b182b10f65d2bed10f65d
712bed003fed3fed3130015d71005d003838383838013838385959131012
363332161612151002062322272613101633323611102623220706556bd3
a076b274426ad3a1d47991b9a97c7ca9a97e7c4a5d02d30104013dac5fb3
feffdafefefec3ad98b7019dfe97eff00168016aee698600>/EKJBOB+Arial AddT42Char 
1 1022 20 <000100df000002fb05c0000a00af402003400d11346b047f028f02990804
ac04010900060502030905010c0201ca0a00b8ffc0400a21233430000120
000100b8ffe0b41010025500b8ffea40110f0f0255001c0c0c0255000e0d
0d025500b8fff040190f0f065500100c0c065500100d0d0655001a0c0540
0d0f3405b8ffc0400e212334300501200540050205190bba013c01850018
2b4e10e45d712b2b10f62b2b2b2b2b2b2b5d712b3c4dfd3c003f3f173901
11393130015d005d2b212311060607353636373302fbb441d35497e22f74
047b3e7c1fae47ca5f00>/EKJBOB+Arial AddT42Char 
1 1242 21 <0001003c0000040705c0001e01c7b10602435458400911100d1813130655
0db8fff4b4111106550db8ffee4009101006550d1e14051eb8ffe8401713
1306551e1e111106551e1c0e1006551e0c0d0d06551eb802bb400c020a17
17201f10110202201f1112392fd4cd1112392fcd002fed2b2b2b2b3fed2b
2b2bc43231301bb10202435458400911100d0c121202550db8fff440090f
1102550d1e14051eb8ffe0400b121302551e140f1102551eb802bbb2020a
17b8ffe8b40b0b025517b8ffec400e0d0d02551717201f10110202201f11
12392fd4cd1112392f2b2bcd002fed2b2b3fed2b2bc43231301b40363b05
3b06bb05bf06bb07c708c91c07490c590c540e6b0c640e7a127a138912bc
12e51ae51bf01a0cbf0bb713021b101c101d101e1006befff00007ffe000
08fff00009fff0401a1e0a10080606ca1c1a141c1c1a081c1a030102081a
1c030d1e10b802a4b34f110111b80118b50d1e1405001eb802bb400f0102
0c0a7317d30000014021233401bb0281002000100138400c11b53f025f02
6f027f020402ba0224001f018fb18b182b10f65df4ed10f62b3c10f4ed00
3f3cfd3c3fedfd5de4111217390111121739870e2e2b0e7d10c401111239
313000383838380138383838005d015d7259592515212637363637363635
34262322060727363633321615140606070606070407fc37021725a39aef
a8997b829c01b913f8d1d3f648a7c2a25c1eadad413c63c07ec4e5666b93
9c8a13cfd9eaad58aabca4886131>/EKJBOB+Arial AddT42Char 
1 1796 22 <00010056ffe6041605c0002b0159b10202435458400b1918400d0d025518
1c0001b8ffc0402b0c0d02550129230a0d0f0c0f1e0a0a29151e1c041e29
1c05290d230d0c181901001220100c0c0255200726b8ffe8b40c0d025526
2f2bcd2f2bcd2fcd2fcd2f0012393f3f10ed10ed12392fedc610c6123910
c42b3210c42b3231301b4028050d160d450d860d0445115711761b035216
6c106a146416750d7914860d8a14891ba50d0a052003b8ffe0400b0b0c0d
0e040701230d0c01b802a4b340000100bb01180029000d0135b40c0c1504
18ba02a4001902684027151e1c05041e290d12735f206f200220180d0d06
55208007732640212334302601002610260226b8fff4b70d0d065526902d
18b80138b219d301ba01380000ffc0400b212334200040000200902cb801
92b18b182b10f65d2bedf4ed10f62b5d712bedf42b5ded003fed3fedfde4
1112392fed10fd5de411123901111217393130013838015d005d01715913
371616333236353426232207371633323635342623220607273636333216
1615140607161615140023222656b41f956b7fafa27d334c14120b73b886
6a698c14b421eaae78ca6b66648290fee8d6c1ff0183189987b0827ca114
9e02787d6382848420b5c767b2645f9c2e1ebd8ec0fef5e6>/EKJBOB+Arial AddT42Char 
1 2270 23 <0002001a0000041005ba000a000d0126403612580c680c9a0ca90cc90c05
4c034c0d94040312010208000c060307050a0b0307000c0c0d0dca030414
030304030d00020c0d040703bb02bb0008000201a0400a000404000c0c00
ca0a04b80266b705050a401d1f340ab8ffe0b4101002550ab8ffe6b40d0d
02550ab8ffeeb40d0d06550ab80137400d07402223340780213507900f02
b8ffc0400b0d14340002100220020302b8ffe0b40d0d025502b8ffe4b60d
0d065502b50eb8018cb18b182b10ec2b2b5d2b10f62b2bf42b2b2b2b3c10
e610fd3c003f3f10f43cf63c1139390111123939872e2b047d10c40f0f0f
313001435c58b9000dffdeb212390db8ffd4400b333903222d3903041d1d
3c2b2b2b2b595d005d435c5840140c400b390c8050390c4026390c221c39
0c402d392b2b2b2b2b5921112135013311331523110311010296fd84029d
93c6c6b4fe35015fa503b6fc4aa5fea102040295fd6b>/EKJBOB+Arial AddT42Char 
1 2622 24 <00010055ffe7042105a6001e0156b10202435458b90001ffc0400d0d0d02
55011c0e0a1e15151c12b802bb400b0f04041e1c0d0e01000718b8ffeab4
0f0f025518b8ffeab40d0d0255182f2b2bcd2fcd2f003fed3fed12392ffd
c410c42b31301b4029120c0d0d06550f0c0d0d06554b1a791d8a1d9613a7
13c30cd60cdb1b080913180e2a1a03093005300bbaffe00003ffe0401013
0a15121313ca0e0f140e13140e0f0db802a440130e0a1e15400ea00e020e
0e0f40150115151c12b802bbb70f0401d340000100b801184020041e1c0d
115f106f107f108f1004108007731840212334301801001810180218b8ff
f4b70d0d065518902012bc0135000f0195000d0138b20eb501ba01380000
ffc0400b212334200040000200901fb80192b18b182b10f65d2bedf4edf4
ed10f62b5d712bedf45d3c003fedfd5de43fed12392f5d11392f5d10ed10
e487082e2b057d10c4001112393130013838383801715d2b2b5913371616
33323635342623220607271321152103363332001514070623222655bd15
996c82b4ad8c578c28a98e02d9fdb74f8491c00108748df4c8fd0180108a
8bc4a29ab24f3f1602f1acfe765cfef6d1c791b2e000>/EKJBOB+Arial AddT42Char 
1 3064 25 <0002004dffe7041505c0001d002a014fb10202435458401f0f011f015f01
03011b281e400d010d0d14051e1b05221e140d0a1e01002510b8fff44019
0d0d0255101e17100f0f025517100c0c0255170c0d0d0255172f2b2b2bcd
2f2bcdd4cd10c5003fed3fed12392f5ded10c45d31301b402d6b19014407
4015441944205a1254206b03640764086a1264207408751c8508861cd608
d4161107200d0d065527b8ffe0b40d0d065523b8ffe0400b0d0d06552120
0d0d065507b8ffe0b42720232021b8ffe04011281e400d500d020d0d141b
01d35f000100b802684009051e1b05221e140d01b80138401200b5257310
40212334301001001010100210b8fff0b70c0c065510902c0aba0138001e
013940163f175f176f177f170417160c0c065517160d0d065517b80224b3
2bc78b182b10f62b2b5deded10f62b5d712bedf4ed003fed3fedfd5de411
12392f5ded313001383838382b2b2b2b015d005d59010726272623220706
060736363332121514060623220011103736333216011416163332363534
2623220603fbb3182c496b564155620241bc67b4fd77d084e1fee49d89e8
adddfd374f8e4e72a4a27b7aaa04530e6a304d303eeedc6360fef7d28aed
7e014b017c01a9c1a8c2fcdd5daa59b89e98afaf>/EKJBOB+Arial AddT42Char 
1 3534 26 <000100610000041605a7000d0070400ec40d01040d010402080409030d00
b802bb4030020104090c0d73030302402123344f025f026f0203021a0f08
7309eb004f015f015f02033f015f016f017f010401190eb80192b18b182b
4e10f45d713c4df4ed4e10f6712b3c4d10ed003f3f3cfd3c391139011112
39313001715d13352115060003060723361212376103b58cfeed4b360fb9
0382f38904faad8c95fe12fefbb8dbad01ea01c79c00>/EKJBOB+Arial AddT42Char 
1 3706 27 <00030053ffe7041905c00017002300300200b10202435458b40c001b1e2e
b8ffc04017131302552e2e12211e0605281e120d1e090c0c0c025509b8ff
f4b60d0d0255092b0fb8fff0b40f0f02550fb8ffe8b40b0b02550fb8ffe8
b60d0d02550f1803b8fff0b41010025503b8fff0b40f0f025503b8fff440
190d0d02550324150c0b0b0255150c0c0c0255150c0d0d0255152f2b2b2b
cd2f2b2b2bcd2f2b2b2bcd2f2b2bcd003fed3fed12392f2bed393931301b
b10602435458b71e090c0c0c065509b8fff4b60d0d0655092b0fb8ffe4b4
0f0f06550fb8ffe4b60d0d06550f1803b8fff0b40f0f065503b8fffc4022
0d0d06550324150c0c0c0655150c0d0d0655150c001b1e2e2e12211e0605
281e120d003fed3fed12392fed3939012f2b2bcd2f2b2bcd2f2b2bcd2f2b
2bcd31301b4037351601291649164926e60ce930050930017d007d017c04
7408710b720c750d7a178b008a018c048608810b840c860d8d17cc11c613
1222b8ffe0b21c201ab8ffe0b220202fb8ffe0b22d2026b8ffe0401e2920
0c001e18000c1b1e2ea02e012e12211e0605281e120d1e73bf090109b802
6740102b730f40202334300f01000f100f020fb80191b6321873b0030103
b80267b2247315b8ffc0400e2123342015401502159031c78b182b10f65d
2bedf45ded10f45d712bedf45ded003fed3fed12395d2fed393901111239
393130013838383838383838015d72710071595901262635343633321615
140607161615140023220035343613141633323635342623220603141616
333236353426232206016a706ce6bfc0ea6b6d878dfef6d9d9fef6916286
6b6885896667883a49905381a8ad827fa7031b29986aa0dadfa06697292c
c488bcff000101c08fc101546884835f638784fcff4d904fa68082aaa800
>/EKJBOB+Arial AddT42Char 
1 4366 32 <0002007201a1043a04060003000700474027050601040709002503012503
020725040406253002019f02cf020202bf05001a09011908575a182b4e10
e410e6002f4ded5d71ed3c10ed103ced10ed011139391139393130012135
2111213521043afc3803c8fc3803c8035ea8fd9ba800>/EKJBOB+Arial AddT42Char 
1 4478 37 <00030096000004e905ba0011001d002a0113b90004fff440470b0b065504
044623562366237309840906691a75057009730b8305830b062716090318
272a1e161d090913121e2a2a2929001c1d1e0201021f1e1e110008182606
0c1010025506b8ffe640330f0f025506120d0d025506060c0c025506080b
0b0655060c0c0c065506140d0d0655065425260c1c101002550c0a0d0d02
550cb8fff440150b0b06550c1a2c1d1e200120000100201010025500b8ff
f6b40f0f025500b8fff6b40d0d025500b8fffab40c0c025500b8fffab40c
0c065500b8fff0400a0d0d0655005d2b3b5c182b10f62b2b2b2b2b2b5d3c
fd3c4e10f62b2b2b4dedf42b2b2b2b2b2b2bed003f3cfd3c3f3cfd3c1239
2f3c10fd3c392f1139111239011217393130015d005d2b33112132161615
140607161615140e0223012132373636353426262321112132373e023534
26262321960226a8cb736667858f5780c18cfe93013d81384a4b46829efe
db016d5e26435a3a54958cfead05ba59b9655ea63327bc8067b160310352
1116664d496f29fba0070c386b4652793100>/EKJBOB+Arial AddT42Char 
1 4886 40 <000100a2000004e805ba000b0095401506051e080807070003041e020102
0a091e0b000807b8ffc0401d1012340754034a200a200d020a1a0d040920
0120000100201010025500b8fff6b40f0f025500b8fff6b40d0d025500b8
fffab40c0c025500b8fffab40c0c065500b8fff0400a0d0d0655005d0c3b
5b182b4e10f42b2b2b2b2b2b5d3c4dfd3c4e10f65d4df4e42b003f3cfd3c
3f3cfd3c12392f3c10fd3c3130331121152111211521112115a20424fc9e
032bfcd5038405baadfe3facfe0dad00>/EKJBOB+Arial AddT42Char 
1 5082 49 <0001009c0000051f05ba0009017db1120bb8ffc0400a13153408180c1602
5503b8ffe840210c16025508020303200708140707080207030308090402
02090708040320060605b8ffecb40f0f025505b8fff2400b0d0d02550512
0c0c025505b8fff7401a0b0b0655055d200b01200b500b600b700b800b05
0b0809200100b8ffc0400d13153420000100201010025500b8fff6b40f0f
025500b8fff6b40d0d025500b8fffa400b0c0c025500040b0b065500b8ff
f7b40c0c065500b8fff8400a0d0d0655005d0a3b59182b10f62b2b2b2b2b
2b2b5d2b3cfd3c105d71f42b2b2b2b3c10fd3c003f3c3f3c123939011139
3987042e2b877dc4b10602435458b90003ffe0b70c113408200c1134002b
2b5931302b2b012b435c58b40840463903b8ffc0b646390840323903b8ff
c0b632390722193902b8ffdeb619390722323902b8ffdeb6323907222339
02b8ffde400b2339070e1439070e133902b8fff4b61339070e1d3902b8ff
f4b61d39070e153902b8fff8b115392b2b2b2b2b2b2b012b2b2b2b2b2b00
2b2b2b2b59331133011133112301119cc70302bac7fcfe05bafb81047ffa
460480fb8000>/EKJBOB+Arial AddT42Char 
1 5508 55 <00010030000004ba05ba00070089400d05021e04030200080706050409b8
0273b320040104b80101b7062001022f030103b80101b5010120000100b8
ffe8400b1010025500080f0f025500b8fff2b40c0c025500b8ffe2b40d0d
025500b8fffcb40c0c065500b8fffeb40d0d065500b80273b308b699182b
10f62b2b2b2b2b2b5d3c10f45d3c10fde45de6103c103c003f3f3cfd3c31
3021112135211521110213fe1d048afe1b050dadadfaf300>/EKJBOB+Arial AddT42Char 
1 5682 72 <0002004bffe8041e043e0015001d015340171f001c150255035d055d0955
0b65036b056f09650b0815b8ffe4b40d0d065511b8ffe440520d0d06551d
1c0d0d06552712d905fa14f61a0431123a19311c41124d1a411c51125c19
521c61126d1a611c78067815f602f618100016010f0d1717501660167016
03161c0f9010a010021010041b1c0a0700ba02aa0001ffc0b41010025501
b8ffc04010101006551001010195131c040b17400db8ffdcb40d0d02550d
b8ffeeb40d0d06550db8ffeab40c0c06550db8ffc04009272a34b00d010d
1a1fb8ffc0b32526341fb8ffc040411e2334301f011f163310240740242a
341f073f074f070307200b0b025507180c0c0255071c0d0d0255070e0b0b
0655071c0c0c065507160d0d065507191e3437182b4e10f42b2b2b2b2b2b
5d2b4dfde44e10712b2bf6712b2b2b2b4ded003fedfd5d2b2be43fed1239
2f5d3cfd713c011112393912393130015d005d2b2b2b0171720117060623
22001110003332001114072116163332360121262726232206035eba2cee
b9e9feef0114dcd5010e01fce80ab285638cfdda02510c3856897ca90156
17a3b4011f0103010c0128fedefef91020afba680195864368a6>/EKJBOB+Arial AddT42Char 
1 6128 78 <00010088000003f805ba000b0261401b060c0d0d0655070656065a09030f
0df305f60603090c1010025506b8fff4b40c0c02550ab8fff4b40c0c0255
09b8fff4b40c0c025503b8ffe840100d0d06555503770a02120620132134
08b8fff0b312273409b8fff0b41227341205b8fff0b312213409b8fff040
84122734060404050406370947040525062d0a580a7703750ada03e30607
a60601230626072508390638093f0d4f0d59045906580759097d04790599
09c606d204d606e406e907f706f90815120a0a0503030402060607090908
0a0a050908082507061407070603040425050a1405050a0a090603040801
02000405060708080b0b000a04b8010f400905040c0c0655052208b8010f
402120073f070207100c0c0655071a900d010d0b2500022501019000013f
004f000200b8fffe40310e0e025500100d0d025500100c0c0255000a0b0b
025500120b0b065500120c0c065500080d0d065500190c0de1214766182b
2b4ef42b2b2b2b2b2b2b5d713c4d10ed10ed4e1071f62b5d4dedf42bed00
3f3c103c103c3f3c3f3c11173987052e2b047d10c487052e182b0e7d10c4
0710083c083c0310083c083cb10602435458400d4b09011f098403020918
0d1134002b5d7159313001435c58400a092c1d3909081d1d3c06b8ffdeb2
1d3906b8ffd4b2203906b8ffd4b121392b2b2b2b2b595d00715d0171002b
2b435c58b90006ffc0b2213903b8ffc0b2163903b8ffdeb2103906b8ffde
b2103903b8ffdeb20c3903b8ffdeb10b392b2b2b2b2b2b59012b2b2b435c
584012dd040108141639090814143c090814143c06b8fff6b2183906b8ff
ecb11b392b2b2b2b2b015d59005d2b2b2b2b2b015d712b33113311013301
012301071188b401aae9fe6a01bfdefea17f05bafcbc01b0fe76fd64021f
7afe5b00>/EKJBOB+Arial AddT42Char 
1 6792 83 <00020087fe690421043e0012001e0162408e0c102d103d104b10043f20b0
20021f20290c231d3215321d421d70209020083a173a1b4a174a1b59085b
0c5c175c1b6a086b0c69106d176b1bc020d314dd18dd1ad31ee414e41ee0
20ff201623042b102b1535043a1046044a105a10e50beb1dfe100b110e03
161c1c06070106161c0e0b000e1924d00a01100a400a600a800a0420400b
0b025520400d0d02550ab8ffe6400b0f0f02550a180d0d02550ab8fffab4
0c0c02550ab8ffeeb40b0b06550ab8fff4b40f0f06550ab8ffe840230c0c
06550a74011333023312250000c001019001a001b001f001041f013f014f
010301b8fffc401d0e0e025501100d0d025501100c0c025501100b0b0255
010c0b0b065501b8fff6b41010065501b8fffc40160f0f0655010c0c0c06
5501120d0d065501191f473718012b4e10f42b2b2b2b2b2b2b2b2b5d7172
3c4d10fdf4e410fd2b2b2b2b2b2b2b2b5d71ed003f3fed3f3fed11391239
3130005d015d717200711311331536363332161615140206232226271103
141633323635342623220687a43a926888d06a75df7b5a8f2e11a67678ab
a77473b1fe6905bd8a51518cff98a3fefb8b4c3afdfb03a4cdc4cbd5cbca
d700>/EKJBOB+Arial AddT42Char 
1 7244 91 <0001000f000003f10426001001dcb1020243545840150f010b0604020906
02060d0a000a0f180f0f02550f2f2b003f3f3f3f11173931301bb70f1201
0f22193906b8ffde405019395a0f96049608990e9a0fc005c006c007cb0f
090f4016391a031309150d1a1035013a0b81018e0b082f1257045907590b
580e9701980a980bb702b80cc80bca0ecc10da03d509d10ddb10e50a1212
b10602435458400b0c0012110f180d10065506b8ffe8400e0d1006550f06
00020d000a0a0206003f3c3f3c111239392b2b01111239391b4066060603
0708090901060609050403030b0f0f100e0d0d010f0f0d100b010009020d
0b030c100a060f020f0a10c600c60902102500091400000903020dc60d01
0d250c03140c0c030a090903030206100d0d0c0c000a4f120112490d7e0c
220a0f6106097e400ab8011bb74006500680060306b80243400e20037e02
224f00010049117cc4182b10f65df4ed1a19fd5dfd1a18ed10e510f4ede6
5d003f3c103c103c3f3c103c103c87052e2b5d877dc4872e182b5d7d10c4
00111239390f0f8708c4870e10c408c4870e10c4c408c4070e103c3c083c
59313001435c58b40e181d390bb8ffde400b1d390c221739032217390bb8
ffdeb2213910b8ffc0400a15390122213909401c392b2b2b2b2b2b2b2b59
5d71002b5d2b2b015d5933010133171617363737330101230327010f0184
fe99e1a32e1c2c25b3d7fe91018bddda3afee9022801fef947304233fbfe
0cfdce014a59fe5d>/EKJBOB+Arial AddT42Char 
/EKJBOB+Arial findfont /CharStrings get begin
/.notdef 0 def
/parenleft 11 def
/parenright 12 def
/hyphen 16 def
/period 17 def
/slash 18 def
/zero 19 def
/one 20 def
/two 21 def
/three 22 def
/four 23 def
/five 24 def
/six 25 def
/seven 26 def
/eight 27 def
/equal 32 def
/B 37 def
/E 40 def
/N 49 def
/T 55 def
/e 72 def
/k 78 def
/p 83 def
/x 91 def
end
/EKJBOB+Arial findfont /Encoding get
dup 0 /.notdef put
dup 40 /parenleft put
dup 41 /parenright put
dup 45 /hyphen put
dup 46 /period put
dup 47 /slash put
dup 48 /zero put
dup 49 /one put
dup 50 /two put
dup 51 /three put
dup 52 /four put
dup 53 /five put
dup 54 /six put
dup 55 /seven put
dup 56 /eight put
dup 61 /equal put
dup 66 /B put
dup 69 /E put
dup 78 /N put
dup 84 /T put
dup 101 /e put
dup 107 /k put
dup 112 /p put
dup 120 /x put
dup 173 /hyphen put
pop
end

userdict /pdf_svglb get setglobal
[/N295/EKJBOB+Arial 1 TZG
[ 24 /breve/caron/circumflex/dotaccent/hungarumlaut/ogonek
/ring/tilde/space/exclam/quotedbl/numbersign
/dollar/percent/ampersand/quotesingle/parenleft/parenright
/asterisk/plus/comma/hyphen/period/slash
/zero/one/two/three/four/five
/six/seven/eight/nine/colon/semicolon
/less/equal/greater/question/at/A
/B/C/D/E/F/G
/H/I/J/K/L/M
/N/O/P/Q/R/S
/T/U/V/W/X/Y
/Z/bracketleft/backslash/bracketright/asciicircum/underscore
/grave/a/b/c/d/e
/f/g/h/i/j/k
/l/m/n/o/p/q
/r/s/t/u/v/w
/x/y/z/braceleft/bar/braceright
/asciitilde/.notdef/bullet/dagger/daggerdbl/ellipsis
/emdash/endash/florin/fraction/guilsinglleft/guilsinglright
/minus/perthousand/quotedblbase/quotedblleft/quotedblright/quoteleft
/quoteright/quotesinglbase/trademark/fi/fl/Lslash
/OE/Scaron/Ydieresis/Zcaron/dotlessi/lslash
/oe/scaron/zcaron/.notdef/Euro/exclamdown
/cent/sterling/currency/yen/brokenbar/section
/dieresis/copyright/ordfeminine/guillemotleft/logicalnot/.notdef
/registered/macron/degree/plusminus/twosuperior/threesuperior
/acute/mu/paragraph/periodcentered/cedilla/onesuperior
/ordmasculine/guillemotright/onequarter/onehalf/threequarters/questiondown
/Agrave/Aacute/Acircumflex/Atilde/Adieresis/Aring
/AE/Ccedilla/Egrave/Eacute/Ecircumflex/Edieresis
/Igrave/Iacute/Icircumflex/Idieresis/Eth/Ntilde
/Ograve/Oacute/Ocircumflex/Otilde/Odieresis/multiply
/Oslash/Ugrave/Uacute/Ucircumflex/Udieresis/Yacute
/Thorn/germandbls/agrave/aacute/acircumflex/atilde
/adieresis/aring/ae/ccedilla/egrave/eacute
/ecircumflex/edieresis/igrave/iacute/icircumflex/idieresis
/eth/ntilde/ograve/oacute/ocircumflex/otilde
/odieresis/divide/oslash/ugrave/uacute/ucircumflex
/udieresis/yacute/thorn/ydieresis
/N244/Helvetica -1 TZ
[ 24 /breve/caron/circumflex/dotaccent/hungarumlaut/ogonek
/ring/tilde/space/exclam/quotedbl/numbersign
/dollar/percent/ampersand/quotesingle/parenleft/parenright
/asterisk/plus/comma/hyphen/period/slash
/zero/one/two/three/four/five
/six/seven/eight/nine/colon/semicolon
/less/equal/greater/question/at/A
/B/C/D/E/F/G
/H/I/J/K/L/M
/N/O/P/Q/R/S
/T/U/V/W/X/Y
/Z/bracketleft/backslash/bracketright/asciicircum/underscore
/grave/a/b/c/d/e
/f/g/h/i/j/k
/l/m/n/o/p/q
/r/s/t/u/v/w
/x/y/z/braceleft/bar/braceright
/asciitilde/.notdef/bullet/dagger/daggerdbl/ellipsis
/emdash/endash/florin/fraction/guilsinglleft/guilsinglright
/minus/perthousand/quotedblbase/quotedblleft/quotedblright/quoteleft
/quoteright/quotesinglbase/trademark/fi/fl/Lslash
/OE/Scaron/Ydieresis/Zcaron/dotlessi/lslash
/oe/scaron/zcaron/.notdef/Euro/exclamdown
/cent/sterling/currency/yen/brokenbar/section
/dieresis/copyright/ordfeminine/guillemotleft/logicalnot/.notdef
/registered/macron/degree/plusminus/twosuperior/threesuperior
/acute/mu/paragraph/periodcentered/cedilla/onesuperior
/ordmasculine/guillemotright/onequarter/onehalf/threequarters/questiondown
/Agrave/Aacute/Acircumflex/Atilde/Adieresis/Aring
/AE/Ccedilla/Egrave/Eacute/Ecircumflex/Edieresis
/Igrave/Iacute/Icircumflex/Idieresis/Eth/Ntilde
/Ograve/Oacute/Ocircumflex/Otilde/Odieresis/multiply
/Oslash/Ugrave/Uacute/Ucircumflex/Udieresis/Yacute
/Thorn/germandbls/agrave/aacute/acircumflex/atilde
/adieresis/aring/ae/ccedilla/egrave/eacute
/ecircumflex/edieresis/igrave/iacute/icircumflex/idieresis
/eth/ntilde/ograve/oacute/ocircumflex/otilde
/odieresis/divide/oslash/ugrave/uacute/ucircumflex
/udieresis/yacute/thorn/ydieresis
/N256/Times-Roman -1 TZ
PDFVars/TermAll get exec end end
%%EndProlog

%%BeginSetup
currentpagedevice /MediaProcessing known {<</MediaProcessingDetails << /Type 8 /ImageOrientation 0>> >> setpagedevice}{<< /StapleDetails<< /Type 8 /Portrait true>> >> setpagedevice} ifelse
Pscript_WinNT_Min dup /min_initialize get exec
featurebegin{
%%BeginNonPPDFeature: JobTimeout 0
0 /languagelevel where{pop languagelevel}{1}ifelse 2 ge{1 dict dup/JobTimeout  4 -1 roll put setuserparams}{statusdict/setjobtimeout get exec}ifelse
%%EndNonPPDFeature
}featurecleanup

featurebegin{
%%BeginNonPPDFeature: WaitTimeout 300
300 /languagelevel where{pop languagelevel}{1}ifelse 2 ge{1 dict dup/WaitTimeout 4 -1 roll put setuserparams}{statusdict/waittimeout 3 -1 roll put}ifelse
%%EndNonPPDFeature
}featurecleanup

featurebegin{
%%BeginFeature: *Collate False
<</Collate false>> setpagedevice
%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *HPColorAsGray False
<</ProcessColorModel /DeviceCMYK>> setpagedevice
%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *PageSize LETTER

  <</DeferredMediaSelection true /PageSize [612 792] /ImagingBBox null /MediaClass null>> setpagedevice
%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *MediaType Auto

%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *StapleLocation None

<<      /MediaProcessing (STAPLING)
        /MediaProcessingDetails <<
        /MediaProcessingOption (NONE)
        /MediaProcessingBoundary 0
        /Type 8 >> >> setpagedevice 
%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *OutputBin Auto

%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *Duplex None

    <</Duplex false /Tumble false>> setpagedevice
%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *HPDuplicateJobNameOverride SWFW

%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *HPCovers Other_Pages

%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *TextAsBlack False

%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *HPOrientRotate180 False

%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *HPConsumerCustomPaper True

%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *PrintQualityGroup PQGroup_1

%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *JRHDInstalled JRHDOff

%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *HPDocPropResourceData HPCabFileName

%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *JRConstraints JRCHDFull

%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *HPColorMode COLOR_MODE

%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *HPPJLEncoding UTF8

%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *HPJobAccounting HPJOBACCT_JOBACNT

%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *HPBornOnDate HPBOD

%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *HPXMLFileUsed hpmcpdps.xml

%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *PSAlignmentFile HPZLS3xr

%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *HPSmartHub Inet_SID_263_BID_514_HID_265

%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *PostScriptCustomPageSize False

%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *DuplexUnit Installed

%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *AccessoryOutputBins None

%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *InstalledMemory 384-495MB

%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *PrinterHardDisk NotInstalled

%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *JobRetention NotInstalled

%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *HPPassthrough True

%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *DeviceIsMopier NotInstalled

%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *AutoConfiguration NotInstalled

%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *HPOutputBinPMLRange 4-11

%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *HPPrnPropResourceData HPCabFileName

%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *HPInstallableHCO 3000Stacker-C8084

%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *HPMOutputBinHCOMap None

%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *HPMOutputBinHCOPMLMap None

%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *HPPDLType PDL_PS

%%EndFeature
}featurecleanup
featurebegin{
%%BeginFeature: *CombineMediaTypesAndInputBins Installed

%%EndFeature
}featurecleanup
1 setlinecap 1 setlinejoin
/mysetup [ 72 72 V 0 0 72 72 V 0 0 ] def 
%%EndSetup

userdict begin /ehsave save def end
%%Page: 1 1
%%PageBoundingBox: 12 13 598 780
%%EndPageComments
%%BeginPageSetup
/DeviceRGB dup setcolorspace /colspABC exch def
mysetup concat colspRefresh
%%EndPageSetup

%%BeginDocument: Pscript_Win_PassThrough
 PDF /docinitialize get exec

/pdfmark where {pop [ {ThisPage} 1 dict begin /BleedBox [  0 0 595.276 841.89 ] def currentdict end /PUT pdfmark } if

/pdfmark where {pop [ {ThisPage} 1 dict begin /TrimBox [  0 0 595.276 841.89 ] def currentdict end /PUT pdfmark } if

/pdfmark where {pop [ {ThisPage} 1 dict begin /ArtBox [  78.54691 565.12801 319.34 811.507 ] def currentdict end /PUT pdfmark } if
PDFVars begin PDF begin PDFVars/InitAll get exec
save
8.362 -24.945 translate
0 0 595.276 841.89 true PDF begin PDFVars begin AS end end
userdict /pdf_svglb currentglobal put true setglobal
 Adobe_CoolType_Utility begin ct_MakeOCF begin ct_saveCIDInit
%!PS-Adobe-3.0 Resource-CIDFont
%%DocumentNeededResources: procset CIDInit
%%IncludeResource: procset CIDInit
%%BeginResource: CIDFont TXDYVB+MS-Gothic
%%Title: (TXDYVB+MS-Gothic Adobe Identity 0)
%%Version: 1
/CIDInit /ProcSet findresource begin
20 dict begin
/CIDFontName /TXDYVB+MS-Gothic def
/CIDFontVersion 1 def
/CIDFontType 0 def
/CIDSystemInfo 3 dict dup begin
  /Registry (Adobe) def
  /Ordering (Identity) def
  /Supplement 0 def
end def
/CIDMapOffset 0 def
/FDBytes 0 def
/GDBytes 3 def
/FontBBox [0 -137 1000 859] def
/FontInfo 2 dict dup begin
/FSType 0 def
/OrigFontType /TrueType def
end readonly def
/CIDCount 65535 def
/FDArray 1 array
dup 0
  %ADOBeginFontDict
  10 dict begin
  /FontType 1 def
  /PaintType 0 def
  /FontName /TXDYVB+MS-Gothic def
/FontMatrix [1 1000 div 0 0 1 1000 div 0 0 ] def
  %ADOBeginPrivateDict
  /Private 8 dict dup begin
  /BlueValues [-15 0 600 650] def
  /MinFeature {16 16} def
  /LanguageGroup 1 def
  /password 5839 def
  /lenIV 4 def
  end def
  %ADOEndPrivateDict
currentdict end
%ADOEndFontDict
put def
/GlyphDirectory 1 dict def
ct_GlyphDirProcs begin GlyphDirectory +
0 <10bf31700ab469119f4e> |
!
end
%%BeginData: 21 Binary Bytes
(Binary) 0 StartData
%%EndData
%%EndResource
 ct_restoreCIDInit /TXDYVB+MS-Gothic-Identity-H /Identity-H 0 [/TXDYVB+MS-Gothic] ct_ComposeFont pop end end 

userdict /pdf_svglb get setglobal
%PDF_BeginEncoding: N143 (TXDYVB+MS-Gothic-Identity-H)
/N143 (TXDYVB+MS-Gothic-Identity-H) /Identity-H [ (TXDYVB+MS-Gothic) ]
 /Adobe-Identity [ /Serif ] 0 TZzero
userdict /pdf_svglb currentglobal put true setglobal
 Adobe_CoolType_Utility begin ct_MakeOCF begin ct_saveCIDInit
%!PS-Adobe-3.0 Resource-CIDFont
%%DocumentNeededResources: procset CIDInit
%%IncludeResource: procset CIDInit
%%BeginResource: CIDFont JVAQLV+SymbolMT
%%Title: (JVAQLV+SymbolMT Adobe Identity 0)
%%Version: 1
/CIDInit /ProcSet findresource begin
20 dict begin
/CIDFontName /JVAQLV+SymbolMT def
/CIDFontVersion 1 def
/CIDFontType 0 def
/CIDSystemInfo 3 dict dup begin
  /Registry (Adobe) def
  /Ordering (Identity) def
  /Supplement 0 def
end def
/CIDMapOffset 0 def
/FDBytes 0 def
/GDBytes 3 def
/FontBBox [0 -220 1113 1005] def
/FontInfo 2 dict dup begin
/FSType 0 def
/OrigFontType /TrueType def
end readonly def
/CIDCount 65535 def
/FDArray 1 array
dup 0
  %ADOBeginFontDict
  10 dict begin
  /FontType 1 def
  /PaintType 0 def
  /FontName /JVAQLV+SymbolMT def
/FontMatrix [1 1000 div 0 0 1 1000 div 0 0 ] def
  %ADOBeginPrivateDict
  /Private 8 dict dup begin
  /BlueValues [-15 0 600 650] def
  /MinFeature {16 16} def
  /LanguageGroup 1 def
  /password 5839 def
  /lenIV 4 def
  end def
  %ADOEndPrivateDict
currentdict end
%ADOEndFontDict
put def
/GlyphDirectory 1 dict def
ct_GlyphDirProcs begin GlyphDirectory +
0 <10bf31704faacd68130743d1032b19039b05d30ed4559c5ecf2da4ace2ab
53168b5c58eb3d8c199cf05ae7> |
!
end
%%BeginData: 21 Binary Bytes
(Binary) 0 StartData
%%EndData
%%EndResource
 ct_restoreCIDInit /JVAQLV+SymbolMT-Identity-H /Identity-H 0 [/JVAQLV+SymbolMT] ct_ComposeFont pop end end 

userdict /pdf_svglb get setglobal
%PDF_BeginEncoding: N150 (JVAQLV+SymbolMT-Identity-H)
/N150 (JVAQLV+SymbolMT-Identity-H) /Identity-H [ (JVAQLV+SymbolMT) ]
 /Adobe-Identity [ /Serif ] 0 TZzero
userdict /pdf_svglb currentglobal put true setglobal
ct_T42Dict begin
-0.664 -0.324 2 1.004
 256 array 0 1 255 {1 index exch /.notdef put} for  /JVAQLV+ArialMT
Type42DictBegin
[<00010000000a000a000a000a63767420962ad276000000ac000006306670
676dcc79599a000006dc0000066e676c7966dcddf4dc00004d1c00000414
686561641e076d8c00000d4c0000003668686561123312ff00000d840000
0024686d74780e34584000000da800001a286c6f63610019d258000027d0
00001a2c6d6178700b470ca8000041fc000000207072657052fec4e90000
421c00000aff6764697200000000000000000000000005ba001905ba001a
05a70019042600180000ffe70000ffe80000ffe7fe69ffe805ba0019fe69
ffe802ea000000b8000000b80000000000a800ad016900ad00bf00c201f0
001800af00b900b400c800170044009c007c009400870006005a00c80089
005200520005004400940119ffb4002f00a1000300a100cd00170057007e
00ba00160118ffe9007f008503d300870085000d002200410050006f008d
014cff75005c00df04830037004c006e00700180ff58ff8eff92ffa400a5
00b903c8fffd000b001a0063006300cdffee05d8ffdc002d005c00950099
00df019209b500400057008000b9039d0072009a035d0401ff67fffa0003
0021007700cd0004004d00cd01c0022b004c006500e70118017c034305d8
ffa3ffb0ffc40003001c005d0068009a00ba013501470221055cff4dffcd
0016002d00780080009900b200b600b600b800bd00da010c05f0ffa4fff0
0019002c0049007f00b400ce01c003fefd81fe3f00000005001800290039
0049006f00be00c700d0012301c1026f050c05320540057affd400140031
0055005700a700b400e601f7027e027e027f03c60446ff42000e00850091
00bf00c200c500e1011a012f014f01560229026f029e03720008002c0031
0031006400690089009800c700de012b01b6020c02cf03a304ab04fb061d
fee0ff0e00060026009b009d00c1010d011801200173018201d601e30243
025f029b02e2039404a904d20761001c005e006d008d00ab00f701120138
0151015b0168017c01870191019901cd01d001e802410254026b02ef0368
037103bd044204420453047304830586058b06e8fe58fec4fed1fef7ff32
ff860051007c008100910095009e00b400b900cf00d900d900df00e20105
010b010e010e012001210155017b017b017e018d01a201a801a901b401d0
01d001e201e901f201f501fb020002000206021b02210222022202230272
02770294029c02cf02cf02d002ec02f903170322032b0335033c0359036f
037103870390039003b503e1041a04cf04ff053205320596059f05a805ab
05c205f0060c0782080008ccfca3fd2afddefe00fe88fe96feb2feb4ffe1
00150019001a001c001f003c005100610061006a0078009600a500af00d3
010c0118011a012a013e014c0151015f016a0171017801820184019a01a5
01a801a901ae01bc01cd01d701ef0200020d021c02210222022e02350242
024f024f025e026502710290029202b402d602fa0307030b030f0315032a
0347035d036503740379039603b003cc03dd03e203f603fc03fc03ff040a
041f04220426042b0447045f0475049e04e704e7055c05cb05e5060a066d
068606b806f10736073e07500751075d078f07b607d4086000b600c300b5
00b700000000000000000000000001e00381034503b5008e0233041902ce
02ce002d005f0064034d023f000002a80188027d01b402240578063b023b
014e00f00426029402c6029f02f6023b034d014b0153006a023100000000
0000061404aa0000003c04c300ed04bc026502ce03b50078060c017e02ef
060c00b201000239000001c50330042b03cb00da03df010704a100db040a
011701ed02a70350010b01bd043e05580021039c00ae0371017d00b50245
00000afb088c012b014e01aa00870054013201f803ff0003024e00b40037
03e30083006b02d800ed00770088009701640467008e0033017c00e700a6
029e0329056e062a061501c90269048a021301b4000204a9000002390124
010305140084015d039a06ef02d9007500cf040a00de03ac04bc02cf02ae
034d04f005520168006d007d00860071ff810079055804d2016700030156
002504e00094007c033204210094007f0072005c002f00b6001800ba00b8
0041034d00720018001f004c016a01550099009a009a009800b200040078
006900140057006e00ce00b4065402b80067050e016500e7000004cbfe52
005affa60099ff67006eff92002dffd40087ff7c00b800a800e5008f00a8
0185fe7b0070001e00d900de014c054602cf0546ff2d028a02d902530296
00b700000000000000000000000000000125011800ea00ea00ae0000003e
05bb008a04d70053003fff8cffd500150028002200990062004a00e4006d
00ee00e5004803c00033fe4e02b1ff460370007905df0051ffa7ff1f010a
0068ff6c004f00bc00a507050061072b4043555441403f3e3d3c3b3a3938
373534333231302f2e2d2c2b2a292827262524232221201f1e1d1c1b1a19
1817161514131211100f0e0d0c0b0a090807060504030201002c45234660
20b02660b004262348482d2c452346236120b02661b004262348482d2c45
234660b0206120b04660b004262348482d2c4523462361b0206020b02661
b02061b004262348482d2c45234660b0406120b06660b004262348482d2c
4523462361b0406020b02661b04061b004262348482d2c0110203c003c2d
2c20452320b0cd442320b8015a51582320b08d44235920b0ed51582320b0
4d44235920b09051582320b00d44235921212d2c20204518684420b00160
2045b04676688a4560442d2c01b10b0a432343650a2d2c00b10a0b432343
0b2d2c00b0172370b101173e01b0172370b10217453ab10200080d2d2c45
b01a234445b01923442d2c2045b00325456164b050515845441b2121592d
2cb00143632362b0002342b00f2b2d2c2045b0004360442d2c01b00643b0
0743650a2d2c2069b04061b0008b20b12cc08a8cb8100062602b0c642364
615c58b00361592d2c45b0112bb0172344b0177ae4182d2c45b0112bb017
23442d2cb01243588745b0112bb0172344b0177ae41b038a45186920b017
23448a8a8720b0a05158b0112bb0172344b0177ae41b21b0177ae4595918
2d2c2d2cb0022546608a46b040618c482d2c4b53205c58b002855958b001
85592d2c20b0032545b019234445b01a23444565234520b00325606a20b0
09234223688a6a606120b01a8ab000527921b21a1a40b9ffe0001a45208a
54582321b03f1b235961441cb114008a5279b31940201945208a54582321
b03f1b235961442d2cb110114323430b2d2cb10e0f4323430b2d2cb10c0d
4323430b2d2cb10c0d432343650b2d2cb10e0f432343650b2d2cb1101143
2343650b2d2c4b525845441b2121592d2c0120b003252349b04060b02063
20b000525823b002253823b002256538008a63381b212121212159012d2c
4bb06451584569b00943608a103a1b212121592d2c01b005251023208af5
00b0016023edec2d2c01b005251023208af500b0016123edec2d2c01b006
2510f500edec2d2c20b001600110203c003c2d2c20b001610110203c003c
2d2cb02b2bb02a2a2d2c00b00743b006430b2d2c3eb02a2a2d2c352d2c76
b8022323701020b802234520b0005058b00161593a2f182d2c21210c6423
648bb84000622d2c21b08051580c6423648bb82000621bb200402f2b59b0
02602d2c21b0c051580c6423648bb81555621bb200802f2b59b002602d2c
0c6423648bb84000626023212d2cb4000100000015b00826b00826b00826
b008260f10161345683ab001162d2cb4000100000015b00826b00826b008
26b008260f1016134568653ab001162d2c4b53234b515a5820458a60441b
2121592d2c4b545820458a60441b2121592d2c4b53234b515a58381b2121
592d2c4b5458381b2121592d2cb0134358031b02592d2cb0134358021b03
592d2c4b54b012435c5a58381b2121592d2cb012435c580cb00425b00425
060c6423646164b807085158b00425b00425012046b01060482046b01060
48590a21211b2121592d2cb012435c580cb00425b00425060c6423646164
b807085158b00425b00425012046b8fff060482046b8fff06048590a2121
1b2121592d2c4b53234b515a58b03a2b1b2121592d2c4b53234b515a58b0
3b2b1b2121592d2c4b53234b515ab012435c5a58381b2121592d2c0c8a03
4b54b00426024b545a8a8a0ab012435c5a58381b2121592d2c4b5258b004
25b0042549b00425b00425496120b0005458212043b0005558b00325b003
25b8ffc038b8ffc038591bb04054582043b0005458b00225b8ffc038591b
2043b0005458b00325b00325b8ffc038b8ffc0381bb00325b8ffc0385959
5959212121212d2c462346608a8a462320468a608a61b8ff806223201023
8ab902c202c28a70456020b0005058b00161b8ffba8b1bb0468c59b01060
68013a2d2cb1020042b123018851b1400188535a58b910000020885458b2
02010243604259b12401885158b920000040885458b2020202436042b124
01885458b2022002436042004b014b5258b2020802436042591bb9400000
80885458b202040243604259b94000008063b80100885458b20208024360
4259b94000010063b80200885458b202100243604259b94000020063b804
00885458b202400243604259595959592d2cb0024354584b53234b515a58
381b2121591b21212121592d000000010000000300003e6810595f0f3cf5
081b080000000000a2e3272a00000000b9d5b4f6faaffd671000080c0000
0009000100010000000000010000073efe4e00431000faaffe2610000001
0000000000000000000000000000068a0600010000000000023900000239
0000023900b002d7005e0473001504730049071d0077055600580187005a
02aa007c02aa007c031d004004ac0072023900aa02aa0041023900ba0239
000004730055047300df0473003c047300560473001a047300550473004d
047300610473005304730055023900b9023900aa04ac007004ac007204ac
00700473005a081f006f0556fffd0556009605c7006605c7009e055600a2
04e300a80639006d05c700a4023900bf04000037055600960473009606aa
009805c7009c063900630556009e0639005805c700a10556005c04e30030
05c700a105560009078d0019055600090556000604e300290239008b0239
00000239002703c100360473ffe102aa00590473004a0473008604000050
047300460473004b02390013047300420473008701c7008801c7ffa20400
008801c7008306aa00870473008704730044047300870473004802aa0085
0400003f02390024047300830400001a05c700060400000f040000210400
002802ac0039021400bc02ac002f04ac00570556fffd0556fffd05c70068
055600a205c7009c0639006305c700a10473004a0473004a0473004a0473
004a0473004a0473004a040000500473004b0473004b0473004b0473004b
023900bd023900230239ffe5023900090473008704730044047300440473
004404730044047300440473008304730083047300830473008304730049
033300800473006b0473001b0473005102cd006d044c000104e3009905e5
000305e50003080000e102aa00de02aa003d0464004e0800000106390053
05b4009a0464004e0464004d0464004d0473fffd049c00a003f4003805b4
007a069600a1046400000231000002f6002f02ec002d0625007f071d0044
04e3008104e3009e02aa00e804ac0072046400540473002e0464003304e5
001a047300860473008c080000ef0556fffd0556fffd0639006308000081
078d00520473fffc0800000002aa005302aa004701c7008001c7006c0464
004e03f4002f04000021055600060156fe390473ffe402aa005c02aa005c
040000170400001704730049023900b901c7006c02aa0047080000250556
fffd055600a20556fffd055600a2055600a20239008d0239ffe002390004
0239001506390063063900630639006305c700a105c700a105c700a10239
00c602aa001902aa000602aa001d02aa002e02aa00e502aa00a202aa006b
02aa003a02aa00b702aa00280473000001c700030556005c0400003f04e3
002904000028021400bc05c7fffd0473004905560006040000210556009e
0473008704ac007204ac00a102aa006b02aa001902aa002106ac006b06ac
006b06ac0021047300000639006d04730042023900b10556005c0400003f
05c700660400005005c700660400005004730046046bffe102aa01f10556
fffd0473004a0556fffd0473004a05c7009e04eb004705c7fffd055600a2
0473004b055600a20473004b0473009601c7004204730096025500880473
009a02ac008305c7009c0473008705c7009c047300870639006304730044
05c700a102aa008505c700a102aa003c0556005c0400003f04e300300239
002404e300300300002305c700a10473008305c700a10473008304e30029
0400002804e3002904000028046800a4063900600662005504a000480474
00480391006204f000440329002e05300048046bffe1040000b002eb0052
08c000330800004f040000990800004f040000990800004f040000980400
009807d5016a05c0009e04ab007204d5009d04ac007104d5022204d50105
05abffe9050001c905ab027e05abffe905ab027e05abffe905ab027e05ab
ffe905abffe905abffe905abffe905abffe905ab01c005ab027e05ab01c0
05ab01c005abffe905abffe905abffe905ab027e05ab01c005ab01c005ab
ffe905abffe905abffe905ab027e05ab01c005ab01c005abffe905abffe9
05abffe905abffe905abffe905abffe905abffe905abffe905abffe905ab
ffe905abffe905abffe905abffe905abffe905abffe905abffe905ab02d6
05ab006605abffea05d5ffff04d500920800000007eb013007eb012007eb
013007eb012004d500b204d5008004d5002a082b0198086b01b807550010
060000f40600006f0440003a0540003704c0003f04150040040000250600
005505e100bf038d008904d5ffd90180008002d50086071500610296000f
04d5009202d6008302d6008304d500b202d600700556fffd0473004a05c7
00660400005005c7006604000050055600a20473004b055600a20473004b
055600a20473004b0639006d047300420639006d047300420639006d0473
004205c700a40473008705c7001f047300060239ffce0239ffce0239ffe4
0239ffe40239fff60239fff5023900a301c700660400003701c7ffa20556
009604000088040000860473009601c7fffa05c7009c0473008705c900a5
0473008b0639006304730044063900630473004405c700a102aa006b0556
005c0400003f04e300300239000c05c700a10473008305c700a104730083
05c700a10473008305c700a104730083078d001905c70006055600060400
002101c700890556fffd0473004a08000001071d00440639005304e30081
023900b9078d001905c70006078d001905c70006078d001905c700060556
00060400002101c7008a02aaffe10473001b04cd005a06ac006b06ac0022
06ac002206ac004a02aa00e202aa006b02aa00de02aaffea0557ffff0646
ffa706b4ffa80312ffa80632ffa706d8ffa70605ffa701c7ff780556fffd
055600960558fffe055600a204e3002905c700a4023900bf055600960558
000b06aa009805c7009c0533006d0639006305c700a40556009e04f20094
04e30030055600060556000906af007f05fb0061023900040556000604a0
0048039100620473008b01c7006b04600088049a008c0400001903870048
0473008b0473005c01c700890400008604000018049c00a00400001a0395
005c04730044048d008303db0056046000880433001105b4007a063f0057
01c7ffc9046000880473004804600088063f0057055700a206eb00320455
00a105c000640556005c023900bf02390004040000370875000d081500a4
06d5003104a900a10515000a05c000a00556fffd054000a7055600960455
00a1056b0000055600a20763000704d5004e05c000a105c000a104a900a1
0540001206aa009805c700a40639006305c000a00556009e05c7006604e3
00300515000a061500520556000905eb009f05550057075500a1078000a1
06550000071500a8054000a505c00055081500a405c7001a0473004a0495
005b0440008802eb008804ab00000473004b055afffb03ab003204780087
047800870380008604ab00180580008c046b008804730044045500880473
00870400005003aa0026040000210695004b0400000f0495008a042b0045
066b008d0695008d0500002805c0008b042b008404150030060000890455
001f0473004b0473000002eb00890415004b0400003f01c7008802390009
01c7ffa20740001306800083047300000380008604000021046b008803e9
00a1034a008808000041089500a00585002d02aa010102aa001e02aa0031
02aa003102aa010102aa007e02aa007e02aa008c02aa008c02aa010102aa
001002aa010102aa01210310007d02aa008c023300d202aa030b02aaff04
023900b90481006904560032033100190411002d04d1009601f9009b030f
005f04ca009b04b8008c01f9009b0413002803b0005003b4003c04ca009b
04cf005001f9009b02d2003c0498005a043c00190488006e045f007303b1
001903d4000a0466009604130028058e00640524002803f2009b03f2009b
03f2009b01e3005a0356005a0686009b01f9ffac041300280413002803b4
ff5703b4ff570448002d058e0064058e0064058e0064058e006404810069
048100690481006904560032033100190411002d04d10096024b0000034a
000004b8008c024b00000413002803b0005003b4003c04cf005002d2003c
0498005a0488006e045f007303d4000a0466009604130028058e00640524
002801f9009b0456003203b00050045f0073049b003c0000ffdc0000ff25
0000ffdc0000fe51028d00ab028d00a002da0043034d007901a8ffba019c
004601e50046019c0046019c004601ad0048019c004601b1004601510046
0435017c0435012e043500b7043500810435012c043500be043500af0435
00810435009a043500db04350085028d00c1043500b30600010006000100
02420036060001000435009e04350098043500cb06000100060001000600
0100060001000600010001b1004606000100060001000600010006000100
06000100060001000600010006000100051bffba06000100060001000600
010005b5003a05b5003a01f4ffba01f4ffba060001000600010006000100
060001000481003604350036043dffba043dffba03e9004a03e9004a067f
0014077600140327ffba041effba067f0014077600140327ffba041effba
051b003204b5002406000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
06000100060001000600010001cf003001b1004601b1004601b1004001b1
004606000100060001000000ffdc0000fe510000ff160000ff160000ff16
0000ff160000ff160000ff160000ff160000ff160000ff160000ffdc0000
ff160000ffdc0000ff200000ffdc0473004a080000000600010006000100
060001000600010006000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
0100060001000600010006000100028d007f028d005d0600010004ee0015
034d007901a8000e01d6ffdc01a8005601d60010037500320375003201a8
002d01d60013051b003204b5002401f4ffba01f4ffba01a8009301d60013
05b5003a05b5003a01f4ffba01f4ffba024200000300fff705b5003a05b5
003a01f4ffba01f4ffba05b5003a05b5003a01f4ffba01f4ffba04810036
04350036043dffba043dffba0481003604350036043dffba043dffba0481
003604350036043dffba043dffba02b3005f02b3005f02b3005f02b3005f
03e9004a03e9004a03e9004a03e9004a0692003e0692003e043fffba043f
ffba0692003e0692003e043fffba043fffba08c9003e08c9003e06c5ffba
06c5ffba08c9003e08c9003e06c5ffba06c5ffba04a7ffba04a7ffba04a7
ffba04a7ffba04a7ffba04a7ffba04a7ffba04a7ffba045a002a039a0036
0435ffba0327ffba045a002a039a00360435ffba0327ffba064f0027064f
00270224ffba021affba04a7004604a700460224ffba021affba04cf002d
04cf002d0327ffba0327ffba040d0047040d004701a8ffba01a8ffba02b4
002302b400230327ffba0327ffba043500450435004501f4ffba01f4ffba
024200360300fff7039affba0327ffba0375003203750032051b003204b5
0024051b003204b5002401f4ffba01f4ffba045a004004ce0049045a0026
04ce0039045a005304ce004a045a005304ce004a0600010006000100019c
0046019c00460600010006000100060001000151004601b1004606000100
0600010001ad004801e5004606000100060001000600010001b1004601b1
004601b1004601b1004601b1004001cf003006000100019c0046019c0046
060001000600010006000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
010006000100028d00ca028d00c7028d00c6060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
0600010006000100060001000600010006000100060001000100ffba0800
ffba1000ffba06dc0063053f004406d500a1055b00830000fddc0000fc2f
0000fca60000fe540000fcd70000fd730000fe290000fe0d0000fd110000
fc670000fd9d0000fbf50000fc720000fed50000fed50000ff02041b00a0
06ac006b06ac00190000feb60000fd730000fe080000fca60000fe530000
fd110000fbc80000faf40000faaf0000fc720000fbaa0000fb6a0000fcf1
0000fc7d0000fbdd0000fcc10000fb980000fdea0000fe840000fdc20000
fcf10000fd5f0000fe760000febc0000fceb0000fd6c0000fd580000fc90
0000fd150000fc2c0000fc130000fc120000fb960000fb9601c700880556
fffd0473004a0556fffd0473004a0556fffd0473004a0556fffd0473004a
0556fffd0473004a0556fffd0473004a0556fffd0473004a0556fffd0473
004a0556fffd0473004a0556fffd0473004a0556fffd0473004a0556fffd
0473004a055600a20473004b055600a20473004b055600a20473004b0556
00a20473004b055600a20473004b055600a20473004b055600a20473004b
055600a20473004b0239006301c7001f023900ba01c7007c063900630473
004406390063047300440639006304730044063900630473004406390063
047300440639006304730044063900630473004406dc0063053f004406dc
0063053f004406dc0063053f004406dc0063053f004406dc0063053f0044
05c700a10473008305c700a10473008306d500a1055b008306d500a1055b
008306d500a1055b008306d500a1055b008306d500a1055b008305560006
04000021055600060400002105560006040000210556fffd0473004a0239
ffe201c7ffb0063900630473004405c700a10473008305c700a104730083
05c700a10473008305c700a10473008305c700a1047300830000fefe0000
fefe0000fefe0000fefe0455fffd02eb000c07630007055afffb04a900a1
0380008604a900a10380008605c700a4046b00880473fffd040000140473
fffd04000014055600090400000f05550057042b0045055500a104730087
0605006304730055063900600473004405b5003a01f4ffba0224ffba021a
ffba04a7004601f4009e01f4001001f4001b01f4001001f4006b01f4fff9
0227ffce01a8000f01a8fff502aa00a402aa00a401a8000e01a8005601a8
00560000ffcf01a8000f01d6ffbf01a8fff501d6ffcd01a8001d01d6fff5
01a8009301d6001303750032037500320375003203750032051b003204b5
002405b5003a05b5003a01f4ffba01f4ffba05b5003a05b5003a01f4ffba
01f4ffba05b5003a05b5003a01f4ffba01f4ffba05b5003a05b5003a01f4
ffba01f4ffba05b5003a05b5003a01f4ffba01f4ffba05b5003a05b5003a
01f4ffba01f4ffba05b5003a05b5003a01f4ffba01f4ffba048100360435
0036043dffba043dffba0481003604350036043dffba043dffba04810036
04350036043dffba043dffba0481003604350036043dffba043dffba0481
003604350036043dffba043dffba0481003604350036043dffba043dffba
02b3003202b3003202b3005f02b3005f02b3005f02b3005f02b3003202b3
003202b3005f02b3005f02b3005f02b3005f02b3005f02b3005f02b30038
02b3003802b3004902b3004903e9004a03e9004a03e9004a03e9004a03e9
004a03e9004a03e9004a03e9004a03e9004a03e9004a03e9004a03e9004a
03e9004a03e9004a03e9004a03e9004a0692003e0692003e043fffba043f
ffba0692003e0692003e043fffba043fffba0692003e0692003e043fffba
043fffba08c9003e08c9003e06c5ffba06c5ffba08c9003e08c9003e06c5
ffba06c5ffba04a7ffba04a7ffba045a002a039a00360435ffba0327ffba
064f0027064f0027064f00270224ffba021affba064f0027064f00270224
ffba021affba064f0027064f00270224ffba021affba064f0027064f0027
0224ffba021affba064f0027064f00270224ffba021affba04a7004604a7
004604a7004604a70046067f0014077600140327ffba041effba067f0014
077600140327ffba041effba04cf002d04cf002d0327ffba0327ffba04cf
002d04cf002d0327ffba0327ffba04cf002d04cf002d0327ffba0327ffba
067f0014077600140327ffba041effba067f0014077600140327ffba041e
ffba067f0014077600140327ffba041effba067f0014077600140327ffba
041effba067f0014077600140327ffba041effba040d0047040d004701a8
ffba01a8ffba040d0047040d004701a8ffba01a8ffba040d0047040d0047
01a8ffba01a8ffba040d0047040d004701a8ffba01a8ffba043500450435
004501f4ffba01f4ffba0435004504350045043500450435004504350045
0435004501f4ffba01f4ffba04350045043500450481003604350036043d
ffba043dffba024200360300fff7031a001a031a001a031a001a03750032
037500320375003203750032037500320375003203750032037500320375
003203750032037500320375003203750032037500320375003203750032
051bffba04b5ffba051b003204b5002401f4ffba01f4ffba037500320375
0032051b003204b5002401f4ffba01f4ffba051b003204b50024067f0045
067f0045067f0045067f004501a800280000fe290000fea20000ff300000
ff1d0000ff120000ff920000fe7e08fc003208ad00320000ffb50000ffb6
0000feed0000ff640000fe7e0000ff9f018d000002f6fffd0000fe820000
ff1004cd00320000ff580000ff580000ff640692003e0692003e043fffba
043fffba08c9003e08c9003e06c5ffba06c5ffba045a002a039a00360435
ffba0327ffba034d007902b400230242003601f4ffba0290ffba01f4002f
01f4003b01f4001201f400b101f4006d067f00140776001401f9009b0000
fed902bc000003f2009b045afff504cefff5045a005304ce004a045a0053
04ce004a045a005304ce004a045a005304ce004a045a005304ce004a045a
005304ce004a04350071043500ad045a000f04ce000f000000000000002a
0000002a0000002a0000002a0000002a0000002a0000002a0000002a0000
002a0000002a0000002a0000002a0000002a0000002a0000002a0000002a
0000002a0000002a0000002a0000002a0000002a0000002a0000002a0000
002a000001e4000001e4000001e4000001e4000001e4000001e4000001e4
000001e4000001e4000001e4000001e4000001e4000001e4000001e40000
01e4000001e4000001e4000001e4000001e4000001e4000001e4000001e4
000001e4000001e4000001e4000001e4000001e4000001e4000001e40000
01e4000001e4000001e4000001e4000001e4000001e4000001e4000001e4
000001e4000001e4000001e4000001e4000001e4000001e4000001e40000
01e4000001e4000001e4000001e4000001e4000001e4000001e4000001e4
000001e4000001e4000001e4000001e40000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400000414000004140000041400000414000004140000041400000414
000004140000041400000414000004140000041400000414000004140000
041400010000068a0100003f0076000700020010002f00560000040d0aff
00030002b1540f4122031700ef031700ff03170003001f0317002f031700
4f0317005f0317008f0317009f03170006000f0317005f0317006f031700
7f031700bf031700f00317000600400317b2923340b80317b28b3340b803
17b36a6c3240b80317b2613340b80317b35c5d3240b80317b357593240b8
0317b34d513240b80317b344493240b80317b23a3340b80317b331343240
b80317b32e423240b80317b3272c3240b80317b312253280b80317b30a0d
32c04116031600d00316000200700316000102c4000f0101001f00a00315
00b0031500020306000f0101001f00400312b32426329fbf030400010302
03010064001fffc00301b20d1132410a02ff02ef0012001f02ee02ed0064
001fffc002edb30e11329f414a02e200af02e200bf02e2000302e202e202
e102e1007f02e00001001002e0003f02e0009f02e000bf02e000cf02e000
ef02e0000602e002e002df02df02de02de000f02dd002f02dd003f02dd00
5f02dd009f02dd00bf02dd00ef02dd000702dd02dd001002dc0001000002
dc0001001002dc003f02dc000202dc02dc001002db000102db02db000f02
da000102da02daffc002d3b2373932b9ffc002d3b22b2f32b9ffc002d3b2
1f2532b9ffc002d3b2171b32b9ffc002d3b2121632b802d2b2f9291fb802
e3b3202b1fa0413002d400b002d40002000002d4001002d4002002d40050
02d4006002d4007002d40006006002d6007002d6008002d6009002d600a0
02d600b002d60006000002d6001002d6002002ca002002cc002002d60030
02d6004002d6005002d6000802d0b2202b1fb802cfb226421f411602ce02
c70017001f02cd02c80017001f02cc02c60017001f02cb02c50017001f02
c902c5001e001f02ca02c6b21e1f00410b02c6000002c7001002c6001002
c7002f02c5000502c1b324121fff411102bf0001001f02bf002f02bf003f
02bf004f02bf005f02bf008f02bf000602bf0222b2641f12410b02bb00ca
0800001f02b200e90800001f02a600a20800406a1f402643493240204349
3240263a3d3240203a3d329f209f26024026969932402096993240268e92
3240208e92324026848c324020848c3240267a813240207a813240266c76
3240206c76324026646a324020646a3240265a5f3240205a5f3240264f54
3240204f5432b8029eb724271f374f6b0120410f02770030027700400277
00500277000402770277027700f90400001f029bb22a2a1fb8029a402b29
2a1f80ba0180bc0180520180a201806501807e01808101803c01805e0180
2b01801c01801e0180400180bb0138000100800140b40180400180bb0138
00010080013940180180ca0180ad01807301802601802501802401802001
3740b80221b2493340b80221b2453340b80221b341423240b80221b33d3e
320f410f0221003f0221007f0221000300bf022100cf022100ff02210003
00400221b320223240b80221b3191e3240b80222b32a3f3240b80221b32e
3a326f414802c3007f02c3008f02c300df02c30004002f02c3006002c300
cf02c30003000f02c3003f02c3005f02c300c002c300ef02c300ff02c300
0600df02220001008f02220001000f0222002f0222003f0222005f022200
7f022200ef0222000600bf022100ef02210002006f0221007f022100af02
210003002f0221003f0221004f0221000302c302c3022202220221022140
1d101c102b1048038f1c010f1e014f1eff1e023700161600000012110811
b8010db6f70df8f70d00094109028e028f001d001f0290028f001d001f02
8fb2f91d1fb80198b226bb1f41150197001e0401001f013900260125001f
013800730401001f0135001c0801001f0134001c02ab001f0132b21c561f
b8010fb2262c1fba010e001e0401b61ff91ce41fe91cb80201b61fe81cbb
1fd720b80401b21fd51cb802abb61fd41c891fc92fb80801b21fbc26b801
01b21fba20b80201b61fb91c381fadcab80401b21f8126b8019ab21f7e26
b8019ab61f7d1c471f6b1cb80401b21f6526b8019ab21f5e73b80401400f
1f52265a1f481c891f441c621f4073b80801b61f3f1c5e1f3c26b8019ab2
1f351cb80401b61f301cbb1f2b1cb80401b61f2a1c561f291cb80101b21f
231eb80401b21f5537b80168402c07960758074f07360732072c0721071f
071d071b071408120810080e080c080a080808060804080208000814b8ff
e0402b000001001406100000010006040000010004100000010010020000
01000200000001000002010802004a00b013034b024b5342014bb0c06300
4b6220b0f65323b8010a515ab005234201b0124b004b5442b0382b4bb807
ff52b0372b4bb007505b58b101018e59b0382bb00288b801005458b801ff
b101018e851bb0124358b900010111858d1bb900010128858d5959001816
763f183f123e113946443e113946443e113946443e113946443e11394660
443e11394660442b2b2b2b2b2b2b2b2b2b2b182b2b2b2b2b2b2b2b2b2b2b
182b1db0964b5358b0aa1d59b0324b5358b0ff1d594bb09353205c58b901
f201f04544b901f101f045445958b9033e01f2455258b901f2033e445959
4bb8015653205c58b9002001f14544b9002601f145445958b9081e002045
5258b90020081e4459594bb8019a53205c58b9002501f24544b9002401f2
45445958b909090025455258b9002509094459594bb8040153205c58b173
244544b1242445445958b917200073455258b9007317204459594bb80401
53205c58b1ca254544b1252545445958b9168000ca455258b900ca168044
59594bb03e53205c58b11c1c4544b11e1c45445958b9011a001c455258b9
001c011a4459594bb05653205c58b11c1c4544b12f1c45445958b9018900
1c455258b9001c01894459594bb8030153205c58b11c1c4544b11c1c4544
5958b90de0001c455258b9001c0de04459592b2b2b2b2b2b2b2b2b2b2b2b
2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b65
422b2b01b33b59635c456523456023456560234560b08b766818b0806220
20b163594565234520b003266062636820b003266165b059236544b06323
4420b13b5c4565234520b003266062636820b003266165b05c236544b03b
2344b1005c455458b15c406544b23b403b4523614459b347503437456523
456023456560234560b089766818b080622020b134504565234520b00326
6062636820b003266165b050236544b034234420b147374565234520b003
266062636820b003266165b037236544b0472344b10037455458b1374065
44b24740474523614459004b5342014b5058b108004259435c58b1080042
59b3020b0a124358601b2159421610703eb0124358b93b21187e1bba0400
01a8000b2b59b00c2342b00d2342b0124358b92d412d411bba0400040000
0b2b59b00e2342b00f2342b0124358b9187e3b211bba01a80400000b2b59
b0102342b0112342002b7475737500184569444569444569447373737374
757374752b2b2b2b74752b2b2b2b2b737373737373737373737373737373
737373737373737373732b2b2b45b0406144737400004bb02a534bb03f51
5a58b1070745b040604459004bb03a534bb03f515a58b10b0b45b8ffc060
4459004bb02e534bb03a515a58b1030345b040604459004bb02e534bb03c
515a58b1090945b8ffc06044592b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b
2b752b2b2b2b2b2b2b435c58b9008002bbb301401e017400735903b01e4b
5402b0124b545ab012435c5a58ba009f02220001007359002b7473012b01
732b2b2b2b2b2b2b2b737373732b002b2b2b2b2b2b004569447345694473
456944737475456944734569444569444569447374456944456944732b2b
2b2b2b732b002b732b74752b2b2b2b2b2b2b2b2b2b2b2b2b2b7374752b00
00>
[1045 ] AllocGlyphStorage
]def 
108 44 
PrepFor2015
Type42DictEnd
1 0 0 <00020100000005000500000300070000211121112521112101000400fc20
03c0fc400500fb002004c000>/JVAQLV+ArialMT AddT42Char 

1 0 213 <> /JVAQLV+ArialMT AddT42Char 

1 0 223 <> /JVAQLV+ArialMT AddT42Char 

1 0 3 <> /JVAQLV+ArialMT AddT42Char 

1 0 4 <> /JVAQLV+ArialMT AddT42Char 

1 0 5 <> /JVAQLV+ArialMT AddT42Char 

1 0 6 <> /JVAQLV+ArialMT AddT42Char 

1 0 7 <> /JVAQLV+ArialMT AddT42Char 

1 0 8 <> /JVAQLV+ArialMT AddT42Char 

1 0 9 <> /JVAQLV+ArialMT AddT42Char 

1 0 10 <> /JVAQLV+ArialMT AddT42Char 

1 0 11 <> /JVAQLV+ArialMT AddT42Char 

1 0 12 <> /JVAQLV+ArialMT AddT42Char 

1 0 13 <> /JVAQLV+ArialMT AddT42Char 

1 0 14 <> /JVAQLV+ArialMT AddT42Char 

1 0 15 <> /JVAQLV+ArialMT AddT42Char 

1 0 16 <> /JVAQLV+ArialMT AddT42Char 

1 0 17 <> /JVAQLV+ArialMT AddT42Char 

1 0 18 <> /JVAQLV+ArialMT AddT42Char 

1 0 19 <> /JVAQLV+ArialMT AddT42Char 

1 0 20 <> /JVAQLV+ArialMT AddT42Char 

1 0 21 <> /JVAQLV+ArialMT AddT42Char 

1 0 22 <> /JVAQLV+ArialMT AddT42Char 

1 0 23 <> /JVAQLV+ArialMT AddT42Char 
1 42 24 <00010055ffe7042105a6001e0156b10202435458b90001ffc0400d0d0d02
55011c0e0a1e15151c12b802bb400b0f04041e1c0d0e01000718b8ffeab4
0f0f025518b8ffeab40d0d0255182f2b2bcd2fcd2f003fed3fed12392ffd
c410c42b31301b4029120c0d0d06550f0c0d0d06554b1a791d8a1d9613a7
13c30cd60cdb1b080913180e2a1a03093005300bbaffe00003ffe0401013
0a15121313ca0e0f140e13140e0f0db802a440130e0a1e15400ea00e020e
0e0f40150115151c12b802bbb70f0401d340000100b801184020041e1c0d
115f106f107f108f1004108007731840212334301801001810180218b8ff
f4b70d0d065518902012bc0135000f0195000d0138b20eb501ba01380000
ffc0400b212334200040000200901fb80192b18b182b10f65d2bedf4edf4
ed10f62b5d712bedf45d3c003fedfd5de43fed12392f5d11392f5d10ed10
e487082e2b057d10c4001112393130013838383801715d2b2b5913371616
33323635342623220607271321152103363332001514070623222655bd15
996c82b4ad8c578c28a98e02d9fdb74f8491c00108748df4c8fd0180108a
8bc4a29ab24f3f1602f1acfe765cfef6d1c791b2e000>/JVAQLV+ArialMT AddT42Char 

1 0 25 <> /JVAQLV+ArialMT AddT42Char 

1 0 26 <> /JVAQLV+ArialMT AddT42Char 

1 0 27 <> /JVAQLV+ArialMT AddT42Char 

1 0 28 <> /JVAQLV+ArialMT AddT42Char 

1 0 29 <> /JVAQLV+ArialMT AddT42Char 

1 0 30 <> /JVAQLV+ArialMT AddT42Char 

1 0 31 <> /JVAQLV+ArialMT AddT42Char 

1 0 32 <> /JVAQLV+ArialMT AddT42Char 

1 0 33 <> /JVAQLV+ArialMT AddT42Char 

1 0 34 <> /JVAQLV+ArialMT AddT42Char 

1 0 35 <> /JVAQLV+ArialMT AddT42Char 

1 0 36 <> /JVAQLV+ArialMT AddT42Char 

1 0 37 <> /JVAQLV+ArialMT AddT42Char 

1 0 38 <> /JVAQLV+ArialMT AddT42Char 

1 0 39 <> /JVAQLV+ArialMT AddT42Char 

1 0 40 <> /JVAQLV+ArialMT AddT42Char 

1 0 41 <> /JVAQLV+ArialMT AddT42Char 

1 0 42 <> /JVAQLV+ArialMT AddT42Char 

1 0 43 <> /JVAQLV+ArialMT AddT42Char 

1 0 44 <> /JVAQLV+ArialMT AddT42Char 

1 0 45 <> /JVAQLV+ArialMT AddT42Char 

1 0 46 <> /JVAQLV+ArialMT AddT42Char 

1 0 47 <> /JVAQLV+ArialMT AddT42Char 

1 0 48 <> /JVAQLV+ArialMT AddT42Char 

1 0 49 <> /JVAQLV+ArialMT AddT42Char 

1 0 50 <> /JVAQLV+ArialMT AddT42Char 

1 0 51 <> /JVAQLV+ArialMT AddT42Char 

1 0 52 <> /JVAQLV+ArialMT AddT42Char 

1 0 53 <> /JVAQLV+ArialMT AddT42Char 

1 0 54 <> /JVAQLV+ArialMT AddT42Char 

1 0 55 <> /JVAQLV+ArialMT AddT42Char 

1 0 56 <> /JVAQLV+ArialMT AddT42Char 

1 0 57 <> /JVAQLV+ArialMT AddT42Char 

1 0 58 <> /JVAQLV+ArialMT AddT42Char 

1 0 59 <> /JVAQLV+ArialMT AddT42Char 

1 0 60 <> /JVAQLV+ArialMT AddT42Char 

1 0 61 <> /JVAQLV+ArialMT AddT42Char 

1 0 62 <> /JVAQLV+ArialMT AddT42Char 

1 0 63 <> /JVAQLV+ArialMT AddT42Char 

1 0 64 <> /JVAQLV+ArialMT AddT42Char 

1 0 65 <> /JVAQLV+ArialMT AddT42Char 

1 0 66 <> /JVAQLV+ArialMT AddT42Char 

1 0 67 <> /JVAQLV+ArialMT AddT42Char 

1 0 68 <> /JVAQLV+ArialMT AddT42Char 

1 0 69 <> /JVAQLV+ArialMT AddT42Char 

1 0 70 <> /JVAQLV+ArialMT AddT42Char 

1 0 71 <> /JVAQLV+ArialMT AddT42Char 

1 0 72 <> /JVAQLV+ArialMT AddT42Char 

1 0 73 <> /JVAQLV+ArialMT AddT42Char 

1 0 74 <> /JVAQLV+ArialMT AddT42Char 

1 0 75 <> /JVAQLV+ArialMT AddT42Char 

1 0 76 <> /JVAQLV+ArialMT AddT42Char 

1 0 77 <> /JVAQLV+ArialMT AddT42Char 

1 0 78 <> /JVAQLV+ArialMT AddT42Char 

1 0 79 <> /JVAQLV+ArialMT AddT42Char 
1 484 80 <0001008700000626043e002301c7b9000dfff4b40d0d065508b8fff4b40d
0d065509b8ffd8404d0b0d342504e404e409e117e52005d505f620021708
202309181b20090303231e1c06151c0b0b06070106231a19100ad0250190
25a025022517171a0e2590110111041010025511180f0f025511b8ffec40
0b0e0e025511140c0c025511b8ffe840170b0b025511020b0b0655110c10
10065511060f0f065511b8fffab40c0c065511b8fff8b40d0d065511b801
5d400c1825901b011b180f0f02551bb8ffec400b0e0e02551b140c0c0255
1bb8ffee40110b0b02551b040b0b06551b0a101006551bb8fffe400b0d0d
06551b0c0f0f06551bb8fffcb40c0c06551bb8015d4016000233232501d0
00019000a000021f003f004f000300b8fffe401d0e0e025500100d0d0255
00100c0c0255000c0b0b025500160b0b065500b8fffcb41010065500b8ff
f440140f0f0655000a0c0c0655000e0d0d065500192425b80178b3214750
182b2b4ef42b2b2b2b2b2b2b2b2b5d71723c4dfde410f42b2b2b2b2b2b2b
2b2b5dedf42b2b2b2b2b2b2b2b2b2b5dfd4e456544e67172003f3c3c3c3f
3f3c4d10ed10ed11173901111239123931304379400e0c141326140c111b
01120d151b01002b012b2b81015d005d2b2b2b3311331536363332161736
3332161511231134262623220615112311342623220606151187a132a66a
76971f7eca9eaab3235c3e7094b458644c813a0426954e5f6258baafb6fd
27029d6c5f3a95a4fd9702b27878509a91fdd900>/JVAQLV+ArialMT AddT42Char 

1 0 81 <> /JVAQLV+ArialMT AddT42Char 

1 0 82 <> /JVAQLV+ArialMT AddT42Char 

1 0 83 <> /JVAQLV+ArialMT AddT42Char 

1 0 84 <> /JVAQLV+ArialMT AddT42Char 

1 0 85 <> /JVAQLV+ArialMT AddT42Char 

1 0 86 <> /JVAQLV+ArialMT AddT42Char 

1 0 87 <> /JVAQLV+ArialMT AddT42Char 

1 0 88 <> /JVAQLV+ArialMT AddT42Char 

1 0 89 <> /JVAQLV+ArialMT AddT42Char 

1 0 90 <> /JVAQLV+ArialMT AddT42Char 

1 0 91 <> /JVAQLV+ArialMT AddT42Char 

1 0 92 <> /JVAQLV+ArialMT AddT42Char 

1 0 93 <> /JVAQLV+ArialMT AddT42Char 

1 0 94 <> /JVAQLV+ArialMT AddT42Char 

1 0 95 <> /JVAQLV+ArialMT AddT42Char 

1 0 96 <> /JVAQLV+ArialMT AddT42Char 

1 0 97 <> /JVAQLV+ArialMT AddT42Char 

1 0 135 <> /JVAQLV+ArialMT AddT42Char 

1 0 188 <> /JVAQLV+ArialMT AddT42Char 

1 0 195 <> /JVAQLV+ArialMT AddT42Char 

1 0 166 <> /JVAQLV+ArialMT AddT42Char 

1 0 196 <> /JVAQLV+ArialMT AddT42Char 

1 0 171 <> /JVAQLV+ArialMT AddT42Char 

1 0 130 <> /JVAQLV+ArialMT AddT42Char 

1 0 193 <> /JVAQLV+ArialMT AddT42Char 

1 0 214 <> /JVAQLV+ArialMT AddT42Char 

1 0 197 <> /JVAQLV+ArialMT AddT42Char 

1 0 226 <> /JVAQLV+ArialMT AddT42Char 

1 0 189 <> /JVAQLV+ArialMT AddT42Char 

1 0 175 <> /JVAQLV+ArialMT AddT42Char 

1 0 228 <> /JVAQLV+ArialMT AddT42Char 

1 0 181 <> /JVAQLV+ArialMT AddT42Char 

1 0 182 <> /JVAQLV+ArialMT AddT42Char 

1 0 179 <> /JVAQLV+ArialMT AddT42Char 

1 0 180 <> /JVAQLV+ArialMT AddT42Char 

1 0 177 <> /JVAQLV+ArialMT AddT42Char 

1 0 178 <> /JVAQLV+ArialMT AddT42Char 

1 0 215 <> /JVAQLV+ArialMT AddT42Char 

1 0 140 <> /JVAQLV+ArialMT AddT42Char 

1 0 227 <> /JVAQLV+ArialMT AddT42Char 

1 0 190 <> /JVAQLV+ArialMT AddT42Char 

1 0 176 <> /JVAQLV+ArialMT AddT42Char 

1 0 229 <> /JVAQLV+ArialMT AddT42Char 

1 0 186 <> /JVAQLV+ArialMT AddT42Char 

1 0 163 <> /JVAQLV+ArialMT AddT42Char 

1 0 132 <> /JVAQLV+ArialMT AddT42Char 

1 0 133 <> /JVAQLV+ArialMT AddT42Char 

1 0 862 <> /JVAQLV+ArialMT AddT42Char 

1 0 150 <> /JVAQLV+ArialMT AddT42Char 

1 0 230 <> /JVAQLV+ArialMT AddT42Char 

1 0 134 <> /JVAQLV+ArialMT AddT42Char 

1 0 142 <> /JVAQLV+ArialMT AddT42Char 

1 0 139 <> /JVAQLV+ArialMT AddT42Char 

1 0 157 <> /JVAQLV+ArialMT AddT42Char 

1 0 169 <> /JVAQLV+ArialMT AddT42Char 

1 0 164 <> /JVAQLV+ArialMT AddT42Char 

1 0 138 <> /JVAQLV+ArialMT AddT42Char 

1 0 256 <> /JVAQLV+ArialMT AddT42Char 

1 0 131 <> /JVAQLV+ArialMT AddT42Char 

1 0 147 <> /JVAQLV+ArialMT AddT42Char 

1 0 240 <> /JVAQLV+ArialMT AddT42Char 

1 0 241 <> /JVAQLV+ArialMT AddT42Char 

1 0 141 <> /JVAQLV+ArialMT AddT42Char 

1 0 151 <> /JVAQLV+ArialMT AddT42Char 

1 0 136 <> /JVAQLV+ArialMT AddT42Char 

1 0 194 <> /JVAQLV+ArialMT AddT42Char 

1 0 220 <> /JVAQLV+ArialMT AddT42Char 

1 0 239 <> /JVAQLV+ArialMT AddT42Char 

1 0 158 <> /JVAQLV+ArialMT AddT42Char 

1 0 170 <> /JVAQLV+ArialMT AddT42Char 

1 0 243 <> /JVAQLV+ArialMT AddT42Char 

1 0 242 <> /JVAQLV+ArialMT AddT42Char 

1 0 244 <> /JVAQLV+ArialMT AddT42Char 

1 0 162 <> /JVAQLV+ArialMT AddT42Char 

1 0 172 <> /JVAQLV+ArialMT AddT42Char 

1 0 200 <> /JVAQLV+ArialMT AddT42Char 

1 0 198 <> /JVAQLV+ArialMT AddT42Char 

1 0 173 <> /JVAQLV+ArialMT AddT42Char 

1 0 98 <> /JVAQLV+ArialMT AddT42Char 

1 0 99 <> /JVAQLV+ArialMT AddT42Char 

1 0 144 <> /JVAQLV+ArialMT AddT42Char 

1 0 100 <> /JVAQLV+ArialMT AddT42Char 

1 0 202 <> /JVAQLV+ArialMT AddT42Char 

1 0 101 <> /JVAQLV+ArialMT AddT42Char 

1 0 199 <> /JVAQLV+ArialMT AddT42Char 

1 0 201 <> /JVAQLV+ArialMT AddT42Char 

1 0 206 <> /JVAQLV+ArialMT AddT42Char 

1 0 203 <> /JVAQLV+ArialMT AddT42Char 

1 0 204 <> /JVAQLV+ArialMT AddT42Char 

1 0 205 <> /JVAQLV+ArialMT AddT42Char 

1 0 231 <> /JVAQLV+ArialMT AddT42Char 

1 0 102 <> /JVAQLV+ArialMT AddT42Char 

1 0 209 <> /JVAQLV+ArialMT AddT42Char 

1 0 207 <> /JVAQLV+ArialMT AddT42Char 

1 0 208 <> /JVAQLV+ArialMT AddT42Char 

1 0 174 <> /JVAQLV+ArialMT AddT42Char 

1 0 103 <> /JVAQLV+ArialMT AddT42Char 

1 0 238 <> /JVAQLV+ArialMT AddT42Char 

1 0 145 <> /JVAQLV+ArialMT AddT42Char 

1 0 212 <> /JVAQLV+ArialMT AddT42Char 

1 0 210 <> /JVAQLV+ArialMT AddT42Char 

1 0 211 <> /JVAQLV+ArialMT AddT42Char 

1 0 104 <> /JVAQLV+ArialMT AddT42Char 

1 0 233 <> /JVAQLV+ArialMT AddT42Char 

1 0 235 <> /JVAQLV+ArialMT AddT42Char 

1 0 137 <> /JVAQLV+ArialMT AddT42Char 

1 0 106 <> /JVAQLV+ArialMT AddT42Char 

1 0 105 <> /JVAQLV+ArialMT AddT42Char 

1 0 107 <> /JVAQLV+ArialMT AddT42Char 

1 0 109 <> /JVAQLV+ArialMT AddT42Char 

1 0 108 <> /JVAQLV+ArialMT AddT42Char 

1 0 110 <> /JVAQLV+ArialMT AddT42Char 

1 0 160 <> /JVAQLV+ArialMT AddT42Char 

1 0 111 <> /JVAQLV+ArialMT AddT42Char 

1 0 113 <> /JVAQLV+ArialMT AddT42Char 

1 0 112 <> /JVAQLV+ArialMT AddT42Char 

1 0 114 <> /JVAQLV+ArialMT AddT42Char 

1 0 115 <> /JVAQLV+ArialMT AddT42Char 

1 0 117 <> /JVAQLV+ArialMT AddT42Char 

1 0 116 <> /JVAQLV+ArialMT AddT42Char 

1 0 118 <> /JVAQLV+ArialMT AddT42Char 

1 0 119 <> /JVAQLV+ArialMT AddT42Char 

1 0 232 <> /JVAQLV+ArialMT AddT42Char 

1 0 120 <> /JVAQLV+ArialMT AddT42Char 

1 0 122 <> /JVAQLV+ArialMT AddT42Char 

1 0 121 <> /JVAQLV+ArialMT AddT42Char 

1 0 123 <> /JVAQLV+ArialMT AddT42Char 

1 0 125 <> /JVAQLV+ArialMT AddT42Char 

1 0 124 <> /JVAQLV+ArialMT AddT42Char 

1 0 183 <> /JVAQLV+ArialMT AddT42Char 

1 0 161 <> /JVAQLV+ArialMT AddT42Char 

1 0 127 <> /JVAQLV+ArialMT AddT42Char 

1 0 126 <> /JVAQLV+ArialMT AddT42Char 

1 0 128 <> /JVAQLV+ArialMT AddT42Char 

1 0 129 <> /JVAQLV+ArialMT AddT42Char 

1 0 234 <> /JVAQLV+ArialMT AddT42Char 

1 0 236 <> /JVAQLV+ArialMT AddT42Char 

1 0 185 <> /JVAQLV+ArialMT AddT42Char 
/JVAQLV+ArialMT findfont /CharStrings get begin
/.notdef 0 def
/dotlessi 213 def
/caron 223 def
/space 3 def
/exclam 4 def
/quotedbl 5 def
/numbersign 6 def
/dollar 7 def
/percent 8 def
/ampersand 9 def
/quotesingle 10 def
/parenleft 11 def
/parenright 12 def
/asterisk 13 def
/plus 14 def
/comma 15 def
/hyphen 16 def
/period 17 def
/slash 18 def
/zero 19 def
/one 20 def
/two 21 def
/three 22 def
/four 23 def
/five 24 def
/six 25 def
/seven 26 def
/eight 27 def
/nine 28 def
/colon 29 def
/semicolon 30 def
/less 31 def
/equal 32 def
/greater 33 def
/question 34 def
/at 35 def
/A 36 def
/B 37 def
/C 38 def
/D 39 def
/E 40 def
/F 41 def
/G 42 def
/H 43 def
/I 44 def
/J 45 def
/K 46 def
/L 47 def
/M 48 def
/N 49 def
/O 50 def
/P 51 def
/Q 52 def
/R 53 def
/S 54 def
/T 55 def
/U 56 def
/V 57 def
/W 58 def
/X 59 def
/Y 60 def
/Z 61 def
/bracketleft 62 def
/backslash 63 def
/bracketright 64 def
/asciicircum 65 def
/underscore 66 def
/grave 67 def
/a 68 def
/b 69 def
/c 70 def
/d 71 def
/e 72 def
/f 73 def
/g 74 def
/h 75 def
/i 76 def
/j 77 def
/k 78 def
/l 79 def
/m 80 def
/n 81 def
/o 82 def
/p 83 def
/q 84 def
/r 85 def
/s 86 def
/t 87 def
/u 88 def
/v 89 def
/w 90 def
/x 91 def
/y 92 def
/z 93 def
/braceleft 94 def
/bar 95 def
/braceright 96 def
/asciitilde 97 def
/bullet 135 def
/Euro 188 def
/quotesinglbase 195 def
/florin 166 def
/quotedblbase 196 def
/ellipsis 171 def
/dagger 130 def
/daggerdbl 193 def
/circumflex 214 def
/perthousand 197 def
/Scaron 226 def
/guilsinglleft 189 def
/OE 175 def
/Zcaron 228 def
/quoteleft 181 def
/quoteright 182 def
/quotedblleft 179 def
/quotedblright 180 def
/endash 177 def
/emdash 178 def
/tilde 215 def
/trademark 140 def
/scaron 227 def
/guilsinglright 190 def
/oe 176 def
/zcaron 229 def
/Ydieresis 186 def
/exclamdown 163 def
/cent 132 def
/sterling 133 def
/currency 862 def
/yen 150 def
/brokenbar 230 def
/section 134 def
/dieresis 142 def
/copyright 139 def
/ordfeminine 157 def
/guillemotleft 169 def
/logicalnot 164 def
/registered 138 def
/macron 256 def
/degree 131 def
/plusminus 147 def
/twosuperior 240 def
/threesuperior 241 def
/acute 141 def
/mu 151 def
/paragraph 136 def
/periodcentered 194 def
/cedilla 220 def
/onesuperior 239 def
/ordmasculine 158 def
/guillemotright 170 def
/onequarter 243 def
/onehalf 242 def
/threequarters 244 def
/questiondown 162 def
/Agrave 172 def
/Aacute 200 def
/Acircumflex 198 def
/Atilde 173 def
/Adieresis 98 def
/Aring 99 def
/AE 144 def
/Ccedilla 100 def
/Egrave 202 def
/Eacute 101 def
/Ecircumflex 199 def
/Edieresis 201 def
/Igrave 206 def
/Iacute 203 def
/Icircumflex 204 def
/Idieresis 205 def
/Eth 231 def
/Ntilde 102 def
/Ograve 209 def
/Oacute 207 def
/Ocircumflex 208 def
/Otilde 174 def
/Odieresis 103 def
/multiply 238 def
/Oslash 145 def
/Ugrave 212 def
/Uacute 210 def
/Ucircumflex 211 def
/Udieresis 104 def
/Yacute 233 def
/Thorn 235 def
/germandbls 137 def
/agrave 106 def
/aacute 105 def
/acircumflex 107 def
/atilde 109 def
/adieresis 108 def
/aring 110 def
/ae 160 def
/ccedilla 111 def
/egrave 113 def
/eacute 112 def
/ecircumflex 114 def
/edieresis 115 def
/igrave 117 def
/iacute 116 def
/icircumflex 118 def
/idieresis 119 def
/eth 232 def
/ntilde 120 def
/ograve 122 def
/oacute 121 def
/ocircumflex 123 def
/otilde 125 def
/odieresis 124 def
/divide 183 def
/oslash 161 def
/ugrave 127 def
/uacute 126 def
/ucircumflex 128 def
/udieresis 129 def
/yacute 234 def
/thorn 236 def
/ydieresis 185 def
end
/JVAQLV+ArialMT findfont /Encoding get
dup 0 /.notdef put
dup 1 /dotlessi put
dup 2 /caron put
dup 32 /space put
dup 33 /exclam put
dup 34 /quotedbl put
dup 35 /numbersign put
dup 36 /dollar put
dup 37 /percent put
dup 38 /ampersand put
dup 39 /quotesingle put
dup 40 /parenleft put
dup 41 /parenright put
dup 42 /asterisk put
dup 43 /plus put
dup 44 /comma put
dup 45 /hyphen put
dup 46 /period put
dup 47 /slash put
dup 48 /zero put
dup 49 /one put
dup 50 /two put
dup 51 /three put
dup 52 /four put
dup 53 /five put
dup 54 /six put
dup 55 /seven put
dup 56 /eight put
dup 57 /nine put
dup 58 /colon put
dup 59 /semicolon put
dup 60 /less put
dup 61 /equal put
dup 62 /greater put
dup 63 /question put
dup 64 /at put
dup 65 /A put
dup 66 /B put
dup 67 /C put
dup 68 /D put
dup 69 /E put
dup 70 /F put
dup 71 /G put
dup 72 /H put
dup 73 /I put
dup 74 /J put
dup 75 /K put
dup 76 /L put
dup 77 /M put
dup 78 /N put
dup 79 /O put
dup 80 /P put
dup 81 /Q put
dup 82 /R put
dup 83 /S put
dup 84 /T put
dup 85 /U put
dup 86 /V put
dup 87 /W put
dup 88 /X put
dup 89 /Y put
dup 90 /Z put
dup 91 /bracketleft put
dup 92 /backslash put
dup 93 /bracketright put
dup 94 /asciicircum put
dup 95 /underscore put
dup 96 /grave put
dup 97 /a put
dup 98 /b put
dup 99 /c put
dup 100 /d put
dup 101 /e put
dup 102 /f put
dup 103 /g put
dup 104 /h put
dup 105 /i put
dup 106 /j put
dup 107 /k put
dup 108 /l put
dup 109 /m put
dup 110 /n put
dup 111 /o put
dup 112 /p put
dup 113 /q put
dup 114 /r put
dup 115 /s put
dup 116 /t put
dup 117 /u put
dup 118 /v put
dup 119 /w put
dup 120 /x put
dup 121 /y put
dup 122 /z put
dup 123 /braceleft put
dup 124 /bar put
dup 125 /braceright put
dup 126 /asciitilde put
dup 127 /bullet put
dup 128 /Euro put
dup 129 /bullet put
dup 130 /quotesinglbase put
dup 131 /florin put
dup 132 /quotedblbase put
dup 133 /ellipsis put
dup 134 /dagger put
dup 135 /daggerdbl put
dup 136 /circumflex put
dup 137 /perthousand put
dup 138 /Scaron put
dup 139 /guilsinglleft put
dup 140 /OE put
dup 141 /bullet put
dup 142 /Zcaron put
dup 143 /bullet put
dup 144 /bullet put
dup 145 /quoteleft put
dup 146 /quoteright put
dup 147 /quotedblleft put
dup 148 /quotedblright put
dup 149 /bullet put
dup 150 /endash put
dup 151 /emdash put
dup 152 /tilde put
dup 153 /trademark put
dup 154 /scaron put
dup 155 /guilsinglright put
dup 156 /oe put
dup 157 /bullet put
dup 158 /zcaron put
dup 159 /Ydieresis put
dup 160 /space put
dup 161 /exclamdown put
dup 162 /cent put
dup 163 /sterling put
dup 164 /currency put
dup 165 /yen put
dup 166 /brokenbar put
dup 167 /section put
dup 168 /dieresis put
dup 169 /copyright put
dup 170 /ordfeminine put
dup 171 /guillemotleft put
dup 172 /logicalnot put
dup 173 /hyphen put
dup 174 /registered put
dup 175 /macron put
dup 176 /degree put
dup 177 /plusminus put
dup 178 /twosuperior put
dup 179 /threesuperior put
dup 180 /acute put
dup 181 /mu put
dup 182 /paragraph put
dup 183 /periodcentered put
dup 184 /cedilla put
dup 185 /onesuperior put
dup 186 /ordmasculine put
dup 187 /guillemotright put
dup 188 /onequarter put
dup 189 /onehalf put
dup 190 /threequarters put
dup 191 /questiondown put
dup 192 /Agrave put
dup 193 /Aacute put
dup 194 /Acircumflex put
dup 195 /Atilde put
dup 196 /Adieresis put
dup 197 /Aring put
dup 198 /AE put
dup 199 /Ccedilla put
dup 200 /Egrave put
dup 201 /Eacute put
dup 202 /Ecircumflex put
dup 203 /Edieresis put
dup 204 /Igrave put
dup 205 /Iacute put
dup 206 /Icircumflex put
dup 207 /Idieresis put
dup 208 /Eth put
dup 209 /Ntilde put
dup 210 /Ograve put
dup 211 /Oacute put
dup 212 /Ocircumflex put
dup 213 /Otilde put
dup 214 /Odieresis put
dup 215 /multiply put
dup 216 /Oslash put
dup 217 /Ugrave put
dup 218 /Uacute put
dup 219 /Ucircumflex put
dup 220 /Udieresis put
dup 221 /Yacute put
dup 222 /Thorn put
dup 223 /germandbls put
dup 224 /agrave put
dup 225 /aacute put
dup 226 /acircumflex put
dup 227 /atilde put
dup 228 /adieresis put
dup 229 /aring put
dup 230 /ae put
dup 231 /ccedilla put
dup 232 /egrave put
dup 233 /eacute put
dup 234 /ecircumflex put
dup 235 /edieresis put
dup 236 /igrave put
dup 237 /iacute put
dup 238 /icircumflex put
dup 239 /idieresis put
dup 240 /eth put
dup 241 /ntilde put
dup 242 /ograve put
dup 243 /oacute put
dup 244 /ocircumflex put
dup 245 /otilde put
dup 246 /odieresis put
dup 247 /divide put
dup 248 /oslash put
dup 249 /ugrave put
dup 250 /uacute put
dup 251 /ucircumflex put
dup 252 /udieresis put
dup 253 /yacute put
dup 254 /thorn put
dup 255 /ydieresis put
pop
end

userdict /pdf_svglb get setglobal
[/N157/JVAQLV+ArialMT 1 TZG
userdict /pdf_svglb currentglobal put true setglobal
ct_T42Dict begin
-0.625 -0.375 2 1.008
 256 array 0 1 255 {1 index exch /.notdef put} for  /ZYCIBP+Arial-BoldMT
Type42DictBegin
[<00010000000a000a000a000a63767420ef1f94cc000000ac0000073a6670
676d08e8ba28000007e8000005d7676c796674b520dd0000530000002c02
68656164cfee209b00000dc00000003668686561127e12ff00000df80000
0024686d7478a006329b00000e1c00001a286c6f63610116068e00002844
00001a2c6d6178700d831203000042700000002070726570412164030000
42900000106f6764697200000000000000000000000005ba001c05ba001c
05a7001c0426001c0000ffe40000ffe40000ffe4fe69ffe405ba001cfe69
ffe402ea0000011d0000011d000000000000000000b200ac00d701280120
00b301fa001700f8011901310049000400f7000300af00fd009500140054
00960112002400160055004901040119012b008c019bff76ffe9003d0092
00a2ffb70182ffaa0016008f00c600f8001c00de04010037004e00550055
006500e903e50059ff9a00080087000b003b00520116006100d600d600f5
00000093009400be017cfff80004001400820092003c00410041ffc1fffc
002a008c049005d809b5009100bb0106ff63ff69001e0022008a022bffd6
ffdf0026005900a300ac0104012b01c004480021006b00850098011903c6
006b009500a400fe010c025d034305bf000000490056006e0077008a00aa
00ca0112015005d805f0ff7bffe70006001300280061006900e90135014d
02a5040cff3effda005b00b900c801190119011901c0045b04a7055bfe3f
ff9dffc2001500b7010a01bc01c10532058efd81ffa1ffae000c00260031
003d004e00560062008300c100c900f100f2027fff7f00480053007700c5
011d01200126012801d60219027e027e03d3002e0041005d006b0075009f
00b000b200ba00bb00bd00d600db00e000e50114011b014a0162019101f2
020c026402cf039b03b403d4040104a9001600230025002a007400a500b6
00cc00cd00cf0105012001300150016a016f0197019d01e002b002ec02f7
0408048304fb04fd0526fee0fefbff4efff50018001a004c007a007f0091
00a300b300b400ce00d500f200f300f601100138016801a101b001e001ec
02090222024f0270029602a502ad034e039103c104350442046b04cd04da
0586058b076107fefca6fe93feadfed1ffb7ffd10003000e001800260046
00690081008f00a500bf00d300d500d900dd00e20119012b0138013b015a
015e016801730188019401ad01c501d101ea01f20200020002000222023b
0244024f026f0272027e02820293029402a502cf02cf02d002da02dd02eb
02f5030503220336037103a103b003b803d003e604100426042e0431044f
045a04ff053205320547055305a805ab05c205f0063c0664067006e80782
078408ccfd2afddefe00fe68feb0feb3ffaa00080059007a0091009e00a2
00af00b400bb00ca00cc00ce00d900e000f40114011a01210127012b0139
0146014b014d0157015c01650182018701920198019b01a201ae01c501c5
01d102070222022b024102530261026502840287028d02b402b402ba02c9
02d602d802ed02f503170323032b03310349035a035b036e03710374037e
03840391039103aa03cf03d303e703e803ed04080417041e0475047a0499
04a704b404d1054c056d056d05a205bf05c005d105fc05fc0602061a061c
062f066a06a806e2070607360750078907d407f30870011c012a011a0120
0000000000000000000000000219000b001e02aa0214047f01ed0000001d
0104000f0091002b01880153011201f3003f03fe0168010e047f01ed036e
03150219041300000000064004b00000027401bb003501c5007f06020301
000004e000b201dc02e004c3023d00d50160011904a7036e05ca022100ab
0426009002bc02bb014200b4023c0256029c030001e501a800e5006b0078
0094016b017300ab01ed013a017d0137017f00d4021603530184003cffa2
02040109014901f0006e031500810464005e000000000000000000000000
000000000000000000000000000000000000013900dc00e9fe9e040d047c
012b00b80096005900ac00df01a900fa0105ffec00170003005500610004
008c00a3008500280120005d00d6007f012601190104016c06cf00b40106
00000737063e047a00f000f900e905ba042604420000ffe7fe69049e04e3
ff37ff2d01200105012000a800740068004700f200e500d900bd00a80068
0047005c0048000a0028003200410050005a0064007d00870091ffb0ff9c
ff83ff79ff6f00cb012000fa012c01fa01a000d500b8005c003c00c800c8
008f00d9018b00b300470000000000000000000000000000000000000000
000000000000000000000000000000000000000000000000000000000000
00000000fe6400c000ea01180125013203b003ed0576059005aa05b405be
05cd063100780084009b00cc00e200f4010a0120016300d100ea00f70108
01420019002c00340041003800480058006c025903bd0043011a007000d3
0028003700420050005a0064007300780082008c009c00a500bd00ce00f0
0110015c00be00d801020117012c016300ea01080041004b0055005f0073
00a60109018301b300410064001e002a00eb00fa010e01380274002c0040
0082009600b600c000cc00dc00e600f000ff010a0120012c013b01440156
016300f70057006401100136005001b10000ffb60039004e004403cc00e5
002401100042012201a400f0006000e0000e001d003905e30102002cfe4e
ff38026903bd011600ff000e00a00054001b003d01710041000f005000fd
0015014f0035fe52002c00d30000404154403f3e3d3c3b3a393837353433
3231302f2e2d2c2b2a292827262524232221201f1e1d1c1b1a1918171615
14131211100f0e0d0c0b0a090807060504030201002c4523466020b02660
b004262348482d2c452346236120b02661b004262348482d2c45234660b0
206120b04660b004262348482d2c4523462361b0206020b02661b02061b0
04262348482d2c45234660b0406120b06660b004262348482d2c45234623
61b0406020b02661b04061b004262348482d2c0110203c003c2d2c204523
20b0cd442320b8015a51582320b08d44235920b0ed51582320b04d442359
20b09051582320b00d44235921212d2c20204518684420b001602045b046
76688a4560442d2c01b10b0a432343650a2d2c00b10a0b4323430b2d2c00
b0172370b101173e01b0172370b10217453ab10200080d2d2c45b01a2344
45b01923442d2c2045b00325456164b050515845441b2121592d2cb00143
632362b0002342b00f2b2d2c2045b0004360442d2c01b00643b00743650a
2d2c2069b04061b0008b20b12cc08a8cb8100062602b0c642364615c58b0
0361592d2c45b0112bb0172344b0177ae4182d2c45b0112bb01723442d2c
b01243588745b0112bb0172344b0177ae41b038a45186920b01723448a8a
8720b0c05158b0112bb0172344b0177ae41b21b0177ae45959182d2c2d2c
b0022546608a46b040618c482d2c4b53205c58b002855958b00185592d2c
20b0032545b019234445b01a23444565234520b00325606a20b009234223
688a6a606120b01a8ab000527921b21a1a40b9ffe0001a45208a54582321
b03f1b235961441cb114008a5279b31940201945208a54582321b03f1b23
5961442d2cb110114323430b2d2cb10e0f4323430b2d2cb10c0d4323430b
2d2cb10c0d432343650b2d2cb10e0f432343650b2d2cb11011432343650b
2d2c4b525845441b2121592d2c0120b003252349b04060b0206320b00052
5823b002253823b002256538008a63381b212121212159012d2c4bb06451
584569b00943608a103a1b212121592d2c01b005251023208af500b00160
23edec2d2c01b005251023208af500b0016123edec2d2c01b0062510f500
edec2d2c20b001600110203c003c2d2c20b001610110203c003c2d2cb02b
2bb02a2a2d2c00b00743b006430b2d2c3eb02a2a2d2c352d2c76b8023623
701020b802364520b0005058b00161593a2f182d2c21210c6423648bb840
00622d2c21b08051580c6423648bb82000621bb200402f2b59b002602d2c
21b0c051580c6423648bb81555621bb200802f2b59b002602d2c0c642364
8bb84000626023212d2cb4000100000015b00826b00826b00826b008260f
10161345683ab001162d2cb4000100000015b00826b00826b00826b00826
0f1016134568653ab001162d2c4b53234b515a5820458a60441b2121592d
2c4b545820458a60441b2121592d2c4b53234b515a58381b2121592d2c4b
5458381b2121592d2cb0134358031b02592d2cb0134358021b03592d2c4b
54b012435c5a58381b2121592d2cb012435c580cb00425b00425060c6423
646164b0035158b00425b00425012046b01060482046b0106048590a2121
1b2121592d2cb012435c580cb00425b00425060c6423646164b807085158
b00425b00425012046b8fff060482046b8fff06048590a21211b2121592d
2c4b53234b515a58b03a2b1b2121592d2c4b53234b515a58b03b2b1b2121
592d2c4b53234b515ab012435c5a58381b2121592d2c0c8a034b54b00426
024b545a8a8a0ab012435c5a58381b2121592d2c462346608a8a46232046
8a608a61b8ff8062232010238ab902a702a78a70456020b0005058b00161
b8ffba8b1bb0468c59b0106068013a2d2cb1020042b123018851b1400188
535a58b910000020885458b202010243604259b12401885158b920000040
885458b202020243604259b12401885458b2022002436042004b014b5258
b2020802436042591bb940000080885458b202040243604259b940000080
63b80100885458b202080243604259b94000010063b80200885458b20210
02436042595959592d00000100000002e667024961af5f0f3cf508190800
00000000a2e33c1d00000000b9d5b513fafafcfd10000815000100090001
00010000000000010000073efe4e00431000fafafe261000000100000000
00000000000000000000068a0600010000000000023900000239000002aa
00b803cb00700473001204730046071d005905c7005a01e7005c02aa006b
02aa0043031d001c04ac00550239007502aa0073023900930239fffd0473
0056047300a2047300330473004d047300260473005b0473005704730057
047300530473004102aa00c902aa00aa04ac005f04ac005504ac005f04e3
006a07cd003d05c7000005c7009605c7006105c700940556009504e30097
0639006205c700960239008c0473002305c7009904e3009d06aa009105c7
009806390059055600950639005905c700960556004a04e3002c05c70093
0556ffff078d0007055600000556fffd04e3001602aa00920239fffd02aa
002604ac00730473ffed02aa002a0473004904e300870473005504e30054
0473004102aa001804e3005404e30092023900930239ffa2047300890239
0093071d007e04e3009104e3005204e3008b04e3005b031d008704730030
02aa001f04e3008d0473000b063900090473000c0473000e04000022031d
003c023d00b0031d002d04ac004305c7000005c7000005c7006105560095
05c700980639005905c70093047300490473004904730049047300490473
004904730049047300570473004104730041047300410473004102390092
0239ffe90239ffcd0239ffd004e3009104e3005204e3005204e3005204e3
005204e3005204e3008d04e3008d04e3008d04e3008d0473004403330056
047300540473000d0473003b02cd00420473fffe04e3008b05e5fff705e5
fff7080000d802aa00bb02aa0005046400310800ffaa0639003f05b40098
046400320464003c0464003c04730001049c006f03f4002c05b4007a0696
00a1046400000231000002f6002502ec001a06250037071d005804e30057
04e3006502aa00c304ac0055046400540473ffec0464001f04e5001a0473
00600473006a080000c905c7000005c700000639005908000048078d0058
0473fffc08000000040000840400006902390098023900720464003103f4
002f0473000e0556fff70156fea90473ffe002aa004b02aa004b04e3001f
04e3001f047300440239009302390075040000710800000105c700000556
009505c7000005560095055600950239006a0239ffae0239ffbf0239ffc1
06390059063900590639005905c7009305c7009305c700930239009302aa
000302aafff302aa001302aa001a02aa00cd02aa009102aa002602aa0060
02aa00a002aa000304e3000a0239000a0556004a0473003004e300160400
0022023d00b005c7fffd04e300530556fff70473000e0556009504e3008b
04ac005504ac006d02aa005b02aa001902aa002806ac005c06ac005c06ac
0028047300000639006204e300540239008c0556004a0473003005c70061
0473005505c700610473005504e30054046bffed02aa01ea05c700000473
004905c700000473004905c7009405c0005105c7fffd0556009504730041
055600950473004104e3009d0239007904e3009d0315009504e3009a03d5
009005c7009804e3009105c7009804e300910639005904e3005205c70096
031d008705c70096031d00500556004a0473003004e3002c02aa001f04e3
002c03d5001e05c7009304e3008d05c7009304e3008d04e3001604000022
04e300160400002204cf009a063900560691005604eb004e04da004e03cc
004e0579004e0392003005b9004e046bffed04d500b8032b004f08c00029
0800004f040000990800004f040000990800004f040000980400009807d5
016a05c7008f04ab005504d5009d04ac005504d5022204d5010505abffe9
050001c905ab027e05abffe905ab027e05abffe905ab027e05abffe905ab
ffe905abffe905abffe905abffe905ab01c005ab027e05ab01c005ab01c0
05abffe905abffe905abffe905ab027e05ab01c005ab01c005abffe905ab
ffe905abffe905ab027e05ab01c005ab01c005abffe905abffe905abffe9
05abffe905abffe905abffe905abffe905abffe905abffe905abffe905ab
ffe905abffe905abffe905abffe905abffe905abffe905ab02d605ab0066
05abffea05d5ffff04d500920800000007eb013007eb012007eb013007eb
012004d500b204d5008004d5002a082b0198086b01b807550010060000f4
0600006f0440003a0540003704c0003f0415004004000025060000550647
008c0473009005abffc701eb008d03d500860715002303e9001804d50092
02d6005c02d6005c04d500b202d6004d05c700000473004905c700610473
005505c70061047300550556009504730041055600950473004105560095
047300410639006204e300540639006204e300540639006204e3005405c7
009604e3009205c7000504e300190239ffba0239ffbb0239ffda0239ffda
0239ffe10239ffe20239006e02390075047300230239ffa205c700990473
00890473008d04e3009d0239ffed05c7009804e3009105c9009c04e3008e
0639005904e300520639005904e3005205c70096031d002a0556004a0473
003004e3002c02aa000705c7009304e3008d05c7009304e3008d05c70093
04e3008d05c7009304e3008d078d0007063900090556fffd0473000e0239
008d05c70000047300490800ffaa071d00580639003f04e3005702aa00c9
078d000706390009078d000706390009078d0007063900090556fffd0473
000e0239009502aaffd70473000d04cd005a06ac005c06ac002906ac0030
06ac002f02aa00bc02aa002602aa00bb03b8fff405c7ffe806d3ffbb073f
ffbb03caffbb0699ffa6076bffc806b4ff9c0239ff2905c7000005c70096
05c000000556009504e3001605c700960239008c05c700990556000006aa
009105c70098052600660639005905c7009a0556009504cd005a04e3002c
0556fffd0556000006790056066a00620239ffcc0556ffff04eb004e039c
004e04e3008e0239008204a8006c04e200900473000f03af004e04e3008e
0453004e023900930476008e0473000f04e500900473000b0390004e04e3
005204f300760429004e04a80076049b00110607007606c2004e0239ffcd
04a8007604e3004e04a8007606c2004e055a00970715002f048900a405b1
00580556004a0239008c0235ffca0473002308c0001a0880009d07000037
04e2009a04fa000005c0009905c7000005c0009b05c70096048900a405b3
fffa05560095073b00170503002c05c0009905c0009904e2009a059d0020
06aa009105c700960639005905c000990556009505c7006104e3002c04fa
000006d400590556000005d8009a059f007d080a009a0827009a06f5001a
07d5009d05c0009b05b100570840009605c000040473004904f1005c04eb
0096035500880514fff90473004105acffff03fa001804eb008c04eb008c
040100880515001905eb009b04d5008804e3005204d5008804e3008b0473
005503eb00150473000e070000540473000c04eb008904a5007206ab008c
06c0008d05d5002806d5009504eb0099046b003806d5009104abfffb0473
004504e3000003550088046b005104730030023900930240ffd00239ffa2
07c000180740008c04e30000040100880473001204d5008803e500960393
00880800004108eb00a30620003002aa010102aa001e02aa003102aa0031
02aa010102aa007f02aa007e02aa008c02aa008c02aa010102aa001002aa
010102aa01210393007d02aa008c026500c802aa030202aaff0102aa00c9
04a90059049b004103a7000a0466003204ea0082022f0087034e005a04ed
00870503007d022f0087042c002803ed004b03f8004104e30087050a0037
022f00870316004b04e800500459000a04c0006404b2006403ff000a0418
000a04950082042c002805b8005a0563002d045e0087045e0087045e0087
0236005004090050068b0087022fffac042c0028042c002803f8ff1603f8
ff160479003205b8005a05b8005a05b8005a05b8005a04a9005904a90059
04a90059049b004103a2000a0466003204ea008202950000038100000503
007d02950000042c002803ed004b03f80041050a00370316004b04e80050
04c0006404b200640418000a04950082042c002805b8005a0563002d022f
0087049b004103ed004b04b2006404db00410000ffdc0000ff250000ffdc
0000fe51028d00ab028d00a002da004303c0007e0196ffba019c004601e5
0046019c0046019c004601ad0048019c004601b1004601510046047e0188
047e0150047e0104047e009e047e012d047e00ea047e00d5047e009c047e
00bc047e00ee04350085028d00c1043500b3060001000600010002be0058
06000100047e00a5047e00bd047e00de0600010006000100060001000600
01000600010001b100460600010006000100060001000600010006000100
06000100060001000600010004e6ffba0600010006000100060001000532
003905320039022cffba022cffba06000100060001000600010006000100
049e0034047800300430ffba0430ffba0376000a0376000a060e00290708
002902e2ffba0456ffba060e00290708002902e2ffba0456ffba05280097
046f000a0600010006000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
060001000600010001cf003001b1004601b1004601b1004001b100460600
0100060001000000ffdc0000fe510000ff160000ff160000ff160000ff16
0000ff160000ff160000ff160000ff160000ff160000ffdc0000ff160000
ffdc0000ff200000ffdc0473002d08000000060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
01000600010006000100028d007f028d00670600010005a0002e03c0007e
01e800000207ffc301bc005e01e0fffa039c0006039c000601bc005e01e0
001a05280097049e0011022cffba022cffba01bc008801e0001a05320039
05320039022cffba022cffba02be0036035200030532003905320039022c
ffba022cffba0532003c0532003c022cffba022cffba049e003404780030
0430ffba0430ffba049e0034047800300430ffba0430ffba049e00340478
00300430ffba0430ffba02be006902be006902be006902be00690376000a
0376000a0376000a0376000a073200400732004004deffba04deffba0732
00400732004004deffba04deffba0880004008800040062cffba062cffba
0880004008800040062cffba062cffba0430ffba0430ffba0430ffba0430
ffba0430ffba0430ffba0430ffba0430ffba0454003403c000460454ffba
02e2ffba0454003403c000460454ffba02e2ffba0610002f0610002f0270
ffba0298ffba04e6002704e600270270ffba0298ffba0454002904540029
02e2ffba02e2ffba039c0023039c002301e0ffba01e0ffba02e2002102e2
00210352ffba0352ffba0454003e0454003e022cffba022cffba02be0058
0352000303c0ffba039cffba039c0006039c000605280097046f000a0528
0097049e0011022cffba022cffba0454000004c4000003e400220454001a
03e400220454001a03e400220454001a0600010006000100019c0046019c
00460600010006000100060001000151004601b100460600010006000100
01ad004801e5004606000100060001000600010001b1004601b1004601b1
004601b1004601b1004001cf003006000100019c0046019c004606000100
060001000600010006000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
0100028d00ca028d00c7028d00c606000100060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
0600010006000100060001000600010002be00690100ffba0800ffba1000
ffbb06d3005905b0005206a3009305cb008d0000fd880000fbc10000fc5f
0000fe310000fcad0000fd550000fe260000fdf10000fd180000fc690000
fd950000fbe00000fc700000fed40000fecd0000fea0041b007806ac005c
06ac00190000fe450000fd550000fda60000fc5f0000fe250000fd180000
fbe00000fafa0000fb360000fc700000fb870000fb9b0000fcce0000fc54
0000fbc30000fc940000fbf50000fdb00000fe590000fd7e0000fc820000
fd340000fe500000fe460000fcd10000fd3e0000fd020000fc3a0000fce9
0000fc260000fc070000fc2f0000fb9e0000fb760239009305c700000473
004905c700000473004905c700000473004905c700000473004905c70000
0473004905c700000473004905c700000473004905c700000473004905c7
00000473004905c700000473004905c700000473004905c7000004730049
055600950473004105560095047300410556009504730041055600950473
004105560095047300410556009504730041055600950473004105560095
047300410239006a0239005d0239008c023900930639005904e300520639
005904e300520639005904e300520639005904e300520639005904e30052
0639005904e300520639005904e3005206d3005905b0005206d3005905b0
005206d3005905b0005206d3005905b0005206d3005905b0005205c70093
04e3008d05c7009304e3008d06a3009305cb008d06a3009305cb008d06a3
009305cb008d06a3009305cb008d06a3009305cb008d0556fffd0473000e
0556fffd0473000e0556fffd0473000e05c70000047300490239ffca0239
ffca0639005904e3005205c7009304e3008d05c7009304e3008d05c70093
04e3008d05c7009304e3008d05c7009304e3008d0000fef90000fef90000
fef40000feef0489fffd03550007073b001705acffff04e2009a04010088
04e2009a0401008805c7009604d500880473000104730012047300010473
0012055600000473000c059f007d04a50072059f009c04e3009205cf0059
0473004c0639005604e3005205320039022cffba0270ffba0298ffba04e6
0027022c0065022c0016022c0016022c0011022c0043022cffd20000fef0
01a8000f01a8fff502aa009002aa009001e8000001bc005e01bc005e0000
ffcb01bc000f01e0ffbf01bcfff501e0ffcd01bc001d01e0000901bc0088
01e0001a039c0006039c0006039c0006039c000605280097046f000a0532
003905320039022cffba022cffba0532003905320039022cffba022cffba
0532003905320039022cffba022cffba0532003905320039022cffba022c
ffba0532003905320039022cffba022cffba0532003905320039022cffba
022cffba0532003905320039022cffba022cffba049e0034047800300430
ffba0430ffba049e0034047800300430ffba0430ffba049e003404780030
0430ffba0430ffba049e0034047800300430ffba0430ffba049e00340478
00300430ffba0430ffba049e0034047800300430ffba0430ffba02be004f
02be004f02be006902be006902be006902be006902be004f02be004f02be
006602be006602be006902be006902be006902be006902be002f02be002f
02be002202be00220376000a0376000a0376000a0376000a0376000a0376
000a0376000a0376000a0376000a0376000a0376000a0376000a0376000a
0376000a0376000a0376000a073200400732004004deffba04deffba0732
00400732004004deffba04deffba073200400732004004deffba04deffba
0880004008800040062cffba062cffba0880004008800040062cffba062c
ffba0430ffba0430ffba0454003403c000460454ffba02e2ffba0610002f
0610002f0610002f0270ffba0298ffba0610002f0610002f0270ffba0298
ffba0610002f0610002f0270ffba0298ffba0610002f0610002f0270ffba
0298ffba0610002f0610002f0270ffba0298ffba04e6002704e6002704e6
002704e60027060e00290708002902e2ffba0456ffba060e002907080029
02e2ffba0456ffba045400290454002902e2ffba02e2ffba045400290454
002902e2ffba02e2ffba045400290454002902e2ffba02e2ffba060e0029
0708002902e2ffba0456ffba060e00290708002902e2ffba0456ffba060e
00290708002902e2ffba0456ffba060e00290708002902e2ffba0456ffba
060e00290708002902e2ffba0456ffba039c0023039c002301e0ffba01e0
ffba039c0023039c002301e0ffb101e0ffb1039c0023039c002301e0ffba
01e0ffba039c0023039c002301e0ffba01e0ffba0454003e0454003e022c
ffba022cffba0454003e0454003e0454003e0454003e0454003e0454003e
022cffba022cffba0454003e0454003e049e0034047800300430ffba0430
ffba02be005803520003031a001a031a001a031a001a039c0006039c0006
039c0006039c0006039c0006039c0006039c0006039c0006039c0006039c
0006039c0006039c0006039c0006039c0006039c0006039c000605280042
046fffd905280097046f000a022cffba022cffba039c0006039c00060528
0097046f000a022cffba022cffba05280097046f000a067f0044067f0045
067f0044067f004501a800280000fe290000fe8c0000ff250000ff230000
fefa0000ff7a0000fe5908fc003208ad00320000ffb50000ffb60000fef0
0000ff590000fe590000ff8c01b4000002f700000000fe850000ff0704cd
00320000ff580000ff580000ff59073200400732004004deffba04deffba
0880004008800040062cffba062cffba0454003403c000460454ffba02e2
ffba03c0007e02e2002102be0058022cffba0290ffba01f4002f01f4003b
01f4001201f400b101f4006d060e002907080029022f00870000fec80350
0000045e008703e4fff50454fff503e400220454001a03e400220454001a
03e400220454001a03e400220454001a03e400220454001a03e400220454
001a047e0072047e00bd03e4000f0454000f000000000000006c0000006c
0000006c0000006c0000006c0000006c0000006c0000006c000001d20000
01d2000001d20000025c000002e6000002e6000002e600000356000003a4
000003e2000004380000053c000005be00000764000008bc000009d60000
0b4800000c7c00000c7c00000e1a00000e1a00000e1a00000e1a00000e1a
00000e1a00000e1a00000e1a00000e1a00000e1a00000e1a00000e1a0000
0e1a00000ed800000f74000010ba000010ba000010ba000010ba000010ba
00001116000011160000111600001116000011e6000011e6000011e60000
11e6000011e6000011e6000011e6000011e6000011e6000011e6000011e6
0000125a0000125a000012c2000012c2000012c2000012c2000014d00000
15cc00001708000017f800001a0400001b0400001ce000001de000001e82
00001e8200001e8200001eee000020a20000218c0000227c0000227c0000
227c00002360000026a6000027c6000028ae000028ae000028ae00002a84
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020000
2c0200002c0200002c0200002c0200002c0200002c0200002c0200002c02
00002c0200002c0200002c0200002c0200002c0200002c0200002c020001
0000068a00f2003c006f000600020010002f00550000064e106f00030002
be0054039a000f0101001fffc00398b310143240b80399b30f1332404110
039500500395000200b0034d00c0034d0002006f0391007f03910002ffc0
034bb22d3132b9ffc0034bb30a0e32104110038b0020038b0080038b0003
00a0038b00010020038b0040038b0002ffc0038bb313163240b80383b20f
1132b9ffc0037bb2303432b9ffc0037bb310183250411403780001036503
6e0023001f037e036e001e001f0363036e001d001f03620364000d001fff
c00340b30f1032804110033f0001033f03150029001f034103160032001f
0344031a001b001fffc00375b20e1132b9ffc00375b2282a32410a034303
180032001f030f030d0034001f03080307b2321f20bb0340000100400388
b3090b3240b80388b2101532bd038503070014001f03800307b2171f0fbd
030a002f030a0002ffc00354b3090d3290410c035400a003540002001f03
6e0001009f036e00010040036eb2090b32410a0345031c0016001f036b03
1d0015001f0346031eb2151fc0bb0393000100400392b3090d3240b8033e
b2083340b8033eb30d0e32c04109033e000100b0038e00c0038e0002ffc0
0390b326383200412603280030032800020020037f0030037f0002001003
8a0030038a0050038a006f038a007f038a009f038a000600000389003003
890002002f037a0070037700900377009f037a0004ffc00315b20f1032b9
ffc00315b2242832b903190318b2321f10bb031a0001ffc0031ab3090e32
40b80318b2121332b9ffc00318b30c0e323fbd0373004f03730002004003
74b31718326fbb032a00010040032cb3181b3240b80370b2090c32bd0317
03160032001fffc00316b20e1132bd031c031e0016001f031d031eb2151f
b0411f031e0001000f031f000102ca02d00015001f02d302d5000d001f02
cf02d0000d001f02cb02d0000d001f02cd02d0000d001f02ce02d0000d00
1fffc002d0b3090c3240b802d2b3090c32e0411c02e50001005f02dd009f
02e5000202bb02c30030001f02da02b80032001f02d902b9003f001f02d8
02b80064001f02b902b80033001f02bab221c81fb802b8b321c81f40b803
9bb20d1632b9ffc002c3b22b2f32b9ffc002c3b21f2532b9ffc002c3b217
1b32b9ffc002c3b2121632412502c202c1001c001f02d702c10024001f02
c102c00022001f02bf02c00018001f02c0027400c8001f02b50235003b00
1f02b40235003b001f02c402bc001e001f02b702b60038001f02b3b20ec8
1fb802b0b207c81fb802afb206c81fb802aeb200c81fb802afb2502f1fbc
02ae02ab001a001f02adb2261a1fb802a8b326241f0fbb0235000102a502
74b21d1f12410a02a1015801f4001f02a000d801f4001f001202a2b237c8
1fb80290b2bc201fb9029002904018374025402d40a6033025302d30a603
2025202d203720a6204110028e0005009f028b0001028b028b0037002002
89003002890040028900900289b20437b041fd027400c002740002008002
7400a0027400020060027400700274000200000274001002740002008002
7400f002740002003f0285004f028500020090027e0090027f0090028000
90028100040090027a0090027b0090027c0090027d000400900274009002
750090027700030070027e0070027f007002800070028100040070027a00
70027b0070027c0070027d00040070027400700275007002770003006002
7e0060027f006002800060028100040060027a0060027b0060027c006002
7d000400600274006002750060027700030050027e0050027f0050028000
50028100040050027a0050027b0050027c0050027d000400500274005002
750050027700030040027e0040027f004002800040028100040040027a00
40027b0040027c0040027d00040040027400400275004002770003003002
7e0030027f003002800030028100040030027a0030027b0030027c003002
7d000400300274003002750030027700030020027e0020027f0020028000
20028100040020027a0020027b0020027c0020027d000400200274002002
750020027700030010027e0010027f001002800010028100040010027a00
10027b0010027c0010027d0004001002740010027500100277000300e002
7e00e0027f00e0028000e00281000400e0027a00e0027b00e0027c00e002
7d000400e0027400e0027500e00277b103d041c5027e00d0027f00d00280
00d00281000400d0027a00d0027b00d0027c00d0027d000400d0027400d0
027500d0027700030030027400400274000200c0027e00c0027f00c00280
00c00281000400c0027a00c0027b00c0027c00c0027d000400c0027400c0
027500c00277000300b0027e00b0027f00b0028000b00281000400b0027a
00b0027b00b0027c00b0027d000400b0027400b0027500b00277000300a0
027e00a0027f00a0028000a00281000400a0027a00a0027b00a0027c00a0
027d000400a0027400a0027500a0027700030090027e0090027f00900280
0090028100040090027a0090027b0090027c0090027d0004009002740090
02750090027700030020027e0020027f002002800020028100040020027a
0020027b0020027c0020027d000400200274002002750020027700030281
01580801001f028001290801001f027f00ec0801001f027e00d80801001f
027d00b10801001f027c00a60801001f027b00820801001f027a00370801
001f027700260801001f027500200801001f0274001f0801b21f370f4116
0235004f0235005f0235006f0235009f023500af023500bf0235000700af
023500cf023500df023500ff02354022040f074f079f07af07bf0705af07
e007020f064f069f06af06bf0605af06e0060220411b020d0001005f0235
0001008f02350001007f023500ef02350002002f0235003f02350002003f
0234004f0234000202350235023402344011ed20ef2a01cf2a01bf2a01af
2a018f2a01410902470104001e001f022000370201001f0158400c263e1f
d8263e1f3726273e1fb8028eb6ec171fb226361fb801bcb226361fb80129
402b26361fec26361fb126361fa626361f8226361f3726361f3226361f2d
26361f2526361f1f26361f37262a1fb801584022263e1fd8263e1fbc263e
1f27263e1f21263e1f20263e1f3700161600000012110840b9020d01a6b3
c50d0009b801bcb227281fb801bbb227301fb801b8b2274f1fb801b7b227
621f410901b600270101001f01b5002002ab001f01afb21fe41fb801adb2
1fe41fb801acb21fbb1fb801a8b21f341fb8015db2272e1fb8015bb227cd
1f410d0155001f0401001f0154001f0401001f0153001f0201001f0152b2
1f561fb80151b21f291fb8012bb227261f410d012a00270125001f012901
5800e4001f0125001f0401001f0124b21fe41fb80123b21f3b1fb80122b2
1f391f410d010800270801001f0106002d0101001f0105001f0101001f01
03b31fbb1fefb901580401400b1fed1f931fec1fe41feb1fb80201b21fd9
20b80401b21fcf25b80156400a1fbc2d9e1fbb1f411fb2410a0158040100
1f00b101580401001f00b001580401b51fa625891f9bb901580125b61f99
1f2e1f8e2db80801b51f8d1f291f89b901580401b21f8220b802ab40131f
801f301f742de41f731f4a1f611f521f5d25b802abb21f5c1fbc0801001f
0059015802abb61f5025891f491fb80125b21f4725b80401400b1f461f79
1f401f271f3920bc02ab001f003801580401b21f372dbc0125001f003201
580125b61f2c1f341f2a25b80801b21f5537b80111402a07f00790075b07
42073b07230722071e071d071408120810080e080c080a08080806080408
0208000814b8ffe0402b0000010014061000000100060400000100041000
0001001002000001000200000001000002010802004a00b013034b024b53
42014bb0c063004b6220b0f65323b8010a515ab005234201b0124b004b54
42b0382b4bb807ff52b0372b4bb007505b58b101018e59b0382bb00288b8
01005458b801ffb101018e851bb0124358b10100858d1bb900010119858d
5959001816763f183f123e113946443e113946443e113946443e11394644
3e11394660443e11394660442b2b2b2b2b2b2b2b2b2b2b182b2b2b2b2b2b
2b2b2b2b182b1db0964b5358b0aa1d59b0324b5358b0ff1d594bb0815320
5c58b9020f020d4544b9020e020d45445958b90470020f455258b9020f04
704459594bb0e453205c58b90020020e4544b90027020e45445958b90842
0020455258b9002008424459594bb8012553205c58b90026020f4544b900
21020f45445958b90a0d0026455258b900260a0d4459594bb8040153205c
58b1d8204544b1202045445958b9250000d8455258b900d825004459594b
b8040153205c58b9015800264544b1262645445958b923200158455258b9
015823204459594bb02953205c58b11f1f4544b12d1f45445958b9010d00
1f455258b9001f010d4459594bb02f53205c58b11f1f4544b1251f454459
58b90135001f455258b9001f01354459594bb8030153205c58b11f1f4544
b11f1f45445958b91428001f455258b9001f14284459592b2b2b2b2b2b2b
2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b
2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b65422b
01b331757ec3456523456023456560234560b08b766818b080622020b17e
754565234520b003266062636820b003266165b075236544b07e234420b1
31c34565234520b003266062636820b003266165b0c3236544b0312344b1
00c3455458b1c3406544b23140314523614459b33f3c5841456523456023
456560234560b089766818b080622020b1583c4565234520b00326606263
6820b003266165b03c236544b058234420b13f414565234520b003266062
636820b003266165b041236544b03f2344b10041455458b141406544b23f
403f452361445945695342014b5058b108004259435c58b108004259b302
0b0a124358601b2159421610703eb0124358b93b21187e1bba040001a800
0b2b59b00c2342b00d2342b0124358b92d412d411bba04000400000b2b59
b00e2342b00f2342b0124358b9187e3b211bba01a80400000b2b59b01023
42b0112342002b2b2b2b2b2b2b2b00b01243584bb035514bb021535a58b1
262645b040614459592b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b7373
73737345b040614418004569444569447373737473737374737473742b2b
2b2b2b2b2b2b2b2b2b2b0073737373737373737373737373737373737373
737373747474747474747474747474747474747474747474757575737475
7575752b7300004bb02a534bb036515a58b1070745b040604459004bb02e
534bb036515a58b1030345b0406044b1090945b8ffc06044592b45694401
74007373732b4569442b012b435c58400a0006000702a006a00702b9ffc0
0274b31a1d326fbd0277007f02770002ffc00277b22f3132b9ffc00277b3
22253240b80274b32f353240b80274b3282a3240b80274b21a2132b8ffc0
b3371a1d32b8ffc0b3251a1d32b8ffc040112d1a1d329025902d9037a025
a02da03706b8ffc0b6a61a1d321fa61fb8028eb22fa60300742b732b2b2b
2b2b2b2b2b742b737459002b2b435c58b9ffc002a1b21c1d32b9ffc002a0
b21c1d322b2b592b73012b2b2b2b002b2b2b2b2b2b2b2b2b2b2b2b2b2b2b
2b2b2b012b2b2b2b2b2b2b73742b2b2b2b2b2b2b2b73732b2b2b2b2b2b73
2b732b2b2b742b2b2b73737373732b73732b2b2b73002b2b2b2b7374732b
732b2b2b2b752b2b2b2b2b2b2b2b752b2b2b2b2b732b2b2b2b7374752b2b
7373732b2b2b2b0000>
[11267 ] AllocGlyphStorage
]def 
108 44 
PrepFor2015
Type42DictEnd
1 0 0 <00020100000005000500000300070042b40201fe0607b8023f4013000504
fe03000a0704fe010019080605fe0203bc0126000901b0011800182b10f6
3cfd3c4e10f43c4dfd3c003f3cfd3c10fc3cfd3c31302111211125211121
01000400fc2003c0fc400500fb002004c000>/ZYCIBP+Arial-BoldMT AddT42Char 

1 0 213 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 223 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 3 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 4 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 5 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 6 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 7 <> /ZYCIBP+Arial-BoldMT AddT42Char 
1 108 8 <00050059ffc506bd05d3000b001b001f002b003b00b2404e1f1c6f1c011c
d51d1e141d1d1e1d0c1c06141e201f342c1c301d23e438f530e41d2b2909
e410f518e41f1e0301003d103d023d17171a002601f02601265c34af002c
01f02c012c5c0f201f200220b80109401d000601f00601065c14af000c01
f00c010c5c4f005f000200193c4d43182b4e10f45d4dfd5d71f6fd5d71f6
5dfd5d71f6fd5d714e456544e65d003f3c3c4dedf4ed2fe4edf4ed111239
0111123912391112391239872e2b5d7d10c4313013343633321615140623
222637141716333237363534272623220706012301330134363332161514
062322263714171633323736353427262322070659ad9499adad9499addb
21192c2d192020192d2c1921013cd0030dcafebfad9697adad9499addb21
192c2d182120192d2d18210450c5bebdc6c5bebdc88f312424318f8f3025
2431fae7060bfb76c5bebec5c6bebec78f302524318f8f3124243100>/ZYCIBP+Arial-BoldMT AddT42Char 

1 0 9 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 10 <> /ZYCIBP+Arial-BoldMT AddT42Char 
1 466 11 <0001006bfe51026805d300100046400e280fa70302080901000910001208
bd012200090001012200000294400a09f30c9b200430040204b80296b311
a56b182b10f65dedfdf4ed10ed003f3f103c103c3130015d012326023510
13363733020215141217160265c199a0635684c089673d3523fe51e701f2
e901210102e0bdfed1fe57eea4fea89b6600>/ZYCIBP+Arial-BoldMT AddT42Char 
1 604 12 <00010043fe51024005d30010004940182702270a6702670a9702a702a80e
07090810000810001210bd012200000009012200000294b408f3059b0cb8
0296b3126a43182b10f6edfde4ed10ed003f3f103c103c3130015d133e03
3534020333161215140702034553443a1c6689bf97a7424bacfe51b2bef8
df75ee01a9012fd7fe1ef8d1effef4fefb00>/ZYCIBP+Arial-BoldMT AddT42Char 

1 0 13 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 14 <> /ZYCIBP+Arial-BoldMT AddT42Char 
1 742 15 <00010075feb901a50119000b003fb509080b060a07b8011e401b069c0138
0b0a0a72012607240f001f00200030000400190c6776182b4e10f45d4de4
fded003f4dedf4fd0111390011393931301321151406060727363637238c
01192a755a37554802880119c97a8d7020741c625500>/ZYCIBP+Arial-BoldMT AddT42Char 
1 854 16 <000100410187026902a00003003240213001400102013700000310032003
30030403440510002000300003001904a56c182b4e10e45d4d10e65d002f
ed5d31301311211141022801870119fee700>/ZYCIBP+Arial-BoldMT AddT42Char 
1 932 17 <00010093000001ac01190003002440150238000a02260f001f0020003000
040019046776182b4e10f45d4dfd003f4ded3130331121119301190119fe
e700>/ZYCIBP+Arial-BoldMT AddT42Char 
1 994 18 <0001fffdffe7023b05d300030038401d0001014902031402020302010003
000a01eb021a0503eb001904936c182b4e10f44ded4e10f64ded003f3c3f
3c87052e2b7d10c431300701330103016bd3fe911905ecfa1400>/ZYCIBP+Arial-BoldMT AddT42Char 
1 1080 19 <00020056ffe7040e05c0000e00200093404b780a880aa701aa07aa09a70e
b709c8090856115916591a561f67116816681a671f08390239063609360d
490249064509460da709cb02c906c409c40dd902db06d409d40d11101820
180218b8ffc0402512163418a6080d1f0f2f0f020f401216340fa600051d
d84f0401041a2214d80b1921d3c2182b4e10f44ded4e10f6714ded003fed
2b713fed2b713130015d005d5d0132171611100706232200111037361722
060706111016163332363736111026260232d5788f9077d5d6fefa9077d5
3350161d344f333350161d344f05c098b4fe5ffe60b696014901a6019eb6
96e941546dfefefefec14041546c01020102c141>/ZYCIBP+Arial-BoldMT AddT42Char 
1 1340 20 <000100a20000032605c00009005640096b027b028b02030204b80129b35f
050105b8025eb708090501000c0900bb015800020001025d400d0500041f
042004b0040404190aba01a701a000182b4e10f45d3c4df63cfd3c003f3c
3f3cf45ded393130005d212111060735362437330326fee79ad16e010230
e404239045ff24c98600>/ZYCIBP+Arial-BoldMT AddT42Char 
1 1470 21 <000100330000040c05c0001d013f405fb518b61ab91bca04c718d018d019
d01a08431b431c431d56199b049518aa04a61c08061a20002806371a4804
43184319431a0824182419241a03162604560488189c1b9c1c9c1daa1caa
1d0812001d101d201d311d761d841d901dd61d081db8ffc040161415341d
02100c0f1d10002000022000300040000300b8ffc0b312163400b802a1b3
02010c0fb8015640231f0c2f0c020c401216340ca6130509d81616014f00
01001a1f0fd8107702191ed3c2182b4e10f44df4ed4e10f6713c3c4d10ed
003ffd2b71e43f3cfd2b5d713c1112390111332b5d435c58b9001dffc0b2
11391db8ffc0b20f391db8ffc0400e10390408103905081139040811392b
2b2b2b2b2b59b10602435458400b091b191b021b13010413000011123911
12395d593130015d4b5158bd001bffe0001cffe0001dffe0383838590171
5d5d5d011121361237363736353426232206072536243332161514060706
040607040cfc2710a0ecbe2b3a6559586808fee8190108c6d9f8474d33fe
f647160105fefb940109dbb13f57555e656a7b1ce8caeaae63b36241f450
2600>/ZYCIBP+Arial-BoldMT AddT42Char 
1 1892 22 <0001004dffe7041b05c0002900d940328715c915027b1c8b1c02a603a905
a714b603ba05b614da18dd19081614018d168d1702210a0d000401171316
211f0d100c0ab80124400c4f0d01400d8f0d020d0d0116b80102400f1f13
2f1302134012163413a61b0501b80156b5100420040204b8ffc040321216
3404a6270db00cc00c020c0c1610d87f1f8f1f9f1faf1fbf1f051fe007d8
4f2401241a2b16d8177701d800192ad3c2182b4e10f44dedf4ed4e10f671
4dedf45ded11392f5d003ffd2b71e43ffd2b71e411392f5d71ed01111239
1139001112391112391112395d313001715d5d005d132516163332363534
2623220737163635342623220607253e0233321716151407161615140023
22244d01100d725157777252364b1f7278584948660bfefd1b6dc379cf7d
67d37e97fee6d2c7fefa018521686e84706a7c15e50369574a5864602c85
9f5b846c88c1731bbc85c1fef0e5>/ZYCIBP+Arial-BoldMT AddT42Char 
1 2236 23 <000200260000044405c0000a000d00df40390c200d39090c190c2b0c530c
6b0ce20c06ed0d01060416042504280d480d5b0da70db70dc60d09010208
000c060d07050a0b0d07000c0c0d0db801ae401a03041403030403020c04
0d030d02040a0007400dc00dd00d030dbb01280008000201b4b600040400
0c0c00b80158b4058f0a010ab80102401210079f07bf0703071a0f3f027f
020202190eba014c014800182b4e10e47110f65d4df45d3cfd3c003f3f10
f43cfd5d3c0111123912393900111239123987052e2b047d10c40f0f0fb1
0602435458400b2d0c3d0c4d0ccd0cdd0c05005d593130015d5d005d2b21
11213501331133152311011101027efda8027cecb6b6fef0feaf0127f603
a3fc5ef7fed9021e01f5fe0b>/ZYCIBP+Arial-BoldMT AddT42Char 
1 2518 24 <0001005bffe7043505a6001d01104029080e200c371245124919990d9e0e
9712da0e0912111312211123128512050004010d0a0c0c0d121111b802a0
40160e0d140e0e0d120a1420013001400103500190010201b80156b51004
20040204b8ffc0b712163404a61b0d0cb8025a400d1f0a2f0a020a401216
340aa614b8ffc0400b1416342014301440140314b801ab401411111f102f
10022f103f104f1003104012163410b802a040130f0f0e040f10e007d8d0
1701401701171a1f0eb8012140120d7701bcd0000140009f00af00030019
1ed3b9014700182b4e10f45d714dedf4e44e10f65d714dedf43c003f3c10
fd2b5d713c10f65d2bfd2b71e43ffd2b71e45d7111123987052e2b0e7d10
c401113900111239111239313001715d1325161633323635342623220727
132111210736333200151407062322245b01180c764d587a79617960e490
02e7fdee2c5e62bb0104698ffecbff0001791d5f6f8f9087876b2102fbfe
f9f92ffef0d9b58ec2da>/ZYCIBP+Arial-BoldMT AddT42Char 
1 2888 25 <00020057ffe7042a05c00017002300bd403b6a0b750887089719a705a708
a90eaa13b90eb611bd13c011cf130d1505361144107a16b502d210d01407
bb00cf0002000401071812101b201b021bb8ffc0401e1216341ba60f0d1f
212f2102214012163421a63f09014009d009ff090309b8014fb3af010101
b8012140221f042f0402044012163404a6150501d800771ed84f0c010c1a
2518d8121924d3c2182b4e10f44ded4e10f6714dedf4ed003ffd2b71f45d
f65d71ed2b713fed2b7101111239001112395d3130015d005d0105262623
220607363332121514002322001110003332160114163332363534262322
06040ffef00a5443597b10699cb0fbfef8cfdefee2012aeea7dbfda17e51
4e687054517004531e5450a0fd7cfef4d4e1fef00159018901930164bbfc
e989957a8b8f857f>/ZYCIBP+Arial-BoldMT AddT42Char 

1 0 26 <> /ZYCIBP+Arial-BoldMT AddT42Char 
1 3196 27 <00030053ffe6041705c0001800240030010db530081d1f3426b8fff8406c
1d1f34c711c713d705d707047510761484100326002a0c36003b0c46004c
0c6e0463086711681577278727970d9818a40da918a91aa61ea727a62ca9
30b91ab71e17771386138614872704970c010c970001001c2e980c010c2b
099700010025032e401216343f2e4f2e022eba028e001cffc04010161834
701c801c02a01c011c1c061228b8ffc04009121634302840280228b8028e
400d120d3f224f2202224012163422b8028e401a06051fd809772bd84f0f
010f1a3219d8037725d8161931d3c2182b4e10f44dedf4ed4e10f6714ded
f4ed003fed2b5d3ffd5d2b1011392f5d712bed5d2b011112395d1112395d
001112395d395d313001715d00715d2b2b01262635343633321615140607
161615140423222726353436131416333236353426232206031416333236
35342623220601486d63e5d3d1e76a607a7ffefdd7c8859d76b95f4f5060
5f4e51601a775957727459676503172ea160a4d6d6a4669f2a31bc7bcbfe
697cd877c70151545e5f544f5f60fd3d74827d76677d8e00>/ZYCIBP+Arial-BoldMT AddT42Char 

1 0 28 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 29 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 30 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 31 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 32 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 33 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 34 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 35 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 36 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 37 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 38 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 39 <> /ZYCIBP+Arial-BoldMT AddT42Char 
1 3610 40 <00010095000004f005ba000b0090403d08050407082506121f05013005af
05020505090304250201020a09250b000807064b0302480a000b010b1a20
0d300d400d030d04092001200030000200b8028bb30c3153182b4e10f45d
3c4dfd3c4e105df65d3c4df43cf43c003f3cfd3c3f3cfd3c11392f5d7143
5c58b90005ffc0b21d3905b8ff80b21a3905b8ff80b113392b2b2b593cfd
3c0305103c3c313033112115211121152111211595043ffce902e0fd2003
3305baf8febbf7fe71f7>/ZYCIBP+Arial-BoldMT AddT42Char 
1 3800 41 <000100970000048405ba00090072403f0805040605250720083008bf08df
08042f08900802080800030425020102090008073f064f06020652030002
01021a200b300b020b04092001200030000200b8028bb30a3153182b4e10
f45d3c4dfd3c4e105df65d3c4df45d3c003f3c3f3cfd3c12392f5d713cfd
3c0305103c3c3130331121152111211521119703edfd3b0264fd9c05baf8
fea5f8fd9100>/ZYCIBP+Arial-BoldMT AddT42Char 
1 3956 42 <00010062ffe705bd05d3002000d84046381e4b1e56077608760c8508840c
8517841b090617061b1217121b28112818281a281e08480b5b0454095a0b
6a047b047a18741ab60eb610c70dc610d710e7100e031c062000b8ffc040
1f1a391f00010025020101161c2d060912400e1234124b4f130113401518
3413b80128402a162d0f0300010120195f130113271256021f202003021a
2022302202221927a00a010f0a1f0a300a030ab8028cb3217e9f182b4e10
f45d714ded4e105df63c4dfd3c10f4ed711112392f3c003ffdf42b5de42b
3fed11392f3cfd712b3c1112393130005d015d5d01352111060423222402
3534123736332004170526262322061510123332363735033f027e5dfe9f
b5e6feaaacc0b98dd2011101332cfeda1fab80c2e5e8bc5dbb43021bf7fd
b85a89c10167d3e501645f49e5ca376c7df6f2fefbfefb4934ba>/ZYCIBP+Arial-BoldMT AddT42Char 

1 0 43 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 44 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 45 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 46 <> /ZYCIBP+Arial-BoldMT AddT42Char 
1 4282 47 <0001009d000004a505ae0005003d401a5007010201020403250500080405
1a0702032001200030000200b8028bb30631b9182b4e10f45d3c4dfd3c4e
10fe3c003f3c4dfd3c3f3c3130015d3311211121159d012802e005aefb49
f700>/ZYCIBP+Arial-BoldMT AddT42Char 

1 0 48 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 49 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 50 <> /ZYCIBP+Arial-BoldMT AddT42Char 
1 4374 51 <00020095000004f805ba000f001b007740250605b914b918034705016705
d605021211250d0e0e001b10250201020f00081627af070107b8ffc0b309
0b3407b8028c40161f1d301d601d701d801d051d100f2001200030000200
b8028bb31c3153182b4e10f45d3c4dfd3c4d1071f62b714ded003f3c3f3c
fd3c12392f3cfd3c3130005d71015d331121201716161514060607062323
1902333236363534262726239501db010e527eaa62974e6ac9c1a2af7643
5e4835a005ba1621ddaf87b8691115fdd704c2fe602e624150680d0a>/ZYCIBP+Arial-BoldMT AddT42Char 

1 0 52 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 53 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 54 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 55 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 56 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 57 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 58 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 59 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 60 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 61 <> /ZYCIBP+Arial-BoldMT AddT42Char 
1 4582 62 <00010092fe63028405ba000700504032063005400502053700033f044f04
020437011000120302060207040510070107f4059b000020013001d00103
016008677c182b10f65d3c10eded5d103c103c3c103c003f3ffd5d3c10fd
5d3c313013112115231133159201f2e7e7fe630757ddfa63dd00>/ZYCIBP+Arial-BoldMT AddT42Char 

1 0 63 <> /ZYCIBP+Arial-BoldMT AddT42Char 
1 4698 64 <00010026fe63021805ba00070044402a3f054f0502053700300440040204
3701120010070606021f030103f40105049b00df0101016009a376182b10
f65d3cfd3c10fd5d3c3c103c003f3fed5d10ed5d31300111213533112335
0218fe0ee7e705baf8a9dd059fdb>/ZYCIBP+Arial-BoldMT AddT42Char 

1 0 65 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 66 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 67 <> /ZYCIBP+Arial-BoldMT AddT42Char 
1 4802 68 <00020049ffe8042e043e0023003201714068071a081c051d161a4a1b481c
4925db10df11093619461957266619672686269219931aa61ab91bc71ac8
1b0c06060d151606191627062915591977028602a606b506c6060cbf34d9
10021d243231112c0d24402b2e3424402228342440191d346f24fc240224
461db8ffc040300e0f343d1d01001d101db01df91d041d1d2c013300400e
0f340f001f0002005521401c113f21401b103f2140181a3421b80274b504
070c0d0a2cb8ffc0b31c113f2cb8ffc0b31b103f2cb8ffc0b3181a342cb8
02744040140b1e3126082909280d591f0c9f0c021f0c01ff0c010c400e16
340c1a4f340134600001008e300101013329215f1701df17014f175f176f
17031719336941182b4e10f45d71724dedf471ed5d4e105df62b5d71724d
edf4e4fd3c003fed2b2b2b3f3c3ffd2b2b2bf45d2be412392f5d712bb106
02435458b22f1d017159edb10602435458b90024ffc0b71b1d3454246424
025d2b595d2b2b2b111239030e103c3c3c313001715d005d710127363633
321616150314161721262726270606232226353436363736373534262322
060106060706151416333237363736350165ff2bd2cfbcb84b031b25feea
0b10070348a45da4bd569b92c54c506f4b54015e36ea243758444c453310
0b02e22e9a945989b7feb88c854c1c3719084646b2885a8d4b1c25201c51
453bfed2123218273c3b563226372465>/ZYCIBP+Arial-BoldMT AddT42Char 
1 5328 69 <00020087ffe8049405ba000f001c009db90012fff840310b39371b471b02
125606560a56165618591cf7070635043b0d3b13351b45044b0d4b13451b
940799090a0c0e010201001ab80274b2050714b8027440130b0b0f000a17
21081a701e011e10290203260fb80129400c01700080000200191d3f4118
2b4e10f4713c4dedfd3ce64e1071f64ded003f3c3fed3fed3f3c31300071
5d015d4358400b6606660a66166618691c055d59005d2b33112111363332
1211100023222627151314171633323635342623220687011982b2c2fefe
fdb95bb140123449795d838467658605bafdf094fee7fef9fef0feda5b59
9c022aa54f709fabb6a19d00>/ZYCIBP+Arial-BoldMT AddT42Char 
1 5580 70 <00010055ffe8043f043e001900e14051580f59125916680f691269167d18
79199702970cc610c618d710d618e906e908e913e915f80613381338154a
124a164618590c690c073a1237163718037705770f8705860f8919a812a7
16b912b616090eb8ffc0b3181b340eb8ffc0b51214340e330db8ffc0b319
1e340db8ffc0b30f11340dba0104000a02744012110b0040181b34004012
1434003390010101ba0101000402744020170701401214340121002f0d40
1214340d214f0e010e1a1b072114191a5841182b4e10f44ded4e10f65d4d
ed2bf4ed2b003ffdf45de42b2b3ffdf42b2be42b2b3130005d7101715d01
052626232206151416333236370506062322001110003332160431feeb0e
634f697d7f6b50661501142bf4cde9feeb0116edc2e502ec32535491aabd
9c5b6f2fbec20126010401070125a700>/ZYCIBP+Arial-BoldMT AddT42Char 
1 5896 71 <00020054ffe8046105ba000f001c0090402d125906590a59125616561859
1c98079909f80909701e801e023a03340c3a1534194a03440c4a15441999
090914b80274b2050b1ab80274400e0b070e0f0001000a17290e0d2601b8
0129400f0f001a8f1e011e102108191d583c182b4e10f44ded4e1071f63c
4dedfd3ce6003f3c3f3c3fed3fed3130005d01715d4358400d6906690a69
1266166618691c065d592121350606232200111012333217112101141716
3332363534262322060461fefb41b15ab7fefbfec2b2820119fd122f447a
6188846764879c5b5901270108010e0119940210fc70aa4c6ea5a4b7a19f
>/ZYCIBP+Arial-BoldMT AddT42Char 
1 6136 72 <00020041ffe80427043e0014001c01a3b90010fff840460b3999099a0d96
10a805a70abb09bb0db81a0808140148024706460a4f1ea80db606b61ac7
0ac80cd60ad80cf807f70d0d1c0f1c15401b1d3415400e11340f15bf15cf
150315b8ffc0b30f1e3f15b8ffc0b30e173f15b8028d400c0f0e12500e60
0e020e181201b8ffc0b6191b3401331200b8ffc0b31d203400b8ffc0b322
293400b8ffc0b32b2d3400b8ffc0b3181c3400b8ffc0400f0e0f34a00001
0000100002005f1212b80274b3040b1218b8027440240b070021012f1521
4f0e010e1a2f1e5f1e6f1e9f1e041e0f2108400d0f3408191d6941182b4e
10f42b4ded4e105df65d4dedf4ed003fed435c584014184028143f18401e
0f3f18401b103f18401c113f2b2b2b2b593ffd435c58b90012ffc0b32814
3f12b8ffc0b31e0f3f12b8ffc0b31b103f12b8ffc0b21c113f2b2b2b2b59
f45d712b2b2b2b2b435c58b90000ffc0b2123900b8ffc0b2173900b8ffb0
b3090a3e00b8ffc0b241213f2b002b2b2b59e42b1112395d435c5840140e
400f1e3f0e401c113f0e401b103f0e400e173f002b2b2b2b592f3cfd2b2b
722b2b3c0111333130015d71005d2b010506062320272635100033320003
211616333236132626232207061702fa011836e9affeeb85690114d3ed01
1206fd40038261425a270378565c3c3c0101522f9aa1b591dd0108012bfe
c7febd7d8b48016c7a7f43437300>/ZYCIBP+Arial-BoldMT AddT42Char 
1 6660 73 <00010018000002e605d3001600b840323604012a04201020115904801805
0804bf180215161102141216110e130f00100e13010010021409080f0b01
5f0bff0b020bb80274400a0601110f1601ff160116b80274401e10000001
f00001000613140a09333f084f085008030828102f115f110211b8010440
0d0e132602145f00a016c0160216b8ffc0b6090c3416191778b902690018
2b4e10f42b713c4dfc3cfd3cfc5d3cf45d19e400183f3c3f5d713cfd5d71
3c3ffd5d7139320f0f0f0f313001715d005d133335343636333217072623
2206151533152311211123189c399975787326433e3d35d2d2fee79c0426
5086845324c41039514bddfcb7034900>/ZYCIBP+Arial-BoldMT AddT42Char 
1 6916 74 <00020054fe510460043e0023002f014e4062771d871d02120c0d7031860d
8031042001230223033001330233034001430243035b0f59145925562956
2b592f6b0ff811f813123b0d33163b28332c4b0d44164b28442cf00cfd17
0a8e0c010c0b0c0d0b2a0c0d270e1617152d0d0c171604182401b8ffc0b5
191b34013300b8ffc0b30e113e00b8ffc0b30b0c3e00b8ffc0b3282a3400
b8ffc0b323253400b8ffc0b331343400b8ffc04009151b34600001005f05
b80274b21f0f27b80274b20e0a2db80274400b15071819062a290b261a18
b80129400919191a1a8f31013101b801b8400a00332421121930583c182b
4e10f44dedf4ed4e1071f63c4d10ed10fde4003f3c3fed3fed3ffdf4722b
2b2b2b2b2bb10602435458b90000ffc0b30e113400b8ffc0b2090c342b2b
59e42b01111217390011123939111239390708103c313000715d015d7143
58400d690f691469256729662b692f065d59005d17051617163332373637
3635350623222726351000333217352111140e0223202635341314163332
36353426232206790141081d28566e3725130d7ec0d67d620101bfc58001
073e70bb8ffef2e2fc8360678e88686583462738151e211631235e9bacb5
8fd5010b011aad95fc47bcba6a3cb98e0e0283a99da19ea5a09d>/ZYCIBP+Arial-BoldMT AddT42Char 
1 7392 75 <000100920000045905ba001600b2402b0f011f0139013302331042014211
de01f9010907051605240258116811050101021314111213031402010fb8
0274401d0307090a0a14150a1600000b0a26080940202434af0901ff0901
091a18b8ffc040162224349018a018027018f01802ef1801180014261615
b8ffc0400f202434a01501f015011519173f3c182b4e10f471722b3c4dfd
3c4e105d71722bf671722b3c4dfd3c003f3c3f3c3c103c3fed3939111739
030e103c083c3130015d005d01113633321e021511211134262623220606
1511211101ab88bd619c4f1dfee720513d466e33fee705bafde59f487088
8ffd910231a75a35448986fdec05ba00>/ZYCIBP+Arial-BoldMT AddT42Char 
1 7648 76 <00020093000001ac05ba000300070077b90009ffc0403f110a3f40095009
028009b009c009d009ef09051f0960097f09a009b0090503060700050403
0f00014000d000e00003005d02010006050607040a0207260104b8ffc040
092124340419083f3c182b4e10f42b3c4dfd3c003f3c3f3c3f3cfd5d713c
0305103c3c103c3c313001715d722b1311211101112111930119fee70119
04b60104fefcfb4a0426fbda>/ZYCIBP+Arial-BoldMT AddT42Char 

1 0 77 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 78 <> /ZYCIBP+Arial-BoldMT AddT42Char 
1 7810 79 <00010093000001ac05ba00030053b90005ffc04029110a3f400550050280
05b005c005d005ef05051f0560057f05a005b0050502010003000a020326
0100b8ffc040092124340019043f3c182b4e10f42b3c4dfd3c003f3c3f3c
313001715d722b3311211193011905bafa46>/ZYCIBP+Arial-BoldMT AddT42Char 
1 7918 80 <0001007e00000698043e0027013bb90029ffc0405d110a3f0506060c1506
160c340334083418342344024508451844230c20032f295309602980299f
29a406a707a60cb506b50cb029d029e0290e00292f2950299f29bf29df29
0629401a1c343f2950298029d029e02905072104071a1d16b80274b20a07
21b80274401e0407101111271b1c1c26270a0100060f10261211405a3560
11016f110111b80246400f1a1b261d1c405a356f1c01601c011cb80246b4
2526262701b80129b2000027b8ffc0b30f093f27b8ffc04036110a3f2740
5a352740413527403c35274024273427403a3d342f27cf27df27030f271f
27802703002720273027ff2704271928e33c182b4e10f45d71722b2b2b2b
2b2b2b3c4d10ed10fd3cf65d712b3cfd3cf6715d2b3cfd3c003f3c3f3c3c
103c103c103c3fed3fed0111123900111239313001722b715d005d012b13
211536333216173636333216171615112111342726232206061511211134
2626232206061511217e01038bc066963046a25c75a2281dfee71d27513b
682efee71e3f3641682dfee7042691a9545555545f5c4498fd59025f9e2e
3c488b96fe0202469b5a2c468499fdfc>/ZYCIBP+Arial-BoldMT AddT42Char 
1 8354 81 <0001009100000459043e0016009f4018071317135a08680804b804013408
34104408440fe9100506b80274401d11070e0d060c0b0b01000a02012616
0040202434af0001ff0001001a18b8ffc040162224349018a018027018f0
1802ef1801180a0b260c0eb80129b20d0d0cb8ffc0400f202434a00c01f0
0c010c19173f3c182b4e10f471722b3c4d10ed10fd3c4e105d71722bf671
722b3c4dfd3c003f3c3c103c3f3c3fed3130005d01715d21211134262623
2206061511211121153633321e02150459fee724513949742bfee701058b
d35d9a4f1f021eac65385084b2fe1f04269cb44368847b00>/ZYCIBP+Arial-BoldMT AddT42Char 
1 8588 82 <00020052ffe8049a043e000d001900974048e801e708f713f71504c702e8
05021219051909025910561356165918970298069808970cb809d502db05
dc09d50ce705e706e80d10a708cb02cc06c308c60c057508890684080311
b80274b20a0b17b80274401404071439071a601b701b021b0e2100191a58
41182b4e10f44ded4e1071f64ded003fed3fed313000715d015d71435840
09691066126616691804015d59005d015d13341236333200151400232224
26251416333236353426232206528afd9cf10134fec9ec92fef78a012096
6e6e95956e6e9602228c01068afec7eff1fec384ffa89ea8a8a09ca8a800
>/ZYCIBP+Arial-BoldMT AddT42Char 

1 0 83 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 84 <> /ZYCIBP+Arial-BoldMT AddT42Char 
1 8828 85 <0001008700000337043e001000a84028970501090e01530566057505032f
12580e680e7012040a090f0c1f0c028f0cff0c023f0c4f0c020cb8027740
29070701000a0302060a28000910093009700904091a7f129f12025f127f
12af12d01204121000260103b80129400b02028001a001020119113fb901
1c00182b4e10f4713c4d10ed10fd3c4e105d71f65d194de400183f3c3f3c
3fed5d717239323130015d005d71004bb017534bb035515a58b10a323859
005d212111211536363332170726232206061101a0fee70105436b446059
57473d3b522f0426976b4435f52e41aafef1>/ZYCIBP+Arial-BoldMT AddT42Char 
1 9056 86 <00010030ffe80410043e002a02c240c00611062308271711172398129814
9727952a09071446140212bb0db90ec721e523f80df62206290d550d650d
950b9712a722b90c07412340244426672264268712871486228324093726
4506460b4a0d4f0f462142220722242726370c352135223523352407060a
05110921180d270c22222223072422402c730c781479157629752a881584
2a9a15952ab422b4230d80018f178c18992aa92ab02c0617211640212334
16401c1f341f1601df16011633082150258f25022540181d34251a2cb8ff
c04017110a3f502c01302c012f2c012c1e213010011033012100b8ffc0b3
0f093f00b8ffc0b3110a3f00b8ffc04009090d3400192b78b8182b4e10fc
2b2b2b4dedf471ed4e105d71722bf62b714dedf471722b2bed00b1060243
54584035060101060116012622362146215401591764016917f6010a0117
02041a21220228130d0c02281a5f04010446280b501a011a4613073ffd5d
3ffd5d1112173911121739111217395d711bb90022ffcbb3282a3421b8ff
cbb3282a3422b8ffe0b31e243421b8ffe0b31f243422b8ffe0b3191a3421
b8ffe0401b191a346b0d0136224622980d9422c422d4220621220c0d0404
1a00b8ffc0b5191b34003301b8ffc0b3172d3f01b8ffb0b3090a3e01b8ff
c0b322253401b8ffc0401d1a1c3400013001400150010460018001f00103
00011001500160010401b8ffc0b313163401b80101404d0004015f04f004
020446280b1640191b3416331740172d3f1740090a3e174035373417402b
2e34174025293417401a1c340f171f175f176f170417551a402224340f1a
01501aff1a021a4613073ffd5d712bf45d2b2b2b2b2b2be42b3ffd5d71f4
2b5d71722b2b2b2be42b111217395d712b2b2b2b2b2b59313001715d0071
7171715d5d435c58b90024ffc940090b123f0f280b123f21b8ffecb60d39
0c140c3921b8ffecb20c3922b8ffeab10b39002b2b2b2b012b2b5900715d
132516163332373635342726272427263534363332161705262623220706
1514171604171615140623222630011a126e636d3725141549feac5b7eda
e5dad428fef7115f586f30201c2601c15958f4efd9fd012f2b5255281c2f
201514114b3e56998abc8e8b313e421f16231e151c664a4b8692d2b0>/ZYCIBP+Arial-BoldMT AddT42Char 
1 9894 87 <0001001fffe80291059d001900cd402920002001230a290f3a0e4a0e590f
07191500180316150017121314011712021401180309070a070c18b80101
400f0017a017b017036017a017c0170317b80104b2150114b80274b30015
0607b80274400e0c0b092f0a2f00002f015f010201b80104402818032617
1255153f149f14af1403601480149014d014f01405001410142014301404
14191a78a0182b4e10f45d71724bb037534bb03b515a58b90014ffc03859
3c4dfc3cfd3cf45d3c10f419e400183fed3f3cfd3c10f45d71e411123911
330f0f0f0f3130015d011523111416163332371706232226262726351123
3533352511027ac00b271c274a18627c4c7a390b098181011a0426e0fe54
822b1c1bda2a335145319501cfe0d3a4fe89>/ZYCIBP+Arial-BoldMT AddT42Char 
1 10182 88 <0001008dffe8045304260016009c401757116711960503090619063c023c
114b024b11e702070fb802744011040b16000a1514140a09061314261515
00b80129400e1640202434af1601ff1601161a18b8ffc040162224349018
a018027018f01802ef1801180a0b260908b8ffc0400f202434a00801f008
010819173f3c182b4e10f471722b3c4dfd3c4e105d71722bf671722b4ded
3c10fd3c003f3c3c103c3f3c3fed3130005d015d21350606232226263511
21111416163332363635112111034e3abd696baa4c01191f523f48722a01
199f55625eaa9602a0fe18e0653b4f75e401c0fbda00>/ZYCIBP+Arial-BoldMT AddT42Char 

1 0 89 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 90 <> /ZYCIBP+Arial-BoldMT AddT42Char 
1 10414 91 <0001000c000004600426000b0198408b2807c804029807b901dc01d507f0
0d0508071a041806280637003808480159017c0175070a26012b0736013a
0746014a07980bf806f80709250426072a0a34043a0a43044e0ac304084c
0a5404590a64046d0a78017d0a94049607ba0ad504dc0afc0a0d03040707
090a160420042a0a33043f0a4604091504190a3a0a4e0a6b0aa704b704c9
0af6040907b8fff0b312183404b8ffd8b315173404b8ffe040150c113401
040a0704000201040a0704080009080303b8ffe0b6292d34ff030103b8ff
e0400f162434032602091402020905060b0bb8ffe0b6292d34f00b010bb8
ffe040171624340b260005140000050605050302060809090b0005b8026d
b2063309b8026d400b08654f0d9f0de00d030d03b8026db202330bb8026d
4012f0000100001000200030000400650cc4a0182b194e10f45d71184ded
f4ed194d105df6184dedf4ed002f3c3c103c3f3c3c103c87052e2b2b712b
877dc4872e182b2b712b877dc401111217390011121739b10602435458b5
0a2009213404b8ffe0b2092134002b2b593130002b2b2b5d717172015d71
71723301012113132101012103030c017ffe910157bcc6014afe980189fe
a7d8da02230203fedc0124fe09fdd10149feb700>/ZYCIBP+Arial-BoldMT AddT42Char 
1 10884 92 <0001000efe510452042600130134b41228050113b8ffe040180c0f340816
0d0f3407160d0f3406160d0f3405160c0f3402b8ffc0401f1a3a34050606
040d0b0e061002001306041302040303010100061360100110b801af4012
0b0f0d2f0e280020153015601503f0150115b8ffc0b322263415b8ffc040
121c1e341517171a043903401819347f030103b80127400902401819347f
020102b801274012013900401c36342000300002001914c4a0182b4e10f4
5d2b4dfd19f45d2bf45d2b18fd4e456544e62b2b71724d10f4e4003fed5d
2f3f3c103c103c0112391139001112391239391139070e103c3130002b01
2b2b2b2b2b5d4bb010534bb03a515a58b2041000bafff00001fff0b10310
013838383859435c58b90005ffe8400e0d113f131013193f131012183f05
b8fff0b313193f05b8fff0b212183f012b2b2b2b2b59132113132101070e
032322272716333236370e012bfef80123fe89432543577f50514e194235
625e190426fd0e02f2fc02b95d623d2211dc0d735900>/ZYCIBP+Arial-BoldMT AddT42Char 

1 0 93 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 94 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 95 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 96 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 97 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 135 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 188 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 195 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 166 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 196 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 171 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 130 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 193 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 214 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 197 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 226 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 189 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 175 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 228 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 181 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 182 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 179 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 180 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 177 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 178 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 215 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 140 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 227 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 190 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 176 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 229 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 186 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 163 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 132 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 133 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 862 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 150 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 230 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 134 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 142 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 139 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 157 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 169 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 164 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 138 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 256 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 131 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 147 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 240 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 241 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 141 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 151 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 136 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 194 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 220 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 239 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 158 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 170 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 243 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 242 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 244 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 162 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 172 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 200 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 198 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 173 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 98 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 99 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 144 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 100 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 202 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 101 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 199 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 201 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 206 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 203 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 204 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 205 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 231 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 102 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 209 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 207 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 208 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 174 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 103 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 238 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 145 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 212 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 210 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 211 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 104 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 233 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 235 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 137 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 106 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 105 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 107 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 109 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 108 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 110 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 160 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 111 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 113 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 112 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 114 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 115 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 117 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 116 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 118 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 119 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 232 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 120 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 122 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 121 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 123 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 125 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 124 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 183 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 161 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 127 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 126 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 128 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 129 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 234 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 236 <> /ZYCIBP+Arial-BoldMT AddT42Char 

1 0 185 <> /ZYCIBP+Arial-BoldMT AddT42Char 
/ZYCIBP+Arial-BoldMT findfont /CharStrings get begin
/.notdef 0 def
/dotlessi 213 def
/caron 223 def
/space 3 def
/exclam 4 def
/quotedbl 5 def
/numbersign 6 def
/dollar 7 def
/percent 8 def
/ampersand 9 def
/quotesingle 10 def
/parenleft 11 def
/parenright 12 def
/asterisk 13 def
/plus 14 def
/comma 15 def
/hyphen 16 def
/period 17 def
/slash 18 def
/zero 19 def
/one 20 def
/two 21 def
/three 22 def
/four 23 def
/five 24 def
/six 25 def
/seven 26 def
/eight 27 def
/nine 28 def
/colon 29 def
/semicolon 30 def
/less 31 def
/equal 32 def
/greater 33 def
/question 34 def
/at 35 def
/A 36 def
/B 37 def
/C 38 def
/D 39 def
/E 40 def
/F 41 def
/G 42 def
/H 43 def
/I 44 def
/J 45 def
/K 46 def
/L 47 def
/M 48 def
/N 49 def
/O 50 def
/P 51 def
/Q 52 def
/R 53 def
/S 54 def
/T 55 def
/U 56 def
/V 57 def
/W 58 def
/X 59 def
/Y 60 def
/Z 61 def
/bracketleft 62 def
/backslash 63 def
/bracketright 64 def
/asciicircum 65 def
/underscore 66 def
/grave 67 def
/a 68 def
/b 69 def
/c 70 def
/d 71 def
/e 72 def
/f 73 def
/g 74 def
/h 75 def
/i 76 def
/j 77 def
/k 78 def
/l 79 def
/m 80 def
/n 81 def
/o 82 def
/p 83 def
/q 84 def
/r 85 def
/s 86 def
/t 87 def
/u 88 def
/v 89 def
/w 90 def
/x 91 def
/y 92 def
/z 93 def
/braceleft 94 def
/bar 95 def
/braceright 96 def
/asciitilde 97 def
/bullet 135 def
/Euro 188 def
/quotesinglbase 195 def
/florin 166 def
/quotedblbase 196 def
/ellipsis 171 def
/dagger 130 def
/daggerdbl 193 def
/circumflex 214 def
/perthousand 197 def
/Scaron 226 def
/guilsinglleft 189 def
/OE 175 def
/Zcaron 228 def
/quoteleft 181 def
/quoteright 182 def
/quotedblleft 179 def
/quotedblright 180 def
/endash 177 def
/emdash 178 def
/tilde 215 def
/trademark 140 def
/scaron 227 def
/guilsinglright 190 def
/oe 176 def
/zcaron 229 def
/Ydieresis 186 def
/exclamdown 163 def
/cent 132 def
/sterling 133 def
/currency 862 def
/yen 150 def
/brokenbar 230 def
/section 134 def
/dieresis 142 def
/copyright 139 def
/ordfeminine 157 def
/guillemotleft 169 def
/logicalnot 164 def
/registered 138 def
/macron 256 def
/degree 131 def
/plusminus 147 def
/twosuperior 240 def
/threesuperior 241 def
/acute 141 def
/mu 151 def
/paragraph 136 def
/periodcentered 194 def
/cedilla 220 def
/onesuperior 239 def
/ordmasculine 158 def
/guillemotright 170 def
/onequarter 243 def
/onehalf 242 def
/threequarters 244 def
/questiondown 162 def
/Agrave 172 def
/Aacute 200 def
/Acircumflex 198 def
/Atilde 173 def
/Adieresis 98 def
/Aring 99 def
/AE 144 def
/Ccedilla 100 def
/Egrave 202 def
/Eacute 101 def
/Ecircumflex 199 def
/Edieresis 201 def
/Igrave 206 def
/Iacute 203 def
/Icircumflex 204 def
/Idieresis 205 def
/Eth 231 def
/Ntilde 102 def
/Ograve 209 def
/Oacute 207 def
/Ocircumflex 208 def
/Otilde 174 def
/Odieresis 103 def
/multiply 238 def
/Oslash 145 def
/Ugrave 212 def
/Uacute 210 def
/Ucircumflex 211 def
/Udieresis 104 def
/Yacute 233 def
/Thorn 235 def
/germandbls 137 def
/agrave 106 def
/aacute 105 def
/acircumflex 107 def
/atilde 109 def
/adieresis 108 def
/aring 110 def
/ae 160 def
/ccedilla 111 def
/egrave 113 def
/eacute 112 def
/ecircumflex 114 def
/edieresis 115 def
/igrave 117 def
/iacute 116 def
/icircumflex 118 def
/idieresis 119 def
/eth 232 def
/ntilde 120 def
/ograve 122 def
/oacute 121 def
/ocircumflex 123 def
/otilde 125 def
/odieresis 124 def
/divide 183 def
/oslash 161 def
/ugrave 127 def
/uacute 126 def
/ucircumflex 128 def
/udieresis 129 def
/yacute 234 def
/thorn 236 def
/ydieresis 185 def
end
/ZYCIBP+Arial-BoldMT findfont /Encoding get
dup 0 /.notdef put
dup 1 /dotlessi put
dup 2 /caron put
dup 32 /space put
dup 33 /exclam put
dup 34 /quotedbl put
dup 35 /numbersign put
dup 36 /dollar put
dup 37 /percent put
dup 38 /ampersand put
dup 39 /quotesingle put
dup 40 /parenleft put
dup 41 /parenright put
dup 42 /asterisk put
dup 43 /plus put
dup 44 /comma put
dup 45 /hyphen put
dup 46 /period put
dup 47 /slash put
dup 48 /zero put
dup 49 /one put
dup 50 /two put
dup 51 /three put
dup 52 /four put
dup 53 /five put
dup 54 /six put
dup 55 /seven put
dup 56 /eight put
dup 57 /nine put
dup 58 /colon put
dup 59 /semicolon put
dup 60 /less put
dup 61 /equal put
dup 62 /greater put
dup 63 /question put
dup 64 /at put
dup 65 /A put
dup 66 /B put
dup 67 /C put
dup 68 /D put
dup 69 /E put
dup 70 /F put
dup 71 /G put
dup 72 /H put
dup 73 /I put
dup 74 /J put
dup 75 /K put
dup 76 /L put
dup 77 /M put
dup 78 /N put
dup 79 /O put
dup 80 /P put
dup 81 /Q put
dup 82 /R put
dup 83 /S put
dup 84 /T put
dup 85 /U put
dup 86 /V put
dup 87 /W put
dup 88 /X put
dup 89 /Y put
dup 90 /Z put
dup 91 /bracketleft put
dup 92 /backslash put
dup 93 /bracketright put
dup 94 /asciicircum put
dup 95 /underscore put
dup 96 /grave put
dup 97 /a put
dup 98 /b put
dup 99 /c put
dup 100 /d put
dup 101 /e put
dup 102 /f put
dup 103 /g put
dup 104 /h put
dup 105 /i put
dup 106 /j put
dup 107 /k put
dup 108 /l put
dup 109 /m put
dup 110 /n put
dup 111 /o put
dup 112 /p put
dup 113 /q put
dup 114 /r put
dup 115 /s put
dup 116 /t put
dup 117 /u put
dup 118 /v put
dup 119 /w put
dup 120 /x put
dup 121 /y put
dup 122 /z put
dup 123 /braceleft put
dup 124 /bar put
dup 125 /braceright put
dup 126 /asciitilde put
dup 127 /bullet put
dup 128 /Euro put
dup 129 /bullet put
dup 130 /quotesinglbase put
dup 131 /florin put
dup 132 /quotedblbase put
dup 133 /ellipsis put
dup 134 /dagger put
dup 135 /daggerdbl put
dup 136 /circumflex put
dup 137 /perthousand put
dup 138 /Scaron put
dup 139 /guilsinglleft put
dup 140 /OE put
dup 141 /bullet put
dup 142 /Zcaron put
dup 143 /bullet put
dup 144 /bullet put
dup 145 /quoteleft put
dup 146 /quoteright put
dup 147 /quotedblleft put
dup 148 /quotedblright put
dup 149 /bullet put
dup 150 /endash put
dup 151 /emdash put
dup 152 /tilde put
dup 153 /trademark put
dup 154 /scaron put
dup 155 /guilsinglright put
dup 156 /oe put
dup 157 /bullet put
dup 158 /zcaron put
dup 159 /Ydieresis put
dup 160 /space put
dup 161 /exclamdown put
dup 162 /cent put
dup 163 /sterling put
dup 164 /currency put
dup 165 /yen put
dup 166 /brokenbar put
dup 167 /section put
dup 168 /dieresis put
dup 169 /copyright put
dup 170 /ordfeminine put
dup 171 /guillemotleft put
dup 172 /logicalnot put
dup 173 /hyphen put
dup 174 /registered put
dup 175 /macron put
dup 176 /degree put
dup 177 /plusminus put
dup 178 /twosuperior put
dup 179 /threesuperior put
dup 180 /acute put
dup 181 /mu put
dup 182 /paragraph put
dup 183 /periodcentered put
dup 184 /cedilla put
dup 185 /onesuperior put
dup 186 /ordmasculine put
dup 187 /guillemotright put
dup 188 /onequarter put
dup 189 /onehalf put
dup 190 /threequarters put
dup 191 /questiondown put
dup 192 /Agrave put
dup 193 /Aacute put
dup 194 /Acircumflex put
dup 195 /Atilde put
dup 196 /Adieresis put
dup 197 /Aring put
dup 198 /AE put
dup 199 /Ccedilla put
dup 200 /Egrave put
dup 201 /Eacute put
dup 202 /Ecircumflex put
dup 203 /Edieresis put
dup 204 /Igrave put
dup 205 /Iacute put
dup 206 /Icircumflex put
dup 207 /Idieresis put
dup 208 /Eth put
dup 209 /Ntilde put
dup 210 /Ograve put
dup 211 /Oacute put
dup 212 /Ocircumflex put
dup 213 /Otilde put
dup 214 /Odieresis put
dup 215 /multiply put
dup 216 /Oslash put
dup 217 /Ugrave put
dup 218 /Uacute put
dup 219 /Ucircumflex put
dup 220 /Udieresis put
dup 221 /Yacute put
dup 222 /Thorn put
dup 223 /germandbls put
dup 224 /agrave put
dup 225 /aacute put
dup 226 /acircumflex put
dup 227 /atilde put
dup 228 /adieresis put
dup 229 /aring put
dup 230 /ae put
dup 231 /ccedilla put
dup 232 /egrave put
dup 233 /eacute put
dup 234 /ecircumflex put
dup 235 /edieresis put
dup 236 /igrave put
dup 237 /iacute put
dup 238 /icircumflex put
dup 239 /idieresis put
dup 240 /eth put
dup 241 /ntilde put
dup 242 /ograve put
dup 243 /oacute put
dup 244 /ocircumflex put
dup 245 /otilde put
dup 246 /odieresis put
dup 247 /divide put
dup 248 /oslash put
dup 249 /ugrave put
dup 250 /uacute put
dup 251 /ucircumflex put
dup 252 /udieresis put
dup 253 /yacute put
dup 254 /thorn put
dup 255 /ydieresis put
pop
end

userdict /pdf_svglb get setglobal
[/N160/ZYCIBP+Arial-BoldMT 1 TZG
0 0 595.276 841.89 re
W
n
q
q
n
0 841.89 595.276 -841.89 re
W
n
true setSA
[/DeviceCMYK] cs 0 0 0 1 sc
79.0894 797.155 m
/N160 12 Tf
(\(a\)) show
78.7314 713.373 m
(\(b\)) show
2 w
4 M
0 j
0 J
[] 0 d
n
263.185 643.354 m
262.673 643.249 262.501 643.324 262.265 642.859 c
261.835 642.013 261.9 641.928 261.978 640.981 c
262.021 640.469 262.109 640.433 262.496 640.092 c
263.091 639.564 263.105 639.106 263.876 639.301 c
264.625 639.489 264.525 639.874 264.652 640.636 c
264.771 641.359 264.593 641.382 264.335 642.068 c
264.113 642.657 264.046 642.63 263.703 643.156 c
263.544 643.397 263.457 643.41 263.185 643.354 c
h
S
n
263.185 642.662 m
262.673 642.557 262.501 642.633 262.265 642.168 c
261.835 641.321 261.9 641.236 261.978 640.289 c
262.021 639.776 262.109 639.74 262.496 639.399 c
263.091 638.872 263.105 638.415 263.876 638.609 c
264.625 638.798 264.525 639.183 264.652 639.943 c
264.771 640.668 264.593 640.69 264.335 641.377 c
264.113 641.966 264.046 641.938 263.703 642.465 c
263.544 642.706 263.457 642.718 263.185 642.662 c
h
S
n
262.812 643.305 m
262.3 643.199 262.128 643.276 261.892 642.811 c
261.46 641.964 261.525 641.879 261.605 640.932 c
261.648 640.419 261.738 640.384 262.123 640.043 c
262.716 639.516 262.73 639.058 263.501 639.252 c
264.25 639.44 264.15 639.824 264.277 640.586 c
264.398 641.31 264.22 641.332 263.96 642.02 c
263.74 642.608 263.673 642.581 263.33 643.107 c
263.171 643.349 263.083 643.36 262.812 643.305 c
h
S
n
263.445 643.107 m
262.933 643.002 262.761 643.079 262.525 642.613 c
262.093 641.767 262.16 641.682 262.238 640.734 c
262.279 640.222 262.369 640.186 262.753 639.845 c
263.349 639.317 263.363 638.859 264.134 639.054 c
264.882 639.242 264.783 639.627 264.91 640.389 c
265.029 641.112 264.853 641.136 264.593 641.822 c
264.373 642.411 264.306 642.383 263.96 642.909 c
263.802 643.15 263.714 643.163 263.445 643.107 c
h
S
n
262.898 642.859 m
262.386 642.754 262.214 642.831 261.978 642.365 c
261.546 641.519 261.613 641.434 261.691 640.486 c
261.734 639.975 261.824 639.938 262.208 639.598 c
262.804 639.07 262.816 638.612 263.587 638.807 c
264.335 638.995 264.236 639.38 264.363 640.141 c
264.484 640.864 264.306 640.888 264.048 641.574 c
263.826 642.163 263.759 642.136 263.416 642.662 c
263.257 642.902 263.169 642.915 262.898 642.859 c
h
S
n
262.726 642.563 m
262.214 642.458 262.042 642.534 261.806 642.068 c
261.375 641.222 261.439 641.137 261.519 640.19 c
261.562 639.678 261.652 639.643 262.037 639.301 c
262.63 638.773 262.644 638.315 263.416 638.51 c
264.164 638.698 264.064 639.083 264.191 639.845 c
264.312 640.568 264.134 640.591 263.876 641.277 c
263.654 641.866 263.587 641.839 263.244 642.365 c
263.085 642.606 262.998 642.619 262.726 642.563 c
h
S
n
263.244 643.453 m
262.732 643.348 262.56 643.425 262.322 642.959 c
261.892 642.112 261.957 642.027 262.037 641.08 c
262.08 640.567 262.167 640.531 262.552 640.19 c
263.148 639.663 263.162 639.205 263.933 639.399 c
264.681 639.588 264.582 639.973 264.708 640.734 c
264.828 641.459 264.65 641.48 264.392 642.168 c
264.169 642.757 264.105 642.729 263.759 643.256 c
263.603 643.497 263.513 643.509 263.244 643.453 c
h
S
n
263.156 642.613 m
262.646 642.508 262.474 642.583 262.238 642.118 c
261.806 641.271 261.871 641.187 261.949 640.24 c
261.992 639.727 262.082 639.691 262.466 639.35 c
263.062 638.822 263.076 638.363 263.845 638.559 c
264.595 638.748 264.496 639.133 264.623 639.895 c
264.742 640.619 264.564 640.642 264.306 641.328 c
264.083 641.916 264.017 641.889 263.673 642.414 c
263.515 642.655 263.427 642.669 263.156 642.613 c
h
S
n
262.869 642.811 m
262.357 642.705 262.185 642.781 261.949 642.316 c
261.519 641.47 261.582 641.385 261.662 640.438 c
261.705 639.925 261.794 639.89 262.179 639.549 c
262.775 639.021 262.789 638.563 263.56 638.758 c
264.308 638.946 264.208 639.331 264.335 640.092 c
264.455 640.816 264.277 640.838 264.019 641.525 c
263.796 642.114 263.732 642.087 263.386 642.613 c
263.228 642.854 263.14 642.866 262.869 642.811 c
h
S
1 w
[2 ] 0 d
n
269.251 641.021 m
269.251 637.71 266.361 635.025 262.792 635.025 c
259.226 635.025 256.335 637.71 256.335 641.021 c
256.335 644.332 259.226 647.016 262.792 647.016 c
266.361 647.016 269.251 644.332 269.251 641.021 c
h
S
2 w
1 j
1 J
[] 0 d
n
256.335 632.449 m
256.335 618.734 l
S
n
270.107 631.963 m
270.107 618.25 l
S
1 w
0 j
0 J
n
281.027 625.725 m
300.629 625.725 l
S
n
283.009 628.594 m
272.167 625.689 l
283.009 622.784 l
h
f
n
245.927 625.456 m
226.326 625.456 l
S
n
243.945 622.587 m
254.787 625.491 l
243.945 628.396 l
h
f
2 w
1 J
n
164.173 644.158 m
161.466 643.475 159.475 645.489 158.76 642.791 c
158.092 640.273 165.218 641.168 163.013 639.781 c
158.231 636.773 154.36 643.447 151.799 638.412 c
149.651 634.19 157.433 637.187 159.533 632.941 c
160.648 630.688 156.444 634.542 154.506 632.941 c
153.227 631.886 158.623 631.898 157.213 631.025 c
154.747 629.498 149.396 633.11 151.412 631.025 c
155.587 626.708 160.147 631.455 162.24 625.826 c
163.791 621.658 157.674 624.805 153.346 625.826 c
150.694 626.451 151.583 628.51 148.898 628.973 c
147.265 629.254 147.805 626.678 146.192 627.059 c
142.965 627.82 144.036 631.507 140.778 630.889 c
137.881 630.338 140.673 627.256 138.266 625.553 c
137.009 624.663 137.216 627.81 135.752 627.332 c
134.516 626.929 135.752 626.032 135.752 624.732 c
S
1 w
0 J
[2 ] 0 d
n
160.32 647.166 m
152.955 644.86 157.198 644.022 152.955 642.553 c
149.807 641.463 148.865 644.669 146.291 642.553 c
144.175 640.813 146.291 639.813 146.291 637.074 c
146.291 635.057 148.196 633.702 146.291 633.038 c
140.827 631.133 140.362 634.313 134.718 633.038 c
131.949 632.412 131.492 632.023 130.333 629.432 c
129.067 626.602 128.351 625.615 130.333 623.232 c
132.613 620.492 133.648 621.756 137.172 621.215 c
140.292 620.736 140.449 620.353 143.485 621.215 c
145.56 621.804 144.663 624.072 146.816 623.954 c
153.288 623.6 152.807 619.85 159.269 620.351 c
163.229 620.658 164.485 621.532 165.405 625.396 c
166.417 629.648 161.69 629.306 162.425 633.614 c
163.192 638.117 165.271 637.187 168.036 640.823 c
169.656 642.955 171.603 642.503 171.193 645.148 c
170.759 647.953 169.46 647.74 166.809 648.752 c
163.688 649.942 163.535 648.069 160.32 647.166 c
h
S
2 w
1 j
1 J
[] 0 d
n
132.992 612.713 m
148.85 596.855 l
S
n
173.961 640.914 m
189.818 625.057 l
S
1 w
0 j
0 J
n
151.554 608.062 m
169.055 620.314 l
S
n
151.531 611.548 m
144.316 602.951 l
154.863 606.789 l
h
f
n
176.33 625.408 m
158.829 613.155 l
S
n
176.353 621.922 m
183.567 630.519 l
173.021 626.681 l
h
f
138.35 568.828 m
/N160 [9.8298 6.883 -6.883 9.8298 0 0] Tf
(long-axis length) show
227.336 603.283 m
/N160 12 Tf
(long-axis length) show
q
n
111.74 652.254 98 70 re
W
n
q
98 0 0 70 111.74 652.254 cm
q
n
0 0 1 1 re
q
W
[/Indexed [/DeviceCMYK] 159
<~mGR$Kh9s]YgsXTVgX4BRgX+9Ng<e-Kg!@pFg!7gBfZhU=fZ_L9f?D@6f#u.1f#l%-
e]Pn)e]Gh&eB#V!e&]Ire&T@nd`94jd`0.fdDj"bd)Ee]d)<\Ycc!PUcbmJRcGI8M
cG@/Hc,%#DbeUi@beL`<bJ(N7bJ(K4bItE0b.Y9,b.P0(b.P-%ah+s!ah"iqaLSWl
a18Kha1/Ee`j`3``j`0]`O;sW`O2mT`3laP`3cXL_mHOH_m?FD_R$:@_Qp1<_6L"7
^p0k3^p'b/^TXS+^TOJ&^94>"^9+4s]r\%o]r\"l]W7eg]W._d];hS`];_J\\u;8W
\u22T\YbuO\YYlK\>>`G\"oNB\"fE>[\B39[\9-7[@s!3[@im0[%E^,Z_*R(ZC[@$
ZCR:!Z(7-sYagpnYFC^jYF:UfY*kCbXdG1]XI"tYX-J\TWg/PPWg&GMWKW5IW03&F
ViciBVNH]?V3$K;UlU97UlL05UQ's1U5Xa.To+I)TS\7%T88"!SqhdrSVDRoS:u@l
RY6%hR=]bdR"9P`Q[j;\Q@F)YQ%!lVP^RZSP'_9NOa;'KOEkjHO*GXENHT4?N-0"<
Mf`e9MK<S6LiI21LN$u.L2Uc+Kl1Q(KPbB&K5>0#JnnruJSJ`rJ8&NoIqW9kI:lsg
HtHadHY$OaH=U=^H"1+[G[anXG@=\UG$nJRF^J8OFC&&LEa;`HE*H<BDd$*?DHTp=
D-'X9CfXF6C/n+2BiIn/BN%\,B2VJ)Al28&A5Gr"@o#_t@STMq@80>o?qa,l?VEuj
?;!cg>":p[=%,CT<C/nM~>]
cs 
<<
/ImageType 1
/Width 280
/Height 200
/ImageMatrix [280 0 0 -200 0 200] 
/BitsPerComponent 8
/Decode [0 255 ] 
/_Filters [currentfile /ASCII85Decode filter dup /LZWDecode filter dup 
] >>
pdf_image J,g]g3$]7K#D>EP:q1$o*=mro@So+\<\5,H7Uo<*jE<[.O@Wn[3@'nb-^757;Rp>H
>q_R=AlC^cenm@9:1mM9jS"!dTMT<$3[GQ$8#0$s<4ZX!SPQ1`C/m<k<ioH)<bk^H
j`\=EYZP^B4!cR^A[GA>6eb>DN[Pj,mFO@3?4ms*LW&3bYhJ>kMhe"b!5O$n&IAW6
_8$%q8h2*J#U:`/81/r36NNnMn9?u7&*QDJ3&!HK+<$#f+osZb81Fn"0#;MZ!&to-
#=O/P=HlKF(k_qk)mj!7$kS6q!eEaAAiU^L_c`@7BK.%?L]`3iQt/"^eVTrMJ?W9?
W!\:_@M&m18f.s>_P(=eBK@+F#_XA*fR-./"^lt[$82Z%*XOU)(b,rf!1UP2K^1_>
&-)_:7aZlT2ujYdCq9`^"2PO@(Pnc(>_)sL]Mo?Mkd-9Z!q;j_%6B:n0(L_MkWB=V
TTCW13,sa@&OlbV+:Ee:THqC]+TOb=KFnJQ'a$#RU(%0Dn1YA3DhN!95&bHjg4GBU
O:?k6-m^-&_&,a#TKn#W$T2?#3"@ql+A3*ZW":9_3?^30&&ob(8/6n'OAl3An$k1b
KJ&]5#t\eLZjhWfW&bVU_,+5L#,lnU!^:`X:tu$O&6ut"!6f`oK&G*?%>#^9,?P)"
F)LRNTR74T!T7oP&&.GK<"$:qn2(P1!;JKZJaO't%Km4MXO,%->O;+d^q_a<g?f/'
8$jE17.]-8cnl+4QF*4nK?rl+o7U.@-jp.e(ebTsJT+BX8hW.r%g%:V8/)5F.LTpB
TeLtK"OG^U$\DdE8Kif(=AToi+_X4+d`in/'8-@lapSAro=PKa!7gWK"CY\K)7#71
=JZ'!V7gc$JCl__\3QuV'Sc:%E!QK[BGLc&pAA#(5EY>CFb84%Sd^2(a;kAip8jo!
L;=Rq$j)S\1(1Ft%BSmJJF6MLD?/lh86*q]`XUTdeM%=re7_XA"#:heI"`_?1^o"F
#]p`5Eell+[p_\[JS?7@=hFlG89,DsGaKfeKF^%U'EitpH4P\FBOL40D&>_TKu#D"
%J(`[i6P]&+?g5liG`0@n[i`oJH@5>&-,)EF?H&r!)ukL8tbZ.>/:(28/I$>3)0m5
i+N`+JO"']o%7?k,R6M//S2tU@9=QT!J#$'o.urMTuY$d/U^4mHUcH;QR\"[NT_!6
p5fNB)GiN<A-i8-5R1N1ohl=VT,Y.^PsJe3"JCSJY1Htd5sR"*J;IigFF"'TQlQ?\
KG?WqP'>6YYt/Y,&d"?pGEQ]9"^lj#)aHdtJOhBs8NeFe^cVn=3h?M*SB`R60Eco^
'`\F]5Ik:6"C<N;A^$RhWt7#fO:oqB!*Ho:O?T@gTF:id.JPLEIKY2R(/-tn5G(<X
)8LJ)!C/7c`cFJ)!;X*c%R:X-#N?#Zl/-@g*L3cci6,@4aBZ`-GV3"@+BY'(KZG_g
UuPGq!<=>H9^0nFcp@sTEbI>GQk_?;8-_Di&d6G?C*(/j$%SK#=U4'%!Vo(g!Dk9N
#'eJr&6KD^6BH?J\.4+76?UkR+p>]S'S:j%B7Ri]CoJj]3S<Eq8]VE+M:rt"j9Y[P
a:i.#d/BCjQ?N=R'EbLL,G/Ni#lq6I!cqph)PAeJ!CT:WN]d:AAKN5RH(U<DQjlAR
7UdIuoO\J*-\<I;G+<BMG%TeE!HinqQ3@(i^iU@pO>;@r$1WF:;/32j/qoND-^q>o
(]j+uMGLN&#2naqK'>=tf0Saf+K-2:-.=SHE_eo;PSlH(nPGcu)da`3p4?8*I"=g)
"eaBbJu=o/J8)lK8,*Lo!#X/"BFLCrE#)9gVL6^JAMLu[`l`r#j4g)j1bH6:3J1Rc
JJsURJ:J#ZYWA0+47mAa-j@?l`/?$+%pWf'%K^bUS*V72X<:MIZ_0trf=2b'LQTpb
A=T.I9\4*=h+.TM!hL4_(Bbjk%5KVN%DeSjR\6>H-abT^6-)(l@."b\o]]7Q0H`5\
S/HrE?K:<JlsL3#l_+;VbCLKY67g@T+Mr*q/94sT.2p3V[Zgk'M:YJNk&iV>;!8Jp
*DU;m"g-qZG:34;Qc[oO!Ro4"5jDn_+BZQ$&6<[6m=n&aFkg.&9F&D4,QnfDm^SNA
$#+4L73G>[SuJRpJYFSWLkUc'_f?$6?(_6)q4C/']-:"\n?S^k(kY(_ToX3-\'V]m
K.*+mdrNGaaR(^Scuombn10<=8Us)oEc0Eh,6ZBo(P;-:$;&;JNF42;2l#<j!/'iH
Vm]L"!'-D-6PKT;<"+@N4OZSG7KNnp,_4f&iS2l/@_f&]!rG0L<p14ueNJ>oWWEQ'
[#7%s1^?a>T\n;h('AAr,M?_:p6r7dK@jQC!rsV7%0/A69XGIc"kJa(-kci1XuEqG
SsK".0a7WJ)rp:_$I@IQYHU@q)JYG+n/SA`i:T/5^etSlg(qW7cjs\FL=>)W&HtG!
_NUArr)0OE8+PdU!C\\fd"6IEB9g/]8ktofp,UKmQj&$%D?@V;/4u$G1XH\6VtQK.
"mN,S5_Rp>Qe3U'b:_'A=2a)FKciJI"(Q"M0;Y8i"g4M;'&;N[#HhGs5!WkkJ_gNq
5b$DUD!;KW0KKJ7A??'%\D3M157$?YTg+A'Uk$r25M+ZV2+un\btq+-%Fco&Y.;+)
,_oY7hDkb\E1=VnpjiG/'1g:!3`09h-r8;)2H;0Qi@G3*9`#8%g2Ob-ckL[uP3m+Z
J.fPuI&B8\/S1t"r4"Sl$,J+K^Qhl-iA5Vl9m;/0/+a[21q;j'UBUm#rR_4fE0Le.
(4/N((5"ae[1)'i4`aONJrjFL5lLk(LRHsMJ5U;NZtocY8Z4V1=d=,nA73_s(#2&f
%33P0ad>f@CtH)_d:.&Ad%dR(r&=h0Act@h[F6Na.g-Q5!,P-(Dl&*IPTABp6GS*d
i?VgmRt916bV]!e*;Bp3P)iGd6<Y=R*d?O.p/!PDU\@^X]4M/F#%5_Y6=as9?taNE
/-lc(8gA4A8+;e:8@p!BZRBS.UdVN/8-L,Dp?Ygs"c*:(<X.J]3K(80?q^Ws>%D#K
7)2K*%Km#2C'G5O:Lp+ib77>+1:o&Wa!5cCic"q9L&q>h!8nE&BB!]=>WF<>53:^"
`>Uet5#VQtT.F#aTIrK`L4TNC8PS2WcI@&Q/sZ[>7=\A4,keBsP&eLb!lWYm"CR8O
$r9\8:;a;2@ofanc3<-2"(5;ANP&oA$3Xao"ta@g``tB27\Cl%@)`Df83TB(CB`Wg
"orDh5Z@tRHFZKr#68'7?u#-4cIAM5G!nZ,UeCsM:f+r*#Jar?TNVMl8su>K=Gk7&
`oI9lkjJZ2i'osYKV2UY-ir69!5K!D&:UmW)U+uOAV7^#B/8=;^,tKh=0Qe,7=`Zn
Em3W#BaO'/a(>D8@]Z[!8O,6=-h-5sUe?S]!^K.IBHTh+`g=r!"%7H$`6(N*k*XAW
E1g$BUMs[PXp?aK#2iD<m4LDX9(4EsiZhW06M(K_<6Cl$#/kmO^dJF#>$pFajPW];
?p^O)\-3'4M.9!Xi/5[P=PABs4j%:<TL(Hpg''`FR\SHn6>T;Lc:K?VhCWi3^choe
@[@'A5i^'OY+EVJ2RDLk!Mg3S9c.TCc=MMWXWnH:7?B<U-j.7gg4\OZB*&:Q=MQ8*
?)3uPb6#GTi^a.W2[&V6o#Q]AWr:*j#B%O?`'abugfpF,#,#:$i)g,d(9W<CRR\3s
XJX-R2FK;i"]A/!OuNUrWWm.@?'6WR`t/@WFDRbQLZK3Q_t4))Fp;f\@)mBQi)3BH
ejNC7mA%#jVhQOq.Z"K@!h`ElAE7dUquk%#;C$bnOE<3%<X&Y:dR<:n`-Q2Lc@,a3
]s+eG_`D(5DVd/*@O+q/&Ss04^k1\5q`mu0$"<s.3("fd6j/ZD`ACmG]M)^$#OQ--
."2?":-NSY;i=K(kAGkY/BY9l:<4PG+@^ZG^>MpVKI)":mm?2J^]KS(Q6YHpi'7Mp
84j"?#0Es&C6D,$2^Kd\"Nt=MbbbO44=6.B?)mr.+ADH=(2(PO5=H#0VR4<Y^4HW\
^Loll?lf@l35!9'<[\L^lkhYB1,__B\e='dLAD"n63\f$N/9q),`&m]n6'9.$&/l#
:&kJFi,9oH6,Up."lNnVZr2E<"u!3DN>,Z4r]RCO"`GO-j)>*tW,3#@"XKa"l9JGO
/8`Jm4:+K`K=Z%*18[<+@_c(KL1(8NP"F^3HUp&DV]JW3W^_SN!PhBW1713NQ<@_W
2CBP&+@dlR*3AAW.I1YYM>o-P>$Js<@V3c##gSYg"A<5k![S86VWp8$5a@-nKrM?^
V$;G3f)Np%$m8"C5]U_bBP6P5U'E63cN45D,R#Eq8]_U\BDPiMqXinIEKo!J7@&t6
p4r]<9!mIJC0j4Oi\6%(9Le$I$gd82H:_\(?sl*oDX-?mpr2:I#>o@c7eBddU,GL-
G4Ul&K0(%VbQNG3!<<UeKh+\pL7"6<NZ]aO-MVZCcikXZ1!&?;<&@t?7VrC5"pAg"
Ub#kb1e3D.DIrBUOI"-Z(.Vn%"UKbbFXB$]n43f\^gp>;$&jbhYs'QYAVTV9M<6\;
T#,V"N/T"a5Y;3DY$7c/&YOFR;Ze[C)IB4-4%N%U`)NAi63fbf"f%H;j'9gS^]r'g
5Gq*X'3##C:/5F31;G2C`LLiP#n,kK"^hZ;jXEFP,=%HUk%gOi+;b,9@Y)K(VU3(U
KBAoHAd&=IQr^f&A=YW=fkOFEE2Gb`-31r>:n$PY875oZdm>q-B#%p!9W5ToV=4T&
Aj7^*6t:7%b3:3!-RC*7jPWK3'.u$5TER^V8cWH,!spGm!!LA45=\&4jdJXAr`"g<
EmB+<!*3H7C;MUg":!!Mi-*gI9W13C-AJiV0T>?W`;1()";[[)TMUL/:p3?CGBH/E
"4IOtT\ISl1aulqa9nBEbp.aF"u!Q-KL&To:gJT>p#&m_UioVT>aN[[TZ$27Af@+j
Qj5$A"Yg?IFTt&YJL,hW1[7F4"(&e'k5.iU*[A*['Cmrt/q'sam>[uo"c68q[&GI8
"gNrN.&[2BSlCUt"is_.j&l_JY7/=325Ha6UVnKN%"<=If1(0D"(Y*)Z8]qiARI7o
WXQ]K:^%+s!f4'n5XkpPk%Dlc7cQI,+=LSClM*"$oAEf`"#r+[35COK"3?es#/iZ]
p9/"UdT5@+7.g`%/q4Kn]1X]l7Ne.=2?PJ:T]eY`AuoY-FCJl68gkJLVcOds4XE!9
EM,c*8C"/!?Sj;3)C1P;V'n+<@L%#!@VPg(LFb]Ve1XDUM#^S"_Ig,I)_1Pr9>lue
W9=9Q18!K(5<qEfamrd)noeO<DEpTcjB-i')Eni@Ck+bS-<Ps:6j%SSR@o6ZPE;(I
]S_Nd:re/PL"rp"!)"Z^RF5!(nsE^`TN\*S:sr!q.kEL?cGE=cOTm0L7mNQbk]u)M
#/drAj7bfsp9pA'DIob*aHC.,[eWp\40)b(#0;Z.Et#i,2]1%el)@O3@4/)o=?mr+
fK=!n7,_._!kF3*E2&CEjuUe"S`?hMKj4][AcZH)>H"+r(q9YMfWL&B9En0b#?=,]
*,R5.=2gn/\3V.SfQn%\)@4>XNmrAMV/LWW5am'^a\#kA[4qk0W<Yb0!*"'>Xug#T
#!bXoK7o,;BEX5Q!onP5m"pWI)XkT?KF!/5pcr&V3K(Zq"J]o<<kOM:0!-6<$i.<!
WeEeWOsVFMEhf`.6jQG"0!ODq!oR$P`N"qo<scZ;Q_jJD8[BE`U0;e`780l]J6W4k
k(Fjb#'ZBg`oM7kY#>dOUu3Et`Mb_QCP2[/>GDfpa[3skZ?AYW-_l>SBVDJZL6j9^
[Y6D0"sT8R=LhgFNT3-fk@FuF/7`.!#*/1E_q5.S@KfIhHKD_1A\:ZgHt0BAKkWqE
2f8e;\pgFB\RTT@/l+f'+uqu!1>?d9C^DO!MFECbd>bhd?oES4Ck9-NXJ?sB=an?P
.",-BUVJ&V!,2r+5i>*-#%1n<Q-'3e@(SqQ?KOrH>C\OI5Qq.--,o;e1eIp>@':'%
=<s5JqRm\T/L+6FKF;LI$Bd=44/)6[X!;Y'#WGtbWaC9_GNTlIc7Yj,=h-t>DenK"
%K9^bBKGCKA,pAHZ2Tq3b)#*/ac!!oK/b2.c`>&hcp/L5aAQ<J?:go8B>?UGKMhhf
-(X2f2dfEN+=:@8r]=`cBa4\EC2k"=!dDF`QTHr)TO*7akQ1`Z;M<oO-<dS8Ue?C5
"MeUScJ!V=:PE`0U9aZMB"VqV1-]/#:LonkeXN8abWB]$Nl>9l$%eGC#:kP#KEt6T
/Akm!a1VhQ>+f7.[&+&Wc&a<)97<5QcZVX,@!il;SkB=l7"ADm_G9_oEUd'u5UHMc
mu,-)>e&p<"%Ggn%^<t449.,?lfR_#8q\eaoOXCPk8J=n[^GUpMZkNB,AoX2OJ^?;
O?Jp!,1fY=Y6`5sUP87pe0...P"Q#,-Y!dci(sUB)MemnjI#'2nHs:W1,m:m0a_&[
A=p:q=pMiZ3l"\&7rLU:e:@heSASX9h1L'K?<gkqRUf>lC6DmDl9#3274W%Hd<:(q
[[o)H-O$M=K`aZZoE=6>gQo0>C4or(GQa[]qP-ht_a(F\oUe18WRXP15XYeVD?f=N
=5ZJ_SFjpi(uNinMUCL\jiq<$9XtFhb&OWijKJdfI\CYF"V`M'oC>JjHqiN_Qp=mZ
!#u3d!d$:&LF'qD+Edrhb&HH-JJ^L3jC&sO<!D/"+8cBja@kcm/ACVL;@<-a.7/_,
BPn)M;f[sp>#J,XFFOmC=bR8b1O=`/1m4[$bhsm68hOrjg&s7fm4mCA<8pIQI;'*T
#(U5e-8,9&l>sIC"2O[E$M9VdqQkfm\?`#/@lOTVDT7FhKHN5W^j64f6s?6GYf89u
@K7S^LI=HP#^A*M'oBlgTkMME$knJNikXJo4rB7c7UlILYX0NGM8fX:phDW%$O+E+
J?WiN)\3=piZU"C8-#2UkEFTkrddA+KnH'b4LcdRPluZ2i4*eW2@]r/6'0H04rt/*
"!Ona<#,fEK)oBFY]rJW%gPHF3Il?<.h794<JuBT5U-VhKYlHF>W<W/"9[W0i-[Er
$sFdj8sl&B(D2@QTb*;j-5ES<KnBtn^g7nrN5f;N0PiKZ$&2i!"6)'g*>4,p!MLW4
,8^_m7/!Y%GXa=tLVi#T+JWa/,um;UNF[uA*YAZ/ooR6k4rb(="G1('\4e1]#Xfjk
+!SE7&;l4InCARI.2\$G_(_,e=ra]#KS'*Eb4@#X'F+[>!.ZU02utF2$E5/8('T8^
TJHL#+NQ/B!hcPo#_W3kX:TuV:_3e]i/f8k!\g)2%jg/</.Vm06SuZl@.Rh?"X0O*
%#"^Y59MIK]O&3(+Q,_@KW;sQbQ;N'0G"BG=Bd6YP-@mu"E"8hM+U&.S3@NQ3j=^!
%jDA=15uiCX+ZT(5S+$ZfJ):e5mUN:L+SK^%>4b.:)'jK/7OsUY0o!B#6AdGLkO_U
*Y?3hUlHN#8SBfF"CY,7%_He46MI_lkXpr=+OF6meMU6H#6M$+/GOqBfH(0H5_F4i
\D_fh#Q`k.*!j"s.aSc[5\Le9J]_cp$Dn7hjNE1Z1WHtXD_&a<.q&]U(^.Yd9.gA7
S$ipa$,!j("X+h>&%o#CRLOp9LfB1a$+l4QKAdA5F!fjB<[J?10a?mSEXLC#KqQ$X
NB:'p1mLE^a>+9ZTbq/R"kVL2%u*APA.8TJU1CfdG[,t3"T`jS(Bl7t;MI]&[-/8\
EI76h"bCG![45lU0Vj<ZCWHtebAC=V5X8^*qLZN[q@s+J?k*Ho@!F(/6bt`A#crPI
&.D7Jj.['f?t^5c"\T[[OZCN^.L7KqkWH&KpXRiRZ!e'HON@eBLJGb=jneJ"]JadK
/W!<R4V7gr1_=Wi1+3ll+`,@8"G%2k&W%]FpdL8He:8,6r6/[e!pdu<3!3j*ed_:;
P$A@s$p+q?L!.YP3(P(\ZjCK?]:032EKqX,GnqqLQc(@GOpZg!n5:"9N^,6,Y*K>=
%]q=W=etsErn%`K+QUdn"''"S#\;b4\.Lqjcn"h(T[Uaifhb45'S0YeCdUHV?@^BD
"C8:e"@/oQXWhXWcP#=C@">ljio#9F&tN:1A]#17ODr$,/d@''3sNLo,"0eF'/$NV
Y@(=B5sbMQX?[@#G<R1fi--AXLuG._bYB0.;?^b07=p+XpW6R`/qAY&\7FOZ_#q`'
0-gmV'Y4VP9(\"VZk\1W2G4%7?]4<U%&51D#tptV!l.B7(nbOIMPCQ,;8f#j20'$)
K$Ppc,nuiS<je-JogK5Dp6,]dFTC.WE6$T;[EoThJ8(E$m^N`.&7@t/fHXaWUl3$M
<s=KN'R%NZ+;^9J[)$]COT?"9Kn-lTKA_b'_HmoX#\(6jYTs>/YSd]Y&e?+`8dW?#
63n^r'g[BT4#+8K/KdjqNfi9E@&/U1RA:0`UXTH4BG%WG$q"0J.g1_i8%hHFnn/4S
,Yo^\K(\I:R#hlN'>\(@?r5."+>#ou%A3_;p4pq6erEVGV(%/m]odUM<PWFN:nTRb
8/N2%k26J0;m'>n.q),iL&j+5%c5@4*'(rB&@B=4\I:cg"$h8*Tqj@EeA59;Pbd91
TM>lG^bmVf:b2d#]H5"IT+\HN9Snr!$NY3c&;"jILTq6t>VJMO!CT'V!;mf<OBDuX
M"(NH2MR[;/X-K4D3?Xk$V4e;>QC96"-\I_gYa1Z/@_2sAp"eR5U0(.,l%M:bQS"i
)ZkQ.#>m0J31$^IGp'=0QR/ga:^mGQ/^YUldaAB9a:Y.b7(P:p:g'%I/2EkP#.G-h
"<[sb0[\eeg1(4W@$D?J?tfD<d_-pB!FM&r]uYd<k"<G:0ma=hPC^MI$j!:_@%ggU
e$.sXK\2M%_Hrom:bEX':j*3J*'4EKC(11D7L6h04bqDV*J70h$fQLbOok@obM#]A
(0D*YA%JCjRso;L[Y5Q.70N">(n$ZA'L;4X-61DV7T4gNKM'[fR'7k?+L3SNEmlTV
cn5KpW[n3u+OXVV.6AnfMm&dK"DpSp!Oddg!5b=BNS"mFW0R3E5Ta[]CMto1\s+!5
%3*Wu8rY:Hm(`B,#$l!UG\!O;T5n*=!:V?Zi5caf:dK-):i$[E4@oiV/TaCjIh!Wd
1'US/(.9R0&c"s=KKt>/6eHYoiQ*g/0X_b6auKS.mK$*0>Xd;=]em^IQi[gsNQRY?
159C+.fB/!f*!$>p@,*/Vd2tjQ')=;?l+JC>i\1B&85H[LnK8_L-]SJ"LrTM6PjQ-
bs`^QZ&NN#5TC)ML`gBH=^.,UBENdH%P0@l"p":cd>MHIBAdcJY015W2KQTG\GupZ
5X8As\Jfc:;%nL)&-i4b%L$7A(PQ8!Q%MaV&fGaCh%;+]!si6@_.Z/l&J-.;bc1r"
G4LDBhAHBC3sroG+'MJ`",OL5"Mi*rPp@9e%k&t5i17?IHFh4[_D$tp\TX:56qE@I
\2'Oebb3SeoDl0eMM+Y;")qQRJMA/Ki,3e-FYMlcfce8%WDoR7N)`GI0.NVqM4m=f
Va3]b9ZmRVJH-=?J:4-mBTNFmVO13o\HO\-PdO!J7!"6mP1`cA'`s_<5g#KIA5E-Z
WoYp*n/==BS]!:f+WYY-W0J!I<'U[2r$I$">S)KX4U9n]&]+N>$j#9H#4U7`Y=N%.
@71o`12[3AC)T+O>`8b$b*/nZKE_G7P8tmZ#1,Yk.hZ5&K&Btta<KIE!3K-H..iC)
&XGiP"IPaVoEi3>Ki]C7!B#)+aluVH6e\H/+B1,g?GgSImpd)_ekTsFJ/LWe.c(fb
3X&D@-3\R#YoRlKL.^,S"ND@F!ROXNJBaoLD)3H!QRE9YA#<JgV;_N"K()UXQ%7#/
V4\EPW%,E80a&ml"CgQtTLjfE8HXbuK#f^!YV*Qo2M7A]!mi6FE&!!G`WJI^K&\nD
GUEQ#'osM71YR)S$Fkq3%\=RdJP[-`RdUo@3$#6iN[`ilOb0=#)1a1UN.I(_qSAHe
?RM%SM,JaCl.le?$(XZS&DAdpZ-BM''Y[]OT'Nbig,4DL7Y#dJNDo)&\Q:>e';'&T
!>$-*1D-U=;'2HtN'X@lck:n3$^LQG!.,7klN33i*e?-.%k&&0HH[-5.75es!<Oc:
/4P6d5fA=H"MdM1-pWD)7^#'CKTJb-TLFLS.fu(t",Jge5Vds//HUk5!a$_!5T#;=
TdZEUXYBs^iAi>XOX[4G!K7u6]#t_*X,TZhP;3FMBgmSmq3s/Y$>`h,8i)cHr=V('
T9oqU0GUC`;1Sc,V5T3eaT<M#%O1caYt,'W;Mgj@g`&6Z0ej-C0G5KNh7E@lJZt*K
!njN7$&O5A!4WUA5T.7t_ii+t.8U`[RDB\AmZ_^SJ;OC>5t:rI@D9Md!>$]3Udfs7
/d(I!KA\o.84J5n.t]6"!h_,tr(R<]6%g(:[idg9BJ]f60`qD0!iRFIO=5]7+p%7u
\1AkU0rg(5V@?E*N%-;2L_^YT)iCB<J;=SmTq_ut^ka*EP.B)'WF);1AM"IjJ;Erl
qFR>^mMk[X2#+'Nn.MOR8XB9lO;S^^X6^E8$+971!N=ob`.`_,";Ru8&%J#.\.'g:
[Leh=$Me)7W83aGP:X;$RWoVTW.L$Hl_OUQJYZ?dU5kP-bbZcu*&)pT_28;M.0?#/
K"sI#^cR1Q3eP42"4/e*0K]E`.0GAjK^_M8La`GI3.kTj"&tTh#VQ8C/qTH7!b`q_
E$58:djNek8<=H.qKNH?Qa,n*Yg=5TJO]`EcB0fYJFS>gEAIu2Yemme!MjZ7_+dP<
#QSn',[$!JM$amB'7i_lJ\W9AknsLMPDNEeb>G)f)#H9C)BG8@J?T<0:]c/,"+XPU
cH,b'oOZ?Bnr62;$P]Fs^s'4`p`u8M+J?T%d)uhoOb'3b$LmtO`"]>!1C,F]XcV*8
GUQ,p.EJ/@K8;JhE&If+2M.;]!q8O.YV8/s:5!"F"CO6BE&WBUhZF-:K%MXVa=%*l
,Q^soJ`n&0_/L8()$*8DMdtDYU)8d(*.`nYJWlE+U+;jE-OA1o!9skaK?O>b'I.:j
PgC*[TZX)5>senOTns3f@/^HTKo8XK#sbVCjSarM]9+OR!)[-SAFuncY(2_7J5^0q
i".dik_j*Z[L**Q;f)M\7^4^+!-Bt2nHpSZKb)N;J9_iZ^mb@l(WC>$Q3q33EDD&j
m/\ou$HeG44Q1mW?\4(^"#)Qa5ViKR0*:VkK&k8[W%`j[5(p.-KJ5iIGVt+E0`pPl
"$eSm]=<Gh'S8"`JiFu-l&5Y9)?F:AP;&,LpkXdCb_V[95!fPV.3C[G2^H2.8m&SJ
qCmdu"IaSd,+odcR(PU2$NP3k&D79&l0+>q+H8YGcac5j9g[>`TG@90Q8f"I=L#aM
OHsPgJ3l\l=kBW'@Z"Ot!)eB!79KV@YdPY[7i2C0A;,PM[^LJWbW#k.^^uo1(BKU6
."l2_dS@J2Ke7hE!B:U@0Gjf*,m%?fJq,78-nYT%07rC=>+d7jBIJJ*0S=m="B7no
n2:A.1P7)/!uNiJ`>AZD,Q\6!Jf#[5(a/pD#r7SZ!:U>nW/SnKE=SA(8jJc[l4&<S
'Fr5KO!J$rH9JHO%6jQA*_T`Hajh1!JKLV2b1TOL5h/+'=\gH9fXRN1]3pa<!e<n"
UhL)7H]uh2K$.kQeNg2E!uer]'a\S\J7&MkRp[0-"OMD@(3mWQgObl&mX]$e!I9d$
q)C'b%(-WSQf&e`H,E!W$j&[@hULOkcmaRb:]be,:)G>[IBS9B4+m#c"5l<F+>R;C
0?Jnog7>4U3$X#'++`o'LksCjTl:\O$4%j^.cBWa_:Mg@JLu_'VPQ/.aiK"?N4lV0
4X%]R&UjaW(oGu0QRMG4.`&'N#qaQqO\""R^^#D"[+uRjQrqiG_DdU&Rt+TI'l^pF
S>8pLXqA1nJ;Bp#+;Fq9/IOi&XJiOef`dc\g5]REfoQE?(s<=j+9<?l*g.;9PX(0M
&-7bqQY74e5UGFZ-%]MP@e*n.FXZ8E-3@R%Js\7pBK?6o3R'6CK+9nnm3Ylt.Utq)
!N7&H^`7pH*<Fe.R:m>K:_!kQViQXbX]VLJ@c*l:1m#e1'7t2LJ/83sd6]]jJ=;l3
..NPso$d]aY`n_4:*p?iblJ"cQfM_.\F3isToH(5P0%APnHPnDk)dZL-tn9ti1qHj
,@LVdPPF:;aI+W)dgJDUJPg6?8BLp_YmVU\$[BIcL^epb`[=-V!8^""W0nXh,j,.S
!dH&D80hh+F6<``!g#*g=?+^,3.m;P<^8<ifIR)s.ES`3B)ikOQ9Pg$)E<_u5t\;@
GS#FN*>+JtN>#/0X.YSDOpDne%hnF5:#?:m!g6e-JKPIG;UheA]n)Q*!:iSk.[6o!
hi=)l!B:B,0H,Lc=+C?26%`&A_k@GMi5^6-Q+9sEBFI,PqUp+uiap\s^_+<F*i@5B
J[>;,pp;DW/:gCmJ=$O6`L:NW)%E]J-\0C08h'jLld]eiJWm5<[;f7Z-3AuN<uURD
AT;?B."_d^K61"D?oN^O+TgRS!miH$V=9(=,4#:RJOg[CEh`Z^)@5[P#bn[<O;EJX
&V3SIMqUug.Yo;E])dK,Vb=:kdK0t>]Ks)F_@1-JdCkM6(!i6[k'Xf^-ln+0T7KNP
!Uq+k7'_B(QfW[N[%OO[!D\Qj6eDPOJKTpZkj+]%>-J(FjP/N!>/H=;*#*EiMP(K2
NW:1o!<>@e,Wr/o!F)t]Aa]&T$*jc.C]"1j+Ta"+ae1$`.lM<hoR\^(!e;tW5W.+P
1P8rgK2=.4YU\@W,m$=TE"F0*YS]NehZ:b"!H?A9;8\_Nf](,(!H8tcg"Mg=$uEG)
QdG0PWbGkQc>8-k;(IUlGi(\U)m/)7Md\fg^onK-e,dW1+*`J?I[E?]Pe$Z:eO8SX
kc*)t&rq#52>@<)3!9^CFn&5R+NP(EJlDcOj:9DMW$+Y21R"#RO\>J//AT5fbfjuT
q8Ltu[h'I0#U'6k1P04d>H\(s(GkN!-\DCT"$eJj\1n(F1BT$]<pa8G%Jp2+5MsH@
JSB7X-m([`'7kEY!E-86p_5SHb:j,<OSj$WhLZ6kK"ZtpAleG_du><CaCs7^.*CBU
0[Un[_[gu-5=gJ/ipMAZ]E&U[!Cg/(b-(f5I2ZMa#h*Dl7\7J!#S!Gp&(?I,keajW
U&c[#.o;E0m`^RX'".7lPplB_\A*p\hh]XI0A6U20G&cM*K%)h!@Bu3!$M"i-..5c
Jd6GmB6/#/-Na0"K"*31i%]j$0`u'8h]O?=3$EkR*J*,i!SACuD1#g6o+5'i+j%t:
b7/XdOpP5&TDdE+UkB#BZc-SqP/rM#fY<Q[7=^:@7HC5m>[.;KdhmY(Pj$Bne\$d]
]4H>%8/"RN^u+hH%CO1g!-)4*aX30iPmb_OTTPi6)/B7R`%CcL2GnUIJ!uN2Rm--b
6<d;4=f)PIg&Yk+!YEok#UBH7+(*)2JljH'V>O]@Y]L+n!ba5:a=.0]/%g*]01[a+
:$hu^*eD29J\W3*[5p!-F-f-0J\^75&Fl@@WZDY@V$<[\>E=kJ)1cL>Sa[0un@T.)
[ZZEHJS>Ljr-hgRb"o_U8*ChXat5a#McdYtN%i.8g3\ifk2kLQSfLc9^l_HPT,tg7
cYH,R&Yfao(2Q@%M`TJ_i53(Xdo3WH%%mmV=^/Gp$4i4=ZX=r,YT3E<*WbIGJlG^#
p[!,8m!d9b!UqE;mAkhP+g[goIk21`cm*0o*eDr^JZ'Rj#T82TnUJA+X=0R6^__Qp
&r6OT==Oc8"G(NZ6m*'IK>G@MGXs;$%>KOFO[s^^+qoi%ic.f!?6'I[6c(PhLeSWr
#R#`Mi3!7t#m>k=i:phA)\RtEno4s9E\/#`KgLne?nrT";eabXKgqn;!([4.TZBGG
'G(T1JT.8e///BnAt]d/:b3CkLBGB?!+[Pm$&1cSn<dH;)@Ta-JNF>56o#L4_j$hL
Qog3:@r^/Zpo%8-$3`a]d"#$<,8Q,(&0\"IIQnb]#:#qhlukuLPm?$*hP4%3*c4J[
_XVH&4XUuf-)0XOYZE<:8>K][i,1:p&;>`;J?2X!(lRLlnJIKW+R0A'@UVfp/1V;9
JcP"R0Jj+J#/['[:lnb8SdC(E=Qlhi+qTTb!CC*,V]a>R!ec+Y:B/.+pc,bd+W*P*
#2t)-(I-k<9`"u"\1jpMd/'IL"<c&B#e^LG-4:s3r(+'o!,*>V!FT@V#D*>`q"Oo`
LaO3oTT]EcX:(CF$S5\Y1(aY??o/8*!8(*WU4DSK%P]Y^5S#1)fM2aWanjd'KIJTE
'8>D<H5d'^Y\kFT_8)3]MLk(e*6l_i:t,e<d'bJ26-tcE$Gs<[/dl-]U*#1X.#9&O
Tl>5k569DOl35"CJF,onn2M)8Tl=0GKE3K3%m+I)2@DTT#[.s29JZ;O9L04[>(hGT
:_Bm,^ePIDn45#==2=SpqupLrm$H;&9ka!L+_10A_%4=\%tgpI6#=Ht&3,=Di+-4#
!R!_`%0Q])Zk'hME"s7AQZsGD!l1huXTD9Z(((/;#Y9uMT[6U["(9bGIY>nk4<"A&
TJ3kYE$@+MVtAtt&-OY^Z4>f3D9i(_iJ;(a9jtE],RM>TGr>lc]\,6g_EbCXMP9fc
,)QG`W8@sAYacek!cWf8LZ+>DT*-<I4^&!j,J98EJJ_4Y"X-c7P1Z'E2A?9HO?sV7
Me8uK@aHMiP_4LR2A)eE.bp$@@1?coKpP1%&1@8&)XKM&OB2@s+ZMds/-(sC_SdT%
('jr-BGu[pi6'sm"n("bDh1/E'FiR69'EP^%lc$J"6c+60gM^79+_6i,(X2X._$T/
F@gAR@KXdb35^AScG[WU[BEL*L&m*AOG8=ZCa07\Lj>+W6*<_@#/WX0/.,h\F=.D^
HWhp,@ZZm%#D.2Bg9uS'$bL7H\:,3j!<U:-5iFCfm-`].4N,hP,t8T"^g%KdYW,9`
,Qo<aTFh6U<Xd/r*[N)E'EZ':%9e<H8q:b%,Zdlq&5Xt`jEUQR:eV7J-mEWWS>MrX
1]p!6#Q[Je)\Zk-@a$XBK*ELIW[+mg5pQd]A[oa2cn5O=&0M(JLr?;<[U\<-9ei;\
,,Jh?>8tX2!l/5I'%LY%!H9]:D\*e=0T$FYBKLI3ehFaLNX\<7<=6Q5+9Tu`(IDM)
$6`(jK]&@4_:V0]!7a.5J91t1paH;q`"rJ_@LYUro`PCD=Z(5'r<_e5@mu1]&6#f_
JNtk[93NIAZ;?8e\LdtTARlu-8.MEk#[<,GZ2t2EJOsN$E^qYo!X'G+5r9pB%N(BH
jm$!2i"AI+^^S243oGo.Ce;\Z&f1O-:7WdV"JFTlV-kt[!5\%),[>rF(nAOg>iL5[
<@T8%/dDmAO)uW_G(L9)$WQmSMnmCO"&OFZ63A>8T]d64#gs;+j$3kn4PtgrS.l$L
8phcj*<Z@Sa9!bPCnSnX8?d%@-0a/90]h%$U^.;nM\cI'gklc"b,s%5gaPL%K#A:,
hn[F@!l3&/0dTMqh>eiQ?qK+;"pRL]l-KV7i4,sZkQSdR^Mq-VE1"#7:u08qE'Sgd
7,i0Q$gQhYTQh7T1C=AS=`(6j<"?/%0h_t#-7A1iWif5,Q(WpJ,,`-uOe=gB(i#qM
n0f%RalsV?#Wi<C,Tg,rHjic(!I0.q,Qt?;&AfU($Ent,K[>_k_D"7[_%7JQi-Z.<
QnS_pm"'cX<s_H@5*Ie-?R`cJ=ogLY@:cU+[<4ICjD4FADroA"a:o(KfFaE7Zm-lb
VG<Ek"XU-G#6In5_#Y*$"K-QC+G)ic.WX5EV(S-(J4']>JP%(%Hjj&+:'Qd+08YDN
$irq[?mb(i"uWigT&<'FJYJZN&7I9.Jl:8&-#3TJ;)4r*dZI,K.'3md\/;XMeBF"*
MmM%TKE-pB_E^Bl$=8'"!-f&M7N2Z-<%%n-O[H4F5mMr$)C]WA&9"cu"lPmgO>9#%
ersJn^i9tf!&Y?e',HLB8S\?aed'$)3adq5BLu)oqU6<$"CSb5J[OW7i$]LQ+N,%g
q:d3hdhZ!"PjmMZZ31e\o.,?MQ@_Hc!l/P5D#fY8?XR1J9#4.PM&:p`"iNiD,+O8l
)^QM`@=dkA(G`cs\2g3V85%kQ@Adso_GE?!=5YELbulP;PS+<5SV!G`clOU>KP83;
0<e&R(J$)J&V<PI$=PV7KYWT\66pP-nd$"o.oe5gcmqHgg#/"`51EJFo-'c/%tV:B
@A6=G#68`g+@'$<_4WRgf8hmq2^%K,_W=?WFpN]P0f)@t5YFApQCq2ZHl\_I-)m+A
Au%Tq^gjp4A<jYbTKiUp:^R5WRna%C@>0Re.)&A/%npM+"@--s"2M.2'nga9.=`C"
i7OKLP/mcW.F4k-5&#R%*0m0.,R>[f&O[Ar>2$4s62,.m)'Dre_14lY>--E[P6kW5
'-RTh$mYtkPS=0g]*TVt+bS$C%RIM!.,^U./3n([ONI2s`4c#1K;X*IHLY+5[br:Y
9FQJLFBCf9OM(X/$R.?#S1G)M;KR3i(#dXHo-D&$Bp7J*m+=C1UkAao<)/O4q^).(
%jRJtPDR\,P9=E&!PfISDR_)"+M8Z[DS-*mp=P99CRECIL]k4Mld<Wca=l!&9u.)u
gPZ3T6U3i!Z?S824N%\&@aaV$Eb,F_Ta^:n0FNH94UC[Z)^fH3Y[!8C#D!R8a+0<d
JfmDd_&+AL+E@n,0JI#[iOWa4<d4DV-m\km]"a=j$NW4!FWajjAT0n839VCe6Jba9
Wqq^`"pJ8]N`_0H/0Q4e"/G@;+C#-o:*bLOk(k!<`[kWdZne@h#-ME979K*^W4kS4
4m)qM-f?>5:'64:"!C,<W6dmSJ-BGs.dCCaV?SJYi/"6e,+pOhll[j2dK3"O;efWS
TQCG(9"@8`4eiQ6U^dLP-3QS7!iSS?81JIi6pUlb#!d.j^i0KI8-WI..*0%+!.Y@5
Q@%!,#R(q*^k`5,63QJ+#=ec^@V>iL*0EL.VoH:P+Fp5"+DjS!YJd_.,S3XG:2:,q
]&e605Y;4?ZK<E%/mpF:_T<#$IO$9&#=adYX7D$?j<J%t#%U7n-#a"MnslpN.V$m-
5U%ahh?(J2>Q>s#A8I`e/d=Ro#/nF`^eP#LUl,Iu0k?lm!(a2Ci*p(R^.%0Ik?ck;
BTu%[@Sqqj9r*S\^/SPQFJ)Bq@W6-nV&0=$,61WC+F4:NAum+icRhZk+C59qJ-`rT
$OGYqj(`5BIL%H#LnJ8`+BAWaXsSl?>ej+#`rm^(?jE?TC6/Ki/Z(8^>XUn8#/GUP
+E.P-8gB5IJ\jr'^do[RP\c/a8RP#Kl)$+'/@id?Ck+i(V*s9M?n24/'nW4^?k`VA
&coj_8,si>TGR^U=@N9;!sAB\6aGWBk#7,",,1C#Uju"qg6a!@ph'^]A;&@J.])Fm
8qQoBci+#U?FFGq_@#@o+?WT<D?_[a+:XP=83DjH<!FIY"u#0bTO=KIYR;SL#L$KZ
!-eaAGR)$E$;Qggi+!nH?pWmh"X&7tX.TSD49qNOs+@`^+p`)M0E^`PXMWnHAWS2_
YQnQTe:L1>V@%+W&1.MS"e]mOTNX[8G47s*Ce+hJNM<;OPaeXg"p=rRU7b)n38i^7
!YKC*LG0jD(2u_[Q;&\XJ5f3M2?`T<"=]kM&/6mrmNQ2)#,SoF7!^JHKIh`G_.]u)
?n*`Weii(6"UH(q%ffk8huq'B[:C?F"7Il#C^,Do/n:W/5[FX;G7=P@$Qu+7j%qSj
EX-!*$,DE)&f<i"I0@FFr1Iab!t=2VK(j,g)$!,1ClgB'IP4)-^]qri5X=O&U';`V
5%VrSW4#l!]EJC$"HF6Q`/I6]8p;\J5d2U`Nt`k;NW_.e.H!6=,_YN^)?G@$-E+'u
;.UB[/->qj\qD+/kQV,S9]STf/5@7+6I=-n!c]D+3/9\bK.9%rK$hI3/r)KF-29[b
`^m/Q@BQndVbUBiZ3?#>3WNn#,*5LVAd<jN$%STSaN@8nGR+LU#69&V@!ZKOGR%V^
-,b<e8<*i2AH%QH"%3-U8q&H""BBtE-NpBskUn'X0LUFN#1)L4"P5CCG&?>sdVQSc
7]&D#9He5:0EQFS.@($j5?L\q"CP=\P_^c_Z2tB3046>;jENGuDFhej0q]p=.$@8V
%':)80Ed9\i#DbC?ihPE#34K.-,:\`+C?_,.j-*!-5HYJ*[*m+/c]!SKNVNRecP;h
SAqei,RRJjL'@,F#Ja^OVH*tqY/MNV#pejAi-#@@Hj49b#ieM^o0rrK#"O\f1M5]L
-g5&?i%.4?Y/!<R+C8F9K\`@n0-Vks-Y+L\?BE&%R;h^hV?eH2^&l/HG:7deKIR%Y
2#n'r==(p7+=Kjt.p2qC-it5>,'HAP.P/@V!Fmm>@i>F>G%5!c9#)duJ6E.V\16Qc
!ItYL"E&&V3f;J97Rc2oNteGPKE?%/9;HC\J3"f<>):Jr0F/X$BC^6qG+;%)"CPsL
5]5,ti&)X!#JcTG@$9,r=)bs$#G>Is+GL/0A:1%f#,It_lBZKV9$ASp"Me3-.RKV;
.X!-EG-Qp5Ur5F5F9;UF18eYuA4e%R0QkHm@B]AW@Mf/7)N*SsFYr^oa)WhjegCGe
^-oO6;SmpLQR:hK-mV[m!(o]A`G1QX-HjVk'@?c=*(dpi!KRoupLmmmC0pYB3.NK8
!'gTR@WLlE-itY@Nne)12MePX!MEO#+CGAG;C?Yg<_HsVE,9$(L]nH#/s4+*7RTsp
(^],T1knO+G:5AB?3XedZ"2Pm[SZ@t`aN75"<^SJ"24qKXPlW*!nG`h;P]haJ14&X
"QJ'Q9@J+j63I9c)qV84c>sL=CB&Ii+_Pj3&\qCW`7.0R0U=b#Vb/9;@9ERZ-NFd#
"DM@R*6s/c!p/o'266idm0>toD$AQ9"HY6f)?[@0SSfXKcqX]h@K?H?!Jk!8#9!Wj
/7N:E9$4GpYi?Q0UK&+A2b4+&j9So->9Lr8LSH-_!,;b3HjB^c9sXj0TP9*&E\rQE
#2iYg!.6384tL0s<+'TZ6=bn-!Wln?0*na4_YDTU&d>5$LdZ&1dYL4=f+IJ73Uk#k
"Eu5:]'r45+O3)K9?/0pL]qI<"/Y.W!d*<VL][Vk!5K,*?kPq!rc4b&!T7)bl)4Vt
r?^JFhi`&M$&Tn+f%Uq<Q;!lh+<E*W(36^27R._Y?lCV2`(G]9/1#s5ko<<L?q<\+
W+U="0_:\+MHFNZ60%UOd(hLr,R?Yj(Z8EG!,`!KAHh"*"@-lJ_K(8VG#ZQl5X7%2
L<:ba-^hMM8k?:5Jr!%9p]ABL9[>=_"\_soe-+]1Zm%^t"bP-TMKVEY!\pdJ;>p]4
VCZ[7"!C[68_=1($38bZEInfH?mBMX^,&3tX"X1f(__c,8c[cZ!C@bqj"!hB6j+W0
<.jlqTHZ#?B8]LmIY&>W:Z)>j:^+lBFJP-I(\V3G%aE3?W^X'A6;*i,PaoZ!KHOAR
[PGj1MNP1#[,>\l0!O"tI!7H"0Ec^Fc/c?A5!k5kG:Bui7&pFN%SBP37N`TTJ51-X
/=CKcbLQScZiE;PeSde9CXfjAH8O"Ui8J[-dF*7m+D3Y%.7/Oj!2']Iij<duQis'f
(7F[)!uGNIi[8;P>/EjkKRe-Mba3iN"+X&L^cVYk<5(j:Eq47)m4=DC1^&>.#!du\
]C3*8/;QXV-Ke$_Mpd,W!uQonE$MSR/OJk@-3`=Ljlril2DWgUG8LL."9;hc<Iuk,
O`3^W,(Nj_DD`Pk#&lpB,fh3B7G7o1N)p!VID@T^2(k7@Z)<CM+N`aL@`Oem.TWd;
\>ZQ&%S@!lD?BRm3.NO`qi`Mj<WHM9i3J._MG=5.Fp28q#;"se&nW[DO99.Z@R^&S
^_SL7Gq25p-3EpSK#LAn9_[I8>W(Rq9XJXb,@I9-@R>H(j8K7u.uY_`G[nUQbd@$-
LS1kfVdN4'ZGPR!HDp7@]O4D:8bBP[pCWJoR:f+q!+A&8pW-g\9-u4fZEAfo[_0U3
TAh7&.nL+HjTo[fJHuK'.27?eFp0"'@T[*1J5@nCAlpKm"[IL2!%9$+TdHYO4VFnF
>0',6).$B."$ffi?pm0Y4?_]F/HaiRd&='_Scnbe-@d9@U@NO)@[_mD<i]i!-k[g/
%2fVOT@anb;,B>o(k/Enjs(eo5]T0sKs^4C.<:p8YO[mQ,.L8I]!B,&_GenBj=I*W
j2s=a_L)J!hE#%ST93MR7l3oX88AL4+iHq2%sCL:3b_uMLQ@D2b`sWu#&sW+\o=ip
8X@cBNC`3,UFumg1_kNVJh\NB'o";ho>3t<MBTsU+iVCJ_G']S11&r[+eF?X"mGGI
2dSfg-Y;M4J7:#7VI?d02bILs&,n<(Ff,L6DcO,sKLB<:8BnATLuSo"_lc7M^>=Me
,/@@gJ7q:mA3]bpIYDSB#]q]hE*Sb%Lp`0"e)j.LfI^eJ=i)D-5Y)-1:19Kj07s6+
n&P_6Fp8`],sjjp9b,LNT''L%G(\%^<J1FK$u8JdFJVJ91"_B!.O1TH'q,_a5Y,n&
jQsGD?4gjVnR+#INWT(8J^'oRZ-@ad"K2_U+^2/89;oY=E0DM'^.F8;#=M.;6nm]=
ChSs-5X_#]2OS%;I:(0/YP*c]<15?,n2P5U+BAcreg'?U3UDRC`"E2XLd^<A/f0hr
i'JOf&I<V@)@Qe%6."gj$5!Gq+T^O-Zq)AN"sX.fO@2bn)%?b$dI;rU*=rM[Jrr$K
5TgPl"+fD*LeKlJ910qRUhh4c#6Y+EOSfYG#nD`D6BOg[?o\l,"JT9-:8q6o<U/Nl
J94+('$2M/n6dLVAHr==TV,CT-l<JP.=kmBBJ468LkJ)L#`qLm$H.U,@5+9!(PI[#
+je;:&/bcV_;Pfa7jo&\L]en/(je96%gI[g0d)i]4VA!O_(:nU-4pOf!kSHZIeG#2
#=Dp=W)eNf&;iuq!Tja'+;VcqFErR^.Lu`9CuFfMCcOr;_PmTa?K`pPlNT^#5d5U!
S=t\V(pKAe7tD5.Ku3@:PWU'##Xngb,d]f7&#TG<D#^]@MS]Z$XdbC]-33'[JO.P\
UoZn%TE#4L%^9?,TV0@[%KT=OTEg$U5S+'LJ:K<a,p@eN$,`F;)X=j^Hoe%;XOM2"
K./L'$GCDg0F0]>F!2bh5f/Q,0`^]4cDAq(8/;EH!+$']TQ!:5"k#(IaoXi>&e>)J
BL32]5d2Tj3iW`b)[<!f]Fq/O#XkD>P9=*FKY^J3#(_;4)@(kT"*P$S@*ga+.3Pp>
#_M!h[df$Q_@2A)J@](@+@s")'8@[G;a(C/"[!M&WGPR6"0_Yq&AWgrKFpX=-r(>-
6/<._0*+%7(f(/<56Z\dXbs-0NSlGA3fI9djFdMkB!D@:3"?&m;"I#LKcpVaKS#kQ
.qJdBWa_@u/tb+T!gd:U#Z)Xo/dm6["@E`Oi0&[#Z\[gaVZagT'FdF.O@U7CX3sTM
"<k9H&HUhR9(5\,1/U%^dkr?sL#MMtp4Rtk32*"T*1@cK_%T_gK`P:Z`r^%FlCak;
0KKLA5aX+PZ4KJ@%FM`#EXf[_i&1qJiC-*1[d>:pP!@@4lJ#<4`E<FR@/EP0K])^p
'8?P7=#3PN]oB>u!)p^U0?\#aS`a'C`HjlObo4.J_#7*#-31)Q$*mJ>LIf5=_\p4p
!2*L+JnTZc#H^6s!!Rpfp`mc\RN(*"#Jm'C-N_PP*gj\X#W@=ULqknQbi&Oq'F"S1
LBfIC]/+RoTg3]4+@-Q0Qfr4Z9U7#6)PY'$iCI&d6agSTqY-[6?jZrXC2'4@Dl?8E
-%P@ol6[03/eD'd79IdJhYL]JcN+#FrM?29=Fn&`$l0BWn"3k4"SbC1h#T2Vg"%Vi
E1g=h*:mJ>5_2$jl=#72[m1-k_=_NcO:K%rHG1L'liJI3!s*pAA&)al08`loQBK[R
!/cn9-7l;$J9DKTBIj8DD@E]`ct7gd(N8E>#e+j<K3d^eBP3^WT4/-4_'6QlUratt
+B/^UnTQc`8C<eO[L,<'?U)PPP6*WS#XDc?"X&dfJg1s>8q88m5m/+6[^JJPZ'PU7
XL\uY>3eIOF!=8NkFa%d$NVKL.&UI:J^n38!H9n"+GegOj!=\eX9MP+!!n+n5YmDl
Io"uX+/p%`"TZr:A8!M(!\d@U!9.\o#<>%Ao`>4p3XZ(@^_N8F<el55o)TsV"b=r8
M95jA,:0],!^KuuJN,7b?uQEDZjrHs:_P4s7Ck%J!bY6OUHu't'S>u&kfS6F0.6HD
[C:lc$d!W95`?BkokFigX;5j\$!5-N=A",nm4RS7+9U9T5\LI1#(Y49(W=WJe3"FZ
E@d<=(t]54:c!6ooGiKK0"bBO0it$t&1l:=,`nZ42eK#O!2'l)V2,HZ1A)<2ojWp7
l!-pM'ZL0qep:Qa%>>9W"uC=F#H)pf"TY8!!a9k'J8l)X#4_j0[4hj<!A+HTH$Or'
W!!u/*<OZZ*Q`7A>ujmi!jO<\W=nLcSgp\!m"glW&mD=F&L]+/Q!?[F9)@3Tq_J5.
&q\J-&L$'MA4b>.WZq6*9_]b8@0Di[K"YGl_$VI.oFEkBEg_e&1JGj?\]1uF%`+j6
"X)S@!iT.e^uMU%i1q:n74d,+&Qa"p$=HNWXGQ'>#"6o;#([WS4Nh_h>\9rhP!\^I
J?TSQPd]`m'YP%#b&o0VQF`19)U8V='SC#5eJdOnA^TJ*4N-6hWlK:EN+:>+L=&.)
;eB^iJ08sP?jm)J:6&6j[!%/c<$'D$#KStf5m3;9)t6=HMtD_/a1T(s,PhV.<NZO)
k'jor6I47k(jH$of9?t/#@g(@!s",jcbi!SJ^?(T&M+c^a'9"sb52=#H?TG+?Ylj4
;eTn(<WV\$!C/=Ba@Lp;\J!Hq;0Wes;9YG2A(KZI6E^N/\mPNL=LD7Y$d%jtaFb%1
%$ND"""=+$ZZ:G(%i?34?qGe*ePL,n9:.-m^$2#N0dt9R4#V<ZFrDK*>l`#i^KCG7
-X8F-!6be$70/LA!%s<[]>\PnR5m[>=:NB;H!CT)'8&abJWmp?0i2GK5\>t\:""\W
O;Q[)2s/^XE%M6roFio9?4!KKD$8rg&-@Iq$aJAb2<6(-5kD(O=Va2O!&@Er8-,Mt
*%_5H6GadQqK&0o$39!"h\LBU>u5?7"e`@D""Rc<#i3ib^c:M-p%E83@d"rRf"X.D
G3Qg>M?BM*`\/XV9EG!O,"?,('t3\5O81GXe560s&3-B/Y"Y,BBtAjREE>_F*X&.c
(I$uJ.KQ1k#&,O$W-FSf0;9K?+C5P.l:FP]M7bAe9_t_"2LgV[af7V)'nW)V6HEU8
"'&c'&9YDgM-e(LC'4plo,*$o&jKMIGkI:<Gi+=/nrfY"#E]W6IfW$n7&?l/^o:pu
B6agdP3&>^F/9B``(:(3YSFk$P*uBU7g1:t&j8<XN[_tg?tq)'!t]@A,q6DjW[bb?
[MPdITIN1a]G%e\+9W'&Oj,4AE1k\V%=sU%#1t3V2;MpS?a(.Daal0ucsR*J@cG(K
]pp#<.eLNaIAh[`JU@/E\dCt`"_rm)SNnm%N0"]g,q'IrI[Jgh=;(mu!6IidIV:uU
7;"RlFqM?pjg`-i]/m2SP7qU9$Sc0bf0`*n'<$?hcll8Z>m@5?cBqZ,3A\["g^2@q
MVu.A\/'X?*eA*"$McE]&<m3/KbT@2P4CW(3;XPTOWNHB\aU44iNAS6]n%lC*/P5`
q&#%KhCGfMJU+i;b%(Ms56/;A'ZcAoiP(se&YK-S&h(0gO;<D7JWK+:!LO`*:`(0L
JX;N!\Nh$`\G1qi:G<=f-2V<s\;rgu&-12CWCXIJTm2RM8WBqd'@NM;1[g9qh4UHL
JOn:fj0f6/JunGKJ:IcQ>FGtq%NpW6T"krQWHerG&$$"jLbeL`=t^/k$3<Ij$K)YN
33IfT)E"#+$e,?9,+Jt,(a)u3M0\Nl!1/eb;6\G7'gN/4T_=A=ifPt;3q*J6lO0W#
'*8FUP6!d#(_$N[U7)W-0;&f+<*fT5(BK,eJN+C@a]a8R)%3qeMGiaNa<6>^"qp_K
`T,jqR#;CZ'c>kn$d%!0,Gm'N#WHc-V.^,7TY(^>(rdH:0&cjWBZR4;l3T9k(I<0\
(nDU[+,E:>Ve@+r5bjq8[1<;3T"+X#+Yg11$]VC+R(DSi@H*j1Tn,0C(^h!)fXuc3
*f[]dNJ]a$&/kRGQFlB;J=0*,+i+ZQRt/>g!9bE1X$*$6=KCr>MLbSdd8l*#_*BH8
Jd<A9ksLBM$SJ\fW[J[7qCRW9h2K\o!I,KIitJK`c*`oSP3N4>3TA&Jhms*:P0b*J
^mg0(]=MAOJ2d`QRTI4"T`H;r)/'g.Odi$1,SBg-)E8?1>8@6q^Cg8p%G;qq+`ejt
hi"/B.E!0_d2E<BH(=sNM/mek8bnuhEfIpl6Fj8'HP6G<*.bUB!SHguFFXAUq$CKc
P<ofkaLRfha-,p%(>skDfThPCrg,07*mblr&/D<GHB`*0.DVjHkSA`J)ZZB/O)+iS
L_g_M;O&^l!;I<E,@?!OG(F$Ab((3737f9oJt;ZELlm6,)Db"D+LtU,2B14tHKQ99
acR,L!9pW)i\VF%0,b,9%%,lOkRooZ+r:6O%<:YF&SrNaZ9S6+&U8tr:mht7di&4g
3.ULLck@qOAMF2bTr>F@nSFIe&cocb!FQmup^_n;9,,>2La5ic#lBM;&qSsX'1`?I
E!uai)hC\,R*biXEKIh2^5Wt\4JS=(:^IdplP^Zf/$KuoBGA#HOJY[_!E^->-lT28
XqtQtN]7O\#oitB*!(j5J[*gb^_IPCU5>=!!>+fYM7SW@4r??O6GhEE=Iut['2L"\
#r%GS+I3$>fGq0].>)AoM8hX0MLc<R!HMh'GfhMRG7Jmb'Ip0lV(W/.UQ`L4P8#O'
d]<G$Rt0/=]nsSKb74eW'p]LE:ah/_[(1a7Ln!WuY2W<hEQ/Fi5lfoqJ\[/*a:Zk:
bQ0gcOBCCkiYi_diX'B"'1+nh3asbI9UMf?N?AseH@3-d_h#(]NPP[Hi5(FH0f9d]
c0u['Gf5Tr&HSur0S#Q3Ym_f6$4'K\!Y?0-YRIek;B*[l!&t&rYnDs<Fs9c8N<H;5
/CTF-Zd4#]:bWH4!#1DhY:1TX!@S.2$^Uit2^.+jU/=Gs@%adg&-7lP!.e7=:^r<I
7gnr0%>dV!fpE5mOZ'_:!;#(^fF4J;L^d1k_hcn\fF02O$_$8uOhdAa"@n#K0ajA4
,9Rp+SR2Co)P"]BNiBmTMPh?BV`m+LO*D@iW[Uj\aaj>%!DjXR?k%Z('a][8_RZA-
0H5RNJhC/uJERr'Tj%rLI(AWD'0,'/RH4G'*M*=BJPZr/,9[%EH(`VF8/YHbQkbRQ
a>\)%Y).ET,5r>l57kXd!CS#\8@Ao,2A&p!U_sZ#WtGjRT9`H=+fLTU8A?;4i$koA
6]"JXR04TK&Z$A,QUp8NMjG!b%ORnRYi0O1EKOH"g^h6XJZ'E:6iXU+quMaHY:((u
JXo<)_\p;1(Lg!,;?/-h,_6dHJ^>0r1cGlbY#`djYrL,LTY(;fg9+PPMilSpHP&\S
PRKeo%S>"`'+kTC*Nua[$@CGH!9Y?%"Uf?jJLL'he\[4Vabp`C4_\^G&Wi:t7>kXc
6kG%[Wst"qoK?/!'S$OLd_A7jkqEeYMXVC4YdTchS:KrY'N(!\&=4KK'OSZ/aUs)\
flRnu"c<`;J:J&mTS&A_&@2?Th_>V5XnmTJ!gB#OJM<r%=]jYKC<q6cYHZO"BZ^p6
]$m%e&33DjLqK@s<<u.>W(KpR;.(F.%>]U5]4/X:XmA%B,/9u=*"W[`Qk^-&$QA5l
an`]%:o"Hf'**+N!:UkWGT/?aUO]=i-&`EPV2DPD_OWC$M>HWLEWZctk7!QXf3'pi
_/V"LKn4N9!2J-(d_M'07=hEa/>cEY<!A6g\drLNJhAdGd+f.6f+$eZ\Ube0UCElY
quLc8%^@:NJNbb[cXJT)03aAJ-jQ@b$jnEnN2&k=B^q/ZM*g.NYiD8!E4dP(K!eb`
)cE2!T\)bsFUBOn7Gnl25cB7\(qSZ:(JkUDR[c?olkJ0k)$s$B0jL<c&-8F88MQ]j
fe3_!aK!,h*5_QZJ\R+&kF@D5NE#K`#RQ%.&@4!HN4?L'6!p.%Lan[]JR'fiN!G4h
_%*2pXGO-f3\UU8*.c:E*Ga4+N<l<KP-GWN'Hm[TW:nX0Ta@C.$kWE9\bA3G$(t*!
J:_rq-lE%X(7\kj56:oo5TYJ2E>QRAf]kN%N\QU5U&eJK'K?Q(H[Jr[3jn7aMq$dG
(_d_4%U66$'S/*Ude8N;F:qC^!MC$"a[HhUqs$@MQs,f+GS;)WQk#m@TDWVanmHuM
a;9.:,k5E(CF9PF;EMi(M$q7.&/E6R\r2[>=#g()=K[4")hD3S.M*JL/($'oUC'"P
OCg;_Aj9i-*09DgJYk1se=!Uf0r+LV!WX!dO;(o4QRmY"Mt"7j98jMg^57a5!=>,r
W:?GB%Z5X>&Qg(kn._AVI#F.@]=?oUB"M;N<e9S0$rM:%SX4kXS;>pMdi%Tf+j=)g
EWGbV2ET+q;,XIa[g3kS'K?F,5p;*[Z*)0CJ8he"5s,-fasC2\OB^1bQO+ic^F.3f
&!XPr!M'46C:I4sk()c$n/VP#[N"T7&Y\k+=j%`M!KA4ZS&j#U,KV#SfU2mEU?Ic.
(_mpklANFof\;44T`5=91V;ATMt5,un@]KCbCO)+,#aF[_'H4tCqJ'MP6_^0WHf1(
>oM?0(/Y10QD9<#a16QJYiGdpWH<1mZ^8md'Md`umaR<ZN]^.l!:sh7^rqsp[O0!&
S"Uq$+aFH8D/K-`]Qeut:nAiq&3oZBTJKR^Qkb1>(^ZUM$^<jrkRXBL*=\b6)pR$=
fFjC(Out]7R@7=+M1m=F(QQRpM@ff=R^<HoH]Rq6>eC6q)#ijF?r[71.Dl"=-DqYi
#m%7X!>lo0F2"=(47_(@#_:unKP:t^8O$ms'DA6`\[n4>W$1:kPR-Lk_eDW/FIF?C
%HT@,o21J2I=V`(1LUCAf\SW_OpdPDQcf2^,Q<Y[Jr)3CNcX$9MEoUR<7OU((Ld[W
8`]!dr"S_Ma""<fn-tghm[;IJ!9bLXb+&L`jGfN<ZO5*@+Is2c%M,KOJ]_JZJC(]2
KaBFJQ4jFe@J#WMp<Ii*T\Ql2(`#Qm$m3&LJoD`]W#YX$k/A@2XKf0HZ'H%WQ_]hr
Y2Po]p(SE*T8\-C)8HoD,I9N%LafV8f]G$kd,#0#CbqAVPdIc[cl.jQn.]l4'o7d2
2ER38I\g2a(I4ChljJZK)1b)GNTPf[Bc,rP^'u!/Q)l12YbVf9T*fjP'JqHD&j^bI
L+]d2&.Z<BOW0KGNYAG;PGea?U/@(kfsh=eN):k%Y_-,p)?F$&RMkY00"m?\rW0MR
!P3W.gPd`c]UDQ6O"d>[&mHS18Nr^@N09QhW0`g#d11`?JKY[=!6L4OckLN'V&=g(
Vi2!teq(t.#Z5OJ!C]m,(^SU\-$=pKMWKh;9T7s#r+Fk]WD!nsqONf`!=RQ6EA%c,
b(/u3#K24V31reh&dX/";+U%k.1h8%JWRrp7Oo/Y"$p=^9IV%o#mMR#!/Nra&;\7k
+Xk!3.M3!l@K?>W-6/8-"@8/8G%s/J"[_1@i+O#=#R*R=Yi'=Q(_;E)Ts2=?4>%K[
_mN=NFA*ntMut5s!0gMM+,pJh^rT>"8JDPdOARun6$EeC"+fuEKJF;C?uT41+=&3H
#m8"On;phn(^c"Mdm3tsBJU9W_>rjd6Ok1LKRs4aW-_2b'8Aj4H44i8,88;>Yoo\n
*YY4P"_$oaPU6tK"@7R":bX(-$ACfDd*@/'$'df/=Fc`;-lB4D_n'Q\GW4=b#/]1m
]t5I-ZAGsjZ!a@t-kXORiW1&\3ZJ_<`F9+F;lU9/i=K>-.S4#A&-W)*C`3J.?sFZS
D)+EpK>B)?^4ahb@N1'I9,n?@l9HVg,)Tc1&Hb;6/.8pQ:f*.'TU8+X\ZqpV&d:Te
F;T`a>KR8*+YZ:t"[QTON26OO["/=pis@*;J2e_YXl*;FgOdQR-k!#3@R@;Q0q2/q
-@kZ]RKN&@3YoMGU4NWLWBs>s1;OeW`QDSE/.VkL+C#7G@!E@fJM7()(kX7+.*2T@
0L?>D6!-M^"=_,Y'aJJg`XP";ng,X3JFel&K7N%,&\V1;e.g!'48CK25eBJqKHVTl
mfMnO+:'B6/NH_9'9GHrL#Gj#(^>e`0F]4^&5&>(O3goCL/Emm0.+-ORLZrFi%,=j
oAsf<"@0aO'rc-X;B?&DE*O0onn9qU"2P78)25MD9a$/OkZ/N)!Hb#dJF0biV1Sc+
4:"Q0\uTE!C*5RG]AVe]DF.IH4;co\fI-uUYK0jC@bB6f3DD@$M_)%t#\Y31^sFq*
9[bmu:El&Z'GC[K<3km88ao0A"0?O@'S@na8Qu>/C/bfgThnJm?XYoB'a@5sq/-:6
\6L)10,fT6kS]O3&;S(u6kol68irooaYLl7eI=cJ]7NgV<"fM&eRI(-/q#rRKOG]p
]7UPr`lWp2fOu1W+^d2=E?MDd%g9`"mM,8ZkYrH*@F0.JaqQ(]F2^i05R+KR_Nbho
eD%6R]+j[-gSeO/=r7>/:bPU+@1G&]Uk)!8'ZFIsI"]a*%Vq#u@N()fKE4V+jg"/k
2ZU://NjfkE!g:RY13,Z&qnhbQkI/#!'\&J=r9dE"[RBb+TdncAJhsci*Zl,q%j1,
OGK<,#"F.L0aOY,P_*jX6U?MS"2n"GK7I!6JB>nn5Xjc\ipNR-3%B!"oGam>9`5"0
U'0E*$)8+sjadC_#b_5<\]%[cJX@kj:6?oS?k>hal#$P&1^3ra(]sbg)'U@i/JKF3
:s=MB>De\DZ$<?<MHD)-+OCsWQ7e&bRl;gP2*Vc&-LX4"b@XA7k:rVj"lMp?.:d7P
S%qc,_5Z!ijV4SgefnG:!T-)%]u6hh$;$%P:GiD'rW-Cd6Jl7R"q*/c!amRP$:l$:
KV<:MF%lDG0J.Wg@:Yq5>RCKk2?k;F*ZdYD%=qB+9-q,AK(+RlM5mrdm5,R\OEM&L
&2j^MRN-p@>f>OY*\nk3+p-s4$)+s/+Fon%(bdiK;PJ\;+?8>M5T0bt)U*E$GRGOI
&lDn,A47eER?ZkI79'%-ET#1V18>sigE7FtUfCU.:dteWabKqq+c.tN8pA)HaTKg/
LB13m"lFPDG<k4)!J<m%d:$!-9MTgo<0\.n6$K,(M+3uM4:&a.S0_o6Q3,De]oiso
4663./]G#=g/3;tNYiI^e;R!j3O8l9NGjBpD@D'T4u,Xh'n``0%$p1,;<GY3K<sD?
9:=P,7f3b??p]4%La*)'4;%_*7&poe*h&r1JX_=uLd8'"@aG89`fjNJ$@@VV79q\^
JeW5*\J14b8CFAC:r!*G;H0ni0pE=F5Ck46#A>4l)BtJHb$-?%BoM/)=WRkN!#93e
&X`\S=:AB$\1nCL'i%]N)GO1R,'%B(-?mnH5kl^JM\ZO"3[1mTW=&jembD&OMMY"'
%TAGlK-lfa<9/9Y#/J_4T(;;N']RLDT_KK.oh8Z@q>g_SM2),b'%@:;.T=>h%i*Pi
$,JY?^'&#cf!#,V^j?JXBZ,q9"25%,XIF/==l,O!!;cd/9dZ[#PIq)N`Ruph@fUs7
8TT?(,hZ&u+M8cu+C(@8N1.1)Q*UL7'QV]+2,VUL&3,b<6'LP!@6cdWS9bBY=CN@t
8pT0gA:f,YGU*E"^_HrZ;Ph4.1Rr(:',`l*9bZp6-H3Ld?q$Am9&9oPG!m"*Qup#,
e7iN&W#DHgN4o=.h`CuQ%Kl2EA4[s$Ol2I[RV$1H8r4ntlP]=O0K"9/9Ld$V22)&m
!`ot;9:TO?d1hbF#m%;2B#';K/B2<@n`g`9b;R$G:cJW/kUm*Ja;0DI9F'`2b)e/7
LY!([8(--(;1O^,!Er6^5fb.h8;%3bE$T&rG&N@1D=9:qdt>t5I$oMl)[#X?$J=8J
bTL"#KRdhu9T^298j_P=Q5FQm<,&6DkbkPe543tU)52!$+G0)\65S9,#U'0[K4'Lt
JRO$2oDBF.5]:%4\/>?5>s=Mu[Kga/'6[uTbd^S&#Oel$:k0r'PTVdbZna<:DR+XO
6924Xo8?J!RK9j-m@iJq<?bO.DIR)oE`<',/YHVf"$gB(_0@V)W2QF=PE:[[fuZ/_
oY\4&:3)kmJ'ciT\!a_rb^fI>,K1.qJi7WSfpP#RC=>u(;k=?4j(_'e`#41p5R<]q
1,I\s'`pK9BpX*B!r(d6X%&DN$=T#bENla$:eLH.a>sNuU&gkt94>Y0oNcY)I]'tZ
$g&!UnKl02^E23l058sm&ijtFBI6S,=9XK,EX\eK1=K)k&-3!AFXb3N"JR7.ijKGF
q;iNE%5B[BJF;&G/M<pRQkaau,RBWb-jPRh8o"F*&d&':7l34H6tHM_V33lX^h=9`
i3JRK&8h_'N\i3C>gZ@l5'U&e(h61faXe58>=ebY"H3MHO]L&<8s'?E^d$lEB:8pq
1e9,,gW/krV[=^/[Z][4HXeB*J9V3K8FYiSmD;nd,MqeF:'W%LEbo%cb04ba!XCu6
4(S1S`[h6&HopA-]ZeMN_PV?gec9(b0kW$l#>diVE.<\l--X6QUppLL+p$t,fRfKk
6bY<`9N/f[eUpgL7NMV=(b"U(ct-\EBf78-KERr%"_rjCN,8dD?L!-4!mP$Rm0r8&
GW)<Z!s!!;,C[B036%[T3s@N8YC(\+,$'4\ihAK(TJh&3rcW#T"R5Q(?r/I"E)NGX
,%=(G!),\WcrPa!0'&6XJ0mMckQU#l&]+n+J3:pC."Yo_56LVVE?&)t#0>^p#,#E1
!.5!D=pH0N<5;&Ri%P9>63X$@6/ZQ*CMKt^p&Rm>,G_3E6T/"R*;_:S"mI]BCL$Y>
S1JTu01KIt+AN%d*)I!t>g#/g+=$tq'ELaa$6kW7A4B"?hG9,I+CJS)8qttD@S1RE
i,H]fltT1'Sd(o#oY=e9+<CQ6?ARMY+CH1Ga'uO\+Ec_K?D=kf,HU(K/4F&p"G5@T
//U$RW%#mk.Gus^^h-#F-<8/M")lI<C_k[`-G:No-AVjs+B7-LDGfJZ6F'W76S)Q\
l?GtG[mVDa6dS"Aia8Xm"m$XKBQsPpHE\r63!0e%BT"!@('/?.,NF6l$tMapc6sl!
Ec;r0@h.O/4L<J)3iU7&+:nPUM&\lE.>DG+WWkR0=Af;@V1n7??rd;Y*)U9g)'a#[
iq<MJBO2<PD99:3i+e(rU+q>2M=(@3!$l/H/-BH%")aQ"@m#J*P8<0V*5e)%6AR_f
ALgWJGu4'D`Ni16k*HN@1%I58,-!Dk4p;<h#,APh?toqgkUE8XAn#F,:>CffPU(j.
VFG<]KBNI=DFguo#0078,A^e@Y*.dt^BqM%+;3$K=98m$8rp,cUa.s.,s09GWsAF>
K03L[U;%>Y"-6C^.#9=8no6!e0`jC_@]3bWqD(Dg&ED9Yb\Fn47QKC+"iVs<b"f"q
<>d"s!T5F1$XP6Y-;&m0Gp##."@U!,QMTXEEap4nDWj"Z1'PI@Y=]#u.L&$EUrl/9
3<J"-9UI#VkX]T1#!c^/L=eY>C,Q&Y"pN:9c"mOo_$DcceVE]Wk?q`Xa9<le#,#K0
B1X(6M`K9L2uk'%?k<>/ciG7!!98tE+;QR#3-L6%9ZNAjKfW/q-j3p%VZe2/&u-p2
Y`'sd0CfMrOj5p8^je*`2*un8anS`Olm5ORFt=nF`g]fg0E^Le4%)E>-a&Tn9Mm!u
Q:"2jb9Be1)[V+j0-Dh@Z'-;@p][=8"lbnUOFE](2+8b$<^h44Uo$7#8d#:l8;,V!
i*$9oga7P<"_HBlTQ&gs-n-`7?`Yg`c3BGrqF`/o"A;M(!)@Wd4uee8:m8(&?kk7*
`CdoX(dK,dJ0Kl)1d!*;Z"VRV6Fo;c1+>PYN?dI7k%n]74>IGC3i#)7Km!NM^7C0@
+QE#?Jr"22eP2d6?E*l'jZIR&.Q*3;Y_kbq&h6SlK'0K4-6pZqc;]<^<&@8;;sr!;
?s:+Xmo64UT]Ra&:0._)aTs]Q):D2?Jli0YfKH>6Ao(cWi06TZ>R%(,EafL^5[[#N
q!%6RR7[ZVKZmTgp0_aQ!=(:Y[AQXt'KD5pLnGG1mCo)'I'[Ma?>"SMD&=p&J2ZDO
TuD:a.5aZCMCG2\k6plDd4\R29P?<'_<*:?At[_,mVdW'AP@M)K"#+W-j-5[$73DH
TL<-;ib;jqKB'TnKE?>T5@:_Y2i#$K5\(*d0KZ0[38dW>E]?-NKUb[:<6(7*a9F9G
:/@j^<K@(cK$"5sE,jn6.@+:?J7o2,O>l)I.Dj.1J2K\N6"Hte?uVjm-^4h@cRe[k
3RS+fPeBfTOEjY&dc7b;Bch""hc&G[.Zf9608i,]Jt)sE=#>eoA;iaXbXPD#B$E)p
UL6Q%dVWu1"p]le/d*]#!sEZo.O^A[1:U%):^2SbMK;$l%!i"d7h1,!@RL<2%gt7+
9L'kXBC<(>PjDOc(BFgNcV,+Q$f2!h4>h$%"[IA<M#s<++L3,?#Cp1dksR0I49Y:i
:F)lE"!.N@#>+t7d(h[H'r-$s&;_-++8)gP5TD>@j>B9ZNhB!@#?V$M)?FUZ!rsZ9
/8CZAG+1gP*5ad7AX3M$&tI"LA>!%:m!;Og<X'1Y04XPW^gmY/9X-o\;'R>r,l5*h
'MPb'0!!#gLshh%$=cO=L4b#OAa0GLA-VAX`N7p.6C>CGcm9f:GD\>'K=$c9RtHY8
,c(9N?o_nP\fsC1#XEl)Kfi+4cqre\XTG2N7>S\ij\TI,?urLk8\Wo8@a$-?f7ZLq
6\mZ$1rr1?"=;;4_NbCHZ!P3]S-<sUo'm\B)*A&#!i%\'"SA5B?3<G6R0g1M!&Oj=
bdO6Z"iie1!-Z4Jk):EV"rQ2H8_3#tib#3@Zt!RBU7,;AKo&/846@M^aPD`So2Vo!
/;+S4TPGsD53!((SS]u4ASUd\4.c0je`h%_a?EJia>!!j2+V0[X&(a0;I\\g5iTM0
D9`>??j29%Be/s9?m9!CYr^p(!m*h3U2&;9M0ZD!+E2u9?rdG=Ad2CqRj3U<UMp<c
B\5.D3'\;]7P$>\,f--A!TG>qi^c9V@0nomTL45XR+<^c.;5\%#,$&B&i@j@33_=K
,%P.aETk6XYY>*c"orHa7sZRnka<=nK.;a%.i!9qJZp7@"!C&;:2*9r',`XX11R3e
-B3$mOp#\E,ks>$'-8Gfd8`u`94nqe3+ENX<Wm.ICr42%!mROZr!/m,XSKVa#h+Zc
"othq>'ZhDbUHK=U=Z:o3C=L:^`"sN<g_q([:ON;UDG_m@b_+f[mG^(R]81IdOL$$
,bs?&^eOs`Xd0PO<7a81PLMPl-j-hkC.Q]l_Q<pX+]HSUA8=+q$T8+38d$7n!aoCB
M&Z[1pNLj-<hN7mi-K;!7R]A+H,u!HjI6eA=h<\p!G,qg75$JQ,@%"PE55^%&1Z\4
3+&[S,jTM:BaG:4.P&@C#RAhi8!NoUB$P':Uu5.;^i#(+:-dhZK/\Xq:IG38Km2H3
"MdBL\Y^t=LE%EPIljcp^c)NTiZoX7@7.1AYaQf4@PNKZ.O(C[KMX_pqD+0>TFH0;
VIHs:@1Fm'i.d\$^fgr3^]NYoXuN10%>+oG=OEU^'&Z]$8KJ&NOp<K=YVnteG$\[7
"pG!@&Ed22Ll=p)b(5M*^a7:Al&;62'dIVqh*_=Y"nmQ0)Lu:l&o(HrG%,%I!]7tR
HXKC2VpY_1-T87i/;!_p6XW2&=t9h!1;GjT?tN!g5Z_>'!0jcDO'uf*Mo?p,ppc6K
i%L#k=[],N3I1s&W;90&<'%*u,Id/jkc.\ne26!5:s8Vpa(@24[PNMr4O_.l6RH.7
_5mc=S15O4#P+C4ON+W6Iiq,aaW:V9L'M+%]B?Q!!YihP:*kr2?_A;?[\>V%aCkk*
7GB"a$eilMXXF7H5UC0Ca9ZQJI(cF)GTmul^gkm+THdpG"5n&#Kc^lcV[mP1.`cX+
MHL"XLD,C8#Cpthq1.#R2Mh1/M$m^2,??p(s*8+38p0V+!u&mJ'\!>tBEOH?A^&^.
oQkru["tSYW0h$l<l,XtY3$BZ;?c:doKY)m"Xsc]>KoO@UKA/N?Cf(;;^=ISrWb]I
"or,PKX"4jD4]0R5(ZrB?q::ZB\I&?]?S'>,gJKG2S?%jc9dt^i)Bp_^;=,uVk@[R
@Kk2uRKTTh70C__^i!&a2aX0@bU^m?^jH<9F?Ul^!koua2\V`iDFsK,0+A>01oi8_
VS^4`3pF_*/+]DV.TVe4@7hS&3k!Y+(SEsPd)kg[Jj,&pdg)k:E!'-oa*)Gi7AhmH
`ic9QcNjT-hG9[l^*#Y/+=JMFADd9gFRH^B@UbUVq?@eJS2hZU!hZO1(@[,5-"Rup
--QE7!"B/8_>u?hA3(cbLP'#SYZrq'&-rBs^sHUC'aobKU&cC4:aZn]K>K?&]NQm%
a@,$lphW#B(.1D2nA(b;%u1MsK`ThB5U@J/#=;i9N(>6/MFBi48;LLs&;Z"6:^(10
#H\%.+M`@9*XN%(_Vl&f9I(,QK)r2AJ4(^tRbGTNd'-n2&.HP:d."81*")pXJQQ.o
3n=iL?123PXkYTLMZtBa/$7A-"LA75iOO244<teu6@g800Gk9+"`faQ&;3:g%-'`"
&P..1+VF&D,!eK@DBBAp"BTheBL4$\MM+:s#fp6kKni$H_!#]L$fVH1gtoPW1`Yoi
K`])5Hr]D=a@.;cP[df5TEiB.XED6;&Fp7K6;3J'&Hs>NBGH2^0MWC<:]O*%#_9fd
%0Q[@,ml,1@!EoO!Ot`8KeG1q%KkqkQ5p+%J8u8)i:rfQ.gj'#!e?pt%'?b,5SscY
JAab[0T6rIJLg'm&d<ibcmk"W&l:+d1p&/I"bAFnV?DH8?l(#gm!9Yj]E$A5,m+.+
Yqf"T80eQF5`dW!"TaEU&d0?8*k3q@UT3U3+M15S,L35OTZ'YNRc4Fbddi-EY`$"'
:uJ93&;FU#8P2m@\iW/,@-BBm:LM(d&d2Vk9GKq!@R?lDiD<Vkae6F;%"p:40Y`1S
J2j2N!?bD\K]ouk&Hm[+;MmD/8lcW0@DFf/"&6Qp&VLH===+8,(hfq&aUh,Y^srh4
V1jJKW#\=L\./RG+=(G6`aDUa#m,q01'[hF5Rmp(.ccHkJNu1S'4+=h2#oJ65U*ai
2nHDE9!XNoJh6,^.#KZnb0)3UP,f#"!PjLBNjhh@G1qUb3Zg',J>5jJ`'G:S&HlNJ
T0lc3RLfmZR;Fdf2.5W=(g9n=(^hMFe5YB/+Inl,A+"@S]sJq-Lnb)-:dPnN_,sL9
:*A[u_ufA5F/oGd-o?nL9uUZ.c:F<d&HopX?jm*Yi&$S%8q;(&#!;PWOgXnKg=SB9
-p/:P!PQ\W!<=5F!<?LJ'jLi7O?aI1d%D3XJ@AP0!s)e>'FY):qW%oV.-PIbXMDUo
#KV,%Bn]ma7!&p=E<%uW[G_HH#Q\%*[s_]N?lqo&FJEm4Kja@LYFu7IEnC/=0O,:q
i92kNenKl(d\ME7+:([AkXHPFTtk7\\sl0X#l,lLlR(kABK`r0+R?\sm=<kT"G]5Y
&cbZ4fn^V$-W/>4+?0XY!%0Zm3/BV+_!+gdSgo9S(';s.To6u0"2L9@!oR5j_;ec*
B#+&0K;=B]+<`-5\0D)g(up,P!<T2r$QCq:7fa_h"e[ij\^s"F^aef#W?_n9B=P:!
TJ7o]9FV"V+D;S4"tP3D#eL'X6&=L(<tG8Y)k]Y'^iE?Rkfe^AO:[JgF<Gj&:_Fd8
n4*t^ep2,Gjo^]e%,AWMBdMOD!EcB.!DHEd#j`-^ig:7mW>I;l$jalW%$K#k#m4b[
c9%6RDH_Wc1+7thK)eqL_%8.qB2n+G0KuoFoO3>ZHjkYfjDa$F?O'uo'*8:$QJUOB
"t-2e8,t8ZM#\t1+RC*h,k1O8J4EkFQj<\""Sj'qBHdt+%@%&%#?S5?N?Ao;Z01%>
;90J($7HI;G-#eD8S/$937Z<))UZ\u/-dX.0+l4T;9If(H]$_h73hkRJT)`]k"+`u
O?QNtF?CcWWTBWpE-$RCC]o9Y)$9jo7Z`uI+OAirQaIqB>C[fj@)Thr`,\6di>!Qp
D+Y`rZuG,P\81#&bn+Ca78:iQ"sD-ISRlaDe9E5A<)A9I+?g)tcn?YpJ..mP&.-1o
,#Ha]`IW/<$pgO6"b;,^JYop`JOh*lE+n_sO=UVT!(I6S0EeFcjD$&((KMZO)$;R!
#N<e%DU.;]!AhMb$?9W0TL*+Y,51,h0ITQt["Cq-S>_!p3X27M)]:ZD@=],j",5S7
0*RjO5sQn%i+XO"F2C9QOcfk^>tucVb3pBL.Ze8(%@&V>$UMil"mA-j(.<=qg3F?L
-^Y,`K,6QL.LM1j`;3G)+BtH\'8L3lhLbM-.Sm?EB^HrX+&g&f_@oHAc]OboTIi8B
O;7t,^`6FK>![]&-:#AB&qVfT$=EX'UC"XQ'nQY=?RQLD"tcRXO?cBg+V4_C^t$lt
GQuX/=9?8qd/_@oOt,NT6m0D[i0-/(_+6?e(17nNZf%C8$i:+N5fsj=,Y'HM.0H5B
JONL@#H8T4"XKHC`BY7Dma@AO:"6M#K7l`d!X;#BS:Q4k6A#;8/dL=>WKg(2$M)Rc
Q2+AoK>f<1_7e8"VStoR7cFac3<UmfHLYW'(m6N[8<r@;P(M&*$*E\5:5Q+%;jNkT
g!CrI^sj9T5\(C]P2?Ec[LL`A[R;N1_$.oi";^dA(@XnD[:pp5_j'AtLs^V"oOJ=0
_[;D3NUJMVBU@,p^NL4A1^9ml)?RgGC78=Q+mCh>1iRIE>$)[m$+p^u6J)BI/#<@K
ZXKRAXpBSD2m]a]:.)6E+W*Xb;!f:?[;\NUNToL-5gZEki(sbTn1+\j1u'Vs7Y"h(
_ZY'tg>%9/0+lsg<'\)=!p`:Fpbk<Y:al04ZZDar?mBATQF;o<o1jgr7Kck!*Wt>L
%`)O.ZgG[I!u]_sQ,2!@A5EsTE[d7/8K.\`OGd(M%arRHV#gc.\EIImHdN*8N9LpY
+[i_nJJtnn:5FlA,@CmFJ2.8YcQS\H10dpAB.*b\,;#WU'[jJu+@VCf+(H`B^r\kG
mEk_Hdc=,k<`=lW[*VF?@@faS\l<FEP>p4rB!$on==3AFJW(:1i;b2c*W]*I1df.*
+X'gXIk=WdVg+3UQ9,;XiA?EC;YO6L+TtSu+(-ZoZD],T!8"/-@pnm8R8[9WA:u%$
86*sS#U9=G$+u1&7&Uq52(t6E(kt.I9)4o."DA:?cnsspFB`FdE1d:%7KcfWM`so-
.`*`XZ.%Ef4?'(>l,+`D1pA805jTMpDS\=nlUGCJ/ENp!d?).^(KQpi]_f!B6IAVf
&I@d0JN4Eq;?@f"R38Jo&/D1f;\DAb%Ib$kE8<I8dhLM/M'.h0W"f?C)i]`04KoP@
qLPq.K/8mj&$XAC'G\Gdg6ml3$Bp0p(`8HoUnX4`.?Ut<!3:WkdX`kAJ:m`Ud2eEL
<ZMcV$pYDf.Io1>_2PV%3O8mhi?fA*.[*.(JRB+@8h.EFq(+<,N!%4Y;!Be<+TWDo
J;=F1TSj1$!!,%u6\$;1WA98Apl!9I^^-p.R+e2u'!HQc[eTV+P*h(MR$>eGQ'4iY
&/Bau)i`oA%YAseZX]!YU`5H!._lXQGg;;LD4;(O!D@[-Z"Lm/c7#H?-/nfR0l6sT
(;1B,MDu4fO;YReP)\.u^6%'6OYK4+kCAp0!FPm]i.M,M&]+g^#Ut$-L^BHi"Vn6G
'S*?B&oY0,e/p+H3O$%'=Lc7>eVo=;&n-EsY`+UY!%LP#JNPZOfWkuQZN5=kLb$oX
C5mdp*J*DgN%i)+C"SWDR7C,[+>DUt.6R[+MkBdtLhS\+5gG[BM@G^N$$n<8n/[^O
(Dc$NN.G/&OhupA&V4?EJJ](Ige0VYUD@n6V0Si$&?:h%/>Z/Y0+jYn1IMOjb_Y4C
!>#oqclE/N*!)]SJOnLhRd7*/X!Aep%_;HZ#R)(?$jem)3qrlDYoJ;X#ln'1!&+P,
:n!\h'nE74!((Zcd?T\Vbd7bJU8id(3Hu1kWhS/@LdHZKMp764@L/E_U"L"YYr@4I
=1nm)!E2PjTFm>0_`i%JXg1$=qagg&8Z#rs#YKaiYRUZ3#CrMk.cT2M)'pbB*uGlj
JZNpX)7P[34;?k++)o<,WDfH6r"(X8&HVp*l!KD6l4)_QLq"-J1#A"RNNUZrU`8,!
@.8^A(BNG8Wd'`FJ/SFAoU,-nLePsA]M5!UKGp52JKPb[=:#f5",c?(!;Hj#@+D.,
*Ir\]Q,&>38-U#`&e-QDYh>&-\BY)Z-k/f80Na9t5e)W-*4fB0&J,\.J0bY58-+ej
JQ`m6d#L[1U]Bm$(5NL@CCR%a:(gA3JJ]:+YSr&u$jeDC&n2D+WE]FtO:0F&5g+tB
J=%!IG`7Ml*U'M\5TG?t##(N1J=mN9@#5U1D&V=J!N7%?YSSU4bb1(O]HnAe@9ao-
DU+]=%\e'W.-dTNbs&oQJY3e[cl4DfiX]g\-Sgd6nspY3*0Tg1'*B0SJ-^[&FoXq0
!<!OgJMn97NL_TD#WN3[L_)`M_%N8N)I[m(fYaVT,R]GU*JfK/OLQR3hj%"ZS)FX(
GT6a8hi0>8!77MB3t"06YQ6S]R,"YM+n?G*$W%.54YRQNW"T[Q(6>Fi!2KFo_oti<
678-,66VVn$FQD.%uCSE$6U+pOkqYsnBKa<%NEe<fGMo\'*5A2UUZJ<MY,E7>RS@n
#a-XK.#:%>*19.3#SR95g3%sS(kD+DUAMRM.G11`%j5O'JVY9GqB65.?]j*(JWUep
n-+?aj,qE9)425"+cEO<$:N=ZJCk!k^on<E:5Pr#)"Xd98^tne"q4Zb&;UsYHnh4#
&qO..;A]pq>2TDh#dl(nQ,P_>J<,7X$Vet_P,JSC8CUGFNLN>pS_t4`J.ki%&ei]E
MX`_Un@Y$bJth$?:2F_naM.`5oS?Ag._t=2\Cd=N?&trM/1E6S0GOm#od/7WW5o`8
4#eD<n"?$Y&=GA5/1M)b6NEN)[V_EKP*l=b%C3P"#Z-[N<6J)4&:n40f[/+]U+-Oq
c49m`(VmnNW79N4$rp[P\j4]]8:d02-DatH1u[)]''6COKF+Tc+itq=Y_Je(G,So"
JKP`!@I+#FWmND$'4&L3d&Il0rIHd7U(G-U,Q!VP_>p#,0%(./3$>"9,"jMGOJA>%
&@?t4]ngKVT8:Nn)7ZarKXmN!Lo?&Y\Z,poEK)-47mR4XZ2=oYhRu9-Jc[A1blk=5
SIs87Wnm'$ckMY*.pcAQNluLV5b&nRN4.aNJN+[$b:8'.)1^WF'#BV<4j5r1$5_se
6`d'`ckTjW/W:+;4Xr.a:(?.74CI[E-!h.Z=e)h/jg3'B("lV@g"_Mt&<0eNUqFdM
r.)5\'S(cqW5o\iJ.r"fhk2`2)Z=!8#Sahj_$]tV^!P2c=WIm%R/sR_\]eoKJ\)7u
3goc)Ok('X3NN5eP`:j@f;K+R=</WT-BSSi!D&oa]?S^D+#V+S,+u9#8M*I(#*g2f
Z.^4Y1"@iM&qP<u1uJ_W:_?3rrdfA_J,q)>*$CVGILO%CQr"/'_]k]25,\b*(s1hj
8s,+$0S(Z,_Y"9M#`^<(g#3"Z\@WuWR8(b25QLiu_>P11RR*(l]Yu,@1W\lfTGPl"
'ES!sNN#X3,']4Y%KRn-V`S<^E7SA>X@)K\RV9\#R/&A)kW?9e!HBbDGU%e7(kLu&
>k*IIO:D;b8M]KP!JJOd7R&WE4?)NR!>lT(!#<CD,``<r(6B+.E23ODEJSUuJERpQ
!#lL=(5O*RVr/*D#T3q&'EH2S$IZJC;0sM+5E$E^$]p!9'r!mJNaVu)_1%CMlrarf
*L(XNNF;(.^6FY@9['a@Sm'LD_T&NP_NVjVBhXaVb#P"s;'7ZRMG(O=.Ip)GIRud8
JUeMM8<4<:&MIkC,`=+=6)D9D?bcC*!8nK@p`:S$(+ATiRF$W!^_;9ell-c\)i,40
HGZn2]8alMJam'.U[/`jQr-,&#l.X4U@b^jR7RZ!!PfXY/2&U-)N]eo!!.8&8Uc1e
)4,"=!2'K'7E-@*F0i++`VpFIX+d*"Um;HQV-)__0^/t_`i<1,aZ,.`kRk7/kb.pe
-efH*amb;,kiG^"RsnFiQkU\-f=j<QX_EW\)GVT`'bq?n3[:/X"`Uj.SXBTgN1^a`
S1K5"<LW]A_\okMLl[+Q=95??NS0\[)$9mq&J+p_!SA3ic<(EE&t19\*3l#an/-_T
&]?:<X<<Q)J0##!'.VqQ$uh3W8;[Ba!^CI$=AZ+?$7+"M_m.oO(QO/W(<m9Tg(k0&
,8)m'R-TPo3D5U^NPH;0i6mToRZ5^/@1nUEd6I^L)M(MW8O6Ml&aP!G!tu6WQ\0/q
]=OFK0;)H?#queh5RINo+:JOld%fW[d52@6N/_5C7*lPI^`NT>33Np'NSs4CR-mdE
\f`]&Q6q`FW"82j';^n.$@!)t,9_Sn$rZ$H!Dj\cGT%5\k49]1(?&)@g)[ADm)0gO
!O7<9JJo05Tu0FNN'SuTS)^&34)gW^X(ejFV\T;X&e>8iB`=<]gY'4_6n0;j!CY(=
I[VZnjV0i%)dHMa&P<T?()4"B7kbSDX(anM*01B#W_l+IdG3p+'EQ8iQcY5SkfaE_
r"Iq;.`#a@)"*n*fIFnk+BXYTE"N,d'<`Xmait'+oc58"ni)(=>2lYIgrhHjCWm8j
$Br7VptC;=@1q;IN,Zi=(.M(<p5D9[Mc>,cKmf*aePs@<i7eO.8s1RV6*RXUS>a.2
/(r0C!%hjrPM(5'Ye1Ig32Ne'mqS%p$qkYuXg]aaLeuljJ.*'B0"P3t%_8jsg,P,u
BSm'3!U(2s6bi\8We!/TW/Q>3;.j;a<t7od!O62t](/:O'`nM[!Kob=R;Nr$'cK;Z
PA^&+O;3XU,mgRp)/9=i?kY-EjT1GeP`\Y$'X'0:WmN=l$R$Z!.PhH:AtD+-QhH<l
=WiMQP/)B"/#-$'lE4_9Zn#nEVa;u!A'14]/I[T^'1iau@Y)WbiV7U3]\nX7.:%MG
*J#t-RmV/rMU[P$K0gVU#a\Ps6DA1."kP.AEkcLW*i0;riW+h1Li$Z/J#A/hWiA@I
8-kst;6*7VFf<QE'I]s^8/FhlneTU8)K#.g0`XY-P_h(0J^mA]'*a#+EA0'P&udEO
F1.Hl\]hPo@=64ano5\K!&3#RMZMK-Bcmcb+Wi5)U(FSoh#.UW#6=N!%M>(YbV\)m
qWaFT#QSO#)$pEI_4]G$'H@U;_SJL19I^ec`BrO>^h,DAL'N@j!:Xqa)%K2*+u+>T
5TL>i"!M?F?=4HSL4c2Xn:4"gSk3M0\E&$(-P4T,![.hs3[>>r`a`tL4;nb;"bX0a
k]fKA(_&jl&J0af,GYSr!RRoA2Brlm"4Gj"KK^Xq=X^]dTVP+''ak2^E;55D5S+5+
@c:^J3Z<QX70:l0Zp>mh#DDd_&<KIS"+deoE&]Zu'EA79)LY)F/fU3^6D8fcTG=fe
D0FZA?KZD<"U-3G3f#=-WRM-(+RjnL,m=L*J`-"t<&tj%K7Yg#`5jZk$A:_dr^]Pu
j7.0,JRHE02_Wd:_h%]0crZ-l`+G,Q=A)+!%E!1B\oJ2\JCm7/-]gBrc)9MSC`8"Y
0L58_!8p*QKOI,4%)8J18e_G["@*NO0a(#TJmbA/b_/N#17U4Po%4Z[8H:rXKPT4*
'o!lf>`_#ig:e=+i@$gNTaJAu'SX@O5*:I?dfL*ab'6/\J,gu'!W]>aL>kkA!%8,r
o,&&pbgS6Y"O+2GferjE&-*#h',saR3=bg("bD2?]Ea"Oqb3r?F/+RR]FIV1R0%:<
+:Eio&2kC/^qq/`\Sh#1jJnlaBF;MRI23,NC+Kpd`iPgm'8C=,&eBbt8juLLJB0dB
"R,Jn>cBuo,b$4K:bqF:i@%;2"Q<0RV'37J.h5%J#W@VF.C`%iKJnW=NE2/a6Dc"V
@a->)_-:$k!)t8lFNa%J5gJ2pBFrNr=.>$%?C*ns#(buo+9oBLO8o^l!GG$ei7'QQ
"p+dJ)"@XpZ7.KV-oFVe"1AOJ%OFD_9hGKqQp"&%@%KqXK.?Xg*Bjel0.3O"X4G+>
l3#nIYCN`pQ.I_m!XpW23&V>&Y*^btBW8>hre06(71h)E#ZM[npV*W,92.AR/aBq(
\TL^+@o1SUD9W#)K7L?(#D,3WpH@o'()K-mNd*L?K0TD^$3LT:4:m-9K>daNO!Bne
]bRY@MP[7_U?mJ&RpV+2iHS,&W2T[3&Q[iZ2St-`3&K4g\L"P>Y^>f-&Hhb17BZ=>
Ipq!q[KnJmJX]WMe2M6fB&5IFh:6q]+Nog!!jk1RjJK.MFW.*UA$VJ$+I*/\U^I?q
&jDQ>Cn$(8a?k]7TZUpZ"S-kW!(G"n(_$+FJ)U1r=E"pq9s[Y.2?@*-F88:9ksp;V
$>`H\N&9WBB<cYMG^u29!h`p6Q68;)&\/rm-_uDI'D-_qPT>D'I<:!^k.ADanq7RF
H3$JN_:6T-9B]%`*je[1h]^'YE2"=>Qurntiq.Hq!Il*>joq,t<!)5_L.!G:'&mFr
M9j6H[78g9^]Js7D6SP@~>

Q
n
Q
Q
Q
q
n
213.226 652.486 98 70 re
W
n
q
98 0 0 70 213.226 652.486 cm
q
n
0 0 1 1 re
q
W
[/Indexed [/DeviceCMYK] 221
<~mGR$Ke]Pn)e]Gh&eB#V!e&]Ire&T@nd`94jd`0.fdDj"bd)Ee]d)<\Ycc!PUcbmJR
cGI8McG@/Hc,%#DbeUi@beL`<bJ(N7bJ(K4bItE0b.Y9,b.P0(b.P-%ah+s!ah"iq
aLSWla18Kha1/Ee`j`3``j`0]`O;sW`O2mT`3laP`3cXL_mHOH_m?FD_R$:@_Qp1<
_6L"7^p0k3^p'b/^TXS+^TOJ&^94>"^9+4s]r\%o]r\"l]W7eg]W._d];hS`];_J\
\u;8W\u22T\YbuO\YYlK\>>`G\"oNB\"fE>[\B39[\9-7[@s!3[@im0[%E^,Z_*R(
ZC[@$ZCR:!Z(7-sYagpnYFC^jYF:UfY*kCbXdG1]XI"tYX-J\TWg/PPWg&GMWKW5I
W03&FViciBVNH]?V3$K;UlU97UlL05UQ's1U5Xa.To+I)TS\7%T88"!SqhdrSVDRo
S:u@lRY6%hR=]bdR"9P`Q[j;\Q@F)YQ%!lVP^RZSP'_9NOa;'KOEkjHO*GXENHT4?
N-0"<Mf`e9MK<S6LiI21LN$u.L2Uc+Kl1Q(KPbB&K5>0#JnnruJSJ`rJ8&NoIqW9k
I:lsgHtHadHY$OaH=U=^H"1+[G[anXG@=\UG$nJRF^J8OFC&&LEa;`HEElNEE*H<B
Dd$*?DHTp=D-'X9CfXF6C/n+2BiIn/BN%\,B2VJ)Al28&A5Gr"@o#_t@80>o?qa,l
?VEuj?;!cg>tRQd>Y.?a>=_-^>":p[=@PUW=%,CT<^]1Q<C/nM<'`_K;F!DG;*R2D
:d-uA:Hgi?:-CW<9KY<8905*58iep38NA^082rL-7lN:*7Q*('6o?b#6SpOu68L=r
5r(+o5VXnl4teMg4YA;d4=r)a4"Ml^3\)Z[3%HEX2_$6V2CU$S2(0gP1aaUM1F=CJ
0dS(F0I.kC/gDM>/Ku></0Q,9.Nff5.3BT2-lsB/-QX9.-64'+,odj(,9%R%+rV@"
+W2-t+;bpq*uGgp*Z#Um*>TCj)\j(f)AEkc(_RG](D.5Z((h,Y'bCoV'+YTR&e5BO
&If0L&.AsI%graF%LWXE%13FB$OI+>$4$n;#mU\8#6kA4"p>&/"9S`+!s/N(!W`<%
z~>]
cs 
<<
/ImageType 1
/Width 280
/Height 200
/ImageMatrix [280 0 0 -200 0 200] 
/BitsPerComponent 8
/Decode [0 255 ] 
/_Filters [currentfile /ASCII85Decode filter dup /LZWDecode filter dup 
] >>
pdf_image J,g]g3$]7K#D>EP:q1$o*=mro@So+\<\5,H7Uo<*jE<[.O@Wn[3@'nb-^757;Rp>H
>q_R=AlC^cenm@9:1mM9jS"!dTMT<$3[GQ$8#0$s<4ZX!SPQ1`C/m<k<ioH)<bBM.
eTSV0<nAkq3n8u,B<0^f(:oCW_S!<^BsnakqW2psh&$rdjVI't^>NZ`7P5&X4h<B;
ppnYsP22!'aEYq)HGZgrj<?oVB`+!Xcpet_'pCR6&.XN86_YX26a)>P(9IHs3&V`f
M8mHlnGId?Q3Td]YhWJE-6*>F67HKnE73IX!oj=?"A1Bg%S'g="ILMK$3n"F==?]e
(_-d=*68t=4<>#h"9Hm-OA?&eL%bXW8;oqJK8<>fLqQ(c8eds,Tlt03-l>(!"5tq?
*!`2,=;cj%OD#R;cK[:q6kKhm$A(O).eJ@dcn>u!TVKs15%)Ge%DC]kj:FKu(e>8B
+QtQf!T8mO$\M6*4q<3bS+$hLBIH4g+M`4Qg]Tns:)$=i63b";k-Ihg^='*iJHMSO
9GW@ke$KkoJP];ZL>e@ZN'pUC.L<dA'N5abEY'_T`UZ]7pV&;B6QQ@R!'C\l^lTN@
!MG5u$q=XW2@Ta&YU]*nZa_e=KEr,+$H_6D7ff8JL`d(X_$m=Y"LX%X&d36$k[>DW
l+9O,O,u11KqXA,g]X<)<=+Dg888`#@/)Vl"I#9)3lF:YbRD!Hi&)AS!5L7+;LlhG
ESFmB3C64*]Un640u-$fK9W#d,i#'*8On>^O>g5D!73%rK(UN[%pQiZ+:*T"n2k;c
Tf$I'KRm=j@iKR;-47LQh7O;"YE23dK]+=U'o)g?@Mjh#J1M$/@#-EILFDc4_qL4\
^'Xs`eFa\lRI5Is7MI\>$A6/S=r53re;J5!QLHJ$Jfo"J"bL.BQ4JTjO;&+V<Ak$h
`F*p:Xp"LW5S3<%85.'*7dPfti6Ru\@`nd;8WX05B(QiC+QtEdKOHi*'a#A&42Z[6
La=6tnp1QPnf3A3&>IHSfV%B3*(psT=B+o&B9qtRSig(Ajakms&6ID7nPCe,"$6We
:4e__+9_e]VAFf9!/MG(eq"V8'nO/kIq&)Dh^,U^JR[ief3JA6Z\0I=cLD$G5[G7I
_9c%1"S/d#'>C%L;@`jfmq$Fo@4r5n!o4U1EcsUE3QQj2i%><;dPpZT_&3@Wl4qGQ
FhS(+>F$[4AX0&:V?[mbk<*SNYQ8A8cOll>7dMN3!C.J*!<=fH!141mGDuB&",CUW
Zj+-=5(CB;('4Im%kRn]rg0uD"%p'9![Nd2'X/U3k)?O67<Aad_[6K<5R/>7&da-i
/d5XU)n0nfj;-)["3`c=!bf6+:Ok#!mM-;J-,sf;^_M=EiY$eB.XRf*p]`,%_Q<IB
$"(dU?>1_Z6MM8W*6I)/DV,?'Uh$p_ifci.AQFBO4LUJf&;I,$;Z[LoeKe@jD!O>!
,+p:@'rW,STKEIV<G2Y'gL()F2F>=3S@6fGl3))<<fK#l#sc*@!amD\!7`+nft\a7
/X-mVFHH>pqe1!ZFg!9+C']AU.Wr"]VFGbpiSV80"&b*p5mSUYP:.uG^hk*n:e77S
gTaY=puSHnW(s*a&St-LYW,Rqe3I[VIumgd.7;MdJ:n\$!.Y[`A:#e3W^;kj'GD_L
-PJb>X?F]T#_IcL1BAs*!fBD<UU0(gJN+=&e-uCR<AJp;$$6oW?+-M1?3pU8OI)pM
r^6r'\m1a#MeXRuT*@KBAtnj$P/.gHM,FMD&sfLs/u:!a;Vg4,_Po9[8kCh)#@Lt"
:>dn1!8o)'^lk]!!'CI9^_\YSFJP.O6%cFg_Sst[>ulJ`#lr'MNI_?]"e`XEJKPIP
!*Bk1JD,a[[hbsA-mAb4H$q;)djEh\P\2HpNA@ie\`lqmD7(c%[r<o]X(9"Lb[&Lg
lBMJb8bIl(!['+>)?jj`o3?41Vp1PN`i9b@N9XO\0n;7)!B;P4#:eQ(WiG0Lqs-X<
g^Z:t4&"sOdCLek[T34,FHaS)V!NL[UieB-J?eW9i/efX?p4b0GROSo9gaLT@lDfO
*3fL.&MN&])o0N14R9$97XMiQ@ru@i/[Q@H1iXF4/C&[bK!BkA[-3_5hd4*%e?f?n
`tpT#IPY"#3*(#rSJ'mocA&,J[:0Gn=><=2/JU5=G&kD',A2\`fE'>kiGQ(aa!ZBE
A))G7nch>[M;_c=p?i+"SRkDg8.pO]*s;S7A-.m,&77m8_8,W=<Zm*tJB8/b=`]d5
M=MD=Fif0gBJ9T`WN)Qn@&p*/`GaE.YIMA3"]jE*;U^%5!]X0tYj.]KW7Ka5'tX*Y
%7r`>0gu/*:^KFt>>jd0,+n?q$A!=nWHclS.&9M6o`h%q=Sl!+clN:aF38>)nG+;:
+d-"Pmfd+K'J6][UYjuJ>j3THYIq4K!<mQGMdeT[Lc,M_!qpU"Yp(e^1,3!H.KmP<
rL7p^]]'&O"[KO<XnB?)5f>uQ13M!Ne`ONl%d([4a'DF$j.V"%)$B'TZJu\DE0Mag
C7pA!"-BZ#'YAj$E7JG"NARJgZ05u-QVd2-8#^M#Uj03-T.:j2=TDhFNW@-90@f%f
2)l/A2G+dr"\K)$3#?<WM0OS%RZ5`^QAmA9r5Ng8Ak""^"Q5J(^4]RK@'g2M:Sm_5
[3h#u_O/^(!o6=fOLDsF9t,?0!!+BJI?%6f@7rn0^SZkr_:VZn9O/341o^qeUQu%o
CmoJ[i!/6Y%Fb5BL]Ik2OO"UoD&(W.YQZSY5p-d@i$ofMXLO4i$Q.bd@8_\b7L--t
&:t6C$(e;-k[.[of14#S2UtOW!2'p8Gm>I0'jM%6LIP])8_3OJRF>->+'>2$7Jd2O
)NkV4Hp"&6^/.]7f[F6$]mqJa%"4r_8\"uu+W[3::e\('\CI\FC18N7\_^^AoH6Fc
Z,>).R*n=Vb$MZ0j<GtZqN(dGF9eV^)KLAn5d40mU+VctdpHSE]Mtbn$pQk!73H"'
_Q2tA:[,RqY)6]P[.THDougn$i&#GLSj.a+9oU2YcY?8V/k?L@Z`(Nl`/p5%XGt1/
"Q3Ym@$V+R1fLCW@t7[.LFi7t&gi9F7o-qc7WSLjH=nUk:rI<n-^Y%\4@IJrFG1X6
`YLJsiW2XQ4m-R>-XJrJmK04!Y95N/UZDF9b$7BRY6E.V0Dnm:>#aEDeI'sg5T0Z5
_WhY0G-D`G03\%lEfgnKEl7YU/KBFO7b[&L"([#D5XnAk:d>BY7\DGTU^dS/F9o[B
N?BRii&CubPQ\cuq2%jG,%Oc.Ce"cHV8b]Nkmg,edTl#f4m+l&`1HN.U&l]W=,`6F
0(K+e6inJLeM"0/BR6odHsFd\?)-InW&dj+]Rmtq'l$\b7bW)5YXYH1IV,,)a(10(
ioq$7!R@-i8l21Y_?Ae%"S',-`O+I*r1GS$9#uBdA(F.89R0"lc!YDp5_@FEL]lX^
#gZ7d`]cW70IA'*ilb0ED;7<0G'&EhKk:CKjY!Ngc9MVD7#*[)jt?sneF_g@"-L82
A?(Ec'XGp#8F.mimX/>749FJ2'd6X(iE-pJ#R+g<4j#+-")`i_`-l4`a9>[/i(4ik
**\A,Z@gX1bR.XK:CdpD:^B+aN\n6U:tZFSl/]cbi+NA2E<V0J38ef_J:eK>nDsh@
-=i3f+<F\MS85o("Q3B[lstMnG&1\d';db1#@>_KQs7gW:Ir9``L)S'7`>kAfHa.*
`pY5^Glr#a"H4U$k.hZS:),Q%'g[._TPat,BE[Q>[AFXi!'Ka?>^^;8INUaNi&h2r
M%33H'4d,"?rR>aS8iNs"TW#!W?.$G%hRdfA7a@#0hc+GgfP\6"mPH"^bc1eBF!IA
#>:1$1:ef-TL@&C>q$d*.P35(oWHLs[qtb%Le/&8%0L7Gi8rr"-!YG_C=0h1"mcYe
B3n(U,^QNl!Q76-VH0fHC(nES'[uC_iGre1H3=4+#AAQT''rICA4BrjpS>sLa(jb4
b%)!<^IBiOc]A:&A5S*%*C+';i)5%QdQGdkTV[N<mWM.!W@2.R"X$JC5^EZCDW4+!
"CPI=TQCDFfQBGS<jS%Xdm3uqZ@:n?Yu-$n72c5ar&@A:C^d$>:85,^p]M]]'F[HB
M&]`qb+Qc"TaXOP&cdC=7nKUl!^IOBA'>Tp6kjaa'S1(;Tt1HWp]b8RH@S=eKP4[=
<eqFt7$*E0Lmp\NL24l[;8=;BXFU]93!Q$nImsuhTLT'jC6+$=Ma0f:!)iQPHF^';
;@!g:^gIBiD?YP7"@m2.i'7GG>R%uY##u]JAS-93;KCc%n4M>/kPS/OiWQ6p:eW!G
k#_ZEc@0Mo4\'PRBB;FZ!)dQe3q-qfC;NR/:51)t!m1eBWVTi%hunb8![&0X$J#8%
1)&V4>G4A!6*tL%=BWV1F4!%naW>U_5uI$X"oq"r0Y1\T]EIG[!WX&<lGl]eHNG^L
"))5^Kj&!e;XhV8Fm&0bTOn@D?tUbq=J/^[04e*jAd.Wj'qdSl?r.&XA-NH;9'!3m
iaMpR'"!f#2WO"+A(=nH0Qq&1X5GD!9ak8l0EeP1TR]iBVOgZ/L.G*246f+6NN@U%
;H30gG>iBMk0BPdC0O*oT-oL/iA_LZU_CRL)PO_]J[>Vn6<9A/WG>>q-,iJjU'72n
F9GX#7frgrRhgMi82U>#a<X49$=-G@Z"(X7WJ1W8E^PW/""^Kbk6c.c4F*T1"nahV
#grd)4pA`8"ZHj4?rienG(?;nj@(h:!(:''\7KO:5)tH-LM4`17W@a\AZ,=3%4VPt
*n`opoT#JFi)6.",njn;A&]YSLk%HR[V2=5F9!ara*n+6.MEs_GbHr/@A"R5YSt;H
"XOmgjTol5NbRR15ep99K\ciFZFQbA."lQ?jtPVW:h,bXGI2K3"oA;;E`h7:@UM#]
bRFRWSq=jX"^kYoDVtVNX967;#"h.JD'!-)BN2iX`&B_eQ<lrZ?3ZR)@&IOHAlt]4
oQNbkFiODn1LrW;CGL%_FA>5UaopOrb/Ob#Kaans3)NuC^Mml!aTstN!@AGq08<mf
'`jV%+f'<Q85cn/S&I'Vn9@e"-j>-)8!4d+OXOY`/<)6ohFT_JF?fu-0]6J`4XR9@
k!fM+oXUgX;e^d!J3ltc_dC2B?N;uFi)[$.5,SMD-4E7)lB8n??3Lb-!bC\?8a]IV
'#(#,"\e(>6thD`k+H*q^4rkO5T4H1JB.jek`)g;(D>RljH7JF>:3lgE%lsK7,/q.
&n*5Qi@#CkO;agu)8Ip1@rbIa&ne'.DFl`V=1XG/Easat'!5?h7ak3;G&+D-"f)&e
bU/]Hc:8#;"lNRoBY4CVk(B\N4N##<i*&@<AA:B::DWj3lCq=\p."9d-0e0"N-q\a
-;F^!>j0:](a;AIG]uDE<F@cfTGiT/?Ck0d4No6Q(#F8ZaOLMA*NRJo"Xmci!gbpX
'ZC3:j&9ir5#2/J(#^,F!@+<^+qt'4)?HiU5XGYG5..B&S.I!#3)I<6GgC-p##E%A
bjq9\-pPLDRUbqaTNXO5>>ZM]Lp%nML&CAhn4sM1Hu=*/!"o;^@S1`9<9V+]Lk&f@
?:7?6Dr;T973VfK7_kZd7)VEO=%#Ham0SH5<d!]R!(PjA"B"HscOX^7oTJ%PA-P:r
4,N2?:TpFiPha&N?\Eet#6#1-(_NG[&_d-rJUA>DU);fR"^k5E9hTT)H__KT#-WQG
a#]@#kc%,b>/21Ti'?"AhFX)5M+X:.+CYRS..(D=!t3PSAe7M/GX&tV!=#En7Z,h1
_Pp%84o1Ic5TBfT'EI&):\C4]?s6Le)li9sX$@-q5Ulm/+Hjpp"2i!B:,,NI9s)CK
IX2QdbOeTYC-O(7Y"5j2KT=b]\n.Ne&7H7b@29HEe.X!G)$-*AGO,HW^1O3'D"QP;
.@BBqUkfEN!T4^o+=(d];?aJJJHV"3!&b#]3i8f9@tt5GJ15#!C:!2fALSUC^`!5=
(9&6/IR_,$/b!c^?J/^)!<<B*TF[/5gr@K';]CP5W76"K'EL\'SCuasC@\>4UUO4:
M6l'I'Ae\$M2KI??VDbI!$:7rSrrNNn).$X`,Ge"8-5Id&E+04!>EX".MfjT)'OG3
i)TsEq'LnIASg^n/&]6JYJ3NI8acgUi#61h63UrYW>F0li&a?6KXXTLZDLgna,6iB
c<am4\qKQ83@:X,I1p'pe>I0b!"[?T*O>m?aCIWXj@XX3&-2bT`lNH.PlYgA!/=^"
!B`5@5V`Bt7D@or<Hrt3pAA?S5Zs4/4n*QB?p"W(*_?fK"5s.iJI2s^%G5)5(*S&B
TlbW/h9;$q>kapskOHfW=MIVuc6RND.$f,-$=jg%?unQd:iOC-baugmZNe]Sq^.%c
>l!A\\><371qp#LV_5I?<uSBG+;b,%%dN/K"%iRQFL2*Ge#4B%Q`BE(8mM]A1>7Qp
WlECf]kNXn5%i7Q"]r'0'`NT4q@EZ1&4$Q]i>NG^F;P$r(+rP=M>Jm<TA_oZjN)a)
n2K'u?ZKhbi<\FJ*PpM]Gr0*G_JP:"L-s*P7Xk:T;s%;q-DgfCK_&?mWs,W+>B4;n
BR_X64Ai=kG'13c%KQPBoN_TmP]jeh(h#rK?0Hs]*GUu(I;ibbjf6<$i:IPQrX[rg
m\(=0+`%sGAeh7kjU(f::#*+oM8&gOMWl5F0@dBb?uOScA7tB6LZ8F'#$lTKZCZ<o
;pn/KElA#Fa048E`hqcP89@6,PGF#tm69T1%g^3^dpE37bT>ORoMZ0]ga*<LjTKiu
bMlhTJqM")g@"C`F:R7$%tOEc^Q9#c8/=L1(;Ws\*`j'5,jE%^#W3_.VU@]V8q0ok
;@&Egai*W"S7CXn@9[L"Y]BkEq=:@6o'ff4?p@&p@Kdl7MaR%]^^'pI7W_HN7k)R_
_>kP`KYg"tJ64]M%gN1jd(iI7*t\ds63qC41)^UVK0ab?Hq#CqM?IBB^e>sZ%gU#2
OK?)E((5mDJa'PuE@VQU7"R\&DJ14QSPJ@3am+t?:TINS2)'PJ-'F+<U(IBSC`SMU
/!\fS<'+7m#6\M0:padJX$X\^5_(g4&ISe1K9;6p.1$L)!eK;iCb-6Pf)ml2%9g5H
NX#$)ON'C:(RNpp_>sXu6l?Vr"lb':BJ9G6B_7a!2P3jG!!KQp%<fBC/.bFl+t^$X
9I(1piaQ<":a?JU"ToC1onS[OL'<1FJEVM?+qtB<JiM(!3#f;ZqjkOHkJ/.397jfQ
j=!913?8UMA&#\URoHI(l60,!V'XsI"Caub8.u-oMf'0%BkdhX!^RZ$'a8$eG24YS
'&3]m@!F<>[Oh2+%g50P(^m6m)VX1*^lUCjYi,Zs`?RY&*69m,Lbe.H%*1C@Kjjaq
('I48<?Oga:eVIRXGgQ=[E)fnNIu3:#cfH^YX/i0!741L!pK8Y`M75X&dj7VQoYf^
knmM<XD^2-huY]R+:!M%4-K(9!Dl<"_G$mt'9-LPi]3$/V#ifC`@4nhPL'S3(P`$I
8ue_<q^eeV<1PAiKFPhj)@42FGS:6r0Ou*%M.@q=!MEgEaLD5@<k9Ym-qMN.!3f/t
K]-$<)?um+3>SZS@mJWIabu\44@&C,'8E45@MQ-<'rPdM!C1-E]Wt1:$7-h>N!i+R
Qpgs"XGAD5!c+>R'*:aiZjX;"YTa8P5]A'l,QTaj!/,mFJ.7,2WX&m4i*[f;UGC1U
RjW.T6YhE"N*`/$6V,oi%N*bR4;('`:fNWQZj73iCqUr(Vm$.rZanT$7(IsOLk$ZU
_AHD>g*'(1%g4KZ,4@9P]FqcR(hFtQ+]Ogs&qpuQ<Z8!H%(ZlN&\qE_2rL>[RVKY!
Cto1;=ABK^G,ES.5bV".iS/3g/dJmoO<Ou4M5<uY8ic*)$)8Wi;@J08EY.^dMUNDs
!s"E:&*74j64Q;4!r!+9i-64Hc6sMZ$ar,!%MK""?s.a3i:+rJ%:a<XeW,;s3)UHd
X(mKqk[K.O1>5t0!ea:H8A'TVGYT<:625mDq&n//Q+TZB*XegugEF=Fi;Ne:K,--o
123G(dLO]4(WEEWW=<hO!s%>^X2DJJ-kL5;P>A%Y!2pgqD9RFj#D'@o'6/]0QN?#D
jN-%r"(4CXJKPF*!5^?CNZbSE&1Y?nPMC>3J:mthHj^l:OYTTB2us6I\rQSK"R=&?
U7ur?JFFcl@@T.YW+c\CJ;P!!J5D(7)S#m1/d4[XL+,AYG"Bt"9k:aBP1(Ig_*C'f
_%[oBTMjGC=;<2KI#]55hXr)G2Zs,O/K>Ha#XMQK"sDD:"!C;4j)>t@J7oRIiiZ:t
+ia^5*9X&[%W.i.Il(P\'Kc@2]N3`sJq-As6#o).#jYh#,^%BLn1"O#+sCAFClFbD
"p9BH*@8L;fn%33=TM>O1SC+d+bK4=^mGf:jIcu%Bd3=<+=IDSC$;)V8/O]:AIQDH
@0U])+[hE]'7r&0!b*Va_.(2'9Ji=i![rR!L^uIqD1k*G5RKfu63n_3)hVbp_d=9.
8M0b5*cqMhRHZ7++Q+&f@ME^@#rk@obSC;2DI\4=DEI2?BTnhb+994e+U9:RJYTAj
N!tGlj`Q:jZF#PjQjWqt>m.qG3c;b"7PZ9M7jY&]!l.sb<b^P-Y&ftO!20Ms!-H,0
iqTTH#U_!mPUm!r_AInBA>fNj1l)_`-,dTV&C#`ZR)?0?ek,'T^l/^T(A`mh=>pK#
oH")gA.2]mR$qEQ'UQ8*BIS0:46D+^b!7ABB3\!1&Knd$&4DH1j'2^5R624o,%E#P
IsQssKcIQ^>O-j]HLn7hb.o2&^h&N,J0]cTn44!S&KP)[!XMW?ZituA#c-P;8JMKQ
o%Me7?-e323$],V%XA]jJQOLXi4^$1%CZ`hPWfAH,UERIJl6-E'sqF.^Z%W,Dp/Ip
JcI4.aT*gqJERu*J8>Ubq*8Ag;V2qF#"ol*So,gpmMnd7gAl47XL'[m,4HaIQ"+/)
&#'Ug"!:n-OfedV._`D*A4DBd_0pK5L)]\["6dN0Z-CXO!`21)/FjOgjC8KZUhN/U
7/*;HH<7cq.SYMf=:8PV0&&Y*(P<9D&AgCsL`lX[)^lqfKZWEoJ1,@Q9:]Hu=`OSJ
@L[me1^7NY'`rn>:$\9V3^Cb!'2l8.&ASm)J4'VC&i>4JU"6n&Hk:jU5@g8J&d52,
aCAJr"Y[2q^BZ+)b/.Nh*:3hU.VO[f5Uo'ME!uc6k5;)TW!e1/-j1Zi`dj^*KWpSU
_RNeXiIZ%1:FS%OOWZ'+:p:^%hB<8mbW1Ik'I*_DH4L/CYTKV/<ZTq]4R,TX/bnB5
5u93=<HK%0&58N;\]8YH32e_dQq%cS*X+'oK=T?3'hlIE";DqF?h+>Db/n'm7#e*"
Q;l#53n-%+kcgr$#i+>&mNXU_,T6aKS=[9SDJ(rh\AlAm_.YP+M,X`\`r!(*6=J8G
jKP3o5%Cf>'0NBN-NtWk'ssoB$R&n0#4VI4KKt%t_:$k'i'RiDb<4Zp*!VM%aOl&W
/\8a'Al8Gc6V7C#4'1MjC[B)W5a.PWJ:J8oY%I[&H-P5h^riCHGf]^Sf18BC7.7Sd
_"*Qq?K<Fl<AV0VP,8(Vi(+0qZ=ZW6'W2,-Z#>1`UV2ul$/\s)^=[+X\&gsU32K"h
K^b]M_PgN'!E^uZT^X'l(jlfZ_ie(6_\*OFg$E+"'*A',NIeAD2U6skK0W9umm2h_
/I^Vc<*hqNHJNIh1]r9j'->quFlq"Ha$T4p9b.sIHnW<.F9I2YZ^1KH6p6/&PusKU
NJ@W_!"rG]/LRMQl"Hka!%K*hQ<`TZ?qk^HdJME_&S[80Z<Q@?n;%\Y?qq%081B6H
W"d,<Ae'Ca5DOdE)bd5sO+g#eO]eL@&EkYM+P.o45X'8*0JE^HZe`+QVM64<%Zh:d
&Ag0!\I0OlE/usg2Gf=(d'9_j`Y*Wj(Eo"X`!X1ceMbR<'bMl3@#(B<"FtaZ^2erN
U$*QGQ[k/$J2dZ38IUj3>Cfp.!BAkqn@?$6jZZeO3q.l[l@XWf'J>30!9bR-0I26P
-A$Ij!fSG10K4X"4ThW?K1S(eWS]QMYS['FVhc1Kl=pTM`W;NR!J>X&aMeaJ@gg2)
4UQhZ.'B'Ga/P2`U[+N_ag47Be.$Bh)IO/-na-g"$ns@<QaiELJLq?-72JdeZ`jW6
5QcO@6C!DbO9s;8&rONX[Z5FjQj_9D>0DgH(BL`ZM><SSn0J-L-A$>=K((CF=S;iQ
1P7A:_jd7uq<K,9jc1`%JZof=E#X?.(4dX='jqaWW#$!6'#SCc6TCGOf]GROq@&$f
[IY7i$'DMr5!;`c6b(U2*%ZubOpl"4JJ]65S(\pNKaQ:?#si\_H>AkHo)UX4/J4>1
l!+cn9:P8fNmq^^i!p^*G_#<R1&qdbkTL!Q;M%^kaA=JlYVUo^3<O4U!uNbfE12hI
j0oon!18TKX'1(A)6dOpJ63)-kS>Ai/fL-'%#Oq>K;0*!K#rQ2-$0&Q.DV:,YIX/$
(F*[Y^_4Z>d]V$AP*&=%cjt\[H)SU#JCosGn<U!JKJ4>o(K+*H)>9RKW5PbXQl:dH
'6+cj6V$*[!7@GiBFKG''S32#OE_m=0I$WY,YNY5!mjI@#X3lc21n.J!s@;YP`-"&
`ua6$aP[W;E6\K(Dh*oR#WS-?BeZj:Rm\[VQMEIiKZ_ND2um]n`_;j3.2s-AO<*rb
U\(1<)[h]%:k?+gV&G(]3_5N4"FsI7&[M[(&.FL3ArI!$PEYU$N/EI#EY2PLQ8:;<
BUFfj57*F-)<_^"J@q=a'EL`?`[DjYYT/5`+36,[cID4_^dS@`4NkMr0b`],kRY4n
B?*8k,O/KaC#k+q$'#S2NS6M#a:CstBFK4bS-kUCkjGnObsQ<m%?$hcZjD:7$C/QX
%2d!A!?)O='`lr#+>T/^.n>,9K;^o/JLH5&lR<_T1cMAcS2/!h=e:1Cgqh]>#Uq]0
AJV5sK)gE/[u#k?qa;%%5(Nt]JX@>VYT8;][K7!`dL[RRYX*oW3eKCIK,?.kdu1!K
?m'\&%(lq20f(P8EWK(@JN5^jBc-p'*PFG8'[hgTR[1.NlFGRHN$JT</86M@/KfG$
%CDZnWEISEd1TiT[Am1,-lrD0O1<7C&@-qmd4gNr/IVmiLb(c@_XiZ,m7o3F7EV&_
6I-Y<X+;DU'hZN/31^.:4Fl5uM?)!=0FRu<)$.PYSi@ho!$Kg2.KeThK8;8b&2:UJ
.OiPcP4KTe/38XPabeX`3<0hG;f3!LkGN&bJIiTJGdA=b;@K*U-W%jaJ:suE(]d1O
!D"/$6M.,$n&(j)MR2r+%6K(@@>UC'&8R>u\EL_*d[USq*68DgC7,(SQ`57I#ri-V
8F2Alri[4(^2%;KeI9&.+cls9TBNej.rt^."Y"LA*#_cWW#L<G*WbIH=OiB4O?3Ph
2?QSbK%MQ)OP5Mah[+'<RQPDV3ALV$jM!#[%C*>TO:mooc2adRJ\q2KfZX@2BUp\g
V/7'da;P(U'@pY>dr?!?,4(N4"@0&\:f*WH;S3lMCDO/CN4K6&EEBKa4>N:W;6;f+
K..6*#E4j%c6Zd^>@isZM2dXIP9S2#TEU;N?:Tr<J=$laBiM0Q$(AXI;:lliclI\n
MqGNf"*c[*7.C?2/-:VU!Sn]SR(rtU%)5Z('SL^^>(_q$7?$/n!4Wu!F!?N][t&]4
JT<r*1<"dl'Y\\fNX\EUC%[%U'909BO\&0K8AM'KJ%FUo.8+GN+pp:1-T)a(bm`N(
!I=`J"Q"Y4%MZrT;G%qf.tHld>>lHHWAqR)#rAQT]AW;j^^gFVCR7qC$AcnV,kD$b
R3<^X!Iu#<\/U"<<.W<lJ]K2@82Ef#KS$R1Jl![-8Uua3Y"@,('q(@JR&CAu__P=1
!]VBSCBOW6"VBU_YDN\2;1shd$*g9<$sh2C^^H"RSdN:d#\CB'j*?0'H6d705>;;$
Yi=V%'dM+/%[>):L]`/]!rt:`Qom6`"0.;;EIf]XJNt#"KsleO/J0K4N*3?I.aJS;
!%N(SJ?lGCU#hJ\@4nfkJZ'MV%JkXc-3G)=bKq_jX1&.<-3>;4+tM=HF(['Bp_'!,
)^q/XcjkVW+p)F#J5d865n^s5'*/J'@=#AS<UpK]Wst=SMT-m*XY?LFi%&JmA7,o[
a;,.%YL$5P3gc8UTj`j!H4@5N!%7n[?ikj=`OuPn4FC]fED71r<(rC4!8%nbR_]J#
K8t0c-&(S$0r>Kn$41E%!DXsAR/W1\(,_&3JY?Dti$?9D/csr[!g"f3S0J)C*eD`-
JE;4f*Ksf-=p_F6QQZ?bU(r]=&:nL;Jl!]nkQ68kOg*L<1^qNrM0D!WM8uW"=!8;'
k":p>Y)$<<N.MG8E"[_]Q[q;?9cS#4kR`9<bSO"@\s'/=l9,Wn(XL2>.uBk>=a6;P
Q[ke$'q</CA^7k$^`J:GJU#2cO;EJX+0sl*%N-W"OuB7$h#Q)iNLPgNJ/86?q:.Q/
JWLfP4+oGh.=udl!f/(Q80EK1)sM#MNQbPP,JaCkd:a./+<VbX0HpQ8*4*)E!5K9L
YS@ge09JilO#gL,.J@41OH%g*7B220E<$"WgQA-@JU.hoiPNh_Z%3GoTCkWEKU<Eo
J0Z%o],8Pho;##*mT,,PWu:S$Z%*,?MLgR)^*s'(;!-B&%Y5b/(RPL@^_d*N+/]Kl
J8!MAH6Tql(P&nc*t8='3A`@m(P.%1m;O6NVW*3+."\*<`CM?X+<[ri(>ZjGX-O!Q
:lp5n(6+oHXtU=d3$/2>j+6\<Td1>OM/.\S*gi$'R8&lqg:!`lCB9O\*AII.[*Y&?
^!g-&<S39SHXbF3aai0pCm';4eB?(@bHdYY/D,WB,0/22=5-bM)W7oP=;6lA'-AnA
eNauY,Mfpe42cJ)$(r(8)!7!k(P-6=kF`iG<"P7^/g%h2["ei!_6Fouh^(N*!Y?c"
i$iE&.EG=2Jk_1)L_g(si*o?'!Iu%P36OrS'7lejl"p<KN#i!B*WcM_!Re-$J-:C:
E8!Pu!Y?IgE<_!0(#L]t!,<g2JWu(/a#d"8:%%ot8;=+*Ss_;P26:11Bh?!;T>.<:
JZd.oaisB3b^a@1.)eVHG_6(Yh%'7g\-1gC_l3WUWft5tPKtU&\l8]4c:fAg(gmgR
Lq&u;-k@dQ!B:mHa<6'G)i9^`b(p4dETu3+_$M",ApH36?m/'>l[iXmJiG%X+<CRi
)hH'GE\ZHTH)DT)!.eT5U+]O(W"U-b67u@\!U_`EW9Sq3=+KP4Sk("*enK\T*0R?)
>ID"mCG$9KH;JduBKTjDg;SpP_?!1E!EQ<Ob7!qCn:=+BQ_DWF5=<\CfDnS\!)O2X
&0XD;T"=caWG-8.W"FS`#ma-KNcec%!<tpP9pbkQTBXP-r68I('nO.@.bGWAa^fqt
F9%E/JP,880&C`lZQ;XZK06Vp:aCX#-A#>L!O*7=ku)507KJq7#arf+doQQp)?KZQ
NQ,B,>H(re%e`;OWo+D<WY-B2s++8n<B(kIYSN<LK6m;'JPi-2!a(DY]dk=7,V`dJ
k_7@.:'#n#eaT0J\SEVgKqTe.r"1jfAfp"0fHNeSJahf]Di&_&k`H=M!F^Pm"Ilrf
UJG_5(^LJJO;!IlDZF,[LcU>1ragYYA<TfJO@M0rmIL`7_b&aT(9eL(kU8/&,=4&T
Jg_B7n/-`V,(W9%rWj=3r;.od14a%%cCbRPi03UKW;tHiD?f#"AJj%!4IBLge+NO:
jnXHn'C6;TU-j3V:^1la0S'.YN]?'Vl(]=-V1?aURu-@+A-k9o$^j@+(Q3dq!`u1r
"Gd%#$jd.CTYhB2i*mLW"ej<<GZ5pt$\sC%@474*+q]XL!T=/d?7cnK`'NnVCc!(B
$3^KMW)PA_#(o6N5cd4'*>"(HJai_f66[&""E721>VeAMLI8oC"DgOQ&d^tC@8Q<^
=>6$J"CaA.L*[=f7q7*`\6q@aM;pn;aCI+L&W0#1+qVh+*Y&@*5i?lL+:np>7RH'9
XBI%dL;O%Ri-6pj&W-a%%)BAV//AQqJfL_R2`q@u!LNk;4<taS$\]b;J7LC@%7gR%
Yi\V%$jD7aT^\=f59&U%6pM5P-^Dm;F*SA&#_kMUV-K\F)iU^>$O^3kcsY5%Lc-'f
4OET5>V$`5cpP$O"U@P_'ab(F^t-^b*ik-MWL+e3Jfojp$)ZXV&./KSfKpDWiCZ-D
K]*1r$\Ap,,RUs[i&IV_%Z36G"_#K>.#R"lO<fXV(k*D,Tl>#jKn3oN*JP`aFJa[u
\oO)bTnm\2L-^&4h7(T.0F@q5cr.7SkVI/kK:rA3'STt??l-.HQokf[W[LCKKts&s
^eCD/,S(##fNd+8@$KRXKE5>j%&T0fHJX5?@YWo&JK(.Fcq[+q%g/K_1tbUQ>P-%F
8WY:fV-td&'8-BW@7)KNh)GlHC(c9nJmbN<%tj35PS+-c1qF*hN.=;0KY\cg,,.a>
0*4l`fH^h,_)PC-UEN/l%"aZs0)[mDlCUm$JRE:=M#oq])i)9IL)pP-:g=qE.nFt*
"bFI")[6;p-OZh\&4dCd_;JU%Wo6bg$Gf938/VT>i(2Y.mM^fo"lVF9(8PA@:oiEG
*OZWaLm(^BJmc)P&qqIt<XU5sSg4XF@4UaX"VI,,)TMi9f\4[#r<JY!YiIhUK!])+
$+/W@,RRLi>#l2g@/sC@!m4M8&1BBc&MI:iNf?BXTSij\#9c>t\,t<QVAiQDq]0dU
ZSMfUBPEPeOX7h?<r]C\RU`&E/:9CNehNhH+:!I2:)Ja0k^jTS!DmAHKgKHs^BT6c
;A+U\+<1]?.KhdFKCXUo0*E]ME#Sss?rdpD%soE/]cb[9G(kKd=U7&g4(&X)+XfiK
2JjA*&qsb%<ur\KQoS9c@5(RnKgCf<+GR_:7Lt+/elJb]hKtBPAecml;eXl@5S=+U
o4=W(m=7;2K0aH)hn,q^8!!j140mX/Wc+[@JaMA@&MIPQW"L;J#[A*f+CMqai"U*'
(_:,tEC6S^/k/CQ,UWk'!g@f]pPY3Y<ZnXi".,)SJKlHI@%\'r!(I<I:cMK`^_&mJ
N.q><*$L%s!OP7lTg6s9"+[<e!^KRb&'7EG!'CI:,$7geTi>L:]mBdA2Lc#oLfl/l
&H\V3$c,(L2[Yi:QUK=0d^V.?!:1R*&7>YAb'd(.!U)<%V#h@i:Q<Ma%"aRQeOtPQ
"<b>pUeifK^s"5_TVN28E*-V98_?-1@&8D3('6a'%qPtONWN*B;o'&=@t669!Abc#
fgF9m1.\-'U/6FABrFB)'a,25PQm65+Y*Q*)?]J:Tto;*"cNp;^(=0T!N7M]cm:WW
O=pulfeER89m-SgC0Ub'2?`FCfE%bs6\([/N/::c&\q0W!>;S]J>*#n2Vn[i/5l_1
#sY%N4SV3-/I#V\)hV'ImS4]O,I+)2RfkYgkMd3XJ:J:8OGF"T80UmgGSC8<*WkD:
lT;(CMZYm:`_ST*+b35k!0@Zl!)[g!+Ip&4Biq8^+n%>IE_h:K@ZUV0,U;5\$QHuX
.947uJgBEf)hc]I!D"jJ^q!p@(j$,,5o'V)'H.VD9[S[UE0E^J-lEYj:tR"N!WZ%,
,4[NK:e_dhV']4X#sC:PTG9`YBoW2O+G#MV]`g[\#*O"uWXZH\G/1m6K3D;KJX@sZ
e)#I#.1jkKF^cgCN"H*+.`qbWp0I`Ub0U,J!WYb&."GUiTcd_N%Z3?BUc\tb,>U"m
7"KR_UkVcO<+sA^3`\Z\pOQ-^!^K9`J7(&9Zo>Qjju=MG'^-)qTP+Uf>HN&]ZkJ*8
D@3$,RX1uIpT^T;:!d.;D[Y9-JhUC9=(+Z&+E`Dp18+<i0d$X_oFA.D"DU2@%08qh
14_,@%Zta1=Jj:Q"5n(c!>$[`TZA,k_d!O\bit*&"Qq2D8qGgQhBcQ%7fcTN/\pld
_E_oCJn(cTJI!j*i4-],=f5oRF3@8"HkIt8D@*"/VR9$>q#Y(kF6.8@"Mg\M)>:'6
^n;9*7RVtho,eU(nPB>'>u.?%1n;DG3!KQSI6R"lJ0[r!-GX<@!l.G)^sFD4Nr\..
O=UPCQp!cI!M^IP&O8Vd(]lY##(XK(7h+Yk!e>M5Jm`="lp6%_@!ioHA2<30!%J6S
RmM\A7Ku.,1,u(R"5nftU;4Gu-D]/?)s22=af?fm+J]PLL,aa&HP0Z#8htuP>RSAN
o`V)R&lrNK:(Lc$`rrs2JYT&5-e0o$cLl@tO?dnr$U%e9oS`i=,`tiq#'YC/L&m1u
7hDBO:rHAn9ujdg2W_4FG#A"Vi)C+e]3GJh_:R\bGA)"a_0.j_0Y((`$'p)TRAlDT
J@t"GN!KmpVt_,u_G7A.3%bDs(lI$dJ5Gc,2B]es(':UjUbn4Y+q3,]Ql\-)[+kbW
J48TXbse-f;5f9N0FDEB7LT;Q*!80^LOeFi"B)'=F/u\3fRg+q+A$PSqrJ8tB\aW)
-l<)&$$OB&1m_6&&2E;C#g/<N#G!<8"=N>r!h_^cJRce*"iG4[2PC9gq3>mFWLk*m
U^!3?=@(le&/?lWU6!K."e42D!98;+lS&hOBIjed)^(0`;>bo9,qkG>>RAPuU-%Kk
N!#5)ebH,fg%.(,/&#W6O>I$IJ2@V4lgP3Bck5_3-j662h?cJ`]&j1o^pa)97fb?&
5C3SG^B='-->D9u(DT`QdeP9\B1I+W=n:j2!3UX(('Cf$1BN>#0u4);"Q7eqp)+DF
fuYs76s-&`[4OuO3'D>UR)J*qX5`_b\0IGrN=dYi#!N"ZV>s&E!ME&niB_E;kO:Y!
Um@k`1<!?K_n$$[&-P79f3g6%UR'TndXAnj5gV";`c<DV&chtDA#'Z#?qLQrrW+>5
4cP1p^bY#Q7\Z[c2(R5ZV3ZGE69(^0,pQqY9R(hrY#+7i,p4`?0OA%AZrUQs!ald0
K.PQI.Ve#OH!j$u^h07ZY-!40eP>9(9*RZd-7M^46uKR\i(+*N%Od2A08)5E,39$h
e0Z:`5\&CEc[M(=n9KOt#p>lJ5a"tgj9Gg5"2Z\<!)EVCaE_?Q-idp[jc'<$Pej-G
f;H3F/&!AV!g/Dl6R-OQ$"dr=I$J)#"QLic`"_><CsK'1aTGq$#)7U5b`5,$"0BKr
,pG)*&l$H5V?Gg+,3ZXkTYdF*`@[5U&%H(EkkH92"p5c[Bf(Hr/IsP<"!lg@XH3P"
<!L-7,m5&h6<p/hXTn*5/gu&SCb3&WhE1ch6K?W"?t]fgNX<LY#_JQL+D;!+lsaGf
.`V%u/5QK249PXnF@%8c+99GI7">FR-"qT+MAEXn(A''PH=BhX$EO9HHj&AL#Rl"[
TF_.L?ilu@ZAWVN$E!jA(4*qn"lMiS,P!M*#5b6\$:MO)l_Zs:5)nPujl:)OTL*[1
dPXCl+N2"6i*&>f-=fA&<cOH&66q.3;#Z>O?_nA;i,f0\5]?#!1*B9j#nZjm&7\La
*(cql77[QsAd:SK#lo\c!.ZI_>p)ge!f^q>#]d3Q5Qr?<"Me7ECI/'l&i67WFbfGi
jV#dF+<WoZ!8nQYEYs*sU]R231hO83?t]gr0K4LprsVI)W]%;Y(l;oAj?e#d`aC3&
=IO!L%>5'9->#<Zn-$UIeq:c\6dd^qgeeGiPb93t7qP\/TN7l&#=L!YK&T'-fJ$hg
WrhVij3mb=DK,%ImU.XM$+Ac4YTV+]jg)H?_^7X!3!B:i#,#i=i.;3,GR%]X"#!>,
kfBpDW!6X%3)1Ss@QFT'C]b4j/n7"j%iBt-<0MhL!8n7e@rO1:&7uF)5c!@"BD;\h
DYnr&a3ZC>U?Js_q>fFdQD16)Zg>\q@*c^N-`YEN/:9Tjdf+rLb[u$MK&S!#kWB!2
"9Wm(0Dop'2Xl?6?,JlTcGE)1+K\IH6`<&5U_!W9BEhp8EC>%*J2k>"N0T)^-t4r)
ZFVAmW)UQ?#f)f65_'(bJd1.2!f7Zn?lV%;3%AB",V3Jom=oXKe,k^Q,=g/b93Q68
=>iR)!FS<*8!cJ2i$8EmmXRJ)!*ff&AB1JO2'=#)@cUL_L]Lln!IukEk_aTnc6s2?
J-U0CD5<B\bqY(K.AC"%X[`GeEb?edpe/cS#HmD*KRORQHPC<(i`6-OX@VH!rd[B@
!*V2&LbfOT,!p%R-@jKW.Tq@Vp53-:a8mV5`@QP(#LL<lP_90ThD`4m</lJSD2&/u
R-)1V=N/_ior_9a3%0APb[;X'Mr_XG+[@e##_T]D.AS-1^A,KQ"mtY';RT_"pFbP%
Lk[JZ6A,PN>XsL2a=A/Qos0[a\g:lJd6^V4YIZ&O36(&l.Y=,QAq1!sYV^MSHK>Lt
DSf&aFO$b&5sRU<-W31l^8;%Shb:*Q!&Wp0\cVpW#;C<R[BhBYff8=F#/G`q"E:2I
1'5T79D&]@K8;QTqBF#_/Vl^qE$!4I,QiQf"lN?S7V#3Xg*gN.0`X$qL*f&6VTAmm
d7:\J2D#/HnS4:i6k'hTTL]6Z9d^\V"YO+)KFk;](s(jX`2n\?@tFi^!+*p;A(?H4
n3D-uH3_J;OVTig[7]Y8YYE<T"/GuWJo#7X#<;*G5\K76N9JFB5%&87B.H<J^c%9/
`4P"e"bqb0i*HWgN!A3VSk8&J^`N.S"p*^6BbQOPjJYO53`XKU1'NR(`#(3/9Ku@2
2ulYbPQWor+9A?Z%>4r&lP.QQhE_Lq5f/\G2h`C7<G+XM;W)7\TMPhf?SETFhns1R
,GKLni`*tjGHU"-o,)"3[8#^G3.a=h?qB%=*E;_qE['L+/YZ3R<hu`,d<:7'N91,5
$384,J92XF9nidBR`_CT;8q=9.1SL2H3<48!l-uM!+6(?ArIj?GTpF;&it$4ZDW:;
,B-sg\6(1f,kA>36GPD]J37s4jOQ^+[&C$O"[kU)8u@]X*/Fg4V"F+C9K3)'"-O-i
7OBF$\c\]?"`QaAl7g\^W%p<nN.QT>!he%C$n4g8"`Cgrkc/s';LR1!;g8O+0Pc3_
JnJ'nEf'H-26m;+1]Y<#JiG&4%SBg"hSK`p1E\7$Cc_*=nj+L4=#Y@,XUIij[K]!3
,q:aH@nqkG7KrMHB$7gh?rY\9s+b0L0jlVAW'H6X-T8A3bu,B\VL2Z.Ee&fS4)68:
lI8M#*D?oN0l(W!nMEu%+p4K??(a4_E7]stEkCSi.I'N;"OrM<53:dA,,e"Bi\5Pq
rB:>53idaj[QBN=XUQi$-R7>km6_X85&0<u"*4d1F"dW0ej1aR!O+DhTI),g6j8*O
1dmL>7,VNUG!i<^#A8!q''9>98-Nhl[\k%\AS(uD'EX-H!t&<*^_H@H9#:ZY"st"/
7]sG-rI%7?0b41ai)EhO(:&aJGG#B-ll`bGhH)5@J_2A)&:R-&%)PJ+"opC_!.?'5
8gbkmV$%tlkmn,V-#QAMRA4^VV@AHa&-YPmKci_;BZY8&/QD&/7oq!t=Km5=8:_#n
4O-M#==+&*(h84'2*(PToaM7Y=p?POa+T>j_I]0'+9W:R<_\b@j"rBVnc=g@"34C5
aN4'_2LnnOiit6?!';*LEI>cb:<VAQ,:&Oo`%kpe/tt+MBbiB3F9Z,Ba+,?mj9@4d
;0%rHJm]:*)MLShZ'>b:#b\7+.VQMUA7f:POlh^#A?9c;quQ=kR!Go\+Bh\)K-q$7
7eSaQCspq(btUN9(,,#SaH@cF>.m0<[Z3sm@fF'D8MFUg!lfWW+B5U4BWCDm-SjBX
J7*O&TI;5jI:+rdmJ))P>'V6$ChADEcuAQPDM=`S#2iknlaIVQj]tA'a?1qHdSc:'
ga)*6TnrMd7lQ&QU1Zf'I:,5?+;=h6$Zc@peo<m-VjIYgJdMLL#t'*h'Z!`V^1dd\
0dkQ6jm6GMJn*_<G6SWVHbMS@&:OGY:qO&p1t8Y*WJl`$#/_R^!oU>1dW)@?"4u2R
knc,U'9U(:Y0u$!^_R3KUA;s__?M=j=8"*-5;b\k[Tghi5XG_=Jkj*8"X\8'Aqt*f
,Z*Qc"m%?A!)Dqq(SA:u6U[O!r>m;G8i;2Q9k9DGD05UK]).E;\0D9#_J%h(>353H
OjdEB_hJ?QH3muL#f)6!^gj!8:8\A^rh)DTk=)f'qc\nE</#c)Y#kgEY$qi;a]cXX
>b"gHoe!TfH=]&=)rX;;8=VE)"WT%\KZGhth3btp!jOA-L>DtS:'_u2A&(hs._bO!
0I9`aceqI(^b.;M)/_,nX;,PJU9Fd'.PI:*]AQ!ZN`jfG'EGo[5X7",qr9u\$j$J:
,Q7Oi7;jD&'PG3I+RLd?KZjLL;Of!JcN$^2UBTUE19mKU#9\m1J;=IRIXfuY2Kf^1
@c@K_?3X<qL^ipa$USJ9S5i#OO3[a:h273&W`,>8a>14POi04Im02l`-89EPi)Ig-
2MSg.dk'V)B.h7a'F@$dKrsnGq7*]0mU;bp#N.oQ1ZNdk7KgU=:U+_f,je<B&0p+?
;RD_nJ7\tZs&!50cI0Db,Rr?g\p5Dh\hhQSY@hXgGpPplUCZl*OOtpi63OT92'Yj=
^dJ?6C'W[W#a<.>$]>NBB`I(FZ(eH,J/Do'L,ArbG/.bpa4<jl438o_;3cg,EL4PW
F8&*?Z!]&.QNf^VQHsX*(/p"%215e<hE<'U"Mf*c+GgQSe;T1"D]iWr,<dCoIRpg)
-NdOh!e=+LnuZ!)_%@Led.b/.PqGE$!M0P)d'N3.liI\_,Q]f973\6ipr<Kn`+Cn]
?m6]o0UP6B%hAsM!jQF+:*g*r_'&6WA3q^_%YuAbi8dWO$jK'bT\PPu)\.\a_2rV0
0HUr8`Zi4&==tBpKL+RZ0X,.A&-kRri:qg^)5@C&iBWY\Q4jWs6P8h7Atg-2c"$Bl
eK..&$A=">:ou3b*MJK]@QGW>.M0&k_;PBM80Se0cpZhXi,hRK,nNT*M4N!G)\7j]
,9`/]4<"W\7m`=4BIF;p7"f$C335k&&IJ[C)"^K&V:0/O)L88p5VO&Z2??(A>/a5F
LID3YN!jpEJHS:_!3gE)+V0>q<1BH-KH:^m"8-'0-mfQ3K0''pTO9f)&rJ&h!I0D;
$F'fR,&qSOF?grX7\[Jad]6NGKS(DO?oTDO&qtm%9G/So&1Rne5qlI["g0n<Tt(N1
P,5YrQmesc8YWBt!q3FU!lGEp7M(2)Qm`J5l52bt"YitO%Kf?@-42f7LaWW5#tQ88
"(<$U,6sq#Frpt*i-Go!6&8\YKqVU($A"jX5SO<N^`is`TR\d4#2r*\'#['Y:(b"o
n2SqAm7OSlKMllC[l8(2D@J7,]OKb@5`d)n^S)<t(W&Ff3Y6jXYVH[ji?1`(K>>u/
#m%h<('OaGAHWUC@D`isL1&`tie4"%?l=_#k]9FNltZ6e`8L\e'*:Eq&-UE(W'1lM
@3@uR"u.5I#6SBo?5SB(npmD^5l=Dh=\9N**%<\$B5&]rU:(I3Mfl>]K$$&3AjoQn
6Z>Ie&1ZtT+HS6o"(8na#9mR+DB[NG\98p"iOUo\L1//:(^/cA'F*-qBGq%=JB0th
1KPDZ'Eh'&d>7i><&b;<9)[NN!hdn)Aq_A;-Zqn"^!<,MEfa1p/)Z'M<NUeP$DC.$
gSP:/!<U[]KV:A'(G-O"BGZ>Q!#n)?5q$1a"eg0I*[Un12NT2WgP?UJ5Y)@f!8qfE
%YTDk:ud2e$ESi3TfZKo=KlkX`p/*:ik:!'-p&&F>Jr9)!c>[8'#]^$+pUa@NO^(a
qES@"KN:fKActD#`"@X;GSZSI!8'm_LdCNE;29A"DAe*-bDI5BiCHJ66]5=pQ*@;H
0:mh_[N(rn30#@BVJ@,$XFT52(TQH0pdWO0^h"sXTRCc-%0OF";@WcOL,KI9He`PM
"3XM'$ff&Ka0Gh6+BBUU@BaJ_K:o^jC\3/p>TSZo\el'5h'0*"U]CHq=M+VN"H?eO
9B8nZ!<<Q!5k$-*5g0oV"<:7c)-'kY9S7oIo*.pPL,mICKS$T%>Zls?E=0&aJtuN!
#odkTi.qmi<a&"Dcm&`\+<;LGC8mQ00kmK:(::kV#okBk2Lo2p'JmB.OZ4WlT\pd,
n5/OYdAT++e-geg!W[`ic3(k4'ttH(ECmdc+D&KJW$"V9<k&Y@TJQqFYV8>ni@-%k
"JUIs<7qXM+Trp\(B\&i%=q^M!Kar"JUg&odKh`7`=9qP"]Y[>'S?Hp-!:5Y%L5;B
\o*$d"Ft2?Xdnl.JdWU=aX*7X9A9dVi.5F9;NU>__<;#0T['NY"EI)%'6*0/L<KCA
?/K$)!T6tHaFIG-!O+HcJA`E00P1^/\2OTL\-aFa=pk?<1,`[mgO][O$%XcZ-pWk3
KGQbn,*Z"_`AO$5TEkPu$Shi-O;gZR#b>:)F=D#O&V8H1`^!oF"&o7.S.Yu2Lm]Sq
KS0o-n5ccEkTlb*f].Ou2@>DThZZ:3*.qX&$`GL',UA2/2=O-=Lk#^QXDf)An2L[R
?j$KZ@+GC`Ibe$Z5EqCt\.Rb7?O1*B3>08uWC%+^_&MG<YM9kWTHJrbksCaP<H&WP
=q)0]+\'7l'SJ/N$pd-1U]?g=93<#=)d@JRX-n+0A-Ga00K";e^_Wkf4Za*=E]=1-
"+W^+?K15+15$(?:V-<)gRN![LBRSg2b8(SJ.6.AW"u=AP.HjGL]me"++fSJ8Cco8
;CPiY!RO^Rk#aGF7G+Y%_s18o&.JX_'EkPR3!oZd)bsd;"b:^e"lmBEN@PmP!i)N,
8s:D"-5p(i2-^F06R.Ue4:iKG]$?om4*6`^'[?\]74!9'A'61.\Y=g`NIVrNL+4:\
i):;_=d60VN#fp:Lg>rq4!BZ<'nS,;%WDt=KaY*m=//Ad&?0,pc,dT!UgU`PQ4mll
\u?E&7W8?iZ<Mj2iW:GLX+<em#R(s)Q32n*5u9cN"Nd-`VR3G??kf@i2B7>\4Da-5
l>I&uR,=9$8W&lG!2*<ifVaT4@"L&/1]mss#3(i3o!JV9TFtgY)GJGR1q]pP<m'R#
<(bObQd$ZVb1n#+BYrVSJ7t44TJ-Wo@A!g4W"fCWE"!0&dl:`o*<T34NX7NT+TS)2
5#?q/6)ZRC+I7soJ,f\%J]*Q0N8_5ibR-X</7o<PhO=eoUn#>B6g2c$JHNCfQP/7i
@%Am$(T@"5EFsTKS.kuh'ELHI#&?J'%"[nc$Pa4'7I*_1>8dj(n<,^4!([V%^j,2_
F)bq_d#_2c86#Y`f.t-BTg*-Oc9X-D!b@bDJT*Gl5t6#YXr6Q*]>&LMq-'T'S/AIA
*fS/o-O87Wplc7e$hROR"GG:mJu0LlhpK@F9_Qg7<YPtZ(c2F>`#&RVC^`.Pk%$mt
YCP-cV?%;\\n*;tEcZbRbH)[dR$d1>YTV/Z@6qKk66uXhXoj37kULuQnc9:1!5Kd[
;Li-c"$ffo9QRkeBPm]2E&`N2$#sK@EN]FOBFKGj<O[ZUYEfAD<nl7:!?`b[^%NG&
noCf8H8H#@mW8W/X5V4ZH#E'S^^5Rt@Wp$X<HZYR$UH(u.6pl459O`l&.gIB&#H6t
e^t&A=>N-oNOf1Q;WMDn6O2Pr(IR[pDZK`^,%S;iSMpqFA&Y-PR-D6uIS@a0=X5ti
O:2-mYe%psJZqc]%"U?h".8+Z">&%.]^S)djTf@):KbpD''0=HQ*Ap)7,dX^C(2F+
<<C<*bEitu#6>Yh;'9NVJ7'(eH&gD?V,4u`-]/+r^60dqFh1f&n(Oo'h?4t3X.`JJ
^MuW0ON37c*W[Fi!AfN\M!tFq*Muqs!8t,[!#(1`O,PPNRtqUdKEm'<bQ16JL_@B$
TF6<a&>='IMmLqg!9=`ZfSu($Nj223;K*Anl]4RV/HY,J&TAuQUBq4%/8,8)=lOul
('1r+[I=q[3T#?Q=WU4C'hV%aRKsG!lAqm41`;!uQl)-/epq2eSdIBW;!3Bsb^ik"
QZ*6iE9Rk$aV`[i!3ht"\Ef#k'*3V"3.b%m@G\IYiZ09/PH/:/W8SDjFG_1N61GmB
.$K3#Mu^s`QJfW2;7MWY+q'eK!>#usE#\mo6S9PB-X`qSi"?'@%[j9#3=33R1\)]6
RBn&JNSp=t@mQ,0<Il8.TQsP9_e^k8Tt6(NM7aQJkSXD'&MZ6LJ3.&Ehusb'#+37P
6DQ(CHn18V$8DMm.5Hhp4'M^;#oGJ(J4q,d9'?s['S,+m4`NOj>?NmO3.Q9u#_SKE
dAEG%Wgf2'OQ+'dTgZS5g'A9((0ZXsq-?JCp(oc-J?d]NERtSS#_;4jJKX38HG2dt
s1;s!X"q>^R<&qD&!4<Sa1PEE.IR`R3PD,s/`=GP_)\FqMR;(BWnEjNj(4Od#S5;*
6Vs\2kS4-'O8rAc2:@d/0eA@D'h4F%O<eS$i][eG'Fgg1*5L`!,UXWG,Hi41(f9*"
i^kOXh2AKFPKDDV;"Xkc!AU8,UZA;[;Y$VS)8Z/3$X%U8lS>r2`flf-%UdJNEERfq
2N4lM!2'jRGSh#8V*=[D[sI)Gaj_\Jg^i&rPGsqU8/dWsb"DQ8MV+[tPdmQ/TapS=
1baXb9R&o,i5^F-NkE*LnNF!nW.<QTQZ9j]HG2G7`C`NIZOE\$.Qj);)hAh2V:cgg
eAm):D\6c=$(),%1\$@\OJI]*/83k(3SZC#ScNdN!LdK:K(><"<>7D*Nt;u0pnL0n
UDuP=QK]4r"5G>1-VN[i,A7A`gD5Yr25=m%PbJbZ6FArp.?:\gM5[[Fr69e+*<FM)
)$t>tR1;VeiYFVE0&*b7)k-k:Xe#4hd*!8^/8,BXUC!WT)qigC@9H7hQ*eKb:"3pZ
^_?glN'A#K'Y7e`5dM&9Td*Ha$eQ+"3HZ=ZXpGXR%!ai@1)#5'n:@MT.#JbG<*h-.
Q[sE.!E+E:\-[\1$&^NM(.kJBZ'pusd`MYu:O)H%$WJ"c>`OYW%`+IKS2H[)d3i=Q
b55b#MDl!+'7rS4N"k6Z_U07-?Q,sn79H8)pt@X381LBhJOfkC1L2lrgFV%&)NrL/
/7h`c"9<,5&\DhX1]Ta^V1>hpTP?cW1fCp<)j]ET5K#t(.m=I$'oK[kMTEUk_jD*o
l_o%DJcSQ.:`4hWd*#Cr!?`5:Z-46#L7;9]!EjJ*+g31`AOSk@ZIFSh/?4c`#mc3(
/NEC4$"lF%"i2C2%L`sc\g`1MRO0^!Oe;k3fWYA^*.b%"Q/i<24/iNpWOhGEJDD^"
9"m"5&V/LQ!@o!EgnG1=^(9fs/EdKBH;CGp!]AU5Qr0>2@K"F"/#5]U3)C)F(r_%t
)\D&.b47L<!1!WS)[r,R\kj1YOOt-H`mGn4`Y@MZ^_;:?*@@^!Z`4ff8WP`+`IPH0
JaCVg1g,gOB+[.mOcTqmJ.Y]KLW4_?7S!_Yg*;.c)Z^c`&'tZXn.s))V>u2s[\0E%
q5Su7'c@Rm!1M]P=[S43$o-tW'A\NgU`Y,t8/.":SdV'QUND&X%90t3_bGbB.@l#4
)@eOV!&?-.I4SGW.mB((T@2g80GT1RTaWK(!AG;jGSVK"R@1V.P`<<UBY>K3#GO""
%nIK;R-KQJ#QS674#<E7BcE2nV^AH=M>WT&@4HeC?\*_A=rA[t'>I'LYJe5L+dlC@
!KDtmRj>oG1=N!!?knp#R'*q86b*5%[#QGp)jqNMO4-ZAF;'4jk7b)W>E(-sU?*^F
8R)ZXc\u94^_etD=M$8rbR<qrWgJ>gTI;AZUYlphEunS>.gi5dXZ4XXp_p!P1+p.X
P#)jQQj5M1%>ZFM-NN3`@BonWT,gJ0Yj`D0-l^3W\.GSH+C,*oGlSa+'aiGW*_GPK
YSB-5KSi#$h'E<<<(DjT_,@YDegnPN+S^ML&HIYW$Xs[7fF<CF'eU);0cF)Cql$6Y
8J%Pm)8)UkWKt@F."M\I0UiC#*2ST*lVeh:gX2cJ4@0$5"$K'%7X,<$F>jf:m5G<s
JIiWK=RV]iUE/:GMPph&8enT"(]i,"UZ!nX4);L8K`GUg2;8suD''r]&E5N_#XXCg
_;_[)*Y;?A$\ACi\/Z^gie_mtY:NV/1)-Z8P5u[LNpmXOBFg0g'J:W6%@Et+HtJg$
\rT;<*?a%&kpfcir"7CZ,O*2JfrlfuP+C+O1-=6ua9*7s3O=e`S(J=_<\ZL<p-,Hs
:Mr#HMr=\)D\`&053V<ndsR@HYR:Ha+uJ_h)@)P5>9@?,$,M`314W3kD`JXYWHf3Z
'Fuf>W8K2tVi=/r8WCTnW"rNl;)mRjclms:SZ(#@`#RBhEcK"85"A4sMqsY\_UkHR
]9,,m!JhO#EL;T]$;i)D*%>e5.*@^p1<<J.c]#[?n/26]\="#dM$]#q#sf3B2:[8\
Ohj=$jmfp%C,Rt*]g4&Z);pa;SH0(;JM7YHNI@%R/2op0VVpl;nRC!5'!M7#2$&>D
OVcO<c(?BsP:h?M$%KmN?&pR,'p.78aW3),C(<mRSU<m:E"dg''KCUT`QC0;iGt'r
igJGj!HVkqqH\X8(7p>u$)#uZ<4!]s)1cAD`3>\\Rhum+Wu"Cb0mRu"&=WYuk$/:7
^Zh!n9[+EB$jcpVR1PgW&>p,UiYq]J&Df1Z\A=[Tdp(,L!(;*`$Pn<?&Xa(?jm-7m
gjh_Mm_q:q*+COgi9HYMQ&;=X8(?fZ;5le>+2IuHQB??KOJ\BS9HAdV*G_2R#`ou(
Z_p,4ih2APf\%,cd\qC)!MCTefGfBoX"[A\0@FhWW3T`\\:FC)D#8nnb?SSB-b:]7
N2QkC&n;ckTGlD1,Wt?-.7>8hE<o-m$\PH>_2Ja6_'==X<7I/ID"@!4$3:;`7tfP3
Elihp.i@R8!<Htm`%XDJ6^FR7^-_CJ/k3hB#M<01<6=!VQ(V.m5Z)qR,M\@3Qk"\.
*_e\5a3e[ai2=K_#6@(5&k^smVTk*c.Z/BL5r]N#FQPfLS-XL!QJ1Sk$8ql^6\u+f
.Tk)/iC1n^!rta?^p(k8M49=r[]TI2JNt9-H%u[q23i3%+DHZ<H:n_%?^UH\R:rh)
L>Pm;mA4r$5,mk!+NM#Y$4CeX!''<OA<rn)S+P^u52pGslLKfHQ+Cq7MeE<h3`F)7
PC`A/9uMWKX)qQ"()lJ:NOGo!`(KC@aT0*h!R)&[:14K3g(2kRMNErJ-kZPW%*?1U
NS0J"MT230HVSUEpPUt2qi78Z"bB2V<NDLN.&krDZN2Hn!RUq*q$mo%>_,ugR#sN;
K,M'6i[IOi)7Tl%eEB5lio3XHR]Q2TF-D,f"@d)($am;A+ul-4L`Eq5>#<*ll3RrG
P!O@2STfNL!nYNXd\m#u(,9:`Gpa&o&rkA8:@hr&#6'rK&.esJ(k^^r@S::un20]f
0"HDM.2!6N'9l\J$Fb2[H[9n&YBp4nQFQ=g$&ZZP5ljm`aAt;d?llVY1ed^9'I)0:
l<)>n"cpM]_O@J14SsBETT(!X$PAOC7D5)(%1NME^R`e[5:R@-O$Ph,/j3Qm5?H,?
rGMggMZ[<Hj7bk<ZG<AXJP[/@JF%OZ9F?0D6ZRVhbh7Nq/#lr"$Yc]E/8#8-/s;EU
PnDLH5T#'N&tUTBP[]d2"\]Kp:&>1V:3e<sa^VC3<IlD8JQqrf>(V;J*?83=.J*-b
Ri^`!G?;7=#qT)=I&0<3MbBl6N]AI,)3#KLldJ9&6l<2,(paPe<t=XJ)b.@$i"Ssr
6id"4#=F'HfP!#X$jHf"d+D/E'+"en@6h>93$8e=`+"h\GXs:tJ\[qO=?IW=M?Q;>
5j3_f,nc(\^sGn7*Z>QF7=lp!La!92K0c07Qs(%;$pl+'T`C0L.2E8E@e$t\<%/N?
`o5kFA1_-r_<aILeX"HmZs%:MLg13D(^j4DJg#Zg>TjB*_EgI!OAI\E#QP](-4[a*
$AEI4J=o[YNe[agi60bZOU95tm*L\T=qd746iqpS9o@.7%gteaOI/+7%L>pO2=Qu&
.7f>Ol,(8]e8-NI$:Vf+:lIgHQA@mO+D=rG,S>iJJ_m&A4=1Vn_I3Fh6mNQXLH<i8
fR-F8%>Y2dJ9Y$9(5W07JY*`X4<P8n,okkTUeVJT@)+2'J`'?G$%eh]*le<^E%DMG
iCIW'L;CZC*JVCp2%9_?0ME6=WuEn'7#Os)%%r-t0a3/Zb$5T@MVpZ/UB)cD)@&Qt
$Gmu@+rnPB&e'I:0_-^QbG!jU.LijQP/;m(TTd%l0iBPt%"od;0SfcclUD:>$ptZ[
K&Gi\'*\JfA/5=l/#!T.TepC9.:B(o"KWa86Tp)G"D8U*+bQ$`Z,"P_%"],-8ef&l
BILQG@,2Y+^n=ogbJ?kk+pimqI'A\8JRD$'K2<s5fVK"<*!QF/\h9>'_6@)^L>gL$
)[5oZEYP976[o6W;([I-/a>[Rp]9c<1E$B+ZtC6Z/*K_C7oA#Q\BIhk[;EuY5V2;S
'0&nj"`Fr/$A'CN+YKK?HQ3`OXCSAVJmcAQ-%l:Y=:Kl,J/S[pYJ<gH6`r9A5(h7U
7[,VMO;7pTNC(,c3e68/%u%h4i30CVZ3CX:Z<0=L"CV9M#(_;,(^D^%GS1.1H"&$*
6(h,-$A2HTr"=Z*pc?NJ?rg;6KF!J_"G$(/@csrRn9>cSJZ)_Nl<u5U&VZpO?KWHU
22;g;XMgcr"0'@2&l2pQ:*'St"T/eAESC]<U+uVW]A$"m,,7"7:fJ58J]qt!-LV9I
qh(l`9]7jbEu516@#Mia#=0BW#D(WK8=3,f';^B.pnOfQ",sGq$R1^"#o'JVkZ6[s
qf"S-K0[0p^#q,C8.u,hm?6,Ii'rCOAH5O:!s(ZMj"NVFM?L5:9lM9b"+aQ@"p"]N
<!Ip,&mc<.!Ut7PLJA2]ET4e'6kok+!Xc3up)9)(BA[qmZJc`N7NSPf?u?1i6!eG'
.?h6JN5lmSgB),\">=9S$Ghn4#=.bg031&=bsChmTYqUt^d&/k82+T4,`.gS`5N55
%m*$i&Kd40T)eHu5,VCoJ`&._!1L'"Ce[-H0MhujMZ<jPOMIE[)?LIjhDBpC'EN_X
#`q>;!8o++2BW>-S<9+7kCDX%V=(/[EOGr,d2E$^*q4\f%g'j-BS'W&plM^1.R:'N
Q.!`NaATj'.$0+VJ2fiYTb_:Z)>XG%1^S`C1j#Z*\J]*%,NON>JLeYGZm3.n5j0Es
.b#C>5[Y"0!I85^3"(9;)W&cE*!8S?&#j$jfmt@(+ok:G!Z'(tPM,.BVhQ&ii*HX^
3JenSXr/s%3XLA]'`oL<:*"shJNtn""5ma8\DnK/^j%+,TI^3GEg#(Q!H8*qV9gd_
3d0(Gh?8@V%5@"C8_::[-QoP^")q^k)`T,H8C4?Je6<uhfkE'8!4XZq84A'V?NVFI
3@CJ8'2I0hOg7H68HlE.gX/>Fb.&"7?sF/W_bgTqN":J_J-)]9-37q]#GR'nUR(`_
+[i[NZf!MB_'gdlOL:Z="7FL41bt>(E3VO46Ei`=/=bnEQ6tNN"_QiPD!3<$R?U_X
hCoa-kCjbj\77#0l@3[[<"0t&/-l6K%X?naR1Wt=#_?AC.a1bHO=+WI!E6T]DutQU
WddTAN4V-h@CS,SgdS%?XT<qu\JN+10l2N^"*!*"JO3&99@t,15c>V(i+NP89gf%J
-j3^M&BiaT-in=ibCIcA)G]Ut,Gs/Z![(;J!Y@U%i2pUcV$oVjM:F3(hQ^<^6k0f,
kQ-31%heq0#3@Y/,QO8L!_]Y<SQHac`@]W%7P%cm&NESL<^2[d&dSKA$Y1\m[k-[t
HeWORIc-;&JX'.Pe("l;jbYZo79ibW4E:Sc&pY]hN`f-c$$kT3`.<X#WIT&1/<AZ/
iEMKk^nWEN0rtn;?sX:nW$VXT?F56!9EBZ-.C@=3#m$\C#(\H5GY@th(o\MoLoL.Q
T_oj`TP=kdiHl_M<Z0)kH%eN['o4`OVSr7[P)>>K\sH^I\\_a0RoSU@&`"jd!Ynh@
,@+en=OQ'W'7;T)n,u"qKun9b`/2V!1\>2`JQ8$K)a2]\TWf3,#lcO`-l.b4!5'q`
(ll\%CWMf-g;u/+CY:cA/mt1^!mjdY!.YCVRVW&iggu@_PZ.\a>RpoM>eh,j-U;Q;
`$SFZ%hZl:"b<Zf0D+Ls=M=/`:*gJj?oA>-J/pC10FO'>oEPt1*<lbNKC%-_g5_.V
51&][Sf5Q2SpfaD$!$)TW+NnDQ,TgiK]1'O,FduiV2",'#Kh-mF'=)J"jO_FK"u%,
)_HFgY1]2SK$IkqQ*(0'K'r,//U"A7gaGl#J6Al(#S6G/!HDF``f:f90gGt,Y,TA!
i%Y"YE$kZ>.#0(`9jF-S-s%OO*2rERBZRG2,=Vm0DA6\qT=>^k+=mqfm4TR6#U[m0
4(aV:>*`aO"M<82LL)IN=Z4Y;1V2T)6PsBR\u74`@*q]]U,p6S[#SAQ8`a*J6A@dC
]T>\.XHe<I2!QSJ;f(C!!M0ARA+%$Z'GeioPuc)bRHBrg?B50>D%uA_Y['d6"-Q"C
Wc62+?Ha_hgr/l6!>%$k@$hUZ:hU8.5(^e.'VmfIp7I_L7$AamGa%V2#"[$;"CQQ<
-O-[_pCk+@[#R7,/$s.glH>^R5gFKr_::.M"^%9/n=S':@S/:\@UQsQ6$"MB_$1q`
^k$QXM<"uZU&G5rM%O+CP$4?<m5)+M/PA>oAZ31+Db@2**V76uJ<1g"@$h4_6XH<0
f^;+7Es>MC^aOYf>!O2]":%Of!'USE@Vqc+"@-Kj@O>A+U`s=^",-Fqi'uTjdKAm&
9<)#c"SVt*3<8%l!J\0:K$Gp#bQ^<j"b[RoX@P*S'Hq*UbV#XEMqC4j-@cTu==Y_&
lgT[;5W(nI04Gn'K;)5&/qt\;Sj5mPTMjl:9*f'#DG;*A!qM*h1^.8h"+q@8$"b@a
Ug6<E]Z>-e!fE@\]OJbu1kH2=TKFhN3jV0070#RV^hO"VmTi1r:r$*7K2;_<IR*!O
?"B1GKq@Yh@(SuQ1B9<:i)0XW+D!m-"Q2Zj@Klr"LkbBL9El[D!d4c9Os24+>lYW?
mRme'Ln%:hq$bPcd"_Io<r+;YO:al/a-m4X6DT>e.*:NQ?u68</Jdh\/J,H#UKVnT
P^8*:$"Os#7C6QV^B6-J8E2f`UB6s!>%#-23FX8R$pk&q8gM;Z46SjU&R)Ug##fMh
4@oJO:`-gF+QZH%,_bImL3!VH11>f+q*W"&%qZ"r^aod3EokfJmtTRMM\^0B7O=GH
/CF^[8p(4UB+]<LiZ'Ku127q6"K)l=nJhYh72XrZN^Q8s7d@:B4s=L>$`Vq$6:sg:
'!"StBHS6A"h6g,9b9_(44."_6:_/h$p%i%:;^<_J6q+8=@]49Pjc7.M+U]c2'?RC
QXEjScL`8fA-=,l[-LsDd(jM663Q4.(Et1_COV"i$3fKk0npN;-;KOU*9m#;(/CbO
C:`^:GXc<##,m>4`0DG8!<*$rH@fB+5\^HlGTajOIY)VJ_h&&f6p8RE!YETY6S0X%
*'Qs*nIi&a668D9C2W,];D)K)68War(=Y(5..OSk99oZj59+4Q$"]9s64b=daH*E_
L-dm78go`Fi7&rAPiS-6,5b22pb=P\3fkZi^fj>a!p/r--E'o0"tIBE.5.Vn3hkJ@
A:f)9/H8Np?(`W$!k>OG4@U__P<a!h-I=fk7S/8H#)Ch6jZG)%/LVpn2DXCrTJ880
-96gB`<6T(k4g'0<;n.t_^T88XO(A8TNqX;.RdBL-MIUm7^pMQDbOq!Yi[_l+@]a4
^=)6uWN%6E*lSL^s34*C^f7mqAp0ug3R4lD$^t_$3X"A["j:@Mi"B<__"j(F+QO6\
K/C[6W8U3DAO_G?^c2IiA-QNT:o_2m!\3@u/:RY+#7C&'MU4B%r_6cs"Q3bnU:aVa
J1j:&1h)P#Ye!FL*u1kN!<uRj,/ZPf\o-M([D41sac&F#gqLR%P9=!qX'DK9;'&4S
7YLLN0c)2EN6#^jI7h4*Cp^sR^/B`G7R.VEl0qkdGR%r!T6%ZKN8b#e1^8]]W.Snl
@Z:Y2o!YK79'dn:^bE-29irT32T&DqA-?1Kb,_@r1=3`f.l7Gq?j)P#"9];#^fUcW
5R'i:/4rVmK=5&4<aB7J:=S_u9gA^Z(6S4t4=!t&![*FG.&cJD\KDbK!,Nt.-JAG4
5XQHXK#4f'YQOr<Xb14B&XL4r"P6';?RIa?@X_sg4p1-W+b2NTJ5QP9>'tj.3[eH[
KNAu4E!>/e9.C];bXi9._OL]ZB/R.Ki)g+)/-SIEGjJ,R+;Y%9A-A[7>tEP^L*e\)
1cpp-"3p6:+?0N+MZ\Jbj[>I=i+FRW&7$J,8juc/7Sj,NaHC#l"XFI4?k,?\Ou=Vk
:dreUkRMlO;O2i(<ZklE+rFr>e2iP*).M#O#l]tTI!uJ2pF=+6jSEtm&mOBc8g#Mb
"+g\aC^5K"en0/C-VspkH3&O7!rtRjXB`#<)\(elALt;hd"Z_Z1s^[l!FQQ##d+0c
(k#drElBHcX:RG8lJXu@!KoDFTQ7tI5'hqL"_cs!5Y@oJN\4iH8kn&4Ao+:ZZ@O5_
-g$"+K5;q)$T0:!96TK9M,l[VP"PdQ#Cp_F:s+@,!1K%\DZ`0[(H?4tg8hAnDl2<E
`Raf!`D-^p"TW!:J8,6tr8gAm;C4,?J.r%"/d*B,dm+IOokf*@_\kg$3P\`$+@-54
%b##X"@,^A"1IQj%Y!Vd"33-<XBmE/0Es?"?\`@uNUFqS9fsul=`T'\[n0[\P&Bp+
L?6l@ZkTmLqJOG0=XbsXo&ru'Co6,_#U"^(+E:R1^rG"a7A[AWC\`MfW5dH5f?:`_
LU_C@XJ8$'!^J\DbH=S_:P,=Jq]JOi?n;F^n-*2E:P*6\7I,L5[i%L_B])pgU1hLL
>TdRE0I?/tQnrmeRj<UV4mKn+./G^73HjGUF(t=LAqX#(.2o'ZFI$S?pgRHc[$[!&
0r&K1#EO%El>HYF[J6nKjjl_p@fF/0Y!@.8?uQ8<a`rF1+[q>I#2iMMAqiQ73\224
<Pp5*M*6NP/*e`3Pbt9l<l70Q;!WX[7lU[&EWs7-"!s*4?pY&?8iFrJ?D>Q%'gTdW
6ES<m"9oL2,D%E':nLV49$9QOU;X*a>+L115XJ7270!Ic5$J,2:M?@XbH(sp5UV19
5tsDh\LsWm`),-1>k(oA5R7AO/8knI<J[Sb6XPaqi8t`*6dI^pV>54K8c^L.rY*[G
#YnNtVuu`GK?V=cj5_Q10;^H-%0q9MMb^YaCl4Q),iku*P\MEgj94Ca$D88dJ6E(g
KE1Rhd5ejoj0nTJ_ENsaS88V3,!fQ##b#>a/32S&M=q'>i;hQt7VP%r7(rc]DYnJ%
"Q2`S7H$[F'7#p<7rgFlg?^!f>a4E9<VkWKi!]U`KPt6n>D4K*/7`Ee>alj2"i;B:
6B\hj4L/??!A%%J,$ZiXl:LM:7Dkl%?r@0,lNX/9P]nCJ9cu=:0mKUTe/MN/=t1pu
K&*M7f0D:ui,/idOpBoo#'*3;,a\^M?&eU(5(f2[@k,6FE,>SUCno?+-gi:r<X3D"
j>N[((c3Du!-]^f36!^+$T)?AGYc2F#/o:#'ge=#;J*jj^=e()0[aOJ$tVm.lf+?9
?mL(!%=k)mP9=<<88TSSQ6QGf=eZ7PL++DK8dAa+8;SN6-4Q9o`aIgr2NA"dO0VQ,
ejqMO8rI&o[j5O;CF=<uGkY!sXB)_Z<?]^kquD0P^k-r,5[>jWKE,%0R,DBu#!o!X
DL6iN5\b9e>1fQk"Z]`k5]MVKaalf;8hrB-=faan'Ec-H!Lce1!(Jo*Ce@0^*D@Y2
VcGBp^,p+:V/QiP<t/>'&cj*p,fIh.+F$k.WAB=.F;Eb[lM*4:63MgX/dQ>I$b\mB
Ad9Z1@["r*"mmT<TEE=D:nU.1n7khr;4/FNdS!hqgTcYO+*'U`,YUtn1p.%ULRuCS
9`Su9^lesgGQu;OEFetiQT'<OOZNeq5imMBY>J-S4BKJJfDo@b0nQ#cB(kk_/7_d7
HaH7ZO<Gi<IY4H43Gos53X&nM$SM!$@g\&qBHj05?Ml^`L*d$'DIf`F3JN54LX[G>
/0\3Y+DUV=Q/Zp`%5)VE_K<\Ej/=KKUR<@\+_H&%[n!?Dg'&^8FF>Op[3<debTir+
-tUn9?l/l\2UcQV"@-9!0$lgJ.TAS^[fD'cI<m36r',Ga+W,]nG^E8]4(uJ<`0:Z4
a/m#u8s"_a#%2-9TO7q6<FnT?h<Mu4-`B+!A0EC&+Olh^-I)crbX<Z`VE%A!l46tY
JcR&t3o(]h`3tKa?s^7n5XnX;&Cr8q[a7A5Q?Srud`Q+\S!R_BcrWf5XQlB,SgYJ9
/B#`3_M2_d3T.o=H]I8P$jrUL!WX>HBLH#+i)Bs>?3WYo",A-)@tFmbF9nOu#:._I
K62OUF+!L-"QjB'D;0hu\iIiB]3F_RJ3F44$?h+F!GaY!/S#$NSt_PWiPbcZbXlcM
j_SS(AE%Td/\!>6$[JaLphEWb,r_3l8ulIik&l0ZMb\i<8--1r,*[7AK4lZSD=+o%
pk!<>fp4r)Aq>&7ASTHn^a.p:@C2td/t.f64%kJiXeLQ%N&%^bic8lO,Q`.j!`-H3
J9V5!!&G.>!TB^XO@gl8NCTcVd,\k%*"N;6YrIt=*t<tB+csWi0HCf5_B?X-3`$=m
"@>C>Y[fR/%#':@^gKDQ(ClAA@;sRe)@R"/Kd2.fUfK&c#K$,eE*Ok*$&/Pui;HnB
*Xi2T@BfgR<@b$OJcNS_//Ag&"9Nc$BN!b&!*m;>YZ9QMGQn8$Z>`ng$j[(@_f\fV
O@UK#K##003-71u$\a0tcp0E9(CUJ![c!f[6']-96!2oU*"E@LhSL2XW+7e,YDqq"
l"5;n:'lJk^jo.L(P</%`.B-lC-fu'"p#ji*D8U?X,"V;0d)-'&A&"\!IQ<V7PkNF
_h$bHK;p:7%#73ti35Tq(CUJ!RR#pt+q]U9+__3;&1'Sd*o"%%ZS]dUi5d)KK-7*:
$Nkr&BG(AsE"3)L5i>NZKjc*))?^Co-49m3@YUn`$ID&*K#*U$'0orE(^)e58/`$t
a]Kc/-%M0B]!!k%9EqZD!"K/5i359WKE3Jf%0<+]#SI:a?pYA*N2nRt116k>cmg/Y
<!Z$f0F.`1i'R.%a3D[ZQifV33"Ua:j$:,t5YTQ_7_iCUmfUB=ZK9H7Qn'aL%<sq7
KE2\s'`t%A'$Gl@GW64e_:V?_!V;jH7Kak?8e_K&o]3oCaV[hk#9gTV('UA[56X-s
A#?<%o((`AWM#V"$I1pC9Flb@]5S/\JH/dk#%<$KVZP6o-4$GEN982XPCPAt"+hqE
*J@/pbr#N0O>rgY.?Zc9/r?eLZsG7L9X=aB4OOAZ'ZEHP<']@_"bRrU7NR6`n5]oP
eAsBU.r0)O0<C?UEGC%\8/.7]M\[Gj9JALh3OjU(Gr!V2iuKBG^nflu1No'kQrg;'
3!lTeKbm4iTeKXV1n\M'$%u_X?4R4#!)sR5aRYg<"(9Se&VC(PHk)h55YMptiK.^k
K9>0I$Yf8;Z4;P]^e:X./SrQ6.X,8UW+N)?2)k]LFp&A/G*jPSCc>6MjCQp#4rK,"
&;2#*iH@ZpJcMH7(h'RIg:>",H;Vm4$!Tq'!3P/oWOQ@R8ecqe!'Uel^lU)Vn=.K[
#m-cI!"i7VIO)WQi/J9P!:dWuQ%Y!*"qA5D47L=9Z=$3CKL"04#6>r$#;gMN=<c(t
P5=&uqm--EkVM/A)-d<\!_NUu$n[2K"lZ\+*X''SXqCsV6TG)J.L0&FheKAF#,'<[
JX$iN^oD?K/#fFu+D;+4a:_gZ;1-023jI87$j#bc!ga"0KUkFTDM3P#X/?")>2V7A
_!iA=n7E0HLaWF7W!rc.@]rFuP']X*OeBPs!ru!D!5LDt!Mr*h!B;<8X8or8(Q/^;
E!l\s:tU?jcj7HLEcVEV#Q`:M"AWV?"-4k2![gSHM3DCtB2S4$:i6QT#SomIoDuud
"p'6N%KkXT%3sAKh]qcB!U_g6//#%+dUC1.lQd#C0MDg>Lcl!Ylk0?JOOM$%_Bj"`
#8qIrP+j,L<C!&d!V?'k%"qSBkFkaFY]:)%E#JdR8CJD(%0?OG;$#b1^;U3X`5uJS
6u!HB'p(fl_72?,5f=54cq4e!80(XnbrhErklQ^"E!'Vn%@L:n!WY<!-3V-L.W?gI
MaJt@7Td:("h8hUE$kbnQkHN"CfH5l:dILgAHFPp#RQr.1[Nm5K-3ts_2p8Om`>Ku
:^R4Dn_?Cn"j9b(-JIMeCJdf\6H)2RA.HaE!jA`RJtRK"_0hH4m*q,K&3t;o!]QhV
_KSUDT\pkBVD8<USJ=t5$Gd8t!XVTI(uQ)1:k9Vh5_'?H7!TbRK(_.I@):&)KVAIn
+pHp>,(qY%%DgsV2B]@CK:/G=!F2F(!+$V7U8"Btck_rj0Yi54<X$Z^$o0C-W.:46
"O>G12s%=IRi%(hSgbRq"d37AFeiWFq$2CJd$k$.'.6Jt7![]n[A6V5!Z8a>ENZU)
=un!6jnm^5;AD\\O>s%m5SRTrj:aci9F3uu%8d:"$E1a%&ece,:#s.&OlkO&Lu$)r
?uQm6$BtXaS(02A-.nFAN!o%gIO0$rGhLYJ<>78f"9>0J!ctCj.hF'4eW^aLi)\P3
_/tF/<1H"b..e@\#($W?T\C#2:eg1e2S_EY!-V4:>]JU[`^H1/!$r<6EOgEcI6dp7
YQe#S$c%Ljh\1\4?VlVg!`B.+J<PHB=^8g(FkQo1QWdD7W$83+9XBo7%r+lG,Dq8q
#:P3i#!nV!"X'`MQbm_CJ>qW4k&OB$n4!du]YXanR1OqR*!&;DSkVYET=_S^<Gk77
,="Q<Qcgt)N_,G;L)#00_E=-I=="/ZWb<jN8.7d\-mRj$0W0NGBp/H?TuT.>J=n/u
!FR2T!$D=C@oUdr7K^4%,#4f`ncr<De9W5XfWD^P9>Ka8"MjL:RQq<Yf-t/j5U<k^
AWF/,@D4)QFJn,O]\aRd@6/,P&1NC-8t/ba5QJu5glOi2JP4ZG/PZG6U-<B4]2*17
X#m/8G)Ao%-3kZ`No?J&'I^nK!Y'i2.]KRGJ?m_(`of,q,V>HMfI6o65d`YG/dK3P
1j$&o@`&74>k?[*f;,[Z(Y"<F'+#s;J@3srA8^N#&.ZKf3t`?S0SECCSROi8!iB,c
g7)5\6)n<)!ItS^dNb4)7,>8G^'2Falkma3rWAVo#,Frs9UG&K>K'+nAI1@FQ^Jg1
1=_Ej5mSmq#aZ421?/f_U'Z65HkZX48dDCKAHTpp&qR)3Dk_lq/f\i"^i2=A!O+!U
f\r[$?.HO/gEQfR]F]]8lqU-#8HloZ)1pP9i=D7Q80.oEZ9qf&!/LWDM#h&eYVAT6
.RcA+K.W8.Tm]1M(egm^arBp@=ti*o.n%e!)UeJodO,/D-BnV%'UT.DZj']k.,fak
>(G@2$pWCOl2i(]">#sc!WZUD5YN+rbUU+V^mGgF(,g%Cq(<p8QJ3"jfeo8qQs!gq
'pc/D>VQW"-M8CWSNp[6;jeUnE/.2YM_FBk0Jg/V/%l"`U'EuO+pK(j_105qrlLRs
UZ7WLH-@,S?][>(J:lB+d2Kf/G7.fI*,sOU/-Z+d":RX1%K"EY5rpFYFc>!*0Y)D4
0FRtIPo1Ia)rM&5(orOu&-5TK$bF+]8.'o?blDHN-YXnVd[[]IL`"5U)&l;P8eV6Q
\3ENG3`+.`.4YF$j:jkhTS#]AZ4)S(m'QQK$n)V#9D&ccW/HLg%e;(u?k@na'EJQH
JVuRZ$i\%S2T'J6(&S+]Zi5J+2h1r<&Y`%5&V25gL:[gkOYQ'M.'8[0Pe-)t^r!n*
+VP/<,+W-+JDrAUBG$oR!Ln)f!CGP<J[.]%o)V\'ZJ#a)JH$:E&":mILsk=\M.7,P
#VAR^JbU7HgN\X,TFsVK](j"4bQ&75bec@$N9e?IJTDKe>Cd&$!A^./p_SK@(lX@H
_mF*sP\J-ocGOW$!5JmKZ/7e!0qn,aR5i["d5<[6#E<6mRBYn@32lo$^k"3=7-&Tj
kbo1]LTUpAJZ'65W"p7bad[i5$fPe:@.Sp\*<DncN9c9LJ_pq=b)>5'$bLAsqR/R:
bG'LnUI2,ZC9f1B('.=q1WTP%#Q~>

Q
n
Q
Q
Q
q
n
213.24 737.917 73.591 73.591 re
W
n
q
73.5908 0 0 73.5908 213.24 737.917 cm
q
n
0 0 1 1 re
q
W
[/Indexed [/DeviceCMYK] 72
<~d`0.fd)Ee]cc!PUcGI8Mc,%#DbeL`<bJ(K4b.Y9,b.P-%ah"iqa18Kh`j`3``O;sW
`3laP_mHOH_R$:@_6L"7^p'b/^TOJ&^9+4s]r\"l]W._d];_J\\u22T\YYlK\"oNB
[\B39[@s!3[%E^,ZC[@$Z(7-sYFC^jY*kCbXI"tYWg/PPWKW5IViciBV3$K;UlL05
U5Xa.SqhdrS:u@lR=]bdQ[j;\Q%!lVNHT4?Mf`e9LiI21L2Uc+KPbB&J8&NoHY$Oa
G@=\UEa;`HE*H<BCfXF6A5Gr">Y.?a=%,CT905*58NA^06o?b#4"Ml^3%HEX1aaUM
0dS(F.Nff5-64'+*uGgp*>TCj((h,Y%graFz~>]
cs 
<<
/ImageType 1
/Width 100
/Height 100
/ImageMatrix [100 0 0 -100 0 100] 
/BitsPerComponent 8
/Decode [0 255 ] 
/_Filters [currentfile /ASCII85Decode filter dup /LZWDecode filter dup 
] >>
pdf_image J-#`oO?aWm#mCD3J=o.U((,jc+[Ft)/fP0%K4@aa*'b;I"G;:L+Fl!O"Tq&aTVrhS
57<e#@N`bA:`UI.b5i3C\2#W;"p9G7n5)#['nSb\F0KcKBFUWR@drU.2E;hVd=L6V
E$u2%YX`8efmSlj1TaL:Z,tf?TFD.F-4j!1,$5)_6u1D)+9V`J]$[NSR\XgG+0*]U
+OF4;'bQhVZ2#8RdOAD'>2YUeL,L'<#=.PCn3e<W#6b5"Y`"`D/VK)AZh9E96Q%\j
b%=[ZVM__li*u,"aAh1AH\HKVdbQM8STr1LXq=DdhXan2c>QP&YTs\^dpqD/=r&e2
^o$=o>Ut=m-l*0aWj0/@eh>_':#UV<B/CIJX'hkSOsdHN*oaH'4$_Psl)LB]3%SR6
\>JMrEpfeRHgpj/!)&+O3fZ0-&[%d;.%rU#MsU;@l"e!8+AFt-V(0_FFLJ,>\/GYT
@'DO""CW,q#K)JSSs?KE>L3S*/^apf0!,[-$3K/\4:Qo#Qm3eBMQ>=*UJ+VYJM,5!
3!H4?'Qf,'CP5`b4",Hb,qG-hSE>@[0EqQ.NBeNk8F]pNYG!L_lGu/i&f0ZA$I[MK
]tgj)$7ZP/]gaESj8TY.0KY1AK#%Sn/?s6\Zj>1kZqq#\/G.lk\?0P""FuO9B!90h
[$(SG;]GNOY7LI6"i:bG%"l$h/97ne.+;6%YY)4<VoL9m#r3\iCrkJDP[g6I\r`\G
XuNEu4q<3CbA-G!.c"!kX\MO2#V1^_i?BjSP#DN/9e$j]9bB16@8/?^WCjb#K#!VD
5\m'&.s3^D3F.Fd4JoP9_B!f0L`1/a1U?j.Pp$RE'84:@6\0<25bi/9=-Du"mGccM
UkYV/ei:_o%eAnb=NKh!jWZ]PXJRZ<6m)fFWlhB1Y?@m%'1e!UGFAOiBGLiHDT`C1
Xt[j]8tn0m6jZhp?CM%6P@=]).B7DS>r_\tmhd:+Q7T9lbLTOs,]3hi#Qd(of_fU=
^>auVo."I7lR8pEs1,D,(nYfs2X@-jRHF4aj-k+\SRUfkW?tI8C9<AuaCK-MT[s7+
-8?9raG<*b4B8kp>A$<kFIBFaPh-bu+H83RqG*8f9,qZMAJeZ["MSU@=l3MU'5sjK
Ggj?V._LBE_q$gG1L@l"bpt\uQ\<;Kig#CV_Gr?9-Yq+'HIMNPbTq)!Ne9_n`Ds>i
j*h+?fb5dr.('q5=F4%8M`GZ8H^>J#gC=9>.P+.G.9ETg&D@aRTGX.9Kih'jZ`n?S
KVQ2W@-=&"?6^nU[Lco@PLeE"0SRn76`$I_>S1(2X3nb`;J9YbZ1qsD`6C$SC/>:j
C,pu&<#\o?5g'J+-Enbc]2IGl5UZa8A>"[Cj4=o?g"Lgm&Z[d@TO$G8o-VM&!<?*/
=OSFL,)?[[USr]^(R&5f7/8;5E%D.Gj6A5:*\8N<Li6+Qp+*?IK=dmn:ucq*4[f\6
,)EcV9;;<-N*+Q(7AD(H*&gYF2:[i-2'Rk0W&CKRmOed,FHZ0OBT'*UJ?UL-^t9N&
?q%Sm.$EF].ki:Z1^1Jo>&6f8br0L%jMG&A!It^a2'>2n5XUGF=B*^C&`R>h7]tiE
@1k3W+n<fEPY9-&&n/kI35-/A"G"!$"+Xbc`huq5B/;W!$)-B>C"k_7MhD.*\n6JJ
FQ&[1b<sN?W3(1F=;n_[M2:8%9?48[a\lgSi'b&>@ZN,gZDU\Yq7Mn*n8mg9_cfb+
"<In4JXm3>,[a.N;F90J-ijfg;^KL&)D9S()eT4;8M/B4??/d,i$)m.#K_9e71i'&
!ant7aFou_5XV#*Xmor.\^;?oD!WYX(uDDA.\0?eC*Ei@:;-?o71m(>WV)(\9^9M%
Tg^n)#5+Y5Op"=Q,i(EP0!:Jh4P(FM/M>7>F-u2-i[DopM@mL`e\EM5'k.+j1NHGQ
fKaYLgmB6]p6ctR(A(NL$WC%>ju80$You(92PqcPf&d+n^kGHeLN(O8ei=/sZC,U+
_0[mdS<m4/eOOa6!_)g5[od*kB;EO$RYIF=ML._'-Y_58QooD&V%uLTJSpQoApP'<
k^-\]'0%E<r4ld_M\0LH3\/3<:XL4e9'0Gc"dH`25mjT!;[*7X8L=mNCb90452N#C
[4dNd4%^*`h52\&04];^..dpMb<4JnC/91P^)O8bW2gXhl!Wo.MC14i74[&N-\V.:
-A(.Y!4WmKR1<XrC:af;\O9X)9rbhE`7Im1&j3>RFIfok@\mor/*?CdePI_!_'gW6
!2L;1E(kX1q)u_F#_j[\/Rfi^bfV>.PU^,ZZWD0O8W8qAB=2ig'E(T+./4.$+BAjN
?n2AQHj`lg-<un#@?'2-$3@Q_"_6g/_=$D0'F4,*VGu*7dU7eF!#_D/NN>j`#).W$
4:FNs5mX.m*Wn)s#XH`S!m7h6)cF23J7/U/ApG$j3=H'(ejqNQ,_YFY,`Aj76)qK\
!Kd):Ana9g!a0m\JhU"1!SB^ET`?'acpe3>XP?J`WY;<"0F&C_,D?+P3gfSr[@&KW
h__]l!9-S5'-21h`.e]2PL!:F_E\<ur$67.O:MAb.KdJ%9HZ0XgSi!`4%.NTWg-[q
p9N*,.-SaMQ2$"gdH"Q3:^dA]%q7e#"T_1g%>$iE%DhcK#ltk_!q8Y`J=5Ju[;N-]
Z8HStV,`X*CO>V3P#e:%rR5JaJUi7RT)_('7gPmr!B_2&5gUMUT_'Jud"2]-=<@V9
$jtc<PLHZP@56+_[5Od3N",_jM+NtW0T;p<J?TjmI(Ec"c=Ob@\0(piZlK9E)A0gd
0a,::%KU$o5R@:b+a$b]X0gnULe/dH/%D8pLLs:?d7(erL'VS_5:*`l*<[Lp)hWZW
$\8j2h#LoHbXoHr@7Q`\&.RKdo:mka7Y:ce4`41E3s]+0l:QL2%YB45$iuGF"sC\o
!WY0V'l+OeV96uT"&uKTOVrj-QdVEQV%sV>a)-aqjPK8\"T[I&"CRH+GsgLT?n1Xq
=G&t%-mMdc8W]U^4DbG04m4A-k*e^H<2TfAeA@q9$?uY\4p1jN>i7N<U+0emUi;#i
,\9T-n1'r%qGkCk\)L"8K1`3iNe>22i!Q\J,8?hfJs\tPh'V-XK=H<g4t9"8DTB&3
8[pnE>4+d6-qLB,#oO&$#"!s&!g!KFTIp<KN%P)UU5bt+XepQaBV3@08Lti3Ka]Yh
HMus.3/;gjL$!ho1/b'nk\W$`$.N75T\6>Yi'R&qY^hPknjC=5H=J..&>"HJ<saMB
IGu[%9!ZkSUnWc*2WpT4V\io2[K23nOME+jU)H+o,nTPe=`G4m6NeONE%D*]/Yom]
TH\+P9R:5e`P\RcbQ9kFDDWVB1;b#UAbN9ggoquoFse9Hlf'>QE&bcgRR.iZL6O;Z
Z>jJ!!^JffA^UX5;ukpX;Xp'n8l/uY>/L=^'naAuk;8G2p1MET2D>WR/FW]+gb*%c
g/+*=9RMJr;B\A+>@j><kSPYoQNi;f^kXD6A*g`m*[nfJf-uBt+ps=h$F2u]+!pM#
Ae7.GbURW@+D-Eg`ah[,,d5-O:-tNPKO@Ru$34V(,\,]LWJk:3dc:k-<6!/cOtPd1
`u1m0,:uMlCA_1rhUj4b-4iL>#tuba/3&D=^Pu3iK>p7;n5o'8[&,1CBMt'mKI0TQ
B>=WM$(<.hkcTT\"s]@FWotVJ/k#2(E/!l`nM;;KR_NL6afYdtA[!V="C`\`Z3a2*
95Jn%%W2AZ6%ZIH`1JNAdi##D;(p-i`+(5j57iG/cXOd.jB>BT5!N`%IBdfG9*-K$
#a$[D+u#g*8Mr+EIRRiB-c[Et!eAE[IOmk![]7."N:]jK/8Gd?33q]O"Rq#$S1(B+
h%4P_!X0==.]FbH,HQA0A*UN*cm=m%HW(J2/,p.?7_;*&Nj6hQK#V4-fNRLUBBd87
.Iu(U,/:nrlQReYi!2)Q^/.AMV8Jb1c\PLh[K>AJ"2H\m0&#0V&?is&PR%\HLefQH
9VUgi"G/3h;llJ0YW?<:KCeYo9U't%Shq*==](P<L,)jr+p/rMnpiK*,-&MS==!M]
>=;O3JpJb?.Rmsn%>-P??njn/kf"`NSIu.g"]Bd_^9";[,Eo.?nJ^\M*1%?k66`d2
&'S6WA=Z>'fSPS@C^/aT(o`Xf;WM=VVCGcG$mR3F2+fJX7fp.mi&J]YjN=;?_t3rq
.WU3:F9bp<b>p^O/mZH]1M?Jh6RF2`5g'42@Kp)-P.2]NG/<a83c1K]@e<Y/HA;g"
Ee;CuX\("BdmfG=_ZS>F,Golu6AhhBh*kqgU;itfob\l6Oi,`qW'EDkHH@Q$+G=/J
-]pAFHTU?%+fV+WK>A:>6VOQ]YU-GT7g10\TK^B6LJL%:BCLfd2HarnQK_RR2-!bZ
jtb%4>>h=E+:;LF:oS<96H]N2;KbG5"O8E'.O\-c'fq1?fT]=)jAYDuDrPg?.,L4R
<q4\(jcisUa]n?<Ofkq#FR2)3,_SfK0r[nqbAa.k*(tqI61H_<E%3Yq(ae<AWGXj+
KI0`;1',[q9;<noPX>HtC9k_oY@=)a#%8*\K_$J[8W7JB<Er>ib)8h,I=bM?lBXgr
AQ%V`8T*uf,apS%;R7TfBnDOQQ>DJr^30WK7"arA63\_HlmRo]X%nQDVFlg/KYMQV
BpCHkUu',O,[P,$IWi@*W!QTnFAF-+.4UNI(._6![Zm*%2F\Bb`_nEu<f>PMRDk8.
jlB3N<g^$e>`F=8aMhdEnB.'@H-8'a$rT*aKR"9c:FWB,#%Bf)#b*.XJB12&bRZun
@m9WaCrZ67Z4alf3-M8*-R:[k[Whi#THHK2=_QY?;`K^c_+5>*/Q&$DQMd]fVf6+O
C3@;l[#e[O'IEpr!*?7\CV;.X#XV"[F"1O;W\IZ:Pb89p6--2OMVW?1i>f2lN$k&>
2*N1_=%EdbFEYl8pAQ?M<1F*SIZULrAiMB:]W<TDGm4pi<JZpY3[ls.^S^^//n-?u
V.>KR0l8'r,eJS/,aF^7JEQK&c%8;RYsZSq'Lad=6OaL"cV85T6''N(W!c&cZ[idl
.<Ur,_U]l0&I_#0Rtmk,DGW,?,c]kX;g'Qu7(n5n11Rg^q8hDke@e>8!/^iH7`@$,
-+klFaMmM/KiPsDBCcBB-t%lIHL$#,l>%4`E-5WQ<=&BB2L&[r%VoSs'C)`pM7f?7
KMt3\WYf]=,!]R6JU_1EJj[[Q,>(aS$8_j3Nb-(*QZ%f!:Q-.aHFWfhGK_1]5[WO8
/=0Zf`4o3t#n>qbOhu"aQsrm;.!#*NO3(1]5StUd~>

Q
n
Q
Q
Q
n
270.129 740.797 -44.143 2.09198 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
270.129 740.797 m
225.986 740.797 l
225.986 742.889 l
270.129 742.889 l
270.129 740.797 l
h
S
240.617 746.181 m
/N157 12 Tf
(5) show
n
241.963 746.689 m
242.456 746.251 243.093 746.032 243.873 746.032 c
244.825 746.032 245.576 746.38 246.126 747.076 c
246.578 747.642 246.805 748.314 246.805 749.092 c
246.805 749.908 246.547 750.577 246.033 751.097 c
245.518 751.616 244.887 751.876 244.138 751.876 c
243.573 751.876 243.033 751.697 242.519 751.338 c
242.98 753.649 l
246.398 753.649 l
246.398 754.657 l
242.141 754.657 l
241.305 750.243 l
242.297 750.11 l
242.453 750.357 242.667 750.559 242.938 750.714 c
243.209 750.869 243.516 750.946 243.858 750.946 c
244.407 750.946 244.85 750.772 245.185 750.424 c
245.52 750.076 245.688 749.601 245.688 748.999 c
245.688 748.366 245.513 747.857 245.164 747.474 c
244.815 747.091 244.386 746.899 243.875 746.899 c
243.452 746.899 243.091 747.035 242.794 747.307 c
242.498 747.579 242.309 747.984 242.227 748.524 c
241.117 748.431 l
241.188 747.708 241.469 747.127 241.963 746.689 c
h
S
250.625 746.181 m
Adobe_CoolType_Utility begin ct_MakeOCF begin ct_GlyphDirProcs begin
/JVAQLV+SymbolMT 1
GetGlyphDirectory
80 <10bf31703a9b8a5acb6cc34e29a78b3543a02f44016a183fa96ee22a4672
260280f37155abc7c5dd97ad1eed691514dd9f216a99d6f5b4ee5ea0e3df
6c86a85cb1432d35d8f83e1dd0e44a84390fd2f3a1bc7a09f154c36bf455
f4e857f45dd2fe43a0a4ae4c94bb93a23f7c67d5a71adfb73c796b01d659
91243f757228ab435b3e5d2cc3be58b1b0f54c63f9a199a520853094fb2c
45d796cbff56c5a93e203b5825ac6ec7293ac1040f3ebb56f6bab9aba62d
aea3cca824d247bf924306d142b5e90d84b404bcf2de9e6844d2f6527427
e9e9b39dc18696fc835d944e> |
!
end end end
/N150 12 Tf
(\000P) show
n
255.215 751.548 m
255.215 747.51 l
254.93 747.24 254.648 747.045 254.37 746.925 c
254.093 746.804 253.853 746.743 253.649 746.743 c
253.477 746.743 253.305 746.794 253.133 746.896 c
252.961 746.999 252.842 747.137 252.775 747.313 c
252.709 747.488 252.676 747.775 252.676 748.173 c
252.676 751.548 l
251.699 751.548 l
251.699 746.88 l
251.699 746.552 251.676 746.154 251.629 745.686 c
251.602 745.412 251.534 745.092 251.425 744.725 c
251.379 744.561 251.355 744.424 251.355 744.315 c
251.355 744.093 251.416 743.907 251.537 743.759 c
251.627 743.649 251.742 743.595 251.883 743.595 c
252.02 743.595 252.142 743.657 252.249 743.782 c
252.356 743.908 252.41 744.076 252.41 744.287 c
252.41 744.408 252.373 744.619 252.299 744.92 c
252.193 745.343 252.145 745.837 252.152 746.404 c
252.312 746.271 252.476 746.171 252.643 746.103 c
252.811 746.035 252.982 746.001 253.158 746.001 c
253.418 746.001 253.728 746.088 254.084 746.262 c
254.44 746.436 254.817 746.744 255.215 747.186 c
255.25 746.752 255.354 746.448 255.527 746.272 c
255.699 746.097 255.931 746.009 256.222 746.009 c
256.516 746.009 256.759 746.108 256.951 746.308 c
257.144 746.507 257.273 746.868 257.34 747.392 c
257.098 747.392 l
257.059 747.103 256.997 746.909 256.912 746.812 c
256.828 746.714 256.737 746.665 256.639 746.665 c
256.56 746.665 256.485 746.694 256.415 746.753 c
256.344 746.812 256.292 746.907 256.256 747.04 c
256.213 747.227 256.191 747.555 256.191 748.022 c
256.191 751.548 l
255.215 751.548 l
h
S
257.539 746.181 m
/N157 12 Tf
(m) show
n
259.385 746.181 m
259.385 749.412 l
259.385 749.979 259.441 750.412 259.555 750.713 c
259.668 751.014 259.85 751.243 260.102 751.399 c
260.354 751.556 260.628 751.634 260.925 751.634 c
261.315 751.634 261.596 751.517 261.768 751.282 c
261.939 751.047 262.025 750.695 262.025 750.227 c
262.025 746.181 l
263.08 746.181 l
263.08 749.798 l
263.08 750.439 263.225 750.906 263.514 751.197 c
263.803 751.488 264.167 751.634 264.604 751.634 c
264.847 751.634 265.058 751.577 265.238 751.464 c
265.418 751.351 265.542 751.201 265.61 751.015 c
265.679 750.83 265.713 750.525 265.713 750.104 c
265.713 746.181 l
266.768 746.181 l
266.768 750.455 l
266.768 751.166 266.601 751.693 266.269 752.035 c
265.936 752.377 265.46 752.548 264.842 752.548 c
264.051 752.548 263.409 752.185 262.916 751.458 c
262.795 751.802 262.587 752.069 262.292 752.261 c
261.998 752.452 261.621 752.548 261.16 752.548 c
260.747 752.548 260.378 752.455 260.054 752.27 c
259.73 752.084 259.471 751.839 259.275 751.534 c
259.275 752.407 l
258.33 752.407 l
258.33 746.181 l
259.385 746.181 l
h
S
[/DeviceCMYK] cs 0 0 0 1 sc
78.5469 631.098 m
/N160 12 Tf
(\(c\)) show
q
1.00301 0 0 -1.01913 0 0 cm
n
135.158 -723.591 73.409 -72.21 re
W
n
q
73.409 0 0 -72.2103 135.157 -723.595 cm
q
n
0 0 1 1 re
q
W
[/Indexed [/DeviceCMYK] 167
<~iRZSniRQJki76>hhpg/dhpg,bhUBo^h9s]YgsXTVgX4BRgX+9Ng<e-Kg!@pFg!7gB
fZhU=fZ_L9f?D@6f#u.1f#l%-e]Pn)e]Gh&eB#V!e&]Ire&T@nd`94jd`0.fdDj"b
d)Ee]d)<\Ycc!PUcbmJRcGI8McG@/Hc,%#DbeUi@beL`<bJ(N7bJ(K4bItE0b.Y9,
b.P0(b.P-%ah+s!ah"iqaLSWla18Kha1/Ee`j`3``j`0]`O;sW`O2mT`3laP`3cXL
_mHOH_m?FD_R$:@_Qp1<_6L"7^p0k3^p'b/^TXS+^TOJ&^94>"]r\%o]r\"l]W7eg
]W._d];hS`];_J\\u;8W\u22T\>>`G\"oNB\"fE>[\B39[\9-7[@s!3[@im0[%E^,
ZC[@$ZCR:!Z(7-sYFC^jYF:UfY*kCbXdG1]XI"tYX-J\TWg/PPWg&GMWKW5IW03&F
ViciBVNH]?UlU97UQ's1U5Xa.To+I)TS\7%SqhdrS:u@lRY6%hR=]bdQ[j;\Q@F)Y
Q%!lVP'_9NOa;'KOEkjHNHT4?Mf`e9LiI21L2Uc+KPbB&K5>0#JSJ`rIqW9kI:lsg
HtHadH=U=^H"1+[G@=\UF^J8OFC&&LEElNEDd$*?DHTp=CfXF6BiIn/BN%\,Al28&
A5Gr"@o#_t@STMq?qa,l?VEuj?;!cg>tRQd>Y.?a>=_-^>":p[=@PUW=%,CT<^]1Q
<C/nM<'`_K;F!DG;*R2D:Hgi?:-CW<9KY<8905*58iep38NA^082rL-7Q*('6o?b#
6SpOu68L=r5r(+o5VXnl4YA;d4"Ml^3\)Z[2_$6V1aaUM0dS(F/Ku><(D.5Z~>]
cs 
<<
/ImageType 1
/Width 306
/Height 301
/ImageMatrix [306 0 0 -301 0 301] 
/BitsPerComponent 8
/Decode [0 255 ] 
/_Filters [currentfile /ASCII85Decode filter dup /LZWDecode filter dup 
] >>
pdf_image J-$iY3$9+J"bZqc5d52e*YA[2!T<I#5U[EVK]6uRN(bT9O@Wn[3?Vp-((#Z20t;`h
'G$-+,19&YQnfbR9r%h.jS!mBS-G_hOP"A44J2qtK#(if80ebn@f]u><dRgRc3*ZP
o^]CYYQi!$5fB$I71<0_;#ku%*>>nM-#kuaNj06&eh)(gLb])<KE@kK.]?N>15J]&
OpdP,D-rJ1m85tg<>tuB5lbk31a!/5"N)D1#aA5")4!cYnbc_%9.,tZj-&=o^b:M%
l_GBnc:0NoT2K>gH6jJl32P)<oaq-5WE,Tk.ojaZI`#X#=fiI?A\.DO[TtAlC9?Lg
I(nM-3'8f7jbhXLBY2(YMT:ncj`9iM/05FXTr<<;N]/B89[u"[e.eAu#uaaU2U0/S
Tqou'HjdFjqP<+!W]3>@\LMWn%CtDsY,]@SbCJn0.iLsaK.Ao>[">@4gAnA^C?4tK
BbKk(7^#/V">Bg+":2<71.&n\07t&950:BTq_D$L.&rE7@^)pqbp--7Y7&3-)m/]U
;@0B3!d^btJNV_Zc+uA/Y(N]-0TcH6gPQ?A#oqS3ck+G*6+?qNQkCbI!dG5(TX*Xu
+pu67#gDZ>,kM.09(u#2@+'<]K-9OeSg4t1h(u)<m+"sdF*-OUKX:no=ToItiY^8J
F`\PRQ0iEI,RW(TS--"\GY1V,fIJSiEqI7(40c`JPg([/eu-eLKj?`7e&:mQc\S+h
Vq+igbm_t8AIoC"5n+Y?dE%"a#h&&#.YV30PrVR82"3k/<)jr2PgoE%TFfXq-!NAW
Q&TE[=5c;](tV&rHXBkJ%>LueXtW4R8p:H(Ai-II_.Uu0oPt1:$Eb%#>:JXn=/WG/
mZ>aIC56b(W>,@th"hA'FPV.Xhfs`3SaqSCi(fUa;bS5/:ScVP$%[\Q/CB+/1`dH7
iRiBR>1`P@.uW#HN\ufKq!:+8=m`L]X@Z)S3AZ8EXJG*\TVTmiY$:d5Gp]LE.nJEf
]:UAN\t/if.&d:6$)DQq"*]DSHAW3enXYoGj<30&pa4XR-4qI&s"k2VJG;I/K=Ta@
f4DU0;QXCWmGAgAMB[&lKRlIW&_Oo*0YB#2F"t26;25ZoJg=Ec+$Ha?V8)IAY4eCS
]Fn5AE)_;o%/KnL1RmoJa)-<*&Wern8%bQ`b>EGl=4Xm!/86]TSK'9H>:R.*!+"+V
FqEs[qlk67\CS8kcL)GE\iX;"hLW0Ln6R'QGiVT[OOof)hJ7jK`,Y$.#H.f1X4M8!
l!_:k.c6j+i,A(?f=j`dq9#2WI;MguQ3Z@P+-Z;2YLV#bG<5`KPG*KQ1&rh;:?l:E
Y(9,`ftc/Im=:]<<mXFa5se9LU6HJuNtIF=ZigM<;$)&U[HBk3+<m6d8P1^c7$Z??
fU.P99o,XfJTDh-Qllb;?mL:'_c$;u]/b#V$+;B@Y)>lH[YP5El[]7>gnIAE6Lad:
PA#:/jANku8]7Ju:ft8"i_Ci('o)jbQjT&X-RnKk;bL8.g&\6/"=>];'4bY.j,-d!
cM;WRB#LdGb&38Pp(p+&r-[Q-=ccMm"A!&6+pc,E:i\F%8GN0U,`sf["K"gD."7%F
"IqpP%2gAS6Em:)DO/_D&B^_?.hi,h"d6Y8b:(=]W!'Vs;Y"un;(41pXM]u)[%><]
+#7L"l]Y7*FNjn6+ClIGOR=H48BJC*A:+eUb>N<r`AoqW/E`Fc<VOVgI7:&Z>+Qk.
H*dnCL!3]=6diDEb8FqX.KolJlB7Jo#2W+tm.=TUM<b0V$Ha-(X!KM,"h4dC7S-07
U[E<,9_t.3hhl'%oWb$?RIr/0i$Bb$Lo5h+M?jQ6,u)1WM1_8``8rL9Y=]+CJnhYf
%F]<u;eBH*JjOOo_*nH$63\0[]T:g0G^IT+RL&bO:T@D1,R?rj-5K<dWgn[@bp85p
HN-LmbE4).Gf@_X#*ie?@'$c->1T.o>AJY,Y'&=-X,?LTmK#JS[[t:9qd.QDZSs-F
,/m[*Iq-eSiZf4jaira5AW?X[VU[6l<9m1V%96:-F]-VpMbc8`9CK93B_"j_?QX-J
jI\:2gB&;G#qKs6XoOWq!da(5/$M%;"Z##o>D?4\!NrY-Y/4#)%<BUnM$%oR:Y=*r
F;GCK,M#RG=]mBOM6ISR5VRr60G4Gl)UD<39FEhE0i7q_a?9t+(u6Yo"O#K/,QMeT
!Qh'POkr!mOT$.H2qpcbfr6SqJ<47bk8E]]Ec6eOIN[\]h8r=C=_'EaVSq+]Z?(#2
#/r*h\7(:k].Q/+C<&:r<u,aG(WV&]*s$=A;o'*e_sRmDi]Kh"Ys8\cfoHnXid6ks
jtk$0dG&/o7@`tM[`A]-\R[YK<H9R@aR7A"TR<)c1Cf8`p5^YoG+k1Wk#_\1BX_R.
]Ep@uU<HGT1*;dHREUQ=/31$Ek3*nWFFb:Si0-:.r:]%>mXid[T+n.B=.1aBLUqei
+Q9:Re8Fe"fJqb[jRPf%Q`ZT6)Jp:)dQ+5t?F&BgM^^g5W:feSWn!MW'HE*>XE''%
`F[99Q&TdP5cg$uO^Z&;I=[H&(3isS:qTe$ad-875pTM1"/QVr/rKcm+eV2+n$Z<<
0^^kbacgJ[dh^52kTWh4O]Rd9A@C*0?uu6:XY//Q5?MEVPN[:6e,l#=JY,50WlV:T
2KHENX#W.e8ch]2^tu"BS3#Y&L(QTiBXi^Dl'tNN'>kfDpq]DZ5Wb&D5!55n"@.kM
I3!#s9MIN57HI7)Qu_2+4B6^r"+8B:o2^Xmq1bC%SGH.U%YV#H-?1:O++sZDQ.GeK
'C"tS:JTMP=?<70iOrP4orfK-32^,7SV.IG50L&`Z#8qb8!0AOTA.I8E<CX8Q5k2/
bWFF(IU2^[o7$j>]DmPKl3!]35),^k.c-Q'dg#HYC"&T4Qh$BUW>6'lRs?'2f#_bT
*:P5r^e"e3j=&4PN2$fi3P)a<]897kJ(MDn<5P8+Em\_B92,G[1DNi'[ibHX@c#At
ZA&GC5pCW>V0ZT]f\Ag)]8>*<,m8$;KO$s2<,V>QXQgDdYga*(DMW=*`5qj!$N+V:
ND)6Wm,%[c>lAI[rMhuBDCRS\Re!PArlqZ*O7N<b"TRkZdZ2sM&-UNr]#rA.-]em@
O;'/5(amZMEi=^[0I6E]fNccUA'd"6D:8<#4E3aX/^QohO37Ci;Hc_"jQd/`:g?@3
ZrKo]33VJTaJ_PRmOtd7r.5(OOF5#Dnk>,HE(@57Jip@.NWu_N"H\q-MS:;?km@T*
!cY%=_lcAR14u=W&u<gqW.7:2n?PE'`%%ofC$[Qb%(#"*#6R6LU_<Q$GVZ#eAF.8L
KqL.ME-uRlqLgt>?pn+,L1_o>DdpLl@Ra&OW2Ao2ROlfXUm+=QDO73,"Qn!H,huEl
L6KQUqr/[O!>Q60.Nu&LHLWan;6:La>nbCP!qAPlBGsP)*tFqW'`pkS,f:@SU=O<l
a\bAM6>[LAJ-7TH(JGbaUfeN972S?bM/OrbnW%q#Pn?lJ:,/?,0qqJVVC+b#`FAQ\
+s@nF/DC=g)sjN5d5iPoBcQXU-BUcWd-2%Fga#bT0+m9X1$K`r4W`TM+!]q50lB_5
E`c1^h9gTuZ32F.#Xq<`%L6ho00LId0,]LT:!t(X0r6(1di-XcNT*GKK0YmC.hE;!
=j5aNb?uh5)P09_6pm=D#6]hogmE'-HtCMQ&DmYp59.aTL5T<QLoA(*MJMO.73r0T
m,ELg,']n?B2,nULhLRu\n_B02LlW$l`_WiYTZoP#]-*F"%t0(0_08'+L7H5P0,do
E@hCp/Pp%+db9G]h_afT/oa`@b/5k7M_@DB08fKW`<@pq56aZi_F-O@UP@2q&?>=9
-drnVEud"KY;1/KL$`Vm0hF/mSu&a0l4Sno1<;ID7K`6QZB+*!P!_;$s##u#oCH:g
o'Se"B&QV^jpLc?">_u8GXdmE/#.d<o7n<lMV:\,b0uO.+WbMU:==fZ,fQ?1V>TdW
#'9%YL[ej0&Q9'jq(e$0(.]92,iV6K;'9[S,qYdde286YL.*lO7KSfKWK%-)7"3)0
@5;LTA1lMOM[?]O,a8!^;!*G,_a&%15b^g1Cs,+#FE?hk]sJh`e06p2+$u(]8Ye",
"PlI$j[]udd'Ln=KIWCHm6kZV7&2;:'N7G6MaaJE.'cJmZsu7`Bh"gc7cRcE1^"sr
X%1Qi5iSh8;Lg,/Ls8kt6-PTc!_#[[R0U*i6Ksn*1po3JW7gcG,RJfi6:X\+-VM<p
9F6bR;m6Ds>oaY)9eD0WPg;h+gblIsAS3F]Nad0ASp.'5:hD2KKAaPJFWt`I5Da]R
B.jIfW\JJF8i-9-MF*N6:;8YR+C\7OJ0$lc=WlnV6:.on8\AAF7SN0=1::6SZia:G
-WL]u<H+O+Q!U?<@_eg+<fXXid\U"uX&uH0ij"6Dl<'PFSPlNX]n^<(n?Z7j$X&7c
'0n'O#p3>FI:!9+>0rlD0Rm'clW#39>L4KlFi";1QOr;3>d:2-XC5/o4^CkL=(5lF
[GJMEG;Ea4,d^7S(-IK#ZJ'Ga6M6Y=eXKps!'9fW"Vmuc<XiL,1CM&8O@).7<<HU+
X&T7i2g/;UjMEWoRltmX"<]N_Jl\')K4'XO^*#sU!)<\-<ot'3:i#N7l!knq,fU;.
-MB?RP2e.":=>6I-&pJsk8?Y-+MV^gO"Z]&W1%4<)E#>QB7iQa_@^Gh%qna%BU8'>
(6HOf7qla[BssU(2PQ_lNCnreC=]Y*:?^k!\klGAR23b@C0;HteSR-&e'"[EET(dI
NG`NRR5XJiFV(%Gi\sp7+eq<&Q@C.r#4pB7E6R?^&5?j_BlT((4dR3ZetmD#f5fHO
CH%\^pGPAt4)?$7Sq@h$<ZYQ@8LR8tFQ."W-'`@)X@?7SU).01f4%1(.5EX!o3`=7
<<j'bR[XS^2rfGObeI):[RLB=AS6<KY4g<MABE:VDG(EjEJj4b<]/4:)p^0J[<TLl
f^t([=tE?(6j6><F_:93+]eOHjlpdoF<_UT,Y]\eQf%lr#C]#PIYr5DGOR'R?ALQ9
K9Tep"m^f#d8?8A#'(4JGSW0H)V"@PS(,`rjbJGF8k/S.5U4qQ`"doW6%e<$KIn/h
3(a9)X+_AL2/5d<dg:KgJU]Q0EgUWMQu;%g"O6]Iob9VPp_/Gj-9#%^,IeeX(-dC?
2i1.rM1bjcA<>e12di#NG/@UD[\8@^/eRKOL?."%-0#`f@KEX7cu3>,9K4Y6h2/@d
UlnG[E):<_ClW@R":ia&5T#SP=U7OX1S?M1_K`cdq'Re8<"Y6eKID1VE)o4hG"T!M
aFYbk35K,<S)]Bs_Jg-5)j`Q+;6jbrGq)=PJRq?bP>.?";#960J!:4Q.!Mp7Y>Lb9
/!V:qlRABifjFqCADehn2VDr/;W^/p[?m;0PKoS`<iEOVnX.I-R5pU`q3kV-Si&MV
iRoc23<ld7`KQ^rRWB?!WiqoCbp&QLf""YC=j2Zsn,d'GSRTF$KjUDGTglTSQXp2a
W2Z-P+ermd]N7FNC`3q0g?F8uN!&HIV$2Sr8=`MZIIel,@N#;E5/L+XEfKS\6tItu
h1sJ#IFrIUq/J_uX[gJIn>79.H/k=.+p,h4Kds75[.o!jW1(q3LnQ,lDC)0\$`=+`
Vcn?1perp,pdY+66<]5#FO1+6nYmFq3p\;p/u(I[l)H9X"<+3h>-(bNYk-n4?95TS
]"K)p_4?*8XA,1cVe)t#nF@LI_:mS$8cVSShVm2KVuRj@X-gbMnV6o7CtespK#=eg
q[Kp=B\NgibfWL\Wos5^$!O[.>.:Q49<q,6X="1QDc*UR0_NU32IeI5RFhXOR'5%=
5GCXW@X)@]8tAgg656X,"b$T]eDNn:@4t#""DN6YeE\ikS=*F"j5Fn:itJY5`s8f*
l+r@"=$Nsf/eo<u#G7,KjN5\?Scq_1@2$1hgOq+6\\\N]!fOWT=h9=E]#$nJ!(4@b
RCeU42S6`:43#Nlb=o>!Mu/1Iqq%+&gS51ZA[MuUgZKQ'lH6a.]qm'`nqWHG.5a3f
2"$dINnqLo^&e-E+Bt5E0h](P<%a[c\nHr;_F)3\1^0C0'V\sPj__Y2RgQ+0D4Add
gX(^Y4EecO`HfYG]Ah*u@Pt]VRQP<)gh]+nE$[UC#(1\FBLLT;IbL<EUj'AjQM0q5
C]VcX>#$iQltM]'c*P_75uhKNq`ZCOl`cZ4mL[[/AisMEe2jRr[.0S4[]jA$pKY4G
:hf<>6:_^e!qI?:d%nk3n]T<B9i%sXVYqDl>p#Cr+t(&OdZrS7CQm3SG#02;-e%%l
$$F`TaE3V.6Tn4m.kB.f\(.UGd*BVX$uOBt/^]WH6@Ep)rHHik.<Gt;fI?:<4buOT
4+^a%-_6L34\:u'9cY6N,]b0#91L_V=+_a;Nds<b+B%CEF?U)36Ytl>>B-LMoE&ao
h*=/C&n@"a/&'8'amq9gRQ#-[Wo$rBZ+(gBQt/PMS;7">PNQ,'g:`NfVupSipn`;r
O0Gnl=\=<LhXBL^1mhF3Ef;%?i(AbAO0pBJDVKLG*'P)?rYs=X+$&Z''ou26^+C:Q
0I4nm[b`pd>;1qgj5jGFj<to,Dl)NjA`W$SDVdE**a8'kCZZ(PCMYfhGBN&sWTP7e
9V(s:abf2\J`(uGkm%mcO?_scO!nI-iSG_.^*P7l3B@'kOBs]f5-FqBcaY%+-J6ET
;peC1A:Xfkm(P]7*n'i&H0pEmk$3Z]>uegsbZ#KsEAo=n[%$CqVMFR<B)^'7K5r[f
m*nT'8@D)NSeDg&I:(NrSOq@[[%";7MIY'1D2so0UYk?mYGq*qN%]P"dr+\G;Z5U'
NC:4l?FEK?p=!=GgtuI\hdY)5^u*cRp=o!ls)aF`jnH.X/0BIHhhP!MTe%:J:nNsR
U&Yo:#/am.#_YYp'8V;1fQ8r,(PtGr+W.Fq0GBELA!%nH?o&:R#%3O+TS,ui(($f-
flU+\*f37\cp6B,E<:^qU;88;2Jk+@#@deEBPoL@M$1Zeg3#4q('rCR[46;k4Z8?r
!g0.`-6s:s`e%&qV1pN3#?pE_BuOsM>)?L9iFq.ATb[o4B>IEO9'nX/5i@ot/4r3/
W`Cej/0pYt$\uXZ0fV<g5oL'anI^V:IS28Wb33#+%XpPtQHcX4T\T#]I7DGT=hq]0
s0UU"k#BL*\iH59"lb_S-QeEmd"k%daU!8K)@Bd=<Bu"J6,VMj\p*Q(#?uii`.J[1
D,-S;g;eV_S%q-2)@$>[@,!Ru?/t=$pQ4>N;A=gV:gP#o@<tle38j+Ih`_E?RbK,S
?sO*E0XM0)Tg:Y)Jj2N$Un>+jZZ,n.E,)2=4\a[gJiO<6QKEe%H_LhYX!f1*WfFqN
&ufjQ]\U4/F?8tTc25lRUJ$+f-)V9#iX*>;X7!QoNtcpl!q5a^!<nQ1%0SsnA'Uu=
.9%]36G^l#%7?"?CEL!%UdgA'1<XAF\.JS&hF2tM>iW@c.M!B9EVs_pWU\a9'"a@.
^=LHT+>35['-ksi2Xb36pF<A1kkbE34KA>)nLV-L^i1h7(-s)h(>[:l7*Q%TYe1?%
dW=0STJ5Vo0X+H2^acUqDo6V2cIF]6LBIlDL^\o8S,#[/.Zu4i#.E'k!!Ofl5Rt0C
3'`:!cf1bF.TIDh_?3?E5_TBG`O$Du:t#g^b83jNNrt^`s#2:k'DTg.;ID*`/VpYG
\g,c+18S)<c%t#IG!7R#!qp(BB*:,HV)Q?$Xfd<22VkcYgZZVoJ6[X%.u^s(68`mM
(N&&ShI3PPHNa)^opT6DQ2Q4ic"71o@(%s*K`X5FI>9$?%4d;;=LC_2;>AEp&*(1u
VZ#Rh[BP?qq*Y7K"$'rmQY%+nFd[i,X\#"72h4\L5e!V;T.YGEPIY?l^58S_=up_V
BimP3#=6:-YRP)u3'"4qGNL!Va1A/OO/!97*:2]J,$GLn$'hO=Zg"b\O=&S&+T+^o
QE@!ZR1;(aoprM]bAaub<h\/!!i37!TPtS*GqYg,ii1$(,C]2sOWVYb5n>C2F*/7m
#kU7*.uEkS#<mn>eMfs]oY%kNe0nU(F4PKj'<%m>]re3_pIhE4BD;dZcseX:M`bJ"
nm52cH)3C]Rmr5-*hkf</Tp;@QRqjOPF-^cJVkp4AGF5ETLY#uTg#:iq[!A(+fjSX
41APs?_arBmb(&oQf>3@j1fG,"kY:o-j3p&a+1rOjhQs"!m-Z9H=.pC!,.bj?7W?,
Klr!OGTt1&1(lSVO;"([!tE@n/n:j!K7S.](C>/1"K@43[&7jJ?F'WbjTpo,=4Bg6
;)XELI>OEPCf-"&'I49Yr]Prbg<"-_;hR-T5Ie?t`2$!+&MO;Tin"kEXAWHE8h.%>
Y]8[P>UV?aMFIaTD5/Y3-rH]r-aSIl,Ks1qn\gd72N&SH4Em(:Pt=Kur!29`Ss9n6
69jI8+pl2F,>p9o!Z<'mibQVljRt"3WAPX>/=cp,IUL;9QRNDTVB\tC@)dA:)HD*&
@'R.U/h(=(V5"$V^kQ(p\FUcc,^kT7MI/p-LCQn'`ZpZi$-]A:,p]9O!A>3^RL+46
aKQ(u%kn4gJ-H"h6cG_[8`ZFU0EpBk86RK;+X@/5Fei.C:XILc5BR0'k3s:(nWIjU
>#<=3;%uh?A:p9]7jD/YH6WR'#oZc"EWHlt-rFTG+gMSPLij/ecBq,KH4N?ugq5NZ
66R,U.7L2Rd#t2.NL7/MUF>pTA-_C^XJ9K$VG/pU1ob:e_G(j'[4l<:a9fH3i1!8#
3?j^YT0`N6:l/1?+]TGV')IguC\%S+o(&`nYV/uA"ULeu`eMju,?Cb.?)$g(bL*5M
7k6#0XRq4.f!C-9W#]iNVImBNC?eH+I5+T?ElZf>G!`1p?DmD%K@Dn[@ST'VZ"1;_
f_V+8m$+uZ7,XsgZ926KMtBt_m'"auHq4iB8gY4Qd_1O@#2O]]+R1Sn;?[n+%FW?Q
#;!rJUsOer;gb(#7UDOOJjY)(^3##>$C&mSI3aUQ!=-sU-<$HBl(sl69n)\7LhV*!
qVAEZ'kdV7RNcX39tH%Ql[`#RG"VDFE4:)Mh?"1n=tSg%Q^iq>X<.,>EO<Fpdb]S&
l$[K^4hip:rKB>>6Z;`I\)^EZ?n`[R5[F]3+>3nl$lai#h/J,D8_:6UfnHZKSq!,G
%cQn!Ld8Z)0=[<i?+CBkEE'"q=B\fFCgeE*Q0G/bf(Ml9hU\g+43+=q+0TL4#OZ7I
^Q\$5jD4hmE#&Sld5*340HNtCFq::V7g`Zd<L7]>%EnD.he!uP,#:8pF_LM6a!Ub3
1O>BKa'@Ie&41BQ3WK>V`#+*V\jN):MT4fFRp/c&UJ-LQd)uRJPD>J9?nkDF=LaR9
K6\(HOjDDd>`03WSHrKdXK=G"%=s3X-0q"iRu;H+16N.[NYmi,qR9Fu>urTMCb*_a
.p.?cB-6fT\CXpS!,Ld_364+tfOVG,Cf;Xc@G]0PRl=t`<AD6D,SJgDmqXLR5%=T,
h,09;E6ukNUh%G!-QAl^DRRs)G#>p/#p3,-@u%a1G5$2bjTk7fq_,GR.G$WL?BEum
c1VamYWE\UCl1LM&Jl$CS55"fSh-2*?IUo]DLF[m\H956,#W=5P+(6'??o7ah*e4&
DSSWO\Ut+*ED41iqR*Y[@FYD?p9lEgQ;+>]k?VVB9uif>#qeIe:c]BbRaO@S.3_1_
3-/4W./[XrcW8F_:MdXn2JHP"9@b4JW53C)Ij>URKl"%-3th-tHBef<+@a4VCY-[-
5u\F[3gH/jl.!>V3%p8)R3t6MhjRVs57VgtGY=&_r'2N(??]2p#C#2?nXK;[6cj=Z
/*0mRR)71aks+imK1`&:n3/u5qK[PU4]N[YrjTK*l(dU;/OB5^ebU\a478V;\Zd=9
42\`mH83#k%D2E\^J!Z7bF^mQk<)AH/0Vp/"7/6L9"s'$54P^29CSWJ<kS%p]aOHr
qpRM\e/d$4X]tS6&r4/IqRrBrY^>+d^o'%G&."J5)Gok6fpJ7eI6@lA!/LiN>6PC:
#mcqT[F?LsfFNMsL5bA42V?k6ckEh6)&k:=)<,]LHBskM.2%19^aW2BZ5boH<@.gm
TqdaQWFD""[2`miS.%*3Z,D0[$j^YsJCkDsC1])g*4Vt<5>eo+qjkS0WBqjSJ7KnA
8I<7<>s`?j*T@Qb_iG8V.`/hLO=VuJ!C7#K0:Rnb^)9Y.`%o"$41a1:/Q*4f4?!X>
VOaMCN79nY"?]"iJj\T(_t4p.r'6DB*gk/<P!hZnZp^Kj7=]J*%O<>gHq;,,DoAm6
7)0YV_3;a_KgOi+`;%9,ZrtB.1IWgi+7"^$/2X&!9uUU!$RAfkM>K`'NCBN-%+JKK
e6K.A8js/,[hF&)C&7m^"MGZu7M=:0TEZT<M#`?l!77$_.C9F1UQRDgLlrjO=R.,6
?AN;6(cq%)dMF>Tisn(eT&QrJ'<%Kh819^6,Usg%38UE?<g%.4!9?>?)03/g'c5R"
T&Vbd)+gGgHq*II8(*,^it3<-Iu@hQ\_Maqi9Noi"Ji,Q87[J^,`!/A?:^ac8?r+%
S;f=0NkYFQ!@3dcdN:%TP(6]ra[AT8P;\5m;jE<.]]>H:baHH"R[JEW-"Fr`%%U$B
Si75Z8c3tWOq+>LFI"JR*,MHB'VN@6JdQn'a@*!64GK0oLU_:3`>#D(>cjWWY+!"`
*Ft3E['<7H$_AWM\<$j:>\(L#[mqF(bMmWcJG+t=].QLa)fsu[`4ibOLQ/SW)Ancn
UQ@.X`kRb%U/1rdBXQ#S"O&9V^V`LI;_*CNWD.*dNZ\nIGSEVT(Qb:*OHSTuUn"C*
4V^>WJWU"bMY_mF+0GH>T51m$(lh<]#9U%f#bVS=Tlp\a&NBn`JT-kT8IZ!1WD-OT
aK(2T""l#iV96')%>2k5pmauT,mn[t\taqg@5e_GR%c,gMkJrj)Qb9<js6J[/M'Q?
RSYcPlps/=:>G9_r:&#N_nMZ4/KFBgB`GXH/'hc#:P@B5K(Mj54e_3<RuI<ll<Va?
+4(`(:b[Jt7$Bcb.89+51t\JJK839eD7n7Bd's3TbGhI%QAge6*h;7G']_kd'2Dfp
O.@$*Pnp7Q(PoHbMd73\4RY[W(s`0u:DFhQ[2i/U'IXD3cj]SuSG'5Z7aI6#1OT)G
bV7ITdSb2f_Hd1nAHIZf",O>fc?-0ddn\8:L8b>0J;jn$q+aj/1<tN0d,d*KRKn\5
"sY',J9m%!:]u;`R#W#PS,/;]D+]r6Wf<`IM.m8E'%-bS(,"R?N/7uE!/s%&75N$a
%lgOh3;qE*J4=e_!:2o"UN)5+ZFc3gO\iVj%)AI%h,V7O<RkDSSR5Cu5)iiVf7d\[
c#/NsDht6%#]2q0K\-_kBo#c(]Sb;_1o?F!D@]H[0+cR`B^Jk@>urP]VOEd+fYLWl
?WaDg/?O?-WD2!5Xk0[^X3G&(bXp$3JCj1EfD>#>&.dD>3nB.<=?mPP<GTG!]sdRS
<]-9T*Inq@MN/^8Y!n<$4cWY3FVN)D=4MLGXe3f\-kA])f.`_SaPU1N<]9gIW+s0Y
B\^!uQTQd&JOgJ3BFqrLf7;Q6Y5H>-_WqeqnYOn:>4H=1eYtEI#Dd?AS[+Y#3GP2X
L!hs8<e/[5^nuXUs&#F)!;^!%d4>U@8LU^bgs?2EAAuBsW`ls%&:f@7d3)ZIb$,6I
-0;E@'seBUZoS)n1.)r5I5BWA\@D,MgT_f(bKr)J^+pG<8@X7V$ZTDt,2>>ibQ-J<
8QabjaA_;f>aX,JW?0j+-=#*fgu,0):!^r*D\%QL?2^mf+u3FEe6X'<h.<`J&<gCM
&mJAh1/567[G.NhgmZdLgVHeF2=ZoB^=`P^04!S9A`L54jP?;l;F?nn0en3,a/AUO
hO)/dW=n't"('6sh!5HA:!C%d(dkk"%2bBQidD6ap+AlIbchb@7?TJf5>@PuS[;XQ
<(Fs%D#oiNP2MU6+:u.md\hEi7EJXR6g(OLN1K1!/0Pa'O:6ZInMZ&77h[gb#s!h"
V`c&M0!IcPlAFNq@`>U4i>NZo0TBL-jPaD\X(\BhHDZtuX$shaiN,PhXrP"b</i#Q
iVQYNh!,3S+jLpgi\[)HSj).4qgcs=6B3F_OW@noQEKX*`>^-r<\5.p/q=urT=-G0
4u)"I1uUP1iD(+!"r7\4(LACL`1AqUhDo#Q3oSXP@I?:f[Q`[`2.A"":!Q)!6gA2\
DrbG;]UYSSK,!C/-/uhT34:EPH0(ie/&d5k4_YnoKd.Psp?"XcOi]!g449B;-csR^
S)WH/+GUMi(LaN_Lencs!#H1p)\B4m&2$%W:_Ujj5\@h*X`Rc&4!_id%CWT]]Q/5#
Yac'++.s_^=1F;2?jB9J`<_Rd$`/XdI@(prArig%THOO\VI<rYkK]Z7i)X[2(2]MS
D[[+p9C?e4)!#<dAjTgMk?o"eE#Ihh*9WD$kG2oCb/U%E10OU*>Aer4[XbKE$YUdL
kV^ZL5R1t&Q&1f]k^69ALu[]h)V=,0\s?u-Olhr^O#t?rU=.*Hr[[-Y:E!Q(6"D[:
H\,sFj6:tVl&KoLDKk9(H*u4LkIDCAa\HL'7USp!beVBd0T=_7Us>j6hWC\n?DjP8
g1lkdk^X')O^De!A=oeh63*mU3!Fh0j><^-)2k$cN=@l>Q)B`*]ig17f\I$,F-*9O
<93S*otr0MSUjIH!N(+-cl@W1hj2n;mL_;lh&FZYS:N1[JOE$rc-f_Hm\Ie45X**m
FLW&A@,FU54m(-CY0GMNLl\FZJ54JR*ms:1+`0%bbA-5iDUk?,%LDd[P<RXfT%T3k
g;-E&OOi49rnZhYhX1([D@YWe[c6^2[1ii+i(iBbN+Z>J.;j\O2_D."R=FY0479r`
(%^DtG4#K^mqhF^D^Ap2cI-W*<R$!d/=?BSIb,&nfl;]bn&+m<d"QE#F9.F%!Oi&H
!Gu]c+RUCiE'FI;G6KSu#&nXHn:ck5Y6h-QQ5P_lZe"M/#4ejrqC:Jq,#j`2Sr^0l
801"uJ1(JL3[HrbqP\,<.k>3c2_fh00+2h8#sSfSP(>[]P2!Xsj9]W6TGQq>SnBM[
T]E@[CeA53Tk(=5E/4h'gbY4Y+h`imDa'%A*P7\u_3.YeTSl/k&YqC:SCO0$#f'"%
_MRj1"ENX=YU;+):GHo<1K:P7NMf>JWTAY#2fjY*o9R3_+PLnD5]adWR#1G95<e]<
HY\C&(Vo*R/gfH\0+s%/oPMU25=eSgr3_![b#_5B2b]VM9u*X+A=Na\LJ\&t;BcG,
oflD0=&j;@/bO$:o-a`_32q%_?h7L#14NP>cT'V(?;6WAO]>Y0(Hn0>@f_V'G"M1r
Zd*`+A&=:>]>nU;heA)6oCfRap<Ji7Df/r9D\(H=FQp_:d(si7"I=R/O5mH$k$X'_
MKNK4_@Z\ueLm6Rodk<O+.SCaK*sbD!,rGjJleZB-_gGk-%^(`!e;a%TIPQ//-=``
!rt%X0<4lXX*T"AH6G."b+rl\PhNFlc)k"PIX\QS%bbV8^<&IknL#))a4V=.q-hnN
F>t<t-hiCa7Z4%V)%AJoS(0Xrq:sEolfn6?'`&<uH8ih>0;NnqVL!HbHC(XX^T74W
XcU#pVI-OCA^Gc<\[]8rHS^D'5b.CM6'B9sT:stcKj.qpE!Ri&?Pf)VbBT'!R^d:O
4R[>c,]hBfLO;>)Je,kM-c^O?VYYe@qObq.\#9/>*;n5^I,bid$1>7lY'gt[!C,"i
jBn=9eM/G\NMd;CYe"R0)o%ooG@+:IPipK)V_$%P['g16=:(,"^5dQ`&fsRTde/UH
%>Y"#2A^rMi6Z^.N)D)@%7[+ToL:#e*KJ//iNVB`2AqInnPS($C,(kXjNo:p&1]8_
94cPuQolE$#_YM%i,C4[#m11C?tnEiI7']ZW7.tEb*3F*KL7TlC`GB0$qom9BoL?,
9:8^m'7b3`<Y^it__k9#<$i7b9gVmfAN!C;ZWca[:h:ho#ejYaf>(YNFZZg*X;>Xd
Y0@3;g90BGQ7<:]Jd&5rYf$f0+jNZ4p1p2565P;h@8P$e66naP7ACHnjEa*9OplEc
3uqX7=di'h<#P?1GspXh\5\pY2U,*O<:'LbL@VgqRb-^>Rj8?cBZF=t(CQH7ktep8
Y;`N^U_/0Jomtb0`Zf2.`PJgf^@jrE)9Lu\i2\UBZY\o#cob#:%am248f!/Tm9<\M
U>`+-NMEHK.bZ/I4;-G\#U?/&4g#]Pi&HTDNh*5.@VY"tY%jpHWppF4l2iV[Yd28!
9CTDQ$**?g3rkFShRr,?KE2&q#R[,RM5Vi'84fn\)oYG7C6Sh&-p!Scde'sYKHVI/
(F)5g3Z4_!P!C/7c'qUj,Y8YK+pgS4TI^HPfXrjG!t`C)Mus't5R\=iZ78^N(r.Os
_IXi6;FqSNKnU[]0[Bl<jZ-)b_%as#-#t3>UcMn0a%o]8>rW?V80B?'1%3kgJk&Hk
EDA./Z;CYQ5rC>j.C'Ad#cr.oN4hWB<1,++&s\A)W=l;?/kboN__KBA4OZ0^1MkqW
c6:Eoe=nb+nNB[3o`7?TPVj%A$C#*A-rL+X,U--Bm4D!8Pgro:;un:5$Ijr=9e%Ji
:'66(20,Ts<_i=$Zi]p6E2V;\?$OUoQ2k&r8./\'A&t^iPpFIlBG2bF15]Egg/>Rc
#hl4F]5,Ur2754b<pD1n,-u6@3$ImYb<!r?bkF<IoF2$lN)VdM7+$)sl[.MJfOoZ^
.5a&>1RK3kK;hsHCK)U,('B?p30V*[a*>5(N3([a-]YuErIU?q$@5MXDJ=>NJHQW/
596dbWg+)a:!bo/"<d.<a7@$WbRUt1)GNkYJT=:!+i4/E4UXU7\1nF;8B''dQ`;>@
2T[es&j^X&-k(]aO;P\3Z<D\Z4^_A7Pq@>Ui!2L)Wg]79G#ad@]muF,$o<Fs+&6kG
pb8V/48.uFE'1/b_f6YsAVHtPg0_qgS^&h\7U47ucI3d6A'kLo-.4>dm\SIFf21f>
Mm>.ae_?M4Epg_i]`AW@!5',&nPS3XGm)3m4L^bF*dc6_%nN3R5VB-'Mq/"a@2V5+
jAhf8)11Z%n=X/Ii0C9BE1h'c]4]Kt?VhJkA@;.i-fGTnR87lhL!BaD4T6GOr+V5j
eN1`V!<MfsG)d]n]7QXW+ES0H5V:tXBIo&!ao@!$?4Og0'*nS[,(u&H'I!6O&I9X6
&h9l1&r<pLeJU4FAJbRcdaeShbOIM[N7#0_fYG<:@s4pL8#_,U\,m$5:@_X9"L+C0
JtoJk!Hgj[0Y6NNnph+nTIhOaTdD'pq.Pf>778>n+&NRZ0r1pU_e(a'U.\p*!1ATs
"M@X.9X/Gd;EQCao`CtZ#*7165litOXs>`'OU*:D0\I<gP9c6ZZ:L-M8M)G<e=;`=
E_o@G7Md@!@[,hl</$01.jVd1:"$mpWlK-`AotGHk@Ea6pB`J%m(G3<ra;jRM)Ha)
%@IQL4HLuc57[=8!7D"I83%%;k.)oBoJKXnYX6.A,i5?'J/HQX,s<V,SWhO!7S^MK
46MRoSq/A<"<$`#'^Y^_K\W(nq/\g:b,V,ML4h86KM!Xu*iFn"8ekj?;N9lO-;EP/
_U(2j;3T*TY<c*RA%"ZI$(M-u=G;>R4Jum:[55s/3Kf/4$`fsD#DbX%/qrF)"(6<_
iW)H(d2XCLG_co?$p9:A'V@_aRgI3.LsbCO90eVI-NGnU!.p1!^gT2("fr%DYUqJX
b,6[WfWiG?*t?cmb]'?u].:/n(][_'4j]'%`,It-KUl")A?MpG>-%hk`EK<uI]jR1
^r!5tCTLoMZ@X"@=t<NuXcCuA3RS^K8/63KUfP+ZJ:1ag*IY-b#/Sqr%q9?YIBh?i
AKfP&ALt%qZPM-:`X=g0XS<I9+BHn>92/F0?)]0SDUp9"F&p@>Z"'*Fba83F*F^an
[pX[AP5;&t^l?7AXodXS$^(QD>A:00mc`Ia/TkoI,J+5!-!di:p]0.,"kD>s?8V+W
mkoX"<YE;PM\I,sAa^jE7Xqr6.qPotRWqp!cWU]FBeURP!dGOfi/6,-n7.;b2TQ9\
95J#[%MT"'lJ<7*,\J-tf7oJi3]Qo[OK^/:"%3t;9u7cR1Z`]]U`EGQjO-SN2MFpm
@`D=ac_A:fM@-p84U#5n'j%V5#O/(75]k)DM*[^hb&Q.q'eB_a+=P+ZLH*;*A;die
].$phfJj9"A^(F(WYq`El3,4uT-g[$)9up5i%LY:rcuJuP<J*arLakuJg7i?6RSuL
.(!7Bd@jK/km\r8'S_r!\n3JZJet>,n0cgQP>Mn)8.9Vp+i<A??YZ5UX#GhNEI,M,
lRO61orc9bk;P9#TLl=1Y4^EA*Y*!+mB*f\ak9hqSnuhLTZD;1#hgA7L'cJ>>t3H#
3Zi5'?+^U?!%2s$E.Mn4c'o@nklj/PG4,=pX3-2%hV?P1+KW6cpYN9q)u3Kj6Ul=f
.aNca:SScfC6>Ol5q(=2Z..RE=b,%<D8tmN;K_mF(FV/eN!.kA7Ih'jE)BIuANkh[
ar*Q3CCO^j49pE7+[d`7&Rm:X#N5M#K5Z1bp,Sm0=:r8ZUR-`-#k$7Vf!Wc6?TT)/
irSbB&_,o4;mj_&.]4>k9]H\=SQ$&T/quY"0hl6kOLLVN@FDC@%`Fnt"*G!%9Sl8<
.K4l!ol@7eHJ4bP]mWq)']%F=05'Z8YI=0(j4sO8GOI]`^4tME-N"C+G2<kpg9k8k
:A-%)Bn+.!miRt%B9S[AJQ6uG8`l/%S71Idc]BeJJpJfADB>VBHFJt$H>,M+keQI:
BHU)e"#"WbYI5q,Gk\CjY)^:CNl4gja9iF$$BEI@cID6Ah!P[5mZ-Z&%eT4Mr(g)g
>X3'#c`ZGLZ@6`#nLKtZcPT$1`4,(5r.JJ%n'2'u_Xd$(o-HNjDQNgJDZ3(\!U5mQ
+s]k_Ad0aK"Cu]K!nIDTXtp/L6"1<[`pUi[?isdj5NDm=5X$I/71,\OB.?#En;L',
*;Uf>%=mjWE8M,_q!UKSmbmsOJDBP-^em@iP@0j6Us_'>Q8EG8lU%BrkEoi@F>D3V
2aagn%9g=h39E^b,m,"VJtBAE;A&DT#geYXYa,I>RT?Ya!cXkb0W%,i`s`(XTT!Rm
K.dVL$Oe`0%'4,s76(f+2[s`\%M7Y1E9e#'o+,g;&)oY^,QA<l_I(\!"#1@!!j*&N
!\3^[_<lX`/PZE8i9-4REtL+b%=Jn%8H;J*1Qag,:mhX/AJE+B5S0n'E3C"\[2%]A
(*cBdE2sbY[2.d_(Ef7b@-%jFHO`=>%Y5E+^uZ(,f+1-G%tL2]bq0J.9b9]+&<W:`
d@CkCV\-.G&a`L8mG+b)[Q`(kkcD)H+WbuCgk?A?k/QWo_?=l!*eg7Pgo!7<.c)=Y
C/W>V:4b;H7Yh?3*"$6K$fK5;^sI4EP:7Wum9n.\EgR9.^idWe?c>#2_T^1)^bBA*
/4V2$/1q%k&1QZUrQdU$@U+S=cRXgt!%-4J;I!TXi[+.lEq3>D#HoGK7O8[V7T*kG
V(j=_Zir4,+`_g4Edga2JdN-F$PJ@Gns(Y%Tdde+.MAP"&u\_AXPbk<-"<>o7@Yg'
N@Vt2//#lcK1dc"K(-(mAHl?q0u#<<*=0Va/j`hrLFk.,m,6=b-3r+BdeqSBD'ou$
,a*?+Z?eAnI4,_^.$BQ='-SgqRlW=".V0nUUH'go%l9qq1\4m/-7XGM8K3Rh/9=Yo
#\P^J>:hWs1b&EDZ[F`C4Z9$<&`s0$a)^e\h^,E8.E$D^NSo6)5R"1O"l`&V7*(Lc
3+()0dU9(tbms,Kb:+Rs6@ed6mckAb'(4]c&-2bA_"\Fjm'/h$:S=eQ@"KQ;<)\iM
7BUCg:XXtOKOQYb$YPeN6EZ&3XtJ4I^pIu*lZ/JZ'"VIN3q.=9U?`_t3ei/9cDW3)
PO.3`nMO#!5@?*(;uE\\!`Kd;"k3k`1_'YQ&d1$,,>0%CZlW"B,=6K&6K&MD1cIe/
5=@=u7'o`Y1fkXFqWBGu8B1#g$3Z+Rk!/C3["`]'FEk2-HmR9mf^sh?FGVe"4VFq(
bS69joU*eb`C]/o54iDN<3!FWoIUaUXGRN]F9t4^&6"h7#;jZQFO1C0e9,j]%Wj65
F>6-K(IOEM6ki#uoLKA>9F93F#..>cPZ^dLQqUL+7PG2HFTY+\)+P//7o^-k[A?C[
.oE=k;=oc&</s)*P*Zh^;[nC7_&+Jsc<BK9.j-7lY)^DtG^;or^7ZHLA6-Kr-Fr<p
"Th4!Ji!`YmKeIg#D6F<!0!f>=L#j+Z%W0m!5K"U<XhgZ%T.N_@.+pTedR6.$ABUd
!^PaqCK500"(rTnU'(P:A-&n18]n2#cY$Sja?&p![-8)#@[=&#8-6c5?no2h1>[$B
Dd>cG?%QWnc3lLpidnN"4c:mup$fo]CL<A*?kroRQ42cT$XkJ=@:^0^V:nah+q6FW
%<a6<[P8p8h.'j+A"]6"i[\Ot7KntL2qC_+G#E39<k1Qh!L?slnJ227@p];R2=+%L
aN%otiFc]9B<k"`eZO7BKcB^96l(bfkX`4%>dfp`C#i?1,11.5@pe/8?n-/2i\t9=
[Z^?q$C8G8p;Lj6bmkN:+Z@qh[b_74j$?^;AB#Es(0+q#>Ar*oE)pL#2JI*HXS%nn
?5FAMf,H7d6#m2`2XO]e2I@N2>h-"f+FlLHJ5C^X66X:rI"]ol7IG<A)"#,iqCeUQ
_"J<.3ptr?9u.YZ5pR":iXV(&%##B%`9mo,g]pp'CU4B0:h!@fphWeSL[$oH"Y@u[
<,<m(9J,1NP`X&Z[ko]$HB%6:pAYj;EqF$pH[mbr^e&nY5C>_3J="B*jWT$tqgE\B
n$h2'0:EJskReWuIi%d-Qi2FO"b;erJFJPL7NI&9=+S3lJdUao:_!SP.YW+$b7q,B
2^<t'2%b&=KQsBkGYa#AR='6_,Ih%dQspHUB82djITUZ?\*nehnUFs.J"Wcji0Ag8
K7J0hLlPJkc6@+mP($N!"*g7<fUi':U=BK#MO68YaAroD['ke+H.Mo8A6;&].&0FB
)^rW+G*jgi%U[FnH#`*P.d.'\3^TmaY:2)1lPOcq*@S_IFjqY%cI[JPf^GKl6@eSo
)1E,,kR[1>%]^9PO@ITiH>Ag68?HliV[7%%8qcY(>3E=H_[;hW]m7Ht9Hjud;cMqJ
X*R8O4kCpA=XTB5L`i*</](SQ8YkP:i%`nK0G"41GskRK8IM`2Pik>t68b$^c]uHm
Q3U9Q;N7!QDaHI*Q[*qEoKeif$^b>rR%W?(i33O@PF69Z+k`=B"MFV"]V&0iS1j(q
=fs+\kV;nBO[9YLo?g`p^*XH1!VsobREi7/d]48<1)\o3C`/g2m?ALV+PB6m=\GBT
;4lcfTIb1[q-Hk-@SdqTTfNkr\ekmeGRf"IU&$".H7P`d1'lQuN-E>g>!2@ZAHdBK
RRg;OW]Y:t:d+W[-G!?LZ9t,s%&;1+VT18Hm'&ZN'8-r8H$9Cl!aKWn-[IOR$O.M[
!+2^5IcATZ$?dG<d,+2A$534o'Djg)4$U'F5I5],ZXGO$!B7?Y4;39*&p2n>CD70`
2@,VQ#!tiaY#/`1k6k6sTJ!1FC_r4L88LcpDUsnsVKVN#aJ67)hF11(<=(S*r`Efn
kh&,([UZQ0Lk\d:<p%B+q]iCSNO#A]ZJbJ`4%HY>4qp(G[$sRmgJAR\<OJ<%[Mred
Rr,VB-b"5d\$T[2H\%BZMQ!Bm\;'BCRS$6uS=7'V7G6/#eJ19;Uh"-j]!=3)p7Sd^
[rL06@GAL#A1Ori-bNj+]XuLrRm"+t42&7![/3e0HWh"#?4Hd@$/9*8!,K$9A%(dF
2kr"FRs@faJ"AI<^h+P$ZdY?^Ohk+a>\X=D#8edlSi8qVGrVmK\5P(8`P<iBKT]"Y
n6k>%GK6u"M#9E$@Nl(P$4-!A;3'WH!@c;5e\+T]&ao'!H68jq3Y5EI&j%u`cKGfl
oFC1$%8PJh@)5rFM!N4JRIRo1U0Ge3!8O5.-&J+^nm)OUE;V+p/7g@8V-+FEDf?g?
!mt!h!&?@]IAW?g.tJAVZs!Pp+pFLC\0A-"US5m?gWXfJbh<*B*7`;f#L2&^&tJ'i
r9;M^n.1aE&01G"*;U<GrXcaE&)@F!r<`tH&()Rhc^c#[]chb$,h(QtLYXLkQ?Y3V
2$Q3'-%.r+)Y%@4A^n!B'qJ/Hh,JBB==JZ'K,/)q?"MTW[ROP?2dLLK>BAT(DQ*do
Z5c*\^jXHMNQkjqY@,3!I,il8ORE(4fq"Z9h4`P.WS615gJmM_h7KK;&KW&Ji#O2n
W;$G-0AQUqh*=aEr-R8==4B!6hH`k4]i/ptM;LXa&Mi'$#]BVlXEQ(Q\pVCh>4`rs
`s(N:,o$RqNJPpaa9?3G:>hjhd+Ah-g^sQQm"%mthTtQI8*sX6'40G\_)&I7/'\/4
mXXr75gW>MKF(g=,]A4*,=ceV\2U9mL?N[$`\$IQX(UT8UUM;s?1XUdBbfP_1Oq/.
V)Y6JC*fij)68G.JJICdFm0kC[GI<*[8f:'%I,-=l>g6$UFs>GY\0Q8l[Y8da&21E
`U&.Am2p]BIbF,Fg[5(smQi;iJICn]hsVQsPCE8-@N?-_>biGBo>6j`H)QK'cA'(I
Yl>Luh]#/%+KH6M!l$,d5:e.r1!.0e+J1Y+$\gUT6"V1!2,F^%Fg^JK:]rtT+Q'^g
J2SMNJ?04b((5i6624D-66m0N`hQE,.$RR]7F"bp6u>41;b,m]"WWOnRZg=l.>5Q<
.$R1E:oC(6][1%?'oBlg;&G6TLl=dP&If5,7AE_tFI5$m-kQ`<!VI@e6C\aBL1qh;
E-sDY$rZ#73u'Bd'7rM$&3<?u04G:)_K@>a:9R6?"[c6C`Af)1Jm.-M8mNKu*Nk*1
eGt"o,)W5K6SQ)X:FI!0KW2e4:j/!F'8aXaX"Eo<O07`Q!Lk[DmN'X>`4-Y'MM<U:
OColg?LD3T:[cfG*Yb.k`CBCn#ej2*/shkM'?W`fME7*aTFU.+Bo']6Mj5Y8@LnN,
P(VKPRf.XJ+;Cg*Eh=G?cR3;2KkaYE3-'`uc\+hc2Ue=t3%D07O<`u34c8Nbf7[lU
4M*0&W>a8Kcr2J&ZN,n?&$pf@4O>oX'1g?Im6"4p[;_K_f0)idAD./<Y\Mr"c-pp)
2rsjhiM=aJ,igs<>FO`d/t8m,].VjLn%::jK(>U->L9(W9`,_9^!'^>"\\<Rm/ir!
ap+]WJIDAh^]=98%"dtB$jj`MWXUX)o$eZ*_>t&j%Ben?/JUV`UbrWLd0)kaXc4;o
e27Yf=[/R!HXPM0Odp2+a!4f8*_4K`LuV$:CQq8uNcJ>L3e[[;7_9/Z\F0fd!1`RA
N;PC\6r-di/hr6jmpRgV*6.n+0@2@/9iGTY3)6\/%g:2Lb)HYC0l6sngL*I^'*9R-
35,GeEp=*d9'A+-K$6jJW3;/5-jlpF+qB9Yi<"rM+io1K*iFUICb^o/+Rt'qGXIom
PF,fTLLK7m,"=R\+T+G88D+E=&4?O!4hDq(W[`jW+G_$B+c'YHj_n=W[BOBd+Ol#d
mBH[7i.)RHJH.A4"D9u-*MHcSHMO9b<Z<*UKA!WgVCC+@c#YIm5)jccg*P\lTa4Zh
_@i0e$Z:M2rPK:`.sN\J>k^tEG2:m!1O3;iUFCQUasHb:U,Vk,J;b<d$\RCjDAZ,W
r'<2rOnb=\MW4EV2icqY^-e%D\NWrWL3[VPWWMH4ACTbJlBA,Y3So+TJU.f]\8*!B
+/I]GB1n`Yi/Z3aWHu"2fIgBcQb0JQ%`*$ed5K4sG?[t/F9=Hu2g-YHb+3doS"Mt?
phDGSIdaoK!]8iQ`XkGp>W3=P@T]KZN"HoS$]\`M#"=\cfg\u-90%$X4>R[Nbh8ac
B+4$r1Zj57J906B0#cL*2V.7oo1ga;j`8#cqutpB]dce]HSsE2,ou961/22N1UXdq
5Y);5+>OZu_W52C!b?l$7+==cM@"iA/-Y*'c+1&r%`-df$NXWgL1l\EPqrbHc]F+(
nDsBSk_hEp9U:NU9I7eoOZ;>34pSmg)ae:F-QrVKK!PM]$PX'nKcKfXo13>JOc2"[
8:c=Yb!?B!$AD@N5=a;F#>5UDD6:%D&>2F_cg6N;Ad!ge'M;<!aTI:uE.b)uU*="`
@P)Pb#/YQ($fPorL*cCR6WbD`ODHm)E9\K3k^Es"$q#iU*[ItGQ?-MN#)WOq.2)uc
,bhN-MZRWF#tVQN@e=&e;33.p?u$YdFD<E\`\s&phNq`0mZ)uj3rrIQ>G7]#O-0E_
8/:#)j=AOYE[!t"V"d;Lfa<lB9YO(Uk4'_$(R"h_9fr,@Pp%gkK`E;p6KhK0,rFY5
d,%e))-mb=XKe'g$6hlOO;Xcib)(m'-VN-A+_D/#R'RiEbdbP-j"+i&.hZU(H*1"V
bVF&*c*tsn_HEcVjda`pF>R.MoH&!XSY1F"JopfN$7(Y'Klok9)=]"`\X/L&%]_CY
(BTJVUFp's#LI`_!^LMK=pLW-PX]!Gdlaaf@'lSZF2ea,n3.+Gn0=&\PSG^q?E]#e
/m$#((BZ7AYLI1#fR"3=__VE(edO5EE2#c&.H:WZlkKSk0OtPp]<*K+&#jM=#Y7c1
WcaU7[1kW9%4u0[1d4igqQL$rp^Bg7/OMAs`41^V*@]D0Sj9>W"i.s07)gWCeR/V_
.a`<*[<)f,q@WnGARVZSc"Ykbd0=AaBU.,X(KUTh>cX]EY8-7N=:5"Q#ec"tYp.-C
nB5:Y9oTRi4>'bJQ"7`@Pm*I[bg]9ECL$C&+a/Ib!W,GQ&5B(32W+nE,cYKoFQ9ef
cJ$uV;hJVFCMMcsh_ZlJ"0N*NDH@UReTQ(U^jTJ,FaC8YR`/DCYSXn^p!;I*fF'>)
i4N(>,?Jn7H*:4tYIC[O&UOt7/4K-DQeM@EX8.6r9q&jVA^B:707iUb)G\p@#N4ql
CFFEN[J3ce><jC:D6]GO'Aj9]lob]Xqa/5F&oGt\?TopC&HQ_?"2^]@cTk,jVQCE8
R02Y=%"Sdimar#2TJ0K+a[J[lk.--\8eD,:Ru!bI^K>YI'lQ"(-QtQHl-R,,X>jZ9
_.pXsTTg$=Qp41ck?AN0CM!T=CXE>`ldf+gJ3_tP?Nh?rTr!g?0ic"<`Vp:^&r'hP
nHT+i#RD2J/prV/kuT89Ul_kt;8CZtJtabXc7P2h1[#%hi$Ud?D$L.7.dk[ND#!4g
];$W\Ib:)W$0a4%V0'G>dpY%-l2(^aFW2OS\t1,2SQ$JL?sqO*J;S+bIB=#$[KekR
?#.^OMMNI"fJj+F2hHgim<O*4H.-AkXe*u7M-VXi?YY,YYI5BFg6HFBKur/d#PT"p
.GL;2kG[@NpMTHV0)@SA@`>NHQM<3\.n9!P+f'uS!XIFfP42cgOb5:oY?I$XnDLRi
2-1IN]#0JHTS(9EopFeL36CLc8[+(J-eR":AFdcH3B;1;!k*;d!Ze,^H+uA#-duq/
ICbnks$>jc8_aTE.HY\np;;0):Oq@A!ru^:Kg7I#7k[6n^ebA\Sr;'K%]+#m\$Pd9
CYKOg8+&YC*Aa;Ahg=9F#sfse"[K"("/'`H24@AIs#.Ln&"j_fOAbq+?gE,*U_A4/
fEqcB.L!&b(I!pb$X]7kKg;4C_FR$"@.YB??sdM00?#g,S,3mqJ*jqCpB"^o$9ahs
5PPXP(k](9%05;r$b-JI;MBY%f=__"5O*0;X98O_cE7]e5WB68Y_/UKSM5>0(7:r6
(^r[.KtZus5KjR%6f%gA#(U@m]pm:M;f"b""U\E?Q3mu3':aT):]Nk,[qg5=F4cd7
#_:RCMBcgDK:7uh'!/kb)-@n0MRgU&+#UtdM;TU31["ml^I%7<[4%St0I=G`.'(hb
[4,;j(`aJtB`RAlTFq85=_*ipDnoQh,J+g9.Fbh95.@K@$PKNM5esJe/hJM66oj$D
@^QbG&cdLu!.-U4C`9b#)o1\k6/-/_'H\_HDScbm_C9-.fY@c7,oN4"MB"!p9IPI^
.Ba.1/"A.@S1R(fkX,116O94"*&<,!1P2DZ[4,=tBGn^835^j-_kAk)WO%C#4<^/4
PG(&Y63G(=5RT,/O]4Z?bXG"e"gE'=`+\tbHq;2FUD&^q]qdn/HS3)":7tP5J62so
(^%,@X;XA>5pQ?1?kGomU(I4Y8.48T'Dhf$(4g-8R91BBGT40RLGc:[aG;.`Ro"]q
M_un.aN,Mqg:RJP,D%m%8?aNncmZV]@1O1r[BLML=;?BH^qL?m]uUf+kRg?!h>m2<
%"nu#b;C>mdNfe5a$\(7W!`TY#YI2+4eTkZU'3h.;Lor%8rOJ#60LUEh>lTj$LeH(
[%7pfSNoTA^"_BSN(V4Q#lq%-P2ls8W"&rnC."G`[[RF3g(p+)fdZ3f]GkJsF:L)>
LRZX)+kRSQaG>Cn*QUiT_Q/:*lV=W>9XN!'6IR%YEq;u+?kS,p!Uq)-UKe-3(EqEH
+iA8l!m_eVBc`)=[_Y!l_jm&-A4-\0Zri#6!4AJ]XH^75]LuTHgKc7Aae3)H!0G>'
k_B1"bQQ/!R@(CRH^^l!Gg![>9?Ro-Hbu=0OKkPe-"Oeb'Z'mP_]e#s9N+[0@Ns$<
a+>SXY95,bUru+nbV'[TV2W]W%+%][L.reEbq_W18@$KF9t]s$c$Vc3^tDG]RgRO\
3LmVu<:%lpBoJkG)AM-=SDjPpirM\EMNepj1Xh[0rebs!)AN^sK%RbB'*(UA]j[Qs
'XNTGfu`4S8\bj0AJtR/hDu2Zb6S_3_U*i?]a^02!L4f/`?IXiSj$g0aOhX:m3Y^r
+OX(/!WX<??lcsH)hFY#!IOXV-ka[^+2URB_)pC:XVjY;ha&C7]s,,4Yml5Is1Of0
,Cn3*oU>jHg,U,+]sO5"O:sf+&]qg"8*mKX^^j&YatY"I^oXcUX4[KYVpP)q8)'2W
fL[OW'e7)%;+)NEm7mXB'\()q<76CDqG"W\#d!A#P5.*<_U4PLa-GX-<JVZYMd!XM
+T\7/JQ$uf1]k"g@(&>tQ:kXITm8?8cN'r4N'Z_UePjc8/Ki]D$7*tl5SZBFAKW.)
(.i&:HSqiQ3?W'd<3QMU"4BU9:,DQ=f-PIBJj36`^/[Me<D]r#@g#eQSrJ/$+r+9@
h-0p9>QJtQ.Re/.-"U*TD%NKf``6OX3=8eA%TlkYRsGqeh.N;R^/gK9R9aQb.XdLI
$'lTa\_V-k6"m1%9W'`W]mZ.QM?PKXR_:Zc4VO>^ket.oYd["58Yb0?PS+CP"9?pP
amj#"7A("$)Sn+]8UqW2=<:X_Vc#r/>'6_DbP-RY+TZtCJP4r8j2kI.6p:IE]pQN*
j:Y(XeCj0A;n2uKK?SkQ!QsDlPG=\b,SDKCrk-G^S&g?c"WAG,%nH"RQU,'#g3utO
@nGcO^rQsaEpE_(7jg#G6ukWC>A>&jfW#YO%7p8O,@+"\&AhiRcr-UB8GJB6_@-fX
3942t?.N:`*[2.7)*f!q#SNg3gE!<qLc]32,hWOb!$/VXTV8iQT_VPRh6?/J71ist
>m+I)R`?#nQb.`B`Ccp(aH*,!&SX<e^!!"+^-rd^/B,q@"`(b;U/bn&>qi&06Hi_8
f&(o-?%ps;V:u[VgaqjK\tV^Nq57O-9NGHY%uoU*Hb_rnleYn$JL0JcK!epHZ&2(D
$BhJeg,Zi02^uj/O@?P29?mO6T"lnML`Ch+S=)U/^r_kJ4pVdP'e`!4Rhs%/]u_.C
$jt+Lf=uPL38bb7gURTKLWFER-%HkaKS+hE]unTm_Ib(9cjX&X$U<sW4epmAA[rJY
$0$$XS]hY'H`98r!m0Q05TS0A"WDpXS7-t5hL!sd"gpul\eG<;Q:hhjjJ[Uq$GG@h
#U5ibmKp@j?p!m<gkiOs+P4j@cjb>1!><TW5gP!R*TAd+:qfD$'[eI5LGctS)*f%/
gs@pq+3Z?)0C$a^'j_p!*A.\FTOjVJ]+X$*32Y%,TM(e)$Xec;!j1PaMXEglGhJZ7
O,TO^cD3]QW;GA._j4\a"J.b2!^G`4A[C3F$U$CY&aNP,$K^,3A4$@X:__u^7fd3m
$k>iS?kA`XGl]6c$2KfriZ7+Mc/f-s0D89a]H#i)%ZscOSd&UaM`V>Ii[1VDAVnu6
qEeKe>7,HVAuH.#`^jO*ULjCAQPNSo(!,KB"s'jW!;K.!TY<[BU/%f>^m5AWHjiU9
%HG+%^d*K;+G*kjJ%"rWe-(7nN?;S=T](ETa;)@F*1BRoV;7N3jO7C.n/"VT(KsoU
JOW*n[$VNo6G8KV>;QXoW!GYPg1mu4;!>AmIP;+Djf3sV=s^?P`ie>(TE+jp5Hke8
_#Rq2iQA"[_!MZJOSe'e3$c-:7U"ae9GRn5X8pU<O1O8*+W$a"\\q5T3KTuS=;6qF
qi_0c*O4ePI^n^uSr,U8AI'&FnCP)!De7m$-dcuREI5.paB!r1*TPGs"l`KKRTV4P
>E^NVqmqc3^sAsS!7IkIH>g'UasO9qAS),^&4c(!'?)$0fd++Y`l/93`b]`A')ot9
p;t<Db1&`tCsGlDk!nE<7dUD8=Q\#(qk3=>Mb^/"D@Y5tmBc24#Aoa`_DoVRY_R)2
U@$IAD<)9>Wc[Fb^?uj6KR=-C,d**<s(]WTE'=`ES],;+)cU&F@/[t0nG0mpT?<\+
'K)7\Q7Pt0hI.qol;/0%4Kuq[iQa2!a^>j7:3%4oY7lB']A)1],L"oP$:._pVZUbq
I;[h0[p&[`<,A.8PqgthgMh8:b2EHOL,\*gJI=(Bn>?7"K?T!Y.jgpg-q+joL>Lhc
7WOnMhsoJSQimC=WrP8o,O;@A`8;t_2"(;2!LTM\E6rO7$^6m.[L"X%I`$2sO#sDA
*U5hZl]IA0f3H/G[i&Yo+#"+mEq6f.Elo,;g2BIW$Yp8B]QR2GY;1/Q!V8^)F&7GV
R*X"^2N^qnF+hJQT/sa-46<;<O-`%PDa3%'5b7p@Sc;%3Pr.i/7:6F4oP8K_XAMRL
c9V7?!.35@RAeL8Vi$tmM_!L[6(,e"%lt-J<&$@/rX3Sq#P&heb6bi%mP;K7]Y2B!
lVTgfN>]O@+HT/(>ZL5UoqT;m5&uGcDsfPUoeX#M$e@k"^%O/G,L#J[hf*dcb/&25
iAY8>&/*aAigB]=XZFN54,?]D8[&W:Qq%[^\t4sN`8i#0)AmM;X;`%^a15`'*T,"h
'9^0hl+PgY,(7euFeAOcN$1DjVSho(@;0`@?eMt',#SE;o="nO4E.H]i=("XV`'[c
-eWkC(^g*P*%_=JF*J@\LqnQG#^H$dq#I,\<)0A@DYYipTJr)U=9Xm?Lc,s6q1/M@
P@EtnQ[--gH>oYThfs(q"t\Z)$n%_nf:r+('A'GsqI-u4cb1W;W&[WDHDdeb-`f`l
7Jb\1qXmHd/-L!;$U@Bu;%q>IRY*b-f)6]oB^p9_PM\]+J^bILJG]l"PbAGjr:iZ)
Lg<GAN!f(J4$dDUJGboL"Kbll\&upp^pfBq/@KOF3kaUNn1C@m+,]j(&)'8Z_'GES
?F>/t0\bufndM5>HjNE4%7h!8;7DG]r>U""RkRUsOBg3I#(R&$KLGue<9D$-J.9]T
.=h2D#[frkQqStG$\X)Hi-7X6$j;/J5d4?Q.MW:V6Vnp3DEK2+87R5H,Tn`V$AN+i
@+:9"*gfW56.p@)4TZ-f,h'<bEd^08#K.:4PnZM,&O;"YEB&t=,(U)9<5CQ"XZrmf
6^,VG=tUGC"6"4OFJ<1n%+&dU]4@9Z"\)Q<QJ17j*Y/NDU&^97(^pY*hf$m"NOgbs
ZU_$[(uu;=#_bW!;&Gg(0,Y)9i)9pk5XT:>8hC[tXVX\g&'Mk3E=CtmFG*\.&kX4S
9eiE".3][92P2+P</!2%Yd7o]&D$5ki2qMS@`_bln`rYs@Bd4od=G'R(GZm<8iti*
^R"9s#'t\?\;27;#6fFJJ?YBl^%D\(58K(5GPhk7!2(J9Y39%+qLS*+*<CaFWsK$D
XV+V&6B;I,!!<c$3Y"N-kWf[]MaP8h^VJRN$+p8r4:_PX&3gn^d,\aUV2ka6)o)H\
F::83b'=BscJUC;6@dj(%RQ;B5:(s`'V*'$YGtD,,gjfHq]asfnHUb/`,lAW'+B-T
-nOjP,UG^^]XTYV/CoEcX4edYcBG?n#!q[=.e:ib]*OTKZYC9L!?bP]#U$9h."hYX
E$2cD+>"kR!5M#T2^#(U]U1\H:b\.:Bco7@"-,`[-r6&Mb5A"JGUSK%1d'X`+Qu5m
Sj_gB%/J>4Ql,uYlcYo'91X2-PVW<0ThQZ4W^s,oG)M4k."L+HL<YV`modpl[CpKS
'?X0O]Se!AKMX0.#)LXQ>nVoi@(dHadGTEt8[$XJ&PQ=u75g3*W'rlYe0+]Z[FDT>
YuFNL;X[Xh-nSa4ei._`a4A=P\QjbEg*p@&Q28M5?!+G(A$YOqQ[`/;;M/Xd9!tVP
>1<'$3T!W%nHZj;F;4>[+BA(-d_KB1r%#&%MOR%NlB*Gei1qAX8k;@&7E;M;$4$[D
lfQ&=+P\[X"#;uO+(.t*@2i8e2VfW@%cui.]es$\JqDAa.gg,,*qg%6d,MU@U@?`W
]feF?)@0!&VL#M`ckn&LC-[pk$c!_2.h,'Y+$?PKF$MN=!dL+O!VII-,Qb31p@8XO
J;rR#5rohrI0#bE>-t)^$\T=@(5QV]"jRb+[U>4Q&=07S1:Y1LW=)2]XdC.;KDLJb
:r5KHS.1a/D5J&%3m0kr\Y0Bua*;AbS&o&8f%h5;I5uM@(=^IXZ:FRN<@$m7_('U\
be&DGD!i=j'3W,!h\@Mpn=ClE3fbHkJTmJX?GRt7"Nfm@\$FrB!ht>9Bikr0\jTm$
R=$:enZ$6E8tS*F,gWE@Qpp"X?[6.1+?b1W2<"et=c@hW^&<IPN9X?1?UFg5&%3cJ
O&-/c=A.-LYp*#38V.j/.6-.8'UDo&_4`rIJH.Q<F9U\S?[\neqQ[sqQs4oT"*$XT
JZ-I)#ul+ecV?;>#7cC>aV8_i\<TIt5`=$!*s8Y3%&P:jNfN^OMFZpNT6';1:19MS
%[CS*;D=j#d6U?;_$s"8r8/a@YS$.te=^8Z(<U&\MpI1jJ^c%N9;<:tjIkhB1/d>q
ZE8Q$a:#UH/4Ijpr.VEsk8(Oig)a\&")uO&/g;q8PG5*%mdSaFLLDlt,Z?hSNcH4"
49F'%[=i;QU;S6:FVs,KGid@RQg%[?j`r*S;T+,[_eUiSbCFk-_HeM!G\e\sBp^5T
nh8[U6-H(HHuh%OPI[:mk*4?t.HCbtM6NN4d4$oYH'HN28A-As.5(4[6'4af3nW6T
,_U-CcP0/;b@lr<L%tJ_F9'-RfGooh!=h#@^?lg-$j!C0L7m&)F.JHKBe<SKeG2*B
&r`?SZ)o\0g:^J7$<9K-aT!J5m2a=%f`IFa.R.(M"^6c<0TIT&!@jn$ad$LRmQ)dp
WQ,^6;><8P;%+aR;]6TbBgbL3r'f[2"qLcBMGd-k`\_fceYANp!^smQAbeBF@E^aN
liT;!#c/sR9i&"a'bYa`YeYB%3MkL=&ljlljrnLd(@G]gac(LA15KEN,h>ctmg^lE
[tk^=O"]u\XV/jiI45e5[N`Hrlga+aKInSb3(4B$X3=u<%Y5P9H3q\"6$m-&4'K3T
]g/A:"6*)$Vcu?$/J40I2O"6rErB`S262*?\_,XEA-B$2[R%@]*Z!LUDUrC65cYK#
gd20aT5*Ii2^sb#$_;ALbm(b!cK]t=Y=^Flg4\'sd#i[g1MFE:]D%DV'V_RQ8L<[(
2mmL1(jC@0+X@\;aSD_ie<`]Wl9G>aU8Yup"'QfQ?)02_TK<4'@Zaou2-.=L64/HY
[9bX)K"!!4^Pd(?Q?'oM1-Cdl9@<$t6^8*)[Ub\Y$Um5]%E^OYKMs<+U+Sj3K*!t]
$J_(<Acft0'U%b)@l+f>8_,lThJc,aoYMLn'QERs-KV/Z`HW"`RM3;U00%SL!s?&<
Q'$4UTh&8uH/pu65-Q71TcS*<"gk#Q#XL^nVSFN$KW8ib:'qIC*%I=:hC&G</I:J$
.=dYE!Y'b82=p#5i-_C'.;0!UE%!3OTVQ(7N:Ae[-Rc7k?dKoP8q`5#+`-1;So%@t
[9U,iWU4kE*G,FsX>M0TiXb@T#$j+S^*e0S&o8jS\k6SU.U+<uCs4$52LI&'gIN"F
5Y8AnDV1g*CMj3%]uIM^S_QK:EZ;.*Z$/[Wh/IVHnBKeo7#m'eVl980A/UP/%f='V
S]`sI.!HW<Fuu,W[UlloR.G]FZ)GJUB4O1r)`1qpZ%iS;F=r\4BgR`I7F*^,VcSdH
<(1@(&6'Y6=MX!oM`O!4U5I9#$48Q;"U#EhNQJ!=<gT+;N"[d6if]E#93T8@`GWu0
M9l6`\P&%Tc7BmHM_=n/[YY:EdWacq^3RQiT;&pj$>iDN-9/(TiHheZ:)EUCB:d4k
YM@o6$8)G6^hnUQIlOkh*]<WOGbE*t5ZC@J&Lp&?IN-PD/J,=,brI.Q<7B"lp`um3
$_,;V\9m@8p2"Kr11TH30D>>\UL`j!+RuX6l]+K;.fU$3q\i4<(U'.ub&dDflWX%$
HM?X'p`ii6%u;KlN%'C2q(7X&DjiVf:,];MNGLlNO$\<255QemDG28$aWbc*m)d09
5U<q?m1PJ[d0#;SbePd6NfN@=i3Q%37V`q.%h=]>RRtO\F2VHSaoZNY56K.m<fXTj
"CuJ%.g:h<XiTM#be/&$`/bIY6_jR96uXEiQ9p6]7R00C9a9bDnje@pN3C71MN60)
P!]OPjA-i%+WdK_R.G9k1+2"rBsq(q7Nb'_V?R\ED@6OWNb3oH&'.4#M:A&MaRROi
R450:Abr.<<1om:,KriK5Tmq&7h(Rr/r-O?nD9^Tis_sB%Z#6;aaQYIni8<;&#s#g
E<8#F#2rDf,gd26nPKs4Z@'M/pIa6S;(/6F/n3$Sf5Ya]Yr\;H*_XFnVT!RG.sTF\
mZWP[Xfm-<aZ]cfeniAnD8T2K,WnYNC70b#6\Lco,`Y5(_"@[eVrUmkA5\Z-3=TR[
7RlJ*i%1,7(=7hu6]C`@E6*h<N\pf'C!Jn0m`$X<\:3V02hIPFOlDD@"E3G/)R*QT
?nOoFMJSC(XFN>6b9"_m$u@/+-7Oi[".F[n#-A$$<auC`0DL7'ba(Ld3'sDDY$V3>
LB0_j,f2O86nClD#'l@91S[,k/i']+d+8?'3l8C8+>E^!mU7]A.=bTH5[u;,KEe`h
33p(FZFqd.Ah+1U#KZ?F_[)<_["a)XVP#^%,-X#"0dJ!A,]ZGC,ns`[%]q7U9laD_
P$]O<HR;X("YsoidW>U:Kb,iD-_aQpY.lA7Anf\NRR0+o&s-&uL][.5,c+$S;P'Ya
%k:;u.]&mii+"8m[k%&M2,_:=o#@p)bTYE]L/E7>ZIphHIkCiH"]G"%cFf-i[Snq.
X/m@,%'nmq<^gtf7gtc%b0Jqfc3$Vo5RP_)`,I"9V[1]FN:-$7k<(\D&k9f_Ne[JJ
k2`b/rh-KYcY"N/Z2@+EqueT("Xf*0ZgBs9W,oaE+Q@eh^c;dsP,<<7dO.L7_mnoF
S,u6X#Y?!<"7TG!`s,DT2PDOL"tlF"KO,tekbH3#W%/G%+MH&)-:fuj_K`Tu;HQAK
!m4D&d1e*dQiplo"DMO08eRL%W5,7N44IBO0CHmC>U0;F0QM3i6=ga.GV8?5[D4j!
WW3*W`\1o?_b%m"mV'"BaAn),,JbZm`ONH+A:A&-L8+-(ap1<F4[`"_7#!J9&K\h>
<CK?rqT;f,c=ef:@n(QU9M'\TLG).iRn59D8'b`G'U;338P!n,.ZS-T<<Ys,$VA38
8d!=1<3]'%AP2<99.@;+Td3lr%'GgK0.:Sum6%NQ]MU@VbtBGdUgX^"^nZpS@VFCj
6l)cef,DaV5`*MQ@_S%@9`JWsa_=M/9gV1@9X%L=nV6cuA8ZZ<AO*.CEQ%X2CT;>/
*^\CRWeqr+&#EIV_I.,a<X--UENKZ@J4nnK9CarBKKVS.65#0C!UP[f2$eCr??RX[
].Iin6;T']OBAm1?quUs.qD7jG=8g:!VR3h`!jeR/B&/)Fn/ME&.0OUde`PR+@<$[
,(CqI;?]Cg"HX2mP^QI&#.9R8-..2Td7Tbk>pp=Y&n5B4`FgH*68rD#i_PpEo&=2&
kTYrdAFJ2Y<./,^2?Yo:,aJN1FpMkm(LZa-Ar3E[WQASC$Xr6++sk*`O4e!D/Ro%h
qOen(<]]5`4t9T$"dV[]l+ZA($"XMJ[C02Kem(6o@57IfVEd>^/"Co;b:qLl.=j2Z
8H,9[*EI"/5QmihBV`m>9Q!Ce6\N0?N=\l50%8meP3U\p6n#o,lotu%DWDFDbs7FC
(of(?3^`n/kf@.>1E<0'6fuW[CbIn=JlTpSA!\CB7H$MmV";sb)Pb66l&^p\P-".m
G#nIK_tRC[cq05@df;p[_(+%H&hS3D@^Js67F&]11cjf66SXKB:Nomdb_OX:7ghh&
KoGtm2)0l3H*N7$_E9b%3r#s([Ak@H%N$V""X'+Ii)dXe!ar[eRNmA4HPG.[;P?MN
aSt7oHn#Eq8:M4qbrHTe/!ncn7nJ-%&mR(_&Qe'CQg8,4nAc=#IrQQ[WRlXf1FRJ=
1Qk@Y`\bpNGC]jD-eK4k.)8(a&9:.L@SiY$ZkjWk.+>!DEb&eMngsp#$FQc1UIs3A
&ktYW+Va/\C@'\;P+*PM*=8Xm+<k'4;j%7([>'b35]D<oA-2".gHBBBYipKtAB6$L
0\48)7SNlIUgYF)*2k#,"'"GijrU>,(;lMAS;JTdV)=@^(7^Hk6`\)X"(`%#Ed)GK
1fFgK;.0u:etZ[oV2VBb7Q1pX#Qa:CH\)UI(dh-*eS=,Rq#F?I6W>q#-m8U5OI""M
`Z]pb<I=ONS9Z':icr=5Z][/GJi(]?)([:/5>K!MPB1d?\N^g*V3F4iP_Jptq6cJJ
=+UE"Q,dqEq1_#[H'Xk7pfVV=mj,rL%-N8o!CPiiA'b7,'Jb<jCSJn-;&rqB_hhNm
4!r"8$moM(#EDoRlSS$TF0-O]Uf#&8AeV\:XHr6_JQ]pS8FX#N0_@_mYp(GD>7BZh
9JB>(OC@;k$J/[KO?t5\JRYY-e-76$UbrF^9'E%b$k!D/j@5C&,+A`aF_'Vg5S@@3
pejHZ07s*&==j2k.1ubZ:rd<KbbE6oM3ERS"%h9"'e+NkI(,,k9Z's_-l43Je!gY!
\lL@>K3]+he=mhW.3^oAcch!,/t`>BVM5'n<ZE8ooj2.KORSFc+X<pPrMY>M^\X#l
qN\<n%B7KFL\J)+VE(Z4%B@ZHb"A%.]!OHn\>FGf"$4/FPgQRNKriWUXVkcR8kTGY
g02)GAU%t-]'C/KP8?8RA"*2eRf."`!)hPTJgFPJ%W2n(j<BRUkCu?;!#qM[)Ron[
P3$#F;Cp.pQM0;BZ8S@gf"#5LU?PU`nDlH4"o-E!.<J-HOfl,S-XSm0B%'[/UVK4c
TM.gOD%Cc`d8%<%F.27^.*H.o9IAknB"GK?ek4r<NJPkPbs64.ABdYD)Gl,NF-8C\
5G7O[[8]ik'Z)5;67n'<JC"c.j+J[#3t/5tR.Lqqr'$i0)Eak1!B3iX$qBCE"VX:Q
q\o;6,E&Z`:-0*^3og]V8.at(8cabO]*ZTJ9Hm(=bmHAGR=Q`s5TRaYI8/51K)3C)
gdLbh879)(.U5ii<UFok?-A(q`[)a3r+`@CP.J;JiI#p[gjCU,J]KGq(P:8[]Slk/
b585JaZpUB]U74SGKK4!aumA[CkU&9$`]9mB58hk'oZ1n]#4_d6DlY3A2JW=U&l#c
9*3t5nVf^Pj]`H<Yc>Hnm^1qdl#i0EMiR]=!*.VFq&QQrCo9_:k;.n[[2R0;MU_ho
($8;YFI5VOPEUu*d2n40W^=>%bAU'CE-'0Rl:qkkhng#*SHo96is_cer4:@1as,R.
2;BRABd8E`a+T$LJ:eG%HRG3ddbKDH;`*&fSc$GQq6$A"h(LJ)=YY&-HNRp`YBCoI
%'o=^&)bFt<_`:$23(T`TdSSDNE4;8gSRKqrRDJ*3h9S#[n]<H3acG;f:$kB.>*Q7
je@!jjiap-2BD)?"+CB*L#5qYhj3OPSc64'Ddp</GBQjAq+KZmF2pH]I[6tljB[M/
"B-t-iiIg5Ga00c?N_*9EL"VEF[cEOZ.^re2A]d/qC8np\QUV!6@uG]i]usQ*?FEs
mO8il8F?Rj5E-*R+@s#k*GX%>jVp@/W3t80k)ZA,(.Spi:eOm%%Vo55&+$O=6\Jm^
`0]'5<A>\b,W@o4A60q)9(0Z>"@4QHOVU#=>[,C9/ZlDmCguJ)A`&FgJX3=jEYP-A
Rq*0>29+%MnmOG47n!LQ?+r67pZO[6$\cYkH&kc]ie')gC'T6b.mRmZ\9%luXX>8H
oZe3E*,"qRg%DK_p%T.S$[MGt:%nU,LOXDL^O,_::7Zlfhk2"bX6'-SL"q0BKE%<d
Jk-)T!&GLP@"YsG&8EAB#2t-s:lJ-s'T3-HR#58t)3"fpJOo9:5p6TUK#*:#Qn/sZ
KYelD?m];9"AHW3q6YAq.[>\(EPSf!JNf:C-^)TU7Z/;paCN^1d!S"tTEbR!=PRq>
6BfNk!V$>@4<:\+.RCl;Hok=;#"'PZ:hIWg&R=aTla<`gG`u>62QE<karRDblX>Y*
DV,ef"tu2)%/Tcn_V_9mM!Z!5R%2Ul<D_LI5sVgaFFp&?6r##X<9`!RR#jug'8cr"
J9Kdc&"Q?[1)U?q=r"bU!n4rDg0ZQ;blJc&G4LR%SOfmVc/:sO0Et7''%!G+;ABRX
]U-n(LS[&sL24#e#^RA*nouHe4*9sDC_,gGJk09-SMr#KGlPIU;c"("k_MX*":.gh
VuoTk157L/;q1(6YPLTc^!Q<a%4+9'EtUlu5UN=ZmgJLX\'*dC%&>@'o*Rd^:eK1M
/p#GJ]^I(q#e3VKMPC4?8n-pCc@U<_6SC2ulq#FN\F2VB'O(mTa_T7m6LkfBW'/IW
2YfOV>!SXuO5'O2+cm%J!N!"O_ZQVe84&+8n7''9_D%K1004/@<=P`8lot/3+KS'G
`3DF'1Wp(5?Dp=B"D5(EENheM"XM<X$)hP^3CX%b?l0+M!.Z>b,J]a(,6<<s'EnM[
4]'n2#h+%>/Wes/U,^:VP,1<5`)@GL$1qhi/P?`%YJ%aJm'<X!d[Ma;.53Vlg$EQH
N45*6<654O#WN?g91q=Y,QQ9ZWa1LOpo_"3pcuG7f2CV3K.,9'#J6Xg=^nN@P,i8&
pf6cqhWn(H$mTtZm(!6eXTT$YX)_/E\P?)3#D,dc)-L"iC-tg!o-<p#dSD'1c%8ir
?ZJtd6:4.R3RBhGK/+clQT*B<+"dT]jZsTtP9d7G,QQtK&AO#4Ar6b\RnOOD'VIVt
k$Xa7T!9^E3n4@1^9P%^1dkb'K/M]L5JQ.0-&c>1%Qp->)&(P`!I6LpPU3=^<NYIG
&p]l,H5::UkQ&>jaB_s:J&=Hr*fHf_8`l5H78Ku+Vrq6H"fgkT2RSidReFQ90gNIo
&o?([e(SRkrn%V#i.ru1kth+#N@e7A`1bSj!%=Hpl"*j.Jn`,*Rpm1E,l-23#WA^U
^n7$(!fQ(G$mu?BVgS%`;We<9T`*nm.OkN(p"SE4F`=tCG7]f\lH:!K78._SHLFQr
04MXed?-OMjCRKT7V'o^TdEJ[<",n:SlF?V?Wk@,W'P'P?H?mU5sUr6)j7e%'5L6]
Y#N+e-<fG$di*P/YR\"FfEDj;!WjZi^)urkA5k8lI)(UQ2HW;:e&W[sk3SD,,E.r7
+mt%:<:H[71^)K176/I<Q@U6*"(L7YMSNN$YS<b_$"R%-cD@Hd0LTW+5nO9r&5L)/
Ta?eVAVqs0'p,>4Q_Auk0nmI_!LR\[+iHE?,VgFAk^E`q$q#1m((eE;ge*Re9T8--
-]k:tcsiInOg/@HSG9Q0ALq4ekthY^(RlfmCKld/1,a`Oh?i4u2%uf#[56G^[NS3j
>[UDgJJFEZ!0KGm;#)Y*@]3VkOi0%0/.*2m"!Jc1^-Cq*YqM9_#E&=S>Hh58557&l
O8AZ&X6*]R_UU#A!MNZZc5i"f%]d[u)(/A:"eHo1_B\-qHOI)3)"KXm8uq#*b=K5H
0N8C1.BarYbsoIW.j/;s?T@-"^AtQKDGG5<O"lV-]%Pl7UUrYk:A)o\;YXu-NA#%>
\sX;cP2dp2TfpNY'@TG3gmg*HMMHQea:LU)8=1q3[)a#F67`Gl\078;773d,9LSt*
A0HOsM'?+OiMa,]UEDa[dF)l%fsL1C8)aHq;s-`t*@Z[O.Qg;V>"!(L0r?eO_9#b!
'PYK/VfhF!cUNO`)4a0o`)<C_lBXk;Z0nVGVQ$0PWXC;e;6)0@T$1(lA;fa)HEVk:
9Jp`BklTm;jgnp@EdDulnKV/E_;l>a05<&f]`S7N]>)E6Gtet0R]lLLP%C6]MLZq^
';W7eF%%me""j[0E"JIjBe=(BaL_d%dK3=X>n@1=4<RnT'Euq1<h7E[No[W$Ei)FO
iobajE5[mT*6O?(Of3#+59e]GqJT$<U^U\-&d3aAjqD14VY^G=3V$c^!C`DOKFTgT
6C>r!I8CD/,pX/TJXO\D7\G5&Zl9QE>+#Y2\>5!\+C%5B6WF7bocPOp"F4f&)R=%*
r":@gLl#f&^;d2N8/4"<P/[C7GH&&>k8QrG(`0u`WrpdD'e/4h%5Sh`Sm`6HK\:M`
+dcTG+_?djk"KNOGo%'ulq.TS3<[<'V\Wb$,E+@AAOMZ78`P.'`aT$2a(_:iW4[Us
b*oFW^e%O>Zqi1%>fBs`Ee(afTLY7K_9YOEN?'e(6PbD_GLRV<(*c,"^i$'.=ufU/
KBm/BX-C"f,3NB]5$t3WUKXKSH!\\TGn1C@-Rk^O&o<F1mbTL0ZnrL/J6T?c1MEK?
M=g$^!X=Q;JkrGEj=c5X?)?NJ.V7"_>fiFGSGBl2mTGPaE`rQLn-W[Je-1BT\%0n#
\WZ3n-51-E8t6gf.KG9\JuW@N?\R=@2E6MZ_jjD6ft>i^n=<s51Dj!k6=XZ]V."=0
edXpDCD4o$\7<DmV)/[tN[iekL8rf*pFgWkOG\&cRE,+&"L4KHM%N!HU);BV,R<hg
@I-8FZ6<$WH`.;?NSD)>MgjNA%sq<bN=u!8@fcK!S`c`=#P\iXk8YE#Fo%.t5sGc9
r&MN3")d7?i?M_M=Q$7Icc4.@*Am]KON="`-aE7FjQh_gbXpl"3Ftl@gq4_M(9,OQ
:M/bEil9L%O3^Z&5EhW@eT<Y3#^S)8aLrs.&]_MXPuK\B9G6knSTkB!S+f>W>`b)M
(1rEF*4e)M\(knH]'iCP<r+IW'C.Zsgtop!7Oj#H6KSPGp`d>!nU'-Pf[/L?.CKo\
U&:\V:]S0'fUhW7)]pU:G%`Hja79unc^f'CW$=/bPh<SZ7Jn0`pF_2nrbS@c\=g`[
&!HF[@&em;[PI[M,P^.FW[\"**KELb!([:/E!n9Ql8^:7%Z$T)C7`3pOIZ\QV5gGf
Ln^ppWfd\fU^A!#G_V=^[/e@DLku$K_T3`k"$5WU_.32Pi]<&rWO$gfR]IDXREmsI
"<DQ*_!:na6U&<>n%`H=&i9kZOPBh`$6N4T&JPX4fqK!$_88_N_"ou@Hd&"]&da2f
5s#4c8;.]pI/qb56%IIE<#LKh_Q.2d_9)>cg!RY-'F:KX'/M('F<e9k4H+?m%M67<
fXj&B9aJp@J8@%ObX`d07i2"P1C=C-5uJ05N@<I`!)cK=+Vl+in/qLAVdf3=377gO
j8gIlN1^Y&(sn0*FfiHlT\pA6_W2*)#sSf&(V9=+fW);8=sN*5T0TZJ:sUaEJ;]n.
$_m$caKZS,NjMAsLr]uJ!"agVgo#,\Xilj"5rTGAH6sKl!%`5KTtE@3Wu2;ENUf>t
,Dr<h'$!NEJ2DYi.aoGqVAkD6S;C!l9+N9#%l%P*^JcbRE=\8UUOb`U!=LPGlPtH_
b.P#'7<o'$gJB`u%hEZ=%WdadfdN4!%Cer'7e0<p"EQuI!(SS[,&@IC]R.\%O%3rh
S(X[ZMJ+;&0beGNa2e?QgmF2Eq\4nE6-6&r'S8EW&'-eua@qE2=V"&:MF`%ab*40m
Ul-<VprLqX8Djre3CHF=gW:($1W5Hu31Mg18[UQ_`/,]RTj&6sh?_4A(u"X&C&.gl
>K!HF`1Z0+3`6e>9GE$RTV)de$u:BX:_gNF`</QIJaSCgF0[!,$Cbe.nIQ&.rl08=
\[4?t,[h&7CC;i.$Ln?ii45Ia?G]>/`M;S<kRmnU'nKQ3PJ@c\q+R0K\h:gHT@C4J
Ms<1#?mi<8(I3ZWTY;onQq+Xec@>tQQi[6f!!!^TJ2isI@@=0Y_\g8l$#>9PKIO_n
4A!braMcoKXPlFc#Kd>8.,%?Cbk$hcY*iGE2>e7(./,i6(.&Zj+7$Nm_VIa^0<l]=
9pcYEHGI,g8f,pH%77mg.?#._1.RGMO[r!f@D<,-kK]%NcE->^/F7mTmCXUtWEDef
q8PL(#<6\X*6BVTU!V+YXVCikcZn3jMlY0oGYbUDccZGefS*,dR8<b>&eW_l'"Ab-
M,5s=cp//``<?:%"pg1n/-Q<Ym0TbrO?*I@RIpsp!(Vmn]Dt)Na&u>k:mo+VNQ[t!
7"\LQZ3R%T%5O."7"_l^Yid'8N6*><J?.rWSAm`+fFDk['tIX6,Li;_"g/f'N0-Po
@,He1HbUe:&*6D/.2*6-]rhF_V<K0H=NhEKBSjTPbVEcX&.cD;V#]h!JF\FCC?h/.
llMU=Ri&CnZdTLKj91S$8Z:a-ROk3fScFHb$%N,u;83tM*"1d4$Y!e/b)Ofk;4@Wk
bPc7?m4OCh9Ir%7UD\V,q?Er3V#[iJc4l<F=GB.mR&(W)!1L<ti[RME490eD'QYTh
OZ55i^UnFn6XYWL,8NY>&Aeb.TkM.SD*A9a%8Ko2;dc"o*![O%@obhtel:m7@T<Df
B<p?,N6Q(+okN&$UDO/O<n.Nf-#YuHeY=A)'n#ETATPGJFM-i3&,g[.Km2.,"H$cV
V-6kRV0ik4I5bW>ZdC9GD1C1D%G2Se==o/en_@5D'%gRufQ;!?aI6$jN6[\H'qbc&
id3L]#Ig,*-b-PjdL(sGm*i(.!0PG2,6C9D?-BO#P\#3&^lAbiHe@m_Q<<TDdJOF+
A!!+%/\mlFM/*I"[ZN/S)%p9jRI%&Kod%^S%_L66\`Bn5d]\4>bt385-!?%['s#"%
!Eu"r61UX1eduWsQG(R'd%CN+nGl7Uc@t&((]m4SgOOq:_BT/AgnQ$>5*'[4+#-/<
"#78J+H4tG8P%_LENC#*9H\0tV>0uu:_5lb_LTl(Vf\^RP7,nS/21K?f28'\W"oD]
+('+3ch2FMQ/g*sRhOGi*9]oK[G5'<h;.<ph?E(KD;r1la-3G8hFS77>7B@6,2RUg
Ut`N_:$T='ldq=Y?I0<kj<bMY^YXhrh[ohF,q_77o8coDPXY9&D>2q,KO9U/?_.AW
XKUNu'OT5AQ+6!Mn='Dl;h/Yle%/rnn-Cm?hct^@M)`'p5d7-7DMo-XNZ)7O5cgmN
[krof%s%&qi/LEi522)FXp!`1lHdWh-fEr!Q?m9Rq+];$Bk%4/258EUZ@^kq!\K78
^!"ub0hoa+'*0V7^H0!8;XN"h-5N[jT6RS0;%Ef21aZ&%JA\n0)D?VXM#]s71=Aje
_RDN=0e$!7'U$5h8<AjSC>Jii>&H=H*`";Gmbir#3M7,gEgM>Wm@<H,dShj1'JCt#
?I1F'/t3M]EkC#A^/fsVfPRMJ$_0dWUZ?ZuA;m+a=:+&j@:[%g,-#)4f_Cm&&LV0d
_AU^.8IoATgZ:>(_--+R7U8h-q&T"C+#[6_Ql+qf%;!3Qk@P9p[6#o([UoNh?[cHk
P:Tr:XHO]:WKq.a#`PWYG/Ot,5!bR#E\?+P#71!-1/[OMMJB^\$`B:R2<3AGbsS.#
Pr+M%2S#+5*#(48he<+9j,@G+nc^#e?YJOs-/gVOqVbE(8#5Jc`e`&$;X0K;Wfm!h
M>M.efk?1B7_6="Vf`Bah@J%`Wp6pnOE@ShYt5DHP30/1=P\>hfbV)`O!.0!cVP%=
K<6+9[R#I-cb2'dAoOe_WB/&!CEC-f0!%l%]ieXICA7p1BolLn]k]3l,jr$1.F\@>
]&r&ib5So$\4<D8I#ZNo(%TYaX46C%R5A&H'erXo=H,T8TN+#ej2uBaE3gnfEJgVI
W%g^\EUa>iASJE&A5SpfZ!tj6SVYi;9H5NU"&m*)9qe\Cf7k_`$JF5&29fr?/JQ0s
H/`P=mOqD^k3b'`XDO'gs4rmjT(3?0o1D>7$eZ/Q$%]psb]&)p^K6!RiPZ!%4J93H
`Xd&2*3N-PaZI<A0p<ZD)VdZL%??V$1nAg(4S2$%2Ma[CA7[<>h9;OKUjIrYoicJ_
'""'0l.6>-qNCgR?pm'?aYKCm$jjR77g\rV_`ea&o%KNJRN!05G4P)d$HF"#BeY9[
C^F4K;f@uu%M&@A<r<pqrBhY*Wcb3.!S$TMO<e$Vn2#SZ@h9L7"jB!HE-MJ(N-t,b
FRc`(g3=1uaP64=6!96knGWO,&mdimKlJdOT('2YbcrY<('nLDU[*'/ae4<9Y*D.5
70bd^#&H5<>=="riU"UM^]t1afI=["VIN3PU+ToJq`;Va$#ZP-Y`kAt]X8pn(9j\'
g3j7jX+7Y9iPsgC%6."+;oQ*Y1A"J8c6qk>fkt>'JEH88nAM0pgnPRLW!Ek]8C\5q
%o#\.C!FXN9]K@3mYq6_VPm%T^mYaUgl?%Q!*JB"'Id+3ILdeg+_aMZa"qnZCs!06
d3L0s^Ffh]NNKd`,^'<S*kDgZFBd"T&U+;F.r[29&$P[<8nefNLFHu\auSP9JEs$Z
X1(JFY4sHf:`)cISV_l@CJi]#;epVCO)F8"DqV]cG7>rS8=fK'"Eug-G>#=4QZekm
GH;R"pR.\[M+*SF%en>3%F9Jg3=g?5e9DBe)@lsq0G[3heTaZS(.QHA5`g56"_RS@
oMilTQJtuMmVM]!g`n8?QUb9DYJhAk/T;+m14\qqZIZJ297p0M?LVEk$D*bm2_PYS
Vb/O5pEk2(FSb]G7Zd\4PI6"q(2VJ;?36HA[1!&?0#I#1B';(FQmaG:^3J;1HS3Sg
/.'q/[9^;mbA9<7nX<9G9E&GNJJQ3oG/sH1i/%l)i;7't0c]R'VMdT5Bh%&/).o=r
g:7pZ(-^S@SRpd"Nk]LXT+oB&mh`)Vi&u\/&aa8":uc&%ku7iCM+6sPJ,p';n7U)G
%?L+De=hc/jSUBL`@mYuMLB?=^^c.uML,9VfXbGK.gNCg#6oV2Tmf:trVVfXKpqud
Y^S8:L]Dfu!t`:V@W>'g$O[N#@DRK(>UBu=704VdQs`*"&46RE#hX#7)%F\SZ?WH=
0,9@tA^[P+Ccqq27KTh4+DiB\Skj!taoY%cO%,mAaSJ=PP<u,l;Fr-n,+VN(ePW]R
6;k3_Wm>FeFF$QeA$Mioob;^5X$F*tBf=*+`n=Xh,:No:;CNDI78FL$F?1n&=0U?j
M,^o00oNqP.JWP#Ef54Wh/;tO>o(=R8Yk]u)T=KnPJsCMH;r1f)bd`rE(Ip%G8c^k
e0nGrU*c(D7-,jWr:3]0K;hf!n.5~>

Q
n
Q
Q
Q
n
199.165 741.182 -44.143 2.09198 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
199.165 741.182 m
155.021 741.182 l
155.021 743.274 l
199.165 743.274 l
199.165 741.182 l
h
S
170.989 746.614 m
/N157 12 Tf
(5) show
n
172.334 747.123 m
172.828 746.685 173.464 746.466 174.245 746.466 c
175.196 746.466 175.947 746.813 176.498 747.509 c
176.95 748.076 177.176 748.748 177.176 749.525 c
177.176 750.342 176.919 751.01 176.404 751.53 c
175.89 752.05 175.258 752.31 174.51 752.31 c
173.945 752.31 173.405 752.13 172.89 751.771 c
173.352 754.083 l
176.77 754.083 l
176.77 755.091 l
172.512 755.091 l
171.676 750.677 l
172.668 750.544 l
172.824 750.791 173.038 750.992 173.31 751.147 c
173.581 751.302 173.888 751.38 174.229 751.38 c
174.779 751.38 175.221 751.206 175.556 750.858 c
175.892 750.51 176.059 750.035 176.059 749.433 c
176.059 748.799 175.885 748.291 175.536 747.908 c
175.187 747.524 174.757 747.333 174.247 747.333 c
173.823 747.333 173.463 747.469 173.166 747.741 c
172.869 748.013 172.68 748.418 172.598 748.958 c
171.489 748.864 l
171.559 748.141 171.841 747.561 172.334 747.123 c
h
S
180.997 746.614 m
/N150 12 Tf
(\000P) show
n
185.586 751.981 m
185.586 747.943 l
185.301 747.674 185.02 747.479 184.742 747.358 c
184.464 747.237 184.224 747.177 184.021 747.177 c
183.849 747.177 183.677 747.228 183.505 747.33 c
183.333 747.432 183.213 747.571 183.147 747.747 c
183.081 747.922 183.047 748.208 183.047 748.606 c
183.047 751.981 l
182.071 751.981 l
182.071 747.314 l
182.071 746.986 182.047 746.588 182.001 746.119 c
181.974 745.846 181.906 745.525 181.797 745.159 c
181.75 744.995 181.727 744.858 181.727 744.749 c
181.727 744.526 181.788 744.341 181.909 744.192 c
181.999 744.083 182.114 744.028 182.254 744.028 c
182.391 744.028 182.513 744.091 182.621 744.216 c
182.728 744.341 182.782 744.509 182.782 744.721 c
182.782 744.842 182.745 745.053 182.67 745.354 c
182.565 745.776 182.516 746.271 182.524 746.838 c
182.684 746.705 182.847 746.605 183.015 746.537 c
183.182 746.469 183.354 746.435 183.529 746.435 c
183.79 746.435 184.099 746.521 184.456 746.695 c
184.812 746.869 185.189 747.177 185.586 747.619 c
185.622 747.186 185.726 746.881 185.898 746.706 c
186.071 746.53 186.303 746.442 186.593 746.442 c
186.887 746.442 187.131 746.542 187.323 746.741 c
187.515 746.94 187.645 747.302 187.711 747.825 c
187.469 747.825 l
187.43 747.536 187.368 747.343 187.284 747.245 c
187.199 747.147 187.108 747.099 187.01 747.099 c
186.932 747.099 186.857 747.128 186.787 747.187 c
186.716 747.245 186.663 747.341 186.628 747.474 c
186.584 747.661 186.563 747.988 186.563 748.456 c
186.563 751.981 l
185.586 751.981 l
h
S
187.911 746.614 m
/N157 12 Tf
(m) show
n
189.756 746.614 m
189.756 749.845 l
189.756 750.412 189.813 750.846 189.926 751.146 c
190.039 751.448 190.222 751.676 190.474 751.833 c
190.725 751.989 191 752.067 191.296 752.067 c
191.687 752.067 191.968 751.95 192.139 751.716 c
192.311 751.481 192.397 751.129 192.397 750.66 c
192.397 746.614 l
193.452 746.614 l
193.452 750.232 l
193.452 750.873 193.596 751.339 193.886 751.63 c
194.175 751.922 194.538 752.067 194.976 752.067 c
195.219 752.067 195.43 752.011 195.609 751.897 c
195.789 751.784 195.914 751.634 195.982 751.449 c
196.05 751.263 196.084 750.959 196.084 750.537 c
196.084 746.614 l
197.139 746.614 l
197.139 750.888 l
197.139 751.6 196.973 752.126 196.64 752.468 c
196.307 752.811 195.832 752.981 195.213 752.981 c
194.423 752.981 193.781 752.618 193.288 751.892 c
193.167 752.235 192.959 752.503 192.664 752.694 c
192.37 752.886 191.992 752.981 191.532 752.981 c
191.118 752.981 190.749 752.889 190.425 752.703 c
190.102 752.518 189.842 752.272 189.647 751.968 c
189.647 752.841 l
188.702 752.841 l
188.702 746.614 l
189.756 746.614 l
h
S
q
n
-223.007 588.369 79.99 79.99 re
W
n
q
79.99 0 0 79.99 -223.007 588.369 cm
Q
Q
q
n
-224.671 679.337 79.99 79.99 re
W
n
q
79.99 0 0 79.99 -224.671 679.337 cm
Q
Q
q
n
-117.471 682.79 79.99 79.99 re
W
n
q
79.99 0 0 79.99 -117.471 682.79 cm
Q
Q
Q
Q
q
127.217 488.721 150.635 22.7851 re
W
0.999985 0 0 0.999985 127.217 488.721 cm
0 w
q
Q
[/DeviceGray] cs 0 sc
0 9.3931 m
/N256 12 Tf
(Figure 1, Shew et al. )
[6.672 3.336 6 6 3.99591 5.32782 3 6 3 3 6.672 
6 5.32782 8.66382 3 5.32782 3.336 3 5.32782 3.336 3 3 
] pdfxs
Q
PDFVars/TermAll get exec end end
restore

%%EndDocument

LH
(%%[Page: 1]%%) = 
%%PageTrailer

%%Page: 2 2
%%PageBoundingBox: 12 13 598 780
%%EndPageComments
%%BeginPageSetup
/DeviceRGB dup setcolorspace /colspABC exch def
mysetup concat colspRefresh
%%EndPageSetup

%%BeginDocument: Pscript_Win_PassThrough

/pdfmark where {pop [ {ThisPage} 1 dict begin /BleedBox [  0 0 595.276 841.89 ] def currentdict end /PUT pdfmark } if

/pdfmark where {pop [ {ThisPage} 1 dict begin /TrimBox [  0 0 595.276 841.89 ] def currentdict end /PUT pdfmark } if

/pdfmark where {pop [ {ThisPage} 1 dict begin /ArtBox [  52.6846 415.507 304.96001 828.575 ] def currentdict end /PUT pdfmark } if
PDFVars begin PDF begin PDFVars/InitAll get exec
save
8.362 -24.945 translate
0 0 595.276 841.89 true PDF begin PDFVars begin AS end end
userdict /pdf_svglb currentglobal put true setglobal
 Adobe_CoolType_Utility begin ct_MakeOCF begin ct_saveCIDInit
%!PS-Adobe-3.0 Resource-CIDFont
%%DocumentNeededResources: procset CIDInit
%%IncludeResource: procset CIDInit
%%BeginResource: CIDFont BHBOWV+Arial-BoldMT
%%Title: (BHBOWV+Arial-BoldMT Adobe Identity 0)
%%Version: 1
/CIDInit /ProcSet findresource begin
20 dict begin
/CIDFontName /BHBOWV+Arial-BoldMT def
/CIDFontVersion 1 def
/CIDFontType 0 def
/CIDSystemInfo 3 dict dup begin
  /Registry (Adobe) def
  /Ordering (Identity) def
  /Supplement 0 def
end def
/CIDMapOffset 0 def
/FDBytes 0 def
/GDBytes 3 def
/FontBBox [-628 -376 2000 1010] def
/FontInfo 2 dict dup begin
/FSType 0 def
/OrigFontType /TrueType def
end readonly def
/CIDCount 65535 def
/FDArray 1 array
dup 0
  %ADOBeginFontDict
  10 dict begin
  /FontType 1 def
  /PaintType 0 def
  /FontName /BHBOWV+Arial-BoldMT def
/FontMatrix [1 1000 div 0 0 1 1000 div 0 0 ] def
  %ADOBeginPrivateDict
  /Private 8 dict dup begin
  /BlueValues [-15 0 600 650] def
  /MinFeature {16 16} def
  /LanguageGroup 1 def
  /password 5839 def
  /lenIV 4 def
  end def
  %ADOEndPrivateDict
currentdict end
%ADOEndFontDict
put def
/GlyphDirectory 1 dict def
ct_GlyphDirProcs begin GlyphDirectory +
0 <10bf317005b6d50bd3b903bc9f60e6e804630266f839393d56ae50a85fbe
ffec110deebde9f8a007323688ac> |
!
end
%%BeginData: 21 Binary Bytes
(Binary) 0 StartData
%%EndData
%%EndResource
 ct_restoreCIDInit /BHBOWV+Arial-BoldMT-Identity-H /Identity-H 0 [/BHBOWV+Arial-BoldMT] ct_ComposeFont pop end end 

userdict /pdf_svglb get setglobal
%PDF_BeginEncoding: N117 (BHBOWV+Arial-BoldMT-Identity-H)
/N117 (BHBOWV+Arial-BoldMT-Identity-H) /Identity-H [ (BHBOWV+Arial-BoldMT) ]
 /Adobe-Identity [ /Serif ] 0 TZzero
userdict /pdf_svglb currentglobal put true setglobal
ct_T42Dict begin
-0.559 -0.375 1.156 1
 256 array 0 1 255 {1 index exch /.notdef put} for  /LEEWGB+Arial-BoldItalicMT
Type42DictBegin
[<00010000000a000a000a000a637674204dfc6493000000ac0000069c6670
676d499f2d4700000748000005fb676c79667e794b39000037dc00000126
686561649b4a813200000d4400000036686865610c5208bb00000d7c0000
0024686d7478b7fafdf400000da000000ef06c6f6361000426a800001c90
00000ef46d61787009470dc000002b840000002070726570599dddfc0000
2ba400000c366764697200000000000000000000000005ba001b05ba001b
05a6001b0426001b0000ffe50000ffe50000ffe5fe6bffe505ba001bfe6c
ffe502e70000011c0000011c0000000000000000007a00d60127011800f5
011200af011d00ca00b400d8012a007c00cd01640016001700fc02240020
010500060018005400aa00ca0107005900b3ffe900a8005700ec04010091
00e0012c005600cc010e00030055009d004e0115ffab00eb0102ffe00017
003a005000900114057605d80182000501030285ff2f000d040100830014
003e009c00d3017c09b5ffd5003700bd044cfff100980118022a000e0070
00e600f00127012d0238025dff6d0061007f00c1010603430593ff2c006e
00fc0386ffa3ffe9000700530055005f007e009700eb013e01c002af0564
001c003f0048004a005d006d00a600ad026605f0000100020026006c00a8
00c700e801ad01db03e803f90408045e048c0525fe3f000e002200330038
0057005f00620073008c009800be0100011f015201990532fd8100160020
00260031003800800082008900b30100010e011101150156019d027e02cf
02ee04a905d8ffcf002600340076007e008300c100c500eb00f20106012e
0130018201b901d10201027902fa0320ff00ffbc002800470052005c0077
00810090009900b200bc00cc01c1024d0343037703b004eb04fbfec4000c
005a0062007b00b300c900d500d60112011c022602ec0321038503a303cc
03f503f90413048304fbfee0002200300031004c004c0053005d0073007a
0087008e00a100ab00b600ba00c100d000d100db00e501150138016b017c
019e01bb01f601fa02210222023c026f029502b002ba02e2031603510354
03710396039a03c603d304110442044b049d04b604da062d06e80761fea5
fee3ff4eff58ff81ff92ffbbffc2ffd3ffee0009000d00220023002c0069
006c00710077007f008c00ae00be00be00c800d700d900da00dc00e500f5
0100010c011b0135014a01530155016c0172018e018f0194019801c501ce
020a02110215024f02500267028602c802cf0339033b03b8042804320445
045a046b0474048605320532054d058c05a805aa05ab05f005fc061206aa
080008ccfd2afddefe68fe76feddff0aff0eff1eff30ff69fff50005001e
0038006100670087009b00a100a400a600ac00c000c400cc00d100d400d9
00dc00dd00de00df00e500f300fc0114011601180118011b012c013e014e
016a0178018101820198019b01a301b601b801bc01c301cd01d001d101d2
01d801e101e201ea01ee01f002030219021f0223022b025f0268027f027f
028602930299029a02ca02cf02cf02d002d602e802ed03100322032f0338
0338033c03410342038a03ab03d0041504170442044f0475047a049d04a6
04c004c104d104e30500051005130524052c054b058b05c005c705f005fc
060e06180626066e0683068406a506b807040716073607820789079b07a1
07d40814082308a008bb011b01280119011a000000000000000000000000
015801c600af034c015901870154010d018a01590014022b00a10471024a
049c028f022a02ab00000000063904b00000000003a9008e0301020f0490
0391019400b50101003b0084013e00770192008c00c6017000db002c009a
03bf03fe02460100030001a4013800f603cf0000ffd501c3013401310147
004a02c804ce05c75c870224025e01d9045e060904c6009302bb04600435
040101b6017901000088038d003600ee037303e400cc016d049000be017c
0104003d023b00f4010400d6010c01100125022e003f0149031901500366
011a011b0179010000d5006e006902b1023f00c40194026b0328017b0132
00f500fe00b305c30099055204d5ff4e04b5ff2000fe007a0000000000aa
022e00b00000018c03600429ff57fef70187031802c10326023d01f20461
0269feae014f013402e503310173027401fb01b3012800a600ca024d0241
011a02a4000d00f500ec00dc00fc00f100b20493038dffde03abfe5102bc
0024055c00d200f00106005102ba01f300d300aa00be027f020800d801ad
043600b5036e00f0036002b802fd01f702f7009e00ae016400af022701db
024000ed065f04e001e56f0e011e0366006d000200a50006006203ee0041
ffe1001f0174ffcfffbf011b024f02ba008900f105c3026f0092007b00be
0099007e0098006100f3006c000c01790005000e000e00b300a100f20053
0017000300050007006e0077009a004a00ba007300d5005d00e800a100dc
00f6007f009900db02010050069c010600f000c200f500fa010800b90032
00af010e003800e4fff604d2000000b40089030100c30713063e048600bd
05bf073e404254403f3e3d3c3b3a393837363534333231302f2e2d2c2b2a
292827262524232221201f1e1d1c1b1a191817161514131211100f0e0d0c
0b0a090807060504030201002c4523466020b02660b004262348482d2c45
2346236120b02661b004262348482d2c45234660b0206120b04660b00426
2348482d2c4523462361b0206020b02661b02061b004262348482d2c4523
4660b0406120b06660b004262348482d2c4523462361b0406020b02661b0
4061b004262348482d2c0110203c003c2d2c20452320b0cd442320b8015a
51582320b08d44235920b0ed51582320b04d44235920b0042651582320b0
0d44235921212d2c20204518684420b001602045b04676688a4560442d2c
01b10b0a432343650a2d2c00b10a0b4323430b2d2c00b0172370b101173e
01b0172370b10217453ab10200080d2d2c45b01a234445b01923442d2c20
45b00325456164b050515845441b2121592d2cb00143632362b0002342b0
0f2b2d2c2045b0004360442d2c01b00643b00743650a2d2c2069b04061b0
008b20b12cc08a8cb8100062602b0c642364615c58b00361592d2c45b011
2bb0172344b0177ae4182d2c45b0112bb01723442d2cb01243588745b011
2bb0172344b0177ae41b038a45186920b01723448a8a8720b0c05158b011
2bb0172344b0177ae41b21b0177ae45959182d2c2d2cb0022546608a46b0
40618c482d2c01182f2d2c20b0032545b019234445b01a23444565234520
b00325606a20b009234223688a6a606120b01a8ab000527921b21a1a40b9
ffe0001a45208a54582321b03f1b235961441cb114008a5279b319402019
45208a54582321b03f1b235961442d2cb110114323430b2d2cb10e0f4323
430b2d2cb10c0d4323430b2d2cb10c0d432343650b2d2cb10e0f43234365
0b2d2cb11011432343650b2d2c4b525845441b2121592d2c0120b0032523
49b04060b0206320b000525823b002253823b002256538008a63381b2121
21212159012d2c4bb06451584569b00943608a103a1b212121592d2c01b0
05251023208af500b0016023edec2d2c01b005251023208af500b0016123
edec2d2c01b0062510f500edec2d2c20b001600110203c003c2d2c20b001
610110203c003c2d2cb02b2bb02a2a2d2c00b00743b006430b2d2c3eb02a
2a2d2c352d2c76b8025623701020b802564520b0005058b00161593a2f18
2d2c21210c6423648bb84000622d2c21b08051580c6423648bb82000621b
b200402f2b59b002602d2c21b0c051580c6423648bb81555621bb200802f
2b59b002602d2c0c6423648bb84000626023212d2cb4000100000015b008
26b00826b00826b008260f10161345683ab001162d2cb4000100000015b0
0826b00826b00826b008260f1016134568653ab001162d2c4b53234b515a
5820458a60441b2121592d2c4b545820458a60441b2121592d2c4b53234b
515a58381b2121592d2c4b5458381b2121592d2c014b53234b515ab00225
b00425b006254923451869525a58b00225b00225b0052546234569604859
2121212d2cb0134358031b02592d2cb0134358021b03592d2c4b54b01243
5c5a58381b2121592d2cb012435c580cb00425b00425060c6423646164b0
035158b00425b00425012046b01060482046b0106048590a21211b212159
2d2cb012435c580cb00425b00425060c6423646164b807085158b00425b0
0425012046b8fff060482046b8fff06048590a21211b2121592d2c4b5323
4b515a58b03a2b1b2121592d2c4b53234b515a58b03b2b1b2121592d2c4b
53234b515ab012435c5a58381b2121592d2c0c8a034b54b00426024b545a
8a8a0ab012435c5a58381b2121592d2c462346608a8a462320468a608a61
b8ff8062232010238ab9034303438a70456020b0005058b00161b8ffba8b
1bb0468c59b0106068013a2d2cb1020042b123018851b1400188535a58b9
10000020885458b202010243604259b12401885158b920000040885458b2
02020243604259b12401885458b2022002436042004b014b5258b2020802
436042591bb940000080885458b202040243604259b94000008063b80100
885458b202080243604259b94000010063b80200885458b2021002436042
595959592d63000100000002e6676636c8475f0f3cf50819080000000000
a351bf3600000000b5c9a691fb86fcfd0941080100030009000100010000
696d00010000073efe4e0043092bfb86fd65094100210007000000000000
00000000000003bc0600010000000000023900000239000002aa007e03cb
012f047300620473005a071d00ba05c700aa01e7013602aa008702aaff60
031d00c904ac00a50239001502aa004f0239005a0239ffa7047300840473
00f30473007c047300680473003804730082047300a6047300d404730087
0473008202aa009002aa005304ac00af04ac00a504ac00af04e300fc07cd
008505c7ffe905c7005205c700c205c700590556005404e30050063900b5
05c70059023900470473003b05c7005104e3005c06aa005305c7005c0639
00b305560053063900b305c7005a0556007e04e300f605c700bb055600e8
078d00f00556ffc2055600eb04e3003302aa0014023900a002aaff8e04ac
00d70473ffed02aa01120473005c04e3004a0473007b04e3007904730077
02aa006e04e3004004e30056023900520239ff200473004d02390050071d
004904e3005604e3007c04e3fff504e3007a031d00420473002d02aa009a
04e3009004730099063900930473ffd30473000d04000022031d0056023d
00b0031dff5204ac008905c7ffed05c7ffe905c700c20556005405c7005c
063900b305c700bb0473005c0473005c0473005c0473005c047300440473
005c0473007a047300770473007704730077047300770239005202390052
023900520239005204e3005604e3007c04e3007c04e3007c04e3007c04e3
007c04e3009004e3009004e3009004e30090047300ad033300e104730078
0473002a0473002c02cd00a60473005a04e3004805e5005905e500590800
012802aa017802aa00ad046400a50800ffbe0639009f05b400e804640082
046400820464008204730031049cffb403f4006805b400ca069600a10464
00000231000002f600a802ec009406250087071d003f04e3006c04e30037
02aa001804ac00a5046400540473ffec0464006f04e50056047300a80473
002e080000be05c7ffe905c7ffe9063900b30800008d078d00770473fffc
080000000400010004000107023900df023900fd0464008203f400890473
000d055600eb0156fe030473003702aa007a02aa001404e3007704e30074
0473fffe0239009302390015040000070800008b05c7fff20556005405c7
ffe9055600540556005402390047023900470239004702390047063900b3
063900b3063900b305c700bb05c700bb05c700bb0239005202aa007302aa
00be02aa00ae02aa00ad02aa014e02aa013402aa000e02aa004402aa007f
02aa00e004e3001e0239003d0556007e0473002d04e3003304000022023d
00b005c7004b04e3007c055600eb0473000d0556005304e3ffed04ac00a5
04ac00bd02aa00eb02aa00a802aa009c06ac00ae06ac00cc06ac009b0473
fff0063900b504e30040023900470556007e0473002d05c700c20473007b
05c700c20473007b04e30079046b008c02aa021005c7ffe90473005c05c7
ffe90473005c05c7005905eb007905c7004b055600540473007705560054
0473007704e3005c0239005004e3005c032b004d04e3005903d5004c05c7
005c04e3005605c7005c04e30056063900b304e3007c05c7005a031d0042
05c7005a031d00420556007e0473002d04e300f602aa008804e300f603d5
009d05c700bb04e3009005c700bb04e3009004e300330400002204e30033
0400002204e10059063900b3069400b504f6007c04e2007e03d40058054f
007c034500a105a1007c046bffed04d5007e032b007908d500140800004f
040000990800004f040000990800004f040000980400009807d5016a05c7
00d504ab00a504d5009d04ac00a504d5022204d5010505abffe9050001c9
05ab027e05abffe905ab027e05abffe905ab027e05abffe905abffe905ab
ffe905abffe905abffe905ab01c005ab027e05ab01c005ab01c005abffe9
05abffe905abffe905ab027e05ab01c005ab01c005abffe905abffe905ab
ffe905ab027e05ab01c005ab01c005abffe905abffe905abffe905abffe9
05abffe905abffe905abffe905abffe905abffe905abffe905abffe905ab
ffe905abffe905abffe905abffe905abffe905ab02d605ab006605abffea
05d5ffff04d500920800000007eb013007eb012007eb013007eb012004d5
00b204d5008004d5002a082b0198086b01b807550010060000f40600006f
0440003a0540003704c0003f041500400400002506000055064200470473
005f05ab005301eb013603d5012f0715008d0421006104d5009202d6005c
02d6005c04d500b202d6007005c7ffe90473005c05c700c20473007b05c7
00c20473007b055600540473007705560054047300770556005404730077
063900b504e30040063900b504e30040063900b504e3004005c7005904e3
005605c7005904e300560239004702390052023900470239005202390047
023900520239000f0239001a0473003b0239ff2005c700510473004d0473
005204e3005c0239ff8b05c7005c04e3005605c9006304e30052063900b3
04e3007c063900b304e3007c05c7005a031dffd70556007e0473002d04e3
00cd02aa002c05c700bb04e3009005c700bb04e3009005c700bb04e30090
05c700bb04e30090078d00f006390093055600eb0473000d0239005005c7
ffe90473005c0800ffbe071d003f0639009f04e3006c02aa0134078d00f0
06390093078d00f006390093078d00f006390093055600eb0473000d0239
013302aa00970473002a04cd005a06ac00ae06ac009d06ac00aa06ac0072
02aa001d02aaffc302aa017802aaffeb05c7ffed06d50073073f007303c9
007306c100670771008406c700670239ffdf05c7ffe905c70052055fffb1
0556005404e3003305c700590239004705c700510556ffb106aa005305c7
005c05420017063900b305be005b0556005304b9002704e300f6055600eb
0556ffc206a100e8063f001202390047055600eb04f6007c03d4005804e3
00540239005204bb009704f7fff40473009e03ef006b04e3005404760095
02390052048700540473ffe604d3fff8047300990399007004e3007c04d8
ffe30442007f04bb0097049fff5d062f009906ad00830239005204bb0097
04e3007c04bb009706ad0083055600540716010804e9005b05c000b30556
007e02390047023900470473003b08c1ffd40856005906d400f604fa0059
056b009c05c1005905c7ffe905aa005c05c7005204e9005b05c7ff660556
0054076bffe20524004c05c1005905c1005904eb0059057fffda06aa0053
05c70059063900b305c100590556005305c700c204e300f6056b009c063f
00ad0556ffc205d5005205aa010907d5005907e9005906d500d808000052
05aa005205c000960856005905d5ffd60473005c04f4008404d500820445
004204f2007a0473007705e4ffcc0415001c04e3009004e30090040e004b
04faffce05eb005004d5004804e3007c04e3004f04e3fff50473007b071d
00490473000d071400820473ffd3052b008804aa00cb071d0090077b0090
05a8008b06d5005204c00047046a004b06eb005204b6ffd80473007704e3
005603c10048048100830473002d02390052023900520239ff2007c1ffce
073f005204e30056040e004b0473000d04e30090049a005903bc00380800
004c092b005905b200a102aa008b02aaffdf02aaffee02aaffee02aa00c2
02aa004002aa003f02aa004902aa004902aa020c02aaffd102aa017a02aa
009f0393012f02aa01960265009c02aa040d02aa000c02aa00c904a9005b
049b004e03a7000a046600e004ea008e022f0087034e010804ed00870503
00e0022f00eb042c00ea03ed004e03f800ef04e30087050a0068022f0030
0316005a04e800af0459000b04c000d604b2006f03ff00ec041800470495
002b042c00eb05b800e105630033045e0030045e00eb045e00eb023600d8
040900d8068b0087022f0087042c00ea042c00c203f8002103f800210479
003205b800e105b800e105b800e105b800e104a9005b04a9005b04a9005b
049b004e03a2000a046600e004ea008e0295007803810070050300e00295
0090042c00ea03ed004e03f800ef050a00680316005a04e800af04c000e2
04b2006f041800470495002b042c00eb05b800e105630033022f0087049b
004e03ed004e04b2006f04db008d0000ffdc0000ff250000ffdc0000fe51
0000ffdc0000fe510000ff160000ff160000ff160000ff160000ff160000
ff160000ff160000ff160000ff160000ffdc0000ff160000ffdc0000ff20
0000ffdc047300870800000006b300b3055f007c067800bb05b600900000
fef30000fcdc0000fd8d0000ff640000fd9d0000fe5c0000ff3b0000ff32
0000fe220000fd710000fe910000fcd70000fd6b0000ffce0000ffc40000
fe42041b004106ac00ae06ac00a80000fefe0000fdd80000feaa0000fd6d
0000ff110000fdce0000fcb70000fbef0000fbef0000fd2b0000fc410000
fc230000fc670000fc030000fb8b0000fc380000fb8b0000fee60000ff49
0000fe480000fc030000fcb20000fdbf0000fdca0000fdca0000fd160000
fcb20000fc440000fc4e0000fb860000fd450000fd3d0000fc730000fc6b
0239005205c7ffe90473005c05c7ffe90473005c05c7ffe90473005c05c7
ffe90473005c05c7ffe90473005c05c7ffe90473005c05c7ffe90473005c
05c7ffe90473005c05c7ffe90473005c05c7ffe90473005c05c7ffe90473
005c05c7ffe90473005c0556005404730077055600540473007705560054
047300770556005404730077055600540473007705560054047300770556
005404730077055600540473007702390047023900520239fffa0239fffa
063900b304e3007c063900b304e3007c063900b304e3007c063900b304e3
007c063900b304e3007c063900b304e3007c063900b304e3007c06b300b3
055f007c06b300b3055f007c06b300b3055f007c06b300b3055f007c06b3
00b3055f007c05c700bb04e3009005c700bb04e30090067800bb05b60090
067800bb05b60090067800bb05b60090067800bb05b60090067800bb05b6
0090055600eb0473000d055600eb0473000d055600eb0473000d05c7ffe9
0473005c0239004702390052063900b304e3007c05c700bb04e3009005c7
00bb04e3009005c700bb04e3009005c700bb04e3009005c700bb04e30090
0000003f0000003f0000003f0000003f04e9003903c10024076bffe205e4
ffcc04eb0059040e004b04eb0059040e004b05c7005904d50048047300e0
047300ae047300740473000b0556ffc20473ffd305aa010904aa00cb05aa
006d04aa005c05fb00b304730065063900b304e3007c0000000000000066
000000660000006600000066000000660000006600000066000000660000
006600000066000000660000006600000066000000660000006600000066
000000660000006600000066000000660000006600000066000000660000
006600000066000000660000006600000066000000660000006600000066
000000660000006600000066000000660000006600000066000000660000
006600000066000000660000006600000066000000660000006600000066
000000660000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260000012600000126000001260000012600000126
000001260000012600000126000001260000012600000126000001260000
012600000126000001260001000003bc0100003f0057000500020010002f
0055000004de0c3600030002b15440b8034db32f333240b8034db23e3340
b8034db345493240b8034db2503340b8034db25a3340b8034db2653380b8
034db31b1b3240b8034db312143240b8034db30b0d320f4115034d007f03
4d00ef034d0003003f034d004f034d008f034d00ff034d0004000f034d00
7f034d0002034cb301221f60bd034b007f034b000200400349b34343327f
bf0349009f034900df0349000300400349b330333240b80349b335353240
b80349b32f313240b80349b327273240b80349b32225320f410c0349003f
0349007f034900cf034900df0349000500400349b30913322f4121034a00
7f034a0002008f034a00bf034a00cf034a00df034a00ef034a0005000f03
4a002f034a004f034a0060034a009f034a0005000f034a00df034a000200
40034ab3293a3240b8034ab312143240b8034ab30b10325041100348007f
0348009f03480003009f0348000100df034800ef0348000200400348b309
103212b9ffc002dcb2404132b9ffc002dcb2393c32b9ffc002deb33c4132
d4411902de0001003002dc004002dc005002dc006002dc00d002dc00e002
dc00f002dc0007000002dc009002dc00a002dc00b002dcb2043790412202
cb0001009002c80001004002cb0001004002c80001003002cb0001003002
c80001002002cb0001002002c80001004002a5000102a50076009002a400
a002a4000202a440255fe006e00702bf06bf0702af06af07029f069f0702
4f064f07020f060f0702af06af07020f415d0342002f0342004f0342009f
03420004000f0342003f0342005f034200af034200c0034200ff03420006
002f0236007f02360002000f0236001f0236002f0236003f0236004f0236
008f0236009f023600bf0236000800af02360001000f0236002f0236003f
0236005f0236007f023600ff0236000600100235007f02350002000f0235
002f023500d002350003007f0235000100100235003f0235004f02350003
034a034a03420342023702370236023602350235ffc002ccb2213432b9ff
c002cbb2213432b9ffc002cab2213432b9ffc002c9b2213432b9ffc002c8
b2213432b8ffc0b36d1a3c32b8ffc0b3e91a3532b9ffc0015bb21a3532b8
ffc0b37c1a3532b8ffc0b3761a3532b8ffc0b3601a3532b8ffc0b32e1a35
32b8ffc0b22a3433b8ffc0b22a3333b8ffc0b22a3233b8ffc0b22a3133b8
ffc0b22a3033b8ffc0b22a2f33b8ffc0b22a2a33b8ffc0b22a2933b8ffc0
b22a2833b8ffc0b22a2133b8ffc0b22a1733b8ffc0b22a1633b8ffc0b22a
1533b8ffc0b22a1433b8ffc0b22a1333b8ffc0b22a1233b8ffc0b22a0d33
b8ffc0b22a0c33b8ffc0b22a0b33b8ffc0b32a1a3532b8ffc0b2273433b8
ffc0b2273333b8ffc0b2273233b8ffc0b2273133b8ffc0b2273033b8ffc0
b2272f33b8ffc0b2272a33b8ffc0b2272933b8ffc0b2272833b8ffc0b227
2133b8ffc0b2271733b8ffc0b2271633b8ffc0b2271533b8ffc0b2271433
b8ffc0b2271333b8ffc0b2271233b8ffc0b2270d33b8ffc0b2270c33b8ff
c0b2270b33b8ffc0b3271a3532b8ffc0b3211a3532b802ccb224351fb802
cbb224351fb802cab224351fb802c9b224351fb802c8400b24351f6d243c
1fe924351fb8015b401f24351f7c24351f7624351f6024351f2e24351f2a
24351f2724351f2124351fb8033fb28e291fb8033eb320231f5f4109033d
006f033d007f033d008f033d00040339b320211f1f41150338002f033800
3f0338004f03380004009f033800af033800bf03380003002f0338003f03
3800020335b624351f8f3f3c1fb80119b6243c1ff724351fb801b3b22435
1fb801abb224351fb80156b224351fb80155b224351fb8011b404e24351f
fa24351fea24351fd224351f7724351f6e24351f5724351f4c24351f4324
351f3d24351f3524351f37010012e001f001021270018001900103010100
090102000800171700000012110840bb0216000000090289b269131fb801
b5b228671f411501b400280401001f01b3015f0401001f01b00069040100
1f01ab00270125001f01aa00270156001f01a2b22a9e1fb8019fb22a321f
b8019db22a291fb80165b2281d1fb80164b228201fb80163b228301fb801
61b228411fb8015bb2279e1f4109015700270801001f0156002a019a001f
0155b22a891fb80154b22a891fb80153b22a431fb8011fb228201fb8011e
b228931f410b011d006902ab001f011b002702ab001f0119002a02abb21f
fa27b80401b21ff927b802abb61ff72a4f1fea2ab80801b61fe92a791fd5
28b80201400f1fd42ecd1fd221cd1fc3282f1fc269b802ab400b1fc069cd
1fbe2a4f1fb124b80401b21f9a2ab80156400b1f992a381f912a351f7c2e
b80401400b1f772ecd1f762aab1f7028b802abb21f6f1fb80401b21f6e21
b8019a400b1f6d27931f652a811f6027b8019ab61f5f2a2a1f572eb80125
b21f5269b80201b21f4c2eb80156b61f4b21cd1f4969b802ab400b1f472a
2b1f4469cd1f432ab80801b21f4128b80401b21f4027b80101401b1f3d21
e41f3b2a381f372ebb1f352a3b1f312ee41f232a451f2269b80156b71f55
0d090d093790b8012340360790dd07907207905507903407902f07902b07
902607902507901e07901d071408120810080e080c080a08080806080408
0208000814b8ffe0402c0000010014061000000100060400000100041000
0001001002000001000200000001000002010802004a0012b013034b024b
5342b0382b4bb807ff52b0372b4bb008505b58b101018e59b0382b4bb0c0
63004b6220b0f65323b8010a515ab005234201b0124b004b544218b00288
b801005458b80119b101018e851bb0124358b900010119858d1bb9000101
19858d59594358ba009f0216000173590016763f183f123e113946443e11
3946443e113946443e113946443e11394660443e11394660442b2b2b2b2b
2b2b2b2b2b2b182b2b2b2b2b2b2b2b2b2b2b2b4b5079b9001f01a8b3071f
36072b2b4b5379b9009001a8b3079036072b2b181db0964b5358b0aa1d59
b0324b5358b0ff1d594bb08953205c58b9021802164544b9021702164544
5958b904b30218455258b9021804b34459594bb8019a53205c58b9002002
184544b90024021845445958b90e080020455258b900200e084459594bb8
02ab53205c58b9001f02174544b90028021745445958b918a5001f455258
b9001f18a54459594bb8040153205c58b169204544b1202045445958b923
000069455258b9006923004459594bb8040153205c58b9015f00244544b1
242445445958b923a0015f455258b9015f23a04459594bb02b53205c58b1
27274544b12e2745445958b9011c0027455258b90027011c4459594bb035
53205c58b127274544b1212745445958b9015f0027455258b90027015f44
59594bb08c53205c58b127274544b12a2745445958b903aa0027455258b9
002703aa4459592b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b
2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b
2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b654245695342014b5058b108004259
435c58b1080042591610703eb0124358b90d193ea51bba00d203eb000b2b
59b00a2342b00b2342003f3f182b103c012f5d435c58b27f01015d595d43
5c58b2ef01015d59060cb0062342b0072342b0124358b93b21187e1bba04
0001a8000b2b59b00c2342b00d2342b0124358b92d412d411bba04000400
000b2b59b00e2342b00f2342b0124358b9187e3b211bba01a80400000b2b
59b0102342b0112342002b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b
7373742b732b2b2b2b2b2b2b2b2b2b2b2b002b2b2b2b2b2b2b2b2b2b2b2b
2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b
2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b0018456944456944456944184569
44184569447373747573737475737473747474747473454473454474004b
b02a534bb038515a58b1070745b040604459004bb02e534bb038515a58b1
030345b0406044b1090945b04061445973737373737373732b7475742b2b
2b435c584031402a3433402a3333402a3233402a3133402a3033402a2f33
402734334027333340273233402731334027303340272f33a0410a02cb00
0100a002c80001009f02cb0001009f02c8403301402a2a33402a29334027
2a3340272933402a123340271233402a283340272833402a2133402a1d35
3240271d353240272133002b2b2b2b2b2b2b2b2b2b2b2b737373732b2b2b
2b2b2b2b2b2b2b2b2b59002b7374752b2b2b737474752b732b2b2b2b2b75
2b0173002b7374752b2b2b2b2b2b2b2b2b2b000000>
[295 ] AllocGlyphStorage
]def 
108 44 
PrepFor2015
Type42DictEnd
1 0 0 <0002010000000500050000030007003cb40201b70607b802f54018000504
b703000a0704b7010019080605b70203b009bfde182b10f63cfd3c4e10f4
3c4dfd3c003f3cfd3c10fc3cfd3c3130211121112521112101000400fc20
03c0fc400500fb002004c000>/LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 213 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 223 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 3 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 4 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 5 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 6 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 7 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 8 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 9 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 10 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 11 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 12 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 13 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 14 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 15 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 16 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 17 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 18 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 19 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 20 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 21 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 22 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 23 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 24 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 25 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 26 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 27 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 28 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 29 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 30 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 31 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 32 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 33 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 34 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 35 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 36 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 37 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 38 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 39 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 40 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 41 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 42 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 43 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 44 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 45 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 46 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 
1 102 47 <0001005c000004a705ba0005009e402e2007012500250320042005360036
033d0440055603530450056f0470047005a7030f0203031f000114000001
0403b802c8400a05000802010201001005b8024240140004100460049f04
cf04df0406041a5007010702bc015d0003022400010244400c3000400050
0003003c060017ba02aa025700182b2b10f65de4fde44e105df65d4de42b
103c003f3c3f3cfd3c87052e2b7d10c43130015d01713301210321075c01
33012dff02ea3305bafb3bf5>/LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 48 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 49 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 50 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 51 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 52 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 53 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 54 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 55 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 56 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 57 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 58 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 59 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 60 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 61 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 62 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 63 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 64 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 65 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 66 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 67 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 68 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 69 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 70 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 71 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 72 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 73 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 74 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 75 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 76 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 77 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 78 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 79 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 80 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 81 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 82 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 83 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 84 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 85 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 86 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 87 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 88 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 89 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 90 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 91 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 92 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 93 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 94 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 95 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 96 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 97 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 135 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 188 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 195 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 166 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 196 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 171 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 130 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 193 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 214 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 197 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 226 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 189 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 175 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 228 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 181 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 182 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 179 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 180 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 177 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 178 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 215 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 140 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 227 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 190 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 176 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 229 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 186 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 163 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 132 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 133 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 764 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 150 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 230 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 134 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 142 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 139 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 157 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 169 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 164 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 138 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 256 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 131 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 147 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 240 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 241 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 141 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 151 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 136 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 194 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 220 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 239 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 158 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 170 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 243 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 242 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 244 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 162 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 172 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 200 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 198 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 173 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 98 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 99 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 144 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 100 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 202 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 101 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 199 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 201 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 206 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 203 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 204 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 205 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 231 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 102 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 209 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 207 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 208 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 174 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 103 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 238 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 145 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 212 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 210 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 211 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 104 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 233 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 235 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 137 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 106 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 105 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 107 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 109 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 108 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 110 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 160 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 111 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 113 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 112 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 114 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 115 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 117 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 116 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 118 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 119 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 232 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 120 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 122 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 121 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 123 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 125 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 124 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 183 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 161 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 127 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 126 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 128 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 129 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 234 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 236 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 

1 0 185 <> /LEEWGB+Arial-BoldItalicMT AddT42Char 
/LEEWGB+Arial-BoldItalicMT findfont /CharStrings get begin
/.notdef 0 def
/dotlessi 213 def
/caron 223 def
/space 3 def
/exclam 4 def
/quotedbl 5 def
/numbersign 6 def
/dollar 7 def
/percent 8 def
/ampersand 9 def
/quotesingle 10 def
/parenleft 11 def
/parenright 12 def
/asterisk 13 def
/plus 14 def
/comma 15 def
/hyphen 16 def
/period 17 def
/slash 18 def
/zero 19 def
/one 20 def
/two 21 def
/three 22 def
/four 23 def
/five 24 def
/six 25 def
/seven 26 def
/eight 27 def
/nine 28 def
/colon 29 def
/semicolon 30 def
/less 31 def
/equal 32 def
/greater 33 def
/question 34 def
/at 35 def
/A 36 def
/B 37 def
/C 38 def
/D 39 def
/E 40 def
/F 41 def
/G 42 def
/H 43 def
/I 44 def
/J 45 def
/K 46 def
/L 47 def
/M 48 def
/N 49 def
/O 50 def
/P 51 def
/Q 52 def
/R 53 def
/S 54 def
/T 55 def
/U 56 def
/V 57 def
/W 58 def
/X 59 def
/Y 60 def
/Z 61 def
/bracketleft 62 def
/backslash 63 def
/bracketright 64 def
/asciicircum 65 def
/underscore 66 def
/grave 67 def
/a 68 def
/b 69 def
/c 70 def
/d 71 def
/e 72 def
/f 73 def
/g 74 def
/h 75 def
/i 76 def
/j 77 def
/k 78 def
/l 79 def
/m 80 def
/n 81 def
/o 82 def
/p 83 def
/q 84 def
/r 85 def
/s 86 def
/t 87 def
/u 88 def
/v 89 def
/w 90 def
/x 91 def
/y 92 def
/z 93 def
/braceleft 94 def
/bar 95 def
/braceright 96 def
/asciitilde 97 def
/bullet 135 def
/Euro 188 def
/quotesinglbase 195 def
/florin 166 def
/quotedblbase 196 def
/ellipsis 171 def
/dagger 130 def
/daggerdbl 193 def
/circumflex 214 def
/perthousand 197 def
/Scaron 226 def
/guilsinglleft 189 def
/OE 175 def
/Zcaron 228 def
/quoteleft 181 def
/quoteright 182 def
/quotedblleft 179 def
/quotedblright 180 def
/endash 177 def
/emdash 178 def
/tilde 215 def
/trademark 140 def
/scaron 227 def
/guilsinglright 190 def
/oe 176 def
/zcaron 229 def
/Ydieresis 186 def
/exclamdown 163 def
/cent 132 def
/sterling 133 def
/currency 764 def
/yen 150 def
/brokenbar 230 def
/section 134 def
/dieresis 142 def
/copyright 139 def
/ordfeminine 157 def
/guillemotleft 169 def
/logicalnot 164 def
/registered 138 def
/macron 256 def
/degree 131 def
/plusminus 147 def
/twosuperior 240 def
/threesuperior 241 def
/acute 141 def
/mu 151 def
/paragraph 136 def
/periodcentered 194 def
/cedilla 220 def
/onesuperior 239 def
/ordmasculine 158 def
/guillemotright 170 def
/onequarter 243 def
/onehalf 242 def
/threequarters 244 def
/questiondown 162 def
/Agrave 172 def
/Aacute 200 def
/Acircumflex 198 def
/Atilde 173 def
/Adieresis 98 def
/Aring 99 def
/AE 144 def
/Ccedilla 100 def
/Egrave 202 def
/Eacute 101 def
/Ecircumflex 199 def
/Edieresis 201 def
/Igrave 206 def
/Iacute 203 def
/Icircumflex 204 def
/Idieresis 205 def
/Eth 231 def
/Ntilde 102 def
/Ograve 209 def
/Oacute 207 def
/Ocircumflex 208 def
/Otilde 174 def
/Odieresis 103 def
/multiply 238 def
/Oslash 145 def
/Ugrave 212 def
/Uacute 210 def
/Ucircumflex 211 def
/Udieresis 104 def
/Yacute 233 def
/Thorn 235 def
/germandbls 137 def
/agrave 106 def
/aacute 105 def
/acircumflex 107 def
/atilde 109 def
/adieresis 108 def
/aring 110 def
/ae 160 def
/ccedilla 111 def
/egrave 113 def
/eacute 112 def
/ecircumflex 114 def
/edieresis 115 def
/igrave 117 def
/iacute 116 def
/icircumflex 118 def
/idieresis 119 def
/eth 232 def
/ntilde 120 def
/ograve 122 def
/oacute 121 def
/ocircumflex 123 def
/otilde 125 def
/odieresis 124 def
/divide 183 def
/oslash 161 def
/ugrave 127 def
/uacute 126 def
/ucircumflex 128 def
/udieresis 129 def
/yacute 234 def
/thorn 236 def
/ydieresis 185 def
end
/LEEWGB+Arial-BoldItalicMT findfont /Encoding get
dup 0 /.notdef put
dup 1 /dotlessi put
dup 2 /caron put
dup 32 /space put
dup 33 /exclam put
dup 34 /quotedbl put
dup 35 /numbersign put
dup 36 /dollar put
dup 37 /percent put
dup 38 /ampersand put
dup 39 /quotesingle put
dup 40 /parenleft put
dup 41 /parenright put
dup 42 /asterisk put
dup 43 /plus put
dup 44 /comma put
dup 45 /hyphen put
dup 46 /period put
dup 47 /slash put
dup 48 /zero put
dup 49 /one put
dup 50 /two put
dup 51 /three put
dup 52 /four put
dup 53 /five put
dup 54 /six put
dup 55 /seven put
dup 56 /eight put
dup 57 /nine put
dup 58 /colon put
dup 59 /semicolon put
dup 60 /less put
dup 61 /equal put
dup 62 /greater put
dup 63 /question put
dup 64 /at put
dup 65 /A put
dup 66 /B put
dup 67 /C put
dup 68 /D put
dup 69 /E put
dup 70 /F put
dup 71 /G put
dup 72 /H put
dup 73 /I put
dup 74 /J put
dup 75 /K put
dup 76 /L put
dup 77 /M put
dup 78 /N put
dup 79 /O put
dup 80 /P put
dup 81 /Q put
dup 82 /R put
dup 83 /S put
dup 84 /T put
dup 85 /U put
dup 86 /V put
dup 87 /W put
dup 88 /X put
dup 89 /Y put
dup 90 /Z put
dup 91 /bracketleft put
dup 92 /backslash put
dup 93 /bracketright put
dup 94 /asciicircum put
dup 95 /underscore put
dup 96 /grave put
dup 97 /a put
dup 98 /b put
dup 99 /c put
dup 100 /d put
dup 101 /e put
dup 102 /f put
dup 103 /g put
dup 104 /h put
dup 105 /i put
dup 106 /j put
dup 107 /k put
dup 108 /l put
dup 109 /m put
dup 110 /n put
dup 111 /o put
dup 112 /p put
dup 113 /q put
dup 114 /r put
dup 115 /s put
dup 116 /t put
dup 117 /u put
dup 118 /v put
dup 119 /w put
dup 120 /x put
dup 121 /y put
dup 122 /z put
dup 123 /braceleft put
dup 124 /bar put
dup 125 /braceright put
dup 126 /asciitilde put
dup 127 /bullet put
dup 128 /Euro put
dup 129 /bullet put
dup 130 /quotesinglbase put
dup 131 /florin put
dup 132 /quotedblbase put
dup 133 /ellipsis put
dup 134 /dagger put
dup 135 /daggerdbl put
dup 136 /circumflex put
dup 137 /perthousand put
dup 138 /Scaron put
dup 139 /guilsinglleft put
dup 140 /OE put
dup 141 /bullet put
dup 142 /Zcaron put
dup 143 /bullet put
dup 144 /bullet put
dup 145 /quoteleft put
dup 146 /quoteright put
dup 147 /quotedblleft put
dup 148 /quotedblright put
dup 149 /bullet put
dup 150 /endash put
dup 151 /emdash put
dup 152 /tilde put
dup 153 /trademark put
dup 154 /scaron put
dup 155 /guilsinglright put
dup 156 /oe put
dup 157 /bullet put
dup 158 /zcaron put
dup 159 /Ydieresis put
dup 160 /space put
dup 161 /exclamdown put
dup 162 /cent put
dup 163 /sterling put
dup 164 /currency put
dup 165 /yen put
dup 166 /brokenbar put
dup 167 /section put
dup 168 /dieresis put
dup 169 /copyright put
dup 170 /ordfeminine put
dup 171 /guillemotleft put
dup 172 /logicalnot put
dup 173 /hyphen put
dup 174 /registered put
dup 175 /macron put
dup 176 /degree put
dup 177 /plusminus put
dup 178 /twosuperior put
dup 179 /threesuperior put
dup 180 /acute put
dup 181 /mu put
dup 182 /paragraph put
dup 183 /periodcentered put
dup 184 /cedilla put
dup 185 /onesuperior put
dup 186 /ordmasculine put
dup 187 /guillemotright put
dup 188 /onequarter put
dup 189 /onehalf put
dup 190 /threequarters put
dup 191 /questiondown put
dup 192 /Agrave put
dup 193 /Aacute put
dup 194 /Acircumflex put
dup 195 /Atilde put
dup 196 /Adieresis put
dup 197 /Aring put
dup 198 /AE put
dup 199 /Ccedilla put
dup 200 /Egrave put
dup 201 /Eacute put
dup 202 /Ecircumflex put
dup 203 /Edieresis put
dup 204 /Igrave put
dup 205 /Iacute put
dup 206 /Icircumflex put
dup 207 /Idieresis put
dup 208 /Eth put
dup 209 /Ntilde put
dup 210 /Ograve put
dup 211 /Oacute put
dup 212 /Ocircumflex put
dup 213 /Otilde put
dup 214 /Odieresis put
dup 215 /multiply put
dup 216 /Oslash put
dup 217 /Ugrave put
dup 218 /Uacute put
dup 219 /Ucircumflex put
dup 220 /Udieresis put
dup 221 /Yacute put
dup 222 /Thorn put
dup 223 /germandbls put
dup 224 /agrave put
dup 225 /aacute put
dup 226 /acircumflex put
dup 227 /atilde put
dup 228 /adieresis put
dup 229 /aring put
dup 230 /ae put
dup 231 /ccedilla put
dup 232 /egrave put
dup 233 /eacute put
dup 234 /ecircumflex put
dup 235 /edieresis put
dup 236 /igrave put
dup 237 /iacute put
dup 238 /icircumflex put
dup 239 /idieresis put
dup 240 /eth put
dup 241 /ntilde put
dup 242 /ograve put
dup 243 /oacute put
dup 244 /ocircumflex put
dup 245 /otilde put
dup 246 /odieresis put
dup 247 /divide put
dup 248 /oslash put
dup 249 /ugrave put
dup 250 /uacute put
dup 251 /ucircumflex put
dup 252 /udieresis put
dup 253 /yacute put
dup 254 /thorn put
dup 255 /ydieresis put
pop
end

userdict /pdf_svglb get setglobal
[/N120/LEEWGB+Arial-BoldItalicMT 1 TZG
userdict /pdf_svglb currentglobal put true setglobal
ct_T42Dict begin
end

userdict /pdf_svglb get setglobal
[/N121/ZYCIBP+Arial-BoldMT 1 TZG
0 0 595.276 841.89 re
W
n
q
q
n
0 841.89 595.276 -841.89 re
W
n
true setSA
[/DeviceCMYK] cs 0 0 0 1 sc
142.102 782.689 m
/N121 12 Tf
(45 mg/mL) show
1 w
4 M
1 j
1 J
[] 0 d
n
192.509 730.61 m
192.509 731.174 l
S
n
140.285 758.243 8.53101 -27.069 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
0 J
n
140.285 758.243 m
148.816 758.243 l
148.816 731.174 l
140.285 731.174 l
140.285 758.243 l
S
1 J
n
140.285 758.243 m
148.816 758.243 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
148.816 758.243 m
148.816 731.174 l
S
n
140.285 731.174 m
140.285 758.243 l
S
n
150.949 769.525 8.515 -38.351 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
150.949 769.525 m
159.464 769.525 l
159.464 731.174 l
150.949 731.174 l
150.949 769.525 l
S
n
150.949 769.525 m
159.464 769.525 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
159.464 769.525 m
159.464 731.174 l
S
n
150.949 731.174 m
150.949 769.525 l
S
n
161.597 749.23 8.533 -18.057 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
161.597 749.23 m
170.13 749.23 l
170.13 731.174 l
161.597 731.174 l
161.597 749.23 l
S
n
161.597 749.23 m
170.13 749.23 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
170.13 749.23 m
170.13 731.174 l
S
n
161.597 731.174 m
161.597 749.23 l
S
n
172.263 735.68 8.51601 -4.50598 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
172.263 735.68 m
180.778 735.68 l
180.778 731.174 l
172.263 731.174 l
172.263 735.68 l
S
n
172.263 735.68 m
180.778 735.68 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
180.778 735.68 m
180.778 731.174 l
S
n
172.263 731.174 m
172.263 735.68 l
S
n
117.906 730.61 m
117.906 731.174 l
S
n
123.238 730.063 m
123.238 731.174 l
S
n
128.57 730.61 m
128.57 731.174 l
S
n
133.886 730.063 m
133.886 731.174 l
S
n
139.219 730.61 m
139.219 731.174 l
S
n
144.551 730.063 m
144.551 731.174 l
S
n
149.883 730.61 m
149.883 731.174 l
S
n
155.216 730.063 m
155.216 731.174 l
S
n
160.531 730.61 m
160.531 731.174 l
S
n
165.864 730.063 m
165.864 731.174 l
S
n
171.195 730.61 m
171.195 731.174 l
S
n
176.528 730.063 m
176.528 731.174 l
S
n
181.844 730.61 m
181.844 731.174 l
S
n
187.177 730.063 m
187.177 731.174 l
S
n
117.906 731.174 m
192.509 731.174 l
S
n
116.791 731.174 m
117.906 731.174 l
S
n
117.341 735.567 m
117.906 735.567 l
S
n
116.791 739.977 m
117.906 739.977 l
S
n
117.341 744.371 m
117.906 744.371 l
S
n
116.791 748.78 m
117.906 748.78 l
S
n
117.341 753.174 m
117.906 753.174 l
S
n
116.791 757.567 m
117.906 757.567 l
S
n
117.341 761.977 m
117.906 761.977 l
S
n
116.791 766.371 m
117.906 766.371 l
S
n
117.341 770.764 m
117.906 770.764 l
S
n
116.791 775.174 m
117.906 775.174 l
S
n
117.341 779.567 m
117.906 779.567 l
S
n
116.791 783.977 m
117.906 783.977 l
S
n
117.906 731.174 m
117.906 785.731 l
S
109.523 731.229 m
/N121 9.60001 Tf
(0) show
105.149 748.896 m
(20) show
105.647 766.703 m
(40) show
133.914 721.258 m
(1.0) show
155.464 720.493 m
(2.0) show
176.695 720.914 m
(3.0) show
142.806 695.877 m
/N121 12 Tf
(48 mg/mL) show
n
129.204 639.511 8.515 -1.65802 re
f
0 J
n
129.204 639.511 m
137.718 639.511 l
137.718 637.853 l
129.204 637.853 l
129.204 639.511 l
[/DeviceCMYK] cs 0 0 0 0 sc
S
1 J
n
129.204 639.511 m
137.718 639.511 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
137.718 639.511 m
137.718 637.853 l
S
n
129.204 637.853 m
129.204 639.511 l
S
n
139.852 656.12 8.53101 -18.267 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
139.852 656.12 m
148.383 656.12 l
148.383 637.853 l
139.852 637.853 l
139.852 656.12 l
S
n
139.852 656.12 m
148.383 656.12 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
148.383 656.12 m
148.383 637.853 l
S
n
139.852 637.853 m
139.852 656.12 l
S
n
150.516 687.663 8.515 -49.81 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
150.516 687.663 m
159.031 687.663 l
159.031 637.853 l
150.516 637.853 l
150.516 687.663 l
S
n
150.516 687.663 m
159.031 687.663 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
159.031 687.663 m
159.031 637.853 l
S
n
150.516 637.853 m
150.516 687.663 l
S
n
161.164 652.788 8.533 -14.935 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
161.164 652.788 m
169.696 652.788 l
169.696 637.853 l
161.164 637.853 l
161.164 652.788 l
S
n
161.164 652.788 m
169.696 652.788 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
169.696 652.788 m
169.696 637.853 l
S
n
161.164 637.853 m
161.164 652.788 l
S
n
171.829 639.511 8.515 -1.65802 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
171.829 639.511 m
180.344 639.511 l
180.344 637.853 l
171.829 637.853 l
171.829 639.511 l
S
n
171.829 639.511 m
180.344 639.511 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
180.344 639.511 m
180.344 637.853 l
S
n
171.829 637.853 m
171.829 639.511 l
S
n
182.477 639.511 8.53101 -1.65802 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
182.477 639.511 m
191.008 639.511 l
191.008 637.853 l
182.477 637.853 l
182.477 639.511 l
S
n
182.477 639.511 m
191.008 639.511 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
191.008 639.511 m
191.008 637.853 l
S
n
182.477 637.853 m
182.477 639.511 l
S
n
117.472 637.29 m
117.472 637.853 l
S
n
122.804 636.743 m
122.804 637.853 l
S
n
128.137 637.29 m
128.137 637.853 l
S
n
133.453 636.743 m
133.453 637.853 l
S
n
138.785 637.29 m
138.785 637.853 l
S
n
144.118 636.743 m
144.118 637.853 l
S
n
149.45 637.29 m
149.45 637.853 l
S
n
154.782 636.743 m
154.782 637.853 l
S
n
160.097 637.29 m
160.097 637.853 l
S
n
165.43 636.743 m
165.43 637.853 l
S
n
170.763 637.29 m
170.763 637.853 l
S
n
176.095 636.743 m
176.095 637.853 l
S
n
181.41 637.29 m
181.41 637.853 l
S
n
186.743 636.743 m
186.743 637.853 l
S
n
192.076 637.29 m
192.076 637.853 l
S
n
117.472 637.853 m
192.076 637.853 l
S
n
116.357 637.853 m
117.472 637.853 l
S
n
116.907 642.247 m
117.472 642.247 l
S
n
116.357 646.656 m
117.472 646.656 l
S
n
116.907 651.05 m
117.472 651.05 l
S
n
116.357 655.46 m
117.472 655.46 l
S
n
116.907 659.854 m
117.472 659.854 l
S
n
116.357 664.247 m
117.472 664.247 l
S
n
116.907 668.657 m
117.472 668.657 l
S
n
116.357 673.05 m
117.472 673.05 l
S
n
116.907 677.444 m
117.472 677.444 l
S
n
116.357 681.853 m
117.472 681.853 l
S
n
116.907 686.247 m
117.472 686.247 l
S
n
116.357 690.657 m
117.472 690.657 l
S
n
117.472 637.853 m
117.472 692.411 l
S
109.54 638.024 m
/N121 9.60001 Tf
(0) show
105.339 655.824 m
(20) show
104.939 673.625 m
(40) show
104.739 690.424 m
(60) show
133.339 628.224 m
(1.0) show
155.14 627.624 m
(2.0) show
175.939 628.024 m
(3.0) show
144.405 606.44 m
/N121 12 Tf
(52 mg/mL) show
n
114.577 565.445 8.543 -5.68097 re
f
0 J
n
114.577 565.445 m
123.12 565.445 l
123.12 559.764 l
114.577 559.764 l
114.577 565.445 l
[/DeviceCMYK] cs 0 0 0 0 sc
S
1 J
n
114.577 565.445 m
123.12 565.445 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
123.12 565.445 m
123.12 559.764 l
S
n
114.577 559.764 m
114.577 565.445 l
S
n
125.256 579.639 8.52699 -19.875 re
f
n
125.256 579.639 m
133.783 579.639 l
133.783 559.764 l
125.256 559.764 l
125.256 579.639 l
[/DeviceCMYK] cs 0 0 0 0 sc
S
n
125.256 579.639 m
133.783 579.639 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
133.783 579.639 m
133.783 559.764 l
S
n
125.256 559.764 m
125.256 579.639 l
S
n
135.918 562.597 8.54401 -2.83301 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
135.918 562.597 m
144.462 562.597 l
144.462 559.764 l
135.918 559.764 l
135.918 562.597 l
S
n
135.918 562.597 m
144.462 562.597 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
144.462 562.597 m
144.462 559.764 l
S
n
135.918 559.764 m
135.918 562.597 l
S
n
146.598 596.667 8.52699 -36.903 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
146.598 596.667 m
155.125 596.667 l
155.125 559.764 l
146.598 559.764 l
146.598 596.667 l
S
n
146.598 596.667 m
155.125 596.667 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
155.125 596.667 m
155.125 559.764 l
S
n
146.598 559.764 m
146.598 596.667 l
S
n
157.261 576.791 8.543 -17.027 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
157.261 576.791 m
165.804 576.791 l
165.804 559.764 l
157.261 559.764 l
157.261 576.791 l
S
n
157.261 576.791 m
165.804 576.791 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
165.804 576.791 m
165.804 559.764 l
S
n
157.261 559.764 m
157.261 576.791 l
S
n
167.939 565.445 8.526 -5.68097 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
167.939 565.445 m
176.466 565.445 l
176.466 559.764 l
167.939 559.764 l
167.939 565.445 l
S
n
167.939 565.445 m
176.466 565.445 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
176.466 565.445 m
176.466 559.764 l
S
n
167.939 559.764 m
167.939 565.445 l
S
n
113.51 559.2 m
113.51 559.764 l
S
n
118.849 558.653 m
118.849 559.764 l
S
n
124.188 559.2 m
124.188 559.764 l
S
n
129.512 558.653 m
129.512 559.764 l
S
n
134.851 559.2 m
134.851 559.764 l
S
n
140.19 558.653 m
140.19 559.764 l
S
n
145.53 559.2 m
145.53 559.764 l
S
n
150.869 558.653 m
150.869 559.764 l
S
n
156.192 559.2 m
156.192 559.764 l
S
n
161.531 558.653 m
161.531 559.764 l
S
n
166.871 559.2 m
166.871 559.764 l
S
n
172.211 558.653 m
172.211 559.764 l
S
n
177.534 559.2 m
177.534 559.764 l
S
n
182.873 558.653 m
182.873 559.764 l
S
n
188.213 559.2 m
188.213 559.764 l
S
n
113.51 559.764 m
188.213 559.764 l
S
n
112.393 559.764 m
113.51 559.764 l
S
n
112.943 564.158 m
113.51 564.158 l
S
n
112.393 568.567 m
113.51 568.567 l
S
n
112.943 572.96 m
113.51 572.96 l
S
n
112.393 577.371 m
113.51 577.371 l
S
n
112.943 581.764 m
113.51 581.764 l
S
n
112.393 586.157 m
113.51 586.157 l
S
n
112.943 590.567 m
113.51 590.567 l
S
n
112.393 594.96 m
113.51 594.96 l
S
n
112.943 599.354 m
113.51 599.354 l
S
n
112.393 603.763 m
113.51 603.763 l
S
n
112.943 608.157 m
113.51 608.157 l
S
n
112.393 612.567 m
113.51 612.567 l
S
n
113.51 559.764 m
113.51 614.321 l
S
104.834 559.543 m
/N121 9.60001 Tf
(0) show
101.48 577.059 m
(20) show
101.253 594.721 m
(40) show
129.574 549.691 m
(1.0) show
150.595 550.126 m
(2.0) show
172.035 549.64 m
(3.0) show
146.076 514.211 m
/N121 12 Tf
(60 mg/mL) show
n
116.435 509.98 8.53101 -42.922 re
f
0 J
n
116.435 509.98 m
124.966 509.98 l
124.966 467.058 l
116.435 467.058 l
116.435 509.98 l
S
1 J
n
116.435 509.98 m
124.966 509.98 l
S
n
124.966 509.98 m
124.966 467.058 l
S
n
116.435 467.058 m
116.435 509.98 l
S
n
127.099 509.98 8.51601 -42.922 re
f
n
127.099 509.98 m
135.615 509.98 l
135.615 467.058 l
127.099 467.058 l
127.099 509.98 l
S
n
127.099 509.98 m
135.615 509.98 l
S
n
135.615 509.98 m
135.615 467.058 l
S
n
127.099 467.058 m
127.099 509.98 l
S
n
159.06 469.199 8.53101 -2.14102 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
159.06 469.199 m
167.591 469.199 l
167.591 467.058 l
159.06 467.058 l
159.06 469.199 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
159.06 469.199 m
167.591 469.199 l
S
n
167.591 469.199 m
167.591 467.058 l
S
n
159.06 467.058 m
159.06 469.199 l
S
n
115.369 466.496 m
115.369 467.058 l
S
n
120.701 465.949 m
120.701 467.058 l
S
n
126.033 466.496 m
126.033 467.058 l
S
n
131.349 465.949 m
131.349 467.058 l
S
n
136.681 466.496 m
136.681 467.058 l
S
n
142.013 465.949 m
142.013 467.058 l
S
n
147.345 466.496 m
147.345 467.058 l
S
n
152.677 465.949 m
152.677 467.058 l
S
n
157.994 466.496 m
157.994 467.058 l
S
n
163.326 465.949 m
163.326 467.058 l
S
n
168.658 466.496 m
168.658 467.058 l
S
n
173.99 465.949 m
173.99 467.058 l
S
n
179.306 466.496 m
179.306 467.058 l
S
n
184.638 465.949 m
184.638 467.058 l
S
n
189.97 466.496 m
189.97 467.058 l
S
n
115.369 467.058 m
189.97 467.058 l
S
n
114.253 467.058 m
115.369 467.058 l
S
n
114.802 471.453 m
115.369 471.453 l
S
n
114.253 475.861 m
115.369 475.861 l
S
n
114.802 480.255 m
115.369 480.255 l
S
n
114.253 484.666 m
115.369 484.666 l
S
n
114.802 489.059 m
115.369 489.059 l
S
n
114.253 493.452 m
115.369 493.452 l
S
n
114.802 497.862 m
115.369 497.862 l
S
n
114.253 502.255 m
115.369 502.255 l
S
n
114.802 506.649 m
115.369 506.649 l
S
n
114.253 511.058 m
115.369 511.058 l
S
n
114.802 515.452 m
115.369 515.452 l
S
n
114.253 519.862 m
115.369 519.862 l
S
n
115.369 467.058 m
115.369 521.616 l
S
106.652 466.612 m
/N121 9.60001 Tf
(0) show
102.643 484.791 m
(20) show
102.646 502.467 m
(40) show
102.63 520.147 m
(60) show
131.031 456.944 m
(1.0) show
152.984 456.967 m
(2.0) show
173.918 456.69 m
(3.0) show
247.737 696.595 m
/N121 12 Tf
(48 mg/mL) show
n
226.417 653.287 8.52901 -15.031 re
f
0 J
n
226.417 653.287 m
234.946 653.287 l
234.946 638.255 l
226.417 638.255 l
226.417 653.287 l
S
1 J
n
226.417 653.287 m
234.946 653.287 l
S
n
234.946 653.287 m
234.946 638.255 l
S
n
226.417 638.255 m
226.417 653.287 l
S
n
237.079 679.038 8.51401 -40.782 re
f
n
237.079 679.038 m
245.593 679.038 l
245.593 638.255 l
237.079 638.255 l
237.079 679.038 l
S
n
237.079 679.038 m
245.593 679.038 l
S
n
245.593 679.038 m
245.593 638.255 l
S
n
237.079 638.255 m
237.079 679.038 l
S
n
247.725 653.287 8.53 -15.031 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
247.725 653.287 m
256.255 653.287 l
256.255 638.255 l
247.725 638.255 l
247.725 653.287 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
247.725 653.287 m
256.255 653.287 l
S
n
256.255 653.287 m
256.255 638.255 l
S
n
247.725 638.255 m
247.725 653.287 l
S
n
258.388 653.287 8.51401 -15.031 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
258.388 653.287 m
266.901 653.287 l
266.901 638.255 l
258.388 638.255 l
258.388 653.287 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
258.388 653.287 m
266.901 653.287 l
S
n
266.901 653.287 m
266.901 638.255 l
S
n
258.388 638.255 m
258.388 653.287 l
S
n
269.033 640.396 8.53 -2.14099 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
269.033 640.396 m
277.563 640.396 l
277.563 638.255 l
269.033 638.255 l
269.033 640.396 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
269.033 640.396 m
277.563 640.396 l
S
n
277.563 640.396 m
277.563 638.255 l
S
n
269.033 638.255 m
269.033 640.396 l
S
n
225.35 637.693 m
225.35 638.255 l
S
n
230.681 637.146 m
230.681 638.255 l
S
n
236.013 637.693 m
236.013 638.255 l
S
n
241.327 637.146 m
241.327 638.255 l
S
n
246.659 637.693 m
246.659 638.255 l
S
n
251.99 637.146 m
251.99 638.255 l
S
n
257.321 637.693 m
257.321 638.255 l
S
n
262.653 637.146 m
262.653 638.255 l
S
n
267.968 637.693 m
267.968 638.255 l
S
n
273.299 637.146 m
273.299 638.255 l
S
n
278.63 637.693 m
278.63 638.255 l
S
n
283.962 637.146 m
283.962 638.255 l
S
n
289.276 637.693 m
289.276 638.255 l
S
n
294.606 637.146 m
294.606 638.255 l
S
n
299.938 637.693 m
299.938 638.255 l
S
n
225.35 638.255 m
299.938 638.255 l
S
n
224.235 638.255 m
225.35 638.255 l
S
n
224.784 642.649 m
225.35 642.649 l
S
n
224.235 647.059 m
225.35 647.059 l
S
n
224.784 651.453 m
225.35 651.453 l
S
n
224.235 655.862 m
225.35 655.862 l
S
n
224.784 660.255 m
225.35 660.255 l
S
n
224.235 664.649 m
225.35 664.649 l
S
n
224.784 669.059 m
225.35 669.059 l
S
n
224.235 673.453 m
225.35 673.453 l
S
n
224.784 677.846 m
225.35 677.846 l
S
n
224.235 682.256 m
225.35 682.256 l
S
n
224.784 686.649 m
225.35 686.649 l
S
n
224.235 691.059 m
225.35 691.059 l
S
n
225.35 638.255 m
225.35 692.813 l
S
216.719 638.016 m
/N121 9.60001 Tf
(0) show
213.319 656.415 m
(20) show
212.719 673.815 m
(40) show
212.919 691.615 m
(60) show
241.319 627.815 m
(1.0) show
263.119 628.215 m
(2.0) show
283.719 628.215 m
(3.0) show
248.337 782.728 m
/N121 12 Tf
(45 mg/mL) show
n
223.975 739.047 8.52901 -8.25702 re
f
0 J
n
223.975 739.047 m
232.504 739.047 l
232.504 730.79 l
223.975 730.79 l
223.975 739.047 l
S
1 J
n
223.975 739.047 m
232.504 739.047 l
S
n
232.504 739.047 m
232.504 730.79 l
S
n
223.975 730.79 m
223.975 739.047 l
S
n
234.637 741.782 8.51401 -10.992 re
f
n
234.637 741.782 m
243.15 741.782 l
243.15 730.79 l
234.637 730.79 l
234.637 741.782 l
S
n
234.637 741.782 m
243.15 741.782 l
S
n
243.15 741.782 m
243.15 730.79 l
S
n
234.637 730.79 m
234.637 741.782 l
S
n
245.283 750.038 8.53 -19.248 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
245.283 750.038 m
253.813 750.038 l
253.813 730.79 l
245.283 730.79 l
245.283 750.038 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
245.283 750.038 m
253.813 750.038 l
S
n
253.813 750.038 m
253.813 730.79 l
S
n
245.283 730.79 m
245.283 750.038 l
S
n
255.946 761.047 8.515 -30.257 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
255.946 761.047 m
264.461 761.047 l
264.461 730.79 l
255.946 730.79 l
255.946 761.047 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
255.946 761.047 m
264.461 761.047 l
S
n
264.461 761.047 m
264.461 730.79 l
S
n
255.946 730.79 m
255.946 761.047 l
S
n
266.592 741.782 8.53101 -10.992 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
266.592 741.782 m
275.123 741.782 l
275.123 730.79 l
266.592 730.79 l
266.592 741.782 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
266.592 741.782 m
275.123 741.782 l
S
n
275.123 741.782 m
275.123 730.79 l
S
n
266.592 730.79 m
266.592 741.782 l
S
n
277.256 736.294 8.51401 -5.50397 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
277.256 736.294 m
285.77 736.294 l
285.77 730.79 l
277.256 730.79 l
277.256 736.294 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
277.256 736.294 m
285.77 736.294 l
S
n
285.77 736.294 m
285.77 730.79 l
S
n
277.256 730.79 m
277.256 736.294 l
S
n
287.902 733.543 8.52899 -2.75299 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
287.902 733.543 m
296.432 733.543 l
296.432 730.79 l
287.902 730.79 l
287.902 733.543 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
287.902 733.543 m
296.432 733.543 l
S
n
296.432 733.543 m
296.432 730.79 l
S
n
287.902 730.79 m
287.902 733.543 l
S
n
222.908 730.228 m
222.908 730.79 l
S
n
228.24 729.681 m
228.24 730.79 l
S
n
233.57 730.228 m
233.57 730.79 l
S
n
238.886 729.681 m
238.886 730.79 l
S
n
244.217 730.228 m
244.217 730.79 l
S
n
249.549 729.681 m
249.549 730.79 l
S
n
254.879 730.228 m
254.879 730.79 l
S
n
260.211 729.681 m
260.211 730.79 l
S
n
265.527 730.228 m
265.527 730.79 l
S
n
270.857 729.681 m
270.857 730.79 l
S
n
276.189 730.228 m
276.189 730.79 l
S
n
281.521 729.681 m
281.521 730.79 l
S
n
286.835 730.228 m
286.835 730.79 l
S
n
292.166 729.681 m
292.166 730.79 l
S
n
297.498 730.228 m
297.498 730.79 l
S
n
222.908 730.79 m
297.498 730.79 l
S
n
221.794 730.79 m
222.908 730.79 l
S
n
222.344 735.185 m
222.908 735.185 l
S
n
221.794 739.594 m
222.908 739.594 l
S
n
222.344 743.987 m
222.908 743.987 l
S
n
221.794 748.397 m
222.908 748.397 l
S
n
222.344 752.791 m
222.908 752.791 l
S
n
221.794 757.185 m
222.908 757.185 l
S
n
222.344 761.595 m
222.908 761.595 l
S
n
221.794 765.987 m
222.908 765.987 l
S
n
222.344 770.381 m
222.908 770.381 l
S
n
221.794 774.79 m
222.908 774.79 l
S
n
222.344 779.185 m
222.908 779.185 l
S
n
221.794 783.595 m
222.908 783.595 l
S
n
222.908 730.79 m
222.908 785.348 l
S
214.46 731.129 m
/N121 9.60001 Tf
(0) show
210.172 748.182 m
(20) show
210.264 765.943 m
(40) show
238.719 720.104 m
(1.0) show
260.484 720.719 m
(2.0) show
281.637 721.188 m
(3.0) show
0 J
1 J
n
226.33 594.715 8.56799 -34.019 re
f
0 J
n
226.33 594.715 m
234.898 594.715 l
234.898 560.696 l
226.33 560.696 l
226.33 594.715 l
S
1 J
n
226.33 594.715 m
234.898 594.715 l
S
n
234.898 594.715 m
234.898 560.696 l
S
n
226.33 560.696 m
226.33 594.715 l
S
n
237.041 603.789 8.552 -43.093 re
f
n
237.041 603.789 m
245.593 603.789 l
245.593 560.696 l
237.041 560.696 l
237.041 603.789 l
S
n
237.041 603.789 m
245.593 603.789 l
S
n
245.593 603.789 m
245.593 560.696 l
S
n
237.041 560.696 m
237.041 603.789 l
S
n
247.734 567.506 8.56801 -6.81 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
247.734 567.506 m
256.303 567.506 l
256.303 560.696 l
247.734 560.696 l
247.734 567.506 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
247.734 567.506 m
256.303 567.506 l
S
n
256.303 567.506 m
256.303 560.696 l
S
n
247.734 560.696 m
247.734 567.506 l
S
n
258.444 565.226 8.55301 -4.52899 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
258.444 565.226 m
266.997 565.226 l
266.997 560.696 l
258.444 560.696 l
258.444 565.226 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
258.444 565.226 m
266.997 565.226 l
S
n
266.997 565.226 m
266.997 560.696 l
S
n
258.444 560.696 m
258.444 565.226 l
S
n
225.26 560.131 m
225.26 560.696 l
S
n
230.615 559.58 m
230.615 560.696 l
S
n
235.971 560.131 m
235.971 560.696 l
S
n
241.309 559.58 m
241.309 560.696 l
S
n
246.664 560.131 m
246.664 560.696 l
S
n
252.02 559.58 m
252.02 560.696 l
S
n
257.373 560.131 m
257.373 560.696 l
S
n
262.729 559.58 m
262.729 560.696 l
S
n
268.068 560.131 m
268.068 560.696 l
S
n
273.422 559.58 m
273.422 560.696 l
S
n
278.777 560.131 m
278.777 560.696 l
S
n
284.133 559.58 m
284.133 560.696 l
S
n
289.472 560.131 m
289.472 560.696 l
S
n
294.827 559.58 m
294.827 560.696 l
S
n
300.183 560.131 m
300.183 560.696 l
S
n
225.26 560.696 m
300.183 560.696 l
S
n
224.141 560.696 m
225.26 560.696 l
S
n
224.691 565.113 m
225.26 565.113 l
S
n
224.141 569.545 m
225.26 569.545 l
S
n
224.691 573.961 m
225.26 573.961 l
S
n
224.141 578.393 m
225.26 578.393 l
S
n
224.691 582.809 m
225.26 582.809 l
S
n
224.141 587.225 m
225.26 587.225 l
S
n
224.691 591.657 m
225.26 591.657 l
S
n
224.141 596.073 m
225.26 596.073 l
S
n
224.691 600.489 m
225.26 600.489 l
S
n
224.141 604.922 m
225.26 604.922 l
S
n
224.691 609.338 m
225.26 609.338 l
S
n
224.141 613.77 m
225.26 613.77 l
S
n
225.26 560.696 m
225.26 615.533 l
S
248.944 606.066 m
/N121 12 Tf
(51 mg/mL) show
215.133 560.672 m
/N121 [9.5993 -0.116898 0.116898 9.5993 0 0] Tf
(0) show
211.691 577.918 m
(20) show
212.207 595.59 m
(40) show
211.77 613.816 m
(60) show
241.391 549.704 m
(1.0) show
262.814 549.168 m
(2.0) show
283.767 548.988 m
(3.0) show
125.6 818.28 m
/N121 12 Tf
(folding) show
237.774 816.78 m
(unfolding) show
63.6073 616.461 m
/N121 [-0.0948944 11.9996 -11.9996 -0.0948944 0 0] Tf
(Probability /%) show
151.611 420.024 m
/N121 12 Tf
(Long-axis Length,) show
254.941 420.024 m
/N120 12 Tf
( L) show
265.605 420.024 m
/N121 12 Tf
( / ) show
275.607 420.024 m
Adobe_CoolType_Utility begin ct_MakeOCF begin ct_GlyphDirProcs begin
/BHBOWV+Arial-BoldMT 2
GetGlyphDirectory
541 <10bf3170232f916e74eb049388e9465c22dc244c49a7bec0bcc510272c82
8ebc475da1af4cf7762801f6b47dea3e870357a0ab23f4e9b96bf1d7c04b
bcf6bbc63f95f75217ff0180f366c481c9baac147871edbcc5aca78c1b37
bdb5bbc21d8595d7> |
80 <10bf31703bc84f280bc926798acdec2516269e7061028d385a31d255844f
a27fc6b4cdd6f6ba3dfabbbaadef207eca864f3bc97abd9a4f1b978df039
4779a47e3088a94b9cee6d3b276eef4d4950e88ef4a61f93e0b6cde961dc
7ec12956bd3a56a59704c6c5b5a401c3674bc856b6c34f276e7f1bc3056d
89b4805ca25b43894c427bc43b36554ede70476f7ee25d1a6c03ed9f5e40
5c72135defa96ede67a5a8ef5fea114c19a857db71952cb83f4d11> |
!
end end end
/N117 12 Tf
(\002\035\000P) show
Q
Q
q
108.862 334.922 133.546 25.3168 re
W
0.999985 0 0 0.999985 108.862 334.922 cm
0 w
q
Q
[/DeviceGray] cs 0 sc
0 11.9248 m
/N256 12 Tf
(Figure 2, Shew et al. )
[6.672 3.336 6 6 3.99591 5.32782 3 6 3 3 6.672 
6 5.32782 8.66382 3 5.32782 3.336 3 5.32782 3.336 3 3 
] pdfxs
Q
PDFVars/TermAll get exec end end
restore

%%EndDocument

LH
(%%[Page: 2]%%) = 
%%PageTrailer

%%Page: 3 3
%%PageBoundingBox: 12 13 598 780
%%EndPageComments
%%BeginPageSetup
/DeviceRGB dup setcolorspace /colspABC exch def
mysetup concat colspRefresh
%%EndPageSetup

%%BeginDocument: Pscript_Win_PassThrough

/pdfmark where {pop [ {ThisPage} 1 dict begin /BleedBox [  0 0 595.276 841.89 ] def currentdict end /PUT pdfmark } if

/pdfmark where {pop [ {ThisPage} 1 dict begin /TrimBox [  0 0 595.276 841.89 ] def currentdict end /PUT pdfmark } if

/pdfmark where {pop [ {ThisPage} 1 dict begin /ArtBox [  75.1685 584.505 369.158 775.399 ] def currentdict end /PUT pdfmark } if
PDFVars begin PDF begin PDFVars/InitAll get exec
save
8.362 -24.945 translate
0 0 595.276 841.89 true PDF begin PDFVars begin AS end end
userdict /pdf_svglb currentglobal put true setglobal

userdict /pdf_svglb get setglobal
%PDF_BeginEncoding: N37 (BHBOWV+Arial-BoldMT-Identity-H)
/N37 (BHBOWV+Arial-BoldMT-Identity-H) /Identity-H [ (BHBOWV+Arial-BoldMT) ]
 /Adobe-Identity [ /Serif ] 0 TZzero
userdict /pdf_svglb currentglobal put true setglobal
ct_T42Dict begin
end

userdict /pdf_svglb get setglobal
[/N80/LEEWGB+Arial-BoldItalicMT 1 TZG
userdict /pdf_svglb currentglobal put true setglobal
ct_T42Dict begin
end

userdict /pdf_svglb get setglobal
[/N96/ZYCIBP+Arial-BoldMT 1 TZG
0 0 595.276 841.89 re
W
n
q
q
n
0 841.89 595.276 -841.89 re
W
n
true setSA
n
122.219 717.469 8.864 -7.59698 re
[/DeviceCMYK] cs 0 0 0 1 sc
f
0.5 w
4 M
1 j
0 J
[] 0 d
n
122.219 717.469 m
131.083 717.469 l
131.083 709.873 l
122.219 709.873 l
122.219 717.469 l
[/DeviceCMYK] cs 0 0 0 0 sc
S
1 J
n
122.219 717.469 m
131.083 717.469 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
131.083 717.469 m
131.083 709.873 l
S
n
122.219 709.873 m
122.219 717.469 l
S
n
144.407 736.497 8.884 -26.624 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
1 w
n
144.407 736.497 m
153.291 736.497 l
153.291 709.873 l
144.407 709.873 l
144.407 736.497 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
0.5 w
n
144.407 736.497 m
153.291 736.497 l
S
n
153.291 736.497 m
153.291 709.873 l
S
n
144.407 709.873 m
144.407 736.497 l
S
n
155.502 766.919 8.883 -57.047 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
1 w
n
155.502 766.919 m
164.385 766.919 l
164.385 709.873 l
155.502 709.873 l
155.502 766.919 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
0.5 w
n
155.502 766.919 m
164.385 766.919 l
S
n
164.385 766.919 m
164.385 709.873 l
S
n
155.502 709.873 m
155.502 766.919 l
S
n
166.596 736.497 8.883 -26.624 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
1 w
n
166.596 736.497 m
175.479 736.497 l
175.479 709.873 l
166.596 709.873 l
166.596 736.497 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
0.5 w
n
166.596 736.497 m
175.479 736.497 l
S
n
175.479 736.497 m
175.479 709.873 l
S
n
166.596 709.873 m
166.596 736.497 l
S
n
177.69 725.084 8.883 -15.212 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
1 w
n
177.69 725.084 m
186.573 725.084 l
186.573 709.873 l
177.69 709.873 l
177.69 725.084 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
0.5 w
n
177.69 725.084 m
186.573 725.084 l
S
n
186.573 725.084 m
186.573 709.873 l
S
n
177.69 709.873 m
177.69 725.084 l
S
n
188.786 713.67 8.883 -3.79803 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
1 w
n
188.786 713.67 m
197.668 713.67 l
197.668 709.873 l
188.786 709.873 l
188.786 713.67 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
0.5 w
n
188.786 713.67 m
197.668 713.67 l
S
n
197.668 713.67 m
197.668 709.873 l
S
n
188.786 709.873 m
188.786 713.67 l
S
n
121.104 709.202 m
121.104 709.873 l
S
n
126.661 708.549 m
126.661 709.873 l
S
n
132.198 709.202 m
132.198 709.873 l
S
n
137.755 708.549 m
137.755 709.873 l
S
n
143.293 709.202 m
143.293 709.873 l
S
n
148.849 708.549 m
148.849 709.873 l
S
n
154.387 709.202 m
154.387 709.873 l
S
n
159.943 708.549 m
159.943 709.873 l
S
n
165.5 709.202 m
165.5 709.873 l
S
n
171.039 708.549 m
171.039 709.873 l
S
n
176.594 709.202 m
176.594 709.873 l
S
n
182.132 708.549 m
182.132 709.873 l
S
n
187.688 709.202 m
187.688 709.873 l
S
n
193.226 708.549 m
193.226 709.873 l
S
n
198.782 709.202 m
198.782 709.873 l
S
n
204.32 708.549 m
204.32 709.873 l
S
n
209.877 709.202 m
209.877 709.873 l
S
1 w
n
121.104 709.873 m
209.877 709.873 l
S
0.5 w
n
119.778 709.873 m
121.104 709.873 l
S
n
120.43 716.72 m
121.104 716.72 l
S
n
119.778 723.569 m
121.104 723.569 l
S
n
120.43 730.417 m
121.104 730.417 l
S
n
119.778 737.246 m
121.104 737.246 l
S
n
120.43 744.094 m
121.104 744.094 l
S
n
119.778 750.942 m
121.104 750.942 l
S
n
120.43 757.79 m
121.104 757.79 l
S
n
119.778 764.637 m
121.104 764.637 l
S
n
120.43 771.485 m
121.104 771.485 l
S
1 w
n
121.104 709.873 m
121.104 774.899 l
S
130.63 698.722 m
/N96 10 Tf
(1.0) show
153.091 698.923 m
(2.0) show
175.361 699.2 m
(3.0) show
110.745 709.786 m
(0) show
107.57 737.462 m
(20) show
108.05 764.333 m
(40) show
182.644 763.313 m
(50 mg / mL) show
182.644 751.313 m
(60 min) show
182.644 739.313 m
(folding) show
n
122.173 640.179 8.864 -10.263 re
f
0.5 w
0 J
n
122.173 640.179 m
131.038 640.179 l
131.038 629.916 l
122.173 629.916 l
122.173 640.179 l
S
1 J
n
122.173 640.179 m
131.038 640.179 l
S
n
131.038 640.179 m
131.038 629.916 l
S
n
122.173 629.916 m
122.173 640.179 l
S
n
133.267 674.399 8.883 -44.483 re
f
n
133.267 674.399 m
142.15 674.399 l
142.15 629.916 l
133.267 629.916 l
133.267 674.399 l
S
n
133.267 674.399 m
142.15 674.399 l
S
n
142.15 674.399 m
142.15 629.916 l
S
n
133.267 629.916 m
133.267 674.399 l
S
n
144.361 670.985 8.884 -41.069 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
1 w
n
144.361 670.985 m
153.245 670.985 l
153.245 629.916 l
144.361 629.916 l
144.361 670.985 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
0.5 w
n
144.361 670.985 m
153.245 670.985 l
S
n
153.245 670.985 m
153.245 629.916 l
S
n
144.361 629.916 m
144.361 670.985 l
S
n
155.457 667.571 8.883 -37.655 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
1 w
n
155.457 667.571 m
164.339 667.571 l
164.339 629.916 l
155.457 629.916 l
155.457 667.571 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
0.5 w
n
155.457 667.571 m
164.339 667.571 l
S
n
164.339 667.571 m
164.339 629.916 l
S
n
155.457 629.916 m
155.457 667.571 l
S
n
166.55 633.33 8.883 -3.414 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
1 w
n
166.55 633.33 m
175.433 633.33 l
175.433 629.916 l
166.55 629.916 l
166.55 633.33 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
0.5 w
n
166.55 633.33 m
175.433 633.33 l
S
n
175.433 633.33 m
175.433 629.916 l
S
n
166.55 629.916 m
166.55 633.33 l
S
n
121.058 629.244 m
121.058 629.916 l
S
n
126.615 628.593 m
126.615 629.916 l
S
n
132.152 629.244 m
132.152 629.916 l
S
n
137.709 628.593 m
137.709 629.916 l
S
n
143.248 629.244 m
143.248 629.916 l
S
n
148.803 628.593 m
148.803 629.916 l
S
n
154.341 629.244 m
154.341 629.916 l
S
n
159.897 628.593 m
159.897 629.916 l
S
n
165.454 629.244 m
165.454 629.916 l
S
n
170.993 628.593 m
170.993 629.916 l
S
n
176.548 629.244 m
176.548 629.916 l
S
n
182.086 628.593 m
182.086 629.916 l
S
n
187.642 629.244 m
187.642 629.916 l
S
n
193.18 628.593 m
193.18 629.916 l
S
n
198.736 629.244 m
198.736 629.916 l
S
n
204.274 628.593 m
204.274 629.916 l
S
n
209.832 629.244 m
209.832 629.916 l
S
1 w
n
121.058 629.916 m
209.832 629.916 l
S
0.5 w
n
119.732 629.916 m
121.058 629.916 l
S
n
120.384 636.765 m
121.058 636.765 l
S
n
119.732 643.613 m
121.058 643.613 l
S
n
120.384 650.46 m
121.058 650.46 l
S
n
119.732 657.29 m
121.058 657.29 l
S
n
120.384 664.137 m
121.058 664.137 l
S
n
119.732 670.985 m
121.058 670.985 l
S
n
120.384 677.834 m
121.058 677.834 l
S
n
119.732 684.681 m
121.058 684.681 l
S
1 w
n
121.058 629.916 m
121.058 694.943 l
S
130.468 619.39 m
(1.0) show
152.569 619.006 m
(2.0) show
174.962 619.087 m
(3.0) show
107.477 685.189 m
(40) show
107.778 657.607 m
(20) show
110.991 630.094 m
(0) show
182.571 682.497 m
(50 mg / mL) show
182.571 670.497 m
(1000 min) show
182.571 658.497 m
(folding) show
n
256.621 687.029 8.86398 -57.202 re
f
0.5 w
0 J
n
256.621 687.029 m
265.485 687.029 l
265.485 629.827 l
256.621 629.827 l
256.621 687.029 l
S
1 J
n
256.621 687.029 m
265.485 687.029 l
S
n
265.485 687.029 m
265.485 629.827 l
S
n
256.621 629.827 m
256.621 687.029 l
S
n
267.714 690.04 8.883 -60.213 re
f
n
267.714 690.04 m
276.597 690.04 l
276.597 629.827 l
267.714 629.827 l
267.714 690.04 l
S
n
276.597 690.04 m
276.597 629.827 l
S
n
267.714 629.827 m
267.714 690.04 l
S
n
278.808 635.85 8.884 -6.02301 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
1 w
n
278.808 635.85 m
287.692 635.85 l
287.692 629.827 l
278.808 629.827 l
278.808 635.85 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
0.5 w
n
278.808 635.85 m
287.692 635.85 l
S
n
287.692 635.85 m
287.692 629.827 l
S
n
278.808 629.827 m
278.808 635.85 l
S
n
289.904 641.874 8.883 -12.047 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
1 w
n
289.904 641.874 m
298.787 641.874 l
298.787 629.827 l
289.904 629.827 l
289.904 641.874 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
0.5 w
n
289.904 641.874 m
298.787 641.874 l
S
n
298.787 641.874 m
298.787 629.827 l
S
n
289.904 629.827 m
289.904 641.874 l
S
n
255.505 629.157 m
255.505 629.827 l
S
n
261.062 628.502 m
261.062 629.827 l
S
n
266.599 629.157 m
266.599 629.827 l
S
n
272.157 628.502 m
272.157 629.827 l
S
n
277.695 629.157 m
277.695 629.827 l
S
n
283.25 628.502 m
283.25 629.827 l
S
n
288.789 629.157 m
288.789 629.827 l
S
n
294.344 628.502 m
294.344 629.827 l
S
n
299.9 629.157 m
299.9 629.827 l
S
n
305.439 628.502 m
305.439 629.827 l
S
n
310.996 629.157 m
310.996 629.827 l
S
n
316.533 628.502 m
316.533 629.827 l
S
n
322.09 629.157 m
322.09 629.827 l
S
n
327.627 628.502 m
327.627 629.827 l
S
n
333.184 629.157 m
333.184 629.827 l
S
n
338.723 628.502 m
338.723 629.827 l
S
n
344.279 629.157 m
344.279 629.827 l
S
1 w
n
255.505 629.827 m
344.279 629.827 l
S
0.5 w
n
254.179 629.827 m
255.505 629.827 l
S
n
254.832 636.598 m
255.505 636.598 l
S
n
254.179 643.37 m
255.505 643.37 l
S
n
254.832 650.141 m
255.505 650.141 l
S
n
254.179 656.932 m
255.505 656.932 l
S
n
254.832 663.704 m
255.505 663.704 l
S
n
254.179 670.473 m
255.505 670.473 l
S
n
254.832 677.246 m
255.505 677.246 l
S
n
254.179 684.016 m
255.505 684.016 l
S
1 w
n
255.505 629.827 m
255.505 694.854 l
S
265.17 618.815 m
(1.0) show
286.965 619.149 m
(2.0) show
309.57 619.114 m
(3.0) show
245.752 630.037 m
(0) show
242.033 656.985 m
(20) show
242.258 683.933 m
(40) show
317.102 683.074 m
(51 mg / mL) show
317.102 671.074 m
(1000 min) show
317.102 659.074 m
(unfolding) show
n
256.81 757.151 8.42798 -45.498 re
f
0.5 w
0 J
n
256.81 757.151 m
265.238 757.151 l
265.238 711.653 l
256.81 711.653 l
256.81 757.151 l
S
1 J
n
256.81 757.151 m
265.238 757.151 l
S
n
265.238 757.151 m
265.238 711.653 l
S
n
256.81 711.653 m
256.81 757.151 l
S
n
267.358 769.296 8.44601 -57.643 re
f
n
267.358 769.296 m
275.804 769.296 l
275.804 711.653 l
267.358 711.653 l
267.358 769.296 l
S
n
267.358 769.296 m
275.804 769.296 l
S
n
275.804 769.296 m
275.804 711.653 l
S
n
267.358 711.653 m
267.358 769.296 l
S
n
277.907 720.753 8.44598 -9.10004 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
1 w
n
277.907 720.753 m
286.353 720.753 l
286.353 711.653 l
277.907 711.653 l
277.907 720.753 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
0.5 w
n
277.907 720.753 m
286.353 720.753 l
S
n
286.353 720.753 m
286.353 711.653 l
S
n
277.907 711.653 m
277.907 720.753 l
S
n
288.455 717.726 8.44702 -6.07202 re
[/DeviceCMYK] cs 0 0 0 0 sc
f
1 w
n
288.455 717.726 m
296.902 717.726 l
296.902 711.653 l
288.455 711.653 l
288.455 717.726 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
0.5 w
n
288.455 717.726 m
296.902 717.726 l
S
n
296.902 717.726 m
296.902 711.653 l
S
n
288.455 711.653 m
288.455 717.726 l
S
0.75 w
n
255.75 711.015 m
255.75 711.653 l
S
n
261.033 710.396 m
261.033 711.653 l
S
n
266.298 711.015 m
266.298 711.653 l
S
n
271.582 710.396 m
271.582 711.653 l
S
n
276.846 711.015 m
276.846 711.653 l
S
n
282.13 710.396 m
282.13 711.653 l
S
n
287.395 711.015 m
287.395 711.653 l
S
n
292.678 710.396 m
292.678 711.653 l
S
n
297.961 711.015 m
297.961 711.653 l
S
n
303.227 710.396 m
303.227 711.653 l
S
n
308.512 711.015 m
308.512 711.653 l
S
n
313.775 710.396 m
313.775 711.653 l
S
n
319.059 711.015 m
319.059 711.653 l
S
n
324.324 710.396 m
324.324 711.653 l
S
n
329.607 711.015 m
329.607 711.653 l
S
n
334.873 710.396 m
334.873 711.653 l
S
n
340.156 711.015 m
340.156 711.653 l
S
1 w
n
255.75 711.653 m
340.156 711.653 l
S
0.75 w
n
254.488 711.653 m
255.75 711.653 l
S
n
255.109 717.562 m
255.75 717.562 l
S
n
254.488 723.489 m
255.75 723.489 l
S
n
255.109 729.397 m
255.75 729.397 l
S
n
254.488 735.323 m
255.75 735.323 l
S
n
255.109 741.231 m
255.75 741.231 l
S
n
254.488 747.14 m
255.75 747.14 l
S
n
255.109 753.067 m
255.75 753.067 l
S
n
254.488 758.976 m
255.75 758.976 l
S
n
255.109 764.901 m
255.75 764.901 l
S
n
254.488 770.81 m
255.75 770.81 l
S
1 w
n
255.75 711.653 m
255.75 773.473 l
S
264.627 700.791 m
(1.0) show
285.089 701.124 m
(2.0) show
306.693 701.089 m
(3.0) show
245.543 712.013 m
(0) show
242.156 735.294 m
(20) show
242.048 759.576 m
(40) show
314.141 765.549 m
(51 mg / mL) show
314.141 753.549 m
(60 min) show
314.141 741.549 m
(unfolding) show
86.0917 675.964 m
/N96 [-0.0948944 11.9996 -11.9996 -0.0948944 0 0] Tf
(Probability /%) show
165.096 589.023 m
/N96 12 Tf
(Long-axis Length,) show
268.426 589.023 m
/N80 12 Tf
( L) show
279.09 589.023 m
/N96 12 Tf
( / ) show
289.092 589.023 m
/N37 12 Tf
(\002\035\000P) show
Q
Q
q
101.9 491.253 134.179 20.2534 re
W
0.999985 0 0 0.999985 101.9 491.253 cm
0 w
q
Q
[/DeviceGray] cs 0 sc
0 6.8615 m
/N256 12 Tf
(Figure 3, Shew et  al)
[6.672 3.336 6 6 3.99591 5.32782 3 6 3 3 6.672 
6 5.32782 8.66382 3 5.32782 3.336 3 3 5.32782 3.336 ] pdfxs
Q
PDFVars/TermAll get exec end end
restore

%%EndDocument

LH
(%%[Page: 3]%%) = 
%%PageTrailer

%%Page: 4 4
%%PageBoundingBox: 12 13 598 780
%%EndPageComments
%%BeginPageSetup
/DeviceRGB dup setcolorspace /colspABC exch def
mysetup concat colspRefresh
%%EndPageSetup

%%BeginDocument: Pscript_Win_PassThrough

/pdfmark where {pop [ {ThisPage} 1 dict begin /BleedBox [  0 0 595 842 ] def currentdict end /PUT pdfmark } if

/pdfmark where {pop [ {ThisPage} 1 dict begin /TrimBox [  0 0 595 842 ] def currentdict end /PUT pdfmark } if

/pdfmark where {pop [ {ThisPage} 1 dict begin /ArtBox [  20.62939 590.858 340.55499 815.62801 ] def currentdict end /PUT pdfmark } if
PDFVars begin PDF begin PDFVars/InitAll get exec
save
8.5 -25 translate
0 0 595 842 true PDF begin PDFVars begin AS end end
userdict /pdf_svglb currentglobal put true setglobal
ct_T42Dict begin
-0.566 -0.305 2 1.004
 256 array 0 1 255 {1 index exch /.notdef put} for  /BAAAAA+TimesNewRoman
Type42DictBegin
[<00010000000a000a000a000a63767420f32cda81000000ac000007c66670
676dc3a61d010000087400000631676c79666cfa85710000528c00011a48
68656164e1088b5600000ea8000000366868656112ef12f600000ee00000
0024686d7478b14216ca00000f0400001a286c6f636106c264360000292c
00001a2c6d6178700d0110ae000043580000002070726570e43894a40000
437800000f1367646972000000000000000000000000058e0000054c001f
054c001c0394001b0000ffe10000ffe40000ffe8fe4afffc056b0023fe6a
ffe00313000000ad000000ad0000000000250096009f002400f0013100c2
00c0004a00a6004100500094004700cf00af000e007901cb000400230044
00a80025011f0002004600170105009900d9005c007200e500e00028004b
00de011200240045007000160039ffe90016004b0088ffb900d9000a0043
00ae00ba016c0153002f00430048022c012b0025008fffc000170028ffcd
ffd80025009d00e50124ffb10048009d00e600110027007f00910012006a
00cafffc00000024006200a7017c01e900210060008b0434048aff6b003b
00b500d5014bff6b004d007905d809b5006c009100a3011701c0ffdfffe7
00be04010065007f00820088009900b200c0022e034305a000200026003d
004e00610065007b00d9011301310340ff27ff42ff99004e00a700f2022b
02c603070011002b0049005f008d00a100af00d600e400f5010b0135019d
01ab01ab01d101ee05d80000004b0075007a0080009d00a600a700ac00b9
013101310217021700020017002900550080008f00a500b200b300d0014b
015901c001c103a50530fe3fff14ff15ffe7ffff002a00580099009f00c1
00e400f40130015901ab01ab03220374041e04740532fd81004d0064009c
00d000d100d600de00e500f500f8012a012a01e1027e027fff57ffa8ffe5
00000008001f00380051005a006f0076007700a200c000c200c400f101fb
0209027e02cf04c5057a05f0ff92001200260042004b004f005100530064
008b00ae00b200b800b800d600f50111012001310138014e01520167018f
019601b801d901d902060221027102ea03b003cb03dc04360505ff3a0012
0016001e001f002300570068006c007e0088009200a500a800c500c90115
0126012d013001d601d901f6023b0244024402a302cf02de0385038f04fc
0586fee0feebfefbff8a0007004400470058007500aa00e400ef01160120
0129016a017301e3027e029002b4030e0310032303350341035403590388
039403c803ce047204ab04da0549056105ab0761fe6efed1ff4bff840000
00010006001e0027002c0034003700620066006a006b006c007000700072
007c0081008a008e0091009200a000ab00b800bf00c900d500dd00ec00f4
0100012101300169016a016d017c0185018e018e019901ac01c101c501c9
01e101f601f601f60222022202280236023f024302460267028502850294
02d002d602e8031c0363037f03800380039e03b603d90400040404ff0532
05320548058b05a706cb07280748076208ccfcedfd2afd59fddefe00fe1a
fe5bfe96fec1fee7ff56ff7900010025002d002e007c00870091009900a1
00a500a500aa00af00b600c600cc00d700dd00ec00f20102010501170118
0123012a012c0131013f014701490149014d01510151015501550157015a
015a0161016201680168017f0180018201830184018d0195019501950198
019901a501a901b601b601b701ba01ba01d501df01e601ea01f202000200
0203021702250227022f0239024302430247024f025202520267026f026f
027002720276027e02a702b302b902d603130325032d03610371039903ae
03c203d403f90402042c042f043c04560467048304cf04d104d804fb051f
05450568059e05c2061b06340655066a069806af06e806fc070607500762
077c07d407ff082500ad00c700aa00b5000000000000000000000000002f
06cf01730514047802df009c0018037005870155002500060254036c038e
03d2056601f0032001da018a0369036bffa3034602f8036f015602bf0122
031f053a0366008c00ff01ab02e102f402e70415015402e90128049101b7
026f034302060000000005d30415048305e8000002d7003a027d01c002c5
03830383ffbd003a059e01df059e02d1002004e0021300df01c001870297
000000ce0269028b0058043405fb0069015a01a905780182013e0288012a
03d4049e00e5032302f301f00196007a00cd014a0424025e023901ab00cf
00fd011e00ed017100700195004001bb01dd01b8000101a803a7014c020c
018d01b0020d0137010000cd032101d4030a005900000000012602150150
02f0025503bc06d00335010100d000d2007a01030130007c000000000000
000000fe006e006600940227002b0045004d00d3013200180097004100f4
febcffe9001605d8058b009100a1032c00520030005d02cb003a009200e5
00e500580086003200ba0099008800300298007cff8001640028004d0065
000200b8016a002f010b001100170100007f00040016022200a6005f0000
00f8000a00ca0043004b01ee0077012000f401c00028045f0000008c0445
00c20060007b008b008b0064005d00c2009c009206b505d3004f01170000
0420fe9e00cc00dc005e004600e30032001a003c0091005a00a1042c0041
002000490071009c009cfe4800400040008600cb0102007d003a003e006a
0050044800290096ff6a0097006900e0004c001b00c90069ff970043ffbd
0052ff83ff8b005fffa1ff5c00670053ffa8002a0076ffb2003600870559
0256052b043400de00c901c4004800db018b00b3004800da011601250118
00ea00ea00ae0000003e05bb008a04d70053003fff8cffd5001500280022
00990062004a00e4006d00ee00e5004803c00033fe4e02b1ff4603700079
05df0051ffa7ff1f010a0068ff6c004f00bc00a5070500ab0080001e05a5
0025042340425554403f3e3d3c3b3a393837363534333231302f2e2d2c2b
2a292827262524232221201f1e1d1c1b1a1918171614131211100f0e0d0c
0b0a090807060504030201002c4523466020b02660b004262348482d2c45
2346236120b02661b004262348482d2c45234660b0206120b04660b00426
2348482d2c4523462361b0206020b02661b02061b004262348482d2c4523
4660b0406120b06660b004262348482d2c4523462361b0406020b02661b0
4061b004262348482d2c0110203c003c2d2c20452320b0cd442320b8015a
51582320b08d44235920b0ed51582320b04d44235920b09051582320b00d
44235921212d2c20204518684420b001602045b04676688a4560442d2c01
b10b0a432343650a2d2c00b10a0b4323430b2d2c00b0172370b101173e01
b0172370b10217453ab10200080d2d2c45b01a234445b01923442d2c2045
b00325456164b050515845441b2121592d2cb00143632362b0002342b00f
2b2d2c2045b0004360442d2c01b00643b00743650a2d2c2069b04061b000
8b20b12cc08a8cb8100062602b0c642364615c58b00361592d2c45b0112b
b0172344b0177ae4182d2c45b0112bb01723442d2cb01243588745b0112b
b0172344b0177ae41b038a45186920b01723448a8a8720b0a05158b0112b
b0172344b0177ae41b21b0177ae45959182d2cb0022546608a46b040618c
482d2c4b53205c58b002855958b00185592d2c20b0032545b019234445b0
1a23444565234520b00325606a20b009234223688a6a606120b01a8ab000
527921b21a1a40b9ffe0001a45208a54582321b03f1b235961441cb11400
8a5279b31940201945208a54582321b03f1b235961442d2cb11011432343
0b2d2cb10e0f4323430b2d2cb10c0d4323430b2d2cb10c0d432343650b2d
2cb10e0f432343650b2d2cb11011432343650b2d2c4b525845441b212159
2d2c0120b003252349b04060b0206320b000525823b002253823b0022565
38008a63381b212121212159012d2c4bb06451584569b00943608a103a1b
212110592d2c01b005251023208af500b0016023edec2d2c01b005251023
208af500b0016123edec2d2c01b0062510f500edec2d2c20b00160011020
3c003c2d2c20b001610110203c003c2d2cb02b2bb02a2a2d2c00b00743b0
06430b2d2c3eb02a2a2d2c352d2c76b802b023701020b802b04520b00050
58b00161593a2f182d2c21210c6423648bb84000622d2c21b08051580c64
23648bb82000621bb200402f2b59b002602d2c21b0c051580c6423648bb8
1555621bb200802f2b59b002602d2c0c6423648bb84000626023212d2cb4
000100000015b00826b00826b00826b008260f10161345683ab001162d2c
b4000100000015b00826b00826b00826b008260f1016134568653ab00116
2d2c4b53234b515a5820458a60441b2121592d2c4b545820458a60441b21
21592d2c4b53234b515a58381b2121592d2c4b5458381b2121592d2c014b
53234b515ab00225b00425b006254923451869525a58b00225b00225b005
25462345696048592121212d2cb0134358031b02592d2cb0134358021b03
592d2c4b54b012435c5a58381b2121592d2cb012435c580cb00425b00425
060c6423646164b807085158b00425b00425012046b01060482046b01060
48590a21211b2121592d2cb012435c580cb00425b00425060c6423646164
b807085158b00425b00425012046b8fff060482046b8fff06048590a2121
1b2121592d2c4b53234b515a58b03a2b1b2121592d2c4b53234b515a58b0
3b2b1b2121592d2c4b53234b515ab012435c5a58381b2121592d2c0c8a03
4b54b00426024b545a8a8a0ab012435c5a58381b2121592d2c462346608a
8a462320468a608a61b8ff8062232010238ab9035803588a70456020b000
5058b00161b8ffba8b1bb0468c59b0106068013a2d2cb1020042b1230188
51b1400188535a58b910000020885458b202010243604259b12401885158
b920000040885458b2020202436042b12401885458b2022002436042004b
014b5258b2020802436042591bb940000080885458b202040243604259b9
4000008063b80100885458b202080243604259b94000010063b802008854
58b202100243604259b94000020063b80400885458b20240024360425959
5959592d2cb0024354584b53234b515a58381b2121591b21212121592d61
63750001000000030000ef56640f5f0f3cf50819080000000000a2e31dc2
00000000b9d5b528fb74fd8c1000080e0000000900010001000003740001
00000721fe4500571000fb74fe2610000001000000000000000000000000
0000068a0639011c00000000020000000200000002aa00e4034400850400
00250400006c06aa00480639004b0171005102aa005402aa002e04000091
048300250200006e02aa005302000091023900030400004a040000f00400
002c040000530400002004000062040000580400004c0400007c04000051
023900b00239008e048300250483002504830025038d005c075e006105c7
0010055600220556004a05c7002304e3002a0473002105c7004805c70023
02aa0033031d002a05c7002204e30029071d002205c7ffe505c700480473
002205c70048055600230473008004e3003e05c7000b05c70012078d001b
05c7000f05c7001304e3001a02aa00a80239000302aa004b03c100250400
ffef02aa0076038d00490400fffb038d004604000044038d004c02aa004f
0400003d0400000d0239003c0239ff63040000110239003d063900110400
000c040000450400fff90400004402aa000d031d00640239001404000002
0400001105c7000d0400001b0400000c038d002903d7011b019a00a103d7
00b10454001405c7000e05c7000e0556004a04e3002a05c7ffe505c70048
05c7000b038d0049038d0049038d0049038d0049038d0049038d0049038d
0046038d004c038d004c038d004c038d004c0239003c0239003c0239000d
023900020400000c04000045040000450400004504000045040000450400
00020400000204000002040000020400006503330062040000810400003d
0400009c02cd007003a0fff204000023061400450614004507d7001e02aa
00ec02aa003904640019071dffe805c7004905b400350464000804640018
0464001804000002049c008603f4004005b4002b0696002e0464003e0231
00000235fffa027b001d062500470556004904000027038d005902aa00e4
0483002404640053040000020464001e04e5001a04000040040000400800
00e605c7000e05c7000e05c70048071d004b05c700430400ffee0800ffed
038d0043038d004302aa00b902aa00c10464001703f4002f0400000c05c7
00130156feab0400ffe902aa007702aa007304730019047300170400008b
0200009102aa00c1038d00430800004105c7000e04e3002a05c7001004e3
002a04e3002a02aa003302aa003202aa003202aa003205c7004805c70048
05c7004805c7000b05c7000b05c7000b0239003c02aa003c02aa001602aa
001702aa003702aa00e902aa009602aa00bb02aa004e02aa009402aa003c
04e300160239001e0473007e031d006404e3001a038d0029019a00a105c7
00230400004405c700130400000c047300240400fff904830025048300a5
02660088026600140266002c06000086060000860600002a0400002105c7
00480400003d02aa003304730080031d00640556004a038d00460556004a
038d0046040000260400ffef02aa01ef05c70010038d004905c70010038d
004905c70023052c004405c7002304e3002a038d004c04e3002a038d004c
04e300290239003d04e300290340003c04e3002902c0003605c7ffe50400
000c05c7ffe50400000c05c70048040000450556002302aa000d05560023
02aa000d04730080031d006404e3003e0239001404e3003e036b001305c7
000b0400000205c7000b0400000204e3001a038d002904e3001a038d0029
04a0002505c7004c05d900470431005703c50046035c0047045000460337
000c049e00450400ffef049500e40285000207c0002c0800004f04000099
0800004f040000990800004f040000980400009807d5016a05c700c00483
002604cd00990483002604d5022204d5010505abffe905ab027e05ab027e
05abffe905ab027e05abffe905ab027e05abffe905abffe905abffe905ab
ffe905abffe905ab01c005ab027e05ab01c005ab01c005abffe905abffe9
05abffe905ab027e05ab01c005ab01c005abffe905abffe905abffe905ab
027e05ab01c005ab01c005abffe905abffe905abffe905abffe905abffe9
05abffe905abffe905abffe905abffe905abffe905abffe905abffe905ab
ffe905abffe905abffe905abffe905ab02d605ab006605abffea05d5ffff
04d500920800000007eb013007eb012007eb013007eb012004d500b204d5
008004d5002a082b0198086b01b807550010060000f40600006f0440003a
0540003704c0003f04150040040000250600005505ab002f046b003b04d5
000301c00089035500a206ab003403d5006404d5009202d6008302d60083
04d500b202d6007005c70010038d00490556004a038d00460556004a038d
004604e3002a038d004c04e3002a038d004c04e3002a038d004c05c70048
0400003d05c700480400003d05c700480400003d05c700230400000d05c7
00230400000d02aa00160239ffde02aa00170239ffdf02aa00330239fffe
02aa003302390039031d002a0239ff6305c70022040000110400001104e3
00290239003d05c7ffe50400000c059d002603f5000c05c7004804000045
05c70048040000450556002302aa000d04730080031d006404e3003b0239
001005c7000b0400000205c7000b0400000205c7000b0400000205c7000e
04000002078d001b05c7000d05c700130400000c0239001605c7000f038d
0049071dffe80556004905c7004904000027023900b2078d001b05c7000d
078d001b05c7000d078d001b05c7000d05c700130400000c02aa00b802aa
ffdb0400003d04cd005a060000860600002a060000310600002502aa00c3
02aa00bb02aa00ec02aaffea05c70010058dff5c0677ff5c034aff5c05c7
ffb60687ff5c05f2ffb30227ffb105c70010055600220525003204e3002a
04e3001a05c7002302aa003305c7002205cd001c071d002205c7ffe50525
004f05c7004805c700250473002204a8002004e3003e05c7001305c7000f
05e7001805f2003c02aa003205c7001304310057035c0047042f000b0227
002503f6fffa0412006e0389000003500046042f000b03d5005102270025
0408001503e10019044a0074039effd3039100460400004503fe0059032b
004603f6fffa038d00180502001c0544004b0227000003f6fffa04000045
03f6fffa0544004b04e3002a0604003704a000250548004b0473008002aa
003302aa0032031d002a06fa000d06fa002705ee00360556002505aa001a
05c7002505c70010049800240556002204a000250575001a04e3002a072b
00120402002b05c7002505c7002505560025056d0012071d002205c70023
05c7004805c70025047300220556004a04e3003e05aa001a0652004c05c7
000f05c700250533fffa081200390812003905a6003606fa002504980024
0548003a083900260556ffee038d00490412004e03c700300348001f0412
001a038d004c05870017032900180448002e0448002e03e3002e03fe000c
0510002e0448002e040000450448002e0400fff9038d0046037f000c0400
000c052f00570400001b0448002e0406001e0629002e0629002e0423000c
0560002d03a6002e036f001b05fa002d03aeffff038d004c03dd00110348
001f036f0046031d00640239003c023900020239ff6305d1000c05c9002d
0400000d03e3002e0400000c0448002e039a002502cf001f0800004107a2
0010040a000d02aa010102aa001c02aa003202aa001202aa010202aa008f
02aa008f02aa008f02aa009002aa010202aa001c02aa010202aa012102d9
005602aa008f025400e002be02af02beff6b023900b003da005f03a40033
02af0021035a004303c5004e023b0043024a004e03d0005803ce00430222
0043039e0043037600330374000f040f006403e2004e0232004302700021
03cd005f03a2004303a200430386005803dc004303ae003d03ca006903c0
004304e200430400002104750043045d00430444004301ac006b02f9006b
06360096023bff9d039e0043039e00430374ff5b0374ff5b03a2003304e2
004304e2004304e2004304e2004303da005f03da005f03da005f03a40033
02af0021035a004303c5004e023b00430279000c03ce004302220043039e
0043037600330374000f03e2004e0270002103cd005f03a2004303860058
03ae003d03ca006903c0004304e2004304000021023b004303a400330376
0033038600580404000f0000ffdc0000ff250000ffdc0000fe51028d00ab
028d00a002da0043034d007901a8ffba019c004601e50046019c0046019c
004601ad0048019c004601b10046015100460435017c0435012e043500b7
043500810435012c043500be043500af043500810435009a043500db0435
0085028d00c1043500b3060001000600010002420036060001000435009e
04350098043500cb060001000600010006000100060001000600010001b1
004606000100060001000600010006000100060001000600010006000100
06000100051bffba06000100060001000600010005b5003a05b5003a01f4
ffba01f4ffba060001000600010006000100060001000481003604350036
043dffba043dffba03e9004a03e9004a067f0014077600140327ffba041e
ffba067f0014077600140327ffba041effba051b003204b5002406000100
060001000600010006000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
01cf003001b1004601b1004601b1004001b1004606000100060001000600
010006000100060001000600010006000100060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
01000400001b080000000600010006000100060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
0100028d007f028d005d0600010004ee0015034d007901a8000e01d6ffdc
01a8005601d60010037500320375003201a8002d01d60013051b003204b5
002401f4ffba01f4ffba01a8009301d6001305b5003a05b5003a01f4ffba
01f4ffba024200000300fff705b5003a05b5003a01f4ffba01f4ffba05b5
003a05b5003a01f4ffba01f4ffba0481003604350036043dffba043dffba
0481003604350036043dffba043dffba0481003604350036043dffba043d
ffba02b3005f02b3005f02b3005f02b3005f03e9004a03e9004a03e9004a
03e9004a0692003e0692003e043fffba043fffba0692003e0692003e043f
ffba043fffba08c9003e08c9003e06c5ffba06c5ffba08c9003e08c9003e
06c5ffba06c5ffba04a7ffba04a7ffba04a7ffba04a7ffba04a7ffba04a7
ffba04a7ffba04a7ffba045a002a039a00360435ffba0327ffba045a002a
039a00360435ffba0327ffba064f0027064f00270224ffba021affba04a7
004604a700460224ffba021affba04cf002d04cf002d0327ffba0327ffba
040d0047040d004701a8ffba01a8ffba02b4002302b400230327ffba0327
ffba043500450435004501f4ffba01f4ffba024200360300fff7039affba
0327ffba0375003203750032051b003204b50024051b003204b5002401f4
ffba01f4ffba045a004004ce0040045a002604ce0030045a005304ce0041
045a005304ce00410600010006000100019c0046019c0046060001000600
0100060001000151004601b10046060001000600010001ad004801e50046
06000100060001000600010001b1004601b1004601b1004601b1004601b1
004001cf003006000100019c0046019c0046060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
060001000600010006000100060001000600010006000100028d00ca028d
00c7028d00c6060001000600010006000100060001000600010006000100
060001000600010006000100060001000600010006000100060001000600
010006000100060001000600010006000100060001000600010006000100
0600010006000100060001000100ffba0800ffba1000ffba05c70048043b
00450635000b045600020000fdcc0000fc140000fd130000fe420000fce0
0000fdd40000fe620000fe2b0000fdb70000fc980000fd880000fc080000
fcfe0000feff0000ff030000fe9e041a00a206000088060000140000fe70
0000fdd40000fdf60000fd770000fe620000fdbb0000fbd80000fbd80000
fb740000fcfe0000fc8c0000fc460000fd270000fcb40000fca80000fcae
0000fc440000fe140000fe700000fd910000fc710000fdc30000fe470000
fe620000fcc30000fde10000fd870000fd4b0000fd970000fd4b0000fc8a
0000fc620000fc090000fbd70239003c05c70010038d004905c70010038d
004905c70010038d004905c70010038d004905c70010038d004905c70010
038d004905c70010038d004905c70010038d004905c70010038d004905c7
0010038d004905c70010038d004905c70010038d004904e3002a038d004c
04e3002a038d004c04e3002a038d004c04e3002a038d004c04e3002a038d
004c04e3002a038d004c04e3002a038d004c04e3002a038d004c02aa0033
0239003c02aa00330239003c05c700480400004505c700480400004505c7
00480400004505c700480400004505c700480400004505c7004804000045
05c700480400004505c70048043b004505c70048043b004505c70048043b
004505c70048043b004505c70048043b004505c7000b0400000205c7000b
040000020635000b045600020635000b045600020635000b045600020635
000b045600020635000b0456000205c700130400000c05c700130400000c
05c700130400000c05c70010038d004902aa00330239000605c700480400
004505c7000b0400000205c7000b0400000205c7000b0400000205c7000b
0400000205c7000b040000020000ff090000ff090000ff090000ff0904a0
00230348001f072b0012058700170556002503e3002e0556002503e3002e
05c700230448002e05c700130400000205c700130400000205c7000f0400
001b0533fffa0406001e053300250400000d05c7002b038d004c05c70048
0400004505b5003a01f4ffba0224ffba021affba04a7004601f4009e01f4
001001f4001b01f4001001f4006b01f4fff90227ffce01a8000f01a8fff5
02aa00a402aa00a401a8000e01a8005601a800560000ffcf01a8000f01d6
ffbf01a8fff501d6ffcd01a8001d01d6fff501a8009301d6001303750032
037500320375003203750032051b003204b5002405b5003a05b5003a01f4
ffba01f4ffba05b5003a05b5003a01f4ffba01f4ffba05b5003a05b5003a
01f4ffba01f4ffba05b5003a05b5003a01f4ffba01f4ffba05b5003a05b5
003a01f4ffba01f4ffba05b5003a05b5003a01f4ffba01f4ffba05b5003a
05b5003a01f4ffba01f4ffba0481003604350036043dffba043dffba0481
003604350036043dffba043dffba0481003604350036043dffba043dffba
0481003604350036043dffba043dffba0481003604350036043dffba043d
ffba0481003604350036043dffba043dffba02b3003202b3003202b3005f
02b3005f02b3005f02b3005f02b3003202b3003202b3005f02b3005f02b3
005f02b3005f02b3005f02b3005f02b3003802b3003802b3004902b30049
03e9004a03e9004a03e9004a03e9004a03e9004a03e9004a03e9004a03e9
004a03e9004a03e9004a03e9004a03e9004a03e9004a03e9004a03e9004a
03e9004a0692003e0692003e043fffba043fffba0692003e0692003e043f
ffba043fffba0692003e0692003e043fffba043fffba08c9003e08c9003e
06c5ffba06c5ffba08c9003e08c9003e06c5ffba06c5ffba04a7ffba04a7
ffba045a002a039a00360435ffba0327ffba064f0027064f0027064f0027
0224ffba021affba064f0027064f00270224ffba021affba064f0027064f
00270224ffba021affba064f0027064f00270224ffba021affba064f0027
064f00270224ffba021affba04a7004604a7004604a7004604a70046067f
0014077600140327ffba041effba067f0014077600140327ffba041effba
04cf002d04cf002d0327ffba0327ffba04cf002d04cf002d0327ffba0327
ffba04cf002d04cf002d0327ffba0327ffba067f0014077600140327ffba
041effba067f0014077600140327ffba041effba067f0014077600140327
ffba041effba067f0014077600140327ffba041effba067f001407760014
0327ffba041effba040d0047040d004701a8ffba01a8ffba040d0047040d
004701a8ffba01a8ffba040d0047040d004701a8ffba01a8ffba040d0047
040d004701a8ffba01a8ffba043500450435004501f4ffba01f4ffba0435
0045043500450435004504350045043500450435004501f4ffba01f4ffba
04350045043500450481003604350036043dffba043dffba024200360300
fff7031a001a031a001a031a001a03750032037500320375003203750032
037500320375003203750032037500320375003203750032037500320375
003203750032037500320375003203750032051bffba04b5ffba051b0032
04b5002401f4ffba01f4ffba0375003203750032051b003204b5002401f4
ffba01f4ffba051b003204b50024067f0045067f0045067f0045067f0045
01a800280000fe290000fea20000ff300000ff1d0000ff120000ff920000
fe7e08fc003208ad00320000ffb50000ffb60000feed0000ff640000fe7e
0000ff9f018d000002f6fffd0000fe820000ff1004cd00320000ff580000
ff580000ff640692003e0692003e043fffba043fffba08c9003e08c9003e
06c5ffba06c5ffba045a002a039a00360435ffba0327ffba034d007902b4
00230242003601f4ffba0290ffba01f4002f01f4003b01f4001201f400b1
01f4006d067f001407760014022200430000fee702bc000004440043045a
fff504cefff5045a005304ce0041045a005304ce0041045a005304ce0041
045a005304ce0041045a005304ce0041045a005304ce0041043500710435
00ad045a000f04ce000f0000000000000076000000760000007600000076
0000013000000228000003f60000062e0000083a00000a6e00000af20000
0b7600000bf800000dd000000ea000000f3e00000f9800000ff000001062
0000119400001278000014480000162600001738000018c400001a3e0000
1b3400001d4800001ece00001f5e0000202c0000214a000021ec0000231c
0000248c0000276e000029f600002d1a00002e9400003006000031d80000
338800003582000037bc000038de00003a3200003da800003ebe0000411a
00004354000044700000466a000047f200004a9200004d8c00004ee20000
50ea0000536c0000574200005b3a00005da000005eea00005f9200006014
000060be000061a6000061e200006238000066320000687600006ad40000
6da6000071860000740a000078a200007bd200007e88000080ca00008534
0000871000008bda00008f42000091ae0000947a000096d4000099040000
9dc80000a01e0000a2c20000a5f00000aa520000aeec0000b1aa0000b3a6
0000b49a0000b5080000b5fa0000b6b80000b7080000b73a0000b7860000
b7bc0000b7f80000b82e0000b8780000b8ae0000b8ee0000b9360000b976
0000b9a40000b9da0000ba060000ba3a0000ba760000bab80000baee0000
bb280000bb580000bb900000bbc80000bc040000bc3c0000bc6e0000bcac
0000bce80000bd260000bd600000bd960000bddc0000be200000bf7c0000
c0540000c24a0000c4b40000c71c0000c7780000c8140000c9b00000ccc8
0000ceca0000d1360000d18e0000d2240000d2240000d4400000d5e40000
d5e40000d6e60000d6e60000d6e60000d91c0000da9e0000da9e0000da9e
0000da9e0000da9e0000da9e0000dc340000dd220000dd220000e08c0000
e2ae0000e40a0000e4b20000e50a0000e50a0000e68c0000e68c0000e68c
0000e7240000e7c00000e8c20000e8fe0000e93c0000e9720000ebb20000
ef460000ef7e0000efb60000f0bc0000f0e20000f18e0000f2300000f314
0000f3140000f35e0000f3900000f3900000f4f60000f55a0000f5ba0000
f5ba0000f5ba0000f8540000f8a40000f8c60000f9da0000fcb20000fcfa
0000fd4e0000fd8c0000fdcc0000fdfc0000fe300000fe840000feca0000
fefc0000ff300000ff680000ff9a0000ffca0001001000010040000101ae
0001022a000102ec000102ec000102ec000102ec00010406000104dc0001
04dc000104dc00010546000105460001054600010584000105c2000105fa
00010644000106c80001080e00010a5200010a8200010ac400010c400001
0e3400010e3400010f560001100e0001112c0001125200011450000115e0
000117ce000117ce000117ce000117ce000117ce000117ce000117ce0001
17ce000117ce000117ce000117ce000117ce0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c0001180c0001180c0001180c0001180c0001
180c0001180c0001180c0001180c0001180c0001180c0001180c0001180c
0001180c0001180c0001180c00011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800011a4800011a480001
1a4800011a4800011a4800011a4800011a4800011a4800011a4800011a48
00011a4800011a4800011a4800011a4800011a4800010000068a00f2003c
0076000700020010002f0056000005ca0f1300030002ba0054ffc003e1b3
45453240b803e1b32b2e3240b803e1b2282932b9ffc003e1b21a1c32bd03
e102ac0027001fffc003dfb2161b32b9ffc003deb2424232b9ffc003deb2
363832b9ffc003deb32a2d32df410a03de00ef03de000203de03df002800
1fffc003dfb3282e32f0410d03df0001037e000f0101001f00a003dd00b0
03dd0002004003dab32426329fbf03cc000103ca03c90064001fffc003c9
b20d1132410a03c703b70012001f03b603b50064001fffc003b5b30e1132
004173038d000100c0038d00d0038d00e0038d00f0038d0004006f03a700
7f03a7008f03a700af03a70004000f03a7001f03a7002f03a7004f03a700
0403ab03ab00ef03a50001000f03a5002f03a5006f03a5008f03a5000400
5403aa0001006b03aa000103a8036a0022001f038c03940015001f038b03
930015001f03a40393001a001f03a20394001e001f03a10393001e001f03
9f0394001e001f039b0394001a001f039a0393001e001f03990394001600
1f039803940016001f03970393001b001f03960394001b001f0395039300
1b001f03760375001a001f03740375001a001f03a00373b21e1f10411e03
930020039300300393000300200394003003940040039400030000039400
010383036c001e001f03b1036c0032001f036d036c0032001fffc0037db2
212332b9ffc0037db3171932a0410a037d00b0037d00c0037d00d0037d00
04ffc0037cb2212332b9ffc0037cb3171932a0412d037c00b0037c00c003
7c00d0037c00040030037300400373000200000373001003730020037300
0300e0037300f00373000200b0037300c0037300d0037300030084037300
90037300a0037300030377036a0029001f0389036ab2281f40b80367b339
40323fbb0366000100400366b3191d328fbb0366000100400366b3090a32
40b80366b3090e3240b80366b3090f323fbb0365000100400365b3090c32
40b80365b31a1d3240b80365b3090e326b410e0363007b03630002001403
6300240363003403630044036300040363b2242f1fba034e006d0800400e
1f7f027f037f047f050430440112bf033200500800001f0012032d003c08
0040291f5f3c01376009700980090310092009300940095009056f037f03
8f03031f032f033f034f035f0305b8ffc0b2073a33b8ffc04047063a3390
0ba00bb00bc00bd00b05b006c006d006e006f00605200630064006500660
06700680069006a006099006900702600b700b800b03100b200b300b400b
500b051f0701a04185036200010000036200100362007003620090036200
0400f0035f00010020035e0020035f0030035f0040035e00040000035e00
00035f0010035f00d0035e00e0035f00050010030f0020030f0030030f00
d0030f00e0030f00050000030f0010030f0050030f0060030f0070030f00
d0030f00060000030f0010030f0020030f0030030f00e0030f00f0030f00
06030f00270000030e0030030e000200e0030e00f0030e0002030e004a00
e0030d00f0030d0002030d002700d002fc0001001002fc002002fc005002
fc000300d002fc00e002fc0002000002fc001002fc002002fc003002fc00
5002fc006002fc000600e002fc00f002fc0002002002fc003002fc004002
fc000302fc406127c02901b02901a02901902901403c3f413240223f4132
1212125f235f255f285fa5046f236f256f286fa5044f234f254f284fa504
3f233f253f283fa5042f232f252f282fa5041f231f251f281fa5048f4caf
4cbf4ccf4c045f4c6f4c7f4c0337b8ffc0b3b22b3032b8ffc0b3b2222532
b8ffc0b5b2191a32370f413b02af0001005f02af009f02af00df02af0003
001f02af002f02af003f02af006f02af000402af02af001f02ad002f02ad
003f02ad004f02ad005f02ad000500df02ad0001000f02ad001f02ad003f
02ad005f02ad009f02ad0005005f02ad00df02ad0002000f02ad001f02ad
003f02ad0003004002acb23a334f414a02ac005f02ac009f02ac0003002f
02ac003f02ac0002000f02ac003f02ac00af02ac000300b002ac00e002ac
0002004f02ac005f02ac00a002ac0003001f02ac002f02ac003f02ac0003
000f035a0001000f035a001f035a003f035a005f035a0070035a000500cf
035700df03570002000f0357001f03570070035700af03570004035a035a
0357035702ad02ad02ac02ac032c400d31151f0016160000001211081041
10020c004a000d01a8004a000d0198004a000d0189004a000d013f004a00
0d0124400e4a0df64a0dbe4a0d864a0d274a0dbe02280041000d01940041
000d0121400b410db4410d4f410d29410d411002170021000d0215002100
0d02060021000d01eb0021000d014e0021000d012c4014210df9210df321
0df1210d9d210d71210d3d210d4110021c001f000d0214001f000d020b00
1f000d0196001f000d014a001f000d0126400b1f0dc61f0d571f0d371f0d
410d019e0141000d00420141000d001e0141000d001b0141000d01f2b40f
440f0009bb01f20044000d0201b23c291fb80200b23c291fb801ffb23c41
1fb801feb23c471fb801fdb23c9e1fb801fab23c931fbc01f9010f010100
1f01f6b224e41f411501f401490401001f01f301490401001f01f1014900
ab001f01f001490067001f01a6003c0125001f01a4b23c811f411501a301
0f019a001f01a200220801001f01a100500401001f019f0149019a001f01
9d01490067001f019cb22c621fb8019bb22c791fbc019a002c0101001f01
97b22ce41fb80193b22c891fb80192b22c6c1fb8018fb2259e1fb8016ab2
3c2a1f4111016700240201001f0163002502ab001f014c010f019a001f01
480149006c001f0147b22c891fb80145b22c9e1fb80144b22c791fb80143
b223311fb80127b23c811fbc012300500101001f011fb223e41f4115011d
0023019a001f011c00230801001f011b00250801001f010e010f0401001f
010d00220401001f0108b223811fb80106b425e41ff73cbb0125001f00f5
010fb29e1fe3bc01490156001f00e20149b2ab1fd1b901490401b21fcf2c
b80125b61fce23bb1fc524b80156b21fc02cb80801b21fbf2cb80201b51f
b124e41fb0b901490201b61faf2c671fad23b80801b21fa523b80201400b
1f9f3c2d1f9b235a1f9925b80201b21f812cbc0401001f006d010f015640
0b1f592c3e1f4c3cab1f4625b80101b21f403cb80125400a1f3a23721f39
3cab1f38b80149b3ab1f3124b80401b21f3025b802abb61f2a24e41f2623
b80156b21f5537ba023500070175402c0774076207560751073b0733072d
0720071d071c071408120810080e080c080a080808060804080208000814
b8ffe0402b00000100140610000001000604000001000410000001001002
000001000200000001000002010802004a00b013034b024b534201b0124b
004b5442b0372b4bb807ff52b0382b4bb008505b58b101018e59b0382bb0
0288b801005458b801ffb101018e851bb0124358b90001012f858d1bb900
01017c858d5959014bb0c063004b6220b0f65323b8010a515ab005234218
0016763f183f123e113946443e113946443e113946443e113946443e1139
4660443e11394660442b2b2b2b2b2b2b2b2b2b2b182b2b2b2b2b2b2b2b2b
2b2b2b2b181db0964b5358b0aa1d59b0324b5358b0ff1d594bb04753205c
58b90271026f4544b90270026f45445958b9017a0271455258b90271017a
4459594bb04753205c58b9002202704544b9003c027045445958b901b300
22455258b9002201b34459594bb04c53205c58b9014900224544b1222245
445958b901c20149455258b9014901c24459594bb06753205c58b9002402
714544b90050027145445958b9021e0024455258b90024021e4459594bb8
020153205c58b9010f00224544b1222245445958b90c00010f455258b901
0f0c004459594bb01c53205c58b125254544b12c2545445958b137254552
58b125374459594bb0ab53205c58b125254544b1232545445958b9015900
25455258b9002501594459594bb8010153205c58b125254544b128254544
5958b902080025455258b9002502084459592b2b2b2b2b2b2b2b2b2b2b2b
2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b
2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b
2b2b2b2b2b65422b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b
2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b01b361dc646345652345
6023456560234560b08b766818b080622020b164dc4565234520b0032660
62636820b003266165b0dc236544b064234420b161634565234520b00326
6062636820b003266165b063236544b0612344b10063455458b163406544
b26140614523614459b3a67f434b456523456023456560234560b0897668
18b080622020b1437f4565234520b003266062636820b003266165b07f23
6544b043234420b1a64b4565234520b003266062636820b003266165b04b
236544b0a62344b1004b455458b14b406544b2a640a645236144594b5242
014b5058b108004259435c58b108004259b3020b0a124358601b21594216
10703eb0124358b93b21187e1bba040001a8000b2b59b00c2342b00d2342
b0124358b92d412d411bba04000400000b2b59b00e2342b00f2342b01243
58b9187e3b211bba01a80400000b2b59b0102342b0112342002b00184569
44456944456944456944737373747373737475752b737374747518456944
7373742b4bb021534bb046515a58b03cb03c45b040604459012b2b2b2b75
7575757575757543584010bf3ccf3c026f3c7f3c8f3c9f3caf3c05757559
43584012bf22cf22025f226f227f228f229f22af2206757559435c58b640
3c9f22ef220375592b2b0174747474454473737474757545447345447374
4544737475737373737300757575737575752b2b757575752b752b435841
220063032d00010003032d0013032d0023032d0033032d0053032d000500
c3032d00d3032d00e3032d00f3032d00040083032d0093032d00a3032d00
b3032d0004032d032d4518694474747575592b4358b900180332b3303532
38b80332b361663238b80332b3535a3238b80332b3454e3238b80332b33c
413218b80332b23f330a410f0332000100ba033200ca033200da033200ea
033200fa03320005033203324518694474752b2b2b2b2b2b597300732b01
2b7575002b2b2b74002b2b2b732b74012b002b2b017373737474732b2b00
732b2b002b2b2b017374732b012b2b012b2b2b2b2b2b2b2b2b2b2b2b2b2b
00017375007373004569440073730173742b2b2b2b2b732b00732b752b2b
732b2b2b2b2b2b2b2b2b2b0000>
[15785 11565 15133 15005 14781 ] AllocGlyphStorage
]def 
108 44 
PrepFor2015
Type42DictEnd
1 0 0 <0002011c0000051c050000030007004db10201bb02be0006000702bfb200
0504b802beb403000a0704b802beb5010019080605bf02be000200030129
0009016b015e00182b10f63cfd3c4e10f43c4dfd3c003f3cfd3c10fc3cfd
3c31302111211125211121011c0400fc2003c0fc400500fb002004c0>/BAAAAA+TimesNewRoman AddT42Char 
5 8116 213 <0001003c0000020703af00160120b1060243545840311412101006551512
10100655161415160705080818081d06550807181701021010065501020f
0f0655010c0d0d0655010cb8fff0b4101006550cb8fff6b40f0f06550cb8
fff0b70d0d06550c0c18171112392f2b2b2bcd2b2b2b1112002f332b1133
3fddcd103130012b2b1bb390180118b8ffc040193232347018af18f01803
201850180240185018601890180418b8ffc0b3383a3418b8ffc0b32d3034
18b8ffc0b323253418b8ffc04025191a340c291e074a2201291e064a2315
270d41141e15440d0716000707060a00010d01240cb8ffc04019363a3490
0c01500c01900cf00c02600c700c020cb217b2a3182b10f65d5d71722bed
3c103c003f3c3f3c1239f5edfc01f52b2b3130012b2b2b2b015d715d2b01
72590111141616331521353236363511342726262322072725017b1a3141
fe43432e1b09071e1a1c280e011403affd2056391c24241a3c550161952c
20190f247000>/BAAAAA+TimesNewRoman AddT42Char 
5 9296 223 <0001003c041e026f05690006004640147a007b0172047a057f0605020300
0f060106d502b8012d401404cf010404010f06010694021907089421545a
182b2b4ef44ded5d11392f002fedeced5d1139393130015d012303330537
3301b2b8be1f0111e51e041e014bd4d4>/BAAAAA+TimesNewRoman AddT42Char 

1 0 3 <> /BAAAAA+TimesNewRoman AddT42Char 
1 118 4 <000200e4ffe401c6056b000c00180068bb02aa00190009ffc04009363834
004040413408b8ffc040141e21340a1af80e673600402a3534a700b70002
01b80349b70d07030d40130b01b80335400d00000a04104016340a4004f8
1910f6edf4ed1112392fed003fed3f10e6313001712b2b2b2b002b014644
012303263534363332161514070332161514062322263534360168265806
432f2f41046e2e41412e2e41410167032a351a3f4c4c4b182bfc30412d2e
41412e2d4100>/BAAAAA+TimesNewRoman AddT42Char 
1 304 5 <00020085032302bc056b000d001a009cb7b819c819f70c030cb8fff8b323
25340cb8fff8b32d303401b8ffe8b32a353400b8ffc8401d2a353419182a
35341a382a3534f70c01070c170c020a1c850e67360d00b80154b307031a
0eb80154b2140300b80335b40d0d0a040eb8033540161a1a17110a6d04c3
176d00110111851b1c94216a7a182b2bf65dfdf6ed1112392fed1112392f
ed003ffd3c3ffd3c31302b01715d2b2b2b2b2b2b01720103272635343633
321615140703210326353436333216151407030240361602382e2b391339
fe623716352d2c3a1a36032301247919193f3a3a315563fedb01287a2c40
3a3b31278efed900>/BAAAAA+TimesNewRoman AddT42Char 
1 552 6 <00020025ffe403db056b001b001f015e405c080507121805171204120e17
06110f07100e171e0d1806110c0710180d1f0a1b06110b07101b0a050900
06110809000710190d180215130314170e16170e02151d0314180d1a0215
1b0a1c1b0a0314010009021504031400090a1b1bb8032740090009140000
090e1717b803274010180d1418180d15161619191a1a010102b803274017
031413131d1d1c1c040403b7071112121e1e1f1f050506b80327402d0710
0f0f0c0c0b0b080807060e0d0d0a0a09001718181b1b000a101111141415
3f0e8717ad0d87601870180218b8020d40170a871b09871bad003f020706
06030f0201025c2058a4182b10f6713c3c103c10f4ede410e4f65de4fdf4
f43c103c103c003f3c103c103c3f3c103c103c3f3c103c103c103c103c10
fd3c103c103c103c103c10f43c103c103c103c103c10fd3c103c103c103c
103c87052e2b7d10c4872e182b7d10c40f0f0f0f0f0f0f0f0f0f0f0f0f0f
0f0f3130015d171323353313213521133303211333033315230333152103
2313210313211321735dabbb45ff0001135b535b015161535faab946fffe
f05d515bfead5f6e015348feab1c01c75201575001c7fe3901c7fe3950fe
a952fe3901c7fe3902190157>/BAAAAA+TimesNewRoman AddT42Char 
1 1014 7 <0003006cff64039905be0025002c0035018fb11c37b80195405913693627
1a2f3788178c2f8930053a344b345f34662c79177619752c763079358905
961dad06ad07af14af15c133c635f905fa35130a19014008272605040421
352d19180420161532252d04352619050401131615180c270ebf01910015
0219000f000e019f00270163b40f0f0c0501bc01ac0004016300210199b4
22221f0d01bb018d00000015018db3af140114b80190401632e2a01c011c
1a003701203740376037e03704370e20b8032740090d0021602170210321
b80212b22ae209b801ea400c100020005f006f0004001936ba0195010100
182b4e10f45d4df4edf45d3cfd3c4e105d71f65d4dedf45ded10ed003f3c
10e4eded3f3c10fded10ede4111239123939111739123939011112391217
39111739b10602435458b90019fff0b309123426b8fff0400d0912340510
0912343510091234002b2b2b2b5931304379402a2e3128291d1e0a0b3031
2f3102062e1e326201280b2a6200311d2d62001e1f2e2d290a2762012827
0b0c00103c103c2b103c103c2b012b2b2a8181818100715d015d2b133316
161711262726353436373533151617161711232626271116161514060715
2335262627011106061514161336373636353426276c2c0b9695e14b35b7
aa4052381da3270d8b8bfc8fd1ba405ea2620162646158ad4b2838414f9d
014e89920e02488b6b4c6d7bb8135c5c050e073efed59f930efe04b0a77c
8ad2108080042328031a01d10c674e497ffc900d1823714042766c00>/BAAAAA+TimesNewRoman AddT42Char 
1 1582 8 <00050048ffc80663056b00030011002200310041014540232b002b0302a9
06a60ca910a925a62ca930b906b60cb910b925b62cb9300c9208030202b8
0327401401001401010001021f1500033e361b460a12460ab80159b60403
0400324623b80159401a3a462a2a0202010003010b27383efa3638502e01
102e402e022eb802de400d4207381ffa15380e1942545a182b4e10f44dfd
f6ed10f65d71fdf6ed003f3f103c103c10edfded103c3c10eded10ed0111
12393911123939872e2b7d10c43130184379407005413425302625254026
38262c253c251026212617161816191603060c251d253331361d0041243e
1d01392b361d003b293e1d011311151d0022051f1d011a0b151d001c091f
1d01352f321d013f26321d01372d3a1d003d283a1d00140f121d01200612
1d01160d1b1d001e081b1d00002b2b2b2b2b2b2b2b012b2b2b2b2b2b2b2b
2b2b2a2b2b2b2b2b2b2b2b2b81005d015d01012301213216151406232226
263534363617220615141716171633323736353427260132161615140623
22262635343636172207061514171633323736353427260570fc245903dc
fc558795a8764f844f508b46334f161124151f302232312003a9478d4daa
7449894f4f894730232d2e22302e24303021056bfa5d05a3e091aebe57ac
6969b1573878c08b49371e12344db4be4d33fd6e5aac67b1bb5aa76b69ae
56353646c3b347333749b2bc4b33>/BAAAAA+TimesNewRoman AddT42Char 
1 2106 9 <0003004bffe105fb056b0031003d004901594026004be04b02104b01060e
091b0b20160e1b20194106472a6f1b6f286f336f427a1b060432014bb8ff
c0b31416344bb8ffc0402c0e123429403327304b43276207601c60296032
653d7032743dda200c0c0d2b13063e3241291c0c0d022a0606b8014c4022
3e1c143e3e1c03042c2e2d302f0701331c2a062c2b3e1341090931980002
98010100b80351b43846230309b8027f400b1047cf1616100b31000201b8
0130b300452606bd01a1003e01c70019002902c6b71c3f1f4b17171a0db8
01834013191f2601268160350135bb3bb16f1f701f021fb8012d401b443c
5f196f197f198f199f19af19bf19cf19df19ef190a19194a4bb80183b321
545a182b2b4ef45d4dedf45dedf45ded7210fd4e456544e64d10f4ed10f4
ed10f6fd3c103c003f3c10ed10ed3fedf43c10ed10ed1217390112173987
0e2e2b7d10c401111239111239391112393910c93130015d2b2b00715d01
5d7271012115060602071616333236371706062322262706062322263534
363726263534373633321615140607161736353427262725363635342623
2206151416132626270606151416333236041501a45753b06e598c474560
142525a46d52a9647cc771a5c2aef02f227e627d779691b87f8ab01e1629
fe827c7b5942575922cd84663d78798a753f75036925073ffec28a68534b
491b8d86596a6e55b07a79f18168853dab5a468d676aa05fe2bcd2902e24
1b050b3b965c485e793a3179fd19b4a67b45a6616ba23200>/BAAAAA+TimesNewRoman AddT42Char 
1 2670 10 <000100510323011a056b000c0051401b0a0e801e67360b182a35340c382a
3534b80bc80bd80be80b040c00b80154b706030e17171a0900b80335400a
0c0c096d03800d54a4182b10f6ed392fed4e10456544e6003f4dfd3c3130
01722b2b2b130326353436333216151407039e3617342d2d3b1a36032301
287b2b403a3b302591fed900>/BAAAAA+TimesNewRoman AddT42Char 
1 2802 11 <00010054fe4a027c058e0013003a40239611a71102860c8911020a980911
009801130100000a09a80e22500601068014545e182b10f65dedfd3c3c10
3c003fed3fed3130005d015d01152627260235100037150606021514171e
02027c9765909c0132f67b9e4e211a4a7dfe6f254c6691018ad4013601ff
6e2a44ecfe96c5d6af8aa79a>/BAAAAA+TimesNewRoman AddT42Char 
1 2934 12 <0001002efe4a0256058e00130039402429042a08480503009801110a9809
13000101090aa80e222006300640060306801558a4182b10f65dedfd3c3c
103c003fed3fed3130015d13351617161215100007353636123534272e02
2e98658f9cfecff77b9f4d21194b7c05642a4b6692fe77d5fecafe016e25
45eb016bc5d5b08aa69a>/BAAAAA+TimesNewRoman AddT42Char 
1 3064 13 <0001009102500370058e005200ea408d1554850f5b36b90ebf1ab346b752
cf1ac346de1ad4460837053b0e380f3a1a3b2635373646335208141d1022
103c1441144214432c1b2c453d1b3d454e1b4e455f1b5f457918731c7343
79488818861c854389489818961c95439848aa18a61ca543ab49ca26ca37
205149433904324c344636041a2b27241d1710041f0a0d00273632040a2b
041f3f2e7c223cb801b7402312344f7c070000980dd515341fd5279836d5
3f3f204c304ccf4cd04c044c85536a7a182b10f65d3c10fdfdfdf4fded00
3ff4f4fd3ce4011112173911123939111217391112391112393911121739
3130005d01715d2b01262726353436333216151406073637363633321615
140607060716171616151406232226272627161716151406232227263534
363637060706070623222635343637363736372627262726353436333216
1601ee04182231241f2e3506372c444222212d42844d33344b794b2d1e1e
493e293d021524301b251e152e0c053b2c49251a1c223029291b603e3b36
4b7b1d2d2d1e214a6e041445446225343636322da14423324f262d1f253a
1d11161b0e1642271e2c2a49312b3943762b28371d152e30873332273052
16102e1c1937120c140d191b0f1a15212f1b2d2a7f00>/BAAAAA+TimesNewRoman AddT42Char 
1 3536 14 <00010025008d045b04c3000b009f401a2f022f0320082009042f00200520
062f0b6f006f0b0660060106410f035100070327000a0351000b00030327
0002035100000008032700090351b60b0b0060050105bd03510004000003
5100040327b70160080108bb060bb80327401a0560000100bb2002300240
027002d00205200201025c0c585e182b10f65d71f45d3cfd3ce45d002fed
e410e45d103c10f4ed10f4ed10f4fde45d3130005d015d25112135211133
11211521110217fe0e01f25001f4fe0c8d01f35201f1fe0f52fe0d00>/BAAAAA+TimesNewRoman AddT42Char 
1 3744 15 <0001006efeab019800c800170053402759025917c4160309176019d01903
0901000704040f081200b612400c0b043a0f151f1580150315b8012a400b
1f0f5f0f020f19189ca4182b4e10f45d4dfd5ded003fede4123901111217
393130015d01711335363635342726232207062322263534363332161514
066e67710907070b251214313a4b3642678ffeab2c228f50130d0914093a
333146735f67b100>/BAAAAA+TimesNewRoman AddT42Char 
1 3902 16 <000100530180025802170003003f40200205801d64367f050101000200b0
030300021001500160019001a001d0010601b80134b5008004545a182b10
f6fd5d3c103c002fed3c103c3130015d2b13211521530205fdfb02179700
>/BAAAAA+TimesNewRoman AddT42Char 
1 3992 17 <00010091ffe4016f00c2000b002b401c0040060b034009403a3509403f35
5f09019f09af090209850c6a7a182b10f671722b2bed003fed3130253216
15140623222635343601002f40412e2e4141c2412e2e41412e2f4000>/BAAAAA+TimesNewRoman AddT42Char 
1 4080 18 <00010003ffe4023e058e0003005240090005cb1f6736000101b80327400d
02031402020303000002010b00b8011f40142003300360037003a003e003
0603bb01ad02cb04b8016fb1df182b10f6edf45ded003f3c3f3c87052e2b
7d10c431302b01012301023efe155001eb058efa5605aa00>/BAAAAA+TimesNewRoman AddT42Char 
1 4194 19 <0002004affe803b705680010002400bab2610820b80106b2050515b80106
b20d0d1ab8010f4012091a002640260240266026a026e026042611b8010f
400e5f006f007f008f00a00005001925ba011e010100182b4e10f45d4ded
4e105d71f64ded003fed3fed31304379404c012423242224020602010301
020607251c1b1d1b1e1b030613260f250b2618191719020621041162001f
061a6201140e116200160c1a620124012062011b08206201121015620019
0a1562002b2b2b2b012b2b2b2b2a2b2b2b2a2b2a2a811334123736333217
16111402062322272637101716333236373611342726272623220706024a
8c745a609c7c9b88d362c2816dc445397136741e2e302439293a44354834
029ee8014f52419fc5feafecfeb695e5c1f7fee8b1956172ac0139e89b73
30213d53fe9c>/BAAAAA+TimesNewRoman AddT42Char 
1 4500 20 <000100f000000306056800160097401440186018a018e018040018401802
76008600020e411301690141000901a00022000301690141000801a00023
000001f8000f016900160141000001f2400e010f0f020902010509080c02
0300ba01f70003014940120e0e0f401135300f7f0f900fa00f040f1917ba
022401e400182b4e10f45d2b3c4d10ede4103c003f3c3f3c111239011139
00f5edfc01f52b2b3130005d01715d13253311141616171521353e023511
34272626232207f0014a21133c5cfe026038160a07251a254204c7a1fb87
72381e022525021d317a02dc942a201e1f00>/BAAAAA+TimesNewRoman AddT42Char 
1 4728 21 <0001002c000003ab0568001e0168408207180b3917181c3d3418401c3d34
19401c3d340f1e161629073c074907a9070640205b045a085b175a186b08
741174129c0b9d0e9911ac0bac0ec905c917c818d917d918e020f904f917
1515011d0419051b15191619171d180709170b180b1d3419471989178f20
0718190202171a190c19060d031902050618171615140713040db8016840
090940140c3f80090109b80333400c10051a8f19019f19af190219ba0333
0003018db301020c1eb8018d400d0006e24f135f136f137f130413b80107
4013400001001a002040208020036020a020022019bb01f90003000d0140
40145f026f027f028f02bf02cf02df02ef020802191fba018e010100182b
4e10f45d4de43ced4e105d71f65d4df45ded10ed003f3cedfd5d713c3ffd
71b10602435458b78f0901bf09cf0902005d71592be41112173911123901
111239390210b10602435458b47d198d1902005d590e3c8710057dc40ec4
31300171725d005d012b2b2b002b01032135000035342623220607233636
33321615140706070207213236363703ab5ffce0016101209e6e649f2625
19cf9ba5dd304aa6f93e01626c57461a0105fefb2501420198a981a67571
b9c6d4906767a2b5fef03810312d>/BAAAAA+TimesNewRoman AddT42Char 
1 5192 22 <00010053ffe8035605680032014cb9000affe0b20c3909b8ffc0403c0c39
4109450a460b4b2204cf09012929382940346034cf34e034f70a07003401
41097f237a2eaa24b924ba2ec92edf23df25db2eea22e9250c490829b801
8cb328281000b802e4b3d0300130b80334b5030510160116b8019fb51d40
2b2f341db80143b3100d2928bb01680014000902e3400b50208020029020
a0200220b80333b3b00c010cb80190400b502d802d02902da02d022db803
33b55f077f070207b802e5400a403401a034c034023400b8013eb74013bf
1302131933ba011e01e800182b4e10f45d4de4105d71f65ded5d71f45ded
5d71e410f43c003fed2bed723fed5ded12392fed3130437940362e2f1e26
0a0f04062221232124212521040605250e26260a2062012f042d62011e0f
206201210b2762010a092e063062011f0d1d62002b2b103c2b012b2b2b2b
2b2a81818181005d01715d7200712b2b1336363332171615140716161514
070621222635343633321716161716333236353427262726262323353e02
353426232207683ab184a35742ba7d807092feeb89632f21191a11781725
2a6697231a1f2b964e204f9f4881609b68044a89956a4f5a949e31b67bb0
81a844271d2c08053f060b9e6c4f4b381d28411e0a5e844f677fa600>/BAAAAA+TimesNewRoman AddT42Char 
1 5670 23 <00020020000003b90568000a000d00d74028160d010f00450d400f03400f
012a0c011507010206010309050601040c0b0d00040c0d04060c0d0db801
1c401207081407070808030407060c08001f0d010dbb019c0006000b019f
400d050106090806060805040c0c04bb0149000300080166400b09090f03
019f03af030203b801f74018013f0001001a000f01600fa00fe00f030f06
40070107190eba018e010100182b4e10f4713c105d71f65d3c4df45d713c
10e610fd3c003f3f392f103c103c10ed10fd723c1139113901111239872e
2b047d10c4011112390f0f0f313000725d015d7172011523112311213501
331123110103b9b6a5fdc202756ea5fe2401f48efe9a0166800382fc8c02
a1fd5f00>/BAAAAA+TimesNewRoman AddT42Char 
1 5944 24 <00010062ffe80379054c0021011e4043a4040112591e691e7f057f067f1d
8c048d1d07350235215503552057216b1c7605791c87028a1a8a1ca303a8
09a023e0230f0023010f1011121315161708140d020303b8011c40112021
1420030420211a1b1c030718040503b8019fb320202113ba01f900180313
400c0d0d01e20002e22121000400ba013e001b0147b58007a0070207b801
f5400a40230140236023022316b801f9b61002a021012103b8019f400920
4010a01002101922ba019501e900182b4e10e45d4d10ed105d3c10ed105d
71f65dede4003f3c10ed10ed3feded12392fed0111391112173987082e2b
057d10c40011121739b10602435458400d72017202722082018202822006
005d59313001715d005d435c58400b6b046f12641e7005701d055d59015d
010721070417161514060607062322263534363332161716333236353426
2726270103794efe685901099b8557845173797a6f2e231a272f4b4d75b1
9e8b6dbc0104054caab6279e88b86bb680273753321c2b102134b17f7bd5
3a2d07020f00>/BAAAAA+TimesNewRoman AddT42Char 
1 6340 25 <00020058ffe803b105680018002800fc402a7509760a770e8209d925e925
060603017d037a047a168517043c0828060503231928190603205f080108
b80143b620260126260f01b8018db318000520b80106b30f0d0100ba0140
0023010f40120b1a002a402a02402a602aa02ae02a042a19ba013e001b01
0f4012001310132013301340139013a01307131929ba011e010100182b4e
10fc5d4dfde44e105d71f64dedf43c003fed3f3ced12392f5ded72121739
0111121739b10602435458b40b061b0602005d5931304379402c1c250912
1d1c1e1c020611250d2625092362011f101b6200210e236201240a266201
1c12206200220c206200002b2b2b012b2b2b2b2b2a8181005d01715d0115
0e0307363332161514070623222726113412243633010615141617163332
36353426232206039684a7a36b2490918bcc677ccc8b61be92010ff86bfd
cc12474633495789887d26570568250d4fa2c78963e0b0aa8caa5cb3011d
b60148fe58fd44875360e1422fa498abfa20>/BAAAAA+TimesNewRoman AddT42Char 
1 6718 26 <0001004cffe403a5054c000b00c1b90004ffe0b3131b3e05b8ffe0402b13
1b3e19080105032a094200400d600da00dca01c902d801d802e00d0b1a00
010b01000d400d0302050404b80193401a03021403030204030d05404735
05e2010640473506e201000400b80199b6a00b010b190c05ba02e8000302
e7400c0004100440045004a0040504bc02e6000c011e010100182b10f65d
ede44e10f45d4df4003f3ced2b10ed2b3f3c87052e2b870e7dc4b1060243
54584009740574068405840604005d5931300171725d0072012b2b132115
012301212207060727ce02d7fe3c700195fe8b713054331d054c26fabe04
c51b2e600b00>/BAAAAA+TimesNewRoman AddT42Char 
1 6964 27 <0003007cffe8038a0568001900260033017a40ba59010109331f332a276f
337a22800b800c801a801b822580268a33a918a51aa725b30cb41ab726bb
27c50ac50bd70d1607000a01060d021a0927160d171a250d250e4b018c01
830d850ea9000e3b003a014b004b0149285f015b275c336a006a01690267
266a2768337b017c27762c7c338f048f0580078008821182128f148f1698
049608941196129b16a626ad27ad33b804b608e90bea0ce90ee927e93229
070d09273a0039013832054408000c1a2704000c1a2704101720b80106b2
06052db80106b2130d1d4109010f00090140000901400030010f00100166
4010003540350240356035a035e035043523bc010f0003013e002a010f40
0a30174017901703171934ba01ee01e900182b4e10f45d4dedf4ed105d71
f6ede4f4ed003fed3fed111217390117393130437940322b2f1e22111604
08152521052362001f071d62012c142a62002e1230620122042062011e08
2062012b162d62002f112d6200002b2b2b2b012b2b2b2b2b818181810171
5d00715d0072012626353436333216151406071617161514062322272635
343625363635342623220615141617130606151416333236353427260189
a15dcca9a4c86cabb0394cdab1c16c567901317840766666803531365350
8d6d6c82264702ab84a05684bfb2724c9e6b884e66718fcb7961735ab1d6
6c7d4f6977764f34682ffee746a560819b7a5748396a>/BAAAAA+TimesNewRoman AddT42Char 
1 7496 28 <00020051ffe403a8056800170027010c40337b27d905d722d92704680479
057d087a09770c780d791377208b0883130a09088f29023b080527182127
1805031e2504000705ba016300180140b42750070107b8014340092f256f
25022525001eb80106b20e0501b8018cb41717000d18ba013e001a010fb7
0012101220120312b8016540120029402980290340296029a029e0290429
01ba01400021010fb7400abf0a020a1928ba011e01e800182b4e10f45d4d
ede4105d71f65dfde4003f3c10ed3fed12392f5ded7210f4ed1112391112
1739011112393931304379402a1b2408110c2610251c2623261f0d216200
1d0f1a62012408216200200b1e62011b111e62012209256200002b2b2b01
2b2b2b2b2b2b2b818101715d005d17353636123706232226353437363332
1716151402070623013635342626232206151417163332366c82e0d1299d
7f8fcc667bc6a77792dec6a1be02331242794d598659415f2e7e1c250275
0124af65ddb7b28ba98aabfbe2fe79816a02b9824e61e178a09ed377562c
>/BAAAAA+TimesNewRoman AddT42Char 
1 7886 29 <000200b0ffe4019003b0000b00170042b10319b80125401d0d67369019a0
1902064000070c40120b0f4015034009349015a0150215bc0125001800d2
010000182b10f65df4ed10ed003fed3fed3130015d2b0132161514062322
2635343613321615140623222635343601212e41412e2e41412c2f41422e
2e414103b0412e2e41412e2e41fd13422e2e41412e2e4200>/BAAAAA+TimesNewRoman AddT42Char 
1 8030 30 <0002008efeab01b803b1000b00230063401b2125c1116736c60fc422020c
0d1b131510090cb6180c0640000714b8034e401f1e40180b03400f091f09
0209361b103a0f211f2180210321c81b19246a7a182b4e10f44dfd5ded10
f45ded003ffded3fed2f10e40111123939123939313001712b0132161514
062322263534360335363635342726232207062322263534363332161514
06011a2e41412e2e41415e67710907070b251214313a4b3642678f03b140
2e2e41412e2e40fafa2c228f50130d0914093a333146735f67b1>/BAAAAA+TimesNewRoman AddT42Char 
1 8236 31 <0001002700bb045b0494000600f3b73703011700180602b1060243545840
0b040008070140090d340105002f2f2b01111239391bb2040303b8032740
0b0605140603020605020303b803274009000114000304000106ba034200
000342b2032002410901440040000102d9000302d9002000040144402e40
05013f056f057f0580050405020101040005400502900501500560050260
058005024005700502000520050205ba0253000301f14016000f06d00602
5f068f06026f067f0602065c07585e182b10f45d5d713cedfc5d5d5d5d5d
713c3c103c002f5d71ed1a19fdfd1a18ed1a1910eded87082e182b047d10
c487082e182b047d10c45931300072015d13011501011501270434fc6203
9efbcc02c201d257fe6efe6a5a01d600>/BAAAAA+TimesNewRoman AddT42Char 
1 8522 32 <0002002501db045c037300030007007cb10607b80327b6054f045f040204
be034c00020003032700010000ff80403b3a35000080000250008000a000
d000e0000500060605050202100101d0010130014001a001030001100120
0103015c090704040303005c08585e182b10f63c103c103c10f65d5d7172
3c103c103c003f5d712b3cfd3cf65d3cfd3c313013211521152115212504
37fbc90437fbc9037352f452>/BAAAAA+TimesNewRoman AddT42Char 
1 8684 33 <0001002500bb0459049400060104400a18001706022b03390302b1060243
5458400b000408070540090d340501002f2f2b01111239391bb2040303b8
0327400b0605140603020605020303b803274009000114000304000100ba
034200060342b2032004410901440040000502d9000302d9002000020144
402b4001013f016f017f01800104010504020f014f01026f017f018f019f
01046f01010f012f014f015f010401ba0253000301f1402806000001c000
e00002400060009000a0000410002000300050000400007000800003005c
08585e182b10f65d5d5d5d713cedfc5d5d5d713c3c3c002f5d71ed1a19fd
fd1a18ed1a1910eded87082e182b047d10c487082e182b047d10c4593130
015d0072010135010135010459fbcc039ffc610434028dfe2e5601920196
5bfe2a00>/BAAAAA+TimesNewRoman AddT42Char 
1 8988 34 <0002005cffe5033b056b0022002e00e8b509080f300202b8ffe040383035
342f303f304f305f307c098b09a50ca51aa31b0926080c0d0e0310160305
211f04010f0e130a06050403100702032103262c7f130113b801b6b50a46
19030001b80352401b2340290b01680000262c07b1df1d010f1d011d8726
106d16e62c30b8016db72640202c302c022cbb020d002f00300137b3219c
5a182b2bf65dfde610f4ed10f47171ed1112392fed003ffdf63c3feded5d
0111121739111217390011123939111739011112173931304379401a171c
080c1b250b180d1d00091a071d010c170a1d01081c0a1d01002b2b012b2b
2b8181015d2b017101233636373636353426232206151416151406232226
3534363332171615140607060607321615140623222635343601c6290731
4d3c24876257643c2e212a45c2a6ce6148415b9141152f41422e2e414101
407ea59371793e7f965230256c1c2431534a71ae78586b499a68a489f441
2f2e41412e2f4100>/BAAAAA+TimesNewRoman AddT42Char 
1 9356 35 <00020061fe46072c058e0042005401dd406aa600a641ec41030019001c10
19151c5019551c76160701100028e800ea41e056f645045850a615a616d0
56042050205120525f1804210020012002204f0468006502671d87000479
008a00fb4103b1084142423342004f523142410200040b041a2a4f413302
04431b00b803424009103e013e6800430143b80342b7420f46260042071c
bb03420019001b0347b54c81361e4617b80351403607462e34360a526704
38313155560b462a3f1aad201b301b401b031b1a5639380f4980490249a8
133a20223022402250220422195556b801d9b3219c5e18b80137852b2b4e
f45d4dedfd5ded4e10f65d4dedf4ed1112392ffde5003ff4fdf4ed10fde6
10e53f3fed10f55dfd5de5111217390112391112173911123910c987100e
3c31304379403b444b373d053047484648454803063b3a3c3a02062c2609
25152620251125242628250d26443d4974004b37491d00062f041d00082d
0b7401161f13b80175b300181d1ab80175b7011c1b191a102513b8017540
1d000e270b7401483a4374014a384c1d000530071d000a2b077400142117
b80175b300191c17b80175b30012230fb80175b5010c290f7401002b2b2b
2b2b2b2b2b012b2b103c103c2b2b2b2b2b2b2b2b2b2b2b2b2b2b2a2a8181
8101715d5d5d5d5d3838005d710103060615141633323612353402242322
040215141204332000133302002122240235101200333204121514020623
222635343706062322263534123736333216173707220706070615141633
3236363736353426058075411c2b2049cd92a5fed3b6e7fe74e7cb0170d4
010701a9743a5afe26fed1eefe68e2f801bffbcf014daea3fc894c4d1294
b244476ebd9c735b43591021c24b4d71503b472c3a808c20384903befe71
e07824202c920148b2ab01229bf5fe34f8e6fe88c1011a010ffeeefeace1
019df8010801c90101abfeb7b9b7fe99a44841385bb36a7f6a9101687153
45456e134f74c590583f4f58b75c9f64424e>/BAAAAA+TimesNewRoman AddT42Char 
1 10094 36 <00020010000005b0056b001c001f0218b102024354584012011f1e021e1d
001c1e1c001d1f011e1c0214be03e2001703e2000703e2000a03e2401708
021c1e030f081c161d001f70018001020101080f0208002f3f12392f5dcd
d0cd2f2f1112173910ededeeec012f2f2f2f2f2f2f107d87c4c41087c4c4
31301b401b080e0f0f0d100a1e091f502106150f13101a111a1b1b1c181d
0621b8ffc0b2253521b8ffc0b330583421b8ffc0b32b2e3421b8ffc0b229
3521b8ffc0b320263421b8ffc0b31a1e3421b8ffc0b2173521b8ffc0b215
3521b8ffc040971013340d0f0b100a1e390f4a0f4610491e4f21590f5710
5514581e6a0f6710681e76108004870e8a0f87108712891e881f9b0f9b10
99119b1eb90fb910bd1ab91ecb0fca10c81dca1edb0fd810eb0fe810e81e
f90ff810f91df91e2c090f4b1b021f1e01011f1e02001d1e1e1c090e0a1b
09161c171b160802071b081511141b15781e0f1020101e1c1c2211101411
70110111100f0e0eb802c94011021e1402021e1f1da50000700180010201
b801b5400c08100f03151616080809081cb801fa40090f11011102a50e40
11b80230b34f1e011eb802ec400e20400e500ef00e030ea7206b8a182b10
f65d191afd5ded181a10ed105ded003f3c103c103c3f3c10f45d3c10fd3c
870e2e2b057d10c4875d0e2e182b87057dc42b180010ed0110c00010ed01
10c00010ed0110c00010ed0110c087107dc43c073c3c073c313001715d2b
2b2b2b2b2b2b2b2b01725d59012107061514161715213536373637013301
16161715213536363534270b0203a9fdf35c223b62fe555519333e01dd23
01d8395d53fde95139286ee6ec01c6d64f271f2f0725250f183093045cfb
988851052525042e212c5f010d0224fddc00>/BAAAAA+TimesNewRoman AddT42Char 
1 10742 37 <00030022000004e6054c001e002b0038027d40305a005a1e8900881e8933
991a9d27ac1aac27e91aea27e72f0c38007a2779339a329933a524aa33d8
1ad827d8280a043ab802e7b30f67363ab8ffc0b31c22343ab8ffc040e315
17343340212c343340191e34324023283432401b1d3444244425891ad901
d624da33e52507042401250d32100315061b1a141e1624162815302e3245
244a34570158195a279602111000103a55015a24603a703a803aa03a081a
301a3250000310071a241e28192f040602031e171e4f3388249a24d93307
203a403a503a6302630360056006600760307606731a731b701e74247327
7a288406861b861e8f33803aca2fda2feb24fa241959080f1f1b09212210
1f1b16212333240003042c00352b1f24032229382c33032e222835350916
2928171716022e280808090890260126b8ffc0b23a3526b8ffc0b2423526
b8ff80b33f413426b8ffc0b343463426b8ffc040144235264c5f1c010a1e
301c021c55042b1f382c31b8ffc040104535124004a004020004a004e004
0304b8ffc0400a0d113400040120040104b801d140252c06131302552c0c
0f0f02552c0c0d0d02552c22100f0e0f1002550f200d0d02550f9e393abc
01d100210061011800182b2b4ef42b2b3c4ded2b2b2bfd5d712b5d714358
b90031032de91bb90031032ded592b103c3c3c10f45d72ed2b2b2b2b2b72
003f3c10ed3f3c10ed1112392fed12173911121739113901111217392b2b
3130437940412f342328181e01071a1b191b020606262425022533262818
2633012f07313301231e2633033401313303271b29330130052e3300251d
2233001e32033533010100103c2b3c2b2b2b012b2b2b2b2b2b2b2b2a8181
8181015d7101727272007271002b2b2b2b012b2b2b005d005d0116171615
140606232135333237363511342726232335213217161615140625161633
3236363534262322071116333236353426262322060703b28d466180dfe5
fd80335525171d274d33024aa463969e7cfd7b255f3992934ec2ba645074
71b5be56c28f3e581b02b41e425c8565b95525362372036c7e212c251824
b77766a10f07073f824d77a816fb6f1ba3784f9254040500>/BAAAAA+TimesNewRoman AddT42Char 
1 11546 38 <0001004affe1050f056b002401024042091e2f012f022f032f1f960f991e
a30fa312b60fb7120b081e011617017d037b1578168d038a169d03961aac
03bb03090c030e04021d48035903052f081011241b00b80105b5021b0101
ba00b8034bb6209a05281c0301b802dfb5112bb0100110b80341b58f0d9f
0d020db8032f402f140902ac000101013210acaf11011f113f1102111a40
260126093c2018010f181f1802180c0d0d02551849256463182b4e10f42b
5d724ded4e105df672714dedf471ed003ffd71f45df4e63fedecf4ed0110
edf4ed10c9313043794020151b060c07251a260b261625061b092d000c15
092d000819052d010a170d2d00002b2b012b2b2b2b2b2b818101715d0072
715d01132326262322060215141216333236371706042320272635341224
33321716333237363704d11f1f3ee6a187da7d76ed9884ca791f66fef0bb
feafb98ab6013fbd938f2a121b141a0b056bfe33cfb689fed4dfb8fef290
71a814b5a8fabafccb0154bb4816131b3000>/BAAAAA+TimesNewRoman AddT42Char 
1 11924 39 <0002002300000579054c00160021010340590b1b0b1d86109510d5100576
107614871098139915c91bc91dd41008181112141d1e03071501871a881e
022808061f1b002122071f1b0d21231721191f280e0e0d02192816160008
1c3c4f1201001210122012301240120512b8ffdeb60d0d0255124923b8ff
c0403e3f354023012023017023a023e023032321170613130255170c0f0f
0255170c0d0d0255172207060c10100255060c0f0f0255061a0d0d025506
9e226163182b4e10f42b2b2b3c4dfd2b2b2b3c4d105d71722bf62b5d724d
ed003f3c10ed3f3c10ed1139392b2b31304379401c1a1e0f15102514261e
0f1c56011a151c56011d111f56011b131956002b2b012b2b2b2b8181005d
7101725d7133353332373635113427262323352120041215100706212716
33320011100023220723335624161c274d3302280130013dc1acc1fe75db
7f56e80132fecef05a7325372173036c7f202c258afebed3fee5bed4621c
01460117011901441d00>/BAAAAA+TimesNewRoman AddT42Char 
1 12294 40 <0001002a000004b4054c00330136403f4035671c771c9b30a918ac30bb30
e035085619700670077f087f09800680078f088f0909241f1b1d2122251f
1b2b212308401010025508210e0e1f091b0807b8ffc04021101002550721
02021f061b071c101b0201230e0f0f1d3300a52b2e002d102d022db802d3
40212c2c2b021514a51d1be81c1c1d0809ac080806ac3f077f0702000710
074f070307b8ffe640501010025507762eac2c2b1f2d2f2d022d6c1aac20
1b401bdf1b031b5350357035a035033500100613130255100c0f0f025510
0c0d0d0255102225240c10100255240c0f0f0255241a0d0d0255249e34e0
b9018700182b10f62b2b2b3cfd2b2b2b3c105df65dedf45de4fdf62b5d5d
ed3c10ed003f3c10ec10fd3c3f3c10fe5d3c10fd3c12392f3cfd3c011112
3910edec0010f52b0110edec0010f52b2b2b3130005d015d011121323736
373311232627262623211114161633333236373637330321353332373636
3511342726232335211323262627262301ac012a7427340625250e0e1252
55fed6102838e67368303e412875fbeb30302b20171a24543004150f2715
333228650502fde8232e74fe28631c2328fe415a2717202f3e7dfeac2517
1040630371811e2825fed76b50150f00>/BAAAAA+TimesNewRoman AddT42Char 
1 12760 41 <000100210000041f054c002d012ab1282fb8011e40372564360904090ab0
2f03982bba2bc62bd903d32be904e90afb04fb0a09700570067f077f0880
0580068f078f0808070a092a0207210c0cb80126400d081b071d1f1b1721
2206210202b801264029051b060e1f1b1621231e1f1b2621232b2c280a08
0c0405020201230c0d0d172d002326002810280228b802d3402527272602
161708272b28ac002901002930294029702904299006061f07014f0701bf
070107b801b5402e000e06131302550e0c0f0f02550e0c0d0d02550e221e
1d0c101002551d0c0f0f02551d1a0d0d02551d9e2e6163182b4e10f42b2b
2b3c4dfd2b2b2b3cf45d71723c10f65d71fde4003f3c3f3c10ee5d10fd3c
12392f3cfd3c111239111239011112392b2b0110edec0010fd2b0110edec
0010fd313000715d015d712b0111333236373311232e0223231114171617
16333315213533323736351134272627262323352113232e022301a3f755
4f0d252501274544f70d0a202c3031fdba305426180d0a1f2b313003f10d
231a45656a0502fdeb4b6ffe354f4a25fe566721191218252531207a036c
672119121825fed65f592800>/BAAAAA+TimesNewRoman AddT42Char 
1 13192 42 <00010048ffe105aa056b0034015d40540a04462e0219271a280210181019
02203640366036780870187019782a90189019b018b0190b2d2f760b870b
0318362e1a503670368c04ad04e036040c03860bc0360348081e1f1b18f3
22121f1b172123341b00b80105b3021b0101ba01b30000034b4043319a2c
1718182206282c030e282209012b1f1e0c131302551e0c0f0f02551e060d
0d02551e22111150129012020f124f1202001210127f12ff120412041010
02551212b8ffe4b40d0d025512b802f8400b0a3c5026010f261f260226b8
fff040100f0f025526100d0d0255264935648a182b4e10f42b2b5d724dfd
f62b2f2b5d71723c10fd2b2b2b3ce4003fed3fed12392f3c10ecf4ed0110
edf4ed2b2b313043794034202b07100825282729272a2703060c2624250f
21113b01201f1011072b0a2d000d230a2d0010200e3b000927062d010b25
0e2d002b2b2b012b2b103c103c2b2b2b2a2b818101715d2b005d015d0172
007271011323262726232007061514121633323637113426262335211523
220706151106062320272635343736373633321617163332363704e92323
355479befefd877196f3804b8c411f4152020d194e1d1473e089fe77cc99
5666b295cb4a796f3813131b03056bfe54a05175cdadefc2fec095262501
88663f21262634256dfe613e3afcbdf7b3a4c369571829152333>/BAAAAA+TimesNewRoman AddT42Char 
1 13698 43 <000100230000059d054c00450177b10202435458b747400d0d02550025b8
fff6b5131302552534b8fffc401213130255341a0d0d0255340c0f0f0255
3413b8fff64013131302551301220c13130255220c0d0d025522b8ffe840
0c10100255220c0f0f0255221a411003e2001d03e2002c03e2002f03e200
2e000c03e2000903e2003f03e2003c03e2400b3d0024242e3d022e1c0a02
003f2f2f3f12392fcd10ededecec10ededecec012f2b2b2b2bc0cd2b2f2b
2b2bdd2bc031302b1b40717047a047d047e0470413479e1c40365047e047
02121f1b0b2122221f1b1c2122341f1b2e2122451f1b3e2122021f1b0a21
23131f1b1b2123251f1b2d2123351f1b3d21230100232324241b3e3d3d0b
0b0a022e2d2d1c1c1b0812132202402201df2201202230227022a022d022
e0220622b80220401a10476047c047032047014745252235503460340234
9e4661dc182b4d10f4723c4dfd3c107172f45d71723cfd3c003f3c103c10
3c3f3c103c103c12392f3cfd3c2b2b2b2b2b2b2b2b3130015d2b015d5901
211134272627262323352115232207060615111417161716333315213533
323736351121111417161716333315213533323736351134272627262323
35211523220706061501a502760d0a202b3030024430302b20170d0a1f2c
3030fdbc30532619fd8a0d0a202b3031fdbb305426180d0a1f2c30300245
31302b1f1802d701846821191218252517104164fc956721191218252531
207a019dfe636721191218252531207a036b682119121825251710416400
>/BAAAAA+TimesNewRoman AddT42Char 
1 14268 44 <0001003300000278054c001f00c1406f21401010025521400d0d02552140
2835192161116436081f1b022122181f1b122122191f1b012123091f1b11
21231211020201081819021313025519080f0f025519040d0d0255192209
70088008e00803ff0801300850086008035f08c008d0080308040f0f0255
081a0d0d025508b8fff8b41313025508b8fffe401d101002550861207021
8021e0210330215021602103c021d0210261dc182b4e5d717210f42b2b2b
2b5d7171723c4dfd2b2b2b3c003f3c3f3c2b2b2b2b31302b2b2b2b251521
353332373635113427262726232335211523220706151114171617163302
78fdbb305426180d0a1f2c30300245315326190d0a202b3025252531207a
036c6721191218252531207afc94672119121800>/BAAAAA+TimesNewRoman AddT42Char 
1 14558 45 <0001002affe10311054c002300e9403b4512015f135f140264177017850c
ab0fc0250512180130254025021a08081f1b0221221d1f1b01212316181c
101619020102301440140250140114b8030ab519280d091d1cb8fffab413
1302551cb8fff4b40f0f02551cb8fff440210d0d02551c22090930084008
8f089f08af0805bf08df08ff080308021313025508b8ffea401410100255
08160d0d0255081a25df100110e02425b80231b321e0a2182b2b4ee45d10
f62b2b2b5d713c4d10fd2b2b2b3c003feded5d713f3c113901111239392b
2b3130437940101a1b0a0c1a0c1c3b010b0a1b0b193b002b01103c2b8181
0171725d005d711335211523220706151114060623222635343736333216
17163332363511342726272623cc02453153261843a4745e6c19212c2033
2717241b2f0d0a202b300527252531207afd6999be8d5d3c31191f2a5b36
4254039e672119121800>/BAAAAA+TimesNewRoman AddT42Char 
1 14898 46 <00010022000005d8054c004302b040b87b0ebe0e026c00017f0075027b0e
763079357a36bf0aba0d086d00011204452e116436360255026502800289
4090029940b30db40eba33ba43d50dd7320d120b01030e02060205328b00
87329e00ac01a00ed132080b0001010002050c1f091e0d2a0025012f093f
094f098c00c634d900f2340f090b190b30013502334042405045a601a302
a540b602b60ab042cd00dc00d001d402d603eb00eb01f001f50af00cf20d
18163316343432303454019900940d9632953409b1060243545840212f0f
221e3c1e454415001530020e300003271816191b1806180829261b273b27
02003f3c10fdc53f3c10fdc5111217397101111239392ffd3c1b4039060d
071b061e1f1b1821222f1f1b2821223c413d1b3c0504041b050f1f1b1721
231f1f1b2721233b343a1b3b010000220e0d140e0e0d410000b802c94054
30341430303400010d3441054530004134043a0d01020c0b0a0907070e70
0ebf0e020e2607040707161619ac183c3b3b2828273d3a3a292926ac2718
1717060605270205083c93040e30302f0480050170050105b80238400c40
0d500d02800d01b00d010db802f9402c2f0f06131302550f0c0f0f02550f
0c0d0d02550f221f1e0c101002551e0c0f0f02551e1a0d0d02551e9e4445
bc013c00210061011900182b2b4ef42b2b2b3c4dfd2b2b2b3cf65d7172fd
5d713c103c103c10e4003f3f103c103c103c10fd3c103c103c103c103c10
3c10fd3c103c103c1112395d2f12173912173901121739870e2e2b7d10c4
870e2e182b7d10c4180010ed0110c02b2b10ed0110c00010ed0110c02b2b
10ed0110c059313001725d71007172435840092f332d412f422d43045d59
5d2b435c58400a3618160d3f0a20143932b8ffe0b6103940100e3901b8ff
e8b20e3900b8ffe0b20e3901b8ffc0b2103900b8ffc0b11039002b2b2b2b
2b2b012b2b5901715d00715d010116161715213532363534262701111417
161716333315213533323736351134272627262323352115232207060615
11363700373635342623233521150e02070607026401f47bae57fd7b3a33
1335fe2c0d0a202b302efdbe305426180d0a1f2c303002422e2f2c1f1814
7501293e1b2a321f01f22c48684c16b502f0fe0f7b590625252718182634
01cffe4b6721191218252531207a036c6722181218252517104064fe6113
6c01105b281e1723252501163f4614b9>/BAAAAA+TimesNewRoman AddT42Char 
2 0 47 <00010029000004b7054c002000b0401b1000100120002001402257026702
77028a209920a920b9200c0122b8018e40330e643655025c1e02091f1b03
212216371b113d220a1f1b102123201f2000300040000300e71c1110021c
2302030800ac016c02b802c4402f16170613130255170c0f0f0255170c0d
0d0255172209090a0c101002550a0c0f0f02550a1a0d0d02550a9e21615d
182b4e10f42b2b2b3c4d10fd2b2b2b3cf4f4ed003f3ced3f3c10e45d3939
2b2b2b313001722b015d0117032135333237363511342726232335211526
0606151114171616333332363604962174fbe6335625151c274d3302666c
5720100c3283639c7e68017707fe9025382074036b7f202c2525012a4079
fcac531f15142e75>/BAAAAA+TimesNewRoman AddT42Char 
2 278 48 <00010022000006f2054c003001c940e80f18010e0008170e190d280f290f
2a043007123d013d2f59186f0168186d2f791897019a2fcb18da18e801eb
180d0d18010a170630463003361836304718031630271826300306180530
1717032b00291826303b003a173918351935303f324f3268007a00761879
1974308a008918853099009730a900a630a032b032cc17c918c032dc17d9
18d032ed17ea18ea19e032f600fa17f7302548014917462f5a015917562f
6a177819c618c530d618d630e518e5300e0f1f1b092122201f1b1a21222e
1f1b282122021f1b082123101f1b162123211f1b27212317181822000114
0018190001191818b802c9403e302f14301817302f182f012f180316171a
1919170209080800003030272808305b000002192f2e22202021a021b021
c021d021e02106219e403201320102b802c9400d100f200f1102550f9e31
61dc182b4e10f42b3c4dfd3c4d105df65d3c4dfd3c3c11392ffe003f3c3c
103c103c103c3f3c103c103c173901113987082e2b057d10c487082e182b
057d10c4182b2b2b2b2b2b3130015d5d7171717100715d435c58401b2f10
140c3f0110140c3f0110103918181139181012390008183917b8ffd0b517
3917301439012b2b2b002b2b2b002b2b59015d005d210111141716333315
213533323736351134272626233521010121152322070615111417163333
152135333237363511010346fdf41b255030fe2830562416140e4b530180
01ec01e401802f5724161c25502ffdc030572316fdf50475fc767d1f2a25
2534207203765a281d2725fbdb042525342072fc8a7d1f2a252534207203
8afb8b00>/BAAAAA+TimesNewRoman AddT42Char 
2 882 49 <0001ffe5ffea05aa054c002701c1404b8a1201128f010102404f358f0201
121d020127022d13381378139802df02ff020713222212101f1b0a212221
1f1b1b2122031f1b092123141f1b1a212312121101020222122214121222
22b801a2400f27ac010a090901021b1a0812090302b802c9400c12531111
2010301040100310b8ffe0b41111025510b8fff4b40f0f025510b8fff4b6
0d0d0255109e29b8ffc040103f35402901202901a029e02902291314b802
c940152121302201c02201220c1010025522100f0f025522b8fff0400a0d
0d025522192861a2182b4e10f42b2b2b5d713c4d10fd3c4d105d71722bf6
2b2b2b5d3c4d10e6fd3c003f3f3c3f3c103c10eded872e2b057d10c40012
390139182b2b2b2b07103c3130005d72435840280912191229013f003912
4f004a125f005a126f006a127a129b01a901bb01b512cb01fa0112ef0201
005d015d5900712b0171435c58b90002ffa8b31e123f02b8ffc0b3160d3f
12b8ffe8b6173901401c3912b8ffe8b21c3912b8ffe8b21b3912b8ffe8b6
19390108183912b8ffd8400f123912161239021015390210193913b8ffd8
b20b3902b8ffd0b20b3902b8fff8b5143902401139002b2b2b2b2b2b2b01
2b2b2b2b2b2b2b002b2b59005d0321011134272623233521152322070615
11230111141716333315213533323736351126262726231b0170033d1c25
502f01d83056241624fc821b264f30fe282f5724163b3d3b1d3b054cfc07
030e7d1f2a2525342072fb890444fcbd7d1f2a252534207203af452c1309
>/BAAAAA+TimesNewRoman AddT42Char 
2 1452 50 <00020048ffe10578056b000c001b00b140319712a807a90aa91004770179
07870188070443080d28000315280609183c1f032f030200031003200330
0340030503491db8ffc0401a3f35201d401d021d113c10092009020f091f
090209491c6463182b4e10f45d724ded4d10712bf65d724ded003fed3fed
313043794032011b0f250b261a2613260e0c112d001b01182d011407112d
001605182d01100a0d2d0119020d2d011208152d001704152d002b2b2b2b
012b2b2b2b2b2b2b2b81015d5d0120001110002120001110373617220706
111017163332121110272602ed01080183fe7afeebfee8fe83dcbff7b66e
898e6db3bff9896e056bfe6ffed4fecbfe68018e013c0143ccb14987a8fe
bcfeb4b388012a0141015cab8800>/BAAAAA+TimesNewRoman AddT42Char 
2 1736 51 <000200220000042b054c001f002c0178b9002effc040933a352f2e751874
1b741c7c28702e951c077918b724ba28db1bdb1cda24061927102e282639
2539273b28302e5a276927702e802e0bc600011a1c291c4b1cd719db1b05
a82801ca24d917da24d927d828eb24061c40231d28080e1f1b082122011f
1b0721230f1f1b152123001d202c2a1d283f234f2302232307152a281616
150208070812001a101a301a401a701a051a492eb8ffc0403e3f35002e01
402eb02e029f2ec02ed02e032e2c010613130255010c0f0f0255010c0d0d
025501220f0e0c101002550e0c0f0f02550e1a0d0d02550e9e2d2eb80177
b3216163182b2b4ef42b2b2b3c4dfd2b2b2b3c4d105d71722bf65d4d4358
b90026032de91bb90026032ded59003f3c3f3c10ed1112392f5ded123939
12392b2b2b31304379401c2429171c182528262917263301241c26330127
192a3301251b2333002b2b012b2b2b2b81810049547940101e22211f233b
04221e203b0021201f0001103c103c2b002b8101715d0071720172005d01
5d2b01111417163333152135333237363511342726232335213216161514
062322262716163332363534262623220701a41c264d34fdbb335625141b
274d3301f1b6d290dbc831724135521d68974884543350027bfe75801f2c
2525381f74036c801f2c254bb27aa6d00e470a0aa18058974b13>/BAAAAA+TimesNewRoman AddT42Char 
2 2242 52 <00020048fe6f0579056b0015002600fd402945015807950103060e015701
580766017601860190009608c70fe50009040f40004201035608039704b8
02d0402f0816281003001eac0808200030007000800004005208080d032b
223c1f132f13020013101320133013401305134928b8ffc0401a3f352028
402802281a3c100d200d020f0d1f0d020d49276463182b4e10f45d724ded
4d10712bf65d724dede412392fed5d003fed3c3fed10f4ed313043794040
092620251c260b0c0a0c020618252423252302061f15222d011d091a2d00
170f1a2d002611222d0121141e2d0015001b0c1e2d000908190e162d0123
12162d012b2b103c2b103c2b012b2b2b2b2a2b2a2b2b8101715d00715d05
161617152624242726272602351000212000111400012207061110171633
3237361134272626038666ed978afec6fee76690547a87018a0118010a01
85feebfe7ab66f8c8e6eb5bc73874a39bd0fb0a60c200565b3653a416101
1bc101300192fe6dfecdf9fe8804ea82a3feb0feb7b28989a2013cf3a680
7900>/BAAAAA+TimesNewRoman AddT42Char 
2 2634 53 <0002002300000568054c00280034020240b224180f0f0255250c0f0f0255
872201128526c523c52d034924a72d02181f172e66240309010925262547
0058016f026f247b017b02731f7320762278258a018720982dab01ab25b7
26bc2dff2415062084018c2484279a24a501a402a624af2dbf2dd830ef2d
ff2d0d120016011a0212281a301a313a2e3a306624692f0a2a08021c1c01
151f1b0f21220025281b00081f1b0e2123161f1b1c212340022c25242422
02011402020124ac022002072a29a507b8ffc040170f0f02550710075007
6007039007a0070207001bac1c34b80191400f32281d1d1c020f0e0e0101
00081221b8ffc0b2583521b8ffc040454f350021af21024f21a0210221b5
10360140367036d036033634080613130255080c0f0f0255080c0d0d0255
082216150c10100255150c0f0f0255151a0d0d0255159e3561b901190018
2b4e10f42b2b2b3c4dfd2b2b2b3c105d72f45d712b2b4358b9002f032de9
1bb9002f032ded59003f3c103c103c3f3c10eded10ed12395d722f2bfd3c
103c191a10ed870e2e182b7d10c40112391a182b2b10ed0110c02b871005
7dc43130184379401c2d311e231f252d232f3301311e2f33012e222c3300
23243020323301002b103c2b012b2b2b81810172715d0072715d435c58b9
0025ffe0b20c3901b8fff0b2143928b8ffe0b614390210193928b8fff0b5
103930100f39002b012b2b2b2b002b59015d2b2b21210106232226271114
171633331521353332373635113427262323352132161615140607011616
170132163332363534262322070568fe96fe3533200d1e101c264c35fdbb
335625151c274d3301eed8cd8fa3ab0118608a6ffc3d131c09c2c59f833a
63027a020101fe76801f2c2525381f74036c801f2c253fa9757db826fe7b
86580c029401a8827f9f1300>/BAAAAA+TimesNewRoman AddT42Char 
2 3306 54 <00010080ffe10405056b00380257401912952c010f010f020b03000f0428
0029052b4f014f0209113ab8014640d03638361a031b045f185f195f1a5f
1b06050d050e002ac03a04740b740d740e760f701e701f702f7030890886
0b870d870e840f872ba804a83310120d330d340d351d331d341d352f012f
022d04201e201f29292d333e013e023f043019301e301f30213d343d3548
0d482a540b560d57105629562b1d1f011f021b331f351b3654185419541a
59325c335c345c355c365a370e030b0b29130b1b29230b203a3b29303a72
12721389249807982f9930a82fc028c12ac62bc03af03a144e08381b006f
021baf01cf0102017f010101ba00b8034b400d359a311c1b1d6f1f1b1e1e
ba1db8034b4034199a142a2b2b3c0c0e140c0c0e2b0c2a0e0426092b0c2a
0e04062301fd0000062831032328140902ac01401e223401011f260126b8
012340102f11bf1102df11012011af11df110311b80287b71fac1e2b1009
0109b80123401f9f2e01bf2eef2eff2e032e404735402ecf2eef2e03002e
202e302ec02e042ebc014600390146011800182b4e10f45d5d2b71724ded
72f4edfd5d7172fd72392f2bed003fed3fed3c10ed111217390111121739
870e2e2b0e7d10c4180010ecf4ed0110edf4ed0010ecf4ed5d011071edf4
ed3130437940362430071328260b2c093300290f26330124132633010730
0933000a2d0c33000b0c2c2b27102a33010f0e292a2512233300082f0633
01002b2b103c103c2b103c103c2b012b2b2b2b2b8181015d00725d435840
09630b660d6710632b045d595d0171722b0071005d435c58400c0b180f39
04300f3933300f39002b2b2b590111232e0223220615141716171e021514
062322272626232206072311331e02333236353426272624262635343633
3217163332363703ab25125dac5c68882b3ee9be8b4befbc3b341fc31a19
1d0725251a58b56c7d91373a27fea4934ce0ad6c7938171a210a056bfe2b
87a05e7f513e334b7d666d94519adf09053f1e2f01d1929160845a32662c
1ec3748c5492d335191f2f00>/BAAAAA+TimesNewRoman AddT42Char 
2 4068 55 <0001003e000004b0054c001f00f1403a5a015a025a1d5a1e6b016b026b1d
6b1e082f213f214f219805971ba805a61b0702011d1e161f1b102122091f
1b0f2123071823001f02100f0821b802c0401309012b0040170e3f120f00
1f005000af000400b80228401a08090613130255090c0f0f0255090c0d0d
0255092217161f2b1eb8ffc0400e170e3f12001e101e5f1ea01e041eba02
280016ffec400b10100255161a0d0d025516b802c0b320645d182b10f62b
2bf45d4358b9001effc0b20b351eb8ffc0b20b0f342b2b592be4103cfd2b
2b2b3cf45d4358400900400b3500400b0f342b2b592be410e6003f3c3f3c
fd3c2b2b0110c910c93130015d005d011323262726262323111417163333
152135333237363511232207060607231304a10f260b131f6754bf1b264f
2ffdc130562416a35f28344a072610054cfec254243a37fbf47d1f2a2525
342072040c0e136c5c013e00>/BAAAAA+TimesNewRoman AddT42Char 
2 4410 56 <0001000bffe005b1054c002e0183b90030ffc0b32a2f3430b8ffc0b32024
3430b8ffc04054161c3428063a064c06790f042523252732233227452345
27a5270729273927025030740b7b0f9a27bf27f826063c0e081f1b022122
1f1f1b1921222a1f1b012123131f1b1821231918180202010225280d092a
29b8fff1b41010025529b8ffe6b40f0f025529b8ffe6b40d0d025529b802
c94010090908400c3908403f35200830080208b8fff4401114140255080c
1313025508061010025508b8fff4b60f0f0255081a30b8ffc040443f3510
30017030a030b030e03004301f200613130255200c0f0f0255200c0d0d02
55202212127f13016f1301130c10100255130e0f0f0255131e0d0d025513
192ff4a2182b4e10f42b2b2b5d5d3c4d10fd2b2b2b3c4e105d712bf62b2b
2b2b5d2b2b3c4d10fd2b2b2b3c003fed3f3c103c103c2b2b2b2b31304b51
79b137084379402621280a112221232102060f252725240e202d00101126
0c292d010b0a2110252d00280b252d002b2b01103c2b103c2b2b2b2a8181
015d71005d0071012b2b2b01352115232207061511140606232226272635
1134262323352115232207061511141e023332363635113427262303d101
e033502b1551edccdee63020454d33024a345424191d4c8f6885d24d1c27
4d05272525431f71fddacce1a19a8259f502127d4e2525352472fdb14fcc
724a74b5d802257f202c>/BAAAAA+TimesNewRoman AddT42Char 
2 4930 57 <00010012ffe105ae054c001f0212b40a0f061f02b10202435458b416011e
100db803e2b70e1f0216070e0207002f3f12393f10fdd0d0c0012f31301b
400c1210210116080b39a9160121b8ffc0b2183521b8ffc0b333353421b8
ffc0b32c2f3421b8ffc04083202334f312fb1ff02103ba17b918bb1ab021
f90705a919ac1abc05b606b90705aa05a706a907aa15a716059b07900f90
129a16902105691564177404790a8021055a165717502165066907055b07
59085b0a5e0e59150540215000540357055306052021340438154600490e
0525062907280828152816050021202130216021d02105b1060243545840
1c000e21200a161a162a160316070d011e100d1b0e06070107081f0e0200
3f3c3f5d10fdc5c5c51112395d01111239391b40140005011b000f15101b
0f0e080d1b0e1f171e1b1fb8ff8740111607062008070722161514161615
050606b802c940351617141616171f0f0f0e0e0002070609fb170117e730
1640169016f0160416e8301540155015b015f01505201560157015801504
15b802ebb6202196216b8a182b2bf45d5d19f45de45d00183f3c3f3c103c
103c87052e2b0e7d10c487052e182b0e7d10c42b180010ed0110c00010ed
0110c00010ed0110c00010ed0110c059313001715d5d5d5d5d5d5d5d5d5d
5d2b2b2b2b005d2b0172435c5840090a1812390f40123904b8ffe8b61039
0808133907b8ffd8b613390a28133904b8ffd8b10f39012b2b2b2b2b2b2b
5959015d0115060706070123012627262627352115060615141701013635
34262726273505ae48253529fe2725fe04271019493e022a5e382e015901
402f3a45050c054c250d213165fb7e04915a141f23052525092e24326afc
e50311742d1d350b01022500>/BAAAAA+TimesNewRoman AddT42Char 
2 5572 58 <0001001bffe1077d054c0039031eb10202435458b609013829261411b803
e2400f12390227021c09301b040b12020b08002f2f3f1217393f3f10fdd0
d0d0d0c0012f31301b401909060d070c080a09070a0a30063907120e1813
390c1813391bb8ffc0b30809341bb8ff80b30809341cb8ff8040e8080934
3609352f4a0959045809a7090626062b082c0b280c2813281a291b2a2827
313606391a3430470644074b0b481b540658075808590a580c581a583054
31690664076c0b681a681b6b33760476067607760a780b7b0c7b1a781b7d
1c7820752f85048c088a1c882f883089319207990b93139318991a981b94
28952f9430a808aa09aa0baa1aa81ba91caa1da72fb307b308b70ab81ab4
30c730f908f90bfc1df9204a682f65306831890904381b6c1e6f1f6e2d04
650765086809034b094c1f48284b2f04591b572f513003500750085a0b03
0407000a030b0b1c162f2a1c291f3107390b09b10602435458401d00123b
3a1b30091c040b110138292614111b1208070b010b0839271202003f3c3c
3f5d3c10fdc5c5c5c5c51112173901111239391b402c091c1c0809090a1c
1c1b1d1e1e080006011b00131a141b13282f291b28120c111b12271e261b
273931381b39b8ff70b31b0b0a20b8ff6f4014300807200c0b0b221b1a14
1b1b1a1c1c1e090a0ab802c940151b1c141b1b1c2f1d080822302f143030
2f31060707b802c9401c303114303031131227282839391200020b0a0a08
0807093b9e06a531b8ff80b2403531b8ffc0b23a3531b8ffc040262d3034
303180319031034f315f316031703180319031e031f0310831e808e70952
0b1bb51a0bba0220001a01fa400b400c500cd00c030ca73a3bb8026ab321
6b8a182b2bf65dede41910e41810fdf4f45d712b2b2bfde6003f3c103c10
3c3f3c3c103c103c103c87052e2b870e7dc487052e182b870e7dc487052e
182b87087dc487052e182b0e7d10c42b2b180010ed0110c00010ed0110c0
0010ed0110c00010ed0110c00010ed0110c00010ed0110c007100e3c083c
083c07103c593130015d5d5d5d5d5d5d5d005d002b2b012b012b2b435c58
40142828160d3f1e28160d3f2030160d3f1f18120b3f002b2b012b2b5901
5d5901152206070607012301012301262726262335211523220615141701
132727262726272627262335211523220615141701013635342627262335
077d35421e142bfe8628fecbfecd24fe6d2d0c14453b01f61835382c010b
e12820151a0d131919132902102438342d010401022c1d16263d054c2526
342384fbbb0363fc9d04667e17262525253022237efd070287725b322613
0d12080625253029337ffd1f02eb7c301728080e2500>/BAAAAA+TimesNewRoman AddT42Char 
2 6554 59 <0001000f000005af054c003f032cb10202435458b4110407181bb803e2b4
063a372825b803e24010261121002e0426193802260219080608003f3f3f
3f1112173910fdd0d0c010fcd0d0c0012f31301b40107911010d1909263a
017800772105121fb8ffe0400e0f392f1014391041402b40410341b8ffc0
408f1f2334760078117a22702b7a2d9a229923a601a610a921a922a923a6
2da92fbb23bb25bb26ba38b63fc810c51bc520c839c041d512d520f90bf0
411c122f1020122220242b282e2f2f3d10301230203b213627302b47000d
12004120413041d04104c62d01742d7c2f852b892f04432b590c59210309
231923163e3f414b1a43270612142e01242e6521a521a52e04b106024354
584022041a41402911262e021100212e041b250407181b1b1a061a083a37
28251b26382602003f3c10fdc5c5c53f3c10fdc5c5c5111217395d011112
39391b404b2e202f012d21202f1022111022123f00012d123f0610071b06
1a201b1b1a272d281b27393f3a1b390501041b051912181b192622251b26
382f371b382d22101022012d1401012d2f3f1212b802c9403e202f142020
2f2e211100042e211100040122393838272726021a191906060508683f01
3f2b0001010f01200130015c0160017001b001c001e001f0010a01b802fa
400f4420532064200320320022a0220222b802c3b6404196216b8a182b2b
f65df45dfd5d71e45d003f3c103c103c3f3c103c103c1112173901173987
0e2e2b870e7dc4870e2e182b870e7dc4180010ed0110c00010ed0110c000
10ed0110c00010ed0110c00010ed0110c00010ed0110c00010ed0110c000
10ed0110c00f0f0f0f593130005d5d4358b2202f015d59015d5d5d5d0171
4358b62f0129222f3e035d595d435840096921642b6f2f6041045d595d2b
01722b002b435c58400f66276938022a18160d3f23100d3902b8ffe84013
0c3923180b392e180b39234816392630163902b8ffc0b616392228163904
b8ffe0b2163914b8ffe0b60b391810123902b8fff0400b12392d08123922
20123938b8ffe8b20f3927b8ffe8b20f3912b8ffd8b20f3920b8ffd8b20f
392bb8ffd8b20f393eb8ffd8b10f39012b2b2b2b2b2b2b2b2b2b2b2b2b2b
2b2b002b2b2b2b2b015d59015d005d590101161617152135363736363534
272627030106061514161715213536373636370101262627352115060615
14171313363635342726262735211506070606070344012379755afdba3a
1c151b090730e6fee42d12364cfe1f33253e70480140fef56d9863027350
3b30d0f12a130c0f2e4801e13924365a5202effe4eb45f052525010b0925
1317171147015cfe943a2715202a03252505101a585b019401879f630325
25032e1c2547fec9013136281515101511012525030f174e6900>/BAAAAA+TimesNewRoman AddT42Char 
2 7570 60 <00010013000005a9054c002e01d5b40500011230b8ffc040a83f3540305e
185e195030042c177b17792679278b178927061905190602003015071528
203050300505050607062815020421002001240728272428252e30304601
4030510158075a1e58285030730673077328732a70308001800684078428
802a80309f2aa301a302a030c41dd51de03020850687078728030107021b
01161f1b1021221f26201b1f00282e1b00091f1b0f21231e181d1b1e2426
18171722272614272726070808b802c940222728142727281826172f2807
30082807272618051f100100001f1f1e02100f081716b8fffab413130255
16b8fff4b40f0f025516b8fff4400f0d0d02551622400809020f0f025509
b8fff4b70d0d025509ac2027b8ffc040120d352027302740275027702780
2790270727b80298b32f6b8a182b1910f45d2b1afd2b2b3c1a18fd2b2b2b
3c003f3c3f3c103c103c1112173901111239391112393987042e2b0e7d10
c487042e182b0e7d10c4011239180010ed0110c02b10ed0110c00010ed01
10c02b10ed0110c0b10602435458b43a263a2702005d593130015d5d7171
0071005d0172012b435c58b90005ffe0400e160d3f0128120b3f0028120b
3f18b8ffe8b20c3907b8ffe8b20c3927b8ffe8b10c39002b2b2b012b2b2b
59015d012115232206060701111417163333152135333237363511012626
272623352115232206151417010136353426262303d001d91a1a64523cfe
b91c26522cfdc030562416fe8c422f4a142602441e2f4f3d011b010a3c1d
3636054c252e5661fdfdfeac7d1f2a2525342072014102386432230a2525
2c2c245efe4b01a25e2e1c2c1900>/BAAAAA+TimesNewRoman AddT42Char 
2 8184 61 <0001001a000004aa054c00110102b41240130113b8ffc04062131a34380f
381044054a0f8604890db709b90fb9100925014e0045014e0a6404620760
13740472077013860483078013a900a90aa50dbf00b801bf0ab80d140f10
050607050303061105060b00010122090a1409090a0910080a0100030611
090109b803404033080a0b23111100020201230708080908200630064006
9f0604061a2f133f134f1303131132201001108e0819121379216b5d182b
2b4ef44df45de44e105de65d103c003f3c4dfd3c3f3c10fd3c10e6123901
11121739111239872e2b7d10c400123939011112173910c910c93130015d
005d012b72435c58b400100c3900b8fff0b214390ab8fff8b11439012b2b
2b59010121323637170321350121220606072313049afc85022c80893521
40fbb00366fe4e6c613315261c054cfb0670ab06fe992504d62f597a0153
>/BAAAAA+TimesNewRoman AddT42Char 
2 8514 62 <000100a8fe6a0260056b0007008140184009010007090304052603021007
06260001120917171a03b8ffc0b2403503b8ffc0b23a3503b8ff80402337
351003200370038003048003900302a0030103870506b001015002600202
02190809b80131b321d25a182b2b4ef4713c4d10fd3cf45d71722b2b2b4e
456544e6003f3c4dfd3c3f3cfd3c01111239393130015d01211121152111
210260fe4801b8fede0122fe6a07014ff99c>/BAAAAA+TimesNewRoman AddT42Char 
2 8682 63 <00010003ffe4023d058e00030064b10105b80103400b1c64366801680202
000101b80327400f02031402020303000002010b01ad02b8ffc0b3121434
02b8ffc0b30b103402b8012fb700ad031904059421b80103b1df182b2b4e
f44dfdf62b2bfd003f3c3f3c87052e2b7d10c43130015d2b130123015301
ea50fe16058efa5605aa>/BAAAAA+TimesNewRoman AddT42Char 
2 8812 64 <0001004bfe690203056b0007008440244009a00902600901030405060726
0100100504260203123f09010917171a010102b00605b8ffc0b23a3505b8
ffc0401e37351005200570058005048005900502a0050105873000af0002
00190809bc013100210054010000182b2b4ef45d4df45d71722b2b3cfd3c
4e10456544e65d003f3c4dfd3c3f3cfd3c01123939313001715d13211121
352111214b01b8fe480122fede056bf8fe4f0664>/BAAAAA+TimesNewRoman AddT42Char 
2 8982 65 <00010025029b039b0568000600bc40220108580e6436d802014901490246
044605590159025604560569016902660466050cb10602435458400c0305
000205050005010508070111123939003f332f3c1112391bb40304030204
b803274009050614050506020303b80327400d0001140003040001050404
0201b802b54009060005006706670302be0144000101b6000301b6000401
44b5055807585e182b4e10f44dedfdfded10edfd003f3cfc3c3c103c8708
2e2b057d10c4872e182b087d10c4593130015d71012b0101230101230101
f201a95cfea2fea25e01af0568fd33024afdb602cd00>/BAAAAA+TimesNewRoman AddT42Char 
2 9214 66 <0001ffeffe460412fe9a00030020b900020327400d000f03003605020167
044748182b10f53c10f43c003fed3130012135210412fbdd0423fe465400
>/BAAAAA+TimesNewRoman AddT42Char 
2 9274 67 <00010076041501bf056e0003003b40147005d005023005010f000100d503
0f0201028401b801fdb63f0001009c0405b80209b3219cdd182b2b4ef471
4dfde45d002ffd5d313001715d1333132376df6a23056efea700>/BAAAAA+TimesNewRoman AddT42Char 
2 9360 68 <00020049ffed038903af0032003d0349b1020243545840203f400d0d0255
3f4013130255151b072e25080b0b0255250c0d0d025525000c33b8fff040
0b1212025533161313025533b8ffdeb41010025533b8fff440150f0f0255
330c0d0d02553339070c0d0d0255072d2eb8ffc04020091202552e33001e
04292c30340c40090b02550c401d1d02550c40111202550cb8ffd4401e09
1202550c0c047f180118401112025518401d1d02551810251e073c2c0400
2fed3fedc42b2b5d12392f2b2b2b2bcd2ffd11123939d42bcd012f2bcd2f
2b2b2b2b2bc0c0dd2b2bc410d4cd31302b2b1b406f0b1c8a330212533601
12201f39803fa809b60a03122b127d007d3386008b0b8b35061d12163a10
3f803f04091c4c054c06452045224c3a403f891d080a0e0720002249014b
0a490b49354b37433a493d570b670b8509840a840b0f54168316021f3f5f
3f0260083300343c2e292d34bb011b000c000cffc0b609390c280b390cb8
ffc0401a3a35100c500c02400c500c600c03200c500c600c760c040c3c18
b8ffd840290b394f185f186f18032f187f1802187e1f100110251e07303c
403c023c2c04702d802d022d35292c30b803464011040b2ec02d012d6025
00330d0c0c343433b8fffcb41010065533bb016700240025ffc0401a0e39
00251f2580259025044025f0250280250125101010065525bb0243000700
15ffc0b21f3915b80167401e1b2f393107400e3920075007800703100701
f0070150070107433e436e182b4e10f45d7172722b4dedf4ed2b10fd2b5d
71722b3cfd2b3c103c103c103c10f65d3c003ff4fde45d10ed713fed72fd
5d712b11395d71722b2b2b2fb10602435458b2030c01005d59ed11123911
123939313043794047353b1c23051337383638020609080a080206212220
220206350b392000111d131c0012130f1f0d1c0122233b05391c00380834
200135340b121c101c010e22101c013a063c1c002b2b2b3c103c2b012b10
3c2b103c2b2b2a2a2a818181017201710071017172005d4358b23f12015d
59015d2b0072435c58b431400e392eb8ffe0b210392eb8ffe0b60e393720
0e3920b8ffe8b20c3920b8ffe0400b0b3918200b3917200b391cb8fff040
1a0b390a280b3937280b390a280a3937280a390a28093937280939002b2b
2b2b2b2b2b2b2b2b2b2b2b2b2b59005d5925060706232226353437363637
353426232207061517140623222635343633321716171615111416163332
3736371506232226271106070606151416333202478d24363d5f7b1e29cb
ec57533f2526022f26252fb09f7a4e3b1c120a170f100c153c7066313a01
972c4f4456384c846d1119826a433144785624896622222c3a2e32342d56
90291f422b85fec9833b14070d3c38964493015d3c192c6039485f00>/BAAAAA+TimesNewRoman AddT42Char 
2 10378 69 <0002fffbffe403b9058e0016002401d2b10202435458b11e05b8fff44010
1010025505140c00180a0d0d0255180cb8ffe6b4131302550cb8fffcb40d
0d02550cb8fffcb40f0f02550cb8fff4400d101002550c0c181700040209
13b803e240111440090d02551415001b25090b21590207003fed3fed3fdd
2bed11121739012f2b2b2b2bdd2bc010c62f2bcd31301bb1060243545840
2618170003020913141500215902071b25090b1e0505262500180c0d0d06
55180210100655180cb8fff8b40d0d06550cb8ffeeb7101006550c0c2625
1112392f2b2bdd2b2bc01112392fcd003fed3fed3fddcd1112173931301b
4079102601a406b606b507ea1f040526430d5d3620267503760486038704
a603ab08074707013a0814270d41131e144418170c00041b160010210121
5902071b25090b1e311f0590050260058005af050305eb0c16000018240c
0c100d500d700d900d04800d900db00d03000d100d200d300db00dc00dd0
0d070db8ffc0b73c350d6025c24b182b4e10f42b5d71723c4d10fd3c103c
10fd5d72ed003fed3fed723f111739f5edfc01f53130437940281920030b
072620031e20011a0a181c0019180b0c1c081e20011f04212001190b1b1c
001d061b2000002b2b2b012b103c103c2b2b2b81810071015d2b005d0172
595901363332161514070623222627113426262322072725331111161633
323635342623220706013b859a8dd2a28bab50a5560f20181c2a0e01132d
336d395b9d9d6435352802f6b9f1d1f495803a3a03b59c481a102370fd28
fddc3233c8bfb0bd1b14>/BAAAAA+TimesNewRoman AddT42Char 
2 10958 70 <00010046ffe4034a03af002101f5b2080401b102024354584020021a060c
10100255060c0f0f0255060c0d0d02550616250f0907602170210221b8ff
c0b513130255211db8ffd4b4131402551db8ffcab6121202551d3103002f
ed2b2bc42b5d3fc4ed012f2b2b2bcdc431301bb11223b8ffc040732a2d34
0023430d5d36170d5705021c135404530553065407581b581c0767057605
80008021b41bc520d020e000e50509370147015618551c5f236018601c76
18721c8a128e1390119018a601a402af23b301c101c707c719e908e41cea
20f4011806024a1257128b1f8b208023f02307112001bcffe00020ffe000
1fffe0b2001d00b803464030102101602180210200211021202150216021
70219021a021b021c021d021e021f0210d21661ddf0f010fc7162509071d
b8ffd8b214391db8ffd8403812391d31030b21cc1f0c014f0c8f0c020c2f
100030004000600070009000b000c000e00009300040000200aa731a831a
02501a019f1a011ab8010c4012f006010006100620063006400605064322
43b9029100182b4e10f472714ded5d7271fd715de47172ed003fed2b2b3f
eded7110f45d7172e412b10602435458400a531d631d731d03931d01005d
7159393130383838013801715d005d017200722b2b435c58b4001018391b
b8fff0b613390510103901b8ffc0b2103920b8ffc0b11039002b2b2b2b01
2b5959017101060623220235340033321615140623222726262726232207
061514163332373637034a25d8839ce80101b487ae312c3b1e110b23233e
643d51a189624e3734015cb5c30106dfd8010e8f4d262f2615761f1e4a62
a1a4fb432e79>/BAAAAA+TimesNewRoman AddT42Char 
3 0 71 <00020044ffe40405058e001f002d024bb1020243545840262f4010100255
2906180d0d025506080f0f0255060c101002550600201d160a0d0d025516
0b20b8fff4401112120255200c1313025520180d0d025520b8fff8400c0f
0f0255201810100255201cba03e2001dffc0b6091002551d1f12b803e240
101340090e0255131400252509072c2c03002fed3fed3fdd2bed2fdd2bed
012f2b2b2b2b2bc0dd2bc410c02f2b2b2bcd31302b1bb106024354584052
1213140000200b0303252509071c701d01401d601d021d1f0b2c2c030b16
0c0d0d0655160410100655160b20141010065520040f0f065520020d0d06
5520202f2e290c0d0d06552906180d0d065506062f2e1112392f2bcd2b11
12392f2b2b2bc0cd2b2b003fed3fdd5d5dcd3fed1217393fddcd31301bb9
002fffc0b34747342fb8ffc040422b2e34602f7c047c058a04802faf2fc0
2f07402f802f02002f162a152b55055508542b960707480701202f370a47
0a560a9804a72aa02f07c02ff02b022020002021baffe0000bffe040453c
204f205e20660a6c207a209f009f20aa07b907c62a0b260813270c41121e
1344151d2716411c1e1d441f0020210b042c1500252509071f2c012c2c1f
030b1f000b210c20b8016740121560168016af16031f1690160216eb2950
06b8ffc0b3282e3406b8ffc0b7473506432e437f182b4e10f42b2b4dedfd
725d3cfd3c3c3c3c3c003f3ced723fed3f11173910f5edfc01f50010f5ed
fc01f531304379401a262b0408272526082920002b042920002807252001
2a052c2000002b2b012b2b2b8181005d3838383801715d00710172715d2b
2b5959250606232226353412333217353426262322072725331114161633
323717052335112e0223220706151416333202c743804a96e0f8c3794f0f
20181a2b0d01112d0f21161b2d0bfef02e063c632f58455bb06c5b67463d
fbc5c501474da99d481a102370fbdda1471c112371c901d84470394f68c8
cad7>/BAAAAA+TimesNewRoman AddT42Char 
3 722 72 <0002004cffe4035303b00014001d037db10202435458402808161415000c
0f100255000e0c0f1002550e0c0d0d02550e153040000120003000020000
10000200b8ffc0b41314025500b8ffc040111111025500000b1b25110700
0710070207b8ffc0b40f10025507b8ffc0b5131402550704b8ffd6b41314
025504b8ffcab71212025504310b0b003fed2b2bc42b2b5d3fed12392f2b
2b5d5d5ded012f2b2bdd2bc02fcdc031301bb10602435458401d158000a0
00b0000320003000400003000010000200000b1b2511070807b8ffc04024
1010065510072007b00703000760078007a00704079204a204b204030431
0b0b07081614b8fff440260d0d065514141f1e15000c0d0d0655000c0f0f
0655000e0c0f0f06550e160d0d06550e0e1f1e1112392f2b2bdd2b2bc011
12392f2bcdd0cd003fed5dc45d5d2b323fed12392f5d5d5dcd31301b4019
125f185d1960006014d6030519201c3917201c3916401c391fb8ffc0400a
434a34081f430d5d361fb8ffc0b32828341fb8ffc040532a2e341b061909
58135e165f175a185b1a07010309060709080c0515490689028c06870c8a
10851da302ab18b513d402d90fda10f402f3031312600760087007800789
09c107c80ff007080401070d84020309baffe00006ffe0404a3609460247
094f1f5402540962027202891389199913a409a40ab808b509b00ac702e7
02e00cf40a1408d007010007d007027107010007100720079007a007b007
06077d041400301615b8ffc040131239125f157f159f15df150415151bd3
040104b8ffd0b2143904b8ffe8b2133904b8ffd84048123904310b0b5c1b
011b25110707cc0816281b390f16016f167f168f160316f4141480080130
0890080230088f08df08031008400860087008b008e0080608aa0e150400
89000200b8032c4012300e400e500e03000e100e200e03f00e010eb8ffc0
4009434a340e431e434b182b4e10f42b7172724dfd713c10fd5d715d713c
10ed5d712b10ed003fed723fed2b2b2b7211392f5d4358b26f15015d592b
3cfd3c10f45d5d7172393130015d00383800715d014358b4060001020271
5971722b2b2b2b2b2b2b0072435c58b90007ffc0400b23390c402d390d40
2d3908b8ffc0b2283907b8ffc0b2283906b8ffc0b21b3907b8ffc0b21b39
08b8ffc0b21b3907b8ffc0b20a3908b8ffc0b20a3907b8ffc0b2093908b8
ffc0400e093915101939192011390d201139002b2b012b002b2b2b2b2b2b
2b2b2b2b2b2b595959130617163332363717060623220235341233321615
252126272626232206da016464875a852d1f15ca98a5ebf1b69ac6fd8701
a805101963365383023bcc747463781489e10101d9eb0107cbaa3a582438
4081>/BAAAAA+TimesNewRoman AddT42Char 
3 1714 73 <0001004f0000037a058c002b0208b1020243545840252d40101002552d40
0f0f02552d400d0d02551b2b01100e0601080e2901080d0d025501120eb8
ffea4012121202550e120d0d02550e0c0f0f02550e06ba03e2000903e240
0a0824251e1700000f290fb8011bb2120608002f3fedc010c03fcded10ed
ed012f2b2b2bc0dd2bc010c410c610c610c6c431302b2b2b1bb106024354
58b9000f011bb2120600b8011b401d2906241e17000829010c0d0d065501
060f0f065501021010065501120eb8ffd8400b0d0d06550e060f0f06550e
b8ffdab7101006550e0e2d2c1112392f2b2b2bc0dd2b2b2bc0002f3fcdcd
3fed3fed31301b403e8b2099159926034403440c48198503850c059a0401
2f2d7f21900690079f089f099e109e11b02d0910061007025f2a5f2b021c
080eb41e08922201b41e07b80308401f231e9f1ebf1e021e11242517012b
50100110302a2912110608070a101b011bb80152b38f2d012db802f6b201
2a2bb80110400d282901120f1110920f0f01240eb8ffc0b36060340eb8ff
c0b33a3a340eb8ffc0b33f3f340eb8ffc0b32431340eb8ffc040161c2134
900e01000e100e5f0e700ec00ed00e060e192cba0306030700182b4e10f4
5d722b2b2b2b2b4ded3c10f43c103c103c3cf43c10e65de472003f3c3f3c
3c3cfd723c3ffd11395d2f2b2b3130437940122527141626251526251628
1c002714241c012b012b2b2b81810172715d0072715d5959011114171633
331521353332363635112335333534363633321716151406232226262726
232206061515331501a61c253e53fddd29284219b2b258b57169583a341e
17334a1f1f262e401cec034cfda680222c2424284462025a483c89be7544
2d381e35216d13133167d6424800>/BAAAAA+TimesNewRoman AddT42Char 
3 2358 74 <0003003dfe4603db03af003b00490059039740821216509726993603002d
105b02762a765302002a062e06528b20043f374f5b6f377526705b8f048f
05831784188f358a3e83458f4b864f95179518994fb804b905b417b418c9
34c94bc05bd05be05bf05b1b1a201533103514361f5b05a7084a363f1b00
160336214a1b0019431211100f0e0d0c0b0a090913131409088025011225
b8ffdeb41214025525b8ffc0b3140c3f25b8ffc0400b120b3f9f25af25bf
250325b8019eb5582b80210121b8ffde400d12140255129f21af21bf2103
21b8ffc0b3140c3f21b8ffc0b3120b3f21b8019e4018904a014a40140c3f
4a40120b3f4a2c121202554a50140114b8010840136f08017f0801084011
14025508350699430143b80331400c194a0a2f1901501980190219bd02d2
00060009034d003c0331400a0607195101512c2c0f4dbe03300030001e03
300039004d0330401f1030016f308f309f300330180f100255300c101006
553035392e0380540154b8ffdeb40d0f025554b8ffcab41014025554b8ff
deb41010065554b8fff0400a0d0f065554251f280128b8ffc04016171a34
8f28014f287028c028d02804280e1010065528b8fff4b40f0f025528b8ff
ee4012101002552875205b305b405ba05bd05b055bb8ffc0401c0b0c345b
0e8f96460146101010065546312016010f167016cf160316b8fff2401110
100255160c11110255160c1010065516b802bd4013993f013f3130035003
02500301000310030203b8ffc0b3191d3403b8ffc0b30b0c3403b8fff4b4
1313025503b8fff4b70f10025503695a5bba01780021010ab189182b2bf6
2b2b2b2b5d7172ed72fd2b2b2b5d71ed2b72e4102b71f62b2b2b5d712b72
ed2b2b2b2b7110e4f42b2b5d72ed10ed10ed003fed723ffde610ed5d713f
10ed7210f42b5d5ded72102b2b2b5ded2b2b5d4358b4cf21df21025d592b
72f4ed5d2b2b2b4358b4cf25df25025d5972103c103c1112173911123939
111239011112393912393931304379407a4b573a4524351c1d1718010526
25323133313431030641264f262e252a265625541c011c3b1e1c004b354d
200042013f20003d053f1c00502d4d1c00522b5420014418461c01552757
1c0156571d3a1b1c011c1b3b004c314a20014b4a3536400243200001003e
043c1c014e2f511c0053295120004517431c00002b2b2b2b103c2b103c10
3c2b103c103c2b103c2b012b2b2b2b2b2b2b2b2b2b2b2b2a2b8181818181
8101725d00715d01710072435c58400a2e10120b3f351012392eb8fff0b1
1239002b2b2b590126263534363332173332161716151407060623231615
140623222706061514161716171617161615140706232227263534373637
363726263534360122061514171633323635342726010606151417163332
363534272627260135545acda08360c22b0e030605030f2b7738c4a54447
2c1f21301c70ce3d5d6f6a9cfbc1854b0b1135075f342b3901154a644434
504c624533fef82f303a64bdb4ab33349ae1014e29935988c44005060917
1a0a0506487080b614263914112007040305090d70527163925732361818
254209631f311f235e0287767a9e5742727a9f5a42fc8133582530243e7f
483416160406>/BAAAAA+TimesNewRoman AddT42Char 
3 3534 75 <0001000d000003f3058e0036028fb10202435458401d384012120255100a
110a080d0d02550a182412120255181a0d0d025518b8fff8b40f0f025518
b8ffe0400c10100255180e131302551826b8ffea401f1010025526213435
272d0121040c0c025521080d0d0255212d18121202552db8fffab40c0c02
552db8fff6b40d0d02552db8fff4b40f0f02552db8ffec400f101002552d
0e131302552d0120040f410a03e2001203e2002503e2002803e200270034
03e2400f3540090d025535360027111d2c0407003fed2f2f3fdd2bed10ed
edecec123939012f2b2b2b2b2b2bdd2b2bc010c4c63210c42b2f2b2b2b2b
2bcd2bc410c431302b1bb106024354584058341210100655351210100655
01200427343536001d2c040711270a02101006550a060f0f06550a0c0d0d
06550a18021010065518060f0f0655180c0d0d0655181838370121021010
065521060f0f0655210c0d0d0655212db8fff0b4101006552db8fff2b40f
0f06552db8fffcb70d0d06552d2d38371112392f2b2b2bdd2b2b2bc01112
392f2b2b2bcd2b2b2b002f2f3fed3fddcd111239393130012b2b1b402f38
402a350a38600d5d360f250f268038903804b038c038d038032b06015038
60387038903804403801200818291e11b8030f4011222d291e274a220a29
1e104a2321291e26b8030e402e2335272e41341e35440120273600001d2c
04072726261111100a19182409900a01b00a010f0a700a9f0acf0a040ab8
02bd40252d0021242e1f2d502d602d702d04802d902d02b02d01002d102d
c02dd02d042d6037a67f182b10f65d5d71723cfd3c10fd5d71723cfd3c00
3f3c103c103c3fed3f3c113939f5edfc01f52b2b2b2b3130437940141a1c
050806251b261c05191c0107081a071d1c012b01103c2b2b2b8181017172
005d015d712b2b5959011136363332161716151114171616331521353332
363736351134262623220607111416163315213532373636351134262623
22072725014d6f82414e701b130e0a3040fe3e1540320a031f4430316a4a
153946fe3a3d2314180f1f1a152f0e0112058efd627a45565c40aafebc57
20181c24242726104e0144965e2f344ffe1c5e2e1f2424130a3856033d9d
481a10237000>/BAAAAA+TimesNewRoman AddT42Char 
3 4350 76 <0002003c00000207058e000b00220249b10202435458b90024ffc0401d0d
0d0255120d080d0d02550d21181010025521180f0f02552113180309b8ff
eeb41313025509b8ffe0b40d0d025509b8ffd6b40f0f025509b8ffceb610
100255090d18b8fff4b41313025518b8ffe2b40d0d025518b8ffe0b40f0f
025518b8ffd6b5101002551820b803e240174f216f217f210321226f0001
0060060106400f0f025506b8ffc0b71313025506220613002f3fd62b2b5d
cd5d10dd5ded012f2b2b2b2bcd2f2b2b2b2bcd10c4c62b2b102bc4313001
2b1bb10602435458400d20121010065521121010065506b8ffc0b44b4b06
5506b8ffc0b44141065506b8ffc04019373706554006010006a006026006
0106000020212207130309b8fff6401c10100655090924230d0210100655
0d020f0f06550d0c0d0d06550d18b8fff0b41010065518b8fff6b40f0f06
5518b8fff0b70d0d0655181824231112392f2b2b2bcd2b2b2b1112392f2b
cd002f3fddcd3fcd5d71722b2b2b3130012b2b1b40199024016024702490
24a024f024052024502402402450240224b8ffc0b332323424b8ffc0b338
3a3424b8ffc0b32d303424b8ffc0b323253424b8ffc0402e191a3418291e
134a220d291e124a2321271941201e21440c190c1390060106390000220c
0713120a900901093903b8ffc0b2433503b8ffc0400f3f35036b0c0c0d19
0d2418402b3918b8ffc0401a363a34901801501801601870189018a018f0
180518b223b2a3182b10f65d71722b2bed3c103c10f42b2bed72003f3c3f
3c3fed7211123910f5edfc01f52b2b3130012b2b2b2b2b015d715d017259
590132161514062322263534361311141616331521353236363511342726
26232207272501292a3b3b2a2a3c3b7e193141fe43432e1b09071e1a1c28
0e0114058e3b2a2a3c3c2a2a3bfe21fd2056391c24241a3c550161952c20
190f2470>/BAAAAA+TimesNewRoman AddT42Char 
3 5044 77 <0002ff63fe46018f058f000b002901c4b10202435458400b281340101002
55131f0309b8fff4b41212025509b8fff4b40d0d025509b8ffe0b40f0f02
5509b8ffd8401310100255090d080d0d02550d0a0f0f02550d1fb8fffeb4
121202551fb8ffecb40d0d02551fb8ffdcb40f0f02551fb8ffd840091010
02551f00062927b803e2400c2840091002552829161bce10002fedcd2fdd
2bed10d6cd012f2b2b2b2bcd2b2b2f2b2b2b2bcd10c42bc631301bb69c1a
010619012bb8ffc0403f37350d2bb20d5d36402b502b902ba80ea81da02b
06202b502b802b03102b902bd02b031a0828272041271e28441913401010
0655131a092a191b20290c0716b8010e400d1000000c071bce100f9f1301
13b80167403c2a900901093903404735032e2b17171a0c0c0d0210100655
0d040f0f06550d080d0d06550d241f1f9020010f20016020a020f0200320
201010065520b8fff5400d0d0d065520b22a2bd121b2a3182b2b4ef42b2b
5d71723c4d10fd2b2b2b3c4e10456544e64df42bed7210ed5d003fed3f3f
b10602435458b006cd1bb49006010639ed725910ed3f3c39113901111239
122b3900f5edfc01f53130437940101c1e0e0f1d251c0f1f1c011e0e1b1c
00002b012b2b81810172715d2b2b00715d59013216151406232226353436
131114062322263534363332171616333236363511342726262322072725
01282b3c3c2b2a3c3c80c8a05b5831211a1b116121182e1609071e1a1c28
0e0114058f3c2b2a3c3c2a2b3cfe20fc66ebe4422323320d075725579102
8c972b21190f2470>/BAAAAA+TimesNewRoman AddT42Char 
3 5622 78 <000100110000040c058e003703bfb10202435458402b1a0c10100255190c
10100255200c0d0d0255110c0d0d0255010c0d0d0255200c0d1002551f16
0d10025526b8ffe8b40d0d025526b8ffe8402b10100255262136272e1f01
21080d0d025521040f0f025521060c0c0255212e0e131302552e16121202
552eb8fff6b40d0d02552eb8fff4b40f0f02552eb8ffeeb4101002552eb8
fffe40100f0f02552e1001111f04260a171a2528b8ffe8b40d0f025528bb
03e20026003503e240123640090d025536370026190c0c0d0d02550cb803
e2b6090c0d0f025509b803e2b10a06003fed2bed2b2f2f3fdd2bed10fd2b
c0c0c011121739012f2b2b2b2b2b2bdd2b2b2bc0c610c4c610c42b2b3130
002b2b2b2b2b012b2b1b40b90f391f3902120610010610019309950a900b
900c9b0f9a119b129a1f9f39b30a0a3919391a5f105f115f1f6c106f116f
1f9b0209eb1eed1f028009810ec603c60fe902e90fed11ef12083f113f18
3f1f38203f39460f720a750f082f022a10202520262f3938013810071510
5501521054200423105701570fe610f510054911481fc209c20ae30a0517
0916101f1d1f1f4502420f060b110f130d1a0c1d0f1e0e1f065303550453
0559105411541306190f1d1d1e1f530204b10602435458402f3618101006
55200110030a27353637007c0c010c7b0901090a0619270c0c3938012102
10100655210c0f0f0655212eb8ffe6b4101006552eb8fff0b40f0f06552e
b8fffab70d0d06552e2e39381112392f2b2b2bdd2b2bc01112392f002f2f
3fcd5dcd5d3fddcd111217393130012b1b4055100f01021112131310191f
1a1e192e291e2727220a02091e0a21291e26272336272f41351e3644002f
000b13101024201f14200102201f0f101030010214010102012000201f13
010427020f0a1010180a37000017b801ec404c180ccc0b0b0a0627262619
19180a0b300c800c02f00c01d00ce00c02700cc00c020c2f17179f180118
1a1f39013921242e00242f2f002e102eb02ec02ed02e05502e01802e902e
022e603839b80178b321a66e182b2b4ef471725d3c4d10ed10ed4e1072f6
5d3c4d10f45d5d5d713c003f3c103c103c3f3c10ed10ed3f3c191112392f
12393912173901103c3c870e2e182b0e7d10c487082e182b0e7d10c40011
12391810f5edfc01f52b10ed0110c02b10ed0110c0870e7d10c4c4070759
313001727271715d005d72015d5d5d5d5d5d00710071435c58b90010ffe8
4014120b3f1f281239012812391d400f391f280f3902b8ffc0b20b390bb8
ffc0b211390fb8ffc0b2113909b8ffc0b211390cb8ffc0b11139012b2b2b
2b002b2b2b2b2b012b59015d590111373637363534262735211506060707
131617161716331521353636353427011114161617152135323736373635
113426262322072725014fe94a0c082126018e526d41ebeb62223024193e
fe43261b28fee7192e4dfe2e4623150b0f0e201a152a110110058efc70d5
44120c0c141d022020022e3bd9fed77b212f0e0a242401151317330167fe
d0593818012424110b17215103429f471b112370>/BAAAAA+TimesNewRoman AddT42Char 
3 6752 79 <0001003d0000020f058e00150191b10202435458b90017fff6401d0d0d02
55140c06010701080d0d025501040f0f025501060c0c0255010cb8fff2b4
131302550cb8ffeab40c0c02550cb8ffe2b40d0d02550cb8ffd6b4101002
550cb8ffdeb50f0f02550c05bd03e2000803e20007001303e2400b131440
090d025514150007002f3fdd2b32ed10eded012f2b2b2b2b2bcd2b2b2bc4
10c410c631302b1bb1060243545840271312101006551414101006551314
1500000007010c0d0d065501021010065501040f0f0655010cb8fff0b410
1006550cb8fff4b40f0f06550cb8fff0b70d0d06550c0c17161112392f2b
2b2bcd2b2b2b002f3f3fddcd3130012b2b1bb79017c017f0170317b8ffc0
b33f463417b8ffc0403a393b340117b20d64365017014017501760177017
9017a017f017070c291e074a2201291e06272314270d41131e1444150000
07060a0001240d0cb8ffc0b33f46340cb8ffc0401a353b34900c01500c01
600c700c900ca00cf00c050cb216b2a3182b10f65d71722b2b3cfd3c003f
3c3f3cf5edfc01f52b2b3130015d0171012b012b2b017259590111141616
3315213532363635113426262322072725017b193447fe3f3f2e1a0e1f18
1a28110111058efb4156381d24241a3c5503409b471a10237000>/BAAAAA+TimesNewRoman AddT42Char 
3 7228 80 <000100110000063003af005703d3b1020243545840175940121202555940
0d0d02551711080d0d025511554c30b8fff4b40f0f025530b8ffeab41010
025530b8fff4400f13130255302b080d0d02552b313746b8fff4b40f0f02
5546b8ffeab41010025546b8fff440211313025546414741080d0d025541
040f0f025541060c0c0255414c14121202554cb8fff4b40f0f02554cb8ff
f6b40d0d02554cb8ffeab4101002554cb8fffa40190c0c02554c0a131302
554c2b040f0f02552b060c0c02552b37b8fff0400b0f0f025537100d0d02
5537b8ffd4400b10100255371c1212025537b8ffea401f0c0c025537020d
0d02553702131302553711040f0f025511060c0c02551120b8ffe8400b0f
0f025520300d0d025520b8ffc2400b10100255202a1212025520b8ffda40
0b0c0c025520020d0d025520b8fffc400b131302552016192f324548b803
e24020475455400c0c02552f55014f556f557f5503555606473118252c0b
073c2c0507003fed3fed2f2f2f3fdd5d5d2bcd10fdc0c0c0c0c0012f2b2b
2b2b2b2b2bcd2b2b2f2b2b2b2b2b2b2bcd2b2b2f2b2b2b2b2b2bcd2b2b2b
c410c42b2b2b10c4102bc42b2b2b10c6102bc431302b2b1bb10602435458
403c252c0b3c2c050b070507545556071831471102101006551120041010
0655202b060f0f06552b02101006552b3741060f0f065541021010065541
4c20b8ffeab70d0d065520205837b8fff8b41010065537b8fff8b40f0f06
5537b8fff2b70d0d06553737584cb8ffeeb40f0f06554cb8fff0b4101006
554cb8fff8b70d0d06554c4c59581112392f2b2b2b11392f2b2b2b11392f
2b10cd2b2b10cd2b2b102bcd2b002f2f2f3fddcd3f3f10ed10ed313001b0
0d4b5458bf0046ffe80045ffe8002fffe80030ffe8b51a18191818183838
3838383838591b401c3407d059ef16038059011159600d5d362b0d019059
01200820291e18b802fcb42237291e31b802fc400b224c291e474a221129
1e17b8030eb4232b291e30b8030db42341291e46b8030d403e2355274d41
541e55440829374d4039292808000725475657073c2c05252c0c0a0b0706
0405074746313018170a5917171a101124213020017020b0200220b80135
400f37292e2b24383037017037b0370237b8013540164d5741244c4c1f4d
504d02804d904d02004d104d024db8ffc0b61416344d605859b8025ab321
a67f18b80164852b2b4ef42b5d71723c4d10fd3c10f471723cfde410f471
723cfd3c4e456544e6003f3c3c3c3c3c3f3c3c3f3c3c4ded10ed3f3c1112
17390111123900f5edfc01f52b2b2b2b2b2b31304379401422240c0f0d25
2326240c211c010e0f220e251c012b01103c2b2b2b81810172005d2b0171
5d5959013637363633321617363633321617161511141716163315213533
323736373635113427262322060707171114161633152135323637363511
342726232207060711141616331521353236363511342726262322072725
33015064122d6833567c15678e4b497121160d0a363dfe3c133b21170a04
1b2756356b4c0202153a46fe314c390b05212c4f3635532d19314bfe3b3f
321a09071e1a1c270f01142b02ec640f262a645f784b4b553a7cfe765620
161f24241710231150018a702e4035480b2bfe4b5e2e1f24242424115201
8a7031401d2c37fe155a361b24241b3b55015e972c21190f2470>/BAAAAA+TimesNewRoman AddT42Char 
3 8454 81 <0001000c000003f703af003302d3b102024354584017354012120255300c
10100255310c101002550e080f1623b8ffea402e10100255231d24290808
0d0d025508040f0f025508060c0c025508162412120255161a0d0d025516
0c1313025516b8fff4b40f0f025516b8ffdeb41010025516b8ffee40260c
0c025516001d040f0f02551d080d0d02551d060c0c02551d291812120255
290e1313025529b8ffeeb41010025529b8fff0b40f0f025529b8fff6b40d
0d025529b8fffa400a0c0c025529001c022430b803e24009314009100255
31320dbe03e2001003e2002203e2002503e24009240f2432071a2c020700
3fed3f2f2f10ededecec10dd2bed11123939012f2b2b2b2b2b2bdd2b2b2b
c02f2b2b2b2b2b2bcd2b2b2b10c410c42b10c410c431302b2b2b1bb10602
435458405e2f1610100655300c10100655311610100655001c0224303132
071a2c02070f24080c0d0d065508021010065508060f0f06550816020d0d
065516021010065516080f0f065516163534001d0c0d0d06551d080f0f06
551d02101006551d29b8fff0b40d0d065529b8fff0b41010065529b8fff2
b70f0f0655292935341112392f2b2b2bdd2b2b2bc01112392f2b2b2bcd2b
2b2b002f2f3fed3fddcd111239393130012b2b2b1b403a35402a35083560
0d5d3630355035603570359035052d040140356035703580359035b03506
b035d03502b0350160358035c035031d0816291e0fb8030f40112229291e
244a2208291e0e4a231d291e23b8030e402e2331272a41301e31441c0023
3233071a2c02072423230f0f0e0a17162407900801b008010f0870089f08
cf080408b802bd401b29331d242a1f295029602970290480299029b02903
002910290229b8ffc04009141634296034a67f182b10f62b5d71723cfd3c
10fd5d71723cfd3c003f3c103c103c3fed3f3c113939f5edfc01f52b2b2b
2b3130437940121819030604251903171c01050618051a1c012b01103c2b
2b8181015d71015d71005d01722b2b595901363332161716151114171616
331521353332363736351134262322071114171616331521353332363511
342626232207272533014ba1924b6c20160e0b3142fe3b1340330a04414d
77760b0e314bfe3b1446310f1f1a1c270f01142b02edc24b563c7cfe7957
1f191c242427260f4f01777d7182fe1d5d161d1b242447640154a5481a0f
2470>/BAAAAA+TimesNewRoman AddT42Char 
3 9326 82 <00020045ffe403b903af000f001d020cb10202435458401c140c06101002
550c0c0f0f02550c0c0d0d02550c100b0b02550c1a04b8fff4b410100255
04b8fff440130b0b0255040c0f0f0255041725080b10250007003fed3fed
012f2b2b2bcd2f2b2b2b2bcd31301bb10602435458400910250007172508
0b1ab8fff4401b0d0d06551a04140c0d0d0655140c100f0f06550c100d0d
06550c04b8fff0400b0d0d065504041e0c0c1f1e1112392f11392f2b102b
2bcd2b10cd2b003fed3fed31301b404512801501a716b616c501c909c41d
d9090612e70a0148094516571585018c09890fd91b071f403235041f430d
5d369f1f01c615c91a02401f014908102500071725080b1204b8ffc0402b
120b3f4f0401400401d0040140045004600470049004b0040604ec0c4012
0b3f400c9f0c020c431e434b182b4e10f4722b4ded5d5d71722b4bb02853
4bb050515ab10c1e49b11f0449525a58bd000cffc00004ffc0001fffc038
3838594358bc001a0332000400140332e910e91bbc001a03320004001403
32ed10ed59003fed3fed313043794036011d12250e2602251c260a250626
110f1420001d011a2001160914200018071a2001130d1020011b03102001
150b17200019051720002b2b2b2b012b2b2b2b2b2b2b2b2b2b8101720171
722b2b71015d0143584011750275067a0a7a0e7a1278167518751c085d59
5d005d435c5840091c1011391b10113915b8fff0b10b39002b2b2b595959
013217161514060623222726353436361722060615141233323635342726
0200d07e6b76cf7fcf7a677dcc53356b429f82617e694703af9e87af7bfc
80a58bad7ef977413f9e7cc8fedea0c3f48c6000>/BAAAAA+TimesNewRoman AddT42Char 
3 9946 83 <0002fff9fe4a03ba03af002700390222b1020243545840293b4013130255
320a2a131302550a060f0f02550a1813190020032913080d0d0255132016
1313025520b8fffab40d0d025520b8fffcb40f0f025520b8fff4400d1010
02552003282b12040e061aba03e2001703e2400b1819182e250e36590607
27b803e24009004009100255000107003fdd2bed3fed2fed2f2f10eded11
121739012f2b2b2b2bdd2bc0c010c6c410c42f2b2bcd31302b1bb1060243
5458b90032fffcb50d0d0655320ab8fff040180d0d06550a0a3b3a032913
0c0d0d06551302101006551320b8fff6b40d0d065520b8ffee401b101006
5520203b3a0328060e270001190e2e250e0b365906070107003f3fed3fed
3f10ddcd11123939011112392f2b2bdd2b2bd0c01112392f2bcd2b31301b
407e0a3b430d5d36391049105b10891104862c013b2c3f3b4b2c5b2c6a11
6a2c73087911792c8408a507e908f9090d303b583359346c3404403b012f
08032829121320291e19862213291e1827230027214f271e004402122b28
03042e1036013659060702072e250e0b19180e32311f0a900a02600a800a
af0a030aeb200213b80167401b2020502170210280210100211021b021c0
21d0210521603ac24b182b10f65d71723c10fd3c10fd5d72ed003f3c3fed
3f3fed7211173910f5edfc01f52b2b030e103c3c3c3c3130437940202f35
070d082534260c26302535073220012f0d3220013309362001310b2e2000
002b2b012b2b2b2b2b2b81810171725d00715d2b59590325331536363332
171615140706232227262711141616331521353316373636351134262623
220705111417161633323736353427262322070602011a26478f4f8a5c71
8870aa4a36283217394bfe20193727131510231e18250134090e6d53643e
515c4058302f24033972d679616c84d4ed9b7f150f2dfee95e331e252501
160b316403625930180e7ffeaa6f233a584e66b9d2714e181200>/BAAAAA+TimesNewRoman AddT42Char 
3 10662 84 <00020044fe4a040003af001d002b01d4b10202435458401a260c0d0d0255
2615160d0d0255150601071e01080d0d0255010eb8ffe84011121202550e
1a0d0d02550e0c131302550eb8ffe0b4101002550eb8fff8b50f0f02550e
05ba03e2000803e24010071d060f1e12232518062959120b070e003f3fed
3fed1239393f10eded012f2b2b2b2b2bcd2bc0c410c42f2bcd2b31301b40
c01b2a0f0f06551b2a0d0d06551b2a101006551a0f1a1e561003012d600d
5d362b201827502d02402d802da428a02d04301a30213f2a382b4f10401a
40214f2a482b580f501a591e50215a2a5f2b6f10621a62216f2a7c10711a
7f1e71217f2b851a8d2b9c0f961a9c1e9621982a9e2ba816a61aab1cad2b
b916be2bcd2bda2bec2bfb2b2a202d732573288f1397139714c02d075313
0122080e291e07272201291e0627231b180f1e1f03231a29012959120b23
251d180707060e1b1b001f1f0eb80167402f001f0190010260018001af01
0301081010065501eb26311015501502bf15cf15ef150315101010065515
432c437f182b4e10f42b71724dedfd2b5d723cfd3c1112392f003f3c3f3c
ed3ffd7211173912392b2b31304379401824281317241726200028132620
00251623200127142920002b2b012b2b818101725d005d017172382b0072
2b2b2b590111141616331521353332373636351106062322263534003332
161736370311342626232206151416333236036b18334afe3213381d1418
5b884985d10114c33960263a358327643f70a0a3733b5c03affb6658321c
2525100b3952018a6c4ff2cbe9012520201c24fd2f01ae4b563cbec1b9c0
3300>/BAAAAA+TimesNewRoman AddT42Char 
3 11264 85 <0001000d000002b703af002801b5b1020243545840282a4013130255061f
171127040f0f025527181f0111080d0d025511040f0f025511060c0c0255
111fb8fff4b40f0f02551fb8fff6b40d0d02551fb8ffee4011101002551f
14121202551f0e131302551fb8fffc400b0f0f02551f011003181619bb03
e20018002603e2400e4f276f277f2703272807180c0307003fcd2f3fdd5d
ed10fdc011123939012f2b2b2b2b2b2bdd2b2b2bc010c4c62b10c410c431
302b1bb10602435458402301100318262728076f097f0902090c03071806
1f01110c0d0d0655110410100655111fb8fffab40d0d06551fb8ffeab40f
0f06551fb8ffeab7101006551f1f2a291112392f2b2b2bdd2b2bc010c400
2f3fcdcd5d3fddcd1112393931301b406f2002200f3202320f4002400f82
0407402a015f2a011f291e18272211291e17862327272041261e2744000a
0b2a111420100104188009010939100c010c590303000718170a5f060140
0601062e1f2a012a0011241f1f1f2001802090200200201020b020c020d0
2005206029a66e182b4e10f45d71723c4d10fd3c1072e47172003f3c3f3c
10ed72ed5d11173901111239390010f5edfc01f52b2b3130017271005d59
590115363332161514062322262322070607111417161633152135323736
373635113426262322072725014c73793748342423571512152d30130d42
3efe2b4622190a050d231a1f270a011503afcece432c27364514295efe49
4c271b24242416102311500163a03d1c0f247000>/BAAAAA+TimesNewRoman AddT42Char 
3 11824 86 <00010064ffe402d503af00310434b1020243545840273340131302553340
0b0b02550201181010025501180f0f0255010f1b1a08270c0b0b02552721
0fb8ffe0b4101002550fb8fff440320f0f02550f310708270f2104122b05
017905016c050105252f0101012a0719771e01631e011e25201a01601a70
1a021a120b003fc45d5ded5d5d2f3fc45ded5d5d5d1217393f012f2b2bcd
2f2bcdd4cd10d42b2bcd31302b2b1bb106024354584032210f2708042a16
1e122e05022a3107601a701a021a19124b05016b057b050205252a07441e
01641e741e021e25120b01210fb8fff2401a0d0d06550f0f33321a080e0d
0d06550827120d0d0655272733321112392f2bcd2bc41112392f2bcdc400
3fed5d5d3fed5d5d10c4c45d3f10c4123911123912173931301b4029092c
192c0212122e400b392c280b391814590c5a269b109424050a070a280a29
603370338033060f33b8012040870d5d36cb0dcb0ec424c425d723d624d9
2ce604e623e624e92c0b123f2c5d2c6e2d7d2c8f018f028f038015801a80
1b801c892d8f2e0d0f010f020a03090c061c0a2cc822c923081c03161412
1c161d19291b2c9909990a9b20932393240b122b0d282c4a2c4f335f3378
29782c860ea823af33e803e61c0c2908311e00bd021e011f012f010201b8
012bb200bd2eb8011a40112a181e19bd1b1e1a1f1a01101a201a021ab801
2bb219bd16b8011a4022121224230d0b040f2724230d0b04051e01c7002e
2f2a31000005252a071a7e191918b803464014162f1e25120b02cc120101
12cf21df21ef210321b80314400b700f01600f700f900f030fb801364019
271a192e1f0801082c9f270160277027802703202730270227ba01200032
0120b14b182b4e10f45d71724ded72f43c10fd5d71fd5d4358b2ff21015d
59392f435c58b2ff01015d59ed003fede4f43c10ed3fed3c103c10e410ed
1112173901111217394358400a242323240d0b140d0d0b870e2e2b0e7d10
c459180010ecf4ed5d720110edf4ed0010ecf4ed5d0110edf4edb1060243
5458b42e20090d34002b5931304379401c28291f20101106071f11211c01
0629081c0020101e1c000728051c01002b2b012b2b81818181015d435840
09fb07f610f611fb28045d5901720071005d435840199f019f029f039f0b
9a0d9015901a901b901c992297239f2d0c5d595d2b017100722b2b435840
0b2f232f248b2c9b249b2c055d59435c584011282019390928193901400a
3902400a391bb8ffc0b20a391ab8ffc040190a392e400a392c400a392c40
09390c101e123f0e201e123f0eb8fff0b21b390eb8fff0b2193924b8ffe8
b2133923b8ffe8b213390cb8ffe8b613392c1813391bb8ffc0b212391ab8
ffc0400f123901401239024012392c20123924b8fff0400f0f392c180f39
03100d392e400d3923b8fff040120d390c100d392c200d392c1811392c18
1139002b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b
2b2b012b2b59005d59590111232626232206151417161717161514062322
272623220723113316163332363534262427263534363332171633323637
02902126775c4656201f5f92cbbd75546c2115170d21211c9e62455761fe
de2d2d9b7b364d331110120c03affec8936a4a2d3828292e4763a27d991e
0a1a01478c8e5139455e903a39577198170f0e18>/BAAAAA+TimesNewRoman AddT42Char 
3 13044 87 <00010014fff1023c04c1001b01fdb1020243545840251d40121302551d40
101002550b0c18121202550c15130105131812120255130e1313025513b8
fff8b40f0f025513b8fff4b40d0d025513b8fff0400c10100255130b082c
0f161404b8011bb2000106003fcdfdd0cd2fedc4012f2b2b2b2b2bddc010
c62f2bcd31302b2b1bb106024354584019170c10100655160c1010065515
0c10100655160c101006551bb8ffe8b4101006551ab8ffe8b41010065519
b8ffe8401410100655700b010b0f1b01156914014914011404b8011b401c
0106082c0f0b1b0105021010065505080f0f0655050c0d0d06550513b8ff
eeb41010065513b8fff0b40f0f065513b8fffab70d0d065513131d1c1112
392f2b2b2bdd2b2b2bd0cd003fed3ffdd05d5dc010cd10c45d3130012b2b
2b2b2b002b2b1bb9000dffe840410c395f015f02023f1d99119919bf15bf
16b819e819079f1d01891a014f0c4f0d5f0c5f0df5180506181518271803
161518191a030118191a03141ba00103153004b8011b401c010330020201
060c35082c0f0b16cf15df15ef15031565141bcc000bb801ec402c200c01
0c2e2f1db01d021d000101040405241450130180130100131013b013c013
d013e0130613601cab89182b10f65d71723cfd3c103c103c105df45ded10
ed10f45d3c003ffde43f3c10ed10edfd3c10e40111173900111739123931
3000715d0171725d00722b59590111331523111416333236373306062322
2626351123353636373637014ad6d63328213e11272380442e582a913773
2d172904c1fed346fdae593e29286263335f63026821166948266500>/BAAAAA+TimesNewRoman AddT42Char 
3 13642 88 <00010002ffe403fd039400250230b1020243545840162740121202550801
080d0d0255010b20281212025520b8fffc400b0f0f0255201e0d0d025520
b8ffe4401310100255201a080d0d02551a121c1212025512b8fff8b40f0f
025512b8fffab40d0d025512b8fff4b5101002551224ba03e2001703e240
0e1825060b200e18061d2c0e0b0708b8ffc0b509100255080a002fdd2bcd
3fed3f1239393f10edec012f2b2b2b2bcd2b2f2b2b2b2bc0dd2bc431302b
1bb1060243545840570740086008700803080a0b200b180e242517182506
18061d2c0e0b0b010810100655010a0f0f0655010c0d0d065501201a040f
0f06551a04101006551a0a0d0d06551a1208082620080f0f065520060d0d
065520202612b8fff2b41010065512b8fff6b40f0f065512b8fff6b70d0d
0655121227261112392f2b2b2b11392f2b2b11392f10cd2b2b2b10cd2b2b
2bc0003fed3f3f10cd10cd111239393fdd5dcd31301b40350127600d5d36
202760277027b02704340b371f3a20481f4820051a08134f1e182723214f
1e25272308270141071e0844200b251d08b8014540130a00252519191806
1d2c0e0e0a0b0a0b0b2120b80167400e00b001010f0170019f01cf010401
b802bd402512191a241212501390130280139013b01303001310132013b0
13c013d01306136026c27f182b4e10f45d71723c4d10fd3c10fd5d713cfd
3c3c103c003f3c10ed3f3c103c103c10ed11123939f5edfc01f52b2b3130
437940101b1c0f111c0f1a1c0010111b101d1c002b01103c2b8181005d01
5d2b59590111141616333237170523350606232226263511342626073521
11141633323637113426273503630f21161f270efeee2d767c454d712c1c
37480141593f2b6d4b395a0394fdd59f471c112371c28042598c80019941
321b0125fd9b8050364c02074e370225>/BAAAAA+TimesNewRoman AddT42Char 
3 14318 89 <00010011ffe403ed0394002002c1b10202435458b60909001a120614be03
e2001103e2002003e2000203e2b10006003fededecec3f2f1239012f3130
1bb106024354584031180a091b080909222109001a0b1416101006551413
06112a10100655111206021610100655020106201610100655200006003f
cd2b3fcd2b3fcd2b3fcd2b3f1239011112392fddcd10ddcd31301b400912
530a58185b190319b8ffd8b20b3522b8ffc0406115351419141a2309220a
2111201224182019201a3a09390a3a12391835193a1a4a084909440a4518
4519491a69089c0899099d1a9a1b9f22a900a808a509a219a21aa81bbe08
b509b60ab618b719ba1abb1bc022d518f60af618fb1a2d9f090122b8ffc0
b332603422b8ffc0b32b313422b8ffc0b31e293422b8ffc0b347473422b8
ffc0b327273422b8ffc0b323233422b8ffc0b311113422b8ffc04040191c
340f227c007201720270057c20810585118f22093a08340a3418391bc606
c021d81a07880a891887190337124818021318141e13001b201e00120a11
1e12b8ff86402c091a192018191930090a1409090a1b1a1a240908140909
08070605040408021e01131212010100061a190b18b8011d40125f0a0110
0a240a9f0ab60ad40a050a7d091bb80167401040062fa008b908ce080308
7d0919751abb011b00200009ffc0b30f123409b8ffc0b3191d3409b8ffc0
b2323509b8ffc0b70c350009c0090209b801bfb610220180220122b8ffc0
b3191d3422b8ffc0b60f133421ab89182b19102b2b7172f45d2b2b2b2b1a
fd18e61910f45d18f41aed1910f45d7218ed003f3c3f3c103c103c10ed01
111739872e2b0e7d10c487052e182b0e7d10c42b180010ed0110c00010ed
0110c00010ed0110c03130015d5d5d712b2b2b2b2b2b2b2b005d015d2b2b
0172435c58b50a20160d3f08b8ffe8b7160d3f09240b3918b8ffe0b21339
0ab8ffe0400a1339082013391b201339012b2b2b2b002b012b2b59595913
211523220615141713133635342726262335211506070607012301262627
26271101af1c272915d5d617080b2234012b3414231cfebb29feb916281f
113203942526202330fe06020d381d0e090f0b252504111e46fcee030536
2f100908>/BAAAAA+TimesNewRoman AddT42Char 
4 0 90 <0001000dffe405b40394002c03cdb10202435458b626211e110e022cb803
e2400e00092618080428251f060f060006003f3f3f2f2f173910fdd0d0d0
d0c0012f31301bb10602435458b90026ffe840440d0d0655181c0d0d0655
081c0d0d065518101010065508101010065508182609040028211e110e02
792c012c00752501250b752801280b1f060f0600062c2c2d21212e2d1112
392f11392f003f3f3f3f5d3f5d10dd5dd0d0d0d0c01112173931302b2b2b
2b2b1bb1122eb8ffc0401c3f351627201020112527202e5f2e6909702ee9
25e928f825f8280c2eb8ffc0b213352eb8ffc040c81b1f34212e2e296436
1d19191f1b23102e040a261d262c2639265517a717a718a726080b253724
37274f004c014d074908472446274d284d298807801080118d2588288829
802e9a109417a718a725bb10b925b928bf2ec825c828d925d928d02e1f00
050407061504170925072709280629351743104311500552075618522989
0b8f1088188919892388258826802e17870986178726030d095901771077
110409090826262725250a0107021e011017111e102023211e2000292c1e
000f0a0e1e0f1f191e1e1fb8ff86b308282720b8ff7d4040182524200807
080907242928142929282627262527300809140808091815181915240a25
140a0a25232424301819141818192926231918170a0908070a002821bb01
ec0020001e01ecb31f010f11bb01ec0010000e01ec400a0f0f10101f1f20
200002bb01ec0001002c01ecb301000618bb016a0025000801a6400f2840
2725252424280b20fc0f650a01b801b1b4c000652923b801084015401b2f
501901a01901bd19cf19df19031992242f18b8011bb7200f250110250125
b8ffc0b30b0c3425bb0110002600150167400c400a2f5f26014026802602
26b801ecb4097d272f08ba011b0008011b400a200028018028f0280228b8
ffc0b50b0c3428a007b80167401b5029018029010029102920294029b029
c029d0290729602dab89182b10f65d7172edf42b5d71191aedfde4f4ed5d
7118f41aed1910f42b5d711afde4f45d717218e41aed10f41aed10f4ed00
3f3c103c103c1a10ed10ed3f3ced10ed103c103c103c103c10ed10ed103c
10ed10ed1112173987052e2b0e7d10c4870e2e182b087d10c487052e182b
087d10c4870e2e182b087d10c42b2b180010ed0110c00010ed0110c00010
ed0110c00010ed0110c00010ed0110c00010ed0110c00710083c083c3130
015d5d71015d005d01722b2b2b015d2b435c58b52610140c3f24b8fff0b3
140c3f13b8ffe0b21d3917b8ffe0b21d3917b8ffe0b2143917b8fff0b217
3925b8fff0b2153917b8fff0b11539012b2b2b2b2b2b2b2b595959132115
060615141713132726272627352115060706151417131336353426273521
1506070123030123012626270d0180352111c4c5341827163c01b4481e14
08d0c114273901215729fece29e5fef525feda1d383c039425041e1c1f2c
fdf101ad873c170e032525031710231415fdf201fb3620131e0225250d69
fceb0249fdb7030249330d00>/BAAAAA+TimesNewRoman AddT42Char 
4 1122 91 <0001001b000003e70394003803f2b10202435458400c260a183426042d00
1c1f2c2fb803e2b42d13100238b803e2b6002d1e11060006003f3f2f2f10
fdd0d0c010fdd0d0c011121739012f31301b408712450a018f0d8f0e8f11
87268734d60bd617da27da33090f2e260a250b240c720a750be632071c3a
2e0f5a36042e3f053f103f1138263f283934303a490b4f104f11461e4926
4c284b34403a56195625503a75077f0b7f107f117f167f1795079f109f11
a718bb261e0e050f100f110f2c1f101f111f2c290a29172f3a0a103a5509
5a36503a04b10602435458402413100279380138001c1f2c762f012f2e26
34180a04002e110600061e2e1d1d392e2e3a391112392f11392f002f2f3f
3f1112173910dd5dd0d0c010dd5dd0d0c031301b40a22618181917161627
3434350a0b0c0c33180a0907071926343534333525128f162f110111350c
0d0d160c1d7d19501e011e2f256f237f2302238f23012319252e2e39332d
f229292733500001007d35013505050725190707243525143535250c1627
2730330c1433330c35342618090c17332725190b382f26180a030c340735
0f1c011c1f1f2c2f2f2e131002381e00121111010100062e042d012d2d1e
1e1d0a0cb80145b56f1601162e25b8010eb320190119b8ffc0400c103540
19b019e019f0190419b8ffc0b30f123419bb0236003300070167b2352e27
b80108b300330133bb02c10039003a024db321cd89182b2bf65dedf4ed10
fd2b5d2b71edf45ded003f3c103c105d3c3f3c103c103c10fd3c3c3c10fd
3c3c103c5d011112391117390011121739870e2e2b870e7dc4870e2e182b
870e7dc4011812397d2f18ec10e45d1112392fe41112392f1112395d2f5d
10e45d10e41112392f107cec5d10e40708103c0e3c870e103c7dc4c4870e
103cc408c4070e103c083c0e3c59313001725d5d2b005d01710071435c58
b9000bfff0b20a390bb8fff8b7093917201e123f0bb8ffe8b31e123f15b8
ffe840091c113f0d401b103f18b8ffe8b31c113f18b8ffe84013170e3f05
40120b3f0718120b3f3640120b3f3ab8ffc0b7120b3f29280f390bb8fff0
b60f3925200f390ab8ffd8b20f3907b8ffe0b20f3932b8ffe0b60d392520
0d3907b8ffe0400f12392620123926201139252011390bb8ffd8b20b390a
b8ffe0b212390ab8ffe0b211390ab8ffe0401b0d39101812391118123917
40123910100f3911100f392c40153913b8fff0b2153916b8fff0b2153912
b8ffc0b215391ab8fff04013153936081539283014392930143911081639
09b8ffe0401b163929401139294015393240153932201139172011390b20
113912b8ffc0b11139012b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b2b
2b2b002b2b2b2b2b2b2b2b2b2b2b2b2b2b2b012b2b2b2b2b2b2b2b002b2b
2b2b59591321152206151417161717373635342623352115060706070713
161617152135323736353427270706151416171521353637363737272626
231b01af2921230b16414b4822260136312431557de4544839fe502d1913
408693442d2dfed5241b265ac0ae4a513d0394251c17183210226868631a
151d252503182272a7feb87931032424140e17175dc4c45b111827022424
05141d77fffc6c37>/BAAAAA+TimesNewRoman AddT42Char 
4 2300 92 <0001000cfe4603f4039400320222b10202435458401409092b2a03007827
01271d120614181010025514b803e2b611181010025511b803e2b6021810
10025502b803e2b632181010025532b803e2b10006003fed2bed2bec2bec
2b3f2fcd5d121739012f31301bb10602435458401e092b001d1411027a32
01320012060006237a2701271d0f141433000034331112392f11392f003f
dd5dc43f3f10dd5dd0d0c0111239393130b0104b5458bd001bfff80019ff
f0001afff0b10a1038383838591b40ab0910120b3f0e2b95290213342e16
64368305850602090905120819081a092b141a26092412241a262b380136
12351b47126809680a6919661a631b682c7808790a7919771a741b782c89
0a891998009809971a962bbb00d034e506230909082b2b2c2a2a0a010802
1e011319141e13002c321e00120a111e12260820191a1a302a0a142a2a0a
2c2b2b24090814092b2a09082b2a1a09040a082c2b2a1a190a0908082313
12120101000627b8ffc0400e120b3f272f23391d0f3417171a19b8010840
1b8f0a01df0af00a02600a700aef0a030a7d3f094f095f0903097d08b801
0e401d2bd60f20010f209f2002208f5f2c012f2c3f2c022c193334a921a6
7f182b2b4ef45d724de45d71e4fdf45df45d5d71fd4e456544e6003f4dfd
e42b3f3c103c103c121739011112173987082e2b0e7d10c4870e2e182b7d
10c401111239180010ed0110c00010ed0110c00010ed0110c00010ed0110
c00710083c083c3130015d01712b005d012b595913211523220615141713
133635342726262335211506060706070106062322263534363332171633
32363737012627262726270c01ab152d2d21dfcd110708222b012a252818
0919fe8b36af513b4c37302139280a1e472441feb70f2119101733039425
271d2745fe3201fa292812090b0d25250418210e3ffc6e8588442c2a3316
0f3e599f02b31f2e230c100c>/BAAAAA+TimesNewRoman AddT42Char 
4 3002 93 <000100290000036c0394001501a9402f12080418049f049f0d9f0ea904b8
04079f17010d17750d31365000580f5015031b04170e130f5e04520fdf04
d00f07b10602435458402801031716030f020e050c4b05017b0501500560
050205300c06440f01740f015f0f6f0f020f30020a003ffd725d5d3ffd72
5d5d11123911123901111239391b400900f6101041151e000bb801244032
0505b40a1e0b040e0f0f24030414030304030b02040f010c0e170d030f02
0e0450050105300d0c06105f0f010f3001020a0fbb023e000e0004023e40
2c03012e9f0001002e500d01300d400d700d030d1a2f173f174f1703170c
2e0b3500020102191617a121cd89182b2b4ef4714df4e44e105df65d724d
f45de410e410e4003f3cfd723c3f3cfd723c391112390111123911123939
111239872e2b877dc4180110edec0010f50110edec0010f5593130017200
722b5d015d435c58b9000effd040091e123f03301e123f04b8ffc0400d1e
123f0f401e123f042416390fb8ffdcb61639042814390fb8ffd8b6143904
7012390fb8ff90b61239041815390fb8ffe8b6153904180f390fb8ffe8b1
0f39012b2b2b2b2b2b2b2b2b2b2b2b002b2b590103213501212206070607
2337211501213236373637035c0bfcd80260fed4613c131b0428060300fd
9a014e694b17100b0119fee724032a1923324afe25fcd4232c206700>/BAAAAA+TimesNewRoman AddT42Char 
4 3510 94 <0001011bfe460349058e00260082404c78037028025b0354126b03641264
137412061e0b686f0a010a0a0b0a15681411006801131ead0b0a7c043824
2418073821210e381b3e113818b315000101141420153015401550157015
0515ba01250028016bb17a182b10f65d3c103c103c10f4edf4ed3c10ed10
3c10fdf43ced003fed3fed1112392f5ded393130005d015d011526263534
363534262735363635342635343637150606151416151406071616151406
1514160349a7d12e796b6b792ed1a7756d2d949390972d6dfe692317e189
48bf35487d0e290e7c4935be4988e216231c7f4c3bc14465be3435c26544
c13b4c7f>/BAAAAA+TimesNewRoman AddT42Char 
4 3754 95 <000100a1fe4600f4058e00030053400c00056a116b36900190020202b801
db400903000517171a000001b80327400d02022003300340030303190405
bc011f0021006a010000182b2b4ef45d3c4d10fd3c4e10456544e6003f4d
ed3130005d012b13112311f453058ef8b8074800>/BAAAAA+TimesNewRoman AddT42Char 
4 3864 96 <000100b1fe4602df058e00260080404a771201250829090254035b126502
650376027503f81d071e0a68200b01d00b010b0b1400680111156814131e
ad0a0a0b7c110438242418073821210e381b3e113818b314010000141415
b80125b327d2dd182b10f63c103c103c10f4edf4ed3c10ed103c10ed10f4
3c10ed003fed3fed12392f5d71ed393130005d71015d1335161615140615
141617150606151416151406073536363534263534363726263534363534
26b1a7d12e796b6b792ed1a7756d2e959390982e6d056b2316e18a48be35
487d0e290e7d4835bf4888e217231d7e4d3bc14366be3435c26544c13b4c
7f00>/BAAAAA+TimesNewRoman AddT42Char 
4 4106 97 <0001002c018e045702a60017006e401d0a03050f1a03150f2903270f3a03
350f7613090910041504010c0d3415b80327b6047c0901003409b8032740
221000989001a001023001400102000110012001030145301901190c980d
451858de182b10f6ed105df65d5d5ded002fedf43c10f4edf43c01111739
3130005d013306062322262726232206072336363332171604333236042a
2d048c652e6add9a414660142c06885c2c2e680153454b6602a382931f5a
405661878f0e1e916000>/BAAAAA+TimesNewRoman AddT42Char 
4 8492 135 <0001007001aa026603a0000b002eb9000601bab600060d17171a03b80153
b309190c0db80153b3219ca4182b2b4ef44dfd4e456544e6003f4dfd3130
013216151406232226353436016b6893936868939203a093686893936868
9300>/BAAAAA+TimesNewRoman AddT42Char 
5 4868 188 <0001ffe9ffe803dc0568002f00d3b5292010113425b8ffe040091011340d
200b103408b8ffe0b30b0d3426b8ffc040281011342624282840090b3428
282a1f0f130e0e180a2f1f40001e1e40090c341e1905180419190a2ab801
06b224050ab8032f4030130d06012e030305040403002f2f03281b270e1b
0f31003140310240316031a031e031041a171d2004031b1e181f1903b901
0f001b2fedd63cdd3c111217395d7110d6edd6ed11392fcd11392fcd1117
39003fed3fed11392f3cdd3c10c62b00103c1a18dd3c1112392f12391112
392f2b001112392b3130012b2b2b2b012106152107211617163332373637
170607062322272627233733353437233733363736333217112302212207
060721034ffdc203022817fdf1084c5997865a36531f564673a1e67e6713
65174a02631754228093e5aba9271afeed9e5c4716024f02e12a294ed38d
a445297314883a5fbf9cfd4e101e254eed9ab258fed50141a782ce00>/BAAAAA+TimesNewRoman AddT42Char 
5 6168 195 <ffff00cbfeab01f500c80106000f5d00000f400900700f010f18c1482b01
2b5d3500>/BAAAAA+TimesNewRoman AddT42Char 
5 1150 166 <00010002fe5103e7056b004200bf4034092b1f01192b6829a540e901e603
070305422302000124420522230221294205052421291421212921052942
04093d702d19250fbb010e00090033010e40422d01000024302302030322
2323092d090e2324010221052942080c362c307500440140446044a044e0
440444162c12af000c100c200c300c400c600c900c070c4d43b8020ab17f
182b10f65deded105d71f6ed121739003f2f12392f3c3c103c10fd3c103c
10ed10eded10ed121739870e2e2b0e7d10c40f0f0f3130015d0133072302
030207062322263534363332161514070615141633323736363736133613
233736363736373637363332161514062322263534363534272623220706
070602afb211ae34785e6f545938422f1e1a270e0a0e0b14111e3a1f0650
0774b10f6333111a22494342513e4b281c1a2516090911201a230b1b036b
42fef3fe49feab6c533d2c2732241416100c07080d0a115e821601892301
df420711172264d43c3b422e232a23151025080b080718213379>/BAAAAA+TimesNewRoman AddT42Char 
5 6202 196 <00020043fec4035300c80017002f008b403d9c1b9c2ea92fb82fc82fe92f
067a0e75178a0e85170418191c270001040f21082a0c18b62a40240b00b6
12400c0b313f1c3a502d010f2d1f2d802d032db8012a400fa0270127c304
3a0f151f1580150315b8012ab30f193031b80174b321545a182b2b4ef44d
fd5dedf65dfd5d72ede4003fede43fede411123939011112393911123939
313001715d13353636353427262322070623222635343633321615140605
353636353427262322070623222635343633321615140673653f0a0b0d0a
1616162a3c4d37426b870163574d0a0a0c0d161711293d4a36446c85fec4
2a395d3d1c0e0e08083c2b3048725769ae242a2d653b230e0d08083e2b30
46755564ad00>/BAAAAA+TimesNewRoman AddT42Char 
5 1844 171 <000300e6ffe4071a00c2000b001700230097407020254025020040060c40
1218401e1e1212060b1b402140433521403f359f21df21020f214f218f21
df21046f21bf21ff210321d80f401540433515403f359f15df15020f154f
158f15df15046f15bf15ff150315d8034009803a351f095f09024f09df09
028f09df090209f824e5dd182b10f65d71722bfdf65d71722b2bfdf65d71
722b2bed003f3c103c10ed10ed10ed3130015d2532161514062322263534
3621321615140623222635343621321615140623222635343601552f4041
2e2e414102d92e41412e2e414102d92e41412e2e4140c2412e2e41412e2f
40412e2e41412e2f40412e2e41412e2f4000>/BAAAAA+TimesNewRoman AddT42Char 
4 6192 130 <00010065fe5b039b057b003f009b400d70410168237823882303053d3d41
130354000501fd003a0342002903420008034200180342000c0144001201
44002f01440035014440113201220132063a670867296718673dcf32ba01
3000240144b205cf0fba0130001e01444011006701672040210121bb4041
95219ca4182b2b19f45d1aede5ededededededede5ede5003f183f2f1910
edededede5e5e5e5ede400103c31300071015d0123020326273636370607
062322263534363332171617161726272627263534363332161514070606
0736373637363332161514062322272626271616170602020c25041c1530
332c06414369302d383b2c19150b5e3c480106071736422e2a43080a4704
473d63101617303b3b2c376e302a29052d323026fe5b01b4010ac7b32c62
5f071c2c36292a390603291a0429151f3780423a484b371e1e27ad460618
270406382a28382f140a035e6629b7fe9700>/BAAAAA+TimesNewRoman AddT42Char 
5 5422 193 <0001008bfe460375058e007d01394014407f707f02807f01410949030645
490645030941b801a1b2097c2d41120342001d0342003e0342000c034200
3801440032014400110144001701440014001402e1b325037c49411301a1
00000342004c0342006e0342005c03420056014400500144007301440079
0144007602e1401067012514760c673e671d672d6741cf09410c01440022
014400280144001401ae0025006a014400640144400b49cf00674c676e67
5c6703ba0144007601aeb367353453b801ae400a2025cb40670167bb7e7f
b80137b3216a7a182b2b19f45d18e6191afd18e41910ededede5ede5eded
ed10edededededede5ede5002f2f182f3f19fdedededede5e5ededede410
fd10edededede5ededede4ed111239390111393900103c103cb106024354
58400b064549034109450606765301111217392fcd59313001715d011616
170606151416170606073636373633321615140623222726272627161617
161514062322263534363736370606070623222635343633321716171617
26262736373635342726273636370e022322263534363332171617161726
272627262726353436333216151406060736363736333216151406232227
26260212082432322c2a3430250927233655312934342829562e1c152908
0a10323a2b2a3a0d2118072d33314c252932352b2849311b152b0925322e
141f20132e30250b29238a31263231262e553319122702060b221502043a
2b2b360b3d062c26394c322832342a2f4f332803d0424028498e6b64894d
294140060a16233226283425130705023d27246e362d3c3e2e1735584144
020c16223127293320150605023d3f273d3b5b7376573633244145030937
3226253122150605032b1428593507121b323d3a391f288d510309182131
26273221170a>/BAAAAA+TimesNewRoman AddT42Char 
5 8482 214 <0001003c041e026f05690006005840217a04c60402750073017704700570
06c403c604d704e7040902030602d500060106b8012d401704cf00000404
0f020102947f0601061907089421545a182b2b4ef45d4dfd5d392f003fed
ec5ded1239393130015d005d13331323250723f9b8be1ffeefe51e0569fe
b5d5d500>/BAAAAA+TimesNewRoman AddT42Char 
5 6478 197 <00070041ffc907bd056b000300120024003300440054006501ad40274f67
806702a906a60da911a927a62ba932a74fb906b50db911b927b52bb932b5
4f0ee808030202b80327400f01001401010002190f0029411d460bb80159
400a13460404030003344625b80159b73d462d2d4d554645b8015940195d
464d4d0202010b493862fa593851ae293841fa41fa393830b801c6400d66
083821fa19380f1966545a182b4e10f44dfdf6ed10f6fde6f6fdf6fdf6ed
003f3c103c10edfded103c10edfded3f3c3c10edfded0111123911123987
2e2b7d10c4313018437940b4056557255326472564265b264f254b266061
5f6102063738363802063226272543263b262b263f251718161815180306
1126062523261b260d251f255654591d006546621d015c4e591d005e4c62
1d013533391d004426411d013c2e391d003e2c411d011412191d00240521
1d011c0c191d001e0a211d015852551d016348551d015a505d1d00614a5d
1d003831341d014228341d013a2f3d1d00402a3d1d001810131d01220713
1d011a0e1d1d0020091d1d00002b2b2b2b2b2b2b2b2b2b2b2b012b2b2b2b
2b2b2b2b2b2b2b2b2b2b2b2b2b2b2a2b2b2b2b2b2b2a2a2b2b2b2b2b2b2b
81005d015d01012301213216161514062322262635343636172207060706
151417163332373635342726013216161514060623222635343636172207
060615141716333237363534272625321616151406062322262635343636
172207061514171633323736363534272604c4fc345903ccfcf64d884daa
744a8b4f4e87471e142112162f21312e21313023027548884f4e8d4771af
508d421f1723262e20303121313220026a44914d488f4949894d4c923f32
1e2d2e21321e1722272f23056bfa5e05a25aac68a9c158a86b68af563510
1d3a4d89b94932344ebfb34934fd6b59ac646da85ac3a869ae5635131d7d
93b44731324bb2bc4e333557a56579a35b59a56675ac53352f49c4b74732
131d8396aa463300>/BAAAAA+TimesNewRoman AddT42Char 
5 9402 226 <ffff0080ffe104050701022600360000010700df00df019800234014011f
3b010f3b019f3bbf3b023b2e78482b01013ab902ac0029002b012b5d7172
3500>/BAAAAA+TimesNewRoman AddT42Char 
5 5226 189 <00010077fff8023303a60005003f400d00010a03040701ad000004ad03ba
0125000501a1400c000210022002300240020502ba010b000601aab1a418
2b10f65dfdf6fd3c10ed003f3c3f3c3130052301013303023339fe7d0183
39f40801d801d6fe2a00>/BAAAAA+TimesNewRoman AddT42Char 
5 2278 175 <0002004bfff006e305580036004801684063700570067f077f0880058006
8f078f0808671a771a971aab33ba33c71a0629163a16871adb16042f0807
210b0b1f081b07062102021f051b061a0d191f44210201230c0c0b100b40
0b700bdf0b04800bb00be00b030b1b2c3ca5290330002f102f022fb802d3
405f2e3600232e2d0212131819e81a13a51a1b2b1d1b084428210908ac07
0705ac10063f064f065f067f0605067630ac2e2b1f2f017f2f8f2f022f2f
011f2f012f6c18ac2019df19ef19031953404a014a000d22375048904802
3f4801a0480148b802df400b403c102520250225494964b9018700182b10
f672fdf65d71723cfd3c105df45dedf45d5d7172e4fdf65ded3c10ed003f
ed3f10f43ced10fc3c103c3f3cfd3c10fe5d3c3fed1112395d712f3c10fd
3c1112390111123910edec0010f50110edec0010f53130437940203d4322
283e25422623253d27402d004322402d003f263c2d0127284124442d002b
103c2b012b2b2b2b2b818101715d005d0111333236273311232626232311
141617163333323637363733032122072207062322240235103736213217
163321132326272627262305342627262322060215141216333236363504
50b77360012727095475b714170f3e68785f334b36286cfe1b8d1e0c9b6c
25a9fee9a48da9014417ab8c7f01d90c2018131934216efe402523324d7c
bd5f54bb854c5c230502fde95f65fe287b4ffe4050300d081a2e447cfeac
010906ab0149c00102c5ed0705fed6761f28160df08253141d92fed3bd9b
fedca6335c8e>/BAAAAA+TimesNewRoman AddT42Char 
5 9526 228 <ffff001a000004aa07010226003d0000010700df012c0198001d400f01d0
18019f1801180a00482b010113b902ac0029002b012b5d5d3500>/BAAAAA+TimesNewRoman AddT42Char 
5 4182 181 <000100b9036501ea056b001a00574021000006180201000a080100041005
0814400db600031c17171a0f101f1080100310b8012ab5053a17191b1cbc
012a002100d2013d00182b2b4ef44dedfd5d4e456544e6003f4df4ed3901
111217390010c93130015d01150607061514171633323736333216151407
062322263534373601bc66251b0c0b0f0a121b11283e1f2b39446a583b05
6b2b3e352735200f0f07093c2d331c26725476614000>/BAAAAA+TimesNewRoman AddT42Char 
5 4354 182 <000100c1036501f2056b001a004f401d09190101000510091400b60d4014
031c17171a053a0f171f1780170317b8012ab310191b1cbc012a002100d2
013d00182b2b4ef44dfd5ded4e456544e6003f4dfde41239011112393931
30015d133536373635342726232207062322263534373633321615140706
ee67251a0b0c0e0b121a11283e1f2a3a436b593b03652f3d3526351f0f0f
07093c2d321c267154766140>/BAAAAA+TimesNewRoman AddT42Char 
5 3882 179 <0002004303670353056b0016002d0082402801000e041817251b1f282208
110b284022b61711400bb600170300032f17171a0f251f2580250325b801
2a400f1b3aa02b012bc30f0e1f0e800e030eb8012a4009043aaf14011419
2e2fb80174b321545a182b2b4ef45d4dedfd5df65dedfd5d4e456544e600
3f3f4d10f4ed10f4ed111239111239011112393911123939313001150606
151417163332363332161514062322263534362515060615141716333236
3332161514062322263534360146584c0a090d0d2c12293d4a37436c8502
5b65400b0b0c0b2c16293d4d38426a86056b292e643b230d0e0f3d2c3045
745564ad26263a5c3e1c0e0e103b2b3148725569ad00>/BAAAAA+TimesNewRoman AddT42Char 
5 4144 180 <ffff004303670353056b010300c4000004a30011400b7031803102000102
2a0329002b015d00>/BAAAAA+TimesNewRoman AddT42Char 
5 3770 177 <0001ffee01c50411020e0003001db900020327400a00001a050167044748
182b10e54e10f6002f4ded3130012135210411fbdd042301c549>/BAAAAA+TimesNewRoman AddT42Char 
5 3826 178 <0001ffed01c50812020f0003001db900020327400a00001a050167044748
182b10e54e10f6002f4ded3130012135210812f7db082501c54a>/BAAAAA+TimesNewRoman AddT42Char 
5 8606 215 <0001001604450296054c0019006e4043a70fb902b60f038907860f861303
760f77138b020366137a027907036a026907640f039902960fa802030001
34118109770c0d168104040d000c680f0d1f0d2f0d030db80170b7006801
191a58de182b4e10f44dedfd5ded003f3c10ed103cf4fdf43c3130015d5d
5d5d5d5d1323363633321716163332363733160606232227262623220706
3620046a4e29222da52820310e1f01335d2f4f753f2c1529180b0449897a
0d116d36555d6d3d502b12241100>/BAAAAA+TimesNewRoman AddT42Char 
4 10458 140 <0002001e022507b5054c0017004201a540468c2f015d2e62187318731975
2d7a2e8618842d8a2e992ea72da82e0c432d492e591903392e4418451a03
3218361a372c0305181f261f27103510362418261a2b2e0820c4421bb801
09b4223dc44242b80109b42321c44225b80109b4232bc44226b80109b422
30c44236b80109b4233cc44237b80109403f2211c4420d8d2208c4420c8d
2314192e2d201819301a202c1917362c2f13022498252798252626362d2e
2e35983636389837370c0d06070712121399000302b8033eb2011617b803
3e402d0018421c981b1b41984242011a0100022d986a2e012ead19193c12
1107083d3c2c2b204417171a2b2a0f210121b80249b63d3099003c013cb8
022a401208039802169817360002360187082a008711bb020d0043004401
dab321587a182b2bf6e4fdf4e410f4ed10ed10f65ded3cfd5ded4e456544
e63c103c103c103c103c12392f4dfd5ded003f3c3c103c10ed3c10ed103c
10fe3c10fe3c10fd3c103c103c2fb10602435458b20f0d01005d593c3c10
ed3c10ed3c103c103c103ced10ed11123939111239011112391112392b2b
2b2b2b2b2b2b2b3130015d5d5d5d5d005d13211723262623231114161715
213536363511232206072325010121150e0215111416171521353e023511
012301111416163333152135323636351134262623353302d816220a5563
4b2842fe8a41234c5f500f2204660111010901173825122649fe723b2913
fecd20fecc11252724fece382712112838054cc94845fdbd542d03242406
2b5202443f4ec9fdc4023c2501142c46fe2c552a04242401162a4101ecfd
6e0289fe1e4429162424142a4501d24c28152500>/BAAAAA+TimesNewRoman AddT42Char 
5 9464 227 <ffff0064ffe402d50569022600560000010600df3900002640100120343f
34af34bf34df34ef34063408b8ffa6b4482b010133b902ad0029002b012b
5d35>/BAAAAA+TimesNewRoman AddT42Char 
5 5326 190 <00010073fff8023703a60005003b400d04030a00010701ad000004ad03ba
0125000501a1b70f021f02af020302bc010b0007009c031f00182b10f65d
fdf6fd3c10fd003f3c3f3c3130133301012313733a018afe763af303a6fe
28fe2a01d600>/BAAAAA+TimesNewRoman AddT42Char 
5 2854 176 <00030043ffe4058803b000230032003b02dbb10602435458b90033ffc040
2130340655338000a000b0000320003000400003000010000200000d3925
1f070a09b8ffc0404e1010065510092009b00903000960098009a0090409
530663067306039206a206b2060306310d0b242519072d25130b29080f10
065529100d0d06552950160d0f0f065516160d0d065516090a3423b8ffde
401e0d0d0655231d0c0c065523101c003033000c0d0d0655000c0f0f0655
0030b8ffd6b70909065530303d3c1112392f2bdd2b2bc0111239392f2b2b
cdd0cd2f2b2bed2b2b003fed3fed3fed5d71c45d5d2b323fed12392f5d5d
5dcd2b31301b4066562054225e345e355e365e3706500050236000602304
4f084f0b8c12861a8c2e053932591c5f32691b6a327104791b742b7c3276
3b8304892fa620b620c6200f0308090f029108101c303b0400033309350a
22230a09061c393310062d235f00010030343333b8ffc0401447355f336f
337f339f330433390624251939251fb80346402219070009010009100920
09600972099209a009b00908097d06310d2d2513130d0b33b8032c402c30
2030a030d03003303c3d0f34016f347f348f340334f4232309cc9f0a0100
0a100a200a300a400a600a060ab802e9400c703dbf3d023d295090160116
b8ffc040092a2e3416433c434b182b4e10f42b724ded105df65d72ed3c10
ed5d711112395d2fed003f3c10ed10fdb10602435458400e530663067306
039206a206b20603005d7159e45d713ff4ed10ed1112395d2b2f3cfd723c
11123911123911123901111239123911173912393931304379406b353b1d
2f0e180305372621253635373502062728262802062b2604263820351c01
212236353a1e331c001d1c3820341c0125182920002c142920002e12301c
0111050e0220000f103621391c013b1d391c033522391c0128172420012a
152d20002f112d1c02030f062002002b2b2b2b2b2b2b01103c2b3c2b2b2b
2b103c2b103c103c2b2b2b2a2a2b2b8181818101715d005d007201725901
061514161633323637170606232226270606232202353412333216173636
333217160701220607061510171633323635340205213627262623220603
5f0243844f507b242124b37d6189233e9f61b0f1f7b06b9e2f3b825e935c
5c05fc4224631b25663e5b597587011b015f011912562f4367023d190d5e
cc64667411c1ad5e4350510101d6e5010f5846554a6363ad013b35405395
fefe945a94bbe90115fa464030397800>/BAAAAA+TimesNewRoman AddT42Char 
5 9582 229 <ffff00290000036c05690226005d0000010700df00810000002fb1011cb8
ffc04019101006552f1c01101c201c027f1c9f1c021c046e482b010117b9
02ad0029002b012b5d71722b3500>/BAAAAA+TimesNewRoman AddT42Char 
4 11166 142 <00020039046002720539000b00170049402c0319542764360c407f120112
00407f0601061917171a0340d009e0090209850f405f156f150215541854
5a182b4e10f45d4dfdf65dfd4e456544e6002f5d4ded2f5ded3130012b01
321615140623222635343621321615140623222635343602062d3f3f2d2d
4040fecc2e3f402c2d403f0539402d2d3f3f2d2d40402d2d3f3f2d2d4000
>/BAAAAA+TimesNewRoman AddT42Char 
5 4818 186 <ffff0013000005a906ac0226003c00000107008e01a201730017400c0102
0238272a482701020235b902ac0029002b012b00>/BAAAAA+TimesNewRoman AddT42Char 
5 894 163 <000200e4fe4601c603ce000b00180057b9000cffc0400a404134101af80e
67360cb8ffc0b32a35340db8fff840092a3034970da70d020db80349b506
130640000db80335400b0c0c03400934104016f81910f6edf4ed392fed00
2fed2f10e6313001722b2b2b2b0132161514062322263534361333131615
140623222635343701562f40412e2e40401a265905432e2f420503ce412e
2e40402e2e41fe7dfcd6351a3f4d4c4c182b>/BAAAAA+TimesNewRoman AddT42Char 
4 6756 132 <00020081fe850384052e002c0036014a407d002c2f142c1d8536b9160510
3601171637244724680b692a682e780b792a88018624892a882e9915b514
d038e038fa1c110a200a21021d0809132d2e1c141408061623241515072c
002d2e2c242320161309060a1a0d0609042d2c240004282e2320031d1613
30150707300814140808140708340d14151a3507040815b801b4b6302511
07130708b8011140232831040b1a2f0f0001001a2f384038023834312f0d
400d020d193714141a0d3738aa21ba010a018800182b2b191112392f184e
10f45d4ded4e105df6714de4003ffdb10602435458400a53286328732803
932801005d7159ed3f3ffded111239011112393911123939872e2b7d10c4
00111239121739111739123939011112173910c987100ec43c3c3c07102b
3c0e3c053c0e3c3130184379401231330e1032250f263110342000330e30
2001002b012b2b2b818101715d00715d0106070623222703231326272635
343736333217133303161716151406232227262726270316171633323636
370513262322070615141603842f745a8351518e469b5124339d78991429
8c4891652530302e371f1208040de438261c293d703a36fe0cdf1c20663c
5223015dbc685123fe7a01ab4c4e6e8cfe886904017ffe6e2d2a363d272e
26163c1f22fd89260d0a3345707002670c4a64a84b7e>/BAAAAA+TimesNewRoman AddT42Char 
4 7258 133 <0002003dffe803d105680043004f018840360f300f392f302f394f390524
401d478d080d0e254420280614230142033e0d0e31144d440a0620470d0e
261d3738343b46349f2e4327bb035c000000260158b42e051d2347b8033a
40340ab1114d461717110b37381f3101317c001f0e900e020e1a51033823
34203628363e382a7c27674a46001a901aa01a031a195051b8017bb32154
5e182b2b4ef45d4dfdf5f4edf4f4f4ed4e10e65d4d10f45ded003f3c10ed
10fdf6ed3ffd3cfd3c10eded113939111239391239391139123901111239
111239391239391112393910c9313043794064484f383d2b302122121c04
092c2608262105237401481c4a1d003c2d3e1d003a2f381d0139384c184a
1d004e16441d0115144f440912061d000706131422042074000506212049
1b471d013d2b3b1d0139303b1d014b194d1d004f154d1d0007130a1d0000
2b2b2b2b2b2b103c103c2b01103c103c2b103c103c2b2b103c2b2b2b2b2b
2b81818181818100495479b645461e1f451f47b802b2b305461e44b802b2
b40145441f2001103c103c2b002b8181005d012116151406071617163332
363717060623222627060623222635343633321617363635342723353326
353436363332161514062322272626272623220615141716172101262623
220615141633323602d3fefe011b23c41c34325368182415a565446e9428
5d3532435c48112a1a020115c2c20d62ad637e7f311d26190b081e1f384f
670c07030102fe57162a152d32271a213f02932e165ea0683f060c4d5309
a1a6316f5050453c435904041a260d58f15f95327aca6b88442032261277
1c1c7c9c49724b21fdba0e0e3127242a3e00>/BAAAAA+TimesNewRoman AddT42Char 
5 14208 862 <0002001b00c603e30489001e002b01b44036a804a829b804b829c904c929
06330b351e02581a581e681a681e7900781a881a881e98009819a91ba82b
b91bb92bc81bc82b10080707b8032740090a09140a0a09111212b8032740
090f10140f0f10020303b803274009000114000001171616b80327400919
181419191812ad11b80350b4107712ad11b802c6b510770f07ad08b80350
b4097707ad08b802c6b509770a03ad02b80350b4017703ad02b802c6b501
770016ad17b80350b4187716ad17b802c640231877190000141c0000051f
0a0a0c140a0a1f050f0f0c140f0f1f1419191c1419191f05410e02850028
033d0022033d001400250327000c035500140355001f032740091c0c4525
cb1ccb1f28b80327400a2f0530050205881f8822b8032740120f14016f14
af14bf14ef140414192c545a182b4e10f45d714dedf4f45ded10e6e6e600
2fedfcfced10e6e6e50112392f001112392f011112392f001112392f0111
12392f001112392f011112392f001112392f0110e4eded00e4e4ed0110e4
eded00e4e4ed0110e4eded00e4e4ed0110e4eded00e4e4ed870e2e2b7d10
c4870e2e182b7d10c4870e2e182b7d10c4870e2e182b7d10c43130007101
5d7101371707161514071707270623222627072737263534372737173636
33321607220615141633323635342626031a8f3a906767903a8f868858a7
28923890666690389234a0494599e097d3d49595d662ac03fb8e398d8495
9a8291378f673d2a8f379175a59d7e8d398e2d39341dd59693d4d6935bb0
5e00>/BAAAAA+TimesNewRoman AddT42Char 
4 12534 150 <00010002000003ff054c00400178403c221f2123222a2135341f36223523
342a33356735861f862a0c561f562a563503461f462a463503352c344235
363b374236231f224223242a25422415b801a7b4420dd32204b801a74012
420cd3231e1f1f222a2b142a2a2b3b2c2b2bb802c940353c3b143c2b2a3c
3b1f2a41152c3b3c0342041f2a2c3b0423401a0d1b3d3c3c2b2b1e1e1d26
1c3e3f3f1b1b0f1c1f1c2f1c3f1c041cb803544047170100001919182617
0316160217170d3635352423020c0d083d3e3e0101a0020102b7031d1c1c
1818af170117b71a1916161522404000030498201f2b5f2b028f2b01302b
012bba01bb00410103b1df182b1910f45d71721afd3c3c3c1a18fd3c103c
3cf45d3c103c103c10f45d3c103c103c003f3c3f3c3c103c12392f3c3c10
3c10fd3c103c103c10f45d3c103c103c10fd3c103c103c103c1112393911
173901111217391112393987082e2b870e7dc4870e2e182b057d10c4182b
2b10ed0110c00010ed0110c00010ed0110c00010ed0110c03130015d5d5d
012115211514171617163333152135333237363736353521352135272135
210326262735211506061514171313363534272627222735211522070607
0321152107025501aafe560b0919253029fdfd204622180904fe5801a80f
fe670179d525473801ba483112d6d515150e320912015a3c1b2b2bd60183
fe5d0701a9496c701f16101629291a132613656c4990244901f057380126
26052415102bfdf901f8321915140d04032626172361fe1b4910>/BAAAAA+TimesNewRoman AddT42Char 
5 9656 230 <000200a1fe4600f4058e00030007005cb604096a11643602bc033f000701
59000601db400d030003020917171a0000010504b80327400c0706072002
400202026a0809bc011f0021006a010000182b2b4ef45d3c3c4d10fd3c3c
3c4e10456544e6103c003f4dfdfde631302b1311231113112311f4535353
058efd1a02e6fb9efd1a02e6>/BAAAAA+TimesNewRoman AddT42Char 
4 7876 134 <0002009cfe700364056800480057017640be2259c31164362b0125242059
3224384830597a4976518a49a059b0590b86268651020a04052975268825
0409200f4e191f291f471f4a4049434944082708282c2f412f432f442f4e
4855574e78007a01772578497651890089018849a61faa42a843bb48e604
e43de943173757474e585503b74fc626d91c038651b626c64fd640045125
46284900090351250049042b061d1f1f38550114555501414343384e2614
4e4e26434e4126042846011d551f042203011d551f434e4126080631bb03
0b002b000d030b401d17682f063f065f06a006b006e00606063b682b3738
2e14380938103628bc0312003e02c600530312b36f220122b80158b5462e
38343603bc0312001a02c6004b03124011104620463046a046b0460546c3
586a7a182b10f65dedfdedf4ed10fd5dedfdedf4fded10ed002fed2f5ded
ed10ed121739011112173911121739870e2e2b0e7d10c4870e2e182b0e7d
10c400111217390111123939111239393130005d5d5d5d71015d5d5d012b
012626353436333216151407062322263534373635342623220615141716
171617161514060716161514062322263534363332161514061514171633
323635342726272627263534363706151417161716173635342627260179
4339a4786e8f1a1322222c08053a3349651b2d6ac94a346a734635a4786c
8f2f1f1f2c10192738436d1f307ebc44336c919725349146349958895203
4b4a7a3f75a58656271e152e1f0f26171429366649402a464d9173525a5b
b6454d70417aa4895825332f281b41111d131e683d3e314b5f8c6b515b5c
b3255b83463b516e35305d7f418d6b3f>/BAAAAA+TimesNewRoman AddT42Char 
4 11166 142 <00020039046002720539000b00170049402c0319542764360c407f120112
00407f0601061917171a0340d009e0090209850f405f156f150215541854
5a182b4e10f45d4dfdf65dfd4e456544e6002f5d4ded2f5ded3130012b01
321615140623222635343621321615140623222635343602062d3f3f2d2d
4040fecc2e3f402c2d403f0539402d2d3f3f2d2d40402d2d3f3f2d2d4000
>/BAAAAA+TimesNewRoman AddT42Char 
4 9944 139 <00030045ffe105d0056b000f001f0041012f4025761276177f2f7f327a35
0547325928552c59386928662d6938751570307031852f0b4f0830b80343
400c315f316f317f31033139333eb8035640142022212133412034256800
391039203930390439b803544010104600032e460f331f332f333f330433
b80354401018460809309831362036229800210121b8012d401b042bb10f
361f362f363f360436e60c1c46a004b004c004f0040404b80323400d1446
500c600c020c8042545a182b10f65dedfd5ded10f45ded10f45dede4f4ed
003fedf45ded3fedf45dedf43c12392f3c10e41112395d2fe43130437940
3a011f12250e2602251e2616260a2506261a25110f1474001f011c740117
0914740019071c7401130d1074011d03107401150b1874001b051874002b
2b2b2b012b2b2b2b2b2b2b2b2b2b2b2b81005d015d013204121514020423
222402353412241722040215141204333224123534022417132326262322
060706061514163332371706232200353400333216171633323637030ab3
0154bfbcfeaeb8b8feafbcbf0154b2a3fecaaeab0134a8a80135abaefeca
bb1427249d6e5280291e28b695c375258bf4c8fef90118da2e3d4e190c10
160b056bb7feabb9b8feaebbbb0152b8b90155b73da8fec9a9a8feccacac
0134a8a90137a8c0fee8777544392b8e4fd4c9a213cb0103b9c0010f0c1a
08111c00>/BAAAAA+TimesNewRoman AddT42Char 
4 13486 157 <0002fffa030f02320568002e003800f4b9002fffc0b20b3900b8ffc04068
0b3906001400262e410040305200df23db2ddb31d937df380b0f240f374f
234a314f388f238f38072f2e3e2e780d880d980da80db80dc80d08190d28
0d800680070438232f351d981ccf2034353a262f983b004b005b0003003f
00030940103909400f398f260126b801c2b51f092f090209b802c6400d03
980f031d1c80143aae131314b8019bb523383800002fba012d0032019b40
0e2940060106810c3e2919393a9421b80103b1df182b2b4ef44df4ed7110
edf43c103c103cfd3c10e610f63c003feded71ed712b2b1139762f185ded
10edf4fded11123939313001715d00715d002b2b01342623220615140623
222635343633321616151514171617163332371506062322262706062322
263534373637363706061514163332363701543535302e2119172171795c
631b02030807060e2c49321a1927093f6c2c354e161e4d34a57857332616
3b25049c6d432b2e2d29221a37583e424cda35080d07061e30351529362d
2e4c302c212e2f1f1e28603022341616>/BAAAAA+TimesNewRoman AddT42Char 
5 1536 169 <00020040fff803c003a60005000b005b401209030707010a0d17171a0a07
ad06060aad09ba0125000b01a1400a08fa0501ad000004ad03ba01250005
01a1b302190c0db801cdb321545a182b2b4ef44dfdf6fd3c10ed10f6fdf6
fd3c10ed4e10456544e6003f3c3f3c313005230101330301230101330301
fc39fe7d018339f402b83afe76018a3af30801d801d6fe2afe2801d801d6
fe2a>/BAAAAA+TimesNewRoman AddT42Char 
5 1062 164 <0001002401d8045c036e00050037bb0005032700000130b2030403b80327
b2020201b8ffc0400c090d34011a07005806585e182b4e10e410f62b3c4d
10fd3c002ffded31301321112311212404384ffc17036efe6a014500>/BAAAAA+TimesNewRoman AddT42Char 
4 9152 138 <00040045ffe105d0056b000f001f0042004c022640b334400b3931400b39
33400b3928400b392d400b392e400b392f4012392f4012392f401439182e
01044e491f643604220a280d2e00340035051f2e1f2f020f280f2e020912
0616061a091e2f352f367b1376150805232823026f196f1f025f1f601160
1703501150175f19037b277f2f022c2f5c275c2f037208272f2e2eb12827
14282827282e2f03272d282c27432f42ac2037ac3634ac3543ac2ff03001
303021352cac2d4a972010210100212021bf210321b80341400c002d2e2e
361f3501b0350135b80341403b0810460003184608093500341034203403
348e3142202b371f3601366c3c802c012c6c802d012d6c1f47010f470147
b110240180249f24af240324b802204014043043434c4c10310131b13d2f
3c8f3c903c033cb80220b60c1c46c0040104b80323400b1446500c010c49
4d6463182b10f65dedfd5ded10f45d3cfd723c103c103c10f45d72ed5d72
e45de45d10f45d3cf43c10f45d3c003fed3fed10f45d723c3c103c10f45d
723ced10ed1112392f5d3ced10ed10ed10ed11123912390111121739872e
2b870e7dc43130184379405444490126452512250e2602251e2616260a25
06261a2544264733014922473b01110f1456001f011c5601170914560019
071c56014625433300262748234a3b01130d1074011d03107401150b1874
001b05187400002b2b2b2b2b103c2b012b2b2b2b2b2b2b2b2b2b2b2b2b2b
2b8181015d5d5d5d5d00715d015d72712b0072012b2b2b002b2b2b2b2b2b
013204121514020423222402353412241722040215141204333224123534
022405213216151406071316171617152301231116163315213532363736
3511342726262313323636353426232207030ab30154bfbcfeaeb8b8feaf
bcbf0154b2a3fecaaeab0134a8a80135abaefecafdd4018291986777d126
1e1322b8feda4c062d43fe91302809070307252ded766d3a7158262e056b
b7feabb9b8feaebbbb0152b8b90155b73da8fec9a9a8feccacac0134a8a9
0137a8d4835d4c731ffed635140c03210195fecb211e21211716104d020b
4a0d1719fe832e5335516e10>/BAAAAA+TimesNewRoman AddT42Char 
5 14146 256 <0001ffef05b60412060a00030022b900020327b400001a0501bc018b0004
0102011900182b10e54e10f6002f4ded3130012135210412fbdd042305b6
5400>/BAAAAA+TimesNewRoman AddT42Char 
4 6540 131 <00020062030302c9056a000b0017008c40100319ae1864368019a019b019
03370812bc0327000601c2000c0327b2000315bc0327000301c2000f0327
40148009a009b009032009300940090309ae189ca4182b10f65d71edfded
003fedfded31304379402a01170d0b0f1d001701151d0111070f1d001305
151d010e0a0c1d0116020c1d011008121d001404121d002b2b2b2b012b2b
2b2b8101712b013216151406232226353436172206151416333236353426
019581b3b4807fb4b3805d82825d5c8382056ab4807fb4b47f80b454825d
5c83835c5d82>/BAAAAA+TimesNewRoman AddT42Char 
4 12276 147 <00010017008d044e04c3000f00c940242f002f012f042f05200a200b200e
200f082007200860076008a007a008060e0d0d020201bb0327000f000003
51b2030807b803514009060b030a0909060605b80327400c04040c03600b
a00b020bbb09b8032740136006a0060206bb05600ea00e020ebb080d070d
b80327401b020504046002a0020202bb010100403a350040363520000100
cb10b80103b15e182b10f65d2b2b3c10e45d3c103c10ed3c103ce45d10f4
5dfde45d002f3c3c10fd3c103c103c103c10f43c10f43cfd3c103c103c31
30005d015d373521112135211133112115211121151701f2fe0e01f25001
f4fe0c01f58d5101a25201f1fe0f52fe5e51>/BAAAAA+TimesNewRoman AddT42Char 
5 12162 240 <000100140298023f0568001c00c3405df908f80c02080c01000400050016
0017001817182718070a1780048005801783189004900590179318c004c0
05c017c018d004d005d616d017d018e004e005e016e017e018f004f005f0
16f017f0181c18140304170503110318021c00b80356b2191918b80144b5
020e0f0d010db80309b20a0102ba0158000a0329401511050781143e0094
020d980e36030302191d585e182b4e10f43c4d10f4ed10fdf4ed003fedfd
3c10f45d3c10fd3c10f43c111239111739011112393130015d7100715d01
07213536373635342623220607233636333216151407060733323637023f
3dfe12f75132533f3956162d0e7f656a85304bdcba5739140330981dc079
4a453d533b3b626f7448424b75b21820>/BAAAAA+TimesNewRoman AddT42Char 
5 12448 241 <0001002c0289020b0568002b00aab10c2db8032940200b6436220a300a76
0686069606a706a50aa02d086406f92a02092a0109072200b80346b39f2b
012bb801a140160423984409540964097409840994090609ad22220416b8
0144b219460fb80158b38f290129b803294013040523222207132b68002e
132681072f1c810cb80229b513192c58a4182b4e10f44dfdedf4ed10f4ed
1112392f3c003fed71fdeded12392fed5ded10fd5de40111123931300071
5d015d2b1336373633321615140716161514062322272635343633321633
32363534262726232335323635342623220737242d40555c6a694849aba1
54251a211a1c6a263850352a3c2f1e4d694237553e04cd4a222f5c374457
1a613b6794181116111c304f352d5210171c5e3d313e5800>/BAAAAA+TimesNewRoman AddT42Char 
4 11078 141 <000100ec04150235056e00030039400f000201010f000100d5020517171a
00b801fdb5038402190405b80209b321e5a4182b2b4ef44df4fd4e456544
e6002f4ded5d3c3130015d010123130235fed92269056efea7015900>/BAAAAA+TimesNewRoman AddT42Char 
4 13100 151 <00010086fe4604460394003800deb9003affc0b211353ab8ffc040140f35
703ab03a02103a011d0924030a190a010610b80145b519154f160116b801
a6401019072c2020190b2d0f242402381d0915b801ecb416920c090ab801
6740220b0b0c400f1006550c360d0d06551f0c012f0c3f0c5f0c03100c4f
0caf0ccf0c040cb801284014203a603a703a803a043a30502a2a38020201
3801b80167400f0000100020008000900005008b39b2b9029100182b10f6
5ded3c103c1112392fed105df45d71722b2b3c10fd3c10f4ed103c111239
2f003f3f3c10ed10fd713c10ed3f3c11121739313001725d2b2b13331114
171616333237113311141716163332373637330606232227262706062322
2726270615141716151406232226353437363736353427c4a4120d462976
76a5080722131a121a0b2a096c514e2a1e0857964d35271c2301220d3826
25321d14020c010394fdeb913528328602affd72641f181b161f47796f3a
2b5966581510301f0f4fa03d2b303e3a332e775018674c054600>/BAAAAA+TimesNewRoman AddT42Char 
4 8584 136 <0001fff2fe4603a3054c0012005bb300070107b802d8400b101204991002
050206ad05ba012500040125401703030206d5022600df010101770f1101
116f140b6e1314b80138b32147df182b2b4ee410f65d4df45d3ceded103c
10eef6ed002f3c3ffd3c10ed5d313001112311231123112e023534373636
332115031e48bb49bfbd642b3ac19c01ef0515f93106cff93104130855b1
6e6e46606337>/BAAAAA+TimesNewRoman AddT42Char 
5 6088 194 <000100910237016f0315000b0022400f00f8060d17171a03f809190c6a7a
182b4e10f44dfd4e456544e6002f4ded3130013216151406232226353436
01002f40412e2e41410315412e2e41412e2e4100>/BAAAAA+TimesNewRoman AddT42Char 
5 9082 220 <000100bbfe7a01f0001000150090402b05179a0e67364915015915691502
79158915022a153a15020a151a15020201019900151400001502010015b8
0144b50202000d6808b80130401001000a1515000b0a0a16000538103401
b8018f400a60007000800003001916ba01ab016000182b4e10f45d4dedf4
ed1112392f3c12392f003f3cfdfd11392fed01111239872e2b0e7d10c431
30015d5d5d5d5d2b25330716161514062322273516333236353426232207
01693c323f3e785f25391c1433462e220a10104f104c36486d072b04432b
1e2c0200>/BAAAAA+TimesNewRoman AddT42Char 
5 11978 239 <00010088029801dd05680019006540230f09000c0211c1420b8d2203c142
0a8d2317190001021219980f000100ad0101020b0ab80158401202050203
00000100841203bf40110111191ab80311b1dd182b4e10f45d4ded3ce45d
103c003ffd3c103c10fc5ded011112391239392b2b3130015d1337331114
17161716331521353237363635113427262623220788cd2306050b103ffe
bb40100c0a05030f0c142f051157fdb03c0e09050820200705163e017647
17100d14>/BAAAAA+TimesNewRoman AddT42Char 
4 13892 158 <0002001d031302630568000b0019009b401b96119918d504038611891802
751179180208181818023d08134606b801c240090c4600031b17171a16bc
019b000301c1000f019bb309191a1bb801c1b32158de182b2b4ef44dedfd
ed4e456544e6003f4dedfded31304379402e0119182611260d0b0f1d0019
01161d0112070f1d001405161d010e0a0c1d0117020c1d011008131d0015
04131d002b2b2b2b012b2b2b2b2b2b8100715d5d5d013216151406232226
353436172206151417163332363534272601447ca3b27a76a4a566344a45
273f394b472c0568a97c7cb4a37d8aab2b5a629f633959609d633e00>/BAAAAA+TimesNewRoman AddT42Char 
5 1688 170 <00020040fff803c003a60005000b005d401209030a0701070c1717190a07
ad06060aad09ba0125000b01a1400a08fa0501ad000004ad03ba01250005
01a1b4021a0d0c0db801cdb321545a182b2b4e10f64dfdf6fd3c10ed10f6
fdf6fd3c10ed4e10456544e4003f3c3f3c31300133010123130133010123
130204390183fe7d39f4fd483a018afe763af303a6fe28fe2a01d601d8fe
28fe2a01d600>/BAAAAA+TimesNewRoman AddT42Char 
5 13252 243 <00040086ffca05dd05680019001d0028002b00ff40273c194c19020f0900
0c1d2b2f2b3f2b052a2b2b2711c1420b8d2203c1420a8d23161911001a1b
1bb8032740321c1d141c1c1d1b1c2d2c0102121d2b251a2621222a26252b
2419980f000100ad01021e28282b291f20202429ad2392220b0ab80158b4
0226272127ba01580022034340271b021a1d1b1c1d051c0b2425d52a2a22
cf271e8421852d0203cf12000001008450110111fa2c2db80181b3216a5e
182b2bf65de45d3cfd3c10f6e43cfd3c10fd3c003f3f103c103c3c10f4ed
3c103c10fd3c10f4ed3c3c103c103c3c103c103cfd5ded11123911390111
12393912393911123911123939872e2b7d10c40111123939182b2b07103c
3130015d5d13373311141716171633152135323736363511342726262322
0725012301011523152335213501331123110186cd2306050b103ffebb40
100c0a05030f0c142f0476fc5a5a03a7012a6c75fea901785475fefc0511
57fdb03c0e09050820200705163e01764717100d1473fa62059efb7851b7
b74901d1fe37013cfec4>/BAAAAA+TimesNewRoman AddT42Char 
5 12742 242 <00030086ffca05d605680019001d003a0149405bf926f82a02082a010422
043517362636040f09000c0a3580228023803583369022902390359336c0
22c023c035c036d022d023d034d035d036e022e023e034e035e036f022f0
23f034f0361d11c1420b8d2203c1420a8d231d1c1cb80327401f1b1a141b
1b1a3632211d1a1c1b043c3b223523032f2136200c980b09980b0ab80158
400d0119980f000100ad010f2b012bbf030900280329002f01580020001e
0356b2373736b8014440451f200201011a1d1c1b0b1d052b982c36212120
a81e2581f03201003201323e001e01301e401e501ee01ef01e051e1a3c00
00010084120203cf12401150110211fa3b6a5e182b10f65d3cfd3c10e45d
4e10f65d714df4715ded10fd3c10f4ed003f3f3c103c3c103c2f3cfd3c10
e410fdfde45d10fc5ded10fd3ced10ed1112391117390111121739111239
872e2b7d10c4182b2b3130015d7100715d13373311141716171633152135
323736363511342726262322072501230101072135363736353426232206
0723363633321615140706073332363786cd2306050b103ffebb40100c0a
05030f0c142f045efc595903a7013b3dfe12f75132533f3956162d0e7f65
6a85304bdcbb563914051157fdb03c0e09050820200705163e0176471710
0d1473fa62059efb09991ec0794a453d533b3b61707547424c74b2172100
>/BAAAAA+TimesNewRoman AddT42Char 
5 13652 244 <0004002affca05dd05680003002c0037003a013b40281d3a200e2d3a300e
3f3a760a850a940aa60a09092b01650af30cf50df526f92b05393a3a3603
0202b8032740230100140101000d230b02010300043c3b3a33353031440d
540d640d740d840d940d060db8011db624cc2323081304b80346b39f2c01
2cbb01670008001a0145b21d2513b80158b38f2a012ab80329b508050003
3536b802bd400b313a382e2f2f322d373738b8011d4018322e3333329230
310b02010b030533347e392df236303931b80145b330603c2cb801ec400f
042e1724232317272c0b202c0b2f10b802bbb517193bcd89182b4e10f44d
fde4ed10ed12392f3c10f4ed10f6fd3c103ce410fd3c003f3f3c3f3cf43c
103c10fd3c103c103c103c103c10fd3c103c3fed71fdeded10fd5de41112
392feded5d01111239123911121739111239872e2b7d10c40704103c3130
005d71015d01012301053637363332161514071616151406232227263534
363332163332363534260735323635342623220701152315233521350133
1123110104fdfc5d5a03a7fb8e242d40555c6a694849aba154251a211a1c
6a26385071774d694237553e05826c74fea801785474fefc0568fa62059e
9b4a222f5c3744571a613b6794181116111c304f354860021c5e3d313e58
fc2351b7b74901d1fe37013cfec4>/BAAAAA+TimesNewRoman AddT42Char 
5 546 162 <00020059fe46033803cf000b002b00dc4042af1001262129255b0f5b2a6b
0f6b2a7c0f7c2a8a0f80138a2a990e990f992ba916ad2410161718031a20
0f102a28040d19181d14101a110e0d0c2b0f0903701d011db801b4400e14
46230c700d800d900db00d040db8034540270639000d700c0c03091a500f
2001052015200220e6031150d026010a261a26022687090f2d012db80295
b503390f090109bf0295002c002d01c800210120029100182b2bf671fde6
7110f45d71ed10f45d71ed1112392fed002ffdf65d3c2feded5d01111239
39111239111239001112393911173901111217393130015d005d01321615
140623222635343613330606021514163332363534263534363332161514
062322263534373e0201c42e41412e2e414123270527a5846857643e3021
2946c3a9aac91d2bd63c03cf412e2e41412e2e41fea37c91fea473849052
311f6b20222f534573afbb82534562f78800>/BAAAAA+TimesNewRoman AddT42Char 
5 2102 172 <ffff0010000005b0070502260024000001070043018b01970022400b0220
210170219021022110b8ffc4b4482b020123b902ac0029002b012b5d5d35
>/BAAAAA+TimesNewRoman AddT42Char 
5 7362 200 <ffff0010000005b007050226002400000107008d018a019700234014024f
23012f233f23027f2301230f31482b020121b902ac0029002b012b5d5d71
3500>/BAAAAA+TimesNewRoman AddT42Char 
5 7206 198 <ffff0010000005b00701022600240000010700d6018a0198002eb3020201
26b902ac0029002b01b10602435458b50026220f10402b1b400b5f24017f
2401240f19482b2b5d5d5935>/BAAAAA+TimesNewRoman AddT42Char 
5 2162 173 <ffff0010000005b006bc022600240000010700d7018b01700024400d029f
2d012f2dcf2ddf2d032d1eb8015eb4482b020131b902ac0029002b012b5d
7235>/BAAAAA+TimesNewRoman AddT42Char 
4 4296 98 <ffff0010000005b006ac0226002400000107008e018901730035b5030202
030226b902ac0029002b01b10602435458b5002f290f10402b1b400f7029
9029cf2903902901291032482b2b5d7159353500>/BAAAAA+TimesNewRoman AddT42Char 
5 8800 219 <00020096041102150590000b001700ce400b0b02040404080b0a043708b1
0602435458400a03090f15041918124606b8ffc0400a0a0d065506060c46
0000003fed332f2bed01111217391bb506460f120112b80309b50940090e
3409b80309400a0c460000034600150115bb030900060000ffc0b3090e34
00b80309b20f4609b8ffc04009090d340985186a7a182b10f62bfdf42b3c
f45ded003ffdf42bf45ded5931304379402a01170d0b0f1d001701151d01
11070f1d001305151d010e0a0c1d0116020c1d011008121d001404121d00
2b2b2b2b012b2b2b2b81005d013216151406232226353436172206151416
3332363534260155507070504f706f50334747333347470590704f507070
504f70454733324848323347>/BAAAAA+TimesNewRoman AddT42Char 
4 4376 99 <ffff0010000005b006a5022600240000010700db01860115001840100302
0029230f10400203023210004827002b012b3535>/BAAAAA+TimesNewRoman AddT42Char 
4 11316 144 <0002ffe8000006e4054c0042004501484067313232304443242444434325
07210d0d37081b07221f1b1c21222c302d1b2c0621020237051b062b252a
1b2b2444392b323030232543142525431b0f1a25302b4632223928242a25
301a1432014338422324234544d00201230d0e0e1c4223393c003b103b02
3bb802d3402b3a38ac3a3902191ae81b1b1c2c2b14a51dac2b1c0819ac47
17171a1a3a2b3bac0f3c1f3c023c49061aac19bb012200060007022c4009
000f2243222246472bb802ecb32c194647ba026700210102b15d182b2b4e
f44ded1112392f3cfd3cf43cf6ed10f65dfde44e10456544e64ded003f3c
eded103c103c10fc3c3f3ced10fe5d3c10ed12392f3cfd3cf43cfd3c1112
391239111239391112390111123911123939111239870e2e2b0e7d10c401
11123939180010ed0110c010edec0010f510ed0110c02b0110edec0010f5
87057d10c43c073c070e103c313001112132363733112326262726232111
141616333332363736373303213533323736351121070615141617152135
3e0237013635342726273521132326272627262321012104030101735e08
24240c2930175dfeff0e2c39b66d7637492f266cfc0633532718fe747c46
3d60fe562c3f4a39019c4d1b227004570f220d251b331d6bfdf5fe9b0165
0502fde8566ffe296445150bfe3f5b23182434446ffeab25312079011ee9
84291c2f07252501245e6a03038f322012190625fed6673627120afd5400
>/BAAAAA+TimesNewRoman AddT42Char 
4 4426 100 <ffff004afe7a050f056b022600260000010700dc015100000031401a0140
2501502560250270258025020025302502a025b025022514b8ffe2b6482b
0101250829002b012b5d5d5d5d5d3500>/BAAAAA+TimesNewRoman AddT42Char 
5 7488 202 <ffff002a000004b4070502260028000001070043012001970015400a0101
350fb94827010137b902ac0029002b012b00>/BAAAAA+TimesNewRoman AddT42Char 
4 4502 101 <ffff002a000004b407050226002800000107008d01200197001b400e012f
373f37023701fa482b010136b902ac0029002b012b5d3500>/BAAAAA+TimesNewRoman AddT42Char 
5 7278 199 <ffff002a000004b40701022600280000010700d601200198003a401f0100
3a01603a803a02503a703a02d03a01e03af03a02403a703a903a033a00b8
ffe2b4482b010136b902ac0029002b012b5d5d5d71717135>/BAAAAA+TimesNewRoman AddT42Char 
5 7424 201 <ffff002a000004b406ac0226002800000107008e011f01730025400d0201
503d803d903da03d043d00b80118b5482b0102023ab902ac0029002b012b
71353500>/BAAAAA+TimesNewRoman AddT42Char 
5 7742 206 <ffff00330000027807050226002c000001070043000101970017b2012118
b8ffa2b4482b010123b902ac0029002b012b3500>/BAAAAA+TimesNewRoman AddT42Char 
5 7536 203 <ffff00330000027807050226002c00000107008d000001970019400c0130
230123096e482b010121b902ac0029002b012b713500>/BAAAAA+TimesNewRoman AddT42Char 
5 7588 204 <ffff00330000027807010226002c0000010700d6000001980039b3010101
26b902ac0029002b01b10602435458b50026221112402b1b400f5f266f26
02bf26011f262f26022618b8fe93b1482b2b715d5d593500>/BAAAAA+TimesNewRoman AddT42Char 
5 7672 205 <ffff00330000027806ac0226002c00000107008effff0173002bb3010202
26b902ac0029002b01b10602435458b702010035231112402b35351bb701
020229180a48272b5900>/BAAAAA+TimesNewRoman AddT42Char 
5 9788 231 <0002002300000578054c0019002800c440651f2676147617030b1d0b2102
071801851d8a21022508061f1b0021220b1f1b1121231a1c242227082326
2f093f0902092228121211021c28191900080f09010909221c1f09010953
292727292a1f3c161a702a012a241a220b1f06010619292a79216163182b
2b4ef45d3c4dfd3c4e105df64ded1112392f10e65d001112392f5d3f3c10
ed3f3c10ed105d3cfd3c123912392b2b31304379401a1d21131814252113
1f56011d181f560120152256011e171c56002b2b012b2b2b8181005d7101
715d33353332373635112335331134272623233521200412151000212716
333200111000232207112115212333562515c3c31c274d330228013b012e
c4fe91fe77d97f56e70132feceef5a730189fe772538207301b64a016c7f
202c258ffec5d3fee1fe70641c01460117011901441dfe0b4a00>/BAAAAA+TimesNewRoman AddT42Char 
4 4556 102 <ffffffe5ffea05aa06bc022600310000010700d7018a0170002140130140
296029022f295f2902291450482b010139b902ac0029002b012b715d3500
>/BAAAAA+TimesNewRoman AddT42Char 
5 7900 209 <ffff0048ffe10578070502260032000001070043018901970017b302011d
00b8fff0b4482702011fb902ac0029002b012b00>/BAAAAA+TimesNewRoman AddT42Char 
5 7792 207 <ffff0048ffe1057807050226003200000107008d018801970019400c024f
1f011f0d10482b02011db902ac0029002b012b713500>/BAAAAA+TimesNewRoman AddT42Char 
5 7844 208 <ffff0048ffe105780701022600320000010700d601880198001db7023f22
ef2202220db8fefcb4482b02011eb902ac0029002b012b5d3500>/BAAAAA+TimesNewRoman AddT42Char 
5 2224 174 <ffff0048ffe1057806bc022600320000010700d701880170001bb5029f29
012900b80140b4482b02012db902ac0029002b012b5d3500>/BAAAAA+TimesNewRoman AddT42Char 
4 4616 103 <ffff0048ffe1057806ac0226003200000107008e01870173001c400e0302
ef250125155a482b02030222b902ac0029002b012b5d3535>/BAAAAA+TimesNewRoman AddT42Char 
5 11688 238 <000100a5010e03da0443000b00de402701020900050703080b0604030800
050a09020b0605cb090634080b0603cb0b0234000902050000b803274009
0b06140b0b06030808b80327b70902140909020008b8032bb2090503bc03
2b0006033d000202d8400b0b34a009b0090209003402b802d8b205cb09b8
032bb2083406b802d840112003cb1f0b01000b200ba00b030bf80cd2b901
0000182b1910f65d7218e61a19fd18f419f418e619fd18f4002f5de419fd
18e619fd3c10fd3c870e2e182b0e7d10c4870e2e182b0e7d10c4010810e0
10e00810e010e00f0f0f0fb10602435458b41903190502005d5913010137
0101170101070101a50161fea03a0160016038fea0016239fe9efe9f0148
016101603afea0016039fea0fe9e3a0162fe9f00>/BAAAAA+TimesNewRoman AddT42Char 
4 11856 145 <00030049ffd1057905780016002200300103406e591701302f2e23231702
0e3e08030d23240e0e02001017220f0110122422170d00052003062d2422
17100d0300071928010f0f230e02140e0e020e0f20120102062d0f280a02
1501031928150328280a090e092d3c1f0601061a40320132203c1012010f
125f12021219316463182b4e10f45d724ded4e1071f6724ded003f3fed3f
ed3f1139111239011112393911123939870e2e2b7d10c400111217390111
12391217391139070e3c3c3c3c07100e3c3c3c3c3130184379402e292c1a
1f131407091e1f1d1f1c1f1b1f040608262b2c2a2c02061a14202d002909
2d2d011f13192d012c07282d00002b2b012b2b2a2b2a81818181060e103c
0111123939005d0137170716161510070623222627072737261110002132
172623220706070606151417010116171633323e0235342726047b833a85
685ef4bce167e354813b84c901880114e35f74d35d364b3b4f4a4902d6fd
53363e596d69867554120e04d6a22ca771e89dfea9d4a34b449f2fa4cf01
4101260191fcb5161e4258fe9fe7b10306fcb25226383f84f0b47b694d00
>/BAAAAA+TimesNewRoman AddT42Char 
5 8068 212 <ffff000bffe005b107050226003800000107004301bc01970015400a0101
3025004827010132b902ac0029002b012b00>/BAAAAA+TimesNewRoman AddT42Char 
5 7950 210 <ffff000bffe005b107050226003800000107008d018b01970015400a0101
3225464827010130b902ac0029002b012b00>/BAAAAA+TimesNewRoman AddT42Char 
5 7998 211 <ffff000bffe005b10701022600380000010700d601ba0198002cb3010101
35b902ac0029002b01b10602435458b50035311209402b1bb46f3501350d
b8fefcb1482b2b715935>/BAAAAA+TimesNewRoman AddT42Char 
4 4670 104 <ffff000bffe005b106ac0226003800000107008e01ba0173002fb5020101
020235b902ac0029002b01b10602435458b50044321209402b1b400a3f38
4f3802382564482b2b5d59353500>/BAAAAA+TimesNewRoman AddT42Char 
5 10694 233 <ffff0013000005a907050226003c00000107008d01af01970015400a0101
3227054827010130b902ac0029002b012b00>/BAAAAA+TimesNewRoman AddT42Char 
5 10808 235 <0002002400000424054c002b003900da403d46081c1f1b1621222b1f1b24
2122101f1b1521231d1f1b2321232c2d331039a501e7242423022ea50f0f
1f0f020fe716161508333c071a3b2b10221d1cb8fffeb4101006551cb8ff
f0b70d0d06551c193a3bb80177b3216163182b2b4ef42b2b3c4dfd3c4e10
f64ded003f3c10f45ded3f3c10f4b10602435458b90001ffc0b2090a342b
59ed01111239392b2b2b2b3130437940382f38020d050604060306030635
3436343734030609080a080b080c08040631323032020638023333012f0d
333301340639330132082e33002b2b012b2b2a2a2a2a8181013332171e02
15140e020706232315141633331521353332373635113426262323352115
232207060615151133323736363534262627262301a44a964a6c8f5b3a62
7c63249b46455429fdbe265d2814164b36280242282c321e1e2c7a445a56
3e653e286104180c135b985e4d835e380d053d814d2525381c7703647235
2c2525170e46638ffdad1c268e5e4b7e470d0800>/BAAAAA+TimesNewRoman AddT42Char 
4 8740 137 <00010023fff303be058e003a00fc403a30194f2d5019601988349b16aa19
078508880f024019783802301a301b020018101820183018044b0805291e
004a221133201f251d2811302f1db801a640200030252f2f0036250a0000
0a2825170a242e20319f1a011a3530303b3c33310db8010840122c31141a
3c393a240605193b3ceb21a64b182b2b4ef43c4dfd3c4e10f64dfdfded11
12392ff45dfde4003fed3f3fed12392fed10ed1112391112393901111239
2b3130437940363438252b1519070c2a253709391c000807350b331c0127
18251c00262529162c1c013808361c01340c361c012619281c002b15281c
002b2b2b2b012b103c2b2b103c2b2b81818181015d5d005d5d5d33353e02
351134373633321615140706071616151402232226353436333216151407
061514171633323736353426273532363534262322061511233c33155d5d
aba2be362861878ab69957692b24272b04060f0f1a3c273393946a6d6957
5166240520395f02e5f96867b78e6a4a362a28c6a1aefefb60422a2d2b24
1011180b120e0e354692d0f40a397d92867880bffbf3>/BAAAAA+TimesNewRoman AddT42Char 
4 4798 106 <ffff0049ffed0389056e02260044000001070043008e0000002540170240
3f703f803f03003f703f803f033f1e16482b020141b902ad0029002b012b
5d713500>/BAAAAA+TimesNewRoman AddT42Char 
4 4744 105 <ffff0049ffed0389056e0226004400000106008d7500001d4010022f413f
414f4103411e16482b02013fb902ad0029002b012b5d3500>/BAAAAA+TimesNewRoman AddT42Char 
4 4862 107 <ffff0049ffed03890569022600440000010600d675000030401802104450
440200447044b044d044e0440510442044024425b8fdd4b4482b020144b9
02ad0029002b012b715d7235>/BAAAAA+TimesNewRoman AddT42Char 
4 4998 109 <ffff0049ffed0389054c022600440000010600d7750000154009024b251e
482b02014fb902ad0029002b012b3500>/BAAAAA+TimesNewRoman AddT42Char 
4 4934 108 <ffff0049ffed038905390226004400000106008e74000028401903027047
8047904703b047c047d04703471e54482b02030244b902ad0029002b012b
5d713535>/BAAAAA+TimesNewRoman AddT42Char 
5 8800 219 <00020096041102150590000b001700ce400b0b02040404080b0a043708b1
0602435458400a03090f15041918124606b8ffc0400a0a0d065506060c46
0000003fed332f2bed01111217391bb506460f120112b80309b50940090e
3409b80309400a0c460000034600150115bb030900060000ffc0b3090e34
00b80309b20f4609b8ffc04009090d340985186a7a182b10f62bfdf42b3c
f45ded003ffdf42bf45ded5931304379402a01170d0b0f1d001701151d01
11070f1d001305151d010e0a0c1d0116020c1d011008121d001404121d00
2b2b2b2b012b2b2b2b81005d013216151406232226353436172206151416
3332363534260155507070504f706f50334747333347470590704f507070
504f70454733324848323347>/BAAAAA+TimesNewRoman AddT42Char 
4 5044 110 <ffff0049ffed03890592022600440000010600db7502001e40100302103e
503e023e1e00482b02030244b902ad0029002b012b5d3535>/BAAAAA+TimesNewRoman AddT42Char 
4 14130 160 <00030049ffe4051803b0003f004600540276b10602435458b90040ffc040
2130340655408000a000b0000320003000400003000010000200000e4425
3c070a09b8ffc040281010065510092009b00903000960098009a0090409
530563057305039205a205b2050305310e0b4bb8011b4031402101002120
21022121524f2d012f2d7f2d022d7e351f2501252535073052405202522c
190b2931312f4f311c090a413fb8fff4402a0d0d06553f3f124738565540
000c0d0d0655000c0f0f065500214b0c0f0f06554b160d0d06554b4b5655
1112392f2b2bc5dd2b2bc01112393939392f2bcdd0cd2fedf4ed003fed71
3fed7210ed5d7111392f5d71ed3fed5d71c45d5d2b323fed12392f5d5d5d
cd2b31301b4056593b553d553e5e415e425e435056075000503f6000603f
044547d650021a1f4a1f43374a4d5020502106251e291f2d4d3b1f3b4d05
09140947022f564933593369339904990b990c9b10a43db43dc23d0b3840
210a09b8ffc040160f1434000910092009f00904097d055f00010030404b
b8011bb5214010400140b8ffc0405f2528345f406f407f409f4004400544
402101002120213021032121524f2d012f2d3f2d7f2d032d7e351f440144
253c1f250125253c350705310e3052405202522c0e190b0f41016f417f41
8f410341f43f3f09cc500a01300a400a600a030ab802e9b2560040b80167
401b2129312f313f3102312f1c4b3f21bf21ef21031f215f21b0210321b8
0152400e4f31501c01501c011c1955434b182b4e10f45d724dedf45d713c
10f45ded10fd3c4d10f65d724ded3c10ed5d71003f3ced7110ed3f3ced72
10ed7210ed5d7111392f5d711112395d2b722f10ed10ed7210e45d2b3901
1112393130015d00715d5d01710072017259010615141633323736371706
070623222726270607060706062322263534363736373534262322070615
140606232227263534363633321617363736333216152521262623220603
2626353506070615141633323602de019070614f323920247756816c4d24
4b0c2b3a142f6a385e81577f9c78504342252611241b27151e499d697c7e
143035476190b5fdc6017a026750506f7e151a87714a5f42275702373317
c9aa3d277816a26c4e2f175a09222f0b1b208560577a41502a5c6c592021
2854321a17202834684847343c1b24c2b7417e737dfdcc2d9145592a5639
594f6429>/BAAAAA+TimesNewRoman AddT42Char 
4 5098 111 <ffff0046fe7a034a03af022600460000010600dc6d000014b2012203b8ff
e7b6482b0101220829002b012b35>/BAAAAA+TimesNewRoman AddT42Char 
4 5194 113 <ffff004cffe40353056e0226004800000107004300a700000022400c0250
1f601f701fa01f041f11b8ffeab4482b020121b902ad0029002b012b5d35
>/BAAAAA+TimesNewRoman AddT42Char 
4 5142 112 <ffff004cffe40353056e0226004800000107008d008200000019400c023f
2101211132482b02011fb902ad0029002b012b5d3500>/BAAAAA+TimesNewRoman AddT42Char 
4 5254 114 <ffff004cffe403530569022600480000010700d6009a00000028b10224b8
ffc0400b0d0d06557024f024022411b8fee8b4482b020120b902ad002900
2b012b5d2b35>/BAAAAA+TimesNewRoman AddT42Char 
4 5320 115 <ffff004cffe4035305380226004800000107008e0099ffff001c400e0302
602701270b5a482b02030224b902ad0029002b012b713535>/BAAAAA+TimesNewRoman AddT42Char 
4 5432 117 <ffff003c00000207056e022600d5000001060043d7000017b301011816b8
ffd3b4482701011ab902ad0029002b012b00>/BAAAAA+TimesNewRoman AddT42Char 
4 5374 116 <ffff003c00000207056e022600d500000106008dbd000022400b014f1a01
7f1a8f1a021a16b8ffe2b4482b010119b902ad0029002b012b5d7135>/BAAAAA+TimesNewRoman AddT42Char 
4 5480 118 <ffff000d000002400569022600d50000010600d6d1000020400a01401d50
1df01d031d0fb8ff38b4482b01011db902ad0029002b012b5d35>/BAAAAA+TimesNewRoman AddT42Char 
4 5536 119 <ffff00020000023b0538022600d500000106008ec9ff0020401202019020
a020e02003201628482b0102021db902ad0029002b012b5d3535>/BAAAAA+TimesNewRoman AddT42Char 
5 10114 232 <00020044ffe403b5058e001f002c01b740d136010109010b021f011f0239
029c0d990e074a014b0268007a00042c0128023c0139020402020a0a0a0b
130114021b0a1a0b30013002400140025a1e5c1f78187822a41ff5011184
01840c800da401047919791e7e2c800004780d75127a147a150449024a0d
491e4b1f043b0139023a2c49010429012802020401240134014201043808
03090a0a02000c0b0b01060706161e0c09070300062a231e200c09060300
050a1a0b010130020a1402020a0102160a230b0f2a0b0201030a1a07000a
012025001a101a501a031a072725130b2ab8fff9b40f1006552ab8fff040
130d0d06552a500f0f0f0f06551f0f010f1a2e16b8fffc401b1010065523
080f0f065523100d0d0655235010160116192d434b182b4e10f4724ded2b
2b2b4e10f6722b4ded2b2b003fed3f5ded3f3f1112173901111239123911
3939870e2e2b7d10c400111217391239011112173912390010c987100ec4
3c87100e3cc4b10602435458b41e38091234002b59313018437940282129
10191826252611262119232000261423200028122a200122172020012415
2720002910272000002b2b2b012b2b2b2b2b2b818101715d5d5d5d5d5d5d
005d5d5d7101072737262627371617371707161215140606232202353437
363332171617260722061514161633323635340201d5f71ee94243371b78
7ff922e5bec273d07fb3fc8a76a431271f3250626082518a4b5b7e9e0491
8737844337242b3c5f8b3782a5fe73b98be982010bcad39a810d0a24a5a7
a2c288e56f9eb1e10110>/BAAAAA+TimesNewRoman AddT42Char 
4 5592 120 <ffff000c000003f7054c022600510000010700d700ab0000002140130140
4150419041035041014102d2482b010145b902ad0029002b012b715d3500
>/BAAAAA+TimesNewRoman AddT42Char 
4 5708 122 <ffff0045ffe403b9056e0226005200000107004300b700000017b302011f
00b8fff0b44827020121b902ad0029002b012b00>/BAAAAA+TimesNewRoman AddT42Char 
4 5652 121 <ffff0045ffe403b9056e0226005200000107008d009e0000001d400f024f
21017f2101210010482b02011fb902ad0029002b012b5d713500>/BAAAAA+TimesNewRoman AddT42Char 
4 5758 123 <ffff0045ffe403b90569022600520000010700d600b600000024400d022f
246f24027024bf24022400b8fef2b4482b020124b902ad0029002b012b5d
7135>/BAAAAA+TimesNewRoman AddT42Char 
4 5880 125 <ffff0045ffe403b9054c022600520000010700d700aa00000024400e020f
2b2f2b3f2b402b9f2b052b00b8014ab4482b02012fb902ad0029002b012b
5d35>/BAAAAA+TimesNewRoman AddT42Char 
4 5820 124 <ffff0045ffe403b905380226005200000107008e00a9ffff002240130302
7027802702df2701270055482b02030224b902ad0029002b012b5d723535
>/BAAAAA+TimesNewRoman AddT42Char 
5 4516 183 <000300170117044d0433000b000f001b0086b7a00ca00f0200b106b8033e
b30e16b110ba033e000d0327b40e403f350eb8ffc040433b350f0e01200e
500e800eb00edf0eff0e069f0ecf0eff0e033f0e6f0e020e300c400c020c
8813b119300f400f020f8803b1090919880f0d4f0ddf0d030d451c58de18
2b10f671f43c10fde45d10fde45d002f5d5d71722b2bfdf6ed10f6ed3130
015d01321615140623222635343601213521013216151406232226353436
0232243333252433330240fbca0436fde525333424243433043333242433
33242433fe4d52fef5342424343424243400>/BAAAAA+TimesNewRoman AddT42Char 
5 0 161 <00030027ffbd03d903d300180021002a0198b10602435458402319200913
06552220091306552219212304261c1c2516072625090b2219212304291f
29b8fff4400d0d0d065529051f0c0d0d06551fb8fff440130b0b06551f12
100f0f065512100d0d06551205b8fff0400b0d0d065505052b12122c2b11
12392f11392f2b102b2bcd2b2b10cd2b11121739003fed3fed111217392b
2b31301b40732801290227194b195a1a7004700770087914702888020b1a
22102c02060c060f160c160f260d3f0d061b22012f08030c22230d0d0200
0f1921211f0e0e010c0f1f1219222a1a041600030529232221190f0c0300
081c26020d0d300e01140e0e010e122b1c251607012f02070e0b2625090b
02b801ecb7012e2950051a2c0eb801ec400d0d2e1f5010120112192b434b
182b4e10f4724dedf4ed4e10f64dedf4ed003fed3f3fe43fed0111123987
0e2e2b7d10c40011121739011112393912173911123939871008c40e3c3c
3c07100e3c3c3c3c3130184379402027281d1e13150608142607261d151f
200027082920011e131c20012806262000002b2b012b2b2b2b8181818100
725d01725d59013717071615140606232226270727372626353436363332
160726262322061514170101161633323635340326852e876a74cd805380
4b872f8d323879cc7a52852033634262822701b1fe6d336245637d034093
2b9887b176fd81333f992b9f3eb44e77f27f34ac5945a0b97c8a0180fe3e
5c45a0c77900>/BAAAAA+TimesNewRoman AddT42Char 
4 6000 127 <ffff0002ffe403fd056e0226005800000107004300bd0000001bb5019f27
01271eb8ffeab4482b010129b902ad0029002b012b5d3500>/BAAAAA+TimesNewRoman AddT42Char 
4 5942 126 <ffff0002ffe403fd056e0226005800000107008d00860000001f4012014f
295f296f297f2904291d16482b010128b902ad0029002b012b5d3500>/BAAAAA+TimesNewRoman AddT42Char 
4 6054 128 <ffff0002ffe403fd0569022600580000010700d600ae0000002cb1012cb8
ffc0400f10100655002c102c402c802c042c1db8ff06b4482b01012cb902
ad0029002b012b5d2b35>/BAAAAA+TimesNewRoman AddT42Char 
4 6124 129 <ffff0002ffe403fd05380226005800000107008e00a9ffff002ab202012f
b8ffc0401311110655c02f01802f012f1e3b482b0102022cb902ad002900
2b012b5d5d2b3535>/BAAAAA+TimesNewRoman AddT42Char 
5 10742 234 <ffff000cfe4603f4056e0226005c00000107008d00a700000027b2010135
b902ad0029002b01b10602435458b601003533060b402b351bb601013609
0048272b5900>/BAAAAA+TimesNewRoman AddT42Char 
5 11188 236 <0002fff9fe4b03ba058e002700390147b10602435458b90032fffc400c0d
0d0655320a060f0f06550ab8fff040180d0d06550a0a3b3a0329130c0d0d
06551302101006551320b8fff6b40d0d065520b8fff8b40f0f065520b8ff
ee401b1010065520203b3a0328060e270001190e2e250e0b365906070100
003f3fed3fed3f10ddcd11123939011112392f2b2b2bdd2b2bd0c0111239
2f2b2bcd2b31301b40407b117f2b8b11032e0820291e19862213291e1827
230027214f271e00442b29280332132b28120304362e2106020036590607
2e250e0b19180e3b17171a0a5032b8023e4011200213242100200120193a
3beb21c24b182b2b4ef45d3c4dfd3c10f4fd4e456544e6003f3c3f4ded3f
ed3f123911121739011112173900f5edfc01f52b2b3130437940202f3507
0d082534260c26302535073220012f0d3220013309362001310b2e20002b
2b012b2b2b2b2b2b8181015d590325331136363332171615140706232227
262711141616331521351716373636351134262623220701111417161633
323736353427262322070602011a26478f4f8a5c718870aa4a3628321739
4bfe20193727131510231e18250134090e6d53643e515c4058302f24051c
72fd4779616c84d4ed9b7f150f2dfee95d321e26260101160b3163054559
31180ffd9efeaa6f233a584e66b9d2714e181200>/BAAAAA+TimesNewRoman AddT42Char 
5 4744 185 <ffff000cfe4603f405390226005c00000107008e00cf0000002fb5020101
020239b902ad0029002b01b10602435458b500423c0013402b1b400a8f3c
903c023c0921482b2b5d59353500>/BAAAAA+TimesNewRoman AddT42Char 
/BAAAAA+TimesNewRoman findfont /CharStrings get begin
/.notdef 0 def
/dotlessi 213 def
/caron 223 def
/space 3 def
/exclam 4 def
/quotedbl 5 def
/numbersign 6 def
/dollar 7 def
/percent 8 def
/ampersand 9 def
/quotesingle 10 def
/parenleft 11 def
/parenright 12 def
/asterisk 13 def
/plus 14 def
/comma 15 def
/hyphen 16 def
/period 17 def
/slash 18 def
/zero 19 def
/one 20 def
/two 21 def
/three 22 def
/four 23 def
/five 24 def
/six 25 def
/seven 26 def
/eight 27 def
/nine 28 def
/colon 29 def
/semicolon 30 def
/less 31 def
/equal 32 def
/greater 33 def
/question 34 def
/at 35 def
/A 36 def
/B 37 def
/C 38 def
/D 39 def
/E 40 def
/F 41 def
/G 42 def
/H 43 def
/I 44 def
/J 45 def
/K 46 def
/L 47 def
/M 48 def
/N 49 def
/O 50 def
/P 51 def
/Q 52 def
/R 53 def
/S 54 def
/T 55 def
/U 56 def
/V 57 def
/W 58 def
/X 59 def
/Y 60 def
/Z 61 def
/bracketleft 62 def
/backslash 63 def
/bracketright 64 def
/asciicircum 65 def
/underscore 66 def
/grave 67 def
/a 68 def
/b 69 def
/c 70 def
/d 71 def
/e 72 def
/f 73 def
/g 74 def
/h 75 def
/i 76 def
/j 77 def
/k 78 def
/l 79 def
/m 80 def
/n 81 def
/o 82 def
/p 83 def
/q 84 def
/r 85 def
/s 86 def
/t 87 def
/u 88 def
/v 89 def
/w 90 def
/x 91 def
/y 92 def
/z 93 def
/braceleft 94 def
/bar 95 def
/braceright 96 def
/asciitilde 97 def
/bullet 135 def
/Euro 188 def
/quotesinglbase 195 def
/florin 166 def
/quotedblbase 196 def
/ellipsis 171 def
/dagger 130 def
/daggerdbl 193 def
/circumflex 214 def
/perthousand 197 def
/Scaron 226 def
/guilsinglleft 189 def
/OE 175 def
/Zcaron 228 def
/quoteleft 181 def
/quoteright 182 def
/quotedblleft 179 def
/quotedblright 180 def
/endash 177 def
/emdash 178 def
/tilde 215 def
/trademark 140 def
/scaron 227 def
/guilsinglright 190 def
/oe 176 def
/zcaron 229 def
/Ydieresis 186 def
/exclamdown 163 def
/cent 132 def
/sterling 133 def
/currency 862 def
/yen 150 def
/brokenbar 230 def
/section 134 def
/dieresis 142 def
/copyright 139 def
/ordfeminine 157 def
/guillemotleft 169 def
/logicalnot 164 def
/registered 138 def
/macron 256 def
/degree 131 def
/plusminus 147 def
/twosuperior 240 def
/threesuperior 241 def
/acute 141 def
/mu 151 def
/paragraph 136 def
/periodcentered 194 def
/cedilla 220 def
/onesuperior 239 def
/ordmasculine 158 def
/guillemotright 170 def
/onequarter 243 def
/onehalf 242 def
/threequarters 244 def
/questiondown 162 def
/Agrave 172 def
/Aacute 200 def
/Acircumflex 198 def
/Atilde 173 def
/Adieresis 98 def
/Aring 99 def
/AE 144 def
/Ccedilla 100 def
/Egrave 202 def
/Eacute 101 def
/Ecircumflex 199 def
/Edieresis 201 def
/Igrave 206 def
/Iacute 203 def
/Icircumflex 204 def
/Idieresis 205 def
/Eth 231 def
/Ntilde 102 def
/Ograve 209 def
/Oacute 207 def
/Ocircumflex 208 def
/Otilde 174 def
/Odieresis 103 def
/multiply 238 def
/Oslash 145 def
/Ugrave 212 def
/Uacute 210 def
/Ucircumflex 211 def
/Udieresis 104 def
/Yacute 233 def
/Thorn 235 def
/germandbls 137 def
/agrave 106 def
/aacute 105 def
/acircumflex 107 def
/atilde 109 def
/adieresis 108 def
/aring 110 def
/ae 160 def
/ccedilla 111 def
/egrave 113 def
/eacute 112 def
/ecircumflex 114 def
/edieresis 115 def
/igrave 117 def
/iacute 116 def
/icircumflex 118 def
/idieresis 119 def
/eth 232 def
/ntilde 120 def
/ograve 122 def
/oacute 121 def
/ocircumflex 123 def
/otilde 125 def
/odieresis 124 def
/divide 183 def
/oslash 161 def
/ugrave 127 def
/uacute 126 def
/ucircumflex 128 def
/udieresis 129 def
/yacute 234 def
/thorn 236 def
/ydieresis 185 def
end
/BAAAAA+TimesNewRoman findfont /Encoding get
dup 0 /.notdef put
dup 1 /dotlessi put
dup 2 /caron put
dup 32 /space put
dup 33 /exclam put
dup 34 /quotedbl put
dup 35 /numbersign put
dup 36 /dollar put
dup 37 /percent put
dup 38 /ampersand put
dup 39 /quotesingle put
dup 40 /parenleft put
dup 41 /parenright put
dup 42 /asterisk put
dup 43 /plus put
dup 44 /comma put
dup 45 /hyphen put
dup 46 /period put
dup 47 /slash put
dup 48 /zero put
dup 49 /one put
dup 50 /two put
dup 51 /three put
dup 52 /four put
dup 53 /five put
dup 54 /six put
dup 55 /seven put
dup 56 /eight put
dup 57 /nine put
dup 58 /colon put
dup 59 /semicolon put
dup 60 /less put
dup 61 /equal put
dup 62 /greater put
dup 63 /question put
dup 64 /at put
dup 65 /A put
dup 66 /B put
dup 67 /C put
dup 68 /D put
dup 69 /E put
dup 70 /F put
dup 71 /G put
dup 72 /H put
dup 73 /I put
dup 74 /J put
dup 75 /K put
dup 76 /L put
dup 77 /M put
dup 78 /N put
dup 79 /O put
dup 80 /P put
dup 81 /Q put
dup 82 /R put
dup 83 /S put
dup 84 /T put
dup 85 /U put
dup 86 /V put
dup 87 /W put
dup 88 /X put
dup 89 /Y put
dup 90 /Z put
dup 91 /bracketleft put
dup 92 /backslash put
dup 93 /bracketright put
dup 94 /asciicircum put
dup 95 /underscore put
dup 96 /grave put
dup 97 /a put
dup 98 /b put
dup 99 /c put
dup 100 /d put
dup 101 /e put
dup 102 /f put
dup 103 /g put
dup 104 /h put
dup 105 /i put
dup 106 /j put
dup 107 /k put
dup 108 /l put
dup 109 /m put
dup 110 /n put
dup 111 /o put
dup 112 /p put
dup 113 /q put
dup 114 /r put
dup 115 /s put
dup 116 /t put
dup 117 /u put
dup 118 /v put
dup 119 /w put
dup 120 /x put
dup 121 /y put
dup 122 /z put
dup 123 /braceleft put
dup 124 /bar put
dup 125 /braceright put
dup 126 /asciitilde put
dup 127 /bullet put
dup 128 /Euro put
dup 129 /bullet put
dup 130 /quotesinglbase put
dup 131 /florin put
dup 132 /quotedblbase put
dup 133 /ellipsis put
dup 134 /dagger put
dup 135 /daggerdbl put
dup 136 /circumflex put
dup 137 /perthousand put
dup 138 /Scaron put
dup 139 /guilsinglleft put
dup 140 /OE put
dup 141 /bullet put
dup 142 /Zcaron put
dup 143 /bullet put
dup 144 /bullet put
dup 145 /quoteleft put
dup 146 /quoteright put
dup 147 /quotedblleft put
dup 148 /quotedblright put
dup 149 /bullet put
dup 150 /endash put
dup 151 /emdash put
dup 152 /tilde put
dup 153 /trademark put
dup 154 /scaron put
dup 155 /guilsinglright put
dup 156 /oe put
dup 157 /bullet put
dup 158 /zcaron put
dup 159 /Ydieresis put
dup 160 /space put
dup 161 /exclamdown put
dup 162 /cent put
dup 163 /sterling put
dup 164 /currency put
dup 165 /yen put
dup 166 /brokenbar put
dup 167 /section put
dup 168 /dieresis put
dup 169 /copyright put
dup 170 /ordfeminine put
dup 171 /guillemotleft put
dup 172 /logicalnot put
dup 173 /hyphen put
dup 174 /registered put
dup 175 /macron put
dup 176 /degree put
dup 177 /plusminus put
dup 178 /twosuperior put
dup 179 /threesuperior put
dup 180 /acute put
dup 181 /mu put
dup 182 /paragraph put
dup 183 /periodcentered put
dup 184 /cedilla put
dup 185 /onesuperior put
dup 186 /ordmasculine put
dup 187 /guillemotright put
dup 188 /onequarter put
dup 189 /onehalf put
dup 190 /threequarters put
dup 191 /questiondown put
dup 192 /Agrave put
dup 193 /Aacute put
dup 194 /Acircumflex put
dup 195 /Atilde put
dup 196 /Adieresis put
dup 197 /Aring put
dup 198 /AE put
dup 199 /Ccedilla put
dup 200 /Egrave put
dup 201 /Eacute put
dup 202 /Ecircumflex put
dup 203 /Edieresis put
dup 204 /Igrave put
dup 205 /Iacute put
dup 206 /Icircumflex put
dup 207 /Idieresis put
dup 208 /Eth put
dup 209 /Ntilde put
dup 210 /Ograve put
dup 211 /Oacute put
dup 212 /Ocircumflex put
dup 213 /Otilde put
dup 214 /Odieresis put
dup 215 /multiply put
dup 216 /Oslash put
dup 217 /Ugrave put
dup 218 /Uacute put
dup 219 /Ucircumflex put
dup 220 /Udieresis put
dup 221 /Yacute put
dup 222 /Thorn put
dup 223 /germandbls put
dup 224 /agrave put
dup 225 /aacute put
dup 226 /acircumflex put
dup 227 /atilde put
dup 228 /adieresis put
dup 229 /aring put
dup 230 /ae put
dup 231 /ccedilla put
dup 232 /egrave put
dup 233 /eacute put
dup 234 /ecircumflex put
dup 235 /edieresis put
dup 236 /igrave put
dup 237 /iacute put
dup 238 /icircumflex put
dup 239 /idieresis put
dup 240 /eth put
dup 241 /ntilde put
dup 242 /ograve put
dup 243 /oacute put
dup 244 /ocircumflex put
dup 245 /otilde put
dup 246 /odieresis put
dup 247 /divide put
dup 248 /oslash put
dup 249 /ugrave put
dup 250 /uacute put
dup 251 /ucircumflex put
dup 252 /udieresis put
dup 253 /yacute put
dup 254 /thorn put
dup 255 /ydieresis put
pop
end

userdict /pdf_svglb get setglobal
[/N93/BAAAAA+TimesNewRoman 1 TZG
userdict /pdf_svglb currentglobal put true setglobal
ct_T42Dict begin
end

userdict /pdf_svglb get setglobal
[/N5/ZYCIBP+Arial-BoldMT 1 TZG
0 0 595 842 re
W
n
q
q
n
0 842 595 -842 re
W
n
true setSA
[/DeviceCMYK] cs 0 0 0 1 sc
58.2354 608.78 m
/N5 [10.5717 0 0 10 0 0] Tf
(30) show
95.2104 608.78 m
(35) show
132.126 608.78 m
(40) show
169.102 608.78 m
(45) show
206.078 608.78 m
(50) show
243.053 608.78 m
(55) show
279.969 608.78 m
(60) show
316.944 608.78 m
(65) show
44.73 636.282 m
(0.0) show
44.73 668.319 m
(0.2) show
44.73 700.357 m
(0.4) show
44.73 732.396 m
(0.6) show
44.73 764.435 m
(0.8) show
44.73 796.473 m
(1.0) show
1 w
4 M
1 j
1 J
[] 0 d
n
62.857 618.988 m
62.857 622.9 l
S
n
81.346 620.915 m
81.346 622.9 l
S
n
99.834 618.988 m
99.834 622.9 l
S
n
118.321 620.915 m
118.321 622.9 l
S
n
136.748 618.988 m
136.748 622.9 l
S
n
155.236 620.915 m
155.236 622.9 l
S
n
173.725 618.988 m
173.725 622.9 l
S
n
192.213 620.915 m
192.213 622.9 l
S
n
210.701 618.988 m
210.701 622.9 l
S
n
229.188 620.915 m
229.188 622.9 l
S
n
247.676 618.988 m
247.676 622.9 l
S
n
266.164 620.915 m
266.164 622.9 l
S
n
284.592 618.988 m
284.592 622.9 l
S
n
303.078 620.915 m
303.078 622.9 l
S
n
321.568 618.988 m
321.568 622.9 l
S
n
62.857 622.9 m
340.055 622.9 l
S
n
60.757 622.9 m
62.857 622.9 l
S
n
58.716 638.89 m
62.857 638.89 l
S
n
60.757 654.937 m
62.857 654.937 l
S
n
58.716 670.928 m
62.857 670.928 l
S
n
60.757 686.976 m
62.857 686.976 l
S
n
58.716 702.966 m
62.857 702.966 l
S
n
60.757 719.014 m
62.857 719.014 l
S
n
58.716 735.005 m
62.857 735.005 l
S
n
60.757 751.052 m
62.857 751.052 l
S
n
58.716 767.042 m
62.857 767.042 l
S
n
60.757 783.09 m
62.857 783.09 l
S
n
58.716 799.082 m
62.857 799.082 l
S
n
62.857 622.9 m
62.857 815.128 l
S
n
175.766 799.141 m
175.762 800.668 174.012 801.621 172.611 800.855 c
171.213 800.089 171.217 798.178 172.618 797.417 c
174.021 796.658 175.768 797.615 175.766 799.14 c
f
n
175.766 799.141 m
175.762 800.668 174.012 801.621 172.611 800.855 c
171.213 800.089 171.217 798.178 172.618 797.417 c
174.021 796.658 175.768 797.615 175.766 799.14 c
S
n
197.975 796.533 m
197.971 798.06 196.221 799.011 194.821 798.247 c
193.422 797.48 193.426 795.57 194.828 794.808 c
196.23 794.048 197.977 795.007 197.975 796.532 c
f
n
197.975 796.533 m
197.971 798.06 196.221 799.011 194.821 798.247 c
193.422 797.48 193.426 795.57 194.828 794.808 c
196.23 794.048 197.977 795.007 197.975 796.532 c
S
n
212.741 790.294 m
212.738 791.823 210.987 792.773 209.588 792.009 c
208.188 791.244 208.191 789.332 209.594 788.571 c
210.998 787.812 212.744 788.769 212.741 790.294 c
f
n
212.741 790.294 m
212.738 791.823 210.987 792.773 209.588 792.009 c
208.188 791.244 208.191 789.332 209.594 788.571 c
210.998 787.812 212.744 788.769 212.741 790.294 c
S
n
227.506 758.256 m
227.504 759.785 225.754 760.736 224.354 759.971 c
222.955 759.205 222.959 757.294 224.359 756.533 c
225.764 755.773 227.51 756.731 227.506 758.256 c
f
n
227.506 758.256 m
227.504 759.785 225.754 760.736 224.354 759.971 c
222.955 759.205 222.959 757.294 224.359 756.533 c
225.764 755.773 227.51 756.731 227.506 758.256 c
S
n
249.717 679.209 m
249.713 680.738 247.963 681.689 246.563 680.925 c
245.164 680.158 245.168 678.248 246.57 677.486 c
247.973 676.726 249.719 677.683 249.717 679.209 c
f
n
249.717 679.209 m
249.713 680.738 247.963 681.689 246.563 680.925 c
245.164 680.158 245.168 678.248 246.57 677.486 c
247.973 676.726 249.719 677.683 249.717 679.209 c
S
n
264.482 660.271 m
264.479 661.798 262.73 662.75 261.328 661.986 c
259.93 661.218 259.934 659.308 261.336 658.546 c
262.738 657.787 264.484 658.746 264.482 660.27 c
f
n
264.482 660.271 m
264.479 661.798 262.73 662.75 261.328 661.986 c
259.93 661.218 259.934 659.308 261.336 658.546 c
262.738 657.787 264.484 658.746 264.482 660.27 c
S
n
286.633 642.125 m
286.629 643.652 284.879 644.605 283.479 643.839 c
282.08 643.074 282.082 641.164 283.484 640.401 c
284.889 639.642 286.635 640.599 286.633 642.125 c
f
n
286.633 642.125 m
286.629 643.652 284.879 644.605 283.479 643.839 c
282.08 643.074 282.082 641.164 283.484 640.401 c
284.889 639.642 286.635 640.599 286.633 642.125 c
S
n
323.607 638.949 m
323.605 640.476 321.855 641.429 320.455 640.665 c
319.055 639.898 319.059 637.988 320.461 637.226 c
321.865 636.466 323.611 637.423 323.607 638.949 c
f
n
323.607 638.949 m
323.605 640.476 321.855 641.429 320.455 640.665 c
319.055 639.898 319.059 637.988 320.461 637.226 c
321.865 636.466 323.611 637.423 323.607 638.949 c
S
n
151.575 801.859 m
154.096 797.72 l
148.994 797.72 l
h
f
n
151.575 801.859 m
154.096 797.72 l
148.994 797.72 l
151.575 801.859 l
S
n
173.725 799.478 m
176.245 795.339 l
171.143 795.339 l
h
f
n
173.725 799.478 m
176.245 795.339 l
171.143 795.339 l
173.725 799.478 l
S
n
195.934 790.008 m
198.455 785.869 l
193.353 785.869 l
h
f
n
195.934 790.008 m
198.455 785.869 l
193.353 785.869 l
195.934 790.008 l
S
n
210.701 736.707 m
213.221 732.566 l
208.119 732.566 l
h
f
n
210.701 736.707 m
213.221 732.566 l
208.119 732.566 l
210.701 736.707 l
S
n
225.467 669.51 m
227.987 665.371 l
222.885 665.371 l
h
f
n
225.467 669.51 m
227.987 665.371 l
222.885 665.371 l
225.467 669.51 l
S
n
247.676 649.21 m
250.197 645.071 l
245.094 645.071 l
h
f
n
247.676 649.21 m
250.197 645.071 l
245.094 645.071 l
247.676 649.21 l
S
n
262.441 644.73 m
264.963 640.591 l
259.861 640.591 l
h
f
n
262.441 644.73 m
264.963 640.591 l
259.861 640.591 l
262.441 644.73 l
S
n
284.592 641.669 m
287.114 637.529 l
282.01 637.529 l
h
f
n
284.592 641.669 m
287.114 637.529 l
282.01 637.529 l
284.592 641.669 l
S
n
87.048 784.398 m
87.045 785.925 85.294 786.876 83.895 786.113 c
82.494 785.345 82.5 783.435 83.9 782.673 c
85.304 781.914 87.051 782.872 87.048 784.397 c
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
87.048 784.398 m
87.045 785.925 85.294 786.876 83.895 786.113 c
82.494 785.345 82.5 783.435 83.9 782.673 c
85.304 781.914 87.051 782.872 87.048 784.397 c
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
109.257 788.763 m
109.254 790.292 107.504 791.244 106.104 790.478 c
104.705 789.712 104.709 787.801 106.109 787.041 c
107.514 786.281 109.26 787.238 109.257 788.763 c
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
109.257 788.763 m
109.254 790.292 107.504 791.244 106.104 790.478 c
104.705 789.712 104.709 787.801 106.109 787.041 c
107.514 786.281 109.26 787.238 109.257 788.763 c
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
131.406 778.556 m
131.402 780.083 129.652 781.037 128.253 780.271 c
126.854 779.504 126.857 777.595 128.26 776.833 c
129.662 776.073 131.408 777.031 131.406 778.556 c
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
131.406 778.556 m
131.402 780.083 129.652 781.037 128.253 780.271 c
126.854 779.504 126.857 777.595 128.26 776.833 c
129.662 776.073 131.408 777.031 131.406 778.556 c
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
153.615 772.773 m
153.611 774.3 151.862 775.251 150.463 774.488 c
149.063 773.722 149.067 771.81 150.469 771.048 c
151.872 770.29 153.619 771.248 153.615 772.773 c
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
153.615 772.773 m
153.611 774.3 151.862 775.251 150.463 774.488 c
149.063 773.722 149.067 771.81 150.469 771.048 c
151.872 770.29 153.619 771.248 153.615 772.773 c
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
175.766 751.113 m
175.762 752.64 174.012 753.591 172.611 752.826 c
171.213 752.06 171.217 750.15 172.618 749.388 c
174.021 748.628 175.768 749.585 175.766 751.111 c
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
175.766 751.113 m
175.762 752.64 174.012 753.591 172.611 752.826 c
171.213 752.06 171.217 750.15 172.618 749.388 c
174.021 748.628 175.768 749.585 175.766 751.111 c
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
197.975 712.156 m
197.971 713.683 196.221 714.634 194.821 713.871 c
193.422 713.103 193.426 711.193 194.828 710.431 c
196.23 709.672 197.977 710.629 197.975 712.155 c
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
197.975 712.156 m
197.971 713.683 196.221 714.634 194.821 713.871 c
193.422 713.103 193.426 711.193 194.828 710.431 c
196.23 709.672 197.977 710.629 197.975 712.155 c
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
220.124 678.472 m
220.121 680 218.371 680.953 216.971 680.187 c
215.572 679.421 215.574 677.511 216.977 676.75 c
218.381 675.99 220.127 676.947 220.124 678.472 c
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
220.124 678.472 m
220.121 680 218.371 680.953 216.971 680.187 c
215.572 679.421 215.574 677.511 216.977 676.75 c
218.381 675.99 220.127 676.947 220.124 678.472 c
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
242.334 649.837 m
242.33 651.365 240.58 652.316 239.18 651.552 c
237.781 650.785 237.785 648.875 239.187 648.113 c
240.59 647.353 242.336 648.311 242.334 649.836 c
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
242.334 649.837 m
242.33 651.365 240.58 652.316 239.18 651.552 c
237.781 650.785 237.785 648.875 239.187 648.113 c
240.59 647.353 242.336 648.311 242.334 649.836 c
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
85.007 792.617 m
87.527 788.478 l
82.426 788.478 l
h
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
85.007 792.617 m
87.527 788.478 l
82.426 788.478 l
85.007 792.617 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
107.217 787.003 m
109.738 782.863 l
104.635 782.863 l
h
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
107.217 787.003 m
109.738 782.863 l
104.635 782.863 l
107.217 787.003 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
129.365 789.896 m
131.887 785.755 l
126.784 785.755 l
h
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
129.365 789.896 m
131.887 785.755 l
126.784 785.755 l
129.365 789.896 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
151.575 787.23 m
154.096 783.09 l
148.994 783.09 l
h
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
151.575 787.23 m
154.096 783.09 l
148.994 783.09 l
151.575 787.23 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
173.725 762.96 m
176.245 758.821 l
171.143 758.821 l
h
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
173.725 762.96 m
176.245 758.821 l
171.143 758.821 l
173.725 762.96 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
195.934 706.425 m
198.455 702.287 l
193.353 702.287 l
h
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
195.934 706.425 m
198.455 702.287 l
193.353 702.287 l
195.934 706.425 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
218.084 671.609 m
220.604 667.469 l
215.502 667.469 l
h
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
218.084 671.609 m
220.604 667.469 l
215.502 667.469 l
218.084 671.609 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
240.292 648.587 m
242.813 644.448 l
237.711 644.448 l
h
[/DeviceCMYK] cs 0 0 0 0 sc
f
n
240.292 648.587 m
242.813 644.448 l
237.711 644.448 l
240.292 648.587 l
[/DeviceCMYK] cs 0 0 0 1 sc
S
n
62.857 799.078 m
176.245 799.463 l
178.767 799.292 l
181.228 799.062 l
183.748 798.833 l
186.27 798.546 l
188.791 798.146 l
191.252 797.63 l
193.773 797.057 l
196.294 796.255 l
198.814 795.339 l
201.275 794.136 l
203.797 792.646 l
206.318 790.813 l
208.839 788.522 l
211.301 785.773 l
213.822 782.392 l
216.342 778.382 l
218.863 773.627 l
221.324 768.013 l
223.846 761.597 l
226.367 754.378 l
228.887 746.302 l
231.348 737.652 l
233.87 728.486 l
236.391 719.091 l
238.912 709.697 l
241.373 700.587 l
243.895 691.937 l
246.414 683.974 l
248.936 676.756 l
251.397 670.398 l
253.918 664.898 l
256.439 660.201 l
258.961 656.191 l
261.422 652.925 l
263.941 650.175 l
266.465 647.941 l
268.926 646.108 l
271.445 644.676 l
273.967 643.472 l
276.488 642.556 l
278.949 641.754 l
281.471 641.181 l
283.993 640.667 l
286.512 640.322 l
288.973 639.978 l
291.495 639.75 l
294.016 639.578 l
296.538 639.406 l
298.996 639.291 l
301.518 639.177 l
304.039 639.119 l
306.561 639.062 l
309.021 639.005 l
311.543 639.005 l
314.064 638.947 l
316.586 638.947 l
319.045 638.89 l
321.568 638.89 l
S
n
151.575 798.684 m
153.796 798.684 l
156.076 798.684 l
158.298 798.626 l
160.578 798.626 l
162.859 798.568 l
165.081 798.511 l
167.361 798.453 l
169.582 798.337 l
171.863 798.222 l
174.084 798.048 l
176.365 797.759 l
178.646 797.414 l
180.867 796.95 l
183.148 796.314 l
185.369 795.447 l
187.65 794.291 l
189.871 792.73 l
192.152 790.648 l
194.434 787.931 l
196.654 784.289 l
198.936 779.664 l
201.156 773.767 l
203.437 766.425 l
205.658 757.637 l
207.939 747.404 l
210.221 735.958 l
212.441 723.759 l
214.722 711.33 l
216.941 699.189 l
219.225 687.973 l
221.444 678.029 l
223.725 669.532 l
226.007 662.536 l
228.229 656.927 l
230.508 652.476 l
232.729 649.066 l
235.01 646.463 l
237.23 644.498 l
239.512 642.996 l
241.793 641.896 l
244.014 641.087 l
246.295 640.509 l
248.516 640.046 l
250.797 639.757 l
253.018 639.527 l
255.299 639.353 l
257.58 639.238 l
259.801 639.122 l
262.082 639.064 l
264.303 639.005 l
266.584 638.949 l
268.805 638.949 l
271.086 638.89 l
273.367 638.89 l
275.588 638.89 l
277.867 638.89 l
280.09 638.89 l
282.371 638.89 l
339.152 638.89 l
S
n
85.007 786.493 m
86.327 786.436 l
S
n
87.828 786.379 m
89.148 786.322 l
S
n
90.649 786.266 m
91.971 786.153 l
S
n
93.471 786.095 m
94.791 786.039 l
S
n
96.291 785.925 m
97.613 785.869 l
S
n
99.113 785.755 m
100.434 785.642 l
S
n
101.934 785.529 m
103.254 785.416 l
S
n
104.756 785.302 m
106.016 785.188 l
S
n
106.016 785.188 m
106.076 785.188 l
S
n
107.576 785.019 m
108.656 784.906 l
S
n
108.656 784.906 m
108.896 784.906 l
S
n
110.398 784.678 m
111.298 784.564 l
S
n
111.298 784.564 m
111.719 784.508 l
S
n
113.219 784.337 m
113.939 784.224 l
S
n
113.939 784.224 m
114.539 784.167 l
S
n
116.04 783.941 m
116.52 783.884 l
S
n
116.52 783.884 m
117.361 783.771 l
S
n
118.861 783.488 m
119.162 783.431 l
S
n
119.162 783.431 m
120.182 783.261 l
S
n
121.683 783.034 m
121.803 782.977 l
S
n
121.803 782.977 m
123.002 782.75 l
S
n
124.504 782.41 m
125.824 782.126 l
S
n
127.324 781.73 m
128.645 781.389 l
S
n
130.146 780.992 m
131.467 780.652 l
S
n
132.967 780.199 m
134.287 779.745 l
S
n
135.789 779.235 m
137.109 778.724 l
S
n
138.609 778.158 m
139.93 777.646 l
S
n
141.432 777.023 m
142.751 776.4 l
S
n
144.252 775.718 m
145.512 775.095 l
S
n
145.512 775.095 m
145.572 775.039 l
S
n
147.073 774.188 m
148.094 773.621 l
S
n
148.094 773.621 m
148.394 773.394 l
S
n
149.895 772.543 m
150.734 772.033 l
S
n
150.734 772.033 m
151.215 771.693 l
S
n
152.716 770.671 m
153.376 770.275 l
S
n
153.376 770.275 m
154.035 769.765 l
S
n
155.537 768.688 m
156.017 768.347 l
S
n
156.017 768.347 m
156.857 767.667 l
S
n
158.357 766.476 m
158.658 766.25 l
S
n
158.658 766.25 m
159.678 765.341 l
S
n
161.18 764.039 m
161.299 763.923 l
S
n
161.299 763.923 m
162.439 762.791 l
S
n
163.881 761.373 m
163.881 761.373 l
S
n
163.881 761.373 m
165.081 760.125 l
S
n
166.461 758.707 m
166.521 758.65 l
S
n
166.521 758.65 m
167.602 757.46 l
S
n
168.862 756.042 m
169.162 755.703 l
S
n
169.162 755.703 m
169.943 754.794 l
S
n
171.084 753.376 m
171.803 752.527 l
S
n
171.803 752.527 m
172.104 752.129 l
S
n
173.244 750.712 m
174.204 749.464 l
S
n
175.225 748.046 m
176.125 746.799 l
S
n
177.206 745.381 m
178.046 744.134 l
S
n
178.946 742.716 m
179.666 741.639 l
S
n
179.666 741.639 m
179.787 741.468 l
S
n
180.748 740.051 m
181.527 738.804 l
S
n
182.488 737.386 m
183.268 736.138 l
S
n
184.169 734.722 m
184.949 733.474 l
S
n
185.79 732.056 m
186.57 730.809 l
S
n
187.41 729.39 m
187.59 729.05 l
S
n
187.59 729.05 m
188.13 728.144 l
S
n
188.971 726.726 m
189.691 725.478 l
S
n
190.531 724.061 m
191.252 722.813 l
S
n
192.031 721.396 m
192.752 720.148 l
S
n
193.533 718.73 m
194.193 717.483 l
S
n
194.974 716.066 m
195.453 715.158 l
S
n
195.453 715.158 m
195.693 714.818 l
S
n
196.475 713.4 m
197.135 712.153 l
S
n
197.915 710.736 m
198.095 710.395 l
S
n
198.095 710.395 m
198.635 709.488 l
S
n
199.415 708.07 m
200.075 706.822 l
S
n
200.916 705.405 m
201.576 704.158 l
S
n
202.416 702.74 m
203.076 701.492 l
S
n
203.857 700.074 m
204.578 698.827 l
S
n
205.357 697.41 m
206.018 696.219 l
S
n
206.018 696.219 m
206.078 696.162 l
S
n
206.918 694.744 m
207.639 693.497 l
S
n
208.418 692.08 m
208.659 691.625 l
S
n
208.659 691.625 m
209.139 690.832 l
S
n
209.979 689.414 m
210.701 688.167 l
S
n
211.479 686.75 m
212.261 685.501 l
S
n
213.16 684.083 m
213.881 682.836 l
S
n
214.781 681.419 m
215.563 680.171 l
S
n
216.463 678.753 m
216.522 678.64 l
S
n
216.522 678.64 m
217.303 677.505 l
S
n
218.264 676.089 m
219.043 674.841 l
S
n
220.064 673.423 m
220.964 672.175 l
S
n
221.925 670.758 m
222.885 669.51 l
S
n
223.904 668.093 m
224.445 667.356 l
S
n
224.445 667.356 m
224.865 666.845 l
S
n
225.947 665.427 m
226.906 664.181 l
S
n
228.107 662.763 m
229.188 661.515 l
S
n
230.448 660.097 m
231.589 658.85 l
S
n
232.909 657.433 m
234.17 656.185 l
S
n
235.611 654.767 m
236.932 653.52 l
S
n
238.432 652.16 m
239.752 651.025 l
S
n
85.007 788.535 m
86.327 788.535 l
S
n
87.828 788.535 m
89.148 788.478 l
S
n
90.649 788.478 m
91.971 788.478 l
S
n
93.471 788.478 m
94.791 788.478 l
S
n
96.291 788.478 m
97.613 788.421 l
S
n
99.113 788.421 m
100.434 788.421 l
S
n
101.934 788.421 m
103.254 788.364 l
S
n
104.756 788.364 m
106.016 788.307 l
S
n
106.016 788.307 m
106.076 788.307 l
S
n
107.576 788.251 m
108.656 788.251 l
S
n
108.656 788.251 m
108.896 788.251 l
S
n
110.398 788.195 m
111.298 788.195 l
S
n
111.298 788.195 m
111.719 788.195 l
S
n
113.219 788.137 m
113.939 788.137 l
S
n
113.939 788.137 m
114.539 788.137 l
S
n
116.04 788.024 m
116.52 788.024 l
S
n
116.52 788.024 m
117.361 787.966 l
S
n
118.861 787.91 m
119.162 787.91 l
S
n
119.162 787.91 m
120.182 787.853 l
S
n
121.683 787.74 m
121.803 787.74 l
S
n
121.803 787.74 m
123.002 787.683 l
S
n
124.504 787.57 m
125.824 787.457 l
S
n
127.324 787.343 m
128.645 787.23 l
S
n
130.146 787.06 m
131.467 786.89 l
S
n
132.967 786.72 m
134.287 786.55 l
S
n
135.789 786.322 m
137.109 786.095 l
S
n
138.609 785.755 m
139.93 785.472 l
S
n
141.432 785.132 m
142.751 784.849 l
S
n
144.252 784.394 m
145.512 783.998 l
S
n
145.512 783.998 m
145.572 783.998 l
S
n
147.073 783.488 m
148.094 783.09 l
S
n
148.094 783.09 m
148.394 782.977 l
S
n
149.895 782.353 m
150.734 781.957 l
S
n
150.734 781.957 m
151.215 781.73 l
S
n
152.716 780.992 m
153.376 780.709 l
S
n
153.376 780.709 m
154.035 780.312 l
S
n
155.537 779.406 m
156.017 779.121 l
S
n
156.017 779.121 m
156.857 778.498 l
S
n
158.357 777.476 m
158.658 777.25 l
S
n
158.658 777.25 m
159.678 776.4 l
S
n
161.18 775.208 m
161.299 775.095 l
S
n
161.299 775.095 m
162.439 773.961 l
S
n
163.82 772.543 m
163.881 772.487 l
S
n
163.881 772.487 m
164.961 771.296 l
S
n
166.221 769.878 m
166.521 769.539 l
S
n
166.521 769.539 m
167.242 768.63 l
S
n
168.322 767.213 m
169.162 766.136 l
S
n
169.162 766.136 m
169.283 765.966 l
S
n
170.242 764.548 m
171.084 763.3 l
S
n
172.043 761.882 m
172.764 760.636 l
S
n
173.604 759.218 m
174.385 757.97 l
S
n
175.165 756.552 m
175.825 755.305 l
S
n
176.545 753.888 m
177.086 752.867 l
S
n
177.086 752.867 m
177.206 752.64 l
S
n
177.926 751.222 m
178.467 749.974 l
S
n
179.187 748.557 m
179.727 747.423 l
S
n
179.727 747.423 m
179.727 747.31 l
S
n
180.387 745.892 m
180.928 744.644 l
S
n
181.588 743.227 m
182.127 741.98 l
S
n
182.729 740.562 m
183.268 739.314 l
S
n
183.869 737.896 m
184.409 736.65 l
S
n
185.01 735.232 m
185.01 735.232 l
S
n
185.01 735.232 m
185.489 733.984 l
S
n
186.029 732.566 m
186.57 731.318 l
S
n
187.109 729.902 m
187.65 728.654 l
S
n
188.191 727.236 m
188.67 725.989 l
S
n
189.211 724.572 m
189.691 723.324 l
S
n
190.23 721.906 m
190.291 721.792 l
S
n
190.291 721.792 m
190.711 720.659 l
S
n
191.252 719.241 m
191.732 717.994 l
S
n
192.272 716.576 m
192.752 715.328 l
S
n
193.293 713.911 m
193.773 712.664 l
S
n
194.252 711.246 m
194.733 709.998 l
S
n
195.273 708.58 m
195.514 708.013 l
S
n
195.514 708.013 m
195.754 707.333 l
S
n
196.294 705.916 m
196.774 704.667 l
S
n
197.375 703.25 m
197.854 702.002 l
S
n
198.395 700.585 m
198.936 699.337 l
S
n
199.475 697.919 m
200.016 696.672 l
S
n
200.615 695.254 m
200.795 694.801 l
S
n
200.795 694.801 m
201.096 694.007 l
S
n
201.756 692.589 m
202.297 691.341 l
S
n
202.896 689.925 m
203.437 688.734 l
S
n
203.437 688.734 m
203.437 688.677 l
S
n
204.098 687.259 m
204.697 686.011 l
S
n
205.357 684.593 m
205.959 683.347 l
S
n
206.678 681.929 m
207.278 680.681 l
S
n
207.999 679.263 m
208.659 678.017 l
S
n
209.439 676.599 m
210.16 675.351 l
S
n
210.94 673.933 m
211.24 673.31 l
S
n
211.24 673.31 m
211.66 672.686 l
S
n
212.561 671.269 m
213.342 670.021 l
S
n
214.301 668.603 m
215.201 667.356 l
S
n
216.222 665.938 m
216.522 665.485 l
S
n
216.522 665.485 m
217.183 664.691 l
S
n
218.383 663.273 m
219.163 662.309 l
S
n
219.163 662.309 m
219.464 662.026 l
S
n
220.844 660.609 m
221.805 659.587 l
S
n
221.805 659.587 m
222.045 659.361 l
S
n
223.545 658 m
224.445 657.207 l
S
n
224.445 657.207 m
224.865 656.866 l
S
n
226.367 655.732 m
227.027 655.221 l
S
n
227.027 655.221 m
227.688 654.767 l
S
n
229.188 653.803 m
229.668 653.52 l
S
n
229.668 653.52 m
230.508 653.009 l
S
n
232.01 652.216 m
232.309 652.045 l
S
n
232.309 652.045 m
233.328 651.535 l
S
n
234.83 650.855 m
234.951 650.798 l
S
n
234.951 650.798 m
236.15 650.345 l
S
n
237.651 649.777 m
238.972 649.38 l
S
31.0869 672.231 m
/N5 [-0.014801 11.9999 -11.9999 -0.014801 0 0] Tf
(Fraction of coiled state) show
166.652 595.375 m
/N5 12 Tf
([PEG] \(mg/mL\)) show
n
255.578 714.059 m
243.738 744.102 l
f
n
252.182 714.85 m
258.859 705.83 l
257.587 716.981 l
h
f
0 j
0 J
n
255.578 714.059 m
243.738 744.102 l
S
n
252.182 714.85 m
258.859 705.83 l
257.587 716.981 l
h
f
n
168.119 721.278 m
181.525 691.901 l
f
n
171.551 720.667 m
164.409 729.323 l
166.266 718.254 l
h
f
[2 ] 0 d
n
168.119 721.278 m
181.525 691.901 l
S
n
171.551 720.667 m
164.409 729.323 l
166.266 718.254 l
h
f
258.078 729.218 m
(fol) show
(d)
[7.31991 ] pdfxs
(ing) show
119.784 695.33 m
(unfolding) show
Q
Q
q
101.9 509.084 142.407 27.2155 re
W
0.999985 0 0 0.999985 101.9 509.085 cm
0 w
q
Q
Q
q
99.3683 509.086 109.494 22.1509 re
W
0.999985 0 0 0.999985 99.3685 509.086 cm
0 w
q
Q
[/DeviceGray] cs 0 sc
0 6.383 m
/N93 12 Tf
(Figure 4, Shew et al. ) show
Q
q
198.737 336.299 100 100 re
W
0.999985 0 0 0.999985 198.737 336.299 cm
0 w
q
Q
Q
q
253.168 450.857 100 100 re
W
0.999985 0 0 0.999985 253.168 450.857 cm
0 w
q
Q
Q
PDFVars/TermAll get exec end end
restore

%%EndDocument

LH
(%%[Page: 4]%%) = 
%%PageTrailer

%%Page: 5 5
%%PageBoundingBox: 12 13 598 780
%%EndPageComments
%%BeginPageSetup
/DeviceRGB dup setcolorspace /colspABC exch def
mysetup concat colspRefresh
%%EndPageSetup

%%BeginDocument: Pscript_Win_PassThrough
PDFVars begin PDF begin PDFVars/InitAll get exec
save
0 0 612 792 true PDF begin PDFVars begin AS end end
0 0 612 792 re
W
n
false setSA
{} settransfer
n
176.1 606.66 m
176.1 607.44 l
176.88 607.44 l
179.28 606.9 l
179.28 606.06 l
178.5 606.06 l
[/CIEBasedABC  9 dict 
dup /CreationDate (19980209064900) put
dup /RenderingIntent (RelativeColorimetric) put
dup /Description (sRGB IEC61966-2.1) put
dup /ColorSpace (RGB ) put
dup /Copyright (Copyright (c) 1998 Hewlett-Packard Company) put
dup /DecodeLMN [

{{0.0000 0.0003 0.0006 0.0009 0.0012 0.0015 0.0018 0.0021 0.0024 0.0027 0.0030 0.0034 0.0037 0.0040 0.0044 0.0048 
0.0052 0.0056 0.0060 0.0065 0.0070 0.0075 0.0080 0.0086 0.0091 0.0097 0.0103 0.0110 0.0116 0.0123 0.0130 0.0137 
0.0144 0.0152 0.0160 0.0168 0.0176 0.0185 0.0194 0.0203 0.0212 0.0222 0.0232 0.0242 0.0252 0.0262 0.0273 0.0284 
0.0296 0.0307 0.0319 0.0331 0.0343 0.0356 0.0369 0.0382 0.0395 0.0409 0.0423 0.0437 0.0452 0.0467 0.0482 0.0497 
0.0513 0.0529 0.0545 0.0561 0.0578 0.0595 0.0612 0.0630 0.0648 0.0666 0.0685 0.0704 0.0723 0.0742 0.0762 0.0782 
0.0802 0.0823 0.0844 0.0865 0.0886 0.0908 0.0931 0.0953 0.0976 0.0999 0.1022 0.1046 0.1070 0.1095 0.1119 0.1144 
0.1170 0.1195 0.1221 0.1248 0.1274 0.1301 0.1329 0.1356 0.1384 0.1413 0.1441 0.1470 0.1500 0.1529 0.1559 0.1590 
0.1620 0.1651 0.1683 0.1714 0.1746 0.1779 0.1812 0.1845 0.1878 0.1912 0.1946 0.1981 0.2016 0.2051 0.2086 0.2122 
0.2159 0.2195 0.2232 0.2270 0.2307 0.2346 0.2384 0.2423 0.2462 0.2502 0.2542 0.2582 0.2622 0.2664 0.2705 0.2747 
0.2789 0.2832 0.2874 0.2918 0.2961 0.3005 0.3050 0.3095 0.3140 0.3185 0.3231 0.3278 0.3325 0.3372 0.3419 0.3467 
0.3515 0.3564 0.3613 0.3663 0.3712 0.3763 0.3813 0.3864 0.3916 0.3967 0.4020 0.4072 0.4125 0.4179 0.4233 0.4287 
0.4342 0.4397 0.4452 0.4508 0.4564 0.4621 0.4678 0.4735 0.4793 0.4851 0.4910 0.4969 0.5029 0.5089 0.5149 0.5210 
0.5271 0.5333 0.5395 0.5457 0.5520 0.5583 0.5647 0.5711 0.5776 0.5841 0.5906 0.5972 0.6038 0.6105 0.6172 0.6240 
0.6308 0.6376 0.6445 0.6514 0.6584 0.6654 0.6724 0.6795 0.6867 0.6939 0.7011 0.7084 0.7157 0.7231 0.7305 0.7379 
0.7454 0.7529 0.7605 0.7682 0.7758 0.7835 0.7913 0.7991 0.8069 0.8148 0.8228 0.8308 0.8388 0.8469 0.8550 0.8632 
0.8714 0.8796 0.8879 0.8963 0.9047 0.9131 0.9216 0.9301 0.9387 0.9473 0.9560 0.9647 0.9734 0.9822 0.9911 1.0000 }
dup 3 -1 roll 0.0000 1.0000 3 copy 3 -1 roll exch ge
{pop pop pop pop pop 255 get}
{pop 3 copy pop le{pop pop pop pop 0 get}{exch dup 4 -1 roll exch sub 3 1 roll sub div 255 mul dup floor dup 3 1 roll sub exch cvi dup 1 add 4 -1 roll exch get 4 -1 roll 3 -1 roll get dup 4 1 roll sub mul add}
ifelse}ifelse}bind
{{0.0000 0.0003 0.0006 0.0009 0.0012 0.0015 0.0018 0.0021 0.0024 0.0027 0.0030 0.0034 0.0037 0.0040 0.0044 0.0048 
0.0052 0.0056 0.0060 0.0065 0.0070 0.0075 0.0080 0.0086 0.0091 0.0097 0.0103 0.0110 0.0116 0.0123 0.0130 0.0137 
0.0144 0.0152 0.0160 0.0168 0.0176 0.0185 0.0194 0.0203 0.0212 0.0222 0.0232 0.0242 0.0252 0.0262 0.0273 0.0284 
0.0296 0.0307 0.0319 0.0331 0.0343 0.0356 0.0369 0.0382 0.0395 0.0409 0.0423 0.0437 0.0452 0.0467 0.0482 0.0497 
0.0513 0.0529 0.0545 0.0561 0.0578 0.0595 0.0612 0.0630 0.0648 0.0666 0.0685 0.0704 0.0723 0.0742 0.0762 0.0782 
0.0802 0.0823 0.0844 0.0865 0.0886 0.0908 0.0931 0.0953 0.0976 0.0999 0.1022 0.1046 0.1070 0.1095 0.1119 0.1144 
0.1170 0.1195 0.1221 0.1248 0.1274 0.1301 0.1329 0.1356 0.1384 0.1413 0.1441 0.1470 0.1500 0.1529 0.1559 0.1590 
0.1620 0.1651 0.1683 0.1714 0.1746 0.1779 0.1812 0.1845 0.1878 0.1912 0.1946 0.1981 0.2016 0.2051 0.2086 0.2122 
0.2159 0.2195 0.2232 0.2270 0.2307 0.2346 0.2384 0.2423 0.2462 0.2502 0.2542 0.2582 0.2622 0.2664 0.2705 0.2747 
0.2789 0.2832 0.2874 0.2918 0.2961 0.3005 0.3050 0.3095 0.3140 0.3185 0.3231 0.3278 0.3325 0.3372 0.3419 0.3467 
0.3515 0.3564 0.3613 0.3663 0.3712 0.3763 0.3813 0.3864 0.3916 0.3967 0.4020 0.4072 0.4125 0.4179 0.4233 0.4287 
0.4342 0.4397 0.4452 0.4508 0.4564 0.4621 0.4678 0.4735 0.4793 0.4851 0.4910 0.4969 0.5029 0.5089 0.5149 0.5210 
0.5271 0.5333 0.5395 0.5457 0.5520 0.5583 0.5647 0.5711 0.5776 0.5841 0.5906 0.5972 0.6038 0.6105 0.6172 0.6240 
0.6308 0.6376 0.6445 0.6514 0.6584 0.6654 0.6724 0.6795 0.6867 0.6939 0.7011 0.7084 0.7157 0.7231 0.7305 0.7379 
0.7454 0.7529 0.7605 0.7682 0.7758 0.7835 0.7913 0.7991 0.8069 0.8148 0.8228 0.8308 0.8388 0.8469 0.8550 0.8632 
0.8714 0.8796 0.8879 0.8963 0.9047 0.9131 0.9216 0.9301 0.9387 0.9473 0.9560 0.9647 0.9734 0.9822 0.9911 1.0000 }
dup 3 -1 roll 0.0000 1.0000 3 copy 3 -1 roll exch ge
{pop pop pop pop pop 255 get}
{pop 3 copy pop le{pop pop pop pop 0 get}{exch dup 4 -1 roll exch sub 3 1 roll sub div 255 mul dup floor dup 3 1 roll sub exch cvi dup 1 add 4 -1 roll exch get 4 -1 roll 3 -1 roll get dup 4 1 roll sub mul add}
ifelse}ifelse}bind
{{0.0000 0.0003 0.0006 0.0009 0.0012 0.0015 0.0018 0.0021 0.0024 0.0027 0.0030 0.0034 0.0037 0.0040 0.0044 0.0048 
0.0052 0.0056 0.0060 0.0065 0.0070 0.0075 0.0080 0.0086 0.0091 0.0097 0.0103 0.0110 0.0116 0.0123 0.0130 0.0137 
0.0144 0.0152 0.0160 0.0168 0.0176 0.0185 0.0194 0.0203 0.0212 0.0222 0.0232 0.0242 0.0252 0.0262 0.0273 0.0284 
0.0296 0.0307 0.0319 0.0331 0.0343 0.0356 0.0369 0.0382 0.0395 0.0409 0.0423 0.0437 0.0452 0.0467 0.0482 0.0497 
0.0513 0.0529 0.0545 0.0561 0.0578 0.0595 0.0612 0.0630 0.0648 0.0666 0.0685 0.0704 0.0723 0.0742 0.0762 0.0782 
0.0802 0.0823 0.0844 0.0865 0.0886 0.0908 0.0931 0.0953 0.0976 0.0999 0.1022 0.1046 0.1070 0.1095 0.1119 0.1144 
0.1170 0.1195 0.1221 0.1248 0.1274 0.1301 0.1329 0.1356 0.1384 0.1413 0.1441 0.1470 0.1500 0.1529 0.1559 0.1590 
0.1620 0.1651 0.1683 0.1714 0.1746 0.1779 0.1812 0.1845 0.1878 0.1912 0.1946 0.1981 0.2016 0.2051 0.2086 0.2122 
0.2159 0.2195 0.2232 0.2270 0.2307 0.2346 0.2384 0.2423 0.2462 0.2502 0.2542 0.2582 0.2622 0.2664 0.2705 0.2747 
0.2789 0.2832 0.2874 0.2918 0.2961 0.3005 0.3050 0.3095 0.3140 0.3185 0.3231 0.3278 0.3325 0.3372 0.3419 0.3467 
0.3515 0.3564 0.3613 0.3663 0.3712 0.3763 0.3813 0.3864 0.3916 0.3967 0.4020 0.4072 0.4125 0.4179 0.4233 0.4287 
0.4342 0.4397 0.4452 0.4508 0.4564 0.4621 0.4678 0.4735 0.4793 0.4851 0.4910 0.4969 0.5029 0.5089 0.5149 0.5210 
0.5271 0.5333 0.5395 0.5457 0.5520 0.5583 0.5647 0.5711 0.5776 0.5841 0.5906 0.5972 0.6038 0.6105 0.6172 0.6240 
0.6308 0.6376 0.6445 0.6514 0.6584 0.6654 0.6724 0.6795 0.6867 0.6939 0.7011 0.7084 0.7157 0.7231 0.7305 0.7379 
0.7454 0.7529 0.7605 0.7682 0.7758 0.7835 0.7913 0.7991 0.8069 0.8148 0.8228 0.8308 0.8388 0.8469 0.8550 0.8632 
0.8714 0.8796 0.8879 0.8963 0.9047 0.9131 0.9216 0.9301 0.9387 0.9473 0.9560 0.9647 0.9734 0.9822 0.9911 1.0000 }
dup 3 -1 roll 0.0000 1.0000 3 copy 3 -1 roll exch ge
{pop pop pop pop pop 255 get}
{pop 3 copy pop le{pop pop pop pop 0 get}{exch dup 4 -1 roll exch sub 3 1 roll sub div 255 mul dup floor dup 3 1 roll sub exch cvi dup 1 add 4 -1 roll exch get 4 -1 roll 3 -1 roll get dup 4 1 roll sub mul add}
ifelse}ifelse}bind] put
dup /MatrixLMN [0.4361 0.2225 0.0139 0.3851 0.7169 0.0971 0.1431 0.0606 0.7141] put
dup /WhitePoint [0.9642 1.0000 0.8249] put]
/E1 exch /ColorSpace defineRes

cs 0 0 0 sc
f
n
182.52 605.04 m
182.52 605.88 l
183.36 605.88 l
185.7 605.22 l
185.7 604.5 l
184.92 604.5 l
f
n
188.94 602.82 m
188.94 603.66 l
189.72 603.66 l
192.12 602.64 l
192.12 601.86 l
191.34 601.86 l
f
n
194.52 599.22 m
194.52 600.06 l
195.3 600.06 l
196.5 597.66 l
196.5 596.88 l
195.72 596.88 l
f
n
197.52 592.86 m
197.52 593.64 l
198.36 593.64 l
199.56 591.24 l
199.56 590.4 l
198.72 590.4 l
f
n
200.76 586.26 m
200.76 587.04 l
201.54 587.04 l
202.5 584.64 l
202.5 583.86 l
201.78 583.86 l
f
n
203.52 579.84 m
203.52 580.62 l
204.36 580.62 l
205.38 578.22 l
205.38 577.44 l
204.54 577.44 l
f
n
206.34 573.42 m
206.34 574.26 l
207.12 574.26 l
208.14 571.8 l
208.14 571.02 l
207.36 571.02 l
f
n
209.16 567.18 m
209.16 568.02 l
209.94 568.02 l
211.14 565.62 l
211.14 564.78 l
210.36 564.78 l
f
n
212.94 561 m
212.94 561.84 l
213.72 561.84 l
216.12 559.8 l
216.12 558.96 l
215.34 558.96 l
f
n
219.54 555.84 m
219.54 556.56 l
220.38 556.56 l
221.16 556.02 l
221.16 555.18 l
220.38 555.18 l
f
n
220.38 555.18 m
220.38 556.02 l
221.16 556.02 l
222.78 555.18 l
222.78 554.4 l
221.94 554.4 l
f
n
225.96 552.24 m
225.96 552.96 l
226.74 552.96 l
229.14 551.58 l
229.14 550.8 l
228.36 550.8 l
f
n
232.2 549.36 m
232.2 550.2 l
232.98 550.2 l
235.38 549.36 l
235.38 548.58 l
234.6 548.58 l
f
n
238.56 547.38 m
238.56 548.16 l
239.34 548.16 l
241.74 547.38 l
241.74 546.6 l
241.02 546.6 l
f
n
245.16 545.4 m
245.16 546.18 l
246 546.18 l
247.56 545.58 l
247.56 544.8 l
246.78 544.8 l
f
n
246.78 544.8 m
246.78 545.58 l
247.56 545.58 l
248.4 545.4 l
248.4 544.56 l
247.56 544.56 l
f
n
251.64 543.96 m
251.64 544.8 l
252.36 544.8 l
254.82 544.38 l
254.82 543.6 l
253.98 543.6 l
f
n
257.82 542.76 m
257.82 543.6 l
258.6 543.6 l
261.18 543.18 l
261.18 542.4 l
260.4 542.4 l
f
n
264.6 541.56 m
264.6 542.4 l
265.44 542.4 l
267.84 542.16 l
267.84 541.38 l
267 541.38 l
f
n
271.02 540.96 m
271.02 541.8 l
271.8 541.8 l
274.2 541.38 l
274.2 540.6 l
273.42 540.6 l
f
n
277.26 540.18 m
277.26 540.96 l
278.04 540.96 l
280.44 540.6 l
280.44 539.76 l
279.6 539.76 l
f
n
283.44 539.4 m
283.44 540.18 l
284.22 540.18 l
286.62 539.76 l
286.62 538.98 l
285.84 538.98 l
f
n
289.86 538.8 m
289.86 539.58 l
290.64 539.58 l
293.04 539.4 l
293.04 538.56 l
292.26 538.56 l
f
n
296.46 538.14 m
296.46 538.98 l
297.24 538.98 l
299.64 538.8 l
299.64 537.96 l
298.86 537.96 l
f
n
303.06 537.6 m
303.06 538.38 l
303.84 538.38 l
306.24 538.14 l
306.24 537.36 l
305.46 537.36 l
f
n
176.1 606.06 m
176.1 606.9 l
176.88 606.9 l
179.28 606.24 l
179.28 605.46 l
178.5 605.46 l
f
n
182.52 604.68 m
182.52 605.46 l
183.36 605.46 l
185.7 604.86 l
185.7 604.02 l
184.92 604.02 l
f
n
188.94 602.04 m
188.94 602.82 l
189.72 602.82 l
192.12 601.44 l
192.12 600.66 l
191.34 600.66 l
f
n
194.76 597.84 m
194.76 598.68 l
195.54 598.68 l
196.92 596.22 l
196.92 595.44 l
196.14 595.44 l
f
n
198.36 591.42 m
198.36 592.26 l
199.08 592.26 l
200.76 589.68 l
200.76 588.84 l
199.92 588.84 l
f
n
202.5 584.4 m
202.5 585.24 l
203.34 585.24 l
204.36 582.84 l
204.36 582 l
203.52 582 l
f
n
205.14 578.22 m
205.14 579.06 l
205.92 579.06 l
206.94 576.66 l
206.94 575.82 l
206.1 575.82 l
f
n
207.54 572.04 m
207.54 572.82 l
208.32 572.82 l
209.34 570.42 l
209.34 569.64 l
208.56 569.64 l
f
n
209.94 565.8 m
209.94 566.64 l
210.72 566.64 l
211.74 563.82 l
211.74 563.04 l
210.96 563.04 l
f
n
214.56 559.62 m
214.56 560.4 l
215.34 560.4 l
217.74 558.42 l
217.74 557.58 l
216.96 557.58 l
f
n
221.16 554.64 m
221.16 555.36 l
221.94 555.36 l
224.34 553.98 l
224.34 553.2 l
223.56 553.2 l
f
n
227.58 551.04 m
227.58 551.76 l
228.36 551.76 l
229.98 551.04 l
229.98 550.2 l
229.14 550.2 l
f
n
229.14 550.2 m
229.14 551.04 l
229.98 551.04 l
230.76 550.8 l
230.76 550.02 l
229.98 550.02 l
f
n
233.4 549 m
233.4 549.78 l
234.18 549.78 l
236.76 549 l
236.76 548.16 l
235.98 548.16 l
f
n
240.18 546.78 m
240.18 547.62 l
241.02 547.62 l
243.42 546.78 l
243.42 546 l
242.58 546 l
f
n
246.78 544.8 m
246.78 545.58 l
247.56 545.58 l
249.78 545.22 l
249.78 544.38 l
249 544.38 l
f
n
252.78 543.78 m
252.78 544.56 l
253.56 544.56 l
256.02 544.2 l
256.02 543.36 l
255.18 543.36 l
f
n
259.02 542.58 m
259.02 543.36 l
259.8 543.36 l
262.2 543 l
262.2 542.16 l
261.42 542.16 l
f
n
265.44 541.56 m
265.44 542.4 l
266.16 542.4 l
268.62 541.98 l
268.62 541.2 l
267.84 541.2 l
f
n
271.8 540.78 m
271.8 541.56 l
272.64 541.56 l
275.04 541.2 l
275.04 540.36 l
274.2 540.36 l
f
n
278.22 540 m
278.22 540.78 l
279 540.78 l
281.46 540.36 l
281.46 539.58 l
280.62 539.58 l
f
n
284.64 539.16 m
284.64 540 l
285.42 540 l
287.46 539.76 l
287.46 538.98 l
286.62 538.98 l
f
n
286.62 539.76 1.62 -0.780029 re
f
n
291.42 538.8 m
291.42 539.58 l
292.26 539.58 l
294.66 539.4 l
294.66 538.56 l
293.82 538.56 l
f
n
297.84 538.14 m
297.84 538.98 l
298.62 538.98 l
301.02 538.8 l
301.02 537.96 l
300.24 537.96 l
f
n
304.26 537.78 m
304.26 538.56 l
305.04 538.56 l
307.44 538.38 l
307.44 537.6 l
306.66 537.6 l
f
n
177.9 436.08 m
177.9 436.86 l
178.74 436.86 l
179.46 436.68 l
179.46 435.84 l
178.74 435.84 l
f
n
182.88 435.48 m
182.88 436.26 l
183.72 436.26 l
187.74 435.66 l
187.74 434.88 l
186.9 434.88 l
f
n
190.92 435.48 1.62 -0.839996 re
f
n
195.72 435.24 3.17999 -0.779999 re
f
n
198.12 434.46 m
198.12 435.24 l
198.9 435.24 l
200.34 435.06 l
200.34 434.28 l
199.56 434.28 l
f
n
203.52 434.64 1.62 -0.779999 re
f
n
208.56 433.68 m
208.56 434.46 l
209.34 434.46 l
213.54 434.28 l
213.54 433.44 l
212.76 433.44 l
f
n
216.78 434.04 1.56 -0.779999 re
f
n
221.58 432.84 m
221.58 433.68 l
222.36 433.68 l
225.54 433.44 l
225.54 432.66 l
224.76 432.66 l
f
n
224.76 433.44 1.44 -0.779999 re
f
n
229.14 433.08 1.62 -0.839996 re
f
n
234.36 431.88 m
234.36 432.66 l
235.2 432.66 l
239.16 432.42 l
239.16 431.64 l
238.38 431.64 l
f
n
242.4 432.42 1.56 -0.779999 re
f
n
247.02 431.46 m
247.02 432.24 l
247.8 432.24 l
251.4 431.88 l
251.4 431.04 l
250.62 431.04 l
f
n
254.58 431.46 1.62001 -0.779999 re
f
n
259.38 430.86 1.62 -0.839996 re
f
n
260.22 430.86 4.01999 -0.839996 re
f
n
267.36 430.68 1.67999 -0.839996 re
f
n
272.22 429.66 m
272.22 430.44 l
273 430.44 l
277.02 430.26 l
277.02 429.48 l
276.24 429.48 l
f
n
280.2 430.02 1.62 -0.779999 re
f
n
285.06 429.84 2.39999 -0.779999 re
f
n
286.62 429.84 3.23999 -0.779999 re
f
n
293.04 429.66 1.62 -0.839996 re
f
n
297.84 428.64 m
297.84 429.48 l
298.62 429.48 l
302.64 429.06 l
302.64 428.28 l
301.86 428.28 l
f
n
305.88 428.82 1.56 -0.779999 re
f
n
310.68 428.64 3.17999 -0.779999 re
f
n
313.08 428.64 2.39999 -0.779999 re
f
n
318.9 428.46 1.56 -0.839996 re
f
n
323.7 427.26 m
323.7 428.04 l
324.48 428.04 l
328.26 427.86 l
328.26 427.08 l
327.48 427.08 l
f
n
331.68 427.62 1.56 -0.779999 re
f
n
336.48 427.44 4.02002 -0.839996 re
f
n
339.72 427.44 1.56 -0.839996 re
f
n
344.52 427.26 1.56 -0.839996 re
f
n
349.32 426.06 m
349.32 426.84 l
350.1 426.84 l
353.88 426.24 l
353.88 425.4 l
353.1 425.4 l
f
n
357.48 425.88 1.67999 -0.839996 re
f
n
362.34 426.06 4.80002 -0.839996 re
f
n
370.32 426.06 1.62 -0.839996 re
f
n
375.12 425.4 m
375.12 426.24 l
375.9 426.24 l
379.74 426.06 l
379.74 425.22 l
378.96 425.22 l
f
n
382.92 426.06 1.85999 -0.839996 re
f
n
387.96 425.04 m
387.96 425.88 l
388.74 425.88 l
392.76 425.64 l
392.76 424.86 l
391.98 424.86 l
f
n
396 425.4 1.56 -0.720001 re
f
n
400.98 424.86 1.56 -0.839996 re
f
n
401.76 424.86 3.66 -0.839996 re
f
n
408.78 424.86 1.80002 -0.839996 re
f
n
413.82 424.02 m
413.82 424.86 l
414.6 424.86 l
418.56 424.68 l
418.56 423.84 l
417.78 423.84 l
f
n
420 421.62 m
420 422.46 l
420.78 422.46 l
420.96 421.62 l
420.96 420.84 l
420.18 420.84 l
f
n
421.2 417 m
421.2 417.84 l
421.98 417.84 l
423.18 414.06 l
423.18 413.22 l
422.4 413.22 l
f
n
423.36 409.2 m
423.36 410.04 l
424.2 410.04 l
424.38 409.2 l
424.38 408.42 l
423.6 408.42 l
f
n
424.8 404.22 m
424.8 405 l
425.58 405 l
426.78 400.98 l
426.78 400.2 l
426 400.2 l
f
n
427.2 396 m
427.2 396.84 l
427.98 396.84 l
428.16 396 l
428.16 395.16 l
427.44 395.16 l
f
n
428.4 391.2 m
428.4 392.04 l
429.18 392.04 l
429.36 388.2 l
429.36 387.42 l
428.64 387.42 l
f
n
429 384.36 0.839996 -1.56 re
f
n
429.36 378.78 m
429.36 379.56 l
430.2 379.56 l
430.62 375.6 l
430.62 374.82 l
429.84 374.82 l
f
n
430.2 371.58 0.839996 -1.56 re
f
n
430.62 365.94 m
430.62 366.78 l
431.4 366.78 l
431.58 362.82 l
431.58 361.98 l
430.8 361.98 l
f
n
431.22 358.74 0.779999 -1.56 re
f
n
431.58 353.16 m
431.58 353.94 l
432.42 353.94 l
432.78 349.92 l
432.78 349.14 l
432 349.14 l
f
n
432.42 345.96 0.779999 -1.62 re
f
n
432.78 340.32 m
432.78 341.16 l
433.62 341.16 l
433.8 337.14 l
433.8 336.36 l
433.02 336.36 l
f
n
433.44 333.12 0.779999 -1.56 re
f
n
433.8 327.54 m
433.8 328.32 l
434.64 328.32 l
435 324.3 l
435 323.52 l
434.22 323.52 l
f
n
434.64 320.34 0.779999 -1.62 re
f
n
435 314.7 m
435 315.54 l
435.84 315.54 l
436.02 311.46 l
436.02 310.74 l
435.18 310.74 l
f
n
435.6 307.5 0.839996 -1.56 re
f
n
436.02 301.92 m
436.02 302.7 l
436.8 302.7 l
437.22 298.68 l
437.22 297.9 l
436.44 297.9 l
f
n
436.62 294.72 0.779999 -1.62 re
f
n
437.04 288.9 m
437.04 289.68 l
437.82 289.68 l
441.6 289.44 l
441.6 288.72 l
440.82 288.72 l
f
n
445.02 289.44 1.79999 -0.720001 re
f
n
450 288.48 m
450 289.26 l
450.84 289.26 l
454.8 289.08 l
454.8 288.24 l
454.08 288.24 l
f
n
458.04 289.08 1.62 -0.839996 re
f
n
462.66 289.08 1.62 -0.839996 re
f
n
177.9 436.08 m
177.9 436.86 l
178.74 436.86 l
179.46 436.68 l
179.46 435.84 l
178.74 435.84 l
f
n
182.88 435.48 m
182.88 436.26 l
183.72 436.26 l
187.74 436.08 l
187.74 435.24 l
186.9 435.24 l
f
n
190.74 433.68 m
190.74 434.46 l
191.52 434.46 l
192.3 433.68 l
192.3 432.84 l
191.52 432.84 l
f
n
195.12 428.82 m
195.12 429.66 l
195.96 429.66 l
198.9 426.42 l
198.9 425.64 l
198.12 425.64 l
f
n
198.12 425.64 m
198.12 426.42 l
198.9 426.42 l
199.08 425.64 l
199.08 424.86 l
198.36 424.86 l
f
n
198.72 421.26 m
198.72 422.04 l
199.56 422.04 l
199.74 421.26 l
199.74 420.42 l
198.9 420.42 l
f
n
199.56 416.46 m
199.56 417.24 l
200.34 417.24 l
200.94 413.22 l
200.94 412.44 l
200.1 412.44 l
f
n
200.58 408.42 m
200.58 409.2 l
201.3 409.2 l
201.54 408.42 l
201.54 407.64 l
200.76 407.64 l
f
n
201.12 403.62 m
201.12 404.4 l
201.96 404.4 l
202.5 400.44 l
202.5 399.6 l
201.78 399.6 l
f
n
202.14 395.64 m
202.14 396.36 l
202.98 396.36 l
203.16 395.64 l
203.16 394.8 l
202.32 394.8 l
f
n
202.98 390.84 m
202.98 391.56 l
203.7 391.56 l
204.36 387.6 l
204.36 386.76 l
203.52 386.76 l
f
n
203.94 382.8 m
203.94 383.58 l
204.72 383.58 l
204.9 382.8 l
204.9 381.96 l
204.18 381.96 l
f
n
204.54 378 m
204.54 378.78 l
205.38 378.78 l
205.92 374.82 l
205.92 373.98 l
205.14 373.98 l
f
n
205.56 370.02 m
205.56 370.74 l
206.34 370.74 l
206.58 370.02 l
206.58 369.18 l
205.74 369.18 l
f
n
206.34 364.74 m
206.34 365.58 l
207.12 365.58 l
207.78 361.38 l
207.78 360.6 l
206.94 360.6 l
f
n
207.78 356.76 m
207.78 357.54 l
208.56 357.54 l
208.74 356.76 l
208.74 355.98 l
207.96 355.98 l
f
n
208.98 352.14 m
208.98 352.98 l
209.76 352.98 l
210.54 349.14 l
210.54 348.36 l
209.76 348.36 l
f
n
210.72 344.34 m
210.72 345.12 l
211.56 345.12 l
211.74 344.34 l
211.74 343.56 l
210.96 343.56 l
f
n
211.92 339.54 m
211.92 340.32 l
212.76 340.32 l
213.72 336.36 l
213.72 335.52 l
212.94 335.52 l
f
n
213.72 331.32 m
213.72 332.1 l
214.56 332.1 l
214.74 331.32 l
214.74 330.54 l
213.96 330.54 l
f
n
214.92 326.52 m
214.92 327.3 l
215.76 327.3 l
216.54 323.1 l
216.54 322.32 l
215.76 322.32 l
f
n
218.76 319.32 m
218.76 320.1 l
219.54 320.1 l
220.38 319.5 l
220.38 318.72 l
219.54 318.72 l
f
n
223.98 315.3 m
223.98 316.08 l
224.76 316.08 l
225.54 315.54 l
225.54 314.7 l
224.76 314.7 l
f
n
224.76 314.7 m
224.76 315.54 l
225.54 315.54 l
228.78 312.66 l
228.78 311.94 l
227.94 311.94 l
f
n
231.96 308.52 m
231.96 309.3 l
232.74 309.3 l
233.58 308.52 l
233.58 307.68 l
232.74 307.68 l
f
n
236.76 304.74 m
236.76 305.46 l
237.6 305.46 l
241.56 302.52 l
241.56 301.68 l
240.78 301.68 l
f
n
245.34 300.9 m
244.62 300.9 l
244.62 301.68 l
245.34 301.92 l
246.18 301.92 l
246.18 301.08 l
f
n
250.44 301.92 m
249.6 301.92 l
249.6 302.7 l
251.4 302.88 l
252.18 302.88 l
252.18 302.1 l
f
n
251.4 302.1 m
251.4 302.88 l
252.18 302.88 l
254.58 301.92 l
254.58 301.08 l
253.8 301.08 l
f
n
257.82 299.28 m
257.82 300.12 l
258.6 300.12 l
259.38 299.7 l
259.38 298.92 l
258.6 298.92 l
f
n
262.38 297.9 m
262.38 298.68 l
263.22 298.68 l
267 298.32 l
267 297.48 l
266.16 297.48 l
f
n
270.6 297.9 1.62 -0.779999 re
f
n
275.4 296.88 m
275.4 297.66 l
276.24 297.66 l
278.64 297.48 l
278.64 296.7 l
277.8 296.7 l
f
n
277.8 296.7 m
277.8 297.48 l
278.64 297.48 l
280.2 297.3 l
280.2 296.46 l
279.42 296.46 l
f
n
283.44 297.12 1.62 -0.839996 re
f
n
288 295.92 m
288 296.7 l
288.84 296.7 l
292.62 296.46 l
292.62 295.68 l
291.84 295.68 l
f
n
296.22 296.28 1.62 -0.779999 re
f
n
301.02 295.26 m
301.02 296.1 l
301.86 296.1 l
305.04 295.92 l
305.04 295.08 l
304.26 295.08 l
f
n
304.26 295.92 1.62 -0.839996 re
f
n
309.06 295.92 1.62 -0.839996 re
f
n
313.86 294.9 m
313.86 295.68 l
314.64 295.68 l
318.24 295.08 l
318.24 294.3 l
317.52 294.3 l
f
n
321.3 293.7 m
321.3 294.48 l
322.08 294.48 l
322.86 294.3 l
322.86 293.52 l
322.08 293.52 l
f
n
326.1 293.28 m
326.1 294.06 l
326.88 294.06 l
330.9 293.7 l
330.9 292.86 l
330.12 292.86 l
f
n
334.08 293.52 1.62 -0.839996 re
f
n
338.88 293.28 1.62 -0.779999 re
f
n
339.72 292.5 m
339.72 293.28 l
340.5 293.28 l
343.68 293.1 l
343.68 292.32 l
342.9 292.32 l
f
n
346.92 292.68 1.56 -0.839996 re
f
n
351.72 291.66 m
351.72 292.5 l
352.5 292.5 l
356.76 292.32 l
356.76 291.48 l
355.92 291.48 l
f
n
359.88 292.08 1.67999 -0.779999 re
f
n
364.74 291.84 2.39999 -0.720001 re
f
n
366.36 291.84 3.17999 -0.720001 re
f
n
372.54 291.84 1.62 -0.720001 re
f
n
377.58 290.88 m
377.58 291.66 l
378.3 291.66 l
382.38 291.3 l
382.38 290.46 l
381.54 290.46 l
f
n
385.56 291.12 1.62 -0.839996 re
f
n
390.36 291.12 3.17999 -0.839996 re
f
n
392.76 291.12 2.39999 -0.839996 re
f
n
398.4 290.88 1.56 -0.779999 re
f
n
403.38 289.92 m
403.38 290.64 l
404.22 290.64 l
408.18 290.46 l
408.18 289.68 l
407.34 289.68 l
f
n
411.42 290.46 1.56 -0.779999 re
f
n
416.16 290.28 4.01999 -0.839996 re
f
n
419.4 290.28 1.56 -0.839996 re
f
n
424.02 290.1 1.56 -0.839996 re
f
n
429 289.08 m
429 289.92 l
429.84 289.92 l
433.8 289.68 l
433.8 288.9 l
433.02 288.9 l
f
n
437.04 289.68 1.56 -0.779999 re
f
n
442.02 289.44 4.79999 -0.720001 re
f
n
449.64 289.26 1.56 -0.779999 re
f
n
454.8 289.08 4.85999 -0.839996 re
f
n
462.66 289.08 1.62 -0.839996 re
f
n
176.1 530.94 m
176.1 531.78 l
176.88 531.78 l
185.7 530.94 l
185.7 530.16 l
184.92 530.16 l
f
n
184.92 530.16 m
184.92 530.94 l
185.7 530.94 l
194.52 530.4 l
194.52 529.56 l
193.74 529.56 l
f
n
193.74 529.56 m
193.74 530.4 l
194.52 530.4 l
203.34 529.74 l
203.34 528.96 l
202.5 528.96 l
f
n
202.5 528.96 m
202.5 529.74 l
203.34 529.74 l
212.16 528.96 l
212.16 528.18 l
211.38 528.18 l
f
n
211.38 528.18 m
211.38 528.96 l
212.16 528.96 l
221.16 528.36 l
221.16 527.52 l
220.38 527.52 l
f
n
220.38 527.52 m
220.38 528.36 l
221.16 528.36 l
229.98 527.76 l
229.98 526.98 l
229.14 526.98 l
f
n
229.14 526.98 m
229.14 527.76 l
229.98 527.76 l
238.8 527.34 l
238.8 526.56 l
237.96 526.56 l
f
n
237.96 526.56 m
237.96 527.34 l
238.8 527.34 l
247.56 526.8 l
247.56 525.96 l
246.78 525.96 l
f
n
246.78 525.96 m
246.78 526.8 l
247.56 526.8 l
256.38 526.32 l
256.38 525.6 l
255.6 525.6 l
f
n
255.6 525.6 m
255.6 526.32 l
256.38 526.32 l
265.44 525.78 l
265.44 524.94 l
264.6 524.94 l
f
n
264.6 524.94 m
264.6 525.78 l
265.44 525.78 l
274.2 525.36 l
274.2 524.58 l
273.42 524.58 l
f
n
273.42 524.58 m
273.42 525.36 l
274.2 525.36 l
283.02 524.94 l
283.02 524.16 l
282.24 524.16 l
f
n
282.24 524.16 m
282.24 524.94 l
283.02 524.94 l
291.84 524.58 l
291.84 523.74 l
291.06 523.74 l
f
n
291.06 523.74 m
291.06 524.58 l
291.84 524.58 l
300.66 524.16 l
300.66 523.38 l
299.82 523.38 l
f
n
299.82 523.38 m
299.82 524.16 l
300.66 524.16 l
309.66 523.74 l
309.66 522.96 l
308.82 522.96 l
f
n
308.82 522.96 m
308.82 523.74 l
309.66 523.74 l
318.48 519.78 l
318.48 518.94 l
317.7 518.94 l
f
n
317.7 518.94 m
317.7 519.78 l
318.48 519.78 l
327.3 468.06 l
327.3 467.28 l
326.46 467.28 l
f
n
326.46 467.28 m
326.46 468.06 l
327.3 468.06 l
336.12 464.7 l
336.12 463.92 l
335.28 463.92 l
f
n
335.28 463.92 m
335.28 464.7 l
336.12 464.7 l
344.88 460.08 l
344.88 459.3 l
344.1 459.3 l
f
n
344.1 459.3 m
344.1 460.08 l
344.88 460.08 l
353.88 456.66 l
353.88 455.88 l
353.1 455.88 l
f
n
353.1 455.88 m
353.1 456.66 l
353.88 456.66 l
362.76 453.66 l
362.76 452.88 l
361.92 452.88 l
f
n
176.1 530.94 m
176.1 531.78 l
176.88 531.78 l
185.7 530.94 l
185.7 530.16 l
184.92 530.16 l
f
n
184.92 530.16 m
184.92 530.94 l
185.7 530.94 l
194.52 530.4 l
194.52 529.56 l
193.74 529.56 l
f
n
193.74 529.56 m
193.74 530.4 l
194.52 530.4 l
203.34 529.74 l
203.34 528.96 l
202.5 528.96 l
f
n
202.5 528.96 m
202.5 529.74 l
203.34 529.74 l
212.16 528.96 l
212.16 528.18 l
211.38 528.18 l
f
n
211.38 528.18 m
211.38 528.96 l
212.16 528.96 l
221.16 528.36 l
221.16 527.52 l
220.38 527.52 l
f
n
220.38 527.52 m
220.38 528.36 l
221.16 528.36 l
229.98 527.76 l
229.98 526.98 l
229.14 526.98 l
f
n
229.14 526.98 m
229.14 527.76 l
229.98 527.76 l
238.8 527.34 l
238.8 526.56 l
237.96 526.56 l
f
n
237.96 526.56 m
237.96 527.34 l
238.8 527.34 l
247.56 526.8 l
247.56 525.96 l
246.78 525.96 l
f
n
246.78 525.96 m
246.78 526.8 l
247.56 526.8 l
256.38 526.32 l
256.38 525.6 l
255.6 525.6 l
f
n
255.6 525.6 m
255.6 526.32 l
256.38 526.32 l
265.44 492.12 l
265.44 491.34 l
264.6 491.34 l
f
n
264.6 491.34 m
264.6 492.12 l
265.44 492.12 l
274.2 478.14 l
274.2 477.3 l
273.42 477.3 l
f
n
273.42 477.3 m
273.42 478.14 l
274.2 478.14 l
283.02 477.12 l
283.02 476.28 l
282.24 476.28 l
f
n
282.24 476.28 m
282.24 477.12 l
283.02 477.12 l
291.84 475.92 l
291.84 475.08 l
291.06 475.08 l
f
n
291.06 475.08 m
291.06 475.92 l
291.84 475.92 l
300.66 474.72 l
300.66 473.88 l
299.82 473.88 l
f
n
299.82 473.88 m
299.82 474.72 l
300.66 474.72 l
309.66 473.1 l
309.66 472.32 l
308.82 472.32 l
f
n
308.82 472.32 m
308.82 473.1 l
309.66 473.1 l
318.48 470.94 l
318.48 470.1 l
317.7 470.1 l
f
n
317.7 470.1 m
317.7 470.94 l
318.48 470.94 l
327.3 468.06 l
327.3 467.28 l
326.46 467.28 l
f
n
326.46 467.28 m
326.46 468.06 l
327.3 468.06 l
336.12 464.7 l
336.12 463.92 l
335.28 463.92 l
f
n
335.28 463.92 m
335.28 464.7 l
336.12 464.7 l
344.88 460.08 l
344.88 459.3 l
344.1 459.3 l
f
n
344.1 459.3 m
344.1 460.08 l
344.88 460.08 l
353.88 456.48 l
353.88 455.64 l
353.1 455.64 l
f
n
353.1 455.64 m
353.1 456.48 l
353.88 456.48 l
362.76 453.9 l
362.76 453.06 l
361.92 453.06 l
f
1 J
1 j
0.192001 w
10 M
[] 0 d
n
176.52 298.32 m
181.5 298.32 l
176.52 382.62 m
181.5 382.62 l
176.52 466.86 m
181.5 466.86 l
176.52 551.04 m
181.5 551.04 l
176.52 273.06 m
179.1 273.06 l
176.52 279.66 m
179.1 279.66 l
176.52 285.3 m
179.1 285.3 l
176.52 290.28 m
179.1 290.28 l
176.52 294.48 m
179.1 294.48 l
176.52 323.7 m
179.1 323.7 l
176.52 338.58 m
179.1 338.58 l
176.52 349.14 m
179.1 349.14 l
176.52 357.18 m
179.1 357.18 l
176.52 364.02 m
179.1 364.02 l
176.52 369.54 m
179.1 369.54 l
176.52 374.4 m
179.1 374.4 l
176.52 378.78 m
179.1 378.78 l
176.52 408 m
179.1 408 l
176.52 422.82 m
179.1 422.82 l
176.52 433.26 m
179.1 433.26 l
176.52 441.48 m
179.1 441.48 l
176.52 448.08 m
179.1 448.08 l
176.52 453.9 m
179.1 453.9 l
176.52 458.7 m
179.1 458.7 l
176.52 462.9 m
179.1 462.9 l
176.52 492.12 m
179.1 492.12 l
176.52 506.94 m
179.1 506.94 l
176.52 517.56 m
179.1 517.56 l
176.52 525.78 m
179.1 525.78 l
176.52 532.32 m
179.1 532.32 l
176.52 537.96 m
179.1 537.96 l
176.52 543 m
179.1 543 l
176.52 547.2 m
179.1 547.2 l
176.52 576.42 m
179.1 576.42 l
176.52 591.24 m
179.1 591.24 l
176.52 601.86 m
179.1 601.86 l
176.52 610.02 m
179.1 610.02 l
464.04 298.32 m
459.06 298.32 l
464.04 382.62 m
459.06 382.62 l
464.04 466.86 m
459.06 466.86 l
464.04 551.04 m
459.06 551.04 l
464.04 273.06 m
461.46 273.06 l
464.04 279.66 m
461.46 279.66 l
464.04 285.3 m
461.46 285.3 l
464.04 290.28 m
461.46 290.28 l
464.04 294.48 m
461.46 294.48 l
464.04 323.7 m
461.46 323.7 l
464.04 338.58 m
461.46 338.58 l
464.04 349.14 m
461.46 349.14 l
464.04 357.18 m
461.46 357.18 l
464.04 364.02 m
461.46 364.02 l
464.04 369.54 m
461.46 369.54 l
464.04 374.4 m
461.46 374.4 l
464.04 378.78 m
461.46 378.78 l
464.04 408 m
461.46 408 l
464.04 422.82 m
461.46 422.82 l
464.04 433.26 m
461.46 433.26 l
464.04 441.48 m
461.46 441.48 l
464.04 448.08 m
461.46 448.08 l
464.04 453.9 m
461.46 453.9 l
464.04 458.7 m
461.46 458.7 l
464.04 462.9 m
461.46 462.9 l
464.04 492.12 m
461.46 492.12 l
464.04 506.94 m
461.64 506.94 l
0 0 0.830994 sc
S
n
461.64 506.94 m
461.46 506.94 l
464.04 517.56 m
461.46 517.56 l
464.04 525.78 m
461.46 525.78 l
464.04 532.32 m
461.46 532.32 l
464.04 537.96 m
461.46 537.96 l
464.04 543 m
461.46 543 l
464.04 547.2 m
461.46 547.2 l
464.04 576.42 m
461.46 576.42 l
464.04 591.24 m
461.46 591.24 l
464.04 601.86 m
461.46 601.86 l
464.04 610.02 m
461.46 610.02 l
176.52 273.06 m
176.52 278.1 l
211.74 273.06 m
211.74 278.1 l
247.2 273.06 m
247.2 278.1 l
282.66 273.06 m
282.66 278.1 l
318.06 273.06 m
318.06 278.1 l
353.52 273.06 m
353.52 278.1 l
388.74 273.06 m
388.74 278.1 l
424.2 273.06 m
424.2 278.1 l
459.66 273.06 m
459.66 278.1 l
185.28 273.06 m
185.28 275.7 l
194.1 273.06 m
194.1 275.7 l
202.98 273.06 m
202.98 275.7 l
220.74 273.06 m
220.74 275.7 l
229.56 273.06 m
229.56 275.7 l
238.38 273.06 m
238.38 275.7 l
256.02 273.06 m
256.02 275.7 l
265.02 273.06 m
265.02 275.7 l
273.84 273.06 m
273.84 275.7 l
291.42 273.06 m
291.42 275.7 l
300.24 273.06 m
300.24 275.7 l
309.3 273.06 m
309.3 275.7 l
326.88 273.06 m
326.88 275.7 l
335.7 273.06 m
335.7 275.7 l
344.52 273.06 m
344.52 275.7 l
362.34 273.06 m
362.34 275.7 l
371.16 273.06 m
371.16 275.7 l
S
n
379.98 273.06 m
379.98 275.7 l
397.56 273.06 m
397.56 275.7 l
406.38 273.06 m
406.38 275.7 l
415.38 273.06 m
415.38 275.7 l
433.02 273.06 m
433.02 275.7 l
441.78 273.06 m
441.78 275.7 l
450.66 273.06 m
450.66 275.7 l
176.52 616.68 m
176.52 611.7 l
211.74 616.68 m
211.74 611.7 l
247.2 616.68 m
247.2 611.7 l
282.66 616.68 m
282.66 611.7 l
318.06 616.68 m
318.06 611.7 l
353.52 616.68 m
353.52 611.7 l
388.74 616.68 m
388.74 611.7 l
424.2 616.68 m
424.2 611.7 l
459.66 616.68 m
459.66 611.7 l
185.28 616.68 m
185.28 614.1 l
194.1 616.68 m
194.1 614.1 l
202.98 616.68 m
202.98 614.1 l
220.74 616.68 m
220.74 614.1 l
229.56 616.68 m
229.56 614.1 l
238.38 616.68 m
238.38 614.1 l
256.02 616.68 m
256.02 614.1 l
265.02 616.68 m
265.02 614.1 l
273.84 616.68 m
273.84 614.1 l
291.42 616.68 m
291.42 614.1 l
300.24 616.68 m
300.24 614.1 l
309.3 616.68 m
309.3 614.1 l
326.88 616.68 m
326.88 614.1 l
335.7 616.68 m
335.7 614.1 l
344.52 616.68 m
344.52 614.1 l
362.34 616.68 m
362.34 614.1 l
371.16 616.68 m
371.16 614.1 l
379.98 616.68 m
379.98 614.1 l
397.56 616.68 m
397.56 614.1 l
406.38 616.68 m
406.38 614.1 l
415.38 616.68 m
415.38 614.1 l
433.02 616.68 m
433.02 614.1 l
441.78 616.68 m
441.78 614.1 l
450.66 616.68 m
450.66 614.1 l
S
n
176.1 617.04 0.779999 -344.4 re
f
n
463.62 617.04 0.839996 -344.4 re
f
n
176.1 273.48 288.36 -0.839996 re
f
n
176.1 617.04 288.36 -0.779968 re
f
n
174.12 609.48 5.16 -5.21997 re
0 0 0 sc
f
n
174.12 609.48 m
174.12 604.5 l
174.12 604.68 m
179.1 604.68 l
178.92 604.68 m
178.92 609.66 l
178.92 609.48 m
173.94 609.48 l
S
n
182.88 607.26 5.22 -5.21997 re
f
n
182.88 607.26 m
182.88 602.28 l
182.88 602.46 m
187.92 602.46 l
187.74 602.46 m
187.74 607.44 l
187.74 607.26 m
182.7 607.26 l
S
n
191.7 603.66 5.22 -5.21997 re
f
n
191.7 603.66 m
191.7 598.68 l
191.7 598.86 m
196.74 598.86 l
196.5 598.86 m
196.5 603.84 l
196.5 603.66 m
191.52 603.66 l
S
n
200.58 585.06 5.16 -5.22003 re
f
n
200.58 585.06 m
200.58 580.08 l
200.58 580.26 m
205.56 580.26 l
205.38 580.26 m
205.38 585.24 l
205.38 585.06 m
200.34 585.06 l
S
n
209.34 565.2 5.22 -5.22003 re
f
n
209.34 565.2 m
209.34 560.16 l
209.34 560.4 m
214.38 560.4 l
214.14 560.4 m
214.14 565.44 l
214.14 565.2 m
209.16 565.2 l
S
n
218.34 558 5.22 -5.21997 re
f
n
218.34 558 m
218.34 552.96 l
218.34 553.2 m
223.32 553.2 l
223.14 553.2 m
223.14 558.24 l
223.14 558 m
218.16 558 l
S
n
227.16 553.2 5.22 -5.22003 re
f
n
227.16 553.2 m
227.16 548.16 l
227.16 548.4 m
232.2 548.4 l
231.96 548.4 m
231.96 553.44 l
231.96 553.2 m
226.92 553.2 l
S
n
244.8 547.62 5.16 -5.21997 re
f
n
244.8 547.62 m
244.8 542.58 l
244.8 542.76 m
249.78 542.76 l
249.6 542.76 m
249.6 547.8 l
249.6 547.62 m
244.62 547.62 l
S
n
262.62 544.38 5.22 -5.21997 re
f
n
262.62 544.38 m
262.62 539.4 l
262.62 539.58 m
267.6 539.58 l
267.36 539.58 m
267.36 544.56 l
267.36 544.38 m
262.38 544.38 l
S
n
284.64 541.8 5.22 -5.22003 re
f
n
284.64 541.8 m
284.64 536.76 l
284.64 536.94 m
289.68 536.94 l
289.44 536.94 m
289.44 541.98 l
289.44 541.8 m
284.4 541.8 l
S
n
306.84 540 5.22 -5.21997 re
f
n
306.84 540 m
306.84 534.96 l
306.84 535.2 m
311.88 535.2 l
311.7 535.2 m
311.7 540.18 l
311.7 540 m
306.66 540 l
174.12 608.82 m
174.12 603.84 l
174.12 604.02 m
179.1 604.02 l
178.92 604.02 m
178.92 609.06 l
178.92 608.82 m
173.94 608.82 l
182.88 606.9 m
182.88 601.86 l
182.88 602.04 m
187.92 602.04 l
187.74 602.04 m
187.74 607.08 l
187.74 606.9 m
182.7 606.9 l
191.7 602.28 m
191.7 597.24 l
191.7 597.48 m
196.74 597.48 l
196.5 597.48 m
196.5 602.46 l
196.5 602.28 m
191.52 602.28 l
200.58 587.28 m
200.58 582.24 l
200.58 582.48 m
205.56 582.48 l
205.38 582.48 m
205.38 587.46 l
205.38 587.28 m
200.34 587.28 l
209.34 565.02 m
209.34 559.98 l
209.34 560.16 m
214.38 560.16 l
214.14 560.16 m
214.14 565.2 l
214.14 565.02 m
209.16 565.02 l
218.34 557.76 m
218.34 552.78 l
218.34 552.96 m
223.32 552.96 l
223.14 552.96 m
223.14 558 l
223.14 557.76 m
218.16 557.76 l
227.16 552.96 m
227.16 547.98 l
227.16 548.16 m
232.2 548.16 l
231.96 548.16 m
231.96 553.2 l
231.96 552.96 m
226.92 552.96 l
244.8 547.62 m
244.8 542.58 l
244.8 542.76 m
249.78 542.76 l
249.6 542.76 m
249.6 547.8 l
249.6 547.62 m
244.62 547.62 l
262.62 544.38 m
262.62 539.4 l
262.62 539.58 m
267.6 539.58 l
267.36 539.58 m
267.36 544.56 l
267.36 544.38 m
262.38 544.38 l
284.64 541.8 m
284.64 536.76 l
284.64 536.94 m
289.68 536.94 l
289.44 536.94 m
289.44 541.98 l
289.44 541.8 m
284.4 541.8 l
306.84 540.18 m
306.84 535.2 l
306.84 535.38 m
311.88 535.38 l
311.7 535.38 m
311.7 540.36 l
311.7 540.18 m
306.66 540.18 l
S
n
174.12 434.46 m
176.52 439.26 l
178.92 434.46 l
174.12 434.46 l
eofill
n
174.12 434.46 m
176.52 439.26 l
178.92 434.46 l
174.12 434.46 l
S
n
178.5 433.68 m
180.96 438.48 l
183.36 433.68 l
178.5 433.68 l
eofill
n
178.5 433.68 m
180.96 438.48 l
183.36 433.68 l
178.5 433.68 l
S
n
187.32 432.66 m
189.72 437.46 l
192.12 432.66 l
187.32 432.66 l
eofill
n
187.32 432.66 m
189.72 437.46 l
192.12 432.66 l
187.32 432.66 l
S
n
196.14 432.42 m
198.54 437.28 l
200.94 432.42 l
196.14 432.42 l
eofill
n
196.14 432.42 m
198.54 437.28 l
200.94 432.42 l
196.14 432.42 l
S
n
204.9 431.64 m
207.36 436.44 l
209.76 431.64 l
204.9 431.64 l
eofill
n
204.9 431.64 m
207.36 436.44 l
209.76 431.64 l
204.9 431.64 l
S
n
213.96 431.22 m
216.36 436.08 l
218.76 431.22 l
213.96 431.22 l
eofill
n
213.96 431.22 m
216.36 436.08 l
218.76 431.22 l
213.96 431.22 l
S
n
222.78 430.68 m
225.18 435.48 l
227.58 430.68 l
222.78 430.68 l
eofill
n
222.78 430.68 m
225.18 435.48 l
227.58 430.68 l
222.78 430.68 l
S
n
231.54 429.84 m
233.94 434.64 l
236.4 429.84 l
231.54 429.84 l
eofill
n
231.54 429.84 m
233.94 434.64 l
236.4 429.84 l
231.54 429.84 l
S
n
240.36 429.66 m
242.76 434.46 l
245.16 429.66 l
240.36 429.66 l
eofill
n
240.36 429.66 m
242.76 434.46 l
245.16 429.66 l
240.36 429.66 l
S
n
249.42 429.06 m
251.82 433.86 l
254.22 429.06 l
249.42 429.06 l
eofill
n
249.42 429.06 m
251.82 433.86 l
254.22 429.06 l
249.42 429.06 l
S
n
258.18 428.04 m
260.58 432.84 l
263.04 428.04 l
258.18 428.04 l
eofill
n
258.18 428.04 m
260.58 432.84 l
263.04 428.04 l
258.18 428.04 l
S
n
267 427.86 m
269.4 432.66 l
271.8 427.86 l
267 427.86 l
eofill
n
267 427.86 m
269.4 432.66 l
271.8 427.86 l
267 427.86 l
S
n
275.82 427.26 m
278.22 432.06 l
280.62 427.26 l
275.82 427.26 l
eofill
n
275.82 427.26 m
278.22 432.06 l
280.62 427.26 l
275.82 427.26 l
S
n
284.64 427.08 m
287.04 431.88 l
289.44 427.08 l
284.64 427.08 l
eofill
n
284.64 427.08 m
287.04 431.88 l
289.44 427.08 l
284.64 427.08 l
S
n
293.46 426.84 m
295.86 431.64 l
298.26 426.84 l
293.46 426.84 l
eofill
n
293.46 426.84 m
295.86 431.64 l
298.26 426.84 l
293.46 426.84 l
S
n
302.28 426.06 m
304.68 430.86 l
307.08 426.06 l
302.28 426.06 l
eofill
n
302.28 426.06 m
304.68 430.86 l
307.08 426.06 l
302.28 426.06 l
S
n
311.04 425.88 m
313.44 430.68 l
315.84 425.88 l
311.04 425.88 l
eofill
n
311.04 425.88 m
313.44 430.68 l
315.84 425.88 l
311.04 425.88 l
S
n
320.1 425.4 m
322.5 430.26 l
324.9 425.4 l
320.1 425.4 l
eofill
n
320.1 425.4 m
322.5 430.26 l
324.9 425.4 l
320.1 425.4 l
S
n
328.92 424.86 m
331.32 429.66 l
333.72 424.86 l
328.92 424.86 l
eofill
n
328.92 424.86 m
331.32 429.66 l
333.72 424.86 l
328.92 424.86 l
S
n
337.68 424.68 m
340.08 429.48 l
342.48 424.68 l
337.68 424.68 l
eofill
n
337.68 424.68 m
340.08 429.48 l
342.48 424.68 l
337.68 424.68 l
S
n
346.5 424.2 m
348.9 429.06 l
351.3 424.2 l
346.5 424.2 l
eofill
n
346.5 424.2 m
348.9 429.06 l
351.3 424.2 l
346.5 424.2 l
S
n
355.56 423 m
357.96 427.86 l
360.36 423 l
355.56 423 l
eofill
n
355.56 423 m
357.96 427.86 l
360.36 423 l
355.56 423 l
S
n
364.32 423.24 m
366.72 428.04 l
369.12 423.24 l
364.32 423.24 l
eofill
n
364.32 423.24 m
366.72 428.04 l
369.12 423.24 l
364.32 423.24 l
S
n
373.14 423.48 m
375.54 428.28 l
377.94 423.48 l
373.14 423.48 l
eofill
n
373.14 423.48 m
375.54 428.28 l
377.94 423.48 l
373.14 423.48 l
S
n
381.9 423.24 m
384.36 428.04 l
386.76 423.24 l
381.9 423.24 l
eofill
n
381.9 423.24 m
384.36 428.04 l
386.76 423.24 l
381.9 423.24 l
S
n
390.78 422.82 m
393.18 427.62 l
395.58 422.82 l
390.78 422.82 l
eofill
n
390.78 422.82 m
393.18 427.62 l
395.58 422.82 l
390.78 422.82 l
S
n
399.78 422.04 m
402.18 426.84 l
404.58 422.04 l
399.78 422.04 l
eofill
n
399.78 422.04 m
402.18 426.84 l
404.58 422.04 l
399.78 422.04 l
S
n
408.54 422.04 m
411 426.84 l
413.4 422.04 l
408.54 422.04 l
eofill
n
408.54 422.04 m
411 426.84 l
413.4 422.04 l
408.54 422.04 l
S
n
417.36 421.8 m
419.76 426.6 l
422.16 421.8 l
417.36 421.8 l
eofill
n
417.36 421.8 m
419.76 426.6 l
422.16 421.8 l
417.36 421.8 l
S
n
426.24 390.84 m
428.64 395.64 l
431.04 390.84 l
426.24 390.84 l
eofill
n
426.24 390.84 m
428.64 395.64 l
431.04 390.84 l
426.24 390.84 l
S
n
435 286.86 m
437.4 291.66 l
439.8 286.86 l
435 286.86 l
eofill
n
435 286.86 m
437.4 291.66 l
439.8 286.86 l
435 286.86 l
S
n
444 286.68 m
446.4 291.48 l
448.8 286.68 l
444 286.68 l
eofill
n
444 286.68 m
446.4 291.48 l
448.8 286.68 l
444 286.68 l
S
n
452.88 286.32 m
455.22 291.12 l
457.62 286.32 l
452.88 286.32 l
eofill
n
452.88 286.32 m
455.22 291.12 l
457.62 286.32 l
452.88 286.32 l
S
n
461.64 286.08 m
464.04 290.88 l
466.44 286.08 l
461.64 286.08 l
eofill
n
461.64 286.08 m
464.04 290.88 l
466.44 286.08 l
461.64 286.08 l
174.12 434.46 m
176.52 439.26 l
178.92 434.46 l
174.12 434.46 l
178.5 433.68 m
180.96 438.48 l
183.36 433.68 l
178.5 433.68 l
187.32 433.26 m
189.72 438.06 l
192.12 433.26 l
187.32 433.26 l
196.14 423.66 m
198.54 428.46 l
200.94 423.66 l
196.14 423.66 l
204.9 358.56 m
207.36 363.36 l
209.76 358.56 l
204.9 358.56 l
213.96 319.5 m
216.36 324.3 l
218.76 319.5 l
213.96 319.5 l
222.78 312.66 m
225.18 317.52 l
227.58 312.66 l
222.78 312.66 l
231.54 305.1 m
233.94 309.9 l
236.4 305.1 l
231.54 305.1 l
240.36 298.5 m
242.76 303.3 l
245.16 298.5 l
240.36 298.5 l
249.42 300.12 m
251.82 304.92 l
254.22 300.12 l
249.42 300.12 l
258.18 296.1 m
260.58 300.9 l
263.04 296.1 l
258.18 296.1 l
267 295.26 m
269.4 300.12 l
271.8 295.26 l
267 295.26 l
275.82 294.72 m
278.22 299.52 l
280.62 294.72 l
275.82 294.72 l
284.64 294.06 m
287.04 298.92 l
289.44 294.06 l
284.64 294.06 l
293.46 293.52 m
295.86 298.32 l
298.26 293.52 l
293.46 293.52 l
302.28 293.1 m
304.68 297.9 l
307.08 293.1 l
302.28 293.1 l
311.04 293.1 m
313.44 297.9 l
315.84 293.1 l
311.04 293.1 l
320.1 291.48 m
322.5 296.28 l
324.9 291.48 l
320.1 291.48 l
328.92 290.88 m
331.32 295.68 l
333.72 290.88 l
328.92 290.88 l
337.68 290.46 m
340.08 295.26 l
342.48 290.46 l
337.68 290.46 l
346.5 289.92 m
348.9 294.72 l
351.3 289.92 l
346.5 289.92 l
355.56 289.44 m
357.96 294.3 l
360.36 289.44 l
355.56 289.44 l
364.32 289.08 m
366.72 293.88 l
369.12 289.08 l
364.32 289.08 l
373.14 289.08 m
375.54 293.88 l
377.94 289.08 l
373.14 289.08 l
381.9 288.24 m
384.36 293.1 l
386.76 288.24 l
381.9 288.24 l
390.78 288.24 m
393.18 293.1 l
395.58 288.24 l
390.78 288.24 l
399.78 287.88 m
402.18 292.68 l
404.58 287.88 l
399.78 287.88 l
408.54 287.7 m
411 292.5 l
413.4 287.7 l
408.54 287.7 l
417.36 287.52 m
419.76 292.32 l
422.16 287.52 l
417.36 287.52 l
426.24 287.04 m
428.64 291.84 l
431.04 287.04 l
426.24 287.04 l
435 286.86 m
437.4 291.66 l
439.8 286.86 l
435 286.86 l
S
n
444 286.68 m
446.4 291.48 l
448.8 286.68 l
444 286.68 l
452.88 286.32 m
455.22 291.12 l
457.62 286.32 l
452.88 286.32 l
461.64 286.08 m
464.04 290.88 l
466.44 286.08 l
461.64 286.08 l
S
n
179.04 531.3 m
179.04 532.68 177.9 533.82 176.58 533.82 c
175.2 533.82 174.06 532.68 174.06 531.3 c
174.06 529.98 175.2 528.84 176.58 528.84 c
177.9 528.84 179.04 529.98 179.04 531.3 c
eofill
n
178.32 529.56 m
178.8 529.98 179.1 530.64 179.1 531.3 c
179.1 532.68 177.96 533.76 176.58 533.76 c
175.2 533.76 174.12 532.68 174.12 531.3 c
174.12 529.92 175.2 528.78 176.58 528.78 c
177.24 528.78 177.9 529.08 178.32 529.56 c
S
n
187.86 530.52 m
187.86 531.9 186.72 533.04 185.34 533.04 c
183.96 533.04 182.82 531.9 182.82 530.52 c
182.82 529.2 183.96 528.06 185.34 528.06 c
186.72 528.06 187.86 529.2 187.86 530.52 c
eofill
n
187.14 528.78 m
187.62 529.2 187.92 529.86 187.92 530.52 c
187.92 531.9 186.78 532.98 185.4 532.98 c
183.96 532.98 182.88 531.9 182.88 530.52 c
182.88 529.14 183.96 528 185.4 528 c
186.06 528 186.66 528.3 187.14 528.78 c
S
n
196.68 529.86 m
196.68 531.24 195.54 532.38 194.16 532.38 c
192.78 532.38 191.64 531.24 191.64 529.86 c
191.64 528.54 192.78 527.4 194.16 527.4 c
195.54 527.4 196.68 528.54 196.68 529.86 c
eofill
n
195.96 528.12 m
196.44 528.54 196.74 529.2 196.74 529.86 c
196.74 531.24 195.6 532.32 194.22 532.32 c
192.78 532.32 191.7 531.24 191.7 529.86 c
191.7 528.48 192.78 527.34 194.22 527.34 c
194.88 527.34 195.48 527.64 195.96 528.12 c
S
n
205.5 529.32 m
205.5 530.7 204.36 531.84 203.04 531.84 c
201.66 531.84 200.52 530.7 200.52 529.32 c
200.52 528 201.66 526.86 203.04 526.86 c
204.36 526.86 205.5 528 205.5 529.32 c
eofill
n
204.78 527.58 m
205.26 528 205.56 528.66 205.56 529.32 c
205.56 530.7 204.42 531.78 203.04 531.78 c
201.66 531.78 200.58 530.7 200.58 529.32 c
200.58 527.94 201.66 526.8 203.04 526.8 c
203.7 526.8 204.36 527.1 204.78 527.58 c
S
n
214.26 528.48 m
214.26 529.86 213.12 531 211.8 531 c
210.42 531 209.28 529.86 209.28 528.48 c
209.28 527.16 210.42 526.02 211.8 526.02 c
213.12 526.02 214.26 527.16 214.26 528.48 c
eofill
n
213.54 526.74 m
214.02 527.16 214.32 527.82 214.32 528.48 c
214.32 529.86 213.18 530.94 211.8 530.94 c
210.42 530.94 209.34 529.86 209.34 528.48 c
209.34 527.1 210.42 525.96 211.8 525.96 c
212.46 525.96 213.12 526.26 213.54 526.74 c
S
n
223.26 527.94 m
223.26 529.32 222.12 530.46 220.8 530.46 c
219.42 530.46 218.28 529.32 218.28 527.94 c
218.28 526.56 219.42 525.42 220.8 525.42 c
222.12 525.42 223.26 526.56 223.26 527.94 c
eofill
n
222.54 526.14 m
223.02 526.62 223.32 527.22 223.32 527.88 c
223.32 529.32 222.18 530.4 220.8 530.4 c
219.42 530.4 218.34 529.32 218.34 527.88 c
218.34 526.5 219.42 525.36 220.8 525.36 c
221.46 525.36 222.12 525.66 222.54 526.14 c
S
n
232.14 527.28 m
232.14 528.66 231 529.8 229.62 529.8 c
228.24 529.8 227.1 528.66 227.1 527.28 c
227.1 525.96 228.24 524.82 229.62 524.82 c
231 524.82 232.14 525.96 232.14 527.28 c
eofill
n
231.42 525.54 m
231.9 525.96 232.2 526.62 232.2 527.28 c
232.2 528.66 231.06 529.74 229.68 529.74 c
228.24 529.74 227.16 528.66 227.16 527.28 c
227.16 525.9 228.24 524.76 229.68 524.76 c
230.34 524.76 230.94 525.06 231.42 525.54 c
S
n
240.9 526.92 m
240.9 528.3 239.76 529.44 238.44 529.44 c
237.06 529.44 235.92 528.3 235.92 526.92 c
235.92 525.6 237.06 524.46 238.44 524.46 c
239.76 524.46 240.9 525.6 240.9 526.92 c
eofill
n
240.18 525.18 m
240.66 525.6 240.96 526.26 240.96 526.92 c
240.96 528.3 239.82 529.38 238.44 529.38 c
237.06 529.38 235.98 528.3 235.98 526.92 c
235.98 525.54 237.06 524.4 238.44 524.4 c
239.1 524.4 239.76 524.7 240.18 525.18 c
S
n
249.72 526.32 m
249.72 527.64 248.58 528.78 247.26 528.78 c
245.88 528.78 244.74 527.64 244.74 526.32 c
244.74 524.94 245.88 523.86 247.26 523.86 c
248.58 523.86 249.72 524.94 249.72 526.32 c
eofill
n
249 524.52 m
249.48 525 249.78 525.66 249.78 526.26 c
249.78 527.64 248.64 528.72 247.26 528.72 c
245.88 528.72 244.8 527.64 244.8 526.26 c
244.8 524.94 245.88 523.8 247.26 523.8 c
247.92 523.8 248.58 524.1 249 524.52 c
S
n
258.54 525.9 m
258.54 527.28 257.4 528.42 256.02 528.42 c
254.64 528.42 253.5 527.28 253.5 525.9 c
253.5 524.58 254.64 523.44 256.02 523.44 c
257.4 523.44 258.54 524.58 258.54 525.9 c
eofill
n
257.82 524.16 m
258.3 524.58 258.6 525.24 258.6 525.9 c
258.6 527.28 257.46 528.36 256.08 528.36 c
254.64 528.36 253.56 527.28 253.56 525.9 c
253.56 524.52 254.64 523.38 256.08 523.38 c
256.74 523.38 257.34 523.68 257.82 524.16 c
S
n
267.54 525.3 m
267.54 526.68 266.4 527.82 265.08 527.82 c
263.7 527.82 262.56 526.68 262.56 525.3 c
262.56 523.98 263.7 522.84 265.08 522.84 c
266.4 522.84 267.54 523.98 267.54 525.3 c
eofill
n
266.82 523.56 m
267.3 523.98 267.6 524.64 267.6 525.3 c
267.6 526.68 266.46 527.76 265.08 527.76 c
263.7 527.76 262.62 526.68 262.62 525.3 c
262.62 523.92 263.7 522.78 265.08 522.78 c
265.74 522.78 266.4 523.08 266.82 523.56 c
S
n
276.36 524.88 m
276.36 526.26 275.22 527.4 273.9 527.4 c
272.52 527.4 271.38 526.26 271.38 524.88 c
271.38 523.56 272.52 522.42 273.9 522.42 c
275.22 522.42 276.36 523.56 276.36 524.88 c
eofill
n
275.64 523.14 m
276.12 523.56 276.42 524.22 276.42 524.88 c
276.42 526.26 275.28 527.34 273.9 527.34 c
272.52 527.34 271.44 526.26 271.44 524.88 c
271.44 523.5 272.52 522.36 273.9 522.36 c
274.56 522.36 275.22 522.66 275.64 523.14 c
S
n
285.18 524.52 m
285.18 525.9 284.04 527.04 282.66 527.04 c
281.28 527.04 280.14 525.9 280.14 524.52 c
280.14 523.2 281.28 522.06 282.66 522.06 c
284.04 522.06 285.18 523.2 285.18 524.52 c
eofill
n
284.46 522.78 m
284.94 523.2 285.24 523.86 285.24 524.52 c
285.24 525.9 284.1 526.98 282.72 526.98 c
281.28 526.98 280.2 525.9 280.2 524.52 c
280.2 523.14 281.28 522 282.72 522 c
283.38 522 283.98 522.3 284.46 522.78 c
S
n
293.94 524.1 m
293.94 525.48 292.8 526.62 291.48 526.62 c
290.1 526.62 288.96 525.48 288.96 524.1 c
288.96 522.78 290.1 521.64 291.48 521.64 c
292.8 521.64 293.94 522.78 293.94 524.1 c
eofill
n
293.22 522.36 m
293.7 522.78 294 523.44 294 524.1 c
294 525.48 292.86 526.56 291.48 526.56 c
290.1 526.56 289.02 525.48 289.02 524.1 c
289.02 522.72 290.1 521.58 291.48 521.58 c
292.14 521.58 292.8 521.88 293.22 522.36 c
S
n
302.82 523.68 m
302.82 525.06 301.68 526.2 300.3 526.2 c
298.92 526.2 297.78 525.06 297.78 523.68 c
297.78 522.36 298.92 521.22 300.3 521.22 c
301.68 521.22 302.82 522.36 302.82 523.68 c
eofill
n
302.1 521.94 m
302.58 522.36 302.88 523.02 302.88 523.68 c
302.88 525.06 301.74 526.14 300.36 526.14 c
298.92 526.14 297.84 525.06 297.84 523.68 c
297.84 522.3 298.92 521.16 300.36 521.16 c
301.02 521.16 301.62 521.46 302.1 521.94 c
S
n
311.82 523.32 m
311.82 524.7 310.68 525.84 309.3 525.84 c
307.92 525.84 306.78 524.7 306.78 523.32 c
306.78 522 307.92 520.86 309.3 520.86 c
310.68 520.86 311.82 522 311.82 523.32 c
eofill
n
311.1 521.58 m
311.58 522 311.88 522.66 311.88 523.32 c
311.88 524.7 310.74 525.78 309.36 525.78 c
307.92 525.78 306.84 524.7 306.84 523.32 c
306.84 521.94 307.92 520.8 309.36 520.8 c
310.02 520.8 310.62 521.1 311.1 521.58 c
S
n
320.58 519.3 m
320.58 520.68 319.44 521.82 318.12 521.82 c
316.74 521.82 315.6 520.68 315.6 519.3 c
315.6 517.98 316.74 516.84 318.12 516.84 c
319.44 516.84 320.58 517.98 320.58 519.3 c
eofill
n
319.86 517.56 m
320.34 517.98 320.64 518.64 320.64 519.3 c
320.64 520.68 319.5 521.76 318.12 521.76 c
316.74 521.76 315.66 520.68 315.66 519.3 c
315.66 517.92 316.74 516.78 318.12 516.78 c
318.78 516.78 319.44 517.08 319.86 517.56 c
S
n
329.4 467.64 m
329.4 469.02 328.26 470.16 326.94 470.16 c
325.56 470.16 324.42 469.02 324.42 467.64 c
324.42 466.32 325.56 465.18 326.94 465.18 c
328.26 465.18 329.4 466.32 329.4 467.64 c
eofill
n
328.68 465.9 m
329.16 466.32 329.46 466.98 329.46 467.64 c
329.46 469.02 328.32 470.1 326.94 470.1 c
325.56 470.1 324.48 469.02 324.48 467.64 c
324.48 466.26 325.56 465.12 326.94 465.12 c
327.6 465.12 328.26 465.42 328.68 465.9 c
S
n
338.22 464.22 m
338.22 465.6 337.08 466.74 335.7 466.74 c
334.32 466.74 333.18 465.6 333.18 464.22 c
333.18 462.9 334.32 461.76 335.7 461.76 c
337.08 461.76 338.22 462.9 338.22 464.22 c
eofill
n
337.5 462.48 m
337.98 462.9 338.28 463.56 338.28 464.22 c
338.28 465.6 337.14 466.68 335.76 466.68 c
334.32 466.68 333.24 465.6 333.24 464.22 c
333.24 462.84 334.32 461.7 335.76 461.7 c
336.42 461.7 337.02 462 337.5 462.48 c
S
n
347.04 459.6 m
347.04 460.98 345.9 462.12 344.58 462.12 c
343.2 462.12 342.06 460.98 342.06 459.6 c
342.06 458.28 343.2 457.14 344.58 457.14 c
345.9 457.14 347.04 458.28 347.04 459.6 c
eofill
n
346.32 457.86 m
346.8 458.28 347.1 458.94 347.1 459.6 c
347.1 460.98 345.96 462.06 344.58 462.06 c
343.2 462.06 342.12 460.98 342.12 459.6 c
342.12 458.22 343.2 457.08 344.58 457.08 c
345.24 457.08 345.9 457.38 346.32 457.86 c
S
n
356.04 456.24 m
356.04 457.62 354.9 458.76 353.58 458.76 c
352.2 458.76 351.06 457.62 351.06 456.24 c
351.06 454.92 352.2 453.78 353.58 453.78 c
354.9 453.78 356.04 454.92 356.04 456.24 c
eofill
n
355.32 454.5 m
355.8 454.92 356.1 455.58 356.1 456.24 c
356.1 457.62 354.96 458.7 353.58 458.7 c
352.2 458.7 351.12 457.62 351.12 456.24 c
351.12 454.86 352.2 453.72 353.58 453.72 c
354.24 453.72 354.9 454.02 355.32 454.5 c
S
n
364.86 453.18 m
364.86 454.56 363.72 455.7 362.34 455.7 c
360.96 455.7 359.82 454.56 359.82 453.18 c
359.82 451.86 360.96 450.72 362.34 450.72 c
363.72 450.72 364.86 451.86 364.86 453.18 c
eofill
n
364.14 451.44 m
364.62 451.86 364.92 452.52 364.92 453.18 c
364.92 454.56 363.78 455.64 362.4 455.64 c
360.96 455.64 359.88 454.56 359.88 453.18 c
359.88 451.8 360.96 450.66 362.4 450.66 c
363.06 450.66 363.66 450.96 364.14 451.44 c
178.32 529.56 m
178.8 529.98 179.1 530.64 179.1 531.3 c
179.1 532.68 177.96 533.76 176.58 533.76 c
175.2 533.76 174.12 532.68 174.12 531.3 c
174.12 529.92 175.2 528.78 176.58 528.78 c
177.24 528.78 177.9 529.08 178.32 529.56 c
187.14 528.78 m
187.62 529.2 187.92 529.86 187.92 530.52 c
187.92 531.9 186.78 532.98 185.4 532.98 c
183.96 532.98 182.88 531.9 182.88 530.52 c
182.88 529.14 183.96 528 185.4 528 c
186.06 528 186.66 528.3 187.14 528.78 c
195.96 528.12 m
196.44 528.54 196.74 529.2 196.74 529.86 c
196.74 531.24 195.6 532.32 194.22 532.32 c
192.78 532.32 191.7 531.24 191.7 529.86 c
191.7 528.48 192.78 527.34 194.22 527.34 c
194.88 527.34 195.48 527.64 195.96 528.12 c
204.78 527.58 m
205.26 528 205.56 528.66 205.56 529.32 c
205.56 530.7 204.42 531.78 203.04 531.78 c
201.66 531.78 200.58 530.7 200.58 529.32 c
200.58 527.94 201.66 526.8 203.04 526.8 c
203.7 526.8 204.36 527.1 204.78 527.58 c
213.54 526.74 m
214.02 527.16 214.32 527.82 214.32 528.48 c
214.32 529.86 213.18 530.94 211.8 530.94 c
210.42 530.94 209.34 529.86 209.34 528.48 c
209.34 527.1 210.42 525.96 211.8 525.96 c
212.46 525.96 213.12 526.26 213.54 526.74 c
222.54 526.14 m
223.02 526.62 223.32 527.22 223.32 527.88 c
223.32 529.32 222.18 530.4 220.8 530.4 c
219.42 530.4 218.34 529.32 218.34 527.88 c
218.34 526.5 219.42 525.36 220.8 525.36 c
221.46 525.36 222.12 525.66 222.54 526.14 c
231.42 525.54 m
231.9 525.96 232.2 526.62 232.2 527.28 c
232.2 528.66 231.06 529.74 229.68 529.74 c
228.24 529.74 227.16 528.66 227.16 527.28 c
227.16 525.9 228.24 524.76 229.68 524.76 c
230.34 524.76 230.94 525.06 231.42 525.54 c
240.18 525.18 m
240.66 525.6 240.96 526.26 240.96 526.92 c
240.96 528.3 239.82 529.38 238.44 529.38 c
237.06 529.38 235.98 528.3 235.98 526.92 c
235.98 525.54 237.06 524.4 238.44 524.4 c
239.1 524.4 239.76 524.7 240.18 525.18 c
249 524.52 m
249.48 525 249.78 525.66 249.78 526.26 c
249.78 527.64 248.64 528.72 247.26 528.72 c
245.88 528.72 244.8 527.64 244.8 526.26 c
244.8 524.94 245.88 523.8 247.26 523.8 c
247.92 523.8 248.58 524.1 249 524.52 c
257.82 524.16 m
258.3 524.58 258.6 525.24 258.6 525.9 c
258.6 527.28 257.46 528.36 256.08 528.36 c
254.64 528.36 253.56 527.28 253.56 525.9 c
253.56 524.52 254.64 523.38 256.08 523.38 c
256.74 523.38 257.34 523.68 257.82 524.16 c
266.82 489.9 m
267.3 490.38 267.6 490.98 267.6 491.64 c
267.6 493.08 266.46 494.16 265.08 494.16 c
263.7 494.16 262.62 493.08 262.62 491.64 c
262.62 490.26 263.7 489.12 265.08 489.12 c
265.74 489.12 266.4 489.42 266.82 489.9 c
275.64 475.86 m
276.12 476.34 276.42 476.94 276.42 477.6 c
276.42 479.04 275.28 480.12 273.9 480.12 c
272.52 480.12 271.44 479.04 271.44 477.6 c
271.44 476.22 272.52 475.08 273.9 475.08 c
274.56 475.08 275.22 475.38 275.64 475.86 c
284.46 474.9 m
284.94 475.32 285.24 475.98 285.24 476.64 c
285.24 478.02 284.1 479.1 282.72 479.1 c
281.28 479.1 280.2 478.02 280.2 476.64 c
280.2 475.26 281.28 474.12 282.72 474.12 c
283.38 474.12 283.98 474.42 284.46 474.9 c
293.22 473.7 m
293.7 474.12 294 474.78 294 475.44 c
294 476.82 292.86 477.9 291.48 477.9 c
290.1 477.9 289.02 476.82 289.02 475.44 c
289.02 474.06 290.1 472.92 291.48 472.92 c
292.14 472.92 292.8 473.22 293.22 473.7 c
302.1 472.5 m
302.58 472.92 302.88 473.58 302.88 474.24 c
302.88 475.62 301.74 476.7 300.36 476.7 c
298.92 476.7 297.84 475.62 297.84 474.24 c
297.84 472.86 298.92 471.72 300.36 471.72 c
301.02 471.72 301.62 472.02 302.1 472.5 c
311.1 470.88 m
311.58 471.3 311.88 471.96 311.88 472.62 c
311.88 474 310.74 475.08 309.36 475.08 c
307.92 475.08 306.84 474 306.84 472.62 c
306.84 471.24 307.92 470.1 309.36 470.1 c
310.02 470.1 310.62 470.4 311.1 470.88 c
319.86 468.66 m
320.34 469.08 320.64 469.74 320.64 470.4 c
320.64 471.78 319.5 472.86 318.12 472.86 c
316.74 472.86 315.66 471.78 315.66 470.4 c
315.66 469.02 316.74 467.88 318.12 467.88 c
318.78 467.88 319.44 468.18 319.86 468.66 c
328.68 465.9 m
329.16 466.32 329.46 466.98 329.46 467.64 c
329.46 469.02 328.32 470.1 326.94 470.1 c
325.56 470.1 324.48 469.02 324.48 467.64 c
324.48 466.26 325.56 465.12 326.94 465.12 c
327.6 465.12 328.26 465.42 328.68 465.9 c
337.5 462.48 m
337.98 462.9 338.28 463.56 338.28 464.22 c
338.28 465.6 337.14 466.68 335.76 466.68 c
334.32 466.68 333.24 465.6 333.24 464.22 c
333.24 462.84 334.32 461.7 335.76 461.7 c
336.42 461.7 337.02 462 337.5 462.48 c
346.32 457.86 m
346.8 458.28 347.1 458.94 347.1 459.6 c
347.1 460.98 345.96 462.06 344.58 462.06 c
343.2 462.06 342.12 460.98 342.12 459.6 c
342.12 458.22 343.2 457.08 344.58 457.08 c
345.24 457.08 345.9 457.38 346.32 457.86 c
355.32 454.26 m
355.8 454.68 356.1 455.34 356.1 456 c
356.1 457.38 354.96 458.46 353.58 458.46 c
352.2 458.46 351.12 457.38 351.12 456 c
351.12 454.62 352.2 453.48 353.58 453.48 c
354.24 453.48 354.9 453.78 355.32 454.26 c
S
n
364.14 451.62 m
364.62 452.1 364.92 452.7 364.92 453.36 c
364.92 454.8 363.78 455.88 362.4 455.88 c
360.96 455.88 359.88 454.8 359.88 453.36 c
359.88 451.98 360.96 450.84 362.4 450.84 c
363.06 450.84 363.66 451.14 364.14 451.62 c
S
148.5 293.52 m
/N295 9.5984 Tf
(0.001)
[5.32426 2.65591 5.39817 5.21868 5.32426 ] pdfxs
154.08 377.761 m
(0.01)
[5.39808 2.58191 5.45855 5.39808 ] pdfxs
159.659 462.06 m
(0.1)
[5.45856 2.58192 5.45856 ] pdfxs
167.699 546.181 m
(1) show
174.479 257.041 m
(08)
[35.2789 32.6383 ] pdfxs
(1) show
(6243240485664)
[30.0583 5.39808 30.0583 5.45855 29.9988 5.39808 29.8183 5.39808 30.0583 5.39808 29.9988 
5.45855 5.39808 ] pdfxs
145.26 423.66 m
/N292 [0 11.2301 -11.2301 0 0 0] Tf
(<R)
[6.59984 8.14943 ] pdfys
151.08 438.24 m
/N292 [0 7.19859 -7.19859 0 0 0] Tf
(g) show
139.5 442.68 m
(2) show
145.26 446.7 m
/N292 [0 11.2301 -11.2301 0 0 0] Tf
(>/)
[6.59984 3.16344 ] pdfys
0 J
0 j
0.119995 w
145.26 456.48 m
Adobe_CoolType_Utility begin ct_MakeOCF begin ct_GlyphDirProcs begin
/EKJCFC+SymbolMT 1
GetGlyphDirectory
42 <10bf31706ea9ea8b42c8f4a6c663e841cb0188bd1a5b15e559964e7b550a
adf412a5f94361a071e61528e127865b8849acc487fc85fc5479f5d4b722
c27149d866803cdb5c7dc3e2d3ab8eeed5b2b882b854c6639eb177fe65b6
1f03ef96957d6ede752f092ca4> |
!
end end end
/N287 [0 11.2301 -11.2301 0 0 0] Tf
(\000*) show
n
145.26 456.48 m
(\000*) pdf_strokepath
319.44 242.64 m
Adobe_CoolType_Utility begin ct_MakeOCF begin ct_GlyphDirProcs begin
/EKJCFC+SymbolMT 1
GetGlyphDirectory
72 <10bf31705d646aa7ff62a135113153bfc1301e38a62bd42355e80570774b
8ddd81a2e30c01184caaa78d0c7e9edc2b4bd6d1427148687e24ed207d7c
975ac82650d22a97dbf4cda81d6502b25adec63a92e05247858c5e90bce9
0b72c18839a78672268e7639145fe24eb3a60f1bb44e04c71cd5401cbf8e
7ec23b5a77318b186586c12609cfbd08f7f8d2125c0b62d165b4fc38d463
c8b4ad8bb8359921d7ffc597d0678a7dab8a1fa2b8314c58e3846c7050e4
ff529ffca13e0f79ba16e92538e481e76a53ae2bb0ac7bb0b564a66b29b2
381ae580db01b2d8b0ac728f328e8b6e7b3fafff78c77dec11aabbf2c618
9e862768e7b4760c2ccda118a30c77bd4e85673f9b0237f3aae6ca8fc82e
39e6460a0265d2b135a9344c3bec7df3904f05a9ba86b1a8> |
!
end end end
/N287 11.2301 Tf
(\000H) show
n
319.44 242.64 m
(\000H) pdf_strokepath
432 411.66 m
/N295 11.2301 Tf
(N=32)
[8.21798 6.35956 6.4786 6.35395 ] pdfxs
432 397.799 m
Adobe_CoolType_Utility begin ct_MakeOCF begin ct_GlyphDirProcs begin
/EKJCFC+SymbolMT 1
GetGlyphDirectory
78 <10bf31706754fb43ae25f5032c0179bc526ce11303f944386fa372164443
0219fc8ff84e9057e20d27eb529d8374d07afa0d7009ed80a12ac1ade50f
5af45655a30864ab3981a9a62d53a9f539aeabff16934353ee86e80fc671
33196ca6aafb3f142cc5cbdca3c852b52a1dc7be78509238b3461018a7a6
eabb46dba9f28e59ebb8dd88221eaf24c81bdfa4c343e14bfa93b3610562
1a18a1851ecf99a36887521a83cd6e7d681363473b4c245952fc73414790
a1b79f538a83> |
!
end end end
/N287 11.2301 Tf
(\000N) show
438.001 397.799 m
/N295 11.2301 Tf
(=20)
[6.6605 6.17874 6.34606 ] pdfxs
303.84 599.88 m
(N=8)
[8.21798 6.4202 6.35395 ] pdfxs
303.84 586.08 m
/N287 11.2301 Tf
(\000N) show
309.841 586.08 m
/N295 11.2301 Tf
(=2)
[6.6605 6.34606 ] pdfxs
330.301 498.12 m
(N=8)
[8.21798 6.36068 6.35395 ] pdfxs
330.301 484.321 m
/N287 11.2301 Tf
(\000N) show
336.301 484.321 m
/N295 11.2301 Tf
(=10)
[6.59984 6.17872 6.2854 ] pdfxs
n
207.78 429.24 m
216.12 425.22 l
211.74 425.22 l
211.74 420.84 l
207.78 429.24 l
eofill
1 J
1 j
0.192001 w
n
211.74 425.22 m
216.54 420.42 l
216.78 420.42 l
S
n
228.6 315.54 m
228.6 324.9 l
230.34 320.7 l
234.6 322.5 l
228.6 315.54 l
eofill
n
230.34 320.7 m
233.4 328.32 l
233.58 328.32 l
S
n
418.38 418.86 m
414.36 410.46 l
414.36 414.84 l
409.98 414.84 l
418.38 418.86 l
eofill
n
414.36 414.84 m
406.38 406.8 l
406.14 406.8 l
S
n
385.56 293.88 m
376.56 295.68 l
380.94 296.88 l
379.74 301.32 l
385.56 293.88 l
eofill
n
380.94 296.88 m
351.9 314.7 l
351.72 314.7 l
S
n
211.74 526.14 m
214.92 517.38 l
211.74 520.56 l
208.56 517.38 l
211.74 526.14 l
eofill
n
211.74 520.56 m
211.74 511.56 l
S
n
365.52 458.1 m
365.52 467.52 l
367.32 463.26 l
371.52 465.12 l
365.52 458.1 l
eofill
n
367.32 463.26 m
372.72 477.3 l
372.96 477.3 l
S
n
215.76 562.2 m
221.4 569.64 l
220.56 565.2 l
225 564.42 l
215.76 562.2 l
eofill
n
220.56 565.2 m
226.92 569.4 l
227.16 569.4 l
S
n
289.44 541.38 m
296.04 547.98 l
294.66 543.78 l
298.86 542.4 l
289.44 541.38 l
eofill
n
294.66 543.78 m
317.52 555 l
317.7 555 l
S
n
271.8 474.06 m
270.24 464.88 l
269.04 469.26 l
264.6 468.06 l
271.8 474.06 l
eofill
n
269.04 469.26 m
263.82 460.5 l
263.58 460.5 l
S
n
446.4 291.48 m
438 295.5 l
442.44 295.5 l
442.44 299.88 l
446.4 291.48 l
eofill
n
442.44 295.5 m
421.62 316.32 l
421.38 316.32 l
S
89.9999 193.14 m
/N282 12 Tf
(F) show
(i)
[3.33838 ] pdfxs
(gur) show
(e)
[5.3302 ] pdfxs
( 5, Sh) show
(e)
[5.3302 ] pdfxs
(w ) show
(et)
[5.3302 3.33838 ] pdfxs
( ) show
(al)
[5.3302 3.33838 ] pdfxs
(. ) show
0 j
0.720001 w
n
216 386.16 87.9 35.34 re
q
1 1 1 sc
eofill
Q
S
q
73.0302 0 0 27.36 223.62 390.12 cm
q
n
0 0 1 1 re
q
W
[/Indexed /N278 /ColorSpace findRes 146
<~s8W,np\3S&hr3PQcHa_>YctI?Zd@(Gj5]1fmdC)Rrq,jTgt^](`PnXKUn!sFOcbcQ
H[C3jIY*0'G'8%HDJjB2DfTl=JUrB%It*<3M3jQqU8"C0dF$Fle+)tulg*l?YHNnD
N,W`TEH,u?FED&(A:oMeS"#nQZEgU7Xfeh0R[T[kH?tC'Lh1./H$O\6W2RMI^ra^?
k2th(r;?$PmtQROI!g=!MMdgiREE[p`l?$Sh;.o&q=XFRp@e4YrVbj>jiGNaPEV2l
OH?'*T!>Q*eC<"%g=hgWQ#1ATI=6O2R$be/_qs8,qYL'#]=Xo9V2p[uWMukiTV0'7
^Zk"IT:_aAQBlZ9FcDB?c-=N)oCM/.kH(bdMi3M1_SW1IVSU*bWiE(mTqUQ.jG/MG
['[48q"VD1\Wi>CJ:N0ja2dT7mG$CM`5KThUSF!8P)bQ_f@SX-g"GZUlDLPX[C*Dr
Kn[1P]ZeUDo()@BSXmsIbLY7qf\"jRqtmk3[tKEf\@B',i8D&P[d`eU]tM,=io9=k
m&R1fGB\7UG^.ZbdW9JN]"5K'e^`!lcN~>]
cs 
<<
/ImageType 1
/Width 152
/Height 57
/ImageMatrix [152 0 0 -57 0 57] 
/BitsPerComponent 8
/Decode [0 255 ] 
/_Filters [currentfile /ASCII85Decode filter dup /LZWDecode filter dup 
] >>
pdf_image J,g]g3$]7K#D>EP:q1$o*=mro@So+\<\5,H7Uo<*jE<[.O@Wn[31'gO!s*q&J5@p:
$3p]+5r)$-eg:_-K)qY'E',6T#mA*g5c@d;'at4t+e[J,*$#Op_,G*F<WjNILdXN@
(m%?:$44R8J;Bjr.M[M'K$_TK,VKN6!s9-sb\/l7?=W#'+N/.W'8;2dU"IS64Wb3U
"7cj3K8KYjLP.E+'O2O^&W#G@5kL4)]O%sB+m?"l(+#.NUuHYd/dNkiMIOuC5TiKF
'h;^2*qg@4(m>)4E7n?sNK+7`AR`JLZ5G50b([_#qlE%8Q[n2fJ;h9P+\aFsnj'9]
+u'l=rG&S?]O<O_!QIs'ZuSnFhMf;`3LnFs]nm;81l;B+H8PjmW2;/+@5tPDL-bui
,_?,+YVrtP$8OOLj+)k)Kd./g3.k_&jrFGs+QtkHd*QMPLEUX)3l=LebV5([Leo(C
"-A=$Jg%q04V(u.C4cWid$QAC,NOl?L7iLo/;TsLqC)cGW;Jl:"9Xc6T](uM4G>Es
^kI>+E97jh655tHU#6bE4Gs<8"#qGio^J#rJ;>=6$1//q6)*?E#TXId=U7@@<$`N@
&0ohl6&R!BP75k2arWg+K30H\"sQ%:&.nJN2,g0anFe2j@5t+hMZc:U4TIlDoi+uu
&/7Nn?uRG+K0n5!%?(A`rmt408JEP2A6=m7LB*^?3nY9CX<8%(n<?BQ,Zs@og=HT1
%h3&_VAU_)'s&O/TU7Pk";b(T&-jFf@Rja*YS&Ai!baZCg;-o/('++5OtmX.d+s=U
!ptFO>rZCP4%s+W%uF9E!*V[C=N+$&"Ftq;O&=j1E&3JOr^fD2@3F\5ATVmC&I&7D
X-h7E.bXu:q8DbhJg8Q&T2/u_7Le:e,iAh0,1'.?]m<Z'8.QlRn1SNT38PY#JaQO>
^`Wn(*!\h?0sEndW8V+b^cea*4b3UI(6)h>T=@@dLmeV\TP5.R5U#WlXp--Ge%fiF
_"%a7@gNNInI6=u%M3'iZ5!o'mioFO+unWiNae\.blM*'2Oast!*1n2,+o2DP!MWJ
1(NAq3^=5s3bSX(iOK.ANFF:jiJ#'tVCD72W+[Ud5^;u5!9!@J,mo7%PO%]D#Q~>

Q
n
Q
Q
n
351 364.38 58.68 49.62 re
q
1 1 1 sc
eofill
Q
S
q
43.6966 0 0 41.58 358.62 368.4 cm
q
n
0 0 1 1 re
q
W
[/Indexed /N278 /ColorSpace findRes 143
<~s8W,pq>%P1\B`CF[C*DXCMU)UY&SH$PEV4"nF5Juj*Z6%JqAU6io9S$o8o&qFEDWK
bfmAuZ>=>n[^NWug=gdrG`%B9naZ/Dp\0N$M:L/,]=Y[nDf;YUWlW9&QBmj(mHr`c
h0j^"IXZb1l06mSfpS7rF`hiLb0#d+O*c5#`5KUjqYH22NP`QLqtp8iWMs`OD5*c!
p@e3^Xf_O!r26HjNfK.1\[h\;rM66b]"5JBS"%+)^&J$1n*f_.P*3Sp^RCU[DJj?m
X/i(nV07$*W2QZXkN@b]Mkd&BE,]d:a2duMpn=CTEcQ3BaiWi5l>q#f_83t=f%,P/
Kn4f+R$a7bGB``Qp$V89XK8MJc-=Y`d;!E2J:N0ASt>00kf(N[`l?$&Yd!K\m!<u(
N/W_fo^mlmL7Om+iSibQhr!&;f:S\-f\"ij^:qe6bN@sLo()@tcd0)0\!<5DLPLY;
K7f;KOkeaIQ^=&geC<UAje/9>VP^6OjQ*SNZ0U`APa%EhhVPH>YLCtL]Y(nIS=Hpl
ZeO6hLkpk:It)0HC!b5R~>]
cs 
<<
/ImageType 1
/Width 91
/Height 87
/ImageMatrix [91 0 0 -87 0 87] 
/BitsPerComponent 8
/Decode [0 255 ] 
/_Filters [currentfile /ASCII85Decode filter dup /LZWDecode filter dup 
] >>
pdf_image J,g]g3$]7K#D>EP:q1$o*=mro@So+P"9\ga7Uo<*&.f0QN_!\W^_e%&$'EAA:`rRc
(_)bSA0BfT5U/%S7Y3o[Uum(<$AF)jM>\2.)%?b%FD>>73#rN.C/A=55X6Klej'9[
(m%BoWIfeT5rF7i#nr1"2JQoY<%A_g.>#rdTO2`7$jIq*"lat3)2s3bg[t8S*YJoO
fNH9TDE&VrZ'0]Wlr6*hAEG%dkhphQbtLY2&:k3V0c^hHRVb0c?ptQf[Bd$!*0Gp-
aN5]J:hOhu-'JYIq%tq2/gkWa7.Pn!Pp%Rj`#F_aBW)Raoj`V.3ENU,!0rH%:AeWB
9H!%VYqU,2Z&A:nL;K\,CZ?'LP7)kbO`6+/^PI]Y0<_Se*%_5$Hjkd_,60Rt6"jrK
/:l0*)BjcD'J+t=6HDA#Tjh[FiPZ!m`[F6;.M!330iAAp7E@HW-k)5q$o3]XFDQO6
TWlZ]TRf'S$HN2IBJYVWoSPJ_C5e#M%3RWS-\)^eQH[DNBJ_S;Osnm4NA@0X.uf^b
\hf*!%&b,(l\qDe$H#-`.Lj89hPJ?SB[@-EN_G<5JAE(33"/+VM?o&*:_5L=,DbD@
Na[Rj&.X>kln/e._"'Vo+h2D+NPhPs+,WG<KFS8ti:7J>""=#17q;&"5E@$KPWK:Q
S72^2_uTEE!/(cc)\"!amMld*S=UW-@o.b,&9<"^%LU,3j\\RDn@/o5@]\*(O(/Ib
,)qm.CabBq\9VbeU!TSfMFs6k$;j'J^75A"aU1*8+BU0E.mjl>.g*]A1+coO6f<h)
,A:Bi&Auli'NW(!pK]77q$o^p_H<FkM;rh+6k7,5'El()@-BNUi*]A4K"tJf&.E#@
$5s)$8Ah"]@_a$-Ku1'?5R/DT'KHVu==Q:EK7GEQ%jE/6,)N*Dk-)<\aH@0u@#2<O
N<@N=(Cqd)NWP?[q&BKt"8KJS5f!a3L6:PAl7VNE`T&FdS*Dn^J,~>

Q
n
Q
Q
n
225 329.52 58.68 48.48 re
q
1 1 1 sc
eofill
Q
S
q
43.6152 0 0 40.44 232.62 333.54 cm
q
n
0 0 1 1 re
q
W
[/Indexed /N278 /ColorSpace findRes 179
<~s8W,sr;?Hhqu6Ton*f_tf\#W[md9E/f%/El`l?*@aJc&9Unjf_V59o\U7%F;XK8M?
_SY0dhW*YVaiVZ2Za6m?Yb@baT:_aNUSFEPT!,?$Xf\_4['[HW]=knk]"5JQWiF4a
b2qaHR$a8&OH??:VQR))[C*EP\@B2a]\M;tKnY5?NK(KZ\[JrTX/i:jS"$=RVm3M3
h;-n;J:NlKPd7U#Q^=%qM2?k;K7&&oCMR^+EcQ,<E-Z_SLPLYaWN"M$fCAD$g"G'%
bKKDEnEfN.p@e4)c-:T^HbR5.It)rlGB[k>CgUOVF`hhDD/F94EF`Tj<`W7^O,q5t
`9-4ESXl=\\$r$'TR(p1P*2!_gY:3+dp??eI=6P,kNAA*S;N2]bfn;ghqr-^Bj+\D
NfK.Xi8DGf_8!b"R[T]:oCHF#@Z-/&o()@;QBmf$Q$@Ouio8s&>[1]G@;]t#FEDX$
qYKLBl@OV>OcbdD_o%:dM"UH6PEV2ZIX]\ld=d1+AS#G(JV!Ukq!783F)uD*=]s(s
cV[P:rVc]EeC7/c9PS<W>?b<>?spdc^f=B7AnGXuG'6b];W6Tne^`42jQ'9><)?Cf
Df9Rgp\3n8k_tIZ`Poeu=BJj7?,t"+q>'hr@q/SA=(c/YL5(HTo^lg1B^+dG;c?WK
g=jitc;%,0d*U-69he5P9%)/9~>]
cs 
<<
/ImageType 1
/Width 91
/Height 85
/ImageMatrix [91 0 0 -85 0 85] 
/BitsPerComponent 8
/Decode [0 255 ] 
/_Filters [currentfile /ASCII85Decode filter dup /LZWDecode filter dup 
] >>
pdf_image J,g]g3$]7K#D>EP:q1$o*=mro@So+\<[%PF!5O+]1g3$aKE+9q?m$R)$3^LIJC&6t
+;"oN-;dU,:b!4gL'%I<?t^N!$AS_Wi:qgh+p#pP:sg,A8gY4.`<)."Uf8fS#R*P`
i,gk*#)_Yg3'^#:/IdS)ooX4-g`*2N!S9&^`+1Y8N@^F+&0P^G%Yqs^EI`][FW:l[
K;$reH9NF4"sX.7"GM5[ON<)Q0cZ;Z,a*h4nG+V5(FBee`:AHFU/DAQ`.Kh5:m=rf
Ld`R,Na`u!'8Za?YioUU<Xt6!iUTiRZ_\A%Me0b-Gd:TV!Q`VSnU/&Y(7#/7E8cS#
$j)fT@Vc=#;CE?86K5h[QsG:[N(JapBp?gtMdo+p'ESA0c@h0CpgUW75sS0Q"lXEP
gP0,2eg6"P@%[[]UM?/T5Qc8<%YLI:i<,aG&3qNClVKb]L-pc+/-M\tj9gT5-nI?<
?te*uK]AdF$4`i8FrLI4i(acoEBjLb$\L](XTRNI@P*SVE:,gtJO<$G!F]Z10a?Rj
iXQDbaqOlUU%i^JKqQdO1659t\ik_?]1NS8UYo63O/)44%5`qj1+3JQd.fd/+E1(,
JcTiiKS#q3*Y*lL!<O2@TWfmTafF>(5mF%$][I-2(k=,e!20TK3T0\<%1.TiIPV=A
+Ep9UWpj@=+MtXY/Va=VZ4%'C-u99DT\qq"07lHnorCD]>RQ:]M%0LkKKpRc^B7lP
&HDo`_D2V^8J"%F+E1p&La5k,2A'Ic"uubfGj7U,UQA.YJck;$Z%0^L=9qD?:pMVY
5`$<X#f9tA)2&"Z?9&=FC'm<9"E>JGO+;<p+G!Hh":0qHJKd1;U/5;j&nIYM&r$J/
[:h!t&EH"VT_#/sO9+,2JH>tQ(9I`b?s'ZViX%2c&-3na(T[4:g)c@YYokG"6peg$
'#EeA(^7a</u8PUk`dY&_HPM%KnC6sJWW@!2(oDHaTbG467AL$%fua`#)*&U+=i1W
ff1%0`$h8f+@PFj-k&A>eeeE[:fKgb,0nsX"N1RV!?bqC$TuHQGs5%JJf&Z*LS8*m
7g1-"68OioG]kbG5WT*#$,Cdn'a'..Ag**8i%9h=Ts3Ysi*ZRV(l"]<Hk-U;&faZ#
UkV)&KHcON;&%Wdn"HC?J=[C.5lb."AB=Ns+,3S$Z7:fL\d10S!6A%N_,(UH+A@Rq
5b8e/:j`hKBJTu=:(9O'>Q?#\2$ZuB!l8gs!Fh.P$/i63J[d04!+[\^642t0i%lk`
C`ka$+qT?nTaF+`&-Xb:'*;Zk+G'GH#N-TJ6%UI/i%QiAE0^`5Ospl-'F6OGh@,45
SdPU5:'n`L-NVS="9]PbL%(Jk6<HN`7!LJD<PFJYcl%FG&/g0%A6"0L=:L5IM1C.(
)hYq'#snb5`$,I9!bcfe5ZePM&A1Mb5^j,LS.>[oAd_dN!smme&-;N]+^[MJ!5[Sk
L2cJm>3KXT6kh3[E8h-gn2Cem4Gn^:n-OuV+9qn^Jr2hM++Vun>/HpO]b2M6!-!u2
!Rr.qYiZ;n=A'dqBMeh6:^TJBU`t=+-A,k$)Sn+[<KL$+!J!5cJA>t9,ZFo(TR%-e
5][KF3"5o(AN7aZ"VQB\2hd?3.gVLM$ZKLUK%RLt")'P&?ti,^^hRdYR"#=68jJ/_
"r)[j56F1_K*dZ4$Ne['"[Kj8O[/+O'YK_66"#<P!B:1u#VV=uU0eKD@Od^H8e>G7
.>#?+$ijroV4iSf:#M<GK'<sX5h$VOi&h>J"[O9(O>$[MZUViC*$TqF1C#V&%t\2f
'LA69#QQObJ@IrhU+eD+d+H28KOZ2M?ml2/;#gX418ePHRP:BU$](`N&tq]8K2@dB
K:$Hb_)PCIi%Pd70K'X(a;=sI3Yk8J!>#;"$jO6a.**5H#G>N@"d$7IaIkg5i;>\B
JP[?'ciF?FKH5bC63=s`^([4,*.n5Q,D!B<#bad%)k^(K6(%oW5dVHPJ5cr-`+pP_
>UY6P!q*n'Ptn!F8ZT1V(mCp#&V.qffhbuZ!,TC\JF!GjjM2L9nHBQa3&lNj5SCtj
I3O7[4bXI:'EV)k#Hk92#]Q@L6PqN\i+*+T+UeI+%IS)L"<E%[+p#ODJ-0Yu#D(kE
#/TVr"[I/p$F2&eKhsuHU"h=)cq6S,pk]5@fEHm-AAc3aYALR):P3qg6c#-a"!G66
g#NQ-6\%i6TSE3)b$%/akYVT#lm=g0V*Y.^TG<"U!<HR`"G>oh!q(:DJSPXUaB40-
)%7$7O>T3-(eYA)0GOZIX'u?r!tTrN-A[4&&-P6O+JNsVMP.s+JESBc_1<AoJNb'O
JIhi*6nnd"WX2al@glf]qSj(;B?6/T&qV5mf?grJWf[DnJNQ,&:`LY[-+<ulF:s4c
6:<XL;[m-)39,#`)FQi2M4lI>?rA6^_MFHa(H<06\gTjp@#+i6GRYuW:(+mO/.A=J
4U6N4#XNEF!T9W'JRK)lNd)QJ[q(9p0]"%lQo,@^llO>:$mC90K*-XC.3io,(k^o(
,!_qQ"f-)Q6#@X.T]dL"@'U]dE$i+`4:;Lh^^WU)W!i`VYn1=8'7h90JKW12!oRN#
J123HiTqF%n7A$/0F5.<DPIID1.-[b4:_IC.YD,4*VMJt$R+FfLP@.I^gKja,YU+P
&CD.VpfI[[*$p:]1nL>Rdioob1C&H=%RZ=/&1DdU#f+@g_shnO"pbnE:c#/nLaWTL
J2Mq?8h3Fd!<o23"p49W=<EA0#_=ra#_<O."=QIV":tS=E@N+sdPqP@<#18V&k%Er
/.c3B'aZ!V%Ku##%[uNL!rLtF6\%$!_9=K`d0_'J_$C01+gHZ=Z5,_s2A>8@ML\O!
)]Z(3#2-eDK)g9'(B>ip)sE%X_+kM.R"5ME'J]<5"9H?#/_gt@%XE$MW(<Qi'7aI)
=^^;\Ce]fn+Nt5oZ6B>QI13jeWhg7m3Zg^S,\Nd#&-5T_%RJa!,Jad\Ui8'j^g[?H
&.UtN'`^c*^tuoE*WU_6'8b-J!;7&)rZH`O%tNL;U9k$<;?S+Ob=DntJ>*Mr1]`,#
#:e6&@9=/8EX'=0'uD!l+P7:an.&ij$t02FJdMea4q.L$"0^nl+CG9>n.7!A,N)>o
?oeoc/.[d_+CG<ZTgB(dr"&jYpOX4p5u\0kTG!od$%RIX63[F_iXGl'.c_KK@(:J)
*!8tl,JX?kMOFX?ecB.oblS(a@0dNt$4m1o&&=&G^^0S*U^@*L%q'bo@KmD%:(UeQ
"lN9>^gI6f$4HoB%6ub<69Yq<GRC*q"i+@J#[ALg<Xtf_%UaA`+U2$M('%b'&`@te
!<rk'/g*C^![,i"9--SG3!^XC$)%\1@+5:p!>RpP!e>Z[Ah4/p0HbpI&ce^4+E0q)
C`sp!Zt[r"?tp*X-3?Iu!Pk_O:DO)k*YPEaa(m4-n<tP0(^@d?V]_;VOes7/oF@PL
#N0V*T]Gpc$jcAs#9]6EJ8,I"=pQ7T"or6<kPd!IZj/j8%`&F+jDk>&Jg:@*&u_B0
+C%h(',dJ3)?Ab$dI\QS(_6Uc'B#l#5SsX^?3C8X&k/la?ks1P!X6Aq#B+PfBT<Fs
js/fI%cH=Li'7YmD&I>\&cg,d@(6aJD!rPP&V2tC^^:NCC^*.BgE>)o^chq;3\LIi
"JBK=JMI4U=CPudp)k3r![ItXH<Gb\"(5sTU(.1>+;CTd%tNX>@#Pc7_?+-k6GRII
5\'rYa9c9$--OL9i%+t\(^C[aMr@nO+9ht!C._sd$UG-?i][VK:uKV1"X!dF?j74,
6Sr0N#XH*2!*EtZ$3VKU"ea]`!;H_jEWhGR&k"@sTMP`"j:..g$Xe&ci&VUM"p3`b
PmJuE^mOV#-jX3[$6X/AVm$XR6jl8u"&l6]TWeLUU(DkK$io-o!4WDe8.J>m"JC8M
!5pH7J-[A0$t+5i+IEW];uj'Nbq04ZkD0BT-6f)c!MJ'V+F4,[Q3Q8f#-A@BT`>5&
'.G'2&HNO0i8jn<j9D9W"JC2IT`tm5"qSKj!oP+,T_8p?3"A2=!<A/(!/U@6hQam(
r5(W(@7h"a?3.;P"q,,r@/Vsuh@ngf%u_><AloD5=9md(O'l]0!B:=88dZ\coO*mf
V@3qi66JN=$k;Pj%a<B'49Wl-$-nPZTX5#uPRCn$26TOY@%%WLj:MC;%q'2U!9+>O
:'r,X'$(Uoi-H)&l3C]f!n,d5Ma/EcO;$SLQQh:rJ:Lj55R*!_Uui3l5cP7/#RS<q
$@pH#_+YOd65;d!%DZum761kY&-X1E&#!5C+HR*fd\rg("ou.8jOOONFBQ^:$UG!T
6=ff*T_JpR$%W?rTR$XS@L\TZ=J4:LTcaZ85&*><ocaYT"NCT(YQc6,l[fTH+=[pZ
BRg(L'`\jt@-"S#('@qs$U>+#c`eP-IM0Hc"dD&!+p\H_!X,/3"lQZf^iJT^%KoE_
i9\#[D7NmOW3rSP$WRla5m.j/V@XkP"tO+7!)<de$j4:)$\1,Y5`u[(\hp'0%H&BY
Jn+l^W"Lig#66L]da0+E"p6#T%cD(35d1BNHj+&@W1Z?f<Xtq$'NQkr%2%#8?u-S9
Hj;q;"ooMXJe/Y>GSJ9L$t(%W!EK4$Qj3V/.tD4@%Yc+!NWS0'NT,a%+@m18MD&A?
%\UQZ5V`A5+_;i%"\(Tc+BejKjp%J"1k:kri,A^Yll\SL&&<55_U\nKE!ubT4Q%h(
_)MsK?jd_A,Tujt+F4T,`X!\\%>(kfi)4!M)bPX&"KrLC^eP8g"*7qm#f*;M!9P!r
iWF]u/clXkkAU[ah@)Y'"%ZBY+M_66$k]kJ0I<e$Ta$$XS-#Bp$.`D`J4X^S(_cud
'gS,t?t'8i*3s5LO5MDs?q@%jZ2qb*"1EY3JIQ=0mO@(&>/CmU@5JU.ljb-j"Mc&`
+Bekt>R_g3!<FeQi,B4K;/>)H#uM7*_?L@`A.6bB!MC3Q_@dEq5(<Sj/qF3-i+HB?
>R!H(%=n3]!+d,6FK"-M#uD@e!X&KGQ!Jr;"$gB)5oL0)ap*DZ+G!F:J3j]R4qV1m
<hL33!iCC]5WiFZ$R=R=?p"JjWWusFKE;Jl5o'f8Fp+HZ!J'9go\K`OA-4Kd=hu?k
+UA]gHjjD%%NqtYfY@Neg'2+N.tD/9OMQb(<"*DI#=,d#!k@q+iWLAZ"<_(Rc4;M"
FqgV3&g9XUJ>A(&+=uGS;1Q"X+EdjQpPhGL'Hl0>%a5!iDj"LG!hb,HUYQU!>Qc2W
!oUp/Tj.kr8-_Eb"b>_F^t]7T,0uqo#9[$+64sEPAW'sk"JlkEPJRk2*!(RGQ_6/D
!+b%t#SDU8%%u#^!#u(!"HV5D+M\6b!9Oa1;A'!Q%\XP6@!S4d*"ZL.Oa3B>TEY[P
KE.[!S7&E0!<G;*p^TPWr#*8?q;Io*j<,Q~>

Q
n
Q
Q
n
297 306.3 60.9 53.7 re
q
1 1 1 sc
eofill
Q
S
q
46.0474 0 0 45.66 304.62 310.32 cm
q
n
0 0 1 1 re
q
W
[/Indexed /N278 /ColorSpace findRes 192
<~s8W,gnF5`.lE[_$R$a81S"$O^Xh;<ZmdBN>qYK+,hl3TSNK&q*[C,2\kN(^bi8EP9
b0"$s?A4)eUnjf[TqSB^ViHdtUSFUEj5[#6VL<l@AnGY"G^,C7P'2"l@U`eS?snG4
IY`f9PEV2gMi4U8Wm&]2:f'uFM2@amS>E'YR[T\0Pa%`0SXGn6Q'IWaeC9G9N,!*B
Bk_:&F)uqbJoG[JGB\7nOca[)EiZ7AYct@)TV,:b<JlZkLPLZ(`PqH?o6GV,?XI/D
>$>i_Dej-(?!U`XFED>8CiOH7U8"BeZ*F9+rFBGLT:_aa[^L^:J5K0@;GpCo=''6U
D.dKoY-+q6Za8u`lgaN8c-=L-9hg7mK4nq3I!g<ZDJl&;SsPe1L5(Fc=]nj/=ADUd
:JXcJOH@8n_!ga\^:q=l\[hV7qg*R7H[C+*QBnVRXCGaMW2QZeo^qnPpO@[B>[1Nb
JUpd"<(otZ;c?W4_o#)=8kVfM_SX04F`h8,AV>_iO,oA$rr0L?](Pah6UO6'k2t@M
fsJ,n5<hB9YHRm%r'a%Cd*U.pgt^Q7fL/+qdaHS7o('<#\D#Zjl07G5<`VLP6-76j
hVR*\8P-b7_:I2ga2c6em-N`kin`GH6:+#R^VA+@cfO9Mq"XWn\$tblmEX#&84Z;%
e^aBep-:l.>?b<?@:@R2dJ<V67RfkZ]=[%\iQ0*]7n6(h`l>^*]u7k-gY:K7f@S3h
bNS0Re'lb~>]
cs 
<<
/ImageType 1
/Width 96
/Height 96
/ImageMatrix [96 0 0 -96 0 96] 
/BitsPerComponent 8
/Decode [0 255 ] 
/_Filters [currentfile /ASCII85Decode filter dup /LZWDecode filter dup 
] >>
pdf_image J,g]g3$]7K#D>EP:q1$o*=mro@So+\<\5,H7Uo<*jE<[.O@Wn[3@'nb-^756+;n.e
%KZZ^!2*^Z+qb1c!l9E6E',6EQUZQM+IGtT'FP)^!LPQS2B33^KAln;LdiX&LP3J$
<<a]r'FI8o6!1?p/f0C7!t\-3=qV;M`^;JRe4;J:N5l$^kia?T*WrIiiTU&c0-CXW
!^V@8=:>TL83d4o&;iq%OU2/P@45e^%h4@>P$k@l9aDE:F)c1^6ld-T#!sJ(O@W1h
L'$BZM+FLC+pnZdJp@'j4t@8'iuk%'Z<>-IMbmm>XLMOh#tsC_#tU:A+c]5`O_DC4
/MWY%VIMTYcq*mKpa0J>]O5Fh(($\.af*bj!$blZ('e>bVO!4Y!1l-.JiKhC%KcEi
)i+Se(rd%/E9&DVj-\1GN<1M)pB^peHk?OVn/)KBJ>b._"%()o%15HFQjNp\)!mQD
!MDt0NoPZH,)jFTjphK'aH@tWmD(gcM?.s<,EG4Ed1MF*5klXaJhSMh%3V;l-in=<
OpclYB\GY,TISZ["Mk@Y&r)#=U_/<STVt'^U0'T0MS_p4XFuW_.NT$Bd*+_m%rf`2
MW8qB&Ip"8<[ImA0Qo1+1J"5eLSOuJ$AtN#!Y'rnfXqTP,9ZCXKHp!/+qR&5a;b;X
)$gt2i?6'!!5S)g*tM6tr]LI-#fm=&JA?IG!l.nfZ\nh10JUB-+USa?EVM^H"@;fT
4GIB$%Q4[T5kkWs6BIKPKAlm(&lPKd)?GMc8=hJf5`k[hNa]Fc4G9D]`YS]LW)sjg
!tZq(OXV]34,b@#ndgZZfR>f?,"Qa+&OQQl4c7+dXr7j'QrlBUUbMX6LEZ_16&%ag
]LDrg\8XBc!ItG4M1OV($:&!,4@Q'=_"7g@iiqtc%"XNF0SG+"$q,VtW?*i$K!W*&
g&N-W$B)hFhEh9o#p;>B!r0VYKOFRG('&lhGUs/R8CA=f.2]E2LuG\M.7HPD^a'O`
5S+S7KUDBt66dVm-k8RWj9busodC>3@'K,W#`e,-)$M1.(8DA(f`k%o7&Yts"JMb^
3!3S[4;Nag)cVLm+u'!GM#cag(^r['/-^ZXGXs.d,e=++"Ce%J-&U`m3^NsXE&8Vi
@urAOV24p%'Z"5Y^,qB!86S-3KPDP3%cZ]SE:.1KRMLOk^g%6PW$*i;6TCJ>^t^@c
E*`mfE+29;cq?6*3Y91)57ZYb%>I-r(r=!57q=^f$(rO_`#(K<5jSp^ZG[T2k[K0T
$r);grZ2*g[KBtM$A?2G(.2bU#@Z,B#>g:`PGh@d5faOgY\";7L^sa,'K?3t)?g.\
'F)B=%09iD-O;,S"Q:%iJcPup_FP=K?rR4.d6&?KHq5JI5VIle_@D+KG6U=F*/&Ks
7"LG`#)]>lK?u.M!?bkPTeHk2ndZs6=IftRKfXkU>8[ES=T[T5NIfGA#m&D(>QCU?
K1PDY71]V'?oSE'_+#-V^i+%^&@;N>A-IM!,QVfLK)lQT)?e,?%cF-BX78dt!UM<\
_O(l;?r@WuckAa_">>RM!%G_#.0ngj!X^Ur1Pe;p$@qn:L&a[JJRGG[^b?3$"]up=
5cP0bF;,!'Orct]0*6^/#)8Li7DtiI"C^@$]0Pcj6"h&C+`Kc(YX0.Y\5Ee:N'W+N
C^5V9,Sa]P:lms-#:A@e&:qb@Kb+Y$JUf<\5ep!ROO>W[n7O5U3!+o_kQp=e'b.t.
,6GY=f7NKI"2TLM$IAc'K@!0r5o;;-0LQ_O&5*?qj?T2"`ZIHnkRjQ%%L6s'#lpnc
%Y6l%J5@^&J2moLMu5%*.%1N/.!,N@9Yh<KgaiK$RLT@LgB'X',>D!X%)G*b$P813
_DjRd@+YYan0Sj#YUflA<&k=/KG"F/33\9>*e7kb$A!F2J]&BlL*6C9!h`"_@Di>+
i$oKJ\8DfX4;*Eg2\=NL1jgJ!.Y7[V&O;FA(*Sn[KM[gA.St$m+B:9(+=nOpn2^sY
O^3XUYTWuuBadI)KE[Jp'Z8if<FLgq$Bt'r7=]WcJ@$^*=GRgY-ib#kHo$IAWYn1^
YcOPf+orgdcVuk.%=fE"MGVeS,5=D.+;P+]J7&CCcp+,_*&WWSp6OfB'F/$1$P@@u
%Db:j%j5,sJ3XMD7B$A(!I,:bUcoiOSaZm"81t2Z/-A4p[1QeC*/FRt'`oqd!qn#j
!C5'?ME#>o6I\MWJuT+'a9;]Sof&"!$3c*M*"EN^(Buhj,3>I."G)4j#r'X@61@eX
^sk[PTF:h=n-9$1\/>=@,S@n\8IU,o'c)<.!<N;a"i)Nc&:e4?_*DR@b-2q<5[Lli
TQLADD'fH@<#EPeE>HJ0#RbTh+@FL>%KPQ<"2G<kKWmN<TX5X?0Tl\B5Z\EqfGOhr
TF1im*sVd^)ZW-D#lpZ(SJS4JMi;ZcQ!fL^@$CnYJT<@D!$),K?UoZ4=+s197LTeY
-@fN>'QnJO"+btgL&fO5!q9ohJNtaj5eX^[n:;&L^_d7U]Es2*!YXIV4bS>E9**Z^
%H<n:!:]V-5l"Fj+YXW7!*U]T3/M$.^^W5BF;@4TE<Lh$,_n(Thuc5D$GkL0K)g3*
!E_Sn0nk/a5jf)3-uoo/=?-D$66*k0@7<J@$35#p!6DsS#\%m0J[q!K6#\@W_E`a*
TWE"I^]qe.n.,dYX:iB8<s[dk1PINI+MbPM$t7Kt"rsEP_gk)Z5aKlLd<7-pL`ZhP
ll#t<2?j<R3t+Mf:*L6gD#b\.&:g,Ldi6dB_H8Al!G#/c@4W'LY]g.7bV+]I,V3b^
;\g3`_h,[k'*5VI$!$mZ!Rf%66nj/'_#P^6ct3`</7T!`3/iZ5"<RZlZikol(P#n$
/]\b0"/'`OJO]&GK4ku.@Ls]@&Bk_R-tO/4A28aeWX!\I@gkW$7Yibj#QgrL('4ro
"OPX@!b`AR+D`ib`0i8E0J<OF\;Z(Q=9q1WX0Vf9*J%7m-NZ7@#GCE1Ls^;LJ1(SO
8d""-%tQJqjJiQ[ckM%M$>&u@MoZ(;GQU572rLP8i6lXrU).5hEr[NsJBS86DusE0
$t-@MJ6EZ(1&rGs$D;-ANq*1#GRbk''aX(.J5#H_g'stP"e_Y,+Yj;<HjcW'$BQ)8
?tofEr!m-&!ap$Pi(OT1GQr_<?f:>\@!W;K$k5RsCu?iOTeb:d4N"rQ!o[Z75qEe%
Sd9,!dGQR1iHQ)fC^!)f!+=FpTI:9m?sfU0&HQhcJ;aeB^_&jb'L2X!+Kc&ZC'm3u
%Nop%+B/JOdK<oem!u;I+SlO4('J#a#G=a$J>rl_-MCg_!FV]2Ji"')cHo.+!.ZO!
TEYT#BFNg^S,bDGTF(lg3XDBj!hjiTLAE%.KF?_b]25)PTIpY'1_q3m#9Y].!A"L"
/-;JZ#RG;LDV/?XU]@(Y%8D!ii=>LQDM"NE(#Ti9@#,6lN+6FJ!FT:G+D:sFH@-nJ
"QZWdNP_8P-k(Vq$NNKu!'Ig1eeK;7$".9I?lB3B=:+'V%O/moTJVsd/el,C!^MJM
i-ki[H:e/a&)gus^r-Dl-4iEj+b9t1JL1_s,RWIKgu,gO+=[Qq5QQ^0!+>X'i"cJ=
3XPk1&AVZgL"_u'>QB:2C8*No^j[#KB&19/$q"n9W*Ta>BFZ0)$ij<Oajpf-@Lth5
#mUG<i@G`Eh?Dgo$P,Q9?jaGPQiOsE"g*jp&hmm)?34Rq#EfjU#j)P,GRr^Xh8A^c
JDLVW)@<)u"TXVkMo&d4RK7qp/4St>aaOYKQ3;^hoDmAHJ:+T:EWCXN'#7fi_DVuK
:_j'5V]]*WJ67N`h^W">%H&-JTMuS#SA'OC/g*Cf5\p^VIKdM&$*nFO^q^0dTE&DB
"Q6El$oA!8=pJJ."[O[aJ1MKG<'m6_!2.doP5GKI!B&jP'HiJFTW/F9WYPSl:`qq(
5XG`f.L0B5'>PLi^ck6'j9m+,'WtgK5R7jMYSTRW"i/b8J5-KFnKRNZj>4$q1UT*W
(_QiH$=P[sCN9pc_InBi%gD"o_%mR^e-caT59QBpiH?!0T+O[TN1_'n$pl1I:^1<(
#-I:sTN22'rWnLn#;d)UJe]ZkW"pb2#JdL>J/F])EWoiq%A?$'5Sab.3X($L#D$t.
!A"d\OU:Z9;%oNG@+l%icibKM&V.e#JG,6a=[>@g&\s\GXo8TV5ZWCr#sdnh!2UFG
j;+F]$Qu+5i1WL=!#FKp6i]1Ne8,2:0Fm:$,9YbK!>.siW!Ql&#P5&eFDEs'^^#cU
J&*B8+?gNj:^k/%q-]9h!<`^H.L5T.&-1>f?nManEWKPP(83u,^ha[WWr<;]Va*=.
i\D-t&4Bo&%mqsS+Q#F_<gT%Y#:$5k?j$Qs_?s^j$`'j75`#9p64#oA$fGn.TKb),
TF[\6!3QA'U;d4B!"kn!%1*dV@-.a1hufW9,=*:T'+.-C5jBJO8lGOP!+5h803I-4
$,HlSTem;!)cs3c%)DKA@)<$H^&gRf"lSW:_02EQY($Fl#GBcSUP&oGD?bWo1gi3G
;8+6i3YGqW%tO9ZJ>`VOc4=>s%r0<n+N@SMUjO;n#pCWfolrl9BF+au#scAD^umGf
GRsmt%RC:)JtXu.`WX*70VC`@!9OK=KEbg.,=)GCj+IRDgdGfW'B#Ypi,0&JA1ZYH
&0q/cTNDnoE^X<_"e^`&J8Pc<P;r+6)=e"NJBeX?&.E,"%%tpI@:0K$Q;Tt9_.##(
i;O(6pdB:'%06A-TE#&PE'%ZFO;?%?!?CKMeiggK$HmGuTP=bk"p'7Q&8(24JCkON
RK]#h%fhn'^^(Dm=q>#>'-Ls(!Fc>m2?n]-,@H@OJG9B"apd5Mk5YJb@6+]_R&q.H
5N$]#KA8FsYRM"=$K*o'i3!YW0E`M="$mh<_/^+&<Y/XC&3s&'1,',%X`fIB&5Fbe
+I<fE1_9Zd'=XnJTkFtfWZYB*GtAtU[`T)Qee91;]*klT,d[neBG'1p&0U0M!E9gW
i,W5d%A;2_?rR?h6k2Lh#n>/i+=%>fb?D]Q$m:(oTme5;0F@f>F.b57!(SJ4\,h;0
&0RJJ2kU\3VSsBp6,8]m!>Jue":Kb&%$/"U!-So]F92JB%)C3u+NOh4')CJ#-%OhY
DWW1:[MPUT&kf/GGPcZ1!!`O($K4'sjKiVeV?DGqrIP:Z!<`Ji.dXud"`ZpHJ,g>b
c3th3$m>8_@0-bnAp0jLNoEcf3<n/E?3Qui"]]bd90bYUp^g#M+@00:YOt[m<"*/h
%63h^@5JCc^^RWp#%25"TYM#pN6e4oOUcd)+Bf"8d-Y5?LL]*HJC#")%LXC)C]G4Y
2M_LS^'CP3&E%4/F@HE>5%MuK&1M3;(].(&=p71N#>\c]/(tEicFtH$+Q2/a@,a2B
ed\:>"B+jpiWKKOrY$O1]LDN'i8+c+$mdlB:8V]+TQC`>=oa(`%X6\8PmSY,ed-eb
@)3`jT\*?hV.(PSSH3UE)/ohr65BR(#2k4G!-)A6%M-?n$,?lQTO*@"cj,+1'juUq
!7L>Q";/FW(BFXATEkdtoEAV\!249;+F9RZ&tNgt#=(6Z!Fc;lE"+!kRO)&>5["I:
^^OUU"MmtF5T0aQkTI\+$=hp&!+_$r1^0P,`Sbn>NHPaWeG]I2G<k!hM$t[Q;AOgk
#f`M=@.Jbe21i'."ZIPH_0A,I>\p'>$35)O!1Emq`Me@l3ZuWX5]:ih]F\KQ/##iM
^tof_E3,_L&5,D"F".Vb4;"6+LdD@W^ciNpXptH7#u9p4N`ZPeC`m.+$/j/4WiQXZ
R3\M)(^mMB^s=O]WW@Xg9d)V6+N+Ztp`Q8#2F,Cr+H;&IC'L>M!5TQWJ3F+1#Sk/D
=.heo+Hcgn=qgY(=16fia9M!j4r7V\#Q(kN^jr6]-'0mJ"KRgg?n;g2Pa%mL'*1c6
!Ep7J?+Ycm$G1<_i2d,j>73-n$Qpc"Jdr.;cjAgD#t?HOi*Hd6$3pR-P-8mVgUOst
apc(E"9<0?P:@9?9,,Vt+JE<Vi6VNjNX5\P#iLXKi._l[('joC(^!e^)n8O+OFSWl
MKsX^)9<,"dNDrQ#rB@&Kt%V#h?Vt"$t'8JDZUC'DBSiP!8LJV+Q*L6^KZ6J&9eO*
6pq9q_@RjP@\@NB5YR\UO$u1.+M7Go5c;TZP`-_c'VT\/\TAseU(r3V@obQ#+F[Pr
$jD09$f'GYiID[0`J73[$".H"5h+%D^_\1%'HpilTZkPDk1%1]$m8LX5V@lk%NrRR
!oY48!6dN?$4>]T!oY[=5fb(a+;:EHW%P!I5em[KJ-nP"%R!9(i$!$S-,lPZ!anJ'
l#[>!=:>6>$t4)c6!t!A3!Ooi[BUJL@#P@SIN[S6%m^-ZTTfYR]uGmddUEP"\_%EX
kEOo+&0V-B?tofeTtamA+McVCUd,A!U^XEU#p>9;iWo\G-46,0#bXLl5aC"'@?B=1
+J@Ks5nFB2c4=38Fs+L'Z%=*+\.K-M#qq5Ee:P0&4/H7%+Fmg#@(HI`Oq%I/#='ma
^ePL"M?d?!h4SKo5ct7VS)h,'&HOrLTPb%NC(Wc@(SOqH#iZ*IEXa.1$lDq+JeeCN
l3a2+!MXBQi=lX7\eY;.%Ub%c*hX[L";X6P'tIJf"<nCBL's7slln7mhTtTGjmIT^
m\178+9~>

Q
n
Q
Q
n
189 482.52 60.9 30.48 re
q
1 1 1 sc
eofill
Q
S
q
46.0906 0 0 22.5 196.62 486.48 cm
q
n
0 0 1 1 re
q
W
[/Indexed /N278 /ColorSpace findRes 132
<~s8W,trVcWjqu$BimdBN+kND*ol-[o+`Pog:a2c3>`iQ8CX/i;#WN"@qe+<2&p@e4M
naYDigodf_TV.sPU8"TbW2$,_VP^5mXf\n7ZFRNVYHP.=\$tDXj3Q&t]"5JQWiDnl
V4XBPVl-GdTqT-3]Xtef[^NWO['Z0dQ^XA3q"XXRnF5Z*kj%Hum-O)lg"DsgT!bu6
Q'IW&R@0+sO,AgPMi3LLLkq"KN-9AfCi!p$BP<6ZM>mMRf@SWZZ*D-]_6^JS\@B&%
KS4GhFE_qQOcbccNK&sYNfoQgaN2HGbKH]WUp.)-S=H+2OH=^3Gh_!-jQ,C]io62e
P_Y$LH[C+Q]tJE*EH?2BEcQ2JI!g6dH@LEoL5(GMR$bb-_TL$Dlg*m5qYItA^R^pd
iSibRi8E8?f\bTDo^qeOq>&=]cC:;mQBmimh;-f=g67_ac-=MK^qfO3o#&A_I=6Ol
daEYrJB>pTIXZ`uK7hOtd+-[sp%A"%bfmf8^0k>VhVR)~>]
cs 
<<
/ImageType 1
/Width 96
/Height 47
/ImageMatrix [96 0 0 -47 0 47] 
/BitsPerComponent 8
/Decode [0 255 ] 
/_Filters [currentfile /ASCII85Decode filter dup /LZWDecode filter dup 
] >>
pdf_image J,g]g3$]7K#D>EP:q1$o*=mro@So+\<\5,H7Uo<*jE<Zj!.]T-)#T[B"9Q_2^i2Oa
&djs,6"%KA0H:Ue:10aqLe&3n$3`c4@(9T")$to2@?@^,2B3*X_k8I.PQW$<L]enF
(m$L!%1.^HYh4-C-kt?g+Y^F)8h1ZW@A;.g(^r&"!?gD'N;OSL&H`5Gd/[u>1`D)<
68>_"E&Sbs#=FX+n9R8$&+38U#loQ&&I=!iJ@I.`)Be<f+],\)1d__7"Tb;&P\<!"
Ob[GP37*aY,n`coU0&\.$7:FIE05u:C).tT/DD[EUkV/_e?"9VR#mt<,*[jM+TY98
<@WcSI(5;8;CW7a#_EV\N(,**K`](EaE!=@"JW-'/-d>k/.[IcMqEpkU<&E(Lk.73
's`G<[OmDh0Vg6-!pI9M$f_5/0T8@9a>1SF^fiN&iK,l0Kcn0I.fi"&di48K:bnlH
?slegNKHgi2N>POTG3(*R$8QmYZ-;#JDh@%%Klet(cVaCkfG3_@[JJ\!s(Nc3",g!
j";rL#il2Li+P"^M;b+b$A6eoj9#EmQpMI>!Z3O8L81KB4!u5F:b[aM+>a^d_6C5i
:l-kg%0^/O:^r4(.!-ktUU;;0!$LKf7"\rn.NJ`r]Rs"U_?fW=<4$%R+GKJtE]f/P
E/4qQ!DKt,,f+0d'n`2FjsMf_!_`k0@APRkKIJ43P(4a$E[QM@-u'T&Be]6E"<fH9
*=[2W8h#gqE'Oj="5V1^Kqbg798,Xm+a9]3V.L8?JqT\B,='Vk"pEkgBGY%^fE<(I
+WuRM$"KhFN<#_uX<</r=HF)'BY_bPL4PGB&-8LR0K.sq?qM[FJM9nVL;PnKPbJ-`
r&K`&+=8ChU]+qa&-3'2"bbkX-l[i(p3qi-@t<DMc2jTr5j;sD!Y^I;Lc,hM+W(Zg
U-oQ9&d/7A<%*U3QGA:_`#B=0!e_oOM2J(TNZ3e"T&tffUICB[n/MrB_4[_4~>

Q
n
Q
Q
n
369 470.82 60.9 51.18 re
q
1 1 1 sc
eofill
Q
S
q
45.6705 0 0 43.2 376.62 474.78 cm
q
n
0 0 1 1 re
q
W
[/Indexed /N278 /ColorSpace findRes 188
<~s8W,UhVRDWk4\NBdaHR)O,p3:Vi$@hP*2!7Za60lSB&[jkND$chr!AMi+-A/FEDVb
NfK[$SYi9]Yct@A\@AWAXJ2G`Q^=&DZ*C+#Up@;3kih7-qtp$XoS&!Q='&I[M2@Oa
QCjeAY-+q=]"5_o_7@+e[^NW5R[W6qir8rV7n6(!It*6/LQdpcX/i;$WiEeI^;.P"
]tM+s_o&sm\"KCeR@0JU]Y+1?r+9PQIXZa-OH?THXf8;!['[3W_SX=4`hfN.YHP.c
h;./QjPf(V:/4Q%DJk2`L67U\S"#nGW2RJG^Rh$gaiVYEEH/Co[Dg,(R$a9-m-InZ
>'t^FUSFTXTqT*1]@GH^;,L2#@q1afP]LneD/F-/E,^5RI=Zs#Q'IWQ`5Gb[=GVch
JqAS`@U`\O?YX=jF`hhWJ:RLmqGU<kH[C*184Z?F8l\kk@:<S[CMRj,DiKa99MA-<
Mi34?KA,&5<)cgd7RgZh?$CL:jlPV&rVb@"f5bnP77BXG<`X$QCuaR9f\"hS;Gr1$
K_>$29he>R8P*Q-B@,#P5X7U&mdBiDpLRoIH$O[]H?r@_:Ngo)nF5p55s`uKdp??e
G^+K%n*aLd>kn*h6psH1mHn%Z=cA;ucHa`$lg$l(6LjU9o()?=6UT8KdFQn"?smBs
gY:E7g"bB<cd0pA>?g@Vl"OjGlK[Y2:f(h=BZeK?4?PatoCL/Kb<A*R5<h@~>]
cs 
<<
/ImageType 1
/Width 95
/Height 90
/ImageMatrix [95 0 0 -90 0 90] 
/BitsPerComponent 8
/Decode [0 255 ] 
/_Filters [currentfile /ASCII85Decode filter dup /LZWDecode filter dup 
] >>
pdf_image J,g]g3$]7K#D>EP:q1$o*=mro@So+\<\5,H7Uo<*jE<[.O@Wn[3@'nb-^757;Rp>H
>q_R=AlC^cenm@*!'jJ>#RgtB!s-4<OAIJF%A$%?_!lkB,SLLd6D7es?nrW0LB4+&
9Lq8f&-tZj0JJS\-52)%!+8W^-n,2tKiQcEX>DIDMhU,@JAa2u"bOa(6)^#a'c;qN
!O3L(O*$$bLLL;BoIqL3&&VoYR0O!a'+dWA;6^+U.1;7A,Z6<P+Ts$Q#pc6J0Ua6r
L;\a1W,,7B'+Jn+ic,232C=X(6'+r/(_4+YM$4G>/4<2V#t&7M0Pi:<'F@1&OpIFg
;pYtF_dTbpL/\6cJla.ti&hQ$(&"JST_p>[$Ru.2(ks0+-k3k?84kH:_4-)]L.pe\
[/sfFD@6Z.EbI%_K'5BO!s$\u.0@;h;Cd[A(a]=h!Iu^0Jq1(%)[)ioB_&gqRt;ME
@%ae7#LLn.'o7H,^(5htTJRLc66KMe$mQ>'(CYl1Z3(/9S6?7*J4OJj")f,H15J7.
A.o>HE$c)B+je"\!WtE$)i)gS81';u8CTMU,@K4O"lc2R)h>e?qB&0-o@Y&+iL!4m
]YQS!)3)aohCa]D5[FU"NsLOM$KHZ22@^snjuO!IYeCm4$P62e!5]_`(PmYC:al^F
O@gZ#JN3'B-3:XG.$$-f//Yi_+S%Z<?jQHGNF7;35)Y'_*[Hg,5fO>],(-[<M4s\m
)[+#s.N\cR!an/!K7NA>!C3ks$A*d^g'Jmt#m<DHU.GPU%g4</6O>R<coctZY_F6U
'R4\(%AZ$k6kLY8'GlN)csRqS+AhDnTjuaK*t;^g(e0MF;&hY$UECm#MF!F5jp<Yl
>XsqY8JE-I@=WeN$:,e\7hR4a-%1_]M$u]^UmTL42W:m1*3fNi.3U!iYi[nMUECfi
!?jVk8q>(D,Vk=qLqEgSiQZT]$RDC8QkI:"=qOBogIMJS+Z_"oNT"cKEJ24[ZkS:a
.U3:B,e,NOLVZ5h*.q\h$6BidQl&/MTSs(($UL_u'F3PUHC,"*i5>e(5s%IR#\-,'
M?q/Ar[#[7!.kl?!l1re-3/kkVM=NUda\XLdO6W0@/+U]K0=1D'8?SY3NONW.-*&j
m6m<NLZ#tZ:83F3-5R!fLKlD4U)<MU'Bt$P:]]pakAUePi0d336I?DV!qKLu!9MTB
5cuM,L`@#BYV`JDc52!rQNb]sM$6aE)Vjg9F9.ZSK+UR$ad>g5:bdQV+HciG+U&/0
%#0X:9H+#t9*bQ4h1ZuU(kX7o'VJDm#=0=D6R\iT5R8S8E,I)>\4m[!:kT(I4<B)a
56@M%)1lfY#_VnB-EH>P!DsCnJhVr^5`@gXd'+).\0u13*&NAr6M'&i;b)?T,lgdf
:B=9$"@8\B`05*U6)ZOD_-m,$?tplP\7>kQ^]]:T*"W+3E"o,+,D)RV%Dd!W$OS"*
.pu,4JLCj1,T%#Dd0^,oO9RY+:^Ve>6l3tD.M1Pm$\sfT#(cP62dpA;";%qe![&jh
i(Sb1JPm<$>QScYBIO!:GRTFr%1iOo/;AFf&)bk\#11bt!K`*?_>l:oiF%9FTe$r<
N2m4LPbJ?o<_NK!Jd(,A(kg@V0LB_)#,%L7JRF9Ed_HJ#iFG@\iX?aEA*=5l:^X(M
:E9Es+=3bh<s%l_&qY?H"Fqh9:S:JH^ncSe+A=>=G9.4oJ/09%S4SK4Q51*CTk]*k
*W\T0!.[TF%A8LZ"7Tb+!6@0eVAU!I5[k8>QrjM7ga34ja<H;qX9O=l*<e^b)8aNi
;;hWbKKuIYa]PYR62V:GPQh=X-o(quX:g0dL^[$L"pX`S.KE9P*!@s#'&c@k&7H>&
!f.Gc&C,]UJ2@X#cmpCdZnDQD$3ZG.s#?rN"G>W(;?5&m$R%2<L#A7@K<U%5TnGqN
&e$+>^jgkc_9fg07MJ*2-l(\p6%dOU)$4Ie!eC=\JWpKM5gWYn!AGJo&7-!&W/_F_
^fUjd'IuOY496(jhZO\<:d[AY,bc7oT:hba6GPN=L28DkTO7f(-mQ'k]KHK#*%XD6
@uKCr!/?/g'@\E:3/OFSK$\m:Kof%<$PX0VJ0ktikQqLPN!'9q2AlQuG7pXo2ho\(
*l&'k$:7EBKYTFH63&BJJIj/[OR,PhkVs/?N"ggs1^8K?=pmUr-=]jr*^EP4![6bg
L1&"I0Yn51i?Tq)J1ejsQmW%BoIL"Sd2L+,JI-jS:'KQ4]R_8@#QXW-Je44L"4.Sd
+`opQd1@g!La<KfQ,iufSW&(n_#cm7,`:SN-pjCa_4]^0KE-N3!O)b25Y)E@O:E33
Gaf=rpG<Hn"9\k<@g3hI?Nhtr'>VDR!EWrqK`H9,$@T]d+UgdEE/0Ij=I][U"?hsS
,V9,FD#k0F8V:Z!#!eOg!s'qY!`DK7"(5I=5YW+!0I-h;OD"r@?l"NZrXQf0#U3^\
.L@h!#gU4>#<QihKog6SEil2a!WZD^14XSccm9"VL^9dV?k*7R56h3C&qM/n&V;\;
ItTLPM/`G"Z8b#U5g]$_cpe`P&6?R,N$=-fC`3@cBK8<p&VZ]rXF_Q_!oT.BA71uL
_a"D1+Q-E/E!'R*0Xhh6[m!USh@<iT57)i_081_u8H9$h;ZMV$JrloIW_a$,./e-<
!"oFN\1kT]N!T\RcSIgOXoL]i<"Lcf)<=H:!?`X$"-?=f.**S9TLV`i+^Qc&Y[7Cg
?j$I/j9.d4$4c=E$pL/7>QDJj!C:A&1VfR`")&p[d$PX1E(M/^cj&@BU^.#g:`onF
GSX_K6O%]d#Xc[4%,cpUJ5@p86LYcn5i"!O$*XJ]^;dL14<+QJ=os9r]*_*]$A7h$
\&%!t(F5eTL(POZ6Vp>d_0dto_($Kli+E@(\-RY9cd0I1$3fAC$\a,;l$Z?$qbf''
(bfb:UHhce@`<^-Z#h!SBIj8dJ3!rieffY_&-\_\.=cs`!Whb2mWNR!HN8d+@'C"=
1]^/*"Q3hH,-D..;@_XC%AsmdKq&\3+;DX1#lp%o_$UUe$l6YF%A4gPCfX\H$3:,N
!2-8)?r@(,0FIk+N8lae6I5oE2@>!,"6VEd+Gpa3/cl"o(L[(OT^WG!X:N+`!T<;W
Tf<LT.Lb5G$(tT.^dJ@a$3<E)!_2`q9DANQ0GIqJ(IE!K_#tLH<!jb^%=oH'i><.M
&eeZs#p?qpJLUnThuk0-:^O5pL,96&-jcO\$"1U[&0<3Lp(a7o%m^C2_0?\<5RW,3
%)C9r@;HLk$k9EZ=^^YYa\i7l?jd7E(+Gn6iX!ce=q[LB!W`oI+UAZ&n-ZtT&n(&<
^j,Yt&C6:P!W\`+O[('uBGJ>d$h8TW_0?GY9FIP1$m>NX5h6>IeJBDL'sX83+Mn0[
r"jo$%UhI8+KQ+3V&=k7&S:Y>TTU&uk8T"*#jgpuOjP1(eK&Y_*O4E@n_kNDjW8F+
*jP)RiW^MJ~>

Q
n
Q
Q
n
315 534.12 60.9 41.88 re
q
1 1 1 sc
eofill
Q
S
q
45.66 0 0 33.84 322.62 538.14 cm
q
n
0 0 1 1 re
q
W
[/Indexed /N278 /ColorSpace findRes 16
<~s8W+DG^,=3OI2E&TV.sVW2PN.LgXUuJ:N0SYctpY^ppna:f'u-E,]K(BNSA=!!!!~>]
cs 
<<
/ImageType 1
/Width 125
/Height 92
/ImageMatrix [125 0 0 -92 0 92] 
/BitsPerComponent 8
/Decode [0 255 ] 
/_Filters [currentfile /ASCII85Decode filter dup /LZWDecode filter dup 
] >>
pdf_image J,g]g3$]7K#D>EP:q1$o*=mro@So+\<\5,H7Uo<*jE<[.O@Wn[3@'nb-^757;Rp>H
>q_R=AlC^cenm@9:1mFS%/+lLT1imj&.f6S"9R!OJ8*(E&OiIGBf*q#%\ZJr<^AUS
fG:GBVcDt=^eK,D<hi[qQ:g'`(N-P1jn9WfNnOlN`oqM;X_-0q!eP;*crIs-0"P"u
QOGJ+%hl<LDq1n#$k&'6h>oIDDC1Wm_.Ka8ph!"GCpI`\(0sBG)l/[1Y1:.5)dR?\
>bJlZk"@.R_<Q.[/T<A%$d7R]&ri1VC!WpAGefn?l35GJFELh/*ttFRl0._(:0a-2
@a+I(\/e>+(_$QIW?0:g#?S"LgUR'_V/lP:J7&^Rk./]Gput!R^^:2oJ7'@p^29V^
__nT\pAV+2qP=0CYQ,T']+%Ceq`dkdk7+b7a;Eb6^`'$U54%$Aj1GggqPcp1gi04m
J.t2.6nX+j_DoaJN?"oP_iOr9d"EV.6>_(0m^3Wh2]T,2&s<9G^iDKh4YdtNf;l/M
!5C!+)lNrAi+eku8eIPj$o;khFX/CjlE[05^bkrhJEZ'H"&,pe9`QUlJ.)K-i"ELG
^/@VV\'g0ZSL_`Y]-fegZg\,_!<?dSNCYj`*9'GLb]]c)J2EHZ<RFnN(<,m&h!S#R
bZr8j.YR\%JA=U-:k8TP*!RWF.l?Y7ZRp5fbE`h#/ZBJMBh>_V'"^h-Q0fGQ;mcdc
:oBt**!Ure68(#L',/tQbfW%pBRugi*Db58AD&n>2T'Gp;):X$5@B!NLJWQR/a<Go
2c;4nY7.fJ<DaR&\HgVVFbNoNdEH"QgU2_15M.qYa`;q,=;dC_aKsauam.o%;nMh#
F&l*0#To>el@&7N7@<aaf1U;t94@q&h9V?tR;+HI8bB+'<&kD!T3g53elDn.drp-d
9sB=dg:418l!`g9:7%hhM$?&Hm&p&^ein;C'i<c@BHOBi\b=p17Vp]\PM"JUdAH#>
/bcMS%+Zd?f5sguK4?f/otG4W(885rmD^f*nGGUO`MgH0Mn/8^4^3PS=`5srJK+SQ
ZGYK2?,bqFL8?-8(S4:,nL-%&^$E@tL<N/mqIQ7#$B6F4m^gAiHJJ6e';g?;-V:9.
XEH4bB9RFAk:MhQ/M?3gC)PXugF$Y8q-I<-bc\6.m@83FC*Ce!]^'P-8ZO?Blm2iO
,]r[EP<3Ks3T70^\DU0b?%=B/F0#G];Np?9D_NdAZGqL\Rk)TA`4c7)GR/p4L]^:B
0mTG%3(.)jN-8gHMjjcUb9.`q=A!j'-+$iR+W1o.C<`G9j@9%WX:p8h/_2IQW9I).
:P8':&>S9b%A>!tHS/a!09itDieoF*/+sjojLSDhA)MLsp*W2I9+YIc;hem%p`f=m
*!oj%G`;<C6f_Mi8>H-1W[%eX<0nXH*,B?5'a?)=JJb&%+HD;$1rX^D9-_qk?N;73
+LYPqSiLb80g+/]Gk3,F(]f]G5!Ye9aXBnO(P<(+;TOGbiY,gh>j?lR8`D*?TS)`h
YcuH=l"iqf`&O#;Y#>n2JJCFdI=getq*h7US!m#HO7<Q3_"Z^^&7J?fV8d#TWN@ME
*+(gj$;a-(ke0t&nXN'@C(hD=(D[^bNQ;<EO?&nJhF^L+'@('bl)KB5]NpT?\c'e+
,oM5Q]OgL@C!^S].OWG9!OFZB:=oDM*_ZoN$O.!a8e2]nKRHl$3aWHM2\dL1?"[d?
?-u"8X/G2,T'jISZ7/mBkPXdCPg5E<6H:gZ]]Z+@JjRE`>t:LPJcW(^F9!4,;2SWp
L@eqE;sH@9k^-o7YR*57.S2Vb79c`bp2&'d>!a\HhPtPR=]Kbu:.Z0^KZCq_6hp^J
X,M]5&E8gJ)R2l7<4Du#0"4=X_+Z8.Ha6[IS(4ICcR;L;MtOfE`(;7'On-/l<fVd`
L>>oYe;f^a^,a@N])Aa`<jl&Gb<(%$^F)X\YM]Jl[V@a;mKKjL-9Bl&Mbu8?[CpiE
#3K,/M,J0.kZBV65WVGo<+(Ll:8P,]?+[do:3Ae0d,KFBg!kAD*S4%VK(^1Bh0X'o
n%M9Ndh2<d8h4JPKf-R!9(aT?b?_uq[kQoAHSVNKoO3$%q=5de7%1:_hniJbnCtKL
Gq%i\=pPIb+Qp]A?Rgk#fT-VR>Y0e%6Y=6&6MsQ3B0sZa>CMWq,:^?#NU]Id7h<V_
^aXApX\8`4YRQ4OQ^if]naadnlQtWIR?Q\WC9^h!^8:1O"]Y#?BW/Bm7Jscao(HLI
msLPTVS&u$-67\uZRi;8-_&YXER#HJ3G2A"TOLn,\kMD)6<J@;,hkl:;e&,W>mU)Q
*dN@Am.f)T'(DW!onf`7@qeuoV6n7/dnCWh6Mf44iaf#jmp?K)[g^E%7]4d?VcIQG
4`i$_e^`^f`Cuh>XnAj'bc_K6_;0+7osm;TgC%J,?&c,_7`j=f04o%VS[8$@&g/:~>

Q
n
Q
Q
n
227.28 559.38 57.12 47.34 re
q
1 1 1 sc
eofill
Q
S
q
41.94 0 0 39.36 234.84 563.4 cm
q
n
0 0 1 1 re
q
W
[/Indexed /N278 /ColorSpace findRes 16
<~s8W+DG^*V(@"<cXOH>QkR$^]H:l'p`TV.sVW2Qr)Y]+Q#\@B&a^qa&S=NJS)BP;&~>]
cs 
<<
/ImageType 1
/Width 128
/Height 121
/ImageMatrix [128 0 0 -121 0 121] 
/BitsPerComponent 8
/Decode [0 255 ] 
/_Filters [currentfile /ASCII85Decode filter dup /LZWDecode filter dup 
] >>
pdf_image J,g]g3$]7K#D>EP:q1$o*=mro@So+\<\5,H7Uo<*jE<[.O@Wbe)&/B2'*/*KJ6?7i
:G8)$5empj'G(QRJu8ToN#G8NNIcXgE$X:\$j?_61Wf!\="U(6^sqX,,T$sp;Q5h)
SCX`&W5QKei)gBq33*-Ionq:?LIJRJ/[cLENeJs_enor17(PfCWa'<3RU+>Y#.jnf
'1oV>O9l!GU_Fq7QHr(%g@1B?1`I%!WTCClH.G<3+/se]^miUZOaYNknGqqV$Hl5K
lMuIK5R,>B"OV=6Cjnla1'_YQ!:3u(=[psCEj=u(05_&aoBnY9/t\2]cseoK5'Aap
/I4jh3k;Er0l".*Gi0)CKE\%LJGbS7+<1F`4\bduU9)[]d`jC]Mno3>CD\2[5;1(n
"!`YkaQpO4,Rh@P&!K'Y^9>.\!<>r@+T'$K>Qgn/0'EfTZS.4rYf$tJ7*gG3]Gh3S
0!b!K[r3KppbQ_BB)9/:Ce!-qLt"!u/F^eql``Whp=MisXHaa8:C;^h2/jgGZF+Uu
3o_H8$bV/7&7fc$71s]h$o0RD#8PJ/Mn4lsa^SC1TSjf%-9O$,R3srAKNPQ-NE!_2
8:Y(Zh4k>CL':B%<<GP/P2p`'9C/^10dTICSNK1'A#.s*bbF$jWiCEX/O?]'OJ&V3
`2+9$Dp7Z*eLJ`doV/H^?F8&$XP5#Le3'9a4gQ+$kLC.)AQINda:W9p!%hm]fs.oR
9$o9&q`<6Wlgt:\EhhKm_(-/e=/QL=\COro?,Ir0e9n!VJ<Xp$#M6G%+V)M*M\,$J
f%\MshTSA82bj!g.lkZArC$4RnLb6nfJe[5nMF28Mf#cp>mYr"G9eg!6S]$"?THc0
ZUi!cPK-fe=Z*Z6foB="4k7%5K6*oTj7@jh5TB0]i>$/KRK/eX2*X/`#.1Y\!&AUh
XB<>t%'6n,)\R^A4(hr)dOgB?4FfWVQ"m?W]Xq,71W*b*'[6W2?*@dCJR)<J-RRmE
Y+qsQ4"(?0`VQZPZJr>.m$kUYc"4Y_;LM&Ve@RJSVTpiiIq,Z`L2r/0Y-Z.HBfqm,
/HQc0EI7:6`;Z/QEV@F6i)udU'6LoGfbj,!P<]Cn]mjUR3]8$&H`r;_LMk@4?=C\1
D86e7!-JC+j6%7ShXGfM[gr=ADr]U+jVP,#ZnEq!!u9=RQOB8L9p5XM?:mt+9ka(1
"4".(o9atu%$j!)kXqEP")3gIifH)4!"F4:4\P$<4m3CZR_d<\k!?s<\%oc.A)04@
U&LN.TN4Y4BI##N!l<pDeXNm.-Hjel!//5Q+4J(,XrN-LB2E!]j.%t9_?1j6jQ&m;
3@i<:HEFZ+"<(5P64d"6\-AU1'Ul*ROYRk,1\B_^OrA)6[$EIlW+7&F*JJDE0#d"p
Je_EBFg25OX>aD;:\8?I7'Q$.=@Tk4e,(G2&;J#E6EoM"A33V9k!##X+<%"VOH>=9
!#R%c@&ueTn-"q;pr`f$!OdDPJ[r[QYoK5qF<V>X[^%)M.AWBqK9!Xd2a\d(U(jo!
EfO??q':6H6l&9&[F`ERTE81nP`DP#,:#3Iq4X>!-Lt!Z5W>/T+S<N]EtQsGG:+IS
H>J+P>"(todjRkjjI6?KD*8^^,>l;"!YA'49f<_KM2\s4&jX$uZuZU&K`@(u?:^M$
76Qq]$;IQbL!!!36_\E#D<M1]bYoik)'nF@8'U'.8ZbFYaqKN8k)l8nN0)h"A!5>*
DGiu`_:#t7SBHLd9t?H^V4j<3&].)fb%XZ9,sa+P4OZk8BhIS/pS\Ndd`*1DGirf>
5P3XS\o`\oj2isI;f)T`)Num)CrW4_T!M>[!EJCO&?D&OO@ra">,m9?XXG[.eg]oZ
CHK8+jmns>GM':_m8C(3#hGMM$XP?CJ33)AF.>:Yd4=m*V3WUF2No"$hRU4V;3&n$
)VSI:$0+J#HE\DNiDJpo5]J.-aOH,>@Es"P[._V.PZ+&*+)HZra9$nDqeT5:$Oj3l
IX^$%NGN-amkW![+\qnpAo:n;\!+Lrf+TBJmR>I5oE>u"a<P.'<;s7kB&gq4H3,ZI
2iEurF5.^WEY,q,9UAcqV46L5-_2\Sk$%`*p76N3I2N$#f)X4::NpK#f!fi=s1i[^
8#YC^][:?0?3EK6bE7I\jTbJ:pE+]tSeWQ%.0L?Z^i^5l26.PaK\Y^5mQa@)04tq7
PT)#RYUj"C(aA-O]3%g"`%]0?]*?J8'kc3`hSN8>^Unl8<`&3I=Jl)J?@-aKZDG&W
Fb%oX!r%MU*0"P)60Md"-X=ukZ[uaNen&<5P)kVsS7\r6g]n:<CRT0Y#O%H%m)i)0
4P,sD$PR&5i1NpdBT>=j.csWkP0.**F/91t&u0<'0-5)Z83HgnSEp;M@gL=:G3M>W
<<Vag>LDTV8>,hlR5.?)bkU?Xg76i\J;,K'F/al4]h2GM0F0E+%j"JI';&oRn&Ut/
346h1TdE6a-Q';s6#927n"/#_k1,&84R-]3Xugbq'o?;!r;SLSig[Pa;Fiis=>Rh`
ab>oZQ><g0GEfGb\k]I0>cn/abHA\sB/"9BWPHl=FuhZd"_aD`Dq44PfN^IoDar3a
2a5C0qHUHC>Q6[mj!3?>qeY>a&I^CZqm\^\Pe=.^Xkg`+/RTBEh%"5<q"Dbbk-HS6
*Z;&is#-PHg>)"QEW[4])U84-!GkcdZ2"\sU&:[c.:*7`GIJ6S(t33le`;_!.F-`;
HZ8[gWPgk+&)J4[[rl#D_)&7!\=M2sF;mL-&D'kLQ)hOSC_,IjcW5.YQc(%R^V"r4
I5E!6,C*':jo!/eo3Q@\H/CdJaQW^~>

Q
n
Q
Q
n
216 435.24 49.68 41.76 re
q
1 1 1 sc
eofill
Q
S
q
34.5394 0 0 33.72 223.62 439.26 cm
q
n
0 0 1 1 re
q
W
[/Indexed /N278 /ColorSpace findRes 180
<~s8W,fn*fl>o=V`KT:_aMU8"otZ.%1Nq>'jSmd>IMI!U*bS=H+MX/i1tW;-/_rr2n0
B4n3CWO&q;^:q=t_84%,_c9]:L5(GZV5:>tY.;*R\$ri;SXi_Z<0!!!Vl-H+]tLGG
WgT9CQBmj5qYGD[GA:l-S"#nKXK8h;[?-K3rVc\'@:=;$FeGD#\@B&f`Pod6`/'5*
gY:K>hVRDWk$MJ&IXZaAUnk2tYChI[OcbckQ'HrQJrbtRh;-oBgt^T9flD+RM2@(I
Mi3siR$3_tSt;P7jQ+nCeq&C'R[T\&MMdCQNME8DZEgd&Q^<J_LS:E8['[2eH[Cp=
P)P?YnaZ-W?snM8J@iG*Pa%D^It-bKl=ajEI=6N_E,]o@FE);?F)uD5A7T:aAo;L(
G'8%?AS"M-93kh/<`W6s:JZ7]H0ae^KnY5!Df9lFG_Ca'@U`eE;GpY#=^#!49he>U
9MEj]dFd+(Bk_9uD/E?U=&Dgl:/4REj5XrlCsUGRXf\_IaiV<4^Kt5Q^qd`f=BOM>
i7co=@q0$Gqtm7fVQd;/iSia">?et]_Y3]so()?eCMUMm]'\nP>[1P#m-NoukMP1S
p%A")d*TtZbK%ZD[^NWoeC=!WnGN4^p\4FSo^pDQbsk/lbfn:%84_@af0_nm`l?"i
8P/12l,^re6:+";;c?1V8)iOf8kM\~>]
cs 
<<
/ImageType 1
/Width 72
/Height 71
/ImageMatrix [72 0 0 -71 0 71] 
/BitsPerComponent 8
/Decode [0 255 ] 
/_Filters [currentfile /ASCII85Decode filter dup /LZWDecode filter dup 
] >>
pdf_image J,g]g3$]7K#D>EP:q1$o*=mro@So+\<\5,H7UlE8e92l7!J(6D?oT>n-\I":5d4WQ
$k<@AjV'<J5Saq9"G1&IW(7@SPQcZtJB2C^'b1F8ZjA]/4<G+8KHX2(N(H^'M+#4#
5bq?o$3PujqS[&L/Jef46NN"a6o,A`"(Etbe8&WPNJ?JEaLj8W*=2s\^``8s5916;
&E3]nKL$-1_-ul%&/I\Z%gU$n5SQYD`PIBVTK"We,RfXR@UT!KQq\q1"ls-;jGXKU
N^O$O#_tbK!<iYg&_LK9+"7O'"QG6uE_c`L2^Is^9L^ZL'+"^aTi6CB"VjH,TZE'I
"TnMA(XeZbOB*'=7"Rb8oR7l4!<b_?=^Z>&MaCp`/V695$4_akLq"c:Tcg'[35OO%
)2^cEAderr=KD]-Mnlt/MrOpS(P/73$8+X'pkfs"!gG)e#6Dao.ga*!\g#.h&B(l3
!uScVZ@O-q%1@cLM&-GL=L9E1U*.Ms$f`YZ1Q;K-e.3!u@+mOKb$a'-M]u8`/d]A`
g`;9f.,[(@A!#gtLh!*t.ZC.$loU3%_"'5g6E",k%n#'T)Mhn]Q6QcgR!^JT,='%.
O2Lbl56g0Kg-:ULprko.JTuW#&2!Ys5n)]pQmW)J!73_9!oV-^K>I&X<Y/dY'GcQO
+CGQgUbFhT1aE@.1lc&'N[p#Q>a?E>K.'n?#RDgi6]?P*\3pHBR\7W\6R`WOKOQp;
7E.]V^dEpR;@Z-WiUEG6!lQc$*SN!Y8d5]tF#5<Q5Z#f2MF-5r7Kd7:&.X<O\K"+t
@&RI'%Wr,G8-l"Nj;s/=#f&HVTig;8%%oWo&rFLS\-Y*EYVm^+MSN[POb.OK*XI9m
a>ek5O;(6A_6OaTOWe\*'SD($$n;S0ib1o>iFq!f5/Wbf*"#!igcl="ar!:'i`HRo
BZ,.=81'"_(+b#'LnZ6D@ITRA$j<NRFWl?Er$MN^J-HAo^rYK,,ls\"15DPg<Z-gg
=QCP/TNLanP3?Qj,)mc2F:dP"+C:Id_^L6R!4+;T+q'$C0JJ@iGht=f!$MZCOTM25
'VtpTllladk^,c*@T_\2%3p]bL_,6T4t!gJ#R1uuG`jmVOhgI0%)0QFZoA4tkf,N<
!"pCSN?L)@]`gfKO>mnEko__lJfmT/HGUe`%#W4n.#APSLl]4?!>'8`6CAi-@AG]3
n1r5hfNJTsHnG[IE$kpQD[q?..D#"""U&ci"i>AAJ^E`q6=9p%JS650n5'XJ+H-B?
9MYoORKc0))[7F$7g*dMj@I(E%KWXT#iMck_=1hrT_'mj0g8"A-jpZ\F:eSJ&0upR
;[:0iN/A2a(4dAP%KS0n!K`<^_JgeFJp]cc<Yd!4LbJlr(cVjH0HPm,@gM#R%tm2k
'#=9,#D)@TY\9++KBOOAK^]u`n?aKt\0V3N*!M#bX;:p,$4*;`.>Dk^.*/>&DWMQA
JRCG>Jr!<O`)HjCE6\O$kQD@qlo6dDGbIH$('3dX!<kat"_9#eIcOI+"L-Gf5]Agh
C%Na)n9X$0#o=/hp^bKg49L-W1D44t9nf6DZ%5/]#L(7#!J#&#gSDIl+cW1\n1"Wn
G[1ma<!ilG>SVh6`="s_+,.LZ,60/1"(CsHPn:A45u8%!JMq5)0OPuRQoPH26neVF
0FpIj(_)HQMhs.k)#td.'EUf4JC'Af!JqHk!Dl.;E!Q\8C(puj0I[3V=pBf0'+_nJ
W.6R4#6\ur$,joA!`9F6_Cu,s?mluqn5'h:k[]u)A53<tcjT'aOq@\i-\HsW70+fJ
#2p+7K<Squ^`Xj-@=Tm@cjUqHYqW&lJ4B_2=!+F*CBEIF'nSmj+b>PY'SL-tL1![_
`$H?7!&Ob0JP8LH(hsY6bUWhc)AO%'"9PB4#)@L#_Z6p6"!Dt48V/JpKfE]TF?gEF
#F#E]5o:5cPW)SD^'-&13"TV.!<s[r(da<X!^]!MLgX0e8Dt<jiS50"$SVp<aA*+n
Y`+@B;B#U<:'7=\&;_MV"Fs&Y&Ri10d?-[r!,,:>%#BlL+RqD,perP,(dnYf2FPM`
+p!HY*<iYu$D7)j,iHmHLa+ef>6"a;_QX:Wo1Jn1E%)-G=@3Dq3!sR8W[-Rt/rJ$P
*!0\/&j\bs3!'cs"R&MbJOBfHqX=Z>#Rq>qA0uuHAfsHSFTg3]&-8IU"Y3u`+X/aB
"D?d$J8@sb,"M`c^^P*I0I@!Wcr10H0Fe0G:pL'1PRqe+/&<I?"@[PBJRK)i`;g)G
+FjNH5efi^!)+.0<&b#"V\;=oL]Tm]cN!u:%&b!kbBJDq!O,RkJH.>1iP[__,-W,B
Lj'<PaI`K!,QWIDUCq$,'njp>,Cn,\&HKa:"gB<uo,(C4TnFnPCA([2.'O2Diq4$8
4sC->L^/JF'ES8V$oHTNe&"3R!K[Qq_h^8`eF9c"crMYa11CRW&4o0<NY+TI.MNfa
?0fiu"p='^!muh]P@73/JY!_jJ8@RV!""O5fTHF_+A2k=*Wq9rEt%$C=5:]B5f?cK
(*T>$KYSQP_$F9#?s@c1B?Rpf?p5"X9%<<M$m*BL2h=Ka>6?!Y+b83E#=+)8"Mg<F
67@0=`#o<gJQ!<"i(mEZ?n)2M6j>qB=q@;d;"?@W'STY:$:'TSo%m[d!Pj*gJI@qY
_.F'B^h=%oe!G_q'H+bMaloNW9aJRK)!9IO!F`npQ[Yf!_XLqBJZLV]&=GM')$'~>

Q
n
Q
Q
n
369 311.52 51.96 48.48 re
q
1 1 1 sc
eofill
Q
S
q
36.9402 0 0 40.44 376.62 315.54 cm
q
n
0 0 1 1 re
q
W
[/Indexed /N278 /ColorSpace findRes 199
<~s8W,Zj5]n.p[e"J[C*E)Ocb]cO/T"U]"5K;l06sWgTI]^@U`eXAS&'KYHY78S"#nm
cHae`d#<pB:f'tW77C9Z=,;ZgV5:#s[^Ni]]V_R'o()@ob0#!TGu%43:/4Pd=BKru
I%$LmT:_ab\$t#BfQ)"Q8P)KN;,L:l<,lntOH>R"Unj]XTqeBXZEgd-St<m=`7!)^
=]nlt7n6HT;IO!BJ:N0*LPMt4XL#7>TV.tDlg$r,6rR#_<`W7$<E3sUDiKa9PEV30
WN!#%Xl\[+jQ,B+>?acp9M8#O8kM]iBk`6RKSG59Vl-H1_o(Eji;NWQrr2oenaY;c
fl1nL84Z9Z?sn(uFFf!oR@0J;U8#u[chdM7m-O)fe'l=V`o?";hr!<c9hfMCDOd5e
^qd`q@q0t:I^HJh^:q=ANfNr2q1F<P`Pof,A7Wa$a+]5$BP;(-I=6TpJ#fWNWiE(^
P*3r/anGH%R$a8U^VB^Er/6Jk5X7SOD/Gi7S\)MGbKJ*%p%=Q6P]q=q\[f7W?=$uG
?ZpU9F)uDZM2@RcQYUAPZ*CQVF`gtq?+@DSg=k8HQBpCahL^?2Q'IVIB4pZ#maTb9
_83t=f%+YRD"$i]o^qeNq"T/]H?a[Z>[1OskN@_[MS6^:7Rfl2kiggWgfdlbAnGY%
H[F;nea;bk0ekE"_SSW+6HmZt$47+O&.m7:dE'DMqtp9Hh;(Fc6Y^@N5s[g+nF.83
(c4'+c-=K;"pPMG%G04`lK[Zsk2nlm5N1S[~>]
cs 
<<
/ImageType 1
/Width 77
/Height 85
/ImageMatrix [77 0 0 -85 0 85] 
/BitsPerComponent 8
/Decode [0 255 ] 
/_Filters [currentfile /ASCII85Decode filter dup /LZWDecode filter dup 
] >>
pdf_image J,g]g3$]7K#D>EP:q1$o*=2^rU%(+<<X]'3!C4G>5UJ')O?rt5Y[B9p#6t@J!>q&U
>nmYK_LYOf>VHNoL4^UffQ(=`L'L)^nGlB6+V>!uP(>#6Q4]ch@%q'hTMR)4#K9$7
@'Cb*(CS4_6&<[[;AkGuUM;ZnCc<=;a!*6_k]S6]Ns5^@4T'4`XAOZrnc8kk1a**[
A3o.\GXW%'KS4^=KTJbO;23VQ#lIRL-'JY2ictr':^;hH"2NSXUf5FQ8qgA-=AU(Y
$A\bVVL4[E,aHOVP0n)J>Si`"T]%<3-8."gp+TDGKZ%@M5tls*"qXe()];9Q@l^2G
-o@BEA2/nQTPHFtN98M)bh^a!&P_1lEHGSCTS%c\+GEMcYU,;SPHk/q6^W6^%\p6:
#RU[DM@9O'_"')b"46boKO]i54+MrK*Ysg3ncTp6U'T`d"7./94.rA<r]g`7#]_)L
KFh<-!<a74/rP?q0L?>O3=IGMi.1;6&Hc.d(4_IUEXII$!>7g-Ufc+T+MsM?&;;B;
[QfnJE/H`0@+^?,!Wh6_+q-e)IO"p0n0ge_A.k2!%>6uM"bpQDQ667F#p_ln"?@f^
&qQ^'1lfIMne$Y-^q)U\TQ#]W$\9HN(6ZcF]G1XDpc]X[j2_SJOoWlV*KpWI.4p2s
aW<s7AC;(nO-+*V$^%)5eQ@oDJ06Y3";RFI'5`=L63ll#H5-pAfIf:@1&*NFL&o@[
71CMeE"O>9:lIgEJN3!D>C\\@5*LV$\4V;1+@n*gJ^HOo+iBBjCBYmf4phojAVrtc
Tm6&>N<%$P#)D:28.1XF=[3dV!<BD;!q551&qT"i\/(,Kj,u"r!t4ONN<',:g^#(0
E[:u:LiP_9JKT%O"$h,S-jrD84A:R0=NEr:,2enFL4Zq*7gFUlF=r,R-ji<EEZ$Pe
L*J[N)3cO?1_8<V<b`RcT`AgR!McV4+pK7X0F\HlG]HXqEM=(?!Mk-14;";i;Cd@p
k[$a]A:V3HOMQ*B4p(i6;%K>:Te[13llKoY!eKl(4UJu684/N5@3#aY,X@;Z'*>Zh
KbU2h&/!'=0U<Xk,.Q,m"e`YU-ih/hSjn_"BHS+S"ZYoTg.3?b:G&&D.@UJb^nG*8
!$P/ol9La4PlT_c:'Uo3392Mr#UrZi&)uMP#7tB[MDGRW0JF+FKFi586F^_;5n'rL
T[k@ilg5g':e-*;P32lH57(`I%?OFd+iQ^-%7(Cb[NnBd`Ae\G^d%r&A#)Bo8?3"_
R(<:%Fo_YX9,)p_8:`H;&H^lE#f<eg!T<t0J^=o2_E$hqYuhWi=>p;?***C)3.f3g
!YqF0;@4QcI0"R]%:Sm#S</U/^j*"nhuXUHE>o9OfJ!Bb=:bLA'FD]s06ptk4Fk40
cU5Jc"JE72`)6dLJafH<5i=#HJ6W,-j(0@-KL>k7E[ALXL&g2f,6IqsRY7(f!.q!H
$M[Tu?^q?&ikQ61p[A2Y:g=-2kYhS7.L?3m%hSfO5tBo;/4GXl'OmFs"2PBjJg=hK
U<ErH;)/fT87r+0cl!*C?3.u0"EM?N0/XSK$fQ2B(4t$C$:)f\75,ttKPUmD@#,2C
\-i>sQnXVQClCY>:Bc91(5UoJ.u8_Q#J`#^JTm=j6%EbR;HsB]J2@<L5X8FhibX;;
OsWV,!tc_>$*URB8qJ0&Q9adqMfKF:_5X1r@)PD8o#sFO+<_!L6ofcp";Cle%KPE<
4or/'cs<jZ"CT/1"0`gm_lu68T\(PC?jmi;j&?NH\.SeG#TDm:#nc,M:BrQ^)8m)6
&AXT9&0Z!F7>O;9i.042@0@0.BFk1'5X#>YC]V>UUG6/p,(m,fV*aAt!atpE:%0bG
!Jl++TbpCWE*rtPJI2G9e-6#*-L_L1&1++`,U>=5A;+D6!MZq[c?I\KJ6Q@dTYqq/
Pq34C.$+F[S2uL(0F5PB-j;pc7u&ja"5%:"&HK`b&>8):JYYJM+Rg!LA^UP]YT9(I
(`&qk-7hMLM@0Jr9:ir1,Cpt,"ghf(!C7D?X"Xd4i:'Tp0`EMO0WY\V!'#dS*/3Q;
<<n*9K`r'1.c!FpZsXf">_$&f6Z$oG^`ZR,Tf<I5GVp(!e2`=m\c`)rCIb+,$3PWN
C-Wmo&RdXH#4YA2c0.k0@1Y&GE"!,iI(flC,_Q=uFpJ-\:SkmL8r1h0*.`><&tiVL
#qunpQ_9NC_5m\C@*0t:Ll;M"a9VmA+9]Vb.LS1c6!bZ>%g(*E'-T2&Mm/?^B(./[
[KO8Fd4Q``kmA%Ge-:\9rZ;+gD$"^KAUm$$.DgmS!<PM,K:jn!_LO3PLS-^M^g8)`
LdhIJM-Pe4HU%QR>nS>0)Zg+.#Qhe7=!4+J!O,lBXQTefU^0PLJQ<\AG]j<EY"F:C
:)XfPP62u`-j3dI#f7]#%UuLS#k8`A'ZJ]6?u/7;X=n=>GTmWL6otb3S-XXQ9EDR^
Q"Y^fE<oAR#JhZ4Mm*To^j#tn@A$_Y4_,TP[Nu@A(^l.=Rk'/+7M.s@;Zk1*$UNF-
#rtp7!oQH^_]]0mK('k8/IDl9^mGL<'L=3K+:pjF((R"I,7-(a)[/2,#f,Xd+4+7=
6?o7=,-2.nO=gQ#\4[H"M#Dq`+<LScXU-slZ%CnS,s`sa#f-4,#>h!(!&.Re+:o.f
.%ikYYS@AXSc&QI&Pmpr/ISfoG(u+D"%$*3#(e6H#13htJ\'kRi.t&-J@Gu2cus;h
K+*Deg)hl6!tkU,&;+t)*<LA_%cGB)J,r+K5d6.UX=tXu!&+Vn(k2ZSQr]!(]E!I9
\d.1>,_EZi%Rh3W#/YY&4L"A`__@ql2i;:$^^:GQ(j[=_\m0u,Xp2eRGR&imKSj_F
,LldZ/tfj5KJ>XQ"70M!/9E"l5T1;gi%,7&pg9kk==D&=OTWD^.Y.$o\Nq>h!2>Dh
M?42?!`5p,i0'Xa:`^DVR0aVFTO!@]mKQ);)@?OF?%][I5t*:E#NDgG"RtOY+Ij66
Jcu-j!J!oSi9HnOeclQV&A^!E@+l9'%MaM1J7Y/Q_!hF+N#)M6+Q0%"JQN)+TR!Ll
]YP^#8Gj/EhA$#='k%d[@.FhYEWUfF#/MJd8\tU=.b?2f!Pk?Ba5RUPjosp'%7!b_
`Jh%HbR_c/+COmF^k<7e8.>Qn&HG9\?m#nt3Zrs/(I0AM_%I=;rX$DE%NnddcI<%A
0E@db!oQ0G"6]o]pm5a$bjGNTT_]Et/>f'[%0/3giEX-l$3EIj''Y\o!+b+T=9Dqb
"lNVd@<*K@_?,81pn/H9JJJqbe.&'q?Jl/)^n)%/E*06r%\\%X5WfY+4pYQakhlFC
JDq.`E^G:K%=n]e^r-XJ%L-<i#68)G@%mqB\ddng"GA<6JVG:THP1iX"9>e=@#/UW
.KI:'DdYs8^odr.l3tHp#(T$5M%C66$kU6'+JB,WJJc5=n.K.*"J@(G8kpM6GRi,M
!<HX8^g[D]ScteVj/*_+A*so$)RD^t%a,nm5ZnM'l3h#='*1K55pQNI:)#tq#1&5@
i<:-.)A*#X"(4G0_iP+3&.nmX"@*M!!Y,m:<"7po&HOj(!CR2Z0JT63#f'&2@<r<s
6j6sF#_;\6?s",YS.n7m'O],g@-eFQg^3LM"2I5,5]."M\.\l)$,^F!5^EXmY/t:)
!<qg&+S>=n$ils+&BY"!!"]F/<WSjG#6;7Dm:ZLX=q7gEOT7oc!87n?k1'JN&tlTH
@$4@f&e*-1o)Tm7i?SmUE"G;h'&_UUKqnjE4q6`8!UTFh!9sQWVQ6C[!J)p8!7o^&
S.-TS%8H$sNlhCNN"WBV%C"IoiC=O^!Xh:^&Kqu#+I!$Q,Sbj:$,?lWiHDnBZ4+^Z
#[duIKTZ[n=q6(=e)l/l@(HV0C`tC(1Z6gtM"V*^KNqpE%H'>PJF::*=p0@^&)f,I
bSXuD4;DR(&n+*4K_,>^<YSsl%j;i*@"Q(#8L"6c!alF.+N+C+0"V+B%>k]&@4EEq
^_"s[&"q8M_"\as1'bV;#XLQ^i!Les!W\oJ%\XX@i>**RD[#&1-(lLd'6FU)XqM,]
&g9@F+\352<YDLl%V.a25r'%Pc4+2/_]^3664s9,(^4lS7%n&l+F#(q1'Z[@'S0Ej
6!=\idL"hY!atR!^u?&Y/-2Fekhm'Ui6*(tkQ9]A"b9#Q_"[un(^6TA%\VSoJ3t&+
p^gj0#B(;d,p;BD>R*Md'7imk!(J?O"p*YL!eAJti'[`66Aial%tRgci(aPcqDs/T
FMP0l+L]<Um,;=lIZC/J5c+`N/.',;#bW.M@87",E!V%0&:c/:Bs>/+1_/FP-c,uq
!14,p'0F;U&g`D:!=TSMapJ,(K]3+ITk"<m8-+7jc2egd5[FO9@Ko/h'(@.[_&`c;
kQ=+Gk^_.i_A!geC^1O^#!i"e!:;8q";8N:'`a[)_!20_<"L2;`9Ca(+RTE+9H[bK
M.%\i@16Ln<W`@,%KR+@i4'6TEY"g*&C3jGk(4(NL*9uA"[M6UT_\hb@0rU@$/fRJ
i,AqZILAD]%j5*a"s+4]FpkD"PG>u"i=ZHihDBaN#_?G#i"crurX%Kk&5G+c"T_i#
GS2c.+[@@TJL`PWfa=Ct%K[+V+IE93)+)BH"Q6^&`l&Ag&-3'K!^OI6crgbWKEZo$
%\V;V?t1*1C'FZ2:4W0V+Sl1*((&oj`I\^7J/YYqi"Y+.!2).kiALn?'Fd>,%A84R
iH>OLk9cjG<?PR.@!EGP5Qi62&V,T;i12$jcj*u+^qcZO+ZRe5#\9U8(*XS,i8Zl6
d)t:T;;quqTb\"KU(Ldh&AWf"+W_Ak-3oM12'<G<TWA>?-k/MS$Y^1T5p:<C3!q1/
<^8DL?lfgY%KN/BmNN2T+\5<Mn,RtM0*#9[_?`cl;@,'S"b<0KJ<gV[0-gbg&chb/
!-A?0=Ogq1BC3VHJ7WgSbQ*2:!H2EL?q:@X,<B9N"^k:>a^,7T_uu`:$6frd_,(Rk
2upqc&RecI+]_jkom,P?%tdU^@WQD[i"Y*BIt3Ig%6Oc$ndRkd'qp.$_+Y4;!Wq=7
Q2hm?+ZKQ)@ZS<p-@l4%@(,I<<Y5?l#,$R?TeHZ.mKZ$RH3/'@N\9,.dtHX;_;P<+
i3!^NAIDrc!'r@HJBSL2=9N"c&HLG`JHZiV#Xs8q$QtW*^kN<W+92DomX[cmJ6^Bm
cjgl`H`DH!aM%n07m?Fd$,GU=U+?k+5Qg7o_9@[kTNV=>#Rc0fJjA/rJH_-Ir!FR6
G/3GT+>BQUU/jMb!Pid_TV2%0rXe"*$U?<UK(pT6,6)%>Jr$]Hi+*:)?9ePp4()k*
TM>qmFpA57+@*jO5Z@j/WXq_mJ#(^)TLKBq9EW)a$dWK7!;%$u"E%VY#@J.&i6E(s
"9CcP%'M&`nei9r#ZT_u"^r;WLF\W47MN[,$)$Jc@'pL(U_a#5(I<3Np)F@2N534=
"#)g,J8>^H*X(F$%=h1S@.4@JL'I^C!l5?QaUf0+N_I5@%H.%J,:X%RQY'B:Md]D4
6#Zir9/qJ@&]!tTl2V"G=p:RX'*)nR+VFgL1(YS:"e]B8!$Da/[t2Go%`*5sPV<O*
m,J(8'4AT^+ILfSdurZ>%`!9(_+k^&fF<AX#`CMOZ.F't9:fOGO[ERj_+4_iW"4Ej
TW#@(i1p@g.MREs$L0)O+GL>6&.i5)KE*b<TG@UF>+&eHVr1q_^cW0\n/t!9&O:dW
MH\CM8su>o&V*[i3KsuYn.Er(!U$$e$Od3[H3PL6rW(:G@+5d,n$-73&-4$a@.F@!
2@!6l#@Jo6!Eog,@LVG>"lf(T@%[\=%L?K6!qg"<+P6_Q4d`hs+@)S7'poNp<WV,6
%=oi-m#Vc51^$*7'4?P#DmU&60EIip,@Fmnjm!#BT"+Zd!!%,W>@7m.?kslZ&n(JD
T]Q?l4;;3n"B'COg]/#'Y?>7fX^Et$+A0K)g)ts&HMOLJJ.<,uU(C`%%c@g1!:g]V
2*Td)"2PHL^eX3ql^%S_!5N*\@L*ST'aFn3Q9e;AN:[7H-cTRA&7F*B#-?jDs)F`A
&HNlB]MK_Y#R(5S#65)]i#W>Xql=,P]ba!Lp>FsNPRk@2!/mIET_#jeJe%m@#4jSY
lbj$AdK;V5&HO8_5S+I""p8&;&7F15+Q*d'*"Ckfa<Cm(!=fl1S#*>C#cPKj$UKI(
(59OF!W9k:dR@qZ1(1_GcGBhe5stdJG8+Ho',#ZrT`dTQ\e%-=AK-3Hbl?%:4:`R.
dE*.0Ao&04'F*Ka'L=Ad5dh0H(_P6_)DT1%L?o%o7?2di+J>MEiC3pc6jk-)$!GCZ
TU#iUQ4#SL$T=m+i9CE[RKT"gf:i`i+<h#<[G*stqE[R)i&hVpapaq>!MJ9\O^6\X
4q&TN!]a^>637~>

Q
n
Q
Q
PDFVars/TermAll get exec end end
restore

%%EndDocument

LH
(%%[Page: 5]%%) = 
%%PageTrailer

%%Page: 6 6
%%PageBoundingBox: 12 13 598 780
%%EndPageComments
%%BeginPageSetup
/DeviceRGB dup setcolorspace /colspABC exch def
mysetup concat colspRefresh
%%EndPageSetup

%%BeginDocument: Pscript_Win_PassThrough
PDFVars begin PDF begin PDFVars/InitAll get exec
save
0 0 612 792 true PDF begin PDFVars begin AS end end
0 0 612 792 re
W
n
false setSA
{} settransfer
n
218.58 415.8 m
217.8 415.8 l
217.8 416.64 l
218.82 416.82 l
219.6 416.82 l
219.6 415.98 l
[/CIEBasedABC  9 dict 
dup /CreationDate (19980209064900) put
dup /RenderingIntent (RelativeColorimetric) put
dup /Description (sRGB IEC61966-2.1) put
dup /ColorSpace (RGB ) put
dup /Copyright (Copyright (c) 1998 Hewlett-Packard Company) put
dup /DecodeLMN [

{{0.0000 0.0003 0.0006 0.0009 0.0012 0.0015 0.0018 0.0021 0.0024 0.0027 0.0030 0.0034 0.0037 0.0040 0.0044 0.0048 
0.0052 0.0056 0.0060 0.0065 0.0070 0.0075 0.0080 0.0086 0.0091 0.0097 0.0103 0.0110 0.0116 0.0123 0.0130 0.0137 
0.0144 0.0152 0.0160 0.0168 0.0176 0.0185 0.0194 0.0203 0.0212 0.0222 0.0232 0.0242 0.0252 0.0262 0.0273 0.0284 
0.0296 0.0307 0.0319 0.0331 0.0343 0.0356 0.0369 0.0382 0.0395 0.0409 0.0423 0.0437 0.0452 0.0467 0.0482 0.0497 
0.0513 0.0529 0.0545 0.0561 0.0578 0.0595 0.0612 0.0630 0.0648 0.0666 0.0685 0.0704 0.0723 0.0742 0.0762 0.0782 
0.0802 0.0823 0.0844 0.0865 0.0886 0.0908 0.0931 0.0953 0.0976 0.0999 0.1022 0.1046 0.1070 0.1095 0.1119 0.1144 
0.1170 0.1195 0.1221 0.1248 0.1274 0.1301 0.1329 0.1356 0.1384 0.1413 0.1441 0.1470 0.1500 0.1529 0.1559 0.1590 
0.1620 0.1651 0.1683 0.1714 0.1746 0.1779 0.1812 0.1845 0.1878 0.1912 0.1946 0.1981 0.2016 0.2051 0.2086 0.2122 
0.2159 0.2195 0.2232 0.2270 0.2307 0.2346 0.2384 0.2423 0.2462 0.2502 0.2542 0.2582 0.2622 0.2664 0.2705 0.2747 
0.2789 0.2832 0.2874 0.2918 0.2961 0.3005 0.3050 0.3095 0.3140 0.3185 0.3231 0.3278 0.3325 0.3372 0.3419 0.3467 
0.3515 0.3564 0.3613 0.3663 0.3712 0.3763 0.3813 0.3864 0.3916 0.3967 0.4020 0.4072 0.4125 0.4179 0.4233 0.4287 
0.4342 0.4397 0.4452 0.4508 0.4564 0.4621 0.4678 0.4735 0.4793 0.4851 0.4910 0.4969 0.5029 0.5089 0.5149 0.5210 
0.5271 0.5333 0.5395 0.5457 0.5520 0.5583 0.5647 0.5711 0.5776 0.5841 0.5906 0.5972 0.6038 0.6105 0.6172 0.6240 
0.6308 0.6376 0.6445 0.6514 0.6584 0.6654 0.6724 0.6795 0.6867 0.6939 0.7011 0.7084 0.7157 0.7231 0.7305 0.7379 
0.7454 0.7529 0.7605 0.7682 0.7758 0.7835 0.7913 0.7991 0.8069 0.8148 0.8228 0.8308 0.8388 0.8469 0.8550 0.8632 
0.8714 0.8796 0.8879 0.8963 0.9047 0.9131 0.9216 0.9301 0.9387 0.9473 0.9560 0.9647 0.9734 0.9822 0.9911 1.0000 }
dup 3 -1 roll 0.0000 1.0000 3 copy 3 -1 roll exch ge
{pop pop pop pop pop 255 get}
{pop 3 copy pop le{pop pop pop pop 0 get}{exch dup 4 -1 roll exch sub 3 1 roll sub div 255 mul dup floor dup 3 1 roll sub exch cvi dup 1 add 4 -1 roll exch get 4 -1 roll 3 -1 roll get dup 4 1 roll sub mul add}
ifelse}ifelse}bind
{{0.0000 0.0003 0.0006 0.0009 0.0012 0.0015 0.0018 0.0021 0.0024 0.0027 0.0030 0.0034 0.0037 0.0040 0.0044 0.0048 
0.0052 0.0056 0.0060 0.0065 0.0070 0.0075 0.0080 0.0086 0.0091 0.0097 0.0103 0.0110 0.0116 0.0123 0.0130 0.0137 
0.0144 0.0152 0.0160 0.0168 0.0176 0.0185 0.0194 0.0203 0.0212 0.0222 0.0232 0.0242 0.0252 0.0262 0.0273 0.0284 
0.0296 0.0307 0.0319 0.0331 0.0343 0.0356 0.0369 0.0382 0.0395 0.0409 0.0423 0.0437 0.0452 0.0467 0.0482 0.0497 
0.0513 0.0529 0.0545 0.0561 0.0578 0.0595 0.0612 0.0630 0.0648 0.0666 0.0685 0.0704 0.0723 0.0742 0.0762 0.0782 
0.0802 0.0823 0.0844 0.0865 0.0886 0.0908 0.0931 0.0953 0.0976 0.0999 0.1022 0.1046 0.1070 0.1095 0.1119 0.1144 
0.1170 0.1195 0.1221 0.1248 0.1274 0.1301 0.1329 0.1356 0.1384 0.1413 0.1441 0.1470 0.1500 0.1529 0.1559 0.1590 
0.1620 0.1651 0.1683 0.1714 0.1746 0.1779 0.1812 0.1845 0.1878 0.1912 0.1946 0.1981 0.2016 0.2051 0.2086 0.2122 
0.2159 0.2195 0.2232 0.2270 0.2307 0.2346 0.2384 0.2423 0.2462 0.2502 0.2542 0.2582 0.2622 0.2664 0.2705 0.2747 
0.2789 0.2832 0.2874 0.2918 0.2961 0.3005 0.3050 0.3095 0.3140 0.3185 0.3231 0.3278 0.3325 0.3372 0.3419 0.3467 
0.3515 0.3564 0.3613 0.3663 0.3712 0.3763 0.3813 0.3864 0.3916 0.3967 0.4020 0.4072 0.4125 0.4179 0.4233 0.4287 
0.4342 0.4397 0.4452 0.4508 0.4564 0.4621 0.4678 0.4735 0.4793 0.4851 0.4910 0.4969 0.5029 0.5089 0.5149 0.5210 
0.5271 0.5333 0.5395 0.5457 0.5520 0.5583 0.5647 0.5711 0.5776 0.5841 0.5906 0.5972 0.6038 0.6105 0.6172 0.6240 
0.6308 0.6376 0.6445 0.6514 0.6584 0.6654 0.6724 0.6795 0.6867 0.6939 0.7011 0.7084 0.7157 0.7231 0.7305 0.7379 
0.7454 0.7529 0.7605 0.7682 0.7758 0.7835 0.7913 0.7991 0.8069 0.8148 0.8228 0.8308 0.8388 0.8469 0.8550 0.8632 
0.8714 0.8796 0.8879 0.8963 0.9047 0.9131 0.9216 0.9301 0.9387 0.9473 0.9560 0.9647 0.9734 0.9822 0.9911 1.0000 }
dup 3 -1 roll 0.0000 1.0000 3 copy 3 -1 roll exch ge
{pop pop pop pop pop 255 get}
{pop 3 copy pop le{pop pop pop pop 0 get}{exch dup 4 -1 roll exch sub 3 1 roll sub div 255 mul dup floor dup 3 1 roll sub exch cvi dup 1 add 4 -1 roll exch get 4 -1 roll 3 -1 roll get dup 4 1 roll sub mul add}
ifelse}ifelse}bind
{{0.0000 0.0003 0.0006 0.0009 0.0012 0.0015 0.0018 0.0021 0.0024 0.0027 0.0030 0.0034 0.0037 0.0040 0.0044 0.0048 
0.0052 0.0056 0.0060 0.0065 0.0070 0.0075 0.0080 0.0086 0.0091 0.0097 0.0103 0.0110 0.0116 0.0123 0.0130 0.0137 
0.0144 0.0152 0.0160 0.0168 0.0176 0.0185 0.0194 0.0203 0.0212 0.0222 0.0232 0.0242 0.0252 0.0262 0.0273 0.0284 
0.0296 0.0307 0.0319 0.0331 0.0343 0.0356 0.0369 0.0382 0.0395 0.0409 0.0423 0.0437 0.0452 0.0467 0.0482 0.0497 
0.0513 0.0529 0.0545 0.0561 0.0578 0.0595 0.0612 0.0630 0.0648 0.0666 0.0685 0.0704 0.0723 0.0742 0.0762 0.0782 
0.0802 0.0823 0.0844 0.0865 0.0886 0.0908 0.0931 0.0953 0.0976 0.0999 0.1022 0.1046 0.1070 0.1095 0.1119 0.1144 
0.1170 0.1195 0.1221 0.1248 0.1274 0.1301 0.1329 0.1356 0.1384 0.1413 0.1441 0.1470 0.1500 0.1529 0.1559 0.1590 
0.1620 0.1651 0.1683 0.1714 0.1746 0.1779 0.1812 0.1845 0.1878 0.1912 0.1946 0.1981 0.2016 0.2051 0.2086 0.2122 
0.2159 0.2195 0.2232 0.2270 0.2307 0.2346 0.2384 0.2423 0.2462 0.2502 0.2542 0.2582 0.2622 0.2664 0.2705 0.2747 
0.2789 0.2832 0.2874 0.2918 0.2961 0.3005 0.3050 0.3095 0.3140 0.3185 0.3231 0.3278 0.3325 0.3372 0.3419 0.3467 
0.3515 0.3564 0.3613 0.3663 0.3712 0.3763 0.3813 0.3864 0.3916 0.3967 0.4020 0.4072 0.4125 0.4179 0.4233 0.4287 
0.4342 0.4397 0.4452 0.4508 0.4564 0.4621 0.4678 0.4735 0.4793 0.4851 0.4910 0.4969 0.5029 0.5089 0.5149 0.5210 
0.5271 0.5333 0.5395 0.5457 0.5520 0.5583 0.5647 0.5711 0.5776 0.5841 0.5906 0.5972 0.6038 0.6105 0.6172 0.6240 
0.6308 0.6376 0.6445 0.6514 0.6584 0.6654 0.6724 0.6795 0.6867 0.6939 0.7011 0.7084 0.7157 0.7231 0.7305 0.7379 
0.7454 0.7529 0.7605 0.7682 0.7758 0.7835 0.7913 0.7991 0.8069 0.8148 0.8228 0.8308 0.8388 0.8469 0.8550 0.8632 
0.8714 0.8796 0.8879 0.8963 0.9047 0.9131 0.9216 0.9301 0.9387 0.9473 0.9560 0.9647 0.9734 0.9822 0.9911 1.0000 }
dup 3 -1 roll 0.0000 1.0000 3 copy 3 -1 roll exch ge
{pop pop pop pop pop 255 get}
{pop 3 copy pop le{pop pop pop pop 0 get}{exch dup 4 -1 roll exch sub 3 1 roll sub div 255 mul dup floor dup 3 1 roll sub exch cvi dup 1 add 4 -1 roll exch get 4 -1 roll 3 -1 roll get dup 4 1 roll sub mul add}
ifelse}ifelse}bind] put
dup /MatrixLMN [0.4361 0.2225 0.0139 0.3851 0.7169 0.0971 0.1431 0.0606 0.7141] put
dup /WhitePoint [0.9642 1.0000 0.8249] put]
/E2 exch /ColorSpace defineRes

cs 0 0 0 sc
f
n
222.42 416.64 m
221.58 416.64 l
221.58 417.36 l
221.76 418.2 l
222.6 418.2 l
222.6 417.36 l
f
n
223.14 419.76 m
222.42 419.76 l
222.42 420.6 l
222.6 421.44 l
223.38 421.44 l
223.38 420.6 l
f
n
223.98 423 m
223.14 423 l
223.14 423.84 l
223.38 424.56 l
224.16 424.56 l
224.16 423.84 l
f
n
224.82 426 m
223.98 426 l
223.98 426.78 l
224.16 427.62 l
225 427.62 l
225 426.78 l
f
n
225.54 429.18 m
224.82 429.18 l
224.82 430.02 l
225 430.8 l
225.78 430.8 l
225.78 430.02 l
f
n
226.2 432.18 m
225.36 432.18 l
225.36 433.02 l
225.54 433.8 l
226.38 433.8 l
226.38 433.02 l
f
n
226.74 435.24 m
226.02 435.24 l
226.02 435.96 l
226.2 436.8 l
226.98 436.8 l
226.98 435.96 l
f
n
226.56 440.04 0.839996 -1.67999 re
f
n
226.74 443.16 0.839996 -1.56 re
f
n
226.98 446.4 0.779999 -1.62 re
f
n
227.94 448.02 m
227.22 448.02 l
227.22 448.8 l
227.4 449.58 l
228.18 449.58 l
228.18 448.8 l
f
n
228.42 451.2 m
227.58 451.2 l
227.58 451.98 l
227.76 452.82 l
228.6 452.82 l
228.6 451.98 l
f
n
228.78 454.38 m
227.94 454.38 l
227.94 455.22 l
228.18 456 l
228.96 456 l
228.96 455.22 l
f
n
229.14 457.62 m
228.42 457.62 l
228.42 458.4 l
228.6 459.18 l
229.38 459.18 l
229.38 458.4 l
f
n
229.62 460.8 m
228.78 460.8 l
228.78 461.58 l
228.96 462.42 l
229.8 462.42 l
229.8 461.58 l
f
n
229.14 465.6 0.839996 -1.62 re
f
n
229.38 468.78 0.779999 -1.56 re
f
n
229.62 471.96 0.720001 -1.56 re
f
n
230.58 473.82 m
229.8 473.82 l
229.8 474.6 l
229.98 475.38 l
230.82 475.38 l
230.82 474.6 l
f
n
231 477 m
230.16 477 l
230.16 477.78 l
230.34 478.62 l
231.18 478.62 l
231.18 477.78 l
f
n
231.36 480.36 m
230.58 480.36 l
230.58 481.2 l
230.82 481.98 l
231.54 481.98 l
231.54 481.2 l
f
n
231.78 483.78 m
231 483.78 l
231 484.62 l
231.18 485.4 l
232.02 485.4 l
232.02 484.62 l
f
n
231.36 488.4 0.839996 -1.62 re
f
n
231.54 491.22 0.839996 -1.62 re
f
n
231.78 494.4 0.779999 -1.62 re
f
n
232.74 496.02 m
232.02 496.02 l
232.02 496.8 l
232.2 497.58 l
232.98 497.58 l
232.98 496.8 l
f
n
233.22 499.2 m
232.38 499.2 l
232.38 499.98 l
232.56 500.82 l
233.4 500.82 l
233.4 499.98 l
f
n
233.58 502.38 m
232.74 502.38 l
232.74 503.22 l
232.98 504 l
233.76 504 l
233.76 503.22 l
f
n
233.94 505.56 m
233.22 505.56 l
233.22 506.4 l
233.4 507.24 l
234.18 507.24 l
234.18 506.4 l
f
n
234.42 508.8 m
233.58 508.8 l
233.58 509.64 l
233.76 510.36 l
234.6 510.36 l
234.6 509.64 l
f
n
234.78 512.04 m
233.94 512.04 l
233.94 512.76 l
234.18 513.6 l
234.96 513.6 l
234.96 512.76 l
f
n
234.42 516.78 0.779999 -1.62 re
f
n
235.38 518.4 m
234.6 518.4 l
234.6 519.18 l
234.78 520.02 l
235.62 520.02 l
235.62 519.18 l
f
n
235.8 521.58 m
234.96 521.58 l
234.96 522.42 l
235.2 523.2 l
235.98 523.2 l
235.98 522.42 l
f
n
236.16 525 m
235.38 525 l
235.38 525.84 l
235.62 526.56 l
236.4 526.56 l
236.4 525.84 l
f
n
236.58 528.42 m
235.8 528.42 l
235.8 529.2 l
235.98 529.98 l
236.82 529.98 l
236.82 529.2 l
f
n
237.6 530.58 1.62 -0.779968 re
f
n
240.78 529.62 m
240.78 530.4 l
241.62 530.4 l
241.8 529.62 l
241.8 528.78 l
240.96 528.78 l
f
n
241.2 526.56 m
241.2 527.4 l
241.98 527.4 l
242.16 526.56 l
242.16 525.84 l
241.38 525.84 l
f
n
241.62 523.62 m
241.62 524.4 l
242.4 524.4 l
242.58 523.62 l
242.58 522.78 l
241.8 522.78 l
f
n
242.16 520.38 m
242.16 521.22 l
243 521.22 l
243.18 520.38 l
243.18 519.6 l
242.4 519.6 l
f
n
242.82 517.2 m
242.82 517.98 l
243.6 517.98 l
243.78 517.2 l
243.78 516.42 l
243 516.42 l
f
n
243.36 513.96 m
243.36 514.8 l
244.2 514.8 l
244.38 513.96 l
244.38 513.18 l
243.6 513.18 l
f
n
243.78 510.84 m
243.78 511.56 l
244.56 511.56 l
244.8 510.84 l
244.8 510 l
244.02 510 l
f
n
244.2 507.6 m
244.2 508.44 l
244.98 508.44 l
245.22 507.6 l
245.22 506.76 l
244.38 506.76 l
f
n
244.56 504.36 m
244.56 505.2 l
245.4 505.2 l
245.58 504.36 l
245.58 503.58 l
244.8 503.58 l
f
n
244.98 501.18 m
244.98 502.02 l
245.76 502.02 l
246 501.18 l
246 500.4 l
245.22 500.4 l
f
n
245.4 498 m
245.4 498.78 l
246.18 498.78 l
246.42 498 l
246.42 497.22 l
245.58 497.22 l
f
n
245.76 494.82 m
245.76 495.6 l
246.6 495.6 l
246.78 494.82 l
246.78 493.98 l
246 493.98 l
f
n
246.42 491.58 m
246.42 492.42 l
247.2 492.42 l
247.38 491.58 l
247.38 490.8 l
246.6 490.8 l
f
n
246.78 488.4 m
246.78 489.18 l
247.62 489.18 l
247.8 488.4 l
247.8 487.62 l
246.96 487.62 l
f
n
247.2 485.22 m
247.2 486 l
247.98 486 l
248.16 485.22 l
248.16 484.38 l
247.38 484.38 l
f
n
247.62 481.98 m
247.62 482.82 l
248.4 482.82 l
248.58 481.98 l
248.58 481.2 l
247.8 481.2 l
f
n
247.98 478.8 m
247.98 479.58 l
248.76 479.58 l
249 478.8 l
249 477.96 l
248.16 477.96 l
f
n
248.4 475.56 m
248.4 476.4 l
249.18 476.4 l
249.36 475.56 l
249.36 474.84 l
248.58 474.84 l
f
n
248.76 472.44 m
248.76 473.16 l
249.6 473.16 l
249.78 472.44 l
249.78 471.6 l
249 471.6 l
f
n
249.36 470.04 0.839996 -1.62 re
f
n
249.78 466.8 0.779999 -1.62 re
f
n
250.2 463.38 0.779999 -1.62 re
f
n
250.56 459.36 m
250.56 460.2 l
251.4 460.2 l
251.58 459.36 l
251.58 458.64 l
250.8 458.64 l
f
n
251.16 456.24 m
251.16 456.96 l
252 456.96 l
252.18 456.24 l
252.18 455.4 l
251.4 455.4 l
f
n
251.76 453 m
251.76 453.84 l
252.6 453.84 l
252.78 453 l
252.78 452.16 l
252 452.16 l
f
n
252.6 449.82 m
252.6 450.6 l
253.38 450.6 l
253.56 449.82 l
253.56 448.98 l
252.78 448.98 l
f
n
253.2 446.82 m
253.2 447.6 l
253.98 447.6 l
254.16 446.82 l
254.16 445.98 l
253.38 445.98 l
f
n
253.8 443.58 m
253.8 444.36 l
254.58 444.36 l
254.76 443.58 l
254.76 442.8 l
253.98 442.8 l
f
n
254.58 440.4 m
254.58 441.24 l
255.36 441.24 l
255.6 440.4 l
255.6 439.56 l
254.76 439.56 l
f
n
255.18 436.98 m
255.18 437.82 l
255.96 437.82 l
256.38 436.98 l
256.38 436.2 l
255.6 436.2 l
f
n
256.38 433.8 m
256.38 434.58 l
257.16 434.58 l
257.58 433.8 l
257.58 433.02 l
256.8 433.02 l
f
n
257.58 430.62 m
257.58 431.4 l
258.36 431.4 l
258.78 430.62 l
258.78 429.78 l
258 429.78 l
f
n
258.78 427.38 m
258.78 428.22 l
259.56 428.22 l
259.98 427.38 l
259.98 426.6 l
259.2 426.6 l
f
n
259.98 424.2 m
259.98 425.04 l
260.76 425.04 l
261.42 424.2 l
261.42 423.36 l
260.58 423.36 l
f
n
262.38 421.2 m
262.38 421.98 l
263.16 421.98 l
264 420.96 l
264 420.24 l
263.16 420.24 l
f
n
265.56 418.02 m
265.56 418.8 l
266.4 418.8 l
267.18 418.38 l
267.18 417.6 l
266.4 417.6 l
f
n
268.8 416.64 m
268.8 417.36 l
269.58 417.36 l
270.36 417.18 l
270.36 416.4 l
269.58 416.4 l
f
n
271.98 416.82 1.62 -0.839996 re
f
n
276 415.8 m
275.16 415.8 l
275.16 416.64 l
279.18 417.84 l
279.96 417.84 l
279.96 417 l
f
n
279.96 417 m
279.18 417 l
279.18 417.84 l
283.98 449.82 l
284.76 449.82 l
284.76 448.98 l
f
n
284.76 448.98 m
283.98 448.98 l
283.98 449.82 l
288.78 550.98 l
289.56 550.98 l
289.56 550.2 l
f
n
289.56 550.2 m
288.78 550.2 l
288.78 550.98 l
293.58 641.22 l
294.36 641.22 l
294.36 640.38 l
f
n
293.58 640.38 m
293.58 641.22 l
294.36 641.22 l
299.16 640.8 l
299.16 640.02 l
298.38 640.02 l
f
n
298.38 640.02 m
298.38 640.8 l
299.16 640.8 l
303.96 575.82 l
303.96 574.98 l
303.18 574.98 l
f
n
303.18 574.98 m
303.18 575.82 l
303.96 575.82 l
308.76 505.2 l
308.76 504.36 l
307.98 504.36 l
f
n
307.98 504.36 m
307.98 505.2 l
308.76 505.2 l
313.56 457.8 l
313.56 456.96 l
312.78 456.96 l
f
n
312.78 456.96 m
312.78 457.8 l
313.56 457.8 l
318.42 433.2 l
318.42 432.42 l
317.58 432.42 l
f
n
317.58 432.42 m
317.58 433.2 l
318.42 433.2 l
323.22 422.64 l
323.22 421.8 l
322.38 421.8 l
f
n
322.38 421.8 m
322.38 422.64 l
323.22 422.64 l
328.02 418.38 l
328.02 417.6 l
327.18 417.6 l
f
n
327.18 417.6 m
327.18 418.38 l
328.02 418.38 l
332.82 417 l
332.82 416.22 l
331.98 416.22 l
f
n
331.98 416.22 m
331.98 417 l
332.82 417 l
337.56 416.64 l
337.56 415.8 l
336.78 415.8 l
f
n
275.82 415.8 m
274.98 415.8 l
274.98 416.64 l
279.18 418.02 l
279.96 418.02 l
279.96 417.18 l
f
n
279.96 417.18 m
279.18 417.18 l
279.18 418.02 l
283.98 451.02 l
284.76 451.02 l
284.76 450.18 l
f
n
284.76 450.18 m
283.98 450.18 l
283.98 451.02 l
288.78 553.8 l
289.56 553.8 l
289.56 553.02 l
f
n
289.56 553.02 m
288.78 553.02 l
288.78 553.8 l
293.58 643.02 l
294.36 643.02 l
294.36 642.18 l
f
n
293.58 642.18 m
293.58 643.02 l
294.36 643.02 l
299.16 639.6 l
299.16 638.82 l
298.38 638.82 l
f
n
298.38 638.82 m
298.38 639.6 l
299.16 639.6 l
303.96 573.18 l
303.96 572.4 l
303.18 572.4 l
f
n
303.18 572.4 m
303.18 573.18 l
303.96 573.18 l
308.76 503.58 l
308.76 502.8 l
307.98 502.8 l
f
n
307.98 502.8 m
307.98 503.58 l
308.76 503.58 l
313.56 457.2 l
313.56 456.42 l
312.78 456.42 l
f
n
312.78 456.42 m
312.78 457.2 l
313.56 457.2 l
318.42 433.02 l
318.42 432.18 l
317.58 432.18 l
f
n
317.58 432.18 m
317.58 433.02 l
318.42 433.02 l
323.22 422.64 l
323.22 421.8 l
322.38 421.8 l
f
n
322.38 421.8 m
322.38 422.64 l
323.22 422.64 l
328.02 418.38 l
328.02 417.6 l
327.18 417.6 l
f
n
327.18 417.6 m
327.18 418.38 l
328.02 418.38 l
332.82 417 l
332.82 416.22 l
331.98 416.22 l
f
n
331.98 416.22 m
331.98 417 l
332.82 417 l
337.56 416.64 l
337.56 415.8 l
336.78 415.8 l
f
n
218.4 415.8 m
217.62 415.8 l
217.62 416.64 l
221.58 417.84 l
222.42 417.84 l
222.42 417 l
f
n
222.42 417 m
221.58 417 l
221.58 417.84 l
226.38 451.8 l
227.22 451.8 l
227.22 451.02 l
f
n
227.22 451.02 m
226.38 451.02 l
226.38 451.8 l
231.18 556.2 l
232.02 556.2 l
232.02 555.42 l
f
n
232.02 555.42 m
231.18 555.42 l
231.18 556.2 l
235.98 645.42 l
236.82 645.42 l
236.82 644.58 l
f
n
235.98 644.58 m
235.98 645.42 l
236.82 645.42 l
241.62 638.82 l
241.62 637.98 l
240.78 637.98 l
f
n
240.78 637.98 m
240.78 638.82 l
241.62 638.82 l
246.42 571.8 l
246.42 571.02 l
245.58 571.02 l
f
n
245.58 571.02 m
245.58 571.8 l
246.42 571.8 l
251.16 502.2 l
251.16 501.42 l
250.38 501.42 l
f
n
250.38 501.42 m
250.38 502.2 l
251.16 502.2 l
255.96 456.24 l
255.96 455.4 l
255.18 455.4 l
f
n
255.18 455.4 m
255.18 456.24 l
255.96 456.24 l
260.76 432.6 l
260.76 431.82 l
259.98 431.82 l
f
n
259.98 431.82 m
259.98 432.6 l
260.76 432.6 l
265.56 422.16 l
265.56 421.44 l
264.78 421.44 l
f
n
264.78 421.44 m
264.78 422.16 l
265.56 422.16 l
270.36 418.38 l
270.36 417.6 l
269.58 417.6 l
f
n
269.58 417.6 m
269.58 418.38 l
270.36 418.38 l
275.16 417 l
275.16 416.22 l
274.38 416.22 l
f
n
274.38 416.22 m
274.38 417 l
275.16 417 l
279.96 416.64 l
279.96 415.8 l
279.18 415.8 l
f
n
218.16 415.8 m
217.38 415.8 l
217.38 416.64 l
221.58 418.02 l
222.42 418.02 l
222.42 417.18 l
f
n
222.42 417.18 m
221.58 417.18 l
221.58 418.02 l
226.38 451.8 l
227.22 451.8 l
227.22 451.02 l
f
n
227.22 451.02 m
226.38 451.02 l
226.38 451.8 l
231.18 556.2 l
232.02 556.2 l
232.02 555.42 l
f
n
232.02 555.42 m
231.18 555.42 l
231.18 556.2 l
235.98 646.2 l
236.82 646.2 l
236.82 645.42 l
f
n
235.98 645.42 m
235.98 646.2 l
236.82 646.2 l
241.62 639.78 l
241.62 639 l
240.78 639 l
f
n
240.78 639 m
240.78 639.78 l
241.62 639.78 l
246.42 571.62 l
246.42 570.78 l
245.58 570.78 l
f
n
245.58 570.78 m
245.58 571.62 l
246.42 571.62 l
251.16 501.42 l
251.16 500.58 l
250.38 500.58 l
f
n
250.38 500.58 m
250.38 501.42 l
251.16 501.42 l
255.96 455.76 l
255.96 455.04 l
255.18 455.04 l
f
n
255.18 455.04 m
255.18 455.76 l
255.96 455.76 l
260.76 432.42 l
260.76 431.58 l
259.98 431.58 l
f
n
259.98 431.58 m
259.98 432.42 l
260.76 432.42 l
265.56 422.16 l
265.56 421.44 l
264.78 421.44 l
f
n
264.78 421.44 m
264.78 422.16 l
265.56 422.16 l
270.36 418.38 l
270.36 417.6 l
269.58 417.6 l
f
n
269.58 417.6 m
269.58 418.38 l
270.36 418.38 l
275.16 417 l
275.16 416.22 l
274.38 416.22 l
f
n
274.38 416.22 m
274.38 417 l
275.16 417 l
279.96 416.64 l
279.96 415.8 l
279.18 415.8 l
f
1 J
1 j
0.190994 w
10 M
[] 0 d
n
176.4 415.98 m
181.38 415.98 l
176.4 462.6 m
181.38 462.6 l
176.4 509.4 m
181.38 509.4 l
176.4 556.2 m
181.38 556.2 l
176.4 602.82 m
181.38 602.82 l
176.4 649.56 m
181.38 649.56 l
176.4 425.4 m
178.98 425.4 l
176.4 434.58 m
178.98 434.58 l
176.4 444 m
178.98 444 l
176.4 453.36 m
178.98 453.36 l
176.4 471.96 m
178.98 471.96 l
176.4 481.38 m
178.98 481.38 l
176.4 490.56 m
178.98 490.56 l
176.4 499.98 m
178.98 499.98 l
176.4 518.82 m
178.98 518.82 l
176.4 528 m
178.98 528 l
176.4 537.42 m
178.98 537.42 l
176.4 546.84 m
178.98 546.84 l
176.4 565.38 m
178.98 565.38 l
176.4 574.8 m
178.98 574.8 l
176.4 584.22 m
178.98 584.22 l
176.4 593.58 m
178.98 593.58 l
176.4 612.18 m
178.98 612.18 l
176.4 621.6 m
178.98 621.6 l
176.4 630.96 m
178.98 630.96 l
176.4 640.2 m
178.98 640.2 l
464.4 415.98 m
459.36 415.98 l
464.4 462.6 m
459.36 462.6 l
464.4 509.4 m
459.36 509.4 l
464.4 556.2 m
459.36 556.2 l
464.4 602.82 m
459.36 602.82 l
464.4 649.56 m
459.36 649.56 l
464.4 425.4 m
461.76 425.4 l
464.4 434.58 m
461.76 434.58 l
464.4 444 m
461.76 444 l
464.4 453.36 m
461.76 453.36 l
464.4 471.96 m
461.76 471.96 l
464.4 481.38 m
461.76 481.38 l
464.4 490.56 m
461.76 490.56 l
464.4 499.98 m
461.76 499.98 l
464.4 518.82 m
461.76 518.82 l
464.4 528 m
461.76 528 l
464.4 537.42 m
461.76 537.42 l
464.4 546.84 m
461.76 546.84 l
464.4 565.38 m
461.76 565.38 l
464.4 574.8 m
461.76 574.8 l
464.4 584.22 m
461.76 584.22 l
464.4 593.58 m
461.76 593.58 l
464.4 612.18 m
461.76 612.18 l
464.4 621.6 m
461.76 621.6 l
464.4 630.96 m
461.76 630.96 l
464.4 640.2 m
461.76 640.2 l
176.4 415.98 m
176.4 420.96 l
224.34 415.98 m
224.34 420.96 l
272.4 415.98 m
272.4 420.96 l
320.34 415.98 m
320.34 420.96 l
368.4 415.98 m
368.4 420.96 l
416.34 415.98 m
416.34 420.96 l
464.4 415.98 m
464.4 420.96 l
188.4 415.98 m
188.4 418.56 l
200.4 415.98 m
200.4 418.56 l
212.4 415.98 m
212.4 418.56 l
236.4 415.98 m
236.4 418.56 l
248.4 415.98 m
248.4 418.38 l
0 0 0.830994 sc
S
n
248.4 418.38 m
248.4 418.56 l
260.4 415.98 m
260.4 418.56 l
284.4 415.98 m
284.4 418.56 l
296.4 415.98 m
296.4 418.56 l
308.34 415.98 m
308.34 418.56 l
332.34 415.98 m
332.34 418.56 l
344.4 415.98 m
344.4 418.56 l
356.4 415.98 m
356.4 418.56 l
380.4 415.98 m
380.4 418.56 l
392.4 415.98 m
392.4 418.56 l
404.34 415.98 m
404.34 418.56 l
428.34 415.98 m
428.34 418.56 l
440.34 415.98 m
440.34 418.56 l
452.4 415.98 m
452.4 418.56 l
176.4 649.56 m
176.4 644.58 l
224.34 649.56 m
224.34 644.58 l
272.4 649.56 m
272.4 644.58 l
320.34 649.56 m
320.34 644.58 l
368.4 649.56 m
368.4 644.58 l
416.34 649.56 m
416.34 644.58 l
464.4 649.56 m
464.4 644.58 l
188.4 649.56 m
188.4 646.98 l
200.4 649.56 m
200.4 646.98 l
212.4 649.56 m
212.4 646.98 l
236.4 649.56 m
236.4 646.98 l
248.4 649.56 m
248.4 646.98 l
260.4 649.56 m
260.4 646.98 l
284.4 649.56 m
284.4 646.98 l
296.4 649.56 m
296.4 646.98 l
308.34 649.56 m
308.34 646.98 l
332.34 649.56 m
332.34 646.98 l
344.4 649.56 m
344.4 646.98 l
356.4 649.56 m
356.4 646.98 l
380.4 649.56 m
380.4 646.98 l
392.4 649.56 m
392.4 646.98 l
404.34 649.56 m
404.34 646.98 l
428.34 649.56 m
428.34 646.98 l
S
n
440.34 649.56 m
440.34 646.98 l
452.4 649.56 m
452.4 646.98 l
S
n
175.98 650.04 0.779999 -234.42 re
f
n
463.92 650.04 0.839996 -234.42 re
f
n
175.98 416.4 288.78 -0.779999 re
f
n
175.98 650.04 288.78 -0.840027 re
f
0 0 0 sc
163.56 412.38 m
/N292 9.58659 Tf
(0) show
150 459.18 m
(0.05)
[5.39816 2.58162 5.39816 5.39816 ] pdfxs
155.58 505.8 m
(0.1)
[5.39816 2.58162 5.39816 ] pdfxs
150 552.599 m
(0.15)
[5.39816 2.58162 5.39816 5.39816 ] pdfxs
155.58 599.219 m
(0.2)
[5.39816 2.58162 5.39816 ] pdfxs
150 645.959 m
(0.25)
[5.39816 2.58162 5.39816 5.39816 ] pdfxs
166.379 401.639 m
(-100-80-60-40-20020)
[3.17983 5.45863 5.15857 37.0187 3.17983 5.39824 39.4182 3.17983 5.39824 39.3587 3.24023 
5.39824 39.4182 3.11943 5.45863 43.7983 45.1788 5.39824 5.31771 ] pdfxs
313.139 616.799 m
(elongated)
[5.45858 2.58164 5.82184 6.00111 5.76144 5.39818 3.24017 5.15852 5.98577 ] pdfxs
313.139 605.399 m
(chain)
[5.45858 5.82184 5.33875 2.58164 5.98577 ] pdfxs
n
306 574.44 m
308.34 583.38 l
309.18 579 l
313.56 579.78 l
306 574.44 l
eofill
n
309.18 579 m
323.58 600 l
323.76 600 l
S
247.62 614.4 m
(compact )
[5.3474 5.8746 8.63841 5.76148 5.39821 5.15855 3.20953 2.68233 ] pdfxs
247.62 603 m
(chain)
[5.31669 5.84388 5.39817 2.58163 5.84388 ] pdfxs
n
247.62 572.82 m
250.2 581.82 l
250.8 577.2 l
255.36 577.8 l
247.62 572.82 l
eofill
n
250.8 577.2 m
264.36 595.2 l
264.54 595.2 l
S
144.42 517.2 m
/N292 [0 11.2165 -11.2165 0 0 0] Tf
(P\(E\)/)
[7.38034 3.77985 7.38034 3.77985 3.01721 ] pdfys
0 J
0 j
0.119995 w
144.42 542.76 m
Adobe_CoolType_Utility begin ct_MakeOCF begin ct_GlyphDirProcs begin
/EKJCFC+SymbolMT 1
GetGlyphDirectory
74 <10bf317079c888c222c2de9c82f6b7e5dabdca8fed4ee12bd9009bde50a7
584db72d7a386fa8686633af0e5fe2c4f30bf6789f4ed05a3f8412f68f52
9c6c193cdaa0fae2431ad8749eaf5a0b366352b0ccc9c2d49a1fae2fd5b9
f2a62e7467de384f396cc5923063895fb8f69bf8d09bc403594118890783
5ee334a7cb870cbf9055d74d56c0e01a19fbedb955ca7cda12a8ddd444b1
92a112de2e9a8da3a2a9b3539508f2b78d92bcf749e08f3e04d05688b1cd
140336c8b7a5918c20> |
!
end end end
/N287 [0 11.2165 -11.2165 0 0 0] Tf
(\000J) show
n
144.42 542.76 m
(\000J) pdf_strokepath
316.74 388.02 m
/N292 11.2165 Tf
(E) show
89.9999 330.96 m
/N282 12 Tf
(F) show
(i)
[3.33838 ] pdfxs
(gur) show
(e)
[5.3302 ] pdfxs
( 6, Sh) show
(e)
[5.3302 ] pdfxs
(w ) show
(et)
[5.3302 3.33838 ] pdfxs
( ) show
(al)
[5.3302 3.33838 ] pdfxs
(. ) show
PDFVars/TermAll get exec end end
restore

%%EndDocument

LH
(%%[Page: 6]%%) = 
%%PageTrailer

%%Page: 7 7
%%PageBoundingBox: 12 13 598 780
%%EndPageComments
%%BeginPageSetup
/DeviceRGB dup setcolorspace /colspABC exch def
mysetup concat colspRefresh
%%EndPageSetup

%%BeginDocument: Pscript_Win_PassThrough
PDFVars begin PDF begin PDFVars/InitAll get exec
save
0 0 612 792 true PDF begin PDFVars begin AS end end
0 0 612 792 re
W
n
false setSA
{} settransfer
n
193.38 415.62 m
192.18 415.62 l
192.18 416.82 l
192.78 419.22 l
193.98 419.22 l
193.98 418.02 l
[/CIEBasedABC  9 dict 
dup /CreationDate (19980209064900) put
dup /RenderingIntent (RelativeColorimetric) put
dup /Description (sRGB IEC61966-2.1) put
dup /ColorSpace (RGB ) put
dup /Copyright (Copyright (c) 1998 Hewlett-Packard Company) put
dup /DecodeLMN [

{{0.0000 0.0003 0.0006 0.0009 0.0012 0.0015 0.0018 0.0021 0.0024 0.0027 0.0030 0.0034 0.0037 0.0040 0.0044 0.0048 
0.0052 0.0056 0.0060 0.0065 0.0070 0.0075 0.0080 0.0086 0.0091 0.0097 0.0103 0.0110 0.0116 0.0123 0.0130 0.0137 
0.0144 0.0152 0.0160 0.0168 0.0176 0.0185 0.0194 0.0203 0.0212 0.0222 0.0232 0.0242 0.0252 0.0262 0.0273 0.0284 
0.0296 0.0307 0.0319 0.0331 0.0343 0.0356 0.0369 0.0382 0.0395 0.0409 0.0423 0.0437 0.0452 0.0467 0.0482 0.0497 
0.0513 0.0529 0.0545 0.0561 0.0578 0.0595 0.0612 0.0630 0.0648 0.0666 0.0685 0.0704 0.0723 0.0742 0.0762 0.0782 
0.0802 0.0823 0.0844 0.0865 0.0886 0.0908 0.0931 0.0953 0.0976 0.0999 0.1022 0.1046 0.1070 0.1095 0.1119 0.1144 
0.1170 0.1195 0.1221 0.1248 0.1274 0.1301 0.1329 0.1356 0.1384 0.1413 0.1441 0.1470 0.1500 0.1529 0.1559 0.1590 
0.1620 0.1651 0.1683 0.1714 0.1746 0.1779 0.1812 0.1845 0.1878 0.1912 0.1946 0.1981 0.2016 0.2051 0.2086 0.2122 
0.2159 0.2195 0.2232 0.2270 0.2307 0.2346 0.2384 0.2423 0.2462 0.2502 0.2542 0.2582 0.2622 0.2664 0.2705 0.2747 
0.2789 0.2832 0.2874 0.2918 0.2961 0.3005 0.3050 0.3095 0.3140 0.3185 0.3231 0.3278 0.3325 0.3372 0.3419 0.3467 
0.3515 0.3564 0.3613 0.3663 0.3712 0.3763 0.3813 0.3864 0.3916 0.3967 0.4020 0.4072 0.4125 0.4179 0.4233 0.4287 
0.4342 0.4397 0.4452 0.4508 0.4564 0.4621 0.4678 0.4735 0.4793 0.4851 0.4910 0.4969 0.5029 0.5089 0.5149 0.5210 
0.5271 0.5333 0.5395 0.5457 0.5520 0.5583 0.5647 0.5711 0.5776 0.5841 0.5906 0.5972 0.6038 0.6105 0.6172 0.6240 
0.6308 0.6376 0.6445 0.6514 0.6584 0.6654 0.6724 0.6795 0.6867 0.6939 0.7011 0.7084 0.7157 0.7231 0.7305 0.7379 
0.7454 0.7529 0.7605 0.7682 0.7758 0.7835 0.7913 0.7991 0.8069 0.8148 0.8228 0.8308 0.8388 0.8469 0.8550 0.8632 
0.8714 0.8796 0.8879 0.8963 0.9047 0.9131 0.9216 0.9301 0.9387 0.9473 0.9560 0.9647 0.9734 0.9822 0.9911 1.0000 }
dup 3 -1 roll 0.0000 1.0000 3 copy 3 -1 roll exch ge
{pop pop pop pop pop 255 get}
{pop 3 copy pop le{pop pop pop pop 0 get}{exch dup 4 -1 roll exch sub 3 1 roll sub div 255 mul dup floor dup 3 1 roll sub exch cvi dup 1 add 4 -1 roll exch get 4 -1 roll 3 -1 roll get dup 4 1 roll sub mul add}
ifelse}ifelse}bind
{{0.0000 0.0003 0.0006 0.0009 0.0012 0.0015 0.0018 0.0021 0.0024 0.0027 0.0030 0.0034 0.0037 0.0040 0.0044 0.0048 
0.0052 0.0056 0.0060 0.0065 0.0070 0.0075 0.0080 0.0086 0.0091 0.0097 0.0103 0.0110 0.0116 0.0123 0.0130 0.0137 
0.0144 0.0152 0.0160 0.0168 0.0176 0.0185 0.0194 0.0203 0.0212 0.0222 0.0232 0.0242 0.0252 0.0262 0.0273 0.0284 
0.0296 0.0307 0.0319 0.0331 0.0343 0.0356 0.0369 0.0382 0.0395 0.0409 0.0423 0.0437 0.0452 0.0467 0.0482 0.0497 
0.0513 0.0529 0.0545 0.0561 0.0578 0.0595 0.0612 0.0630 0.0648 0.0666 0.0685 0.0704 0.0723 0.0742 0.0762 0.0782 
0.0802 0.0823 0.0844 0.0865 0.0886 0.0908 0.0931 0.0953 0.0976 0.0999 0.1022 0.1046 0.1070 0.1095 0.1119 0.1144 
0.1170 0.1195 0.1221 0.1248 0.1274 0.1301 0.1329 0.1356 0.1384 0.1413 0.1441 0.1470 0.1500 0.1529 0.1559 0.1590 
0.1620 0.1651 0.1683 0.1714 0.1746 0.1779 0.1812 0.1845 0.1878 0.1912 0.1946 0.1981 0.2016 0.2051 0.2086 0.2122 
0.2159 0.2195 0.2232 0.2270 0.2307 0.2346 0.2384 0.2423 0.2462 0.2502 0.2542 0.2582 0.2622 0.2664 0.2705 0.2747 
0.2789 0.2832 0.2874 0.2918 0.2961 0.3005 0.3050 0.3095 0.3140 0.3185 0.3231 0.3278 0.3325 0.3372 0.3419 0.3467 
0.3515 0.3564 0.3613 0.3663 0.3712 0.3763 0.3813 0.3864 0.3916 0.3967 0.4020 0.4072 0.4125 0.4179 0.4233 0.4287 
0.4342 0.4397 0.4452 0.4508 0.4564 0.4621 0.4678 0.4735 0.4793 0.4851 0.4910 0.4969 0.5029 0.5089 0.5149 0.5210 
0.5271 0.5333 0.5395 0.5457 0.5520 0.5583 0.5647 0.5711 0.5776 0.5841 0.5906 0.5972 0.6038 0.6105 0.6172 0.6240 
0.6308 0.6376 0.6445 0.6514 0.6584 0.6654 0.6724 0.6795 0.6867 0.6939 0.7011 0.7084 0.7157 0.7231 0.7305 0.7379 
0.7454 0.7529 0.7605 0.7682 0.7758 0.7835 0.7913 0.7991 0.8069 0.8148 0.8228 0.8308 0.8388 0.8469 0.8550 0.8632 
0.8714 0.8796 0.8879 0.8963 0.9047 0.9131 0.9216 0.9301 0.9387 0.9473 0.9560 0.9647 0.9734 0.9822 0.9911 1.0000 }
dup 3 -1 roll 0.0000 1.0000 3 copy 3 -1 roll exch ge
{pop pop pop pop pop 255 get}
{pop 3 copy pop le{pop pop pop pop 0 get}{exch dup 4 -1 roll exch sub 3 1 roll sub div 255 mul dup floor dup 3 1 roll sub exch cvi dup 1 add 4 -1 roll exch get 4 -1 roll 3 -1 roll get dup 4 1 roll sub mul add}
ifelse}ifelse}bind
{{0.0000 0.0003 0.0006 0.0009 0.0012 0.0015 0.0018 0.0021 0.0024 0.0027 0.0030 0.0034 0.0037 0.0040 0.0044 0.0048 
0.0052 0.0056 0.0060 0.0065 0.0070 0.0075 0.0080 0.0086 0.0091 0.0097 0.0103 0.0110 0.0116 0.0123 0.0130 0.0137 
0.0144 0.0152 0.0160 0.0168 0.0176 0.0185 0.0194 0.0203 0.0212 0.0222 0.0232 0.0242 0.0252 0.0262 0.0273 0.0284 
0.0296 0.0307 0.0319 0.0331 0.0343 0.0356 0.0369 0.0382 0.0395 0.0409 0.0423 0.0437 0.0452 0.0467 0.0482 0.0497 
0.0513 0.0529 0.0545 0.0561 0.0578 0.0595 0.0612 0.0630 0.0648 0.0666 0.0685 0.0704 0.0723 0.0742 0.0762 0.0782 
0.0802 0.0823 0.0844 0.0865 0.0886 0.0908 0.0931 0.0953 0.0976 0.0999 0.1022 0.1046 0.1070 0.1095 0.1119 0.1144 
0.1170 0.1195 0.1221 0.1248 0.1274 0.1301 0.1329 0.1356 0.1384 0.1413 0.1441 0.1470 0.1500 0.1529 0.1559 0.1590 
0.1620 0.1651 0.1683 0.1714 0.1746 0.1779 0.1812 0.1845 0.1878 0.1912 0.1946 0.1981 0.2016 0.2051 0.2086 0.2122 
0.2159 0.2195 0.2232 0.2270 0.2307 0.2346 0.2384 0.2423 0.2462 0.2502 0.2542 0.2582 0.2622 0.2664 0.2705 0.2747 
0.2789 0.2832 0.2874 0.2918 0.2961 0.3005 0.3050 0.3095 0.3140 0.3185 0.3231 0.3278 0.3325 0.3372 0.3419 0.3467 
0.3515 0.3564 0.3613 0.3663 0.3712 0.3763 0.3813 0.3864 0.3916 0.3967 0.4020 0.4072 0.4125 0.4179 0.4233 0.4287 
0.4342 0.4397 0.4452 0.4508 0.4564 0.4621 0.4678 0.4735 0.4793 0.4851 0.4910 0.4969 0.5029 0.5089 0.5149 0.5210 
0.5271 0.5333 0.5395 0.5457 0.5520 0.5583 0.5647 0.5711 0.5776 0.5841 0.5906 0.5972 0.6038 0.6105 0.6172 0.6240 
0.6308 0.6376 0.6445 0.6514 0.6584 0.6654 0.6724 0.6795 0.6867 0.6939 0.7011 0.7084 0.7157 0.7231 0.7305 0.7379 
0.7454 0.7529 0.7605 0.7682 0.7758 0.7835 0.7913 0.7991 0.8069 0.8148 0.8228 0.8308 0.8388 0.8469 0.8550 0.8632 
0.8714 0.8796 0.8879 0.8963 0.9047 0.9131 0.9216 0.9301 0.9387 0.9473 0.9560 0.9647 0.9734 0.9822 0.9911 1.0000 }
dup 3 -1 roll 0.0000 1.0000 3 copy 3 -1 roll exch ge
{pop pop pop pop pop 255 get}
{pop 3 copy pop le{pop pop pop pop 0 get}{exch dup 4 -1 roll exch sub 3 1 roll sub div 255 mul dup floor dup 3 1 roll sub exch cvi dup 1 add 4 -1 roll exch get 4 -1 roll 3 -1 roll get dup 4 1 roll sub mul add}
ifelse}ifelse}bind] put
dup /MatrixLMN [0.4361 0.2225 0.0139 0.3851 0.7169 0.0971 0.1431 0.0606 0.7141] put
dup /WhitePoint [0.9642 1.0000 0.8249] put]
/E3 exch /ColorSpace defineRes

cs 0 0 0 sc
f
n
195 421.98 m
193.8 421.98 l
193.8 423.18 l
194.4 425.58 l
195.6 425.58 l
195.6 424.38 l
f
n
196.8 428.4 m
195.6 428.4 l
195.6 429.6 l
196.2 432 l
197.4 432 l
197.4 430.8 l
f
n
198.36 434.76 m
197.16 434.76 l
197.16 435.96 l
197.82 438.36 l
199.02 438.36 l
199.02 437.16 l
f
n
200.4 441.24 m
199.2 441.24 l
199.2 442.44 l
200.22 444.78 l
201.42 444.78 l
201.42 443.58 l
f
n
202.98 447.6 m
201.78 447.6 l
201.78 448.8 l
202.8 451.2 l
204 451.2 l
204 450 l
f
n
205.38 454.02 m
204.18 454.02 l
204.18 455.22 l
205.2 457.62 l
206.4 457.62 l
206.4 456.42 l
f
n
207.78 460.38 m
206.58 460.38 l
206.58 461.58 l
207.6 463.98 l
208.8 463.98 l
208.8 462.78 l
f
n
210.18 466.8 m
208.98 466.8 l
208.98 468 l
210 470.76 l
211.2 470.76 l
211.2 469.56 l
f
n
213.36 473.64 m
212.16 473.64 l
212.16 474.84 l
213.6 477.24 l
214.8 477.24 l
214.8 476.04 l
f
n
216.96 479.82 m
215.76 479.82 l
215.76 481.02 l
216.96 483.42 l
218.16 483.42 l
218.16 482.22 l
f
n
220.38 486.18 m
219.18 486.18 l
219.18 487.44 l
220.56 489.84 l
221.76 489.84 l
221.76 488.64 l
f
n
223.98 492.42 m
222.78 492.42 l
222.78 493.62 l
224.34 496.02 l
225.54 496.02 l
225.54 494.82 l
f
n
228.42 499.02 m
227.22 499.02 l
227.22 500.22 l
228.78 502.62 l
229.98 502.62 l
229.98 501.42 l
f
n
232.74 505.56 m
231.54 505.56 l
231.54 506.76 l
233.4 509.16 l
234.6 509.16 l
234.6 507.96 l
f
n
237.6 511.8 m
236.4 511.8 l
236.4 513 l
238.2 515.4 l
239.4 515.4 l
239.4 514.2 l
f
n
242.4 517.98 m
241.2 517.98 l
241.2 519.18 l
243.36 522 l
244.56 522 l
244.56 520.8 l
f
n
248.4 524.82 m
247.2 524.82 l
247.2 526.02 l
249.6 528.42 l
250.8 528.42 l
250.8 527.22 l
f
n
254.58 531 m
253.38 531 l
253.38 532.2 l
255.6 534.42 l
256.8 534.42 l
256.8 533.22 l
f
n
260.76 536.58 m
259.56 536.58 l
259.56 537.78 l
261.96 539.64 l
263.16 539.64 l
263.16 538.38 l
f
n
266.94 541.56 m
265.74 541.56 l
265.74 542.76 l
267.96 544.62 l
269.16 544.62 l
269.16 543.42 l
f
n
269.16 543.42 m
267.96 543.42 l
267.96 544.62 l
268.8 545.16 l
270 545.16 l
270 543.96 l
f
n
273.78 547.02 m
272.58 547.02 l
272.58 548.22 l
274.8 549.96 l
276 549.96 l
276 548.76 l
f
n
279.78 551.58 m
278.58 551.58 l
278.58 552.78 l
279.42 553.38 l
280.62 553.38 l
280.62 552.18 l
f
n
280.62 552.18 m
279.42 552.18 l
279.42 553.38 l
280.98 554.4 l
282.18 554.4 l
282.18 553.2 l
f
n
286.38 556.02 m
285.18 556.02 l
285.18 557.22 l
287.58 558.78 l
288.78 558.78 l
288.78 557.58 l
f
n
292.56 559.98 m
291.42 559.98 l
291.42 561.18 l
294 562.8 l
295.2 562.8 l
295.2 561.6 l
f
n
299.4 564.24 m
298.2 564.24 l
298.2 565.38 l
300.78 566.82 l
301.98 566.82 l
301.98 565.62 l
f
n
306 567.78 m
304.8 567.78 l
304.8 568.98 l
307.14 570.18 l
308.34 570.18 l
308.34 568.98 l
f
n
312.18 571.02 m
310.98 571.02 l
310.98 572.22 l
313.14 573.42 l
314.34 573.42 l
314.34 572.22 l
f
n
318.18 574.2 m
316.98 574.2 l
316.98 575.4 l
319.62 576.84 l
320.82 576.84 l
320.82 575.64 l
f
n
324.96 577.8 m
323.76 577.8 l
323.76 579 l
325.62 579.96 l
326.82 579.96 l
326.82 578.76 l
f
n
326.82 578.76 m
325.62 578.76 l
325.62 579.96 l
326.34 580.44 l
327.54 580.44 l
327.54 579.24 l
f
n
331.38 581.16 m
330.18 581.16 l
330.18 582.36 l
332.34 583.56 l
333.54 583.56 l
333.54 582.36 l
f
n
337.38 584.22 m
336.18 584.22 l
336.18 585.42 l
336.96 585.78 l
338.16 585.78 l
338.16 584.58 l
f
n
338.16 584.58 m
336.96 584.58 l
336.96 585.78 l
338.58 586.62 l
339.78 586.62 l
339.78 585.42 l
f
n
343.8 587.4 m
342.6 587.4 l
342.6 588.6 l
345.18 589.8 l
346.38 589.8 l
346.38 588.6 l
f
n
350.58 590.82 m
349.38 590.82 l
349.38 592.02 l
351.78 593.22 l
352.98 593.22 l
352.98 592.02 l
f
n
357.18 593.76 m
355.98 593.76 l
355.98 594.96 l
358.38 595.98 l
359.58 595.98 l
359.58 594.78 l
f
n
363.36 596.64 m
362.16 596.64 l
362.16 597.84 l
364.32 598.8 l
365.52 598.8 l
365.52 597.6 l
f
n
369.42 599.22 m
368.16 599.22 l
368.16 600.42 l
370.8 601.62 l
372 601.62 l
372 600.42 l
f
n
376.14 601.98 m
374.94 601.98 l
374.94 603.18 l
377.34 604.2 l
378.54 604.2 l
378.54 603 l
f
n
382.8 604.38 m
381.6 604.38 l
381.6 605.58 l
383.16 606.18 l
384.36 606.18 l
384.36 604.98 l
f
n
384.36 604.98 m
383.16 604.98 l
383.16 606.18 l
384 606.42 l
385.2 606.42 l
385.2 605.22 l
f
n
388.98 606.6 m
387.78 606.6 l
387.78 607.8 l
390 608.58 l
391.2 608.58 l
391.2 607.38 l
f
n
394.98 608.82 m
393.78 608.82 l
393.78 609.96 l
394.56 610.2 l
395.76 610.2 l
395.76 609 l
f
n
395.76 609 m
394.56 609 l
394.56 610.2 l
396.18 610.8 l
397.38 610.8 l
397.38 609.6 l
f
n
401.58 611.16 m
400.38 611.16 l
400.38 612.36 l
402.78 613.2 l
403.98 613.2 l
403.98 612 l
f
n
408.12 613.38 m
406.92 613.38 l
406.92 614.58 l
409.32 615.42 l
410.52 615.42 l
410.52 614.22 l
f
n
414.78 615.78 m
413.58 615.78 l
413.58 616.98 l
415.98 617.82 l
417.18 617.82 l
417.18 616.62 l
f
n
420.6 617.82 m
419.4 617.82 l
419.4 619.02 l
421.8 619.8 l
423 619.8 l
423 618.6 l
f
n
427.14 619.8 m
425.94 619.8 l
425.94 621 l
428.34 621.78 l
429.54 621.78 l
429.54 620.58 l
f
n
433.8 621.78 m
432.6 621.78 l
432.6 622.98 l
435 623.58 l
436.14 623.58 l
436.14 622.38 l
f
n
440.34 623.58 m
439.14 623.58 l
439.14 624.78 l
440.76 625.2 l
441.96 625.2 l
441.96 624 l
f
n
441.96 624 m
440.76 624 l
440.76 625.2 l
441.54 625.38 l
442.74 625.38 l
442.74 624.18 l
f
n
446.16 625.2 m
444.96 625.2 l
444.96 626.4 l
447.36 627 l
448.56 627 l
448.56 625.8 l
f
n
452.58 627 m
451.38 627 l
451.38 628.2 l
452.16 628.38 l
453.36 628.38 l
453.36 627.18 l
f
n
453.36 627.18 m
452.16 627.18 l
452.16 628.38 l
453.78 628.8 l
454.98 628.8 l
454.98 627.6 l
f
n
458.94 628.56 m
457.74 628.56 l
457.74 629.76 l
460.14 630.42 l
461.34 630.42 l
461.34 629.22 l
f
n
252 415.62 m
250.8 415.62 l
250.8 416.82 l
256.38 450 l
257.58 450 l
257.58 448.8 l
f
n
257.58 448.8 m
256.38 448.8 l
256.38 450 l
267.96 489.18 l
269.16 489.18 l
269.16 487.98 l
f
n
269.16 487.98 m
267.96 487.98 l
267.96 489.18 l
279.42 515.4 l
280.62 515.4 l
280.62 514.2 l
f
n
280.62 514.2 m
279.42 514.2 l
279.42 515.4 l
291 535.38 l
292.2 535.38 l
292.2 534.18 l
f
n
292.2 534.18 m
291 534.18 l
291 535.38 l
302.4 550.38 l
303.6 550.38 l
303.6 549.18 l
f
n
303.6 549.18 m
302.4 549.18 l
302.4 550.38 l
313.98 562.8 l
315.18 562.8 l
315.18 561.6 l
f
n
315.18 561.6 m
313.98 561.6 l
313.98 562.8 l
325.62 574.2 l
326.82 574.2 l
326.82 573 l
f
n
326.82 573 m
325.62 573 l
325.62 574.2 l
336.96 584.58 l
338.16 584.58 l
338.16 583.38 l
f
n
338.16 583.38 m
336.96 583.38 l
336.96 584.58 l
348.6 593.04 l
349.74 593.04 l
349.74 591.84 l
f
n
349.74 591.84 m
348.6 591.84 l
348.6 593.04 l
360 600.42 l
361.2 600.42 l
361.2 599.22 l
f
n
361.2 599.22 m
360 599.22 l
360 600.42 l
371.58 607.38 l
372.78 607.38 l
372.78 606.18 l
f
n
372.78 606.18 m
371.58 606.18 l
371.58 607.38 l
383.16 613.38 l
384.36 613.38 l
384.36 612.18 l
f
n
384.36 612.18 m
383.16 612.18 l
383.16 613.38 l
394.56 619.2 l
395.76 619.2 l
395.76 618 l
f
n
395.76 618 m
394.56 618 l
394.56 619.2 l
406.2 624 l
407.4 624 l
407.4 622.8 l
f
n
407.4 622.8 m
406.2 622.8 l
406.2 624 l
417.54 628.8 l
418.74 628.8 l
418.74 627.6 l
f
n
418.74 627.6 m
417.54 627.6 l
417.54 628.8 l
429.18 633.36 l
430.38 633.36 l
430.38 632.16 l
f
n
430.38 632.16 m
429.18 632.16 l
429.18 633.36 l
440.76 637.38 l
441.96 637.38 l
441.96 636.18 l
f
n
441.96 636.18 m
440.76 636.18 l
440.76 637.38 l
452.16 641.22 l
453.36 641.22 l
453.36 640.02 l
f
n
453.36 640.02 m
452.16 640.02 l
452.16 641.22 l
463.56 643.98 l
464.76 643.98 l
464.76 642.78 l
f
n
255 415.62 m
253.8 415.62 l
253.8 416.82 l
256.38 427.2 l
257.58 427.2 l
257.58 426 l
f
n
257.58 426 m
256.38 426 l
256.38 427.2 l
267.96 466.8 l
269.16 466.8 l
269.16 465.6 l
f
n
269.16 465.6 m
267.96 465.6 l
267.96 466.8 l
279.42 491.58 l
280.62 491.58 l
280.62 490.38 l
f
n
280.62 490.38 m
279.42 490.38 l
279.42 491.58 l
291 510 l
292.2 510 l
292.2 508.8 l
f
n
292.2 508.8 m
291 508.8 l
291 510 l
302.4 526.02 l
303.6 526.02 l
303.6 524.82 l
f
n
303.6 524.82 m
302.4 524.82 l
302.4 526.02 l
313.98 538.38 l
315.18 538.38 l
315.18 537.18 l
f
n
315.18 537.18 m
313.98 537.18 l
313.98 538.38 l
325.62 549.18 l
326.82 549.18 l
326.82 547.98 l
f
n
326.82 547.98 m
325.62 547.98 l
325.62 549.18 l
336.96 558.96 l
338.16 558.96 l
338.16 557.76 l
f
n
338.16 557.76 m
336.96 557.76 l
336.96 558.96 l
348.6 567.18 l
349.74 567.18 l
349.74 565.98 l
f
n
349.74 565.98 m
348.6 565.98 l
348.6 567.18 l
360 574.98 l
361.2 574.98 l
361.2 573.78 l
f
n
361.2 573.78 m
360 573.78 l
360 574.98 l
371.58 582 l
372.78 582 l
372.78 580.8 l
f
n
372.78 580.8 m
371.58 580.8 l
371.58 582 l
383.16 588 l
384.36 588 l
384.36 586.8 l
f
n
384.36 586.8 m
383.16 586.8 l
383.16 588 l
394.56 594 l
395.76 594 l
395.76 592.8 l
f
n
395.76 592.8 m
394.56 592.8 l
394.56 594 l
406.2 599.22 l
407.4 599.22 l
407.4 598.02 l
f
n
407.4 598.02 m
406.2 598.02 l
406.2 599.22 l
417.54 604.38 l
418.74 604.38 l
418.74 603.18 l
f
n
418.74 603.18 m
417.54 603.18 l
417.54 604.38 l
429.18 609.24 l
430.38 609.24 l
430.38 607.98 l
f
n
430.38 607.98 m
429.18 607.98 l
429.18 609.24 l
440.76 613.38 l
441.96 613.38 l
441.96 612.18 l
f
n
441.96 612.18 m
440.76 612.18 l
440.76 613.38 l
452.16 617.64 l
453.36 617.64 l
453.36 616.44 l
f
n
453.36 616.44 m
452.16 616.44 l
452.16 617.64 l
463.56 620.82 l
464.76 620.82 l
464.76 619.56 l
f
n
183.78 415.62 m
182.58 415.62 l
182.58 416.82 l
183 419.22 l
184.2 419.22 l
184.2 418.02 l
f
n
184.98 421.98 m
183.78 421.98 l
183.78 423.18 l
184.2 425.58 l
185.4 425.58 l
185.4 424.38 l
f
n
186.18 428.4 m
184.98 428.4 l
184.98 429.6 l
185.64 432 l
186.84 432 l
186.84 430.8 l
f
n
187.56 434.76 m
186.36 434.76 l
186.36 435.96 l
186.84 438.36 l
188.04 438.36 l
188.04 437.16 l
f
n
189 441.24 m
187.8 441.24 l
187.8 442.44 l
188.4 444.78 l
189.6 444.78 l
189.6 443.58 l
f
n
190.62 447.6 m
189.42 447.6 l
189.42 448.8 l
189.96 451.2 l
191.16 451.2 l
191.16 450 l
f
n
192.18 454.02 m
190.98 454.02 l
190.98 455.22 l
191.58 457.62 l
192.78 457.62 l
192.78 456.42 l
f
n
193.8 460.38 m
192.6 460.38 l
192.6 461.58 l
193.2 463.98 l
194.4 463.98 l
194.4 462.78 l
f
n
195.42 466.8 m
194.22 466.8 l
194.22 468 l
194.76 470.4 l
195.96 470.4 l
195.96 469.2 l
f
n
196.98 473.16 m
195.78 473.16 l
195.78 474.36 l
196.38 476.76 l
197.58 476.76 l
197.58 475.56 l
f
n
198.6 479.58 m
197.4 479.58 l
197.4 480.78 l
198.18 483.42 l
199.38 483.42 l
199.38 482.22 l
f
n
200.58 486.18 m
199.38 486.18 l
199.38 487.44 l
200.4 489.84 l
201.6 489.84 l
201.6 488.64 l
f
n
203.4 492.42 m
202.2 492.42 l
202.2 493.62 l
203.16 496.02 l
204.36 496.02 l
204.36 494.82 l
f
n
206.16 498.78 m
205.02 498.78 l
205.02 499.98 l
205.98 502.38 l
207.18 502.38 l
207.18 501.18 l
f
n
208.8 505.38 m
207.6 505.38 l
207.6 506.58 l
208.56 508.98 l
209.76 508.98 l
209.76 507.78 l
f
n
211.62 512.04 m
210.42 512.04 l
210.42 513.18 l
211.8 515.4 l
213 515.4 l
213 514.2 l
f
n
215.22 517.98 m
214.02 517.98 l
214.02 519.18 l
215.4 521.76 l
216.6 521.76 l
216.6 520.62 l
f
n
219 524.82 m
217.8 524.82 l
217.8 526.02 l
219.36 528.42 l
220.56 528.42 l
220.56 527.22 l
f
n
222.96 531.36 m
221.76 531.36 l
221.76 532.56 l
223.62 534.78 l
224.82 534.78 l
224.82 533.58 l
f
n
227.76 537.42 m
226.56 537.42 l
226.56 538.62 l
228.42 541.02 l
229.62 541.02 l
229.62 539.82 l
f
n
232.38 543.6 m
231.18 543.6 l
231.18 544.8 l
233.4 547.56 l
234.6 547.56 l
234.6 546.36 l
f
n
238.2 550.2 m
237 550.2 l
237 551.4 l
239.22 553.8 l
240.42 553.8 l
240.42 552.6 l
f
n
244.02 556.38 m
242.82 556.38 l
242.82 557.58 l
244.8 559.98 l
246 559.98 l
246 558.78 l
f
n
249.96 562.38 m
248.76 562.38 l
248.76 563.58 l
251.16 565.8 l
252.36 565.8 l
252.36 564.6 l
f
n
256.38 568.38 m
255.18 568.38 l
255.18 569.58 l
256.38 570.78 l
257.58 570.78 l
257.58 569.58 l
f
n
257.58 569.58 m
256.38 569.58 l
256.38 570.78 l
258 571.98 l
259.2 571.98 l
259.2 570.78 l
f
n
262.98 573.6 m
261.78 573.6 l
261.78 574.8 l
264.18 576.6 l
265.38 576.6 l
265.38 575.4 l
f
n
269.16 578.22 m
267.96 578.22 l
267.96 579.42 l
270.36 580.98 l
271.56 580.98 l
271.56 579.78 l
f
n
275.58 582.6 m
274.38 582.6 l
274.38 583.8 l
277.02 585.6 l
278.22 585.6 l
278.22 584.4 l
f
n
282 586.98 m
280.8 586.98 l
280.8 588.18 l
283.38 589.98 l
284.58 589.98 l
284.58 588.78 l
f
n
288.78 591.6 m
287.58 591.6 l
287.58 592.8 l
290.22 594.42 l
291.42 594.42 l
291.42 593.22 l
f
n
295.2 595.62 m
294 595.62 l
294 596.82 l
296.16 598.2 l
297.36 598.2 l
297.36 597 l
f
n
301.2 599.4 m
300 599.4 l
300 600.6 l
302.4 601.98 l
303.6 601.98 l
303.6 600.78 l
f
n
307.56 603 m
306.36 603 l
306.36 604.2 l
309 605.58 l
310.2 605.58 l
310.2 604.38 l
f
n
314.34 606.78 m
313.14 606.78 l
313.14 607.98 l
313.98 608.4 l
315.18 608.4 l
315.18 607.2 l
f
n
315.18 607.2 m
313.98 607.2 l
313.98 608.4 l
315.54 609.24 l
316.74 609.24 l
316.74 607.98 l
f
n
320.58 609.96 m
319.38 609.96 l
319.38 611.16 l
321.78 612.36 l
322.98 612.36 l
322.98 611.16 l
f
n
326.82 613.02 m
325.62 613.02 l
325.62 614.22 l
328.02 615.24 l
329.22 615.24 l
329.22 614.04 l
f
n
333.18 615.78 m
331.98 615.78 l
331.98 616.98 l
334.56 618.18 l
335.76 618.18 l
335.76 616.98 l
f
n
339.78 618.78 m
338.58 618.78 l
338.58 619.98 l
341.16 621.18 l
342.36 621.18 l
342.36 619.98 l
f
n
346.56 621.78 m
345.36 621.78 l
345.36 622.98 l
347.76 624 l
348.96 624 l
348.96 622.8 l
f
n
352.8 624.6 m
351.6 624.6 l
351.6 625.8 l
353.76 626.82 l
354.96 626.82 l
354.96 625.62 l
f
n
358.8 627.18 m
357.6 627.18 l
357.6 628.38 l
360 629.4 l
361.2 629.4 l
361.2 628.2 l
f
n
365.34 630 m
364.14 630 l
364.14 631.2 l
366.54 632.16 l
367.74 632.16 l
367.74 630.96 l
f
n
372 632.64 m
370.8 632.64 l
370.8 633.84 l
371.58 634.2 l
372.78 634.2 l
372.78 633 l
f
n
372.78 633 m
371.58 633 l
371.58 634.2 l
373.2 634.8 l
374.4 634.8 l
374.4 633.6 l
f
n
378.18 635.04 m
376.98 635.04 l
376.98 636.18 l
379.38 637.2 l
380.58 637.2 l
380.58 636 l
f
n
384.36 637.38 m
383.16 637.38 l
383.16 638.58 l
385.56 639.42 l
386.76 639.42 l
386.76 638.16 l
f
n
390.78 639.42 m
389.58 639.42 l
389.58 640.62 l
392.16 641.4 l
393.36 641.4 l
393.36 640.2 l
f
n
397.38 641.4 m
396.18 641.4 l
396.18 642.6 l
398.76 643.38 l
399.96 643.38 l
399.96 642.18 l
f
n
404.16 643.38 m
402.96 643.38 l
402.96 644.58 l
405.36 645.42 l
406.56 645.42 l
406.56 644.22 l
f
n
409.98 645.24 m
408.78 645.24 l
408.78 646.44 l
411.18 646.98 l
412.38 646.98 l
412.38 645.78 l
f
n
416.34 646.98 m
415.14 646.98 l
415.14 648.18 l
417.54 648.84 l
418.74 648.84 l
418.74 647.64 l
f
n
175.8 604.2 m
175.8 605.4 l
176.94 605.4 l
188.4 590.82 l
188.4 589.62 l
187.2 589.62 l
f
n
187.2 589.62 m
187.2 590.82 l
188.4 590.82 l
199.98 576.36 l
199.98 575.16 l
198.78 575.16 l
f
n
198.78 575.16 m
198.78 576.36 l
199.98 576.36 l
211.62 561.84 l
211.62 560.64 l
210.42 560.64 l
f
n
210.42 560.64 m
210.42 561.84 l
211.62 561.84 l
222.96 547.38 l
222.96 546.18 l
221.76 546.18 l
f
n
221.76 546.18 m
221.76 547.38 l
222.96 547.38 l
234.6 532.8 l
234.6 531.6 l
233.4 531.6 l
f
n
233.4 531.6 m
233.4 532.8 l
234.6 532.8 l
246 518.4 l
246 517.2 l
244.8 517.2 l
f
n
244.8 517.2 m
244.8 518.4 l
246 518.4 l
257.58 503.82 l
257.58 502.62 l
256.38 502.62 l
f
n
256.38 502.62 m
256.38 503.82 l
257.58 503.82 l
269.16 489.36 l
269.16 488.16 l
267.96 488.16 l
f
n
267.96 488.16 m
267.96 489.36 l
269.16 489.36 l
280.62 475.02 l
280.62 473.82 l
279.42 473.82 l
f
n
279.42 473.82 m
279.42 475.02 l
280.62 475.02 l
292.2 460.38 l
292.2 459.18 l
291 459.18 l
f
n
291 459.18 m
291 460.38 l
292.2 460.38 l
303.6 445.98 l
303.6 444.78 l
302.4 444.78 l
f
n
302.4 444.78 m
302.4 445.98 l
303.6 445.98 l
315.18 431.4 l
315.18 430.2 l
313.98 430.2 l
f
n
313.98 430.2 m
313.98 431.4 l
315.18 431.4 l
326.82 417 l
326.82 415.8 l
325.62 415.8 l
f
n
325.62 417 1.20001 -1.38 re
f
1 J
1 j
0.190994 w
10 M
[] 0 d
n
176.4 415.98 m
181.38 415.98 l
176.4 432.6 m
181.38 432.6 l
176.4 449.4 m
181.38 449.4 l
176.4 466.02 m
181.38 466.02 l
176.4 482.58 m
181.38 482.58 l
176.4 499.38 m
181.38 499.38 l
176.4 516 m
181.38 516 l
176.4 532.8 m
181.38 532.8 l
176.4 549.42 m
181.38 549.42 l
176.4 566.16 m
181.38 566.16 l
176.4 582.84 m
181.38 582.84 l
176.4 599.4 m
181.38 599.4 l
176.4 616.2 m
181.38 616.2 l
176.4 632.82 m
181.38 632.82 l
176.4 420.96 m
178.98 420.96 l
176.4 424.02 m
178.98 424.02 l
176.4 426 m
178.98 426 l
176.4 427.62 m
178.98 427.62 l
176.4 429 m
178.98 429 l
176.4 430.02 m
178.98 430.02 l
176.4 430.98 m
178.98 430.98 l
176.4 431.82 m
178.98 431.82 l
176.4 437.64 m
178.98 437.64 l
176.4 440.58 m
178.98 440.58 l
176.4 442.62 m
178.98 442.62 l
176.4 444.18 m
178.98 444.18 l
176.4 445.62 m
178.98 445.62 l
176.4 446.82 m
178.98 446.82 l
176.4 447.78 m
178.98 447.78 l
176.4 448.62 m
178.98 448.62 l
176.4 454.38 m
178.98 454.38 l
176.4 457.44 m
178.98 457.44 l
176.4 459.36 m
178.98 459.36 l
176.4 460.98 m
178.98 460.98 l
176.4 462.42 m
178.98 462.42 l
176.4 463.38 m
178.98 463.38 l
176.4 464.4 m
178.98 464.4 l
176.4 465.18 m
178.98 465.18 l
176.4 471 m
178.98 471 l
176.4 474 m
178.98 474 l
176.4 476.04 m
178.98 476.04 l
176.4 477.6 m
178.98 477.6 l
176.4 478.98 m
178.98 478.98 l
176.4 480.18 m
178.98 480.18 l
176.4 481.02 m
178.98 481.02 l
176.4 481.98 m
178.98 481.98 l
176.4 487.8 m
178.98 487.8 l
176.4 490.56 m
178.98 490.56 l
176.4 492.78 m
178.98 492.78 l
176.4 494.4 m
178.98 494.4 l
176.4 495.78 m
178.98 495.78 l
176.4 496.8 m
178.98 496.8 l
176.4 497.76 m
178.98 497.76 l
176.4 498.6 m
178.98 498.6 l
176.4 504.36 m
178.98 504.36 l
176.4 507.42 m
178.98 507.42 l
176.4 509.4 m
178.98 509.4 l
176.4 511.02 m
178.98 511.02 l
176.4 512.4 m
178.98 512.4 l
176.4 513.6 m
178.98 513.6 l
176.4 514.38 m
178.98 514.38 l
176.4 515.4 m
178.98 515.4 l
176.4 520.98 m
178.98 520.98 l
176.4 523.98 m
178.8 523.98 l
0 0 0.830994 sc
S
n
178.8 523.98 m
178.98 523.98 l
176.4 526.2 m
178.98 526.2 l
176.4 527.76 m
178.98 527.76 l
176.4 528.96 m
178.98 528.96 l
176.4 530.16 m
178.98 530.16 l
176.4 531.18 m
178.98 531.18 l
176.4 532.02 m
178.98 532.02 l
176.4 537.78 m
178.98 537.78 l
176.4 540.84 m
178.98 540.84 l
176.4 542.76 m
178.98 542.76 l
176.4 544.44 m
178.98 544.44 l
176.4 545.82 m
178.98 545.82 l
176.4 546.84 m
178.98 546.84 l
176.4 547.8 m
178.98 547.8 l
176.4 548.58 m
178.98 548.58 l
176.4 554.4 m
178.98 554.4 l
176.4 557.4 m
178.98 557.4 l
176.4 559.44 m
178.98 559.44 l
176.4 561 m
178.98 561 l
176.4 562.38 m
178.98 562.38 l
176.4 563.58 m
178.98 563.58 l
176.4 564.6 m
178.98 564.6 l
176.4 565.38 m
178.98 565.38 l
176.4 571.2 m
178.98 571.2 l
176.4 574.2 m
178.98 574.2 l
176.4 576.18 m
178.98 576.18 l
176.4 577.8 m
178.98 577.8 l
176.4 579.24 m
178.98 579.24 l
176.4 580.2 m
178.98 580.2 l
176.4 581.16 m
178.98 581.16 l
176.4 582 m
178.98 582 l
176.4 587.82 m
178.98 587.82 l
176.4 590.82 m
178.98 590.82 l
176.4 592.8 m
178.98 592.8 l
176.4 594.42 m
178.98 594.42 l
176.4 595.8 m
178.98 595.8 l
176.4 597 m
178.98 597 l
S
n
176.4 597.84 m
178.98 597.84 l
176.4 598.8 m
178.98 598.8 l
176.4 604.62 m
178.98 604.62 l
176.4 607.38 m
178.98 607.38 l
176.4 609.6 m
178.98 609.6 l
176.4 611.16 m
178.98 611.16 l
176.4 612.6 m
178.98 612.6 l
176.4 613.56 m
178.98 613.56 l
176.4 614.58 m
178.98 614.58 l
176.4 615.42 m
178.98 615.42 l
176.4 621.18 m
178.98 621.18 l
176.4 624.18 m
178.98 624.18 l
176.4 626.22 m
178.98 626.22 l
176.4 627.84 m
178.98 627.84 l
176.4 629.22 m
178.98 629.22 l
176.4 630.42 m
178.98 630.42 l
176.4 631.2 m
178.98 631.2 l
176.4 632.16 m
178.98 632.16 l
176.4 637.8 m
178.98 637.8 l
176.4 640.8 m
178.98 640.8 l
176.4 643.02 m
178.98 643.02 l
176.4 644.58 m
178.98 644.58 l
176.4 645.78 m
178.98 645.78 l
176.4 646.98 m
178.98 646.98 l
176.4 648 m
178.98 648 l
176.4 648.84 m
178.98 648.84 l
464.4 415.98 m
459.36 415.98 l
464.4 432.6 m
459.36 432.6 l
464.4 449.4 m
459.36 449.4 l
464.4 466.02 m
459.36 466.02 l
464.4 482.58 m
459.36 482.58 l
464.4 499.38 m
459.36 499.38 l
464.4 516 m
459.36 516 l
464.4 532.8 m
459.36 532.8 l
464.4 549.42 m
459.36 549.42 l
464.4 566.16 m
459.36 566.16 l
464.4 582.84 m
459.36 582.84 l
464.4 599.4 m
459.36 599.4 l
464.4 616.2 m
459.36 616.2 l
464.4 632.82 m
459.36 632.82 l
464.4 420.96 m
461.76 420.96 l
464.4 424.02 m
461.76 424.02 l
464.4 426 m
461.76 426 l
464.4 427.62 m
461.76 427.62 l
464.4 429 m
461.76 429 l
464.4 430.02 m
461.76 430.02 l
464.4 430.98 m
461.76 430.98 l
464.4 431.82 m
461.76 431.82 l
464.4 437.64 m
461.76 437.64 l
464.4 440.58 m
461.76 440.58 l
464.4 442.62 m
461.76 442.62 l
464.4 444.18 m
461.76 444.18 l
464.4 445.62 m
461.76 445.62 l
464.4 446.82 m
461.76 446.82 l
464.4 447.78 m
461.76 447.78 l
464.4 448.62 m
461.76 448.62 l
464.4 454.38 m
461.76 454.38 l
464.4 457.44 m
461.76 457.44 l
464.4 459.36 m
461.76 459.36 l
464.4 460.98 m
461.76 460.98 l
464.4 462.42 m
461.76 462.42 l
464.4 463.38 m
461.76 463.38 l
464.4 464.4 m
461.76 464.4 l
464.4 465.18 m
462 465.18 l
S
n
462 465.18 m
461.76 465.18 l
464.4 471 m
461.76 471 l
464.4 474 m
461.76 474 l
464.4 476.04 m
461.76 476.04 l
464.4 477.6 m
461.76 477.6 l
464.4 478.98 m
461.76 478.98 l
464.4 480.18 m
461.76 480.18 l
464.4 481.02 m
461.76 481.02 l
464.4 481.98 m
461.76 481.98 l
464.4 487.8 m
461.76 487.8 l
464.4 490.56 m
461.76 490.56 l
464.4 492.78 m
461.76 492.78 l
464.4 494.4 m
461.76 494.4 l
464.4 495.78 m
461.76 495.78 l
464.4 496.8 m
461.76 496.8 l
464.4 497.76 m
461.76 497.76 l
464.4 498.6 m
461.76 498.6 l
464.4 504.36 m
461.76 504.36 l
464.4 507.42 m
461.76 507.42 l
464.4 509.4 m
461.76 509.4 l
464.4 511.02 m
461.76 511.02 l
464.4 512.4 m
461.76 512.4 l
464.4 513.6 m
461.76 513.6 l
464.4 514.38 m
461.76 514.38 l
464.4 515.4 m
461.76 515.4 l
464.4 520.98 m
461.76 520.98 l
464.4 523.98 m
461.76 523.98 l
464.4 526.2 m
461.76 526.2 l
464.4 527.76 m
461.76 527.76 l
464.4 528.96 m
461.76 528.96 l
464.4 530.16 m
461.76 530.16 l
464.4 531.18 m
461.76 531.18 l
464.4 532.02 m
461.76 532.02 l
464.4 537.78 m
461.76 537.78 l
464.4 540.84 m
461.76 540.84 l
464.4 542.76 m
461.76 542.76 l
464.4 544.44 m
461.76 544.44 l
S
n
464.4 545.82 m
461.76 545.82 l
464.4 546.84 m
461.76 546.84 l
464.4 547.8 m
461.76 547.8 l
464.4 548.58 m
461.76 548.58 l
464.4 554.4 m
461.76 554.4 l
464.4 557.4 m
461.76 557.4 l
464.4 559.44 m
461.76 559.44 l
464.4 561 m
461.76 561 l
464.4 562.38 m
461.76 562.38 l
464.4 563.58 m
461.76 563.58 l
464.4 564.6 m
461.76 564.6 l
464.4 565.38 m
461.76 565.38 l
464.4 571.2 m
461.76 571.2 l
464.4 574.2 m
461.76 574.2 l
464.4 576.18 m
461.76 576.18 l
464.4 577.8 m
461.76 577.8 l
464.4 579.24 m
461.76 579.24 l
464.4 580.2 m
461.76 580.2 l
464.4 581.16 m
461.76 581.16 l
464.4 582 m
461.76 582 l
464.4 587.82 m
461.76 587.82 l
464.4 590.82 m
461.76 590.82 l
464.4 592.8 m
461.76 592.8 l
464.4 594.42 m
461.76 594.42 l
464.4 595.8 m
461.76 595.8 l
464.4 597 m
461.76 597 l
464.4 597.84 m
461.76 597.84 l
464.4 598.8 m
461.76 598.8 l
464.4 604.62 m
461.76 604.62 l
464.4 607.38 m
461.76 607.38 l
464.4 609.6 m
461.76 609.6 l
464.4 611.16 m
461.76 611.16 l
464.4 612.6 m
461.76 612.6 l
464.4 613.56 m
461.76 613.56 l
464.4 614.58 m
461.76 614.58 l
464.4 615.42 m
461.76 615.42 l
464.4 621.18 m
461.76 621.18 l
464.4 624.18 m
461.76 624.18 l
464.4 626.22 m
461.76 626.22 l
464.4 627.84 m
461.76 627.84 l
464.4 629.22 m
461.76 629.22 l
464.4 630.42 m
461.76 630.42 l
464.4 631.2 m
461.76 631.2 l
464.4 632.16 m
461.76 632.16 l
464.4 637.8 m
461.76 637.8 l
464.4 640.8 m
461.76 640.8 l
464.4 643.02 m
461.76 643.02 l
464.4 644.58 m
461.76 644.58 l
464.4 645.78 m
461.76 645.78 l
464.4 646.98 m
461.76 646.98 l
464.4 648 m
461.76 648 l
464.4 648.84 m
461.76 648.84 l
176.4 415.98 m
176.4 420.96 l
233.94 415.98 m
233.94 420.96 l
291.6 415.98 m
291.6 420.96 l
349.2 415.98 m
349.2 420.96 l
406.74 415.98 m
406.74 420.96 l
464.4 415.98 m
464.4 420.96 l
187.8 415.98 m
187.8 418.56 l
199.38 415.98 m
199.38 418.56 l
210.96 415.98 m
210.96 418.56 l
222.42 415.98 m
222.42 418.56 l
245.4 415.98 m
245.4 418.56 l
256.98 415.98 m
256.98 418.38 l
S
n
256.98 418.38 m
256.98 418.56 l
268.62 415.98 m
268.62 418.56 l
279.96 415.98 m
279.96 418.56 l
303 415.98 m
303 418.56 l
314.58 415.98 m
314.58 418.56 l
326.16 415.98 m
326.16 418.56 l
337.56 415.98 m
337.56 418.56 l
360.54 415.98 m
360.54 418.56 l
372.18 415.98 m
372.18 418.56 l
383.76 415.98 m
383.76 418.56 l
395.16 415.98 m
395.16 418.56 l
418.2 415.98 m
418.2 418.56 l
429.78 415.98 m
429.78 418.56 l
441.36 415.98 m
441.36 418.56 l
452.76 415.98 m
452.76 418.56 l
176.4 649.56 m
176.4 644.58 l
233.94 649.56 m
233.94 644.58 l
291.6 649.56 m
291.6 644.58 l
349.2 649.56 m
349.2 644.58 l
406.74 649.56 m
406.74 644.58 l
464.4 649.56 m
464.4 644.58 l
187.8 649.56 m
187.8 646.98 l
199.38 649.56 m
199.38 646.98 l
210.96 649.56 m
210.96 646.98 l
222.42 649.56 m
222.42 646.98 l
245.4 649.56 m
245.4 646.98 l
256.98 649.56 m
256.98 646.98 l
268.62 649.56 m
268.62 646.98 l
279.96 649.56 m
279.96 646.98 l
303 649.56 m
303 646.98 l
314.58 649.56 m
314.58 646.98 l
326.16 649.56 m
326.16 646.98 l
337.56 649.56 m
337.56 646.98 l
360.54 649.56 m
360.54 646.98 l
372.18 649.56 m
372.18 646.98 l
383.76 649.56 m
383.76 646.98 l
395.16 649.56 m
395.16 646.98 l
S
n
418.2 649.56 m
418.2 646.98 l
429.78 649.56 m
429.78 646.98 l
441.36 649.56 m
441.36 646.98 l
452.76 649.56 m
452.76 646.98 l
S
n
175.98 650.04 0.779999 -234.42 re
f
n
463.92 650.04 0.839996 -234.42 re
f
n
175.98 416.4 288.78 -0.779999 re
f
n
175.98 650.04 288.78 -0.840027 re
f
0 0 0 sc
149.22 412.38 m
/N295 9.58659 Tf
(10)
[5.33877 5.33877 ] pdfxs
160.02 417.36 m
/N295 6.4231 Tf
(-20)
[2.16325 3.59564 3.59564 ] pdfxs
149.22 445.8 m
/N295 9.58659 Tf
(10)
[5.33877 5.33877 ] pdfxs
160.02 450.78 m
/N295 6.4231 Tf
(-18)
[2.16325 3.59564 3.59564 ] pdfxs
149.22 479.16 m
/N295 9.58659 Tf
(10)
[5.33877 5.33877 ] pdfxs
160.02 484.2 m
/N295 6.4231 Tf
(-16)
[2.16325 3.59564 3.59564 ] pdfxs
149.22 512.58 m
/N295 9.58659 Tf
(10)
[5.33877 5.33877 ] pdfxs
160.02 517.62 m
/N295 6.4231 Tf
(-14)
[2.16325 3.59564 3.59564 ] pdfxs
149.22 545.82 m
/N295 9.58659 Tf
(10)
[5.33877 5.33877 ] pdfxs
160.02 550.8 m
/N295 6.4231 Tf
(-12)
[2.16325 3.59564 3.59564 ] pdfxs
149.22 579.24 m
/N295 9.58659 Tf
(10)
[5.33877 5.33877 ] pdfxs
160.02 584.22 m
/N295 6.4231 Tf
(-10)
[2.16325 3.59564 3.59564 ] pdfxs
152.4 612.6 m
/N295 9.58659 Tf
(10)
[5.39816 5.39816 ] pdfxs
163.2 617.64 m
/N295 6.4231 Tf
(-8)
[2.2198 3.65219 ] pdfxs
169.2 403.2 m
/N295 9.58659 Tf
(203040506070)
[5.39818 52.1386 5.45858 52.198 5.33875 52.198 5.45858 52.1386 5.45858 52.198 5.33875 
5.45858 ] pdfxs
0 J
0 j
0.119995 w
139.62 520.02 m
Adobe_CoolType_Utility begin ct_MakeOCF begin ct_GlyphDirProcs begin
/EKJCFC+SymbolMT 1
GetGlyphDirectory
58 <10bf317054a314237da54d77895bd9cf6f1927c0e468faa214c19ffa1184
dccf645339f7b76829527fb1061e34d7f75278bfcd7792b6b9b47e92679d
6a6dea3e1feb8faae1d45340f948412faf1764e08b078f5d08f353975f93
97a36b9fb88b3bf50c52267ca43829befbb0f62dbdd416e380a02203f962
e62972cecbbe171c69e4308bba0cfbfe4b48d4f8b7f08f847847d5b0ebf3
9d305c7ebe69f985704c758e6304d8dd49adcd14a1b8900e0865010ba218
9fc25190a6308b6df0fa18b1377c1d6409> |
!
end end end
/N287 [0 11.2165 -11.2165 0 0 0] Tf
(\000:) show
n
139.62 520.02 m
(\000:) pdf_strokepath
139.62 528.78 m
/N292 [0 11.2165 -11.2165 0 0 0] Tf
(\(E\))
[3.77985 7.38035 3.77985 ] pdfys
317.58 391.98 m
/N292 11.2165 Tf
(E) show
n
329.22 554.4 m
319.8 554.22 l
323.76 556.2 l
321.78 560.16 l
329.22 554.4 l
eofill
1 J
1 j
0.190994 w
n
323.76 556.2 m
240.42 583.98 l
240.18 583.98 l
S
229.14 588.78 m
Adobe_CoolType_Utility begin ct_MakeOCF begin ct_GlyphDirProcs begin
/EKJCFC+SymbolMT 4
GetGlyphDirectory
32 <10bf31706fd83f377bda10399f5cf379a108083b36bf6dc10d6bebb6f4d8
24ebcb90b326f0> |
20 <10bf317005ae401898a54b0ec88c93653a841b7c07218a0a0af06af651c0
73314768784630c60de0cec7076aae8ac05e0ffb3252a32fb505ec42ec45
b10eb1008cff2b494a361061c2d5bbbf1b865befe550661077e7a3907c17
9eaa0e5611f975bc03093225a461c3c44f> |
19 <10bf31705d64a97b17e82783860bae6f0b1855871b61f87b3fbee64b9c80
f2a6b534dfdab6ab9c225754341b7c5624f17521fcf3f24dbd218666011f
77370638323ffa7735f08e5511892e83930a8474c68440f6478a49e9b83b
465322f7cc3720b4d142d2822859c64a9895e7442123698914d3e79d42e0
bf7cc3cdc873f69c5f21def18aa5c0a4f3b2287176900140658919a0a5b9
248e9289a3b38c0c475fa449c76a28bdfc6c61054a9236701993> |
!
end end end
/N287 11.2165 Tf
(\000N\000 \000\024\000\023)
[6.23073 5.99077 5.82031 5.69246 ] pdfxs
n
364.32 604.8 m
354.96 605.4 l
359.34 607.02 l
357.78 611.4 l
364.32 604.8 l
eofill
n
359.34 607.02 m
307.56 630.42 l
307.38 630.42 l
S
288.36 632.82 m
Adobe_CoolType_Utility begin ct_MakeOCF begin ct_GlyphDirProcs begin
/EKJCFC+SymbolMT 3
GetGlyphDirectory
24 <10bf317049845615ceab2cb35844ace30baf4a03459f7f3724855f50c18a
60c2261d41c9fb517ed7a7337438a0f15a384b7fb530f91dee69b979dd2e
dc1d293ac57f6fc13cc0458dc629fe8a62dcae665ed3f5fd731baec61d7c
9cd2f3cf4238a189e87274c8c10d9648748e8e5079ebe1692402e7f881fa
dbf06873128b926aea097e66f89d79636e1f76cc733eee719b559b5e03ce
b3acd9dd20db7961> |
!
end end end
(\000N\000 \000\030)
[6.23073 5.99077 5.69246 ] pdfxs
n
291.6 460.02 m
298.56 466.2 l
296.76 462 l
300.96 460.2 l
291.6 460.02 l
eofill
n
296.76 462 m
321.18 471.24 l
321.36 471.24 l
S
329.94 469.56 m
/N295 11.2165 Tf
(exp\(-E/k)
[6.25212 5.624 6.41813 3.59934 3.75076 7.38042 3.24161 5.624 ] pdfxs
371.82 463.8 m
/N295 7.1899 Tf
(B) show
376.62 469.56 m
/N295 11.2165 Tf
(T\))
[6.72193 3.60374 ] pdfxs
n
313.98 607.2 m
308.58 614.76 l
312.36 612.6 l
314.58 616.44 l
313.98 607.2 l
eofill
n
312.36 612.6 m
307.56 629.58 l
307.38 629.58 l
S
n
273.18 552.78 m
264.54 556.38 l
269.16 556.56 l
268.98 561.18 l
273.18 552.78 l
eofill
n
269.16 556.56 m
240.42 583.2 l
240.18 583.2 l
S
89.9999 344.76 m
/N282 12 Tf
(F) show
(i)
[3.33838 ] pdfxs
(gur) show
(e)
[5.3302 ] pdfxs
( 7, Sh) show
(e)
[5.3302 ] pdfxs
(w ) show
(et)
[5.3302 3.33838 ] pdfxs
( ) show
(al)
[5.3302 3.33838 ] pdfxs
(. ) show
PDFVars/TermAll get exec end end
restore

%%EndDocument

LH
(%%[Page: 7]%%) = 
%%PageTrailer

%%Trailer
%%BoundingBox: 12 13 598 780
%%DocumentNeededResources: 
%%DocumentSuppliedResources: 
%%+ procset Pscript_WinNT_ErrorHandler 5.0 0
%%+ procset Pscript_WinNT_Min 5.0 0
%%+ procset Pscript_Win_Basic 5.0 0
%%+ procset Pscript_Win_Utils_L2 5.0 0
Pscript_WinNT_Min dup /min_terminate get exec
%%EOF
%-12345X@PJL EOJ
%-12345X
